Tailored Hotspots from Airy-Based Surface Plasmon Polaritons

Surface plasmons have attracted growing interest from the photonics community due to their inherent ability to controllably confine light below the diffraction limit and their direct application in trapping and transporting matter at the nanoscale. This method, known as plasmonic tweezers, employs confined fields generated by either localized plasmons or surface plasmon polaritons (SPP), which originate in the vicinity of nanostructure-based traps or across structureless platforms, respectively. Herein, we present a new theoretical method for generating intense light hotspots and engineering their features by overlapping Airy SPPs (ASPP) at a smooth dielectric-metal interface. We coherently add pairs of Hermite-Gauss modes that belong to a novel complete basis set of finite-energy ASPPs, which yield highly confined plasmonic hotspots ($\approx \lambda$/10) without the need of using any nanostructured platform. Mode order and relative spacing parameters can be used to tailor the intensity and quality factor of said hotspots, largely outperforming their Gaussian-only-based counterparts. Our method opens a promising venue to confine light at the nanoscale using ASPP-based structured light, which helps to advance the development of structureless plasmonic tweezers and holds promising potential for its application in optical signal processing and plasmonic circuitry.

==> references.tex <==

@article{camden2008controlled,
  title={Controlled plasmonic nanostructures for surface-enhanced spectroscopy and sensing},
  author={Camden, Jon P and Dieringer, Jon A and Zhao, Jing and Van Duyne, Richard P},
  journal={Acc. of Chem. Res.},
  volume={41},
  number={12},
  pages={1653--1661},
  year={2008},
  publisher={ACS Publications}
}

@article{jahn2016plasmonic,
  title={Plasmonic nanostructures for surface enhanced spectroscopic methods},
  author={Jahn, Martin and Patze, Sophie and Hidi, Izabella J and Knipper, Richard and Radu, Andreea I and M{\"u}hlig, Anna and Y{\"u}ksel, Sezin and Peksa, Vlastimil and Weber, Karina and Mayerh{\"o}fer, Thomas and others},
  journal={Analyst},
  volume={141},
  number={3},
  pages={756--793},
  year={2016},
  publisher={Royal Society of Chemistry}
}


%Plasmonic biosensing

@article{mejia2018plasmonic,
  title={Plasmonic biosensing: Focus review},
  author={Mej{\'\i}a-Salazar, JR and Oliveira Jr, Osvaldo N},
  journal={Chem. Rev.},
  volume={118},
  number={20},
  pages={10617--10625},
  year={2018},
  publisher={ACS Publications}
}

@article{rodrigo2015mid,
  title={Mid-infrared plasmonic biosensing with graphene},
  author={Rodrigo, Daniel and Limaj, Odeta and Janner, Davide and Etezadi, Dordaneh and Garc{\'\i}a de Abajo, F Javier and Pruneri, Valerio and Altug, Hatice},
  journal={Science},
  volume={349},
  number={6244},
  pages={165--168},
  year={2015},
  publisher={American Association for the Advancement of Science}
}

@article{brolo2012plasmonics,
  title={Plasmonics for future biosensors},
  author={Brolo, Alexandre G},
  journal={Nat. Photonics},
  volume={6},
  number={11},
  pages={709--713},
  year={2012},
  publisher={Nature Publishing Group UK London}
}


% Near-field microscopy   near-field scanning optical microscopes

@article{rotenberg2014mapping,
  title={Mapping nanoscale light fields},
  author={Rotenberg, N and Kuipers, L},
  journal={Nat. Photonics},
  volume={8},
  number={12},
  pages={919--926},
  year={2014},
  publisher={Nature Publishing Group UK London}
}

@article{zayats2005nano,
  title={Nano-optics of surface plasmon polaritons},
  author={Zayats, Anatoly V and Smolyaninov, Igor I and Maradudin, Alexei A},
  journal={Phys. Rep.},
  volume={408},
  number={3-4},
  pages={131--314},
  year={2005},
  publisher={Elsevier}
}


@article{minovich2011generation,
  title={Generation and near-field imaging of {Airy}  surface plasmons},
  author={Minovich, Alexander and Klein, Angela E and Janunts, Norik and Pertsch, Thomas and Neshev, Dragomir N and Kivshar, Yuri S},
  journal={Phys. Rev. Lett.},
  volume={107},
  number={11},
  pages={116802},
  year={2011},
  publisher={APS}
}


%Manipulation of light


@article{gong2018nanoscale,
  title={Nanoscale chiral valley-photon interface through optical spin-orbit coupling},
  author={Gong, Su-Hyun and Alpeggiani, Filippo and Sciacca, Beniamino and Garnett, Erik C and Kuipers, L},
  journal={Science},
  volume={359},
  number={6374},
  pages={443--447},
  year={2018},
  publisher={American Association for the Advancement of Science}
}


@article{bliokh2017optical,
  title={Optical momentum and angular momentum in complex media: from the {Abraham--Minkowski} debate to unusual properties of surface plasmon-polaritons},
  author={Bliokh, Konstantin Y and Bekshaev, Aleksandr Y and Nori, Franco},
  journal={New J. of Phys.},
  volume={19},
  number={12},
  pages={123014},
  year={2017},
  publisher={IOP Publishing}
}

@article{miroshnichenko2013polarization,
  title={Polarization traffic control for surface plasmons},
  author={Miroshnichenko, Andrey E and Kivshar, Yuri S},
  journal={Science},
  volume={340},
  number={6130},
  pages={283--284},
  year={2013},
  publisher={American Association for the Advancement of Science}
}



@article{puerto2016femtosecond,
  title={Femtosecond laser-controlled self-assembly of amorphous-crystalline nanogratings in silicon},
  author={Puerto, Daniel and Garcia-Lechuga, Mario and Hernandez-Rueda, Javier and Garcia-Leis, Adianez and Sanchez-Cortes, Santiago and Solis, Javier and Siegel, Jan},
  journal={Nanotechnology},
  volume={27},
  number={26},
  pages={265602},
  year={2016},
  publisher={IOP Publishing}
}

@article{noordam2020plasmon,
  title={Plasmon-induced enhancement of nonlinear optical processes in a double-resonant metallic nanostructure grating},
  author={Noordam, ML and Hernandez-Rueda, J and Talsma, LY and Kuipers, L},
  journal={Appl. Phys. Lett.},
  volume={116},
  number={10},
  year={2020},
  publisher={AIP Publishing}
}


@article{hernandez2024engineering,
  title={Engineering of self-bending surface plasmon polaritons through {Hermite-Gaussian} mode expansion},
  author={Hernandez-Rueda, J. and Sanz, A. S. and Mart{\'\i}nez-Herrero, R},
  journal={arXiv preprint arXiv:2412.08706},
  year={2024}
}



@article{kocsis:Science:2011,
 author  = {S. Kocsis and B. Braverman and S. Ravets and M. J. Stevens and R. P. Mirin and L. K. Shalm and A. M. Steinberg},
 journal = {Science},
 title   = {Observing the average trajectories of single photons in a two-slit interferometer},
 volume  = {332},
 pages   = {1170-1173},
 year    = {2011},
 doi     = {10.1126/science.1202218},
}

@article{coalson:JLightTech:1994,
 author               = {R. D. Coalson and D. K. Pant and A. Ali and D. W. Langer},
 journal              = {J. Light. Tech.},
 pages                = {1015-1022},
 title                = {Computing the eigenmodes of lossy field-induced optical waveguides},
 volume               = {12},
 year                 = {1994},
}

@article{kotsifaki2024hybrid,
  title={Hybrid Metamaterial Optical Tweezers for Dielectric Particles and Biomolecules Discrimination},
  author={Kotsifaki, Domna G and Truong, Viet Giang and Dindo, Mirco and Laurino, Paola and Chormaic, Sile Nic},
  journal={arXiv preprint arXiv:2402.12878},
  year={2024}
}

@article{kotsifaki2021dynamic,
  title={Dynamic multiple nanoparticle trapping using metamaterial plasmonic tweezers},
  author={Kotsifaki, Domna G and Truong, Viet Giang and Nic Chormaic, S{\'\i}le},
  journal={Appl. Phys. Lett.},
  volume={118},
  number={2},
  year={2021},
  publisher={AIP Publishing}
}

@article{kotsifaki2020fano,
  title={Fano-resonant, asymmetric, metamaterial-assisted tweezers for single nanoparticle trapping},
  author={Kotsifaki, Domna G and Truong, Viet Giang and Chormaic, S{\'\i}le Nic},
  journal={Nano Lett.},
  volume={20},
  number={5},
  pages={3388--3395},
  year={2020},
  publisher={ACS Publications}
}

@article{herrmann:AJP:2002,
 author               = {T. W\"unscher and H. Hauptmann and F. Herrmann},
 journal              = {Am. J. Phys.},
 pages                = {599-606},
 title                = {Which way does the light go?},
 volume               = {70},
 year                 = {2002},
}

@article{jcm:wg-lanz:03,
 author               = {J. Campos-Mart{\'\i}nez and Rob D. Coalson},
 journal              = {Appl. Opt.},
 journal-iso          = {Appl. Optics},
 keywords-plus        = {OPTICAL WAVE-GUIDES; SCHRODINGER-EQUATION; PROPAGATION; DESIGN},
 language             = {English},
 month                = {MAR 20},
 number               = {9},
 number-of-cited-refe = {20},
 pages                = {1732-1742},
 publisher            = {OPTICAL SOC AMER},
 subject-category     = {Optics},
 times-cited          = {0},
 title                = {The wide-angle equation and its solution through the short-time iterative Lanczos method},
 type                 = {Article},
 unique-id            = {ISI:000181708400020},
 volume               = {42},
 year                 = {2003},
}

@article{mataloni:PRL:2010,
 author               = {L. Sansoni and F. Sciarrino and G. Vallone and P. Mataloni and A. Crespi and R. Ramponi and R. Osellame},
 journal              = {Phys. Rev. Lett.},
 pages                = {200503(1-4)},
 title                = {Polarization entangled state measurement on a chip},
 volume               = {105},
 year                 = {2010},
}

@article{pepe:AppOpt:1999,
 author               = {D. K. Pant and R. D. Coalson and M. I. Hern{\'a}ndez and J. Campos-Mart{\'\i}nez},
 journal              = {Appl. Opt.},
 pages                = {3917-3923},
 title                = {Optimal control theory for optical waveguide design: Application to $Y$-branch structures},
 volume               = {38},
 year                 = {1999},
}

@article{pepe:AppOpt:2003,
 author               = {J. Campos-Mart{\'\i}nez and R. D. Coalson},
 journal              = {Appl. Opt.},
 pages                = {1732-1742},
 title                = {The wide-angle equation and its solution through the short-time iterative Lanczos method},
 volume               = {42},
 year                 = {2003},
}

@article{pepe:JLightTech:1998,
 author               = {D. K. Pant and R. D. Coalson and M. I. Hern{\'a}ndez and J. Campos-Mart{\'\i}nez},
 journal              = {J. Light. Tech.},
 pages                = {292-300},
 title                = {Optimal control theory for the design of optical waveguides},
 volume               = {16},
 year                 = {1998},
}

@article{politi:science:2008,
 author               = {A. Politi and M. J. Cryan and J. G. Rarity and S. Yu and J. L. O'Brien},
 journal              = {Science},
 pages                = {646-649},
 title                = {Silica-on-silicon waveguide quantum circuits},
 volume               = {320},
 year                 = {2008},
}

@article{sanz:AnnPhysPhoton:2010,
 author               = {A. S. Sanz and M. Davidovi\'c and M. Bo\v{z}i\'c and S. Miret-Art\'es},
 journal              = {Ann. Phys.},
 pages                = {763-784},
 title                = {Understanding interference experiments with polarized light through photon trajectories},
 volume               = {325},
 year                 = {2010},
 doi                  = {10.1016/j.aop.2009.12.005},
 url                  = {https://doi.org/10.1016/j.aop.2009.12.005},
}

@article{sanz:JCP-Talbot:2007,
 author               = {A. S. Sanz and S. Miret-Art\'es},
 journal              = {J. Chem. Phys.},
 pages                = {234106(1-11)},
 title                = {A causal look into the quantum {talbot} effect},
 volume               = {126},
 year                 = {2007},
 doi                  = {10.1063/1.2741555},
}

@article{sanz:JPA:2008,
	doi = {10.1088/1751-8113/41/43/435303},
	url = {https://doi.org/10.1088/1751-8113/41/43/435303},
	year = {2008},
	month = {sep},
	publisher = {{IOP} Publishing},
	volume = {41},
	number = {43},
	pages = {435303},
	author = {A S Sanz and S Miret-Art{\'{e}}s},
	title = {A trajectory-based understanding of quantum interference},
	journal = {J. Phys. A: Math. Theor.}
}

@article{sanz:JRLR:2010,
 author               = {M. Bo\v{z}i\'c and M. Davidovi\'c and T. L. Dimitrova and S. Miret-Art\'es and A. S. Sanz and A. Weis},
 journal              = {J. Russ. Laser Res.},
 pages                = {117-128},
 title                = {Generalized Arago-Fresnel laws: The EME-flow-line description},
 volume               = {31},
 year                 = {2010},
}

@article{sanz:PhysScrPhoton:2009,
 author               = {M. Davidovi\'c and A. S. Sanz and D. Arsenovi\'c and M. Bo\v{z}i\'c and S. Miret-Art\'es},
 journal              = {Phys. Scr.},
 pages                = {014009(1-5)},
 title                = {Electromagnetic energy flow lines as possible paths of photons},
 volume               = {T135},
 year                 = {2009},
}

@article{parker:AJP:1971,
 author               = {S. Parker},
 journal              = {Am. J. Phys.},
 pages                = {420-424},
 title                = {A single-photon double-slit interference experiment},
 volume               = {39},
 year                 = {1971},
}

@article{parker:AJP:1972,
 author               = {S. Parker},
 journal              = {Am. J. Phys.},
 pages                = {1003-1007},
 title                = {Single-photon double-slit interference -- A demonstration},
 volume               = {49},
 year                 = {1972},
}

@article{rueckner:AJP:1996,
 author               = {W. Rueckner and P. Titcomb},
 journal              = {Am. J. Phys.},
 pages                = {184-188},
 title                = {A lecture demonstration of single photon interference},
 volume               = {64},
 year                 = {1996},
}

@article{weis:AJP:2008,
 author               = {T. L. Dimitrova and A. Weis},
 journal              = {Am. J. Phys.},
 pages                = {137-142},
 title                = {The wave-particle duality of light: A demonstration experiment},
 volume               = {76},
 year                 = {2008},
}

@article{weis:EJP:2010,
 author               = {T. L. Dimitrova and A. Weis},
 journal              = {Eur. J. Phys.},
 pages                = {625-637},
 title                = {Single photon quantum erasing: A demonstration experiment},
 volume               = {31},
 year                 = {2010},
}

@article{weis:PhysScr:2009,
 author               = {T. L. Dimitrova and A. Weis},
 journal              = {Phys. Scr.},
 pages                = {014003(1-4)},
 title                = {Lecture demonstrations of interference and quantum erasing with single photons},
 volume               = {T135},
 year                 = {2009},
}

@article{xiang:naturecomm:2011,
 author               = {J. S. Volker and Y. Ziliang and F. Rupert and W. Yuan and B. Guy and Y. Xiaobo and Z. Xiang},
 journal              = {Nat. Commun.},
 pages                = {331(1-5)},
 title                = {Experimental demonstration of low-loss optical waveguiding at deep sub-wavelength scales},
 volume               = {2},
 year                 = {2011},
}

@article{banerjee-josaa:89,
 author   = {S. Banerjee and A. Sharma},
 journal  = {J. Opt. Soc. Am. A},
 pages    = {1884-1894},
 title    = {Propagation characteristic of optical waveguiding structures by direct solution of the Helmholtz equation for total fields},
 volume   = {6},
 year     = {1989},
}

@article{scarmozzino-rev:00,
 author    = {R. Scarmozzino and A. Gopinath and R. Pregla and S. Herlfert },
 journal   = {J. Opt. Soc. Am. A},
 pages     = {150-162},
 title     = {Numerical techniques for modeling guided-wave photonic devices},
 volume    = {6},
 year      = {2000},
}

@article{min-fiber:97,
 author    = {D.-S. Min and D. W. Langer and D. K. Pant and R. D. Coalson},
 journal   = {Fiber Integr. Opt.},
 pages     = {331-342},
 title     = {Numerical techniques for modeling guided-wave photonic devices},
 volume    = {16},
 year      = {1997},
}

@article{feit-fleck:JCompPhys:1982,
 author    = {M. D. Feit and J. A. Fleck, Jr. and A. Steiger},
 journal   = {J. Comput. Phys.},
 title     = {Solution of the Schr\"odinger equation by a spectral method},
 volume = {47},
 number = {3},
 pages = {412-433},
 year = {1982},
 issn = {0021-9991},
 doi = {https://doi.org/10.1016/0021-9991(82)90091-2},
 url = {https://www.sciencedirect.com/science/article/pii/0021999182900912}
}

@article{feit-fleck:JCP:1983,
 author    = {M. D. Feit and J. A. Fleck, Jr.},
 journal   = {J. Chem. Phys.},
 volume    = {78},
 title     = {Solution of the Schr\"odinger equation by a spectral method II: Vibrational energy levels of triatomic molecules},
 pages     = {301-308},
 year      = {1983},
}

@article{feit-fleck:JCP:1984,
 author    = {M. D. Feit and J. A. Fleck, Jr.},
 journal   = {J. Chem. Phys.},
 volume    = {80},
 title     = {Wave packet dynamics and chaos in the H\'enon-Heiles system},
 pages     = {2578-2584},
 year      = {1984},
}

@article{feit-fleck:ApplOpt:1978,
 author    = {M. D. Feit and J. A. Fleck, Jr.},
 journal   = {Appl. Opt.},
 number = {24},
 pages = {3990--3998},
 publisher = {Optica Publishing Group},
 title = {Light propagation in graded-index optical fibers},
 volume = {17},
 month = {Dec},
 year = {1978},
 url = {https://opg.optica.org/ao/abstract.cfm?URI=ao-17-24-3990},
 doi = {10.1364/AO.17.003990}
}

@article{feit-fleck:ApplOpt:1980-1,
 author    = {M. D. Feit and J. A. Fleck, Jr.},
 journal   = {Appl. Opt.},
 number = {7},
 pages = {1154--1164},
 publisher = {Optica Publishing Group},
 title = {Computation of mode properties in optical fiber waveguides by a propagating beam method},
 volume = {19},
 month = {Apr},
 year = {1980},
 url = {https://opg.optica.org/ao/abstract.cfm?URI=ao-19-7-1154},
 doi = {10.1364/AO.19.001154}
}

@article{feit-fleck:ApplOpt:1980-2,
 author    = {M. D. Feit and J. A. Fleck, Jr.},
 journal   = {Appl. Opt.},
 volume    = {19},
 title     = {Computation of mode eigenfunctions in graded-index optical fibers by the propagating beam method},
 pages     = {2240-2246},
 year      = {1980},
}

@article{feit-fleck:ApplOpt:1980-3,
 author    = {M. D. Feit and J. A. Fleck, Jr.},
 journal   = {Appl. Opt.},
 volume    = {19},
 title     = {Model properties and dispersion for two optical fiber-index profiles by the propagating beam method},
 pages     = {3140-3150},
 year      = {1980},
}

@BOOK{bornwolf-bk,
  AUTHOR =       {M. Born and E. Wolf},
  TITLE =        {Principles of Optics. Electromagnetic Theory of Propagation, Interference and Diffraction of Light},
  PUBLISHER =    {Cambridge University Press},
  YEAR =         {1999},
  address =      {Cambridge},
  edition =      {7th},
}

@BOOK{buchdahl-bk,
  AUTHOR =       {H. A. Buchdahl},
  TITLE =        {An Introduction to Hamiltonian Optics},
  PUBLISHER =    {Cambridge University Press},
  YEAR =         {1970},
  address =      {Cambridge},
}

@BOOK{buchdahl-bk-old,
  AUTHOR =       {H. A. Buchdahl},
  TITLE =        {An Introduction to Hamiltonian Optics},
  PUBLISHER =    {Dover},
  YEAR =         {1993},
  address =      {New York},
}

@article{glogel:JOSA:1969,
 author    = {D. Gloge and D. Marcuse},
 journal   = {J. Opt. Soc. Am.},
 title     = {Formal quantum theory of light rays},
 volume    = {59},
 pages     = {1629-1631},
 year      = {1969},
}

@article{kahn:JOSA:1983,
 author    = {W. K. Kahn and S. Yang},
 journal   = {J. Opt. Soc. Am.},
 title     = {Hamiltonian analysis of beams in an optical slab guide},
 volume    = {73},
 pages     = {684-690},
 year      = {1983},
}

@article{longhi:PRE:2003,
 author    = {S. Longhi and D. Janner and M. Marano and P. Laporta},
 journal   = {Phys. Rev. E},
 title     = {Quantum-mechanical analogy of beam propagation in waveguides with a bent axis: Dynamic-model stabilization and radiation-loss suppresion},
 volume    = {67},
 pages     = {036601(1-9)},
 year      = {2003},
}

@article{bohm:PR:1952-1,
  title = {A Suggested Interpretation of the Quantum Theory in Terms of ``Hidden'' Variables. I},
  author = {Bohm, David},
  journal = {Phys. Rev.},
  volume = {85},
  issue = {2},
  pages = {166--179},
  numpages = {0},
  year = {1952},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.85.166},
  url = {https://link.aps.org/doi/10.1103/PhysRev.85.166}
}

@article{bohm:PR:1952-2,
  title = {A Suggested Interpretation of the Quantum Theory in Terms of ``Hidden'' Variables. II},
  author = {Bohm, David},
  journal = {Phys. Rev.},
  volume = {85},
  issue = {2},
  pages = {180--193},
  numpages = {0},
  year = {1952},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.85.180},
  url = {https://link.aps.org/doi/10.1103/PhysRev.85.180}
}

@BOOK{holland-bk,
  AUTHOR =       {P. R. Holland},
  TITLE =        {The Quantum Theory of Motion},
  PUBLISHER =    {Cambridge University Press},
  YEAR =         {1993},
  address =      {Cambridge},
}

@article{madelung:ZPhys:1926,
 author    = {E. Madelung},
 journal   = {Z. Phys.},
 title     = {Quantentheorie in hydrodynamischer Form},
 volume    = {40},
 issue     = {3},
 pages     = {322--326},
 year      = {1926},
 doi = {https://doi.org/10.1007/BF01400372},
 url = {https://link.springer.com/article/10.1007/BF01400372},
}

@article{birula:PRD:1971,
 author    = {I. Bialynicki-Birula and Z. Bialynicka-Birula},
 journal   = {Phys. Rev. D},
 title     = {Magnetic monopoles in the hydrodynamic formulation of quantum mechanics},
 volume    = {3},
 pages     = {2410-2412},
 year      = {1971},
}

@BOOK{birula-bk,
  AUTHOR     = {I. Bialynicki-Birula and M. Cieplak and J. Kaminski},
  TITLE      = {Theory of Quanta},
  PUBLISHER  = {Oxford University Press},
  YEAR       = {1992},
  address    = {Oxford},
}

@article{hirsch:JCP:1974-1,
 author    = {J. O. Hirschfelder and A. C. Christoph and W. E. Palke},
 journal   = {J. Chem. Phys.},
 title     = {Quantum mechanical streamlines. I. Square potential barrier},
 volume    = {61},
 pages     = {5435-5455},
 year      = {1974},
}

@article{hirsch:JCP:1974-2,
 author    = {J. O. Hirschfelder and C. J. Goebel and L. W. Bruch},
 journal   = {J. Chem. Phys.},
 title     = {Quantized vortices around wavefunction nodes. II},
 volume    = {61},
 pages     = {5456-5459},
 year      = {1974},
}

@article{hirsch:JCP:1976-1,
 author    = {J. O. Hirschfelder and K. T. Tang},
 journal   = {J. Chem. Phys.},
 title     = {Quantum mechanical streamlines. III. Idealized reactive atom-diatomic molecule collision},
 volume    = {64},
 pages     = {760-785},
 year      = {1976},
}

@article{hirsch:JCP:1976-2,
 author    = {J. O. Hirschfelder and K. T. Tang},
 journal   = {J. Chem. Phys.},
 title     = {Quantum mechanical streamlines. IV. Collision of two sphere with square potential wells or barriers},
 volume    = {65},
 pages     = {470-486},
 year      = {1976},
}

@article{hirsch:JCP:1977,
 author    = {J. O. Hirschfelder},
 journal   = {J. Chem. Phys.},
 title     = {The angular momentum, creation, and significance of quantized vortices},
 volume    = {67},
 pages     = {5477-5483},
 year      = {1977},
}

@BOOK{wyatt-bk,
  AUTHOR     = {R. E. Wyatt},
  TITLE      = {Quantum Dynamics with Trajectories},
  PUBLISHER  = {Springer},
  YEAR       = {2005},
  address    = {New York},
}

@BOOK{duerr-bk:2009,
  AUTHOR     = {D. D\"urr and S. Teufel},
  TITLE      = {Bohmian Mechanics. The Physics and Mathematics of Quantum Theory},
  PUBLISHER  = {Springer},
  YEAR       = {2009},
  address    = {Berlin},
}

@BOOK{duerr-bk:2013,
  AUTHOR     = {D. D\"urr and S. Goldstein and N. Zangh\`{\i}},
  TITLE      = {Quantum Physics without Quantum Philosophy},
  PUBLISHER  = {Springer},
  YEAR       = {2013},
  address    = {Berlin},
}

@BOOK{press-bk-1,
  AUTHOR     = {W. H. Press and S. A. Teukolsky and W. T. Vetterling and B. P. Flannery},
  TITLE      = {Numerical Recipes in Fortran 77: The Art of Scientific Computing},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {1992},
  address    = {Cambridge},
  volume     = {1st},
  edition    = {2nd},
}

@BOOK{press-bk-2,
  AUTHOR     = {W. H. Press and s. A. Teukolsky and W. T. Vetterling and B. P. Flannery},
  TITLE      = {Numerical Recipes in Fortran 90: The Art of Parallel Scientific Computing},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {1996},
  address    = {Cambridge},
  volume     = {2nd},
  edition    = {2nd},
}

@article{sanz:JPCM:2002,
 author    = {A. S. Sanz and F. Borondo and S. Miret-Art\'es},
 journal   = {J. Phys.: Condens. Matter},
 title     = {Particle diffraction studied using quantum trajectories},
 volume    = {14},
 pages     = {6109-6145},
 year      = {2002},
 doi       = {10.1088/0953-8984/14/24/312},
}

@article{sanz:CP:2011,
 author    = {A. S. Sanz and D. L\'opez-Dur\'an and T. Gonz\'alez-Lezana},
 journal   = {Chem. Phys.},
 title     = {Investigating transition state resonances in the time domain by means of Bohmian mechanics: The F+HD reaction},
 volume    = {399},
 pages     = {151-161},
 year      = {2012},
}

@article{tien:RMP:1977,
 author    = {P. K. Tien},
 journal   = {Rev. Mod. Phys.},
 title     = {Integrated optics and new wave phenomena in optical waveguides},
 volume    = {49},
 pages     = {361-420},
 year      = {1981},
}

@article{tien:radiosci:1981,
 author    = {P. K. Tien},
 journal   = {Radio Sci.},
 title     = {Rules of refractive index and a potential well model of the optical waveguides},
 volume    = {16},
 pages     = {437-444},
 year      = {1981},
}

@article{leforestier:jcompphys:1991,
 author    = {C. Leforestier and R. H. Bisseling and C. Cerjan and M. D. Feit and R. Friesner
 and A. Guldberg and A. Hammerich and G. Jolicard and W. Karrlein and H.-D. Meyer and N. Lipkin
 and O. Roncero and R. Kosloff},
 journal   = {J. Comp. Phys.},
 title     = {A comparison of different propagation schemes for the time dependent schr\"odinger equation},
 volume    = {94},
 pages     = {59-80},
 year      = {1991},
}

@book{zurek-bk,
  author     = {W. H. Zurek and J. A. Wheeler},
  title      = {Quantum Theory of Measurement},
  publisher  = {Princeton University Press},
  year       = {1983},
  address    = {Princeton, NJ},
}

@book{belinfante-bk,
  author     = {F. J. Belinfante},
  title      = {A Survey of Hidden-Variables Theories},
  publisher  = {Pergamon},
  year       = {1973},
  address    = {New York},
}

@book{tarozzi-bk,
  author     = {},
  editor     = {G. Tarozzi and A. van der Merwe},
  title      = {Open Questions in Quantum Physics},
  publisher  = {Reidel},
  year       = {1985},
  address    = {Dordrecht},
}

@book{ballentine-bk,
  author     = {L. E. Ballentine},
  title      = {Quantum Mechanics. A Modern Development},
  publisher  = {World Scientific},
  year       = {1998},
  address    = {Singapore},
}

@article{bell:physics:1964,
 author    = {J. S. Bell},
 journal   = {Physics},
 title     = {On the Einstein-Podolsky-Rosen Paradox},
 volume    = {1},
 pages     = {195-200},
 year      = {1964},
}

@article{bell:RMP:1966,
 author    = {J. S. Bell},
 journal   = {Rev. Mod. Phys.},
 title     = {On the problem of hidden variables in quantum mechanics},
 volume    = {38},
 pages     = {447-452},
 year      = {1966},
}

@article{aspect:PRL:1981,
 author    = {A. Aspect and P. Grangier and G. Roger},
 journal   = {Phys. Rev. Lett.},
 title     = {Experimental tests of realistic local theories via Bell's theorem},
 volume    = {47},
 pages     = {460-463},
 year      = {1981},
}

@article{aspect:PRL:1982-1,
 author    = {A. Aspect and P. Grangier and G. Roger},
 journal   = {Phys. Rev. Lett.},
 title     = {Experimental realization of Einstein-Podolsky-Rosen-Bohm gedankenexperiment: A new violation of Bell's inequalities},
 volume    = {49},
 pages     = {91-94},
 year      = {1982},
}

@article{aspect:PRL:1982-2,
 author    = {A. Aspect and J. Dalibard and G. Roger},
 journal   = {Phys. Rev. Lett.},
 title     = {Experimental test of Bell's inequalities using time-varying analyzers},
 volume    = {49},
 pages     = {1804-1807},
 year      = {1982},
}

@article{goldstein:phystoday:1,
 author    = {S. Goldstein},
 journal   = {Phys. Today},
 title     = {Quantum theory without observers. Part I},
 volume    = {51},
 issue     = {3},
 pages     = {42-46},
 year      = {1998},
}

@article{goldstein:phystoday:2,
 author    = {S. Goldstein},
 journal   = {Phys. Today},
 title     = {Quantum theory without observers. Part II},
 volume    = {51},
 issue     = {4},
 pages     = {38-42},
 year      = {1998},
}

@book{chattaraj-bk,
  editor     = {P. K. Chattaraj},
  title      = {Quantum Trajectories},
  publisher  = {CRC Taylor and Francis},
  year       = {2010},
  address    = {New York},
}

@BOOK{sanz:CRC:2010,
  AUTHOR     = {A. S. Sanz and X. Gim\'enez and J. M. Bofill and S. Miret-Art\'es},
  editor     = {P. K. Chattaraj},
  title      = {Quantum Trajectories},
  CHAPTER    = {Time-dependent density functional theory from a Bohmian perspective},
  pages      = {105-119},
  publisher  = {CRC Taylor and Francis},
  year       = {2010},
  address    = {New York},
}

@book{oriols-bk,
  editor     = {X. Oriols and J. Mompart},
  title      = {Applied Bohmian Mechanics: From Nanoscale Systems to Cosmology},
  publisher  = {Pan Standford Publishing},
  year       = {2012},
  address    = {Singapore},
}

@BOOK{sanz:PanStanford:2012,
  AUTHOR     = {A. S. Sanz and S. Miret-Art\'es},
  editor     = {X. Oriols and J. Mompart},
  title      = {Applied Bohmian Mechanics: From Nanoscale Systems to Cosmology},
  CHAPTER    = {The role of trajectories in quantum chemistry and chemical physics},
  pages      = {235-301},
  publisher  = {Pan Standford Publishing},
  year       = {2012},
  address    = {Singapore},
}

@article{wyatt:prl:1999,
 author    = {C. L. Lopreore and R. E. Wyatt},
 journal   = {Phys. Rev. Lett.},
 title     = {Quantum wave packet dynamics with trajectories},
 volume    = {82},
 pages     = {5190-5193},
 year      = {1999},
}

@article{wyatt:cpl:1999,
 author    = {C. L. Lopreore and R. E. Wyatt},
 journal   = {Chem. Phys. Lett.},
 title     = {Quantum wave packet dynamics with trajectories: reflections on a downhill ramp potential},
 volume    = {325},
 pages     = {73-78},
 year      = {2000},
}

@article{sanz:EPL:2001,
 author    = {A. S. Sanz and F. Borondo and S. Miret-Art\'es},
 journal   = {Europhys. Lett.},
 title     = {On the classical limit in atom-surface diffraction},
 volume    = {55},
 pages     = {303-309},
 year      = {2001},
}

@article{sanz:prb:2000,
 author    = {A. S. Sanz and F. Borondo and S. Miret-Art\'es},
 journal   = {Phys. Rev. B},
 title     = {Causal trajectories description of atom diffraction by surfaces},
 volume    = {61},
 pages     = {7743-7751},
 year      = {2000},
}

@book{bell-bk,
  author     = {J. S. Bell},
  title      = {Speakable and Unspeakable in Quantum Mechanics},
  publisher  = {Cambridge University Press},
  year       = {1987},
  address    = {Cambridge},
}

@article{englert:zna:1993-1,
 author    = {B.-G. Englert and M. O. Scully and G. S\"ussmann and H. Walther},
 journal   = {Z. Naturforsch. A},
 title     = {Surrealistic Bohm trajectories},
 volume    = {47},
 pages     = {1175-1186},
 year      = {1993},
}

@article{duerr:zna:1993,
 author    = {D. D\"urr and W. Fusseder and S. Goldstein and N. Zangh\`i},
 journal   = {Z. Naturforsch. A},
 title     = {Comment on `Surrealistic Bohm trajectories'},
 volume    = {48},
 pages     = {1261-1262},
 year      = {1993},
}

@article{duerr:JStatPhys:1992a,
 author    = {D. D\"urr and S. Goldstein and N. Zangh\`{\i}},
 journal   = {J. Stat. Phys.},
 title     = {Quantum equilibrium and the origin of absolute uncertainty},
 volume    = {67},
 pages     = {843-907},
 year      = {1992},
}

@article{englert:zna:1993-2,
 author    = {B.-G. Englert and M. O. Scully and G. S\"ussmann and and H. Walther},
 journal   = {Z. Naturforsch. A},
 title     = {Reply to comment on `Surrealistic Bohm trajectories'},
 volume    = {48},
 pages     = {1263-1264},
 year      = {1993},
}

@article{scully:PhysScr:1998,
 author    = {M. O. Scully},
 journal   = {Phys. Scr.},
 title     = {Do Bohm trajectories always provide a trustworthy physical picture of particle motion?},
 volume    = {T76},
 pages     = {41-46},
 year      = {1998},
}

@article{jonsson:ZPhys:1961,
 author    = {C. J\"onsson},
 journal   = {Z. Phys.},
 title     = {Elektroneninterferenzen an mehreren k\"unstlich hergestellten Feinspalten},
 volume    = {161},
 pages     = {454-474},
 year      = {1961},
}

@article{jonsson:AJP:1974,
 author    = {C. J\"onsson and D. Brandt and S. Hirschi},
 journal   = {Am. J. Phys.},
 title     = {Electron diffraction at multiple slits},
 volume    = {42},
 pages     = {4-11},
 year      = {1974},
}

@article{hirschi:AJP:1974,
 author    = {S. Hirschi},
 journal   = {Am. J. Phys.},
 title     = {Erratum: ``Electron diffraction at multiple slits'' [Am. J. Phys. 42, 4 (1974)]},
 volume    = {42},
 pages     = {423},
 year      = {1974},
}

@article{pozzi:AJP:1973,
 author    = {O. Donati and G. F. Missiroli and G. Pozzi},
 journal   = {Am. J. Phys.},
 title     = {An experiment on electron interference},
 volume    = {41},
 pages     = {639-644},
 year      = {1973},
}

@article{pozzi:AJP:1976,
 author    = {P. G. Merli and G. F. Missiroli and G. Pozzi},
 journal   = {Am. J. Phys.},
 title     = {On the statistical aspect of electron interference phenomena},
 volume    = {44},
 pages     = {306-307},
 year      = {1976},
}

@article{pozzi:AJP:1978,
 author    = {G. Matteucci and G. Pozzi},
 journal   = {Am. J. Phys.},
 title     = {Two further experiments on electron interference},
 volume    = {46},
 pages     = {619-623},
 year      = {1978},
}

@article{pozzi:AJP:2007,
 author    = {S. Frabboni and G.-C. Gazzadi and G. Pozzi},
 journal   = {Am. J. Phys.},
 title     = {Young's double-slit interference experiment with electrons},
 volume    = {75},
 pages     = {1053-1055},
 year      = {2007},
}

@article{pozzi:EJP:2013,
 author    = {G. Matteucci and M. Pezzi and G. Pozzi and G. L. Alberghi and F. Giorgi and  A. Gabrielli and N. S. Cesari and M. Villa and A. Zoccoli and S. Frabboni and G. C. Gazzadi},
 journal   = {Eur. J. Phys.},
 title     = {Build-up of interference patterns with single electrons},
 volume    = {34},
 pages     = {511-517},
 year      = {2013},
}

@article{tonomura:ajp:1989,
 author    = {A. Tonomura and J. Endo and T. Matsuda and T. Kawasaki and H. Ezawa},
 journal   = {Am. J. Phys.},
 title     = {Demonstration of single-electron buildup of an interference pattern},
 volume    = {57},
 pages     = {117-120},
 year      = {1989},
}

@article{shimizu:pra:1992,
 author    = {F. Shimizu and K. Shimizu and H. Takuma},
 journal   = {Phys. Rev. A},
 title     = {Double-slit interference with ultracold metastable neon atoms},
 volume    = {46},
 pages     = {R17-R20},
 year      = {1992},
}

@article{cerofolini:lnc:1980,
 author    = {C. F. Cerofolini},
 journal   = {Lett. Nuovo Cim.},
 title     = {On the nature of the subquantum medium},
 volume    = {29},
 pages     = {305-309},
 year      = {1980},
}

@article{nelson:pr:1966,
 author    = {E. Nelson},
 journal   = {Phys. Rev.},
 title     = {Derivation of the Schr\"odinger equation from Newtonian mechanics},
 volume    = {150},
 pages     = {1079-1085},
 year      = {1966},
}

@article{penna:jmp:1969,
 author    = {L. de la Pe{\~n}a-Auerbach},
 journal   = {J. Math. Phys.},
 title     = {New formulation of stochastic theory and quantum mechanics},
 volume    = {10},
 pages     = {1620-1630},
 year      = {1969},
}

@article{penna:jmp:1971,
 author    = {L. de la Pe{\~n}a-Auerbach},
 journal   = {J. Math. Phys.},
 title     = {Stochastic theory of quantum mechanics for particles with spin},
 volume    = {12},
 pages     = {453-461},
 year      = {1971},
}

@article{bohm:pr:1954,
 author    = {D. Bohm and J. P. Vigier},
 journal   = {Phys. Rev.},
 title     = {Model of the causal interpretation of quantum theory in terms of a fluid with irregular fluctuations},
 volume    = {96},
 pages     = {208-216},
 year      = {1954},
}

@article{sanz:cpl:2007,
title = {Aspects of nonlocality from a quantum trajectory perspective: A WKB approach to Bohmian mechanics},
journal = {Chem. Phys. Lett.},
volume = {445},
number = {4},
pages = {350-354},
year = {2007},
issn = {0009-2614},
doi = {https://doi.org/10.1016/j.cplett.2007.08.002},
url = {https://www.sciencedirect.com/science/article/pii/S0009261407010561},
author = {A. S. Sanz and S. Miret-Art\'es},
}

@article{berry:JPA:1996,
 author    = {M. V. Berry},
 journal   = {J. Phys. A: Math. Theor.},
 title     = {Quantum fractals in boxes},
 volume    = {29},
 pages     = {6617-6629},
 year      = {1996},
 doi       = {10.1088/0305-4470/29/20/016},
}

@article{sanz:JPA:2005,
 author    = {A. S. Sanz},
 journal   = {J. Phys. A: Math. Theor.},
 title     = {A Bohmian approach to quantum fractals},
 volume    = {38},
 pages     = {6037-6049},
 year      = {2005},
 doi       = {10.1088/0305-4470/38/26/013},
}

@article{sanz:cpl:2008,
 author    = {A. S. Sanz and S. Miret-Art\'es},
 journal   = {Chem. Phys. Lett.},
 title     = {Interplay of causticity and vorticality within the complex quantum Hamilton-Jacobi formalism},
 volume    = {458},
 pages     = {239-243},
 year      = {2008},
}

@article{chou:prl:2009,
 author    = {C.-C. Chou and A. S. Sanz and S. Miret-Art\'es and R. E. Wyatt},
 journal   = {Phys. Rev. Lett.},
 title     = {Hydrodynamic view of wave-packet interference: Quantum caves},
 volume    = {102},
 pages     = {250401(1-4)},
 year      = {2009},
}

@article{chou:annphys:2010,
 author    = {C.-C. Chou and A. S. Sanz and S. Miret-Art\'es and R. E. Wyatt},
 journal   = {Ann. Phys.},
 title     = {Quantum interference within the complex quantum Hamilton-Jacobi formalism},
 volume    = {325},
 pages     = {2193-2211},
 year      = {2010},
}

@article{sanz:jcp:2004,
 author    = {A. S. Sanz and F. Borondo and S. Miret-Art\'es},
 journal   = {J. Chem. Phys.},
 title     = {Quantum trajectories in atom-surface scattering with single adsorbates: The role of quantum vortices},
 volume    = {120},
 pages     = {8794-8806},
 year      = {2004},
 doi       = {10.1063/1.1683136},
}

@article{sanz:prb:2004,
 author    = {A. S. Sanz and F. Borondo and S. Miret-Art\'es},
 journal   = {Phys. Rev. B},
 title     = {Role of quantum vortices in atomic scattering from single adsorbates},
 volume    = {69},
 pages     = {115413(1-5)},
 year      = {2004},
 doi       = {10.1103/PhysRevB.69.115413},
}

@article{sanz:cpl:2009,
 author    = {A. S. Sanz and X. Gim\'enez and J. M. Bofill and S. Miret-Art\'es},
 journal   = {Chem. Phys. Lett.},
 title     = {Understanding chemical reactions within a generalized Hamilton-Jacobi framework},
 volume    = {478},
 pages     = {89-96},
 year      = {2009},
}

@article{sanz:cpl:2010E,
 author    = {A. S. Sanz and X. Gim\'enez and J. M. Bofill and S. Miret-Art\'es},
 journal   = {Chem. Phys. Lett.},
 title     = {Erratum to `Understanding chemical reactions within a generalized Hamilton-Jacobi framework' [Chem. Phys. Lett. {\bf 478} (2009) 89]},
 volume    = {488},
 pages     = {235-236},
 year      = {2010},
}

@article{prosser:ijtp:1976-1,
 author    = {R. D. Prosser},
 journal   = {Int. J. Theor. Phys.},
 title     = {The interpretation of diffraction and interference in terms of energy flow},
 volume    = {15},
 pages     = {169-180},
 year      = {1976},
}

@article{prosser:ijtp:1976-2,
 author    = {R. D. Prosser},
 journal   = {Int. J. Theor. Phys.},
 title     = {Quantum theory and the nature of interference},
 volume    = {15},
 pages     = {181-193},
 year      = {1976},
}

@book{scully-zubairy-bk,
  author     = {M. O. Scully and S. Zubairy},
  title      = {Quantum Optics},
  publisher  = {Cambridge University Press},
  year       = {1997},
  address    = {Cambridge},
}

@article{ehrenberg:procphyssocb:1949,
 author    = {W. Ehrenberg and R. E. Siday},
 journal   = {Proc. Phys. Soc. B},
 title     = {The refractive index in electron optics and the principles of dynamics},
 volume    = {62},
 pages     = {8-21},
 year      = {1949},
}

@article{aharonov:pr:1959,
 author    = {Y. Aharonov and D. Bohm},
 journal   = {Phys. Rev.},
 title     = {Significance of electromagnetic potentials in the quantum theory},
 volume    = {115},
 pages     = {485-491},
 year      = {1959},
}

@article{aharonov:pr:1961,
 author    = {Y. Aharonov and D. Bohm},
 journal   = {Phys. Rev.},
 title     = {Further considerations on electromagnetic potentials in the quantum theory},
 volume    = {123},
 pages     = {1511-1524},
 year      = {1961},
}

@article{josephson:rmp:1974,
 author    = {B. D. Josephson},
 journal   = {Rev. Mod. Phys.},
 title     = {The discovery of tunnelling supercurrents},
 volume    = {46},
 pages     = {251-254},
 year      = {1974},
}

@article{bohm:nuovocim:1976,
 author    = {D. Bohm and B. J. Hiley},
 journal   = {Nuovo Cim.},
 title     = {Non-locality and polarisation correlations of annihilation quanta},
 volume    = {35B},
 pages     = {137-144},
 year      = {1967},
}

@article{butt:jpg:1976,
 author    = {A. R. Wilson and J. Lowe and D. K. Butt},
 journal   = {J. Phys. G},
 title     = {Measurement of the relative planes of polarization of annihilation quanta as a function of separation distance},
 volume    = {2},
 pages     = {613-624},
 year      = {1976},
}

@book{bohm-hiley-bk,
  author     = {D. Bohm and B. J. Hiley},
  title      = {The Undivided Universe},
  publisher  = {Routledge},
  year       = {1993},
  address    = {New York},
}

@book{wheeler:1978,
  AUTHOR =       {J. A. Wheeler},
  editor =       {A. R. Marlow},
  TITLE =        {The past and the delayed-choice double-slit experiment},
  PUBLISHER =    {Academic Press},
  YEAR =         {1978},
  series =       {Mathematical Foundations of Quantum Theory},
  pages =        {9-47},
  address =      {New York},
}

@book{wheeler:1983,
  AUTHOR =       {W. A. Miller and J. A. Wheeler},
  editor =       {S. Kamefuchi and},
  TITLE =        {Delayed-choice experiments and Bohr's elementary quantum phenomenon},
  PUBLISHER =    {Physical Society of Japan},
  YEAR =         {1983},
  series =       {Proc. Int. Symp. Foundation of Quantum Mechanics (Tokyo)},
  pages =        {140-151},
  address =      {Tokyo},
}

@article{hiley:physscr:2006,
 author    = {B. J. Hiley and R. E. Callaghan},
 journal   = {Phys. Scr.},
 title     = {Delayed-choice experiments and the Bohm approach},
 volume    = {74},
 pages     = {336-348},
 year      = {2006},
}

@article{hiley:arxiv:2011,
 author    = {M. de Gosson and B. J. Hiley},
 journal   = {arXiv:1010.2622v2},
 title     = {Zeno paradox for Bohmian trajectories: The unfolding of the metatron},
 volume    = {},
 pages     = {},
 year      = {2011},
}

@article{hiley:foundphys:1982,
 author    = {C. Dewdney and B. J. Hiley},
 journal   = {Found. Phys.},
 title     = {A quantum potential description of one-dimensional time-dependent scattering from square barriers},
 volume    = {12},
 pages     = {27-48},
 year      = {1982},
}

@article{wyatt:JCP:1999,
 author    = {R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Quantum wave packet dynamics with trajectories: Application to reactive scattering},
 volume    = {111},
 pages     = {4406-4413},
 year      = {1999},
}

@BOOK{schiff-bk,
  AUTHOR     = {L. I. Schiff},
  TITLE      = {Quantum Mechanics},
  PUBLISHER  = {McGraw-Hill},
  YEAR       = {1968},
  address    = {Singapore},
  edition    = {3rd},
}

@BOOK{liboff-bk,
  AUTHOR     = {R. L. Liboff},
  TITLE      = {Introductory Quantum Mechanics},
  PUBLISHER  = {Addison-Wesley},
  YEAR       = {1980},
  address    = {Reading, MA},
}

@article{brumer:pra:2006,
 author    = {P. Brumer and J. Gong},
 journal   = {Phys. Rev. A},
 title     = {Born rule in quantum and classical mechanics},
 volume    = {73},
 pages     = {052109(1-4)},
 year      = {2006},
}

@article{sanz:jcp:2005,
 author    = {A. S. Sanz and S. Miret-Art\'es},
 journal   = {J. Chem. Phys.},
 title     = {Quantum trajectories in elastic atom-surface scattering: Threshold and selective adsorption resonances},
 volume    = {122},
 pages     = {014702(1-12},
 year      = {2005},
}

@article{elster:1899,
 author    = {J. Elster and H. Geitel},
 journal   = {Verhandlungen der Deutschen Physikalischen Gesellschaft},
 title     = {\"Uber den Einflu{\ss} eines magnetischen Feldes auf die durch die Becquerelstrahlen bewirkte Leitf\"ahigkeit der Luft},
 volume    = {1},
 pages     = {136-138},
 year      = {1899},
}

@BOOK{goldstein-bk,
  AUTHOR     = {H. Goldstein and C. Poole and J. Safko},
  TITLE      = {Classical Mechanics},
  PUBLISHER  = {Addison Wesley},
  YEAR       = {2001},
  address    = {New York},
  edition    = {3rd},
}

@BOOK{tannor-bk,
  AUTHOR     = {D. J. Tannor},
  TITLE      = {Introduction to Quantum Mechanics: A Time-Dependent Perspective},
  PUBLISHER  = {University Science Books},
  YEAR       = {2006},
  address    = {Sausalito, CA},
}

@BOOK{feynman-bk1,
  AUTHOR     = {R. P. Feynman and A. R. Hibbs},
  TITLE      = {Quantum Mechanics and Path Integrals},
  PUBLISHER  = {McGraw-Hill},
  YEAR       = {1965},
  address    = {New York},
}

@BOOK{feynman-bk2,
  AUTHOR     = {R. P. Feynman},
  TITLE      = {Path Integral Approach to Quantum Mechanics},
  PUBLISHER  = {University Science Books},
  YEAR       = {2006},
  address    = {Sausalito, CA},
}

@article{egger:MonWeaRev:1996,
 author    = {J. Egger},
 journal   = {Am. Meteor. Soc.},
 title     = {Volume conservation in phase space: A fresh look at numerical integration schemes},
 volume    = {124},
 pages     = {1955-1964},
 year      = {1996},
}

@article{sommer:MonWeaRev:2010,
 author    = {M. Sommer and S. Reich},
 journal   = {Am. Meteor. Soc.},
 title     = {Phase space volume conservation under space and time discretization schemes for the shallow-water equations},
 volume    = {138},
 pages     = {4229-4236},
 year      = {2010},
}

@BOOK{mazur-bk:2007,
  AUTHOR     = {J. Mazur},
  TITLE      = {Zeno's Paradox: Unraveling the Ancient Mystery behind the Science of Space and Time},
  PUBLISHER  = {Plume},
  YEAR       = {2007},
  address    = {New York},
}

@article{sanz:JPA:2011,
 author    = {A. S. Sanz and S. Miret-Art\'es},
 journal   = {J. Phys. A: Math. Theor.},
 title     = {Setting-up tunneling conditions by means of Bohmian mechanics},
 volume    = {44},
 pages     = {485301(1-17)},
 year      = {2011},
}

@article{gonzalo:PRA:2011,
 author    = {M. A. Porras and A. Luis and I. Gonzalo and A. S. Sanz},
 journal   = {Phys. Rev. A},
 title     = {Zeno dynamics in wave packet diffraction spreading},
 volume    = {84},
 pages     = {052109(1-6)},
 year      = {2011},
}

@article{misra:JMathPhys:1977,
 author    = {B. Misra and E. C. G. Sudarshan},
 journal   = {J. Math. Phys.},
 title     = {The Zeno's paradox in quantum theory},
 volume    = {18},
 pages     = {756-763},
 year      = {1977},
}

@article{misra:PRD:1977,
 author    = {C. B. Chiu and E. C. G. Sudarshan and B. Misra},
 journal   = {Phys. Rev. D},
 title     = {Time evolution of unstable quantum systems and a resolution of Zeno's paradox},
 volume    = {16},
 pages     = {520-529},
 year      = {1977},
}

@article{peres:AmJPhys:1980,
 author    = {A. Peres},
 journal   = {Am. J. Phys.},
 title     = {Zeno paradox in quantum theory},
 volume    = {48},
 pages     = {931-932},
 year      = {1980},
}

@article{pascazio:JPA:2008,
 author    = {P. Facchi and S. Pascazio},
 journal   = {J. Phys. A: Math. Theor.},
 title     = {Quantum Zeno dynamics: mathematical and physical aspects},
 volume    = {41},
 pages     = {493001(1-45)},
 year      = {2008},
}

@article{pascazio:PRL:2001,
 author    = {P. Facchi and H. Nakazato and S. Pascazio},
 journal   = {Phys. Rev. Lett.},
 title     = {From the quantum zeno to the inverse quantum Zeno effect},
 volume    = {86},
 pages     = {2699-2702},
 year      = {2001},
}

@article{itano:PRA:1990,
 author    = {W. M. Itano and D. J. Heinzen and J. J. Bollinger and D. J. Wineland},
 journal   = {Phys. Rev. A},
 title     = {Quantum Zeno effect},
 volume    = {41},
 pages     = {2295-2300},
 year      = {1990},
}

@article{cook:PhysScr:1988,
 author    = {R. J. Cook},
 journal   = {Phys. Scr.},
 title     = {What are quantum jumps?},
 volume    = {T21},
 pages     = {49-51},
 year      = {1988},
}

@BOOK{dirac-bk:1930,
  AUTHOR     = {P. A. M. Dirac},
  TITLE      = {Principles of Quantum Mechanics},
  PUBLISHER  = {Oxford University Press},
  YEAR       = {1930},
  address    = {Oxford},
}

@BOOK{vonNeumann-bk:1932,
  AUTHOR     = {J. von Neumann},
  TITLE      = {Die Mathematische Grundlagen der Quantenmechanik},
  PUBLISHER  = {Springer Verlag},
  YEAR       = {1932},
  address    = {Berlin},
}

@BOOK{vonNeumann-bk:1932En,
  AUTHOR     = {J. von Neumann and R. T. Beyer (transl.)},
  TITLE      = {Mathematical Foundations of Quantum Mechanics},
  PUBLISHER  = {Princeton University Press},
  YEAR       = {1955},
  address    = {Princeton},
}

@BOOK{parker-bk:1994,
  AUTHOR     = {C. B. Parker},
  TITLE      = {McGraw Hill Encyclopaedia of Physics},
  PUBLISHER  = {McGraw Hill},
  YEAR       = {1994},
  address    = {Princeton},
  edition    = {2nd},
}

@article{raizen:PRL:2001,
 author    = {M. C. Fischer and B. Guti\'errez-Medina and M. G. Raizen},
 journal   = {Phys. Rev. Lett.},
 title     = {Observation of the quantum Zeno and anti-Zeno effects in an unstable system},
 volume    = {87},
 pages     = {040402(1-4)},
 year      = {2001},
}

@article{raizen:Nature:1997,
 author    = {S. R. Wilkinson and C. F. Bharucha and M. C. Fischer and K. W. Madison and P. R. Morrow and Q. Niu and B. Sundaram and M. G. Raizen},
 journal   = {Nature},
 title     = {Experimental evidence for non-exponential decay in quantumtunnelling},
 volume    = {387},
 pages     = {575-577},
 year      = {1997},
}

@article{luis:PRA:1998,
 author    = {A. Luis and L. S\'anchez-Soto},
 journal   = {Phys. Rev. A},
 title     = {Anti-Zeno effect in parametric down-conversion},
 volume    = {57},
 pages     = {781-787},
 year      = {1998},
}

@article{kaulakys:PRA:1997,
 author    = {B. Kaulakys and V. Gontis},
 journal   = {Phys. Rev. A},
 title     = {Quantum anti-Zeno effect},
 volume    = {56},
 pages     = {1131-1137},
 year      = {1997},
}

@article{kofman:Nature:2000,
 author    = {A. G. Kofman and G. Kurizki},
 journal   = {Nature},
 title     = {Acceleration of quantum decay processes by frequent observations},
 volume    = {405},
 pages     = {546-550},
 year      = {2000},
}

@BOOK{kloeden-bk:1992,
  AUTHOR     = {P. E. Kloeden and E. Platen},
  TITLE      = {Numerical Solution of Stochastic Differential Equations},
  PUBLISHER  = {Springer},
  YEAR       = {1992},
  address    = {Berlin},
}

@BOOK{breuer-bk:2002,
  AUTHOR     = {H.-P. Breuer and F. Petruccione},
  TITLE      = {The Theory of Open Quantum Systems},
  PUBLISHER  = {Oxford University Press},
  YEAR       = {2002},
  address    = {Oxford},
}

@article{tomas:2011,
 author    = {C. Sanz-Sanz and A. S. Sanz and T. Gonz\'alez-Lezana and O. Roncero and S. Miret-Art\'es},
 journal   = {},
 title     = {Revisiting Zeno's paradox: Flying arrows for atom-diatom reactions},
 volume    = {},
 pages     = {(1-4)},
 year      = {submitted, 2011},
 archivePrefix        = {arXiv},
 eprint               = {1111.1520},
}

@article{coffey:JPA:2008,
 author    = {T. M. Coffey and R. E. Wyatt and W. C. Schieve},
 journal   = {J. Phys. A: Math. Theor.},
 title     = {Monte Carlo generation of Bohmian trajectories},
 volume    = {41},
 pages     = {335304},
 year      = {2008},
}

@article{coffey:JPA:2010,
 author    = {T. M. Coffey and R. E. Wyatt and W. C. Schieve},
 journal   = {J. Phys. A: Math. Theor.},
 title     = {Quantum trajectories from kinematic considerations},
 volume    = {43},
 pages     = {335301},
 year      = {2010},
}

@article{brandt:PLA:1998,
 author    = {S. Brandt and H. Dahmen and E. Gjonaj and T. Stroh},
 journal   = {Phys. Lett. A},
 title     = {Quantile motion and tunneling},
 volume    = {249},
 pages     = {265},
 year      = {1998},
}

@article{englert:PRL:1996,
 author    = {B.-G. Englert},
 journal   = {Phys. Rev. Lett.},
 title     = {Fringe visibility and which-way information: An inequality},
 volume    = {77},
 pages     = {2154-2157},
 year      = {1996},
}

@article{chapman:PRL:1995,
 author    = {M. S. Chapman and T. D. Hammond and A. Lenef and J. Schmiedmayer and R. A. Rubenstein and E. Smith and D. E. Pritchard},
 journal   = {Phys. Rev. Lett.},
 title     = {Photon scattering from atoms in an atom interferometer: Coherence lost and regained},
 volume    = {75},
 pages     = {3783-3787},
 year      = {1995},
}

@article{fonseca-guerra:JComputChem:2004,
 author    = {C. Fonseca-Guerra and J.-W. Handgraaf and E. J. Baerends and F. M. Bickelhaupt},
 journal   = {J. Comput. Chem.},
 title     = {Voronoi deformation density (VDD) charges: Assessment of the Mulliken, Bader, Hirshfeld, Weinhold, and VDD methods for charge analysis},
 volume    = {25},
 pages     = {189-210},
 year      = {2004},
}

@article{sanz:AJP:2012,
 author    = {A. S. Sanz and S. Miret-Art\'es},
 journal   = {Am. J. Phys.},
 title     = {Quantum phase analysis with quantum trajectories: A step towards the creation of a Bohmian thinking},
 volume    = {80},
 pages     = {525-533},
 year      = {2012},
doi = {10.1119/1.3698324},
URL = {https://doi.org/10.1119/1.3698324},
}

@PROCEEDINGS{dorlas:SPIE:2004,
   author = {T. C. Dorlas and R. F. O'Connell},
    title = {Quantum Zeno and anti-Zeno effects: An exact model},
booktitle = {Quantum Information and Computation II},
     year = {2004},
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = {5436},
   eprint = {arXiv:quant-ph/0501098},
   editor = {E. Donkor and A. R. Pirich and H. E. Brandt},
    pages = {194-201},
publisher = {SPIE},
  address = {Bellingham, WA},
}

@article{sanz:AnnPhys:2012,
 author    = {A. S. Sanz and C. Sanz-Sanz and T. Gonz\'alez-Lezana and O. Roncero and S. Miret-Art\'es},
 journal   = {Ann. Phys.},
 title     = {Quantum Zeno effect: Quantum shuffling and Markovianity},
 volume    = {327},
 pages     = {1277-1289},
 year      = {2012},
}

@article{octavio:JCP:2012,
 author    = {C. Sanz-Sanz and A. S. Sanz and T. Gonz\'alez-Lezana and O. Roncero and S. Miret-Art\'es},
 journal   = {J. Chem. Phys.},
 title     = {Communication: Quantum Zeno-based control mechanism for molecular fragmentation},
 volume    = {136},
 pages     = {121101(1-4)},
 year      = {2012},
}

@article{helen:JPCM:2011,
 author    = {H. C. Pe\~nate-Rodr{\'\i}guez and R. Mart{\'\i}nez-Casado and G. Rojas-Lorenzo and A. S. Sanz and S. Miret-Art\'es},
 journal   = {J. Phys.: Condens. Matter},
 title     = {Quantum Zeno and anti-Zeno effects in surface diffusion of interacting adsorbates},
 volume    = {24},
 pages     = {104013(1-10)},
 year      = {2012},
}

@BOOK{gutzwiller:1990,
  AUTHOR     = {M. C. Gutzwiller},
  TITLE      = {Chaos in Classical and Quantum Mechanics},
  PUBLISHER  = {Springer-Verlag},
  YEAR       = {1990},
  address    = {New York},
}

@article{sanz:PhysRep:2007,
 author    = {A. S. Sanz and S. Miret-Art\'es},
 journal   = {Phys. Rep.},
 title     = {Selective adsorption resonances: Quantum and stochastic approaches},
 volume    = {451},
 pages     = {37-154},
 year      = {2007},
}

@article{fortagh:RMP:2007,
 author    = {J. Fort\'agh and C. Zimmermann},
 journal   = {Rev. Mod. Phys.},
 title     = {Magnetic microtraps for ultracold atoms},
 volume    = {79},
 pages     = {235-289},
 year      = {2007},
}

@BOOK{brumer-bk:2003,
  AUTHOR     = {M. Shapiro and P. Brumer},
  TITLE      = {Principles of the Quantum Control of Molecular Processes},
  PUBLISHER  = {Wiley},
  YEAR       = {2003},
  address    = {New York},
}

@article{sanz:AnnPhys:2013,
 author    = {A. S. Sanz and S. Miret-Art\'es},
 journal   = {Ann. Phys.},
 title     = {On the unique mapping relationship between initial and final quantum states},
 volume    = {339},
 pages     = {11-21},
 year      = {2013},
}

@article{sinha:Science:2010,
 author    = {U. Sinha and C. Couteau and T. Jennewein and R. Laflamme and G. Weihs},
 journal   = {Science},
 title     = {Ruling out multi-order interference in quantum mechanics},
 volume    = {329},
 pages     = {418-421},
 year      = {2010},
}

@article{uiberacker:Nature:2007,
 author    = {M. Uiberacker and Th. Uphues and M. Schultze and A. J. Verhoef and V. Yakovlev and M. F. Kling
              and J. Rauschenberger and N. M. Kabachnik and H. Schr\"oder and M. Lezius and K. L. Kompa and
              H.-G. Muller and M. J. J. Vrakking and S. Hendel and U. Kleineberg and U. Heinzmann and M. Drescher
              and F. Krausz},
 journal   = {Nature},
 title     = {Attosecond real-time observation of electron tunneling in atoms},
 volume    = {446},
 pages     = {627-632},
 year      = {2007},
}

@article{arndt:NatCommun:2011,
 author    = {S. Gerlich and S. Eibenberger and M. Tomandl and S. Nimmrichter and K. Hornberger and P. J. Fagan and J. T\"uxen and M. Mayor and M. Arndt},
 journal   = {Nat. Commun.},
 title     = {Quantum interference of large organic molecules},
 volume    = {2:263},
 pages     = {1-5},
 year      = {2011},
}

@article{bowman:JCP:1975,
 author    = {C. J. Ray and J. M. Bowman},
 journal   = {J. Chem. Phys.},
 title     = {Quasiclassical trajectory calculation of He-LiF(001) diffraction scattering},
 volume    = {63},
 pages     = {5231-5234},
 year      = {1975},
}

@article{bowman:JCP:1977,
 author    = {C. J. Ray and J. M. Bowman},
 journal   = {J. Chem. Phys.},
 title     = {Quasiclassical studies of rigid rotor-solid surface diffraction scattering},
 volume    = {66},
 pages     = {1122-1126},
 year      = {1977},
}

@article{diaz:PRL:2004,
 author    = {D. Far{\'\i}as and C. D{\'\i}az and P. Rivi\`ere and H. F. Busnego and P. Nieto and M. F. Somers and G. J. Kroes and A. Salin and F. Mart{\'\i}n},
 journal   = {Phys. Rev. Lett.},
 title     = {In-plane and out-of-plane diffraction of H$_2$ from metal surfaces},
 volume    = {93},
 pages     = {246104(1-4)},
 year      = {2004},
}

@article{diaz:PRB:2005,
 author    = {C. D{\'\i}az and M. F. Somers and G. J. Kroes and H. F. Busnego and A. Salin and F. Mart{\'\i}n},
 journal   = {Phys. Rev. B},
 title     = {Quantum and classical dynamics of H$_2$ scattering from Pd(111) at off-normal incidence},
 volume    = {72},
 pages     = {035401(1-10)},
 year      = {2005},
}

@article{diaz:JCP:2005,
 author    = {C. D{\'\i}az and H. F. Busnego and P. Rivi\`ere and D. Far{\'\i}as and P. Nieto and M. F. Somers and G. J. Kroes and A. Salin and F. Mart{\'\i}n},
 journal   = {J. Chem. Phys.},
 title     = {A classical dynamics method for H$_2$ diffraction from metal surfaces},
 volume    = {122},
 pages     = {154706(1-8)},
 year      = {2005},
}

@article{miller:JPCA:2011,
 author    = {W. H. Miller},
 journal   = {J. Phys. Chem. A},
 title     = {The semiclassical initial value representation: A potentially practical way for adding quantum effects to classical molecular dynamics simulations},
 volume    = {105},
 pages     = {2942-2955},
 year      = {2001},
}

@article{pollak:PRL:2003,
 author    = {S. Zhang and E. Pollak},
 journal   = {Phys. Rev. Lett.},
 title     = {Monte Carlo method for evaluating the quantum real time propagator},
 volume    = {91},
 pages     = {190201(1-4)},
 year      = {2003},
}

@BOOK{zhang-bk,
  AUTHOR     = {J. Z. H. Zhang},
  TITLE      = {Theory and Application of Quantum Molecular Dynamics},
  PUBLISHER  = {World Scientific},
  YEAR       = {1999},
  address    = {Singapore},
}

@article{bittner:JCP:2003,
 author    = {E. R. Bittner},
 journal   = {J. Chem. Phys.},
 title     = {Quantum initial value representation using approximate Bohmian trajectories},
 volume    = {119},
 pages     = {1358-1364},
 year      = {2003},
}

@article{makri:JCP:2003,
 author    = {Y. Zhao and N. Makri},
 journal   = {J. Chem. Phys.},
 title     = {Bohmian versus semiclassical description of interference phenomena},
 volume    = {119},
 pages     = {60-67},
 year      = {2003},
}

@article{makri:JPCA-1:2004,
 author    = {J. Liu and N. Makri},
 journal   = {J. Phys. Chem. A},
 title     = {Forward-backward quantum dynamics for time correlation functions},
 volume    = {108},
 pages     = {806-812},
 year      = {2004},
}

@article{makri:JPCA-2:2004,
 author    = {J. Liu and N. Makri},
 journal   = {J. Phys. Chem. A},
 title     = {Monte Carlo Bohmian dynamics from trajectory stability properties},
 volume    = {108},
 pages     = {5408-5416},
 year      = {2004},
}

@article{makri:MolPhys:2005,
 author    = {J. Liu and N. Makri},
 journal   = {Mol. Phys.},
 title     = {Bohm's formulation in imaginary time: estimation of energy eigenvalues},
 volume    = {103},
 pages     = {1083-1090},
 year      = {2005},
}

@article{franco:JCP:2017,
 author  = {B. Gu. and I. Franco},
 journal  = {J. Chem. Phys.},
 title  = {Partial hydrodynamic representation of quantum molecular dynamics},
 volume  = {146},
 pages  = {194104(1-8)},
 year   = {2017},
}

@BOOK{sanz-bk-1,
  AUTHOR     = {A. S. Sanz and S. Miret-Art\'es},
  TITLE      = {A Trajectory Description of Quantum Processes. I. Fundamentals},
  PUBLISHER  = {Springer},
  volume     = {850},
  series     = {Lecture Notes in Physics},
  YEAR       = {2012},
  address    = {Berlin},
}

@BOOK{sanz-bk-2,
  AUTHOR     = {A. S. Sanz and S. Miret-Art\'es},
  TITLE      = {A Trajectory Description of Quantum Processes. II. Applications},
  PUBLISHER  = {Springer},
  volume     = {831},
  series     = {Lecture Notes in Physics},
  YEAR       = {2014},
  address    = {Berlin},
}

@article{ballentine:RMP:1979,
 author    = {L. E. Ballentine},
 journal   = {Rev. Mod. Phys.},
 title     = {The statistical interpretation of quantum mechanics},
 volume    = {42},
 pages     = {358-381},
 year      = {1979},
}

@article{sanz:SSR:2004,
 author    = {R. Guantes and A. S. Sanz and J. Margalef-Roig and S. Miret-Art\'es},
 journal   = {Surf. Sci. Rep.},
 title     = {Atom-surface diffraction: a trajectory description},
 volume    = {53},
 pages     = {199-330},
 year      = {2004},
}

@article{kosloff:JCP:1983,
 author    = {R. Kosloff and D. Kosloff},
 journal   = {J. Chem. Phys.},
 title     = {A Fourier method solution for the time dependent Schr\"odinger equation: A study of the reaction H$^+$+H$_2$, D$^+$+HD, and D$^+$+H$_2$},
 volume    = {79},
 pages     = {1823-1833},
 year      = {1983},
}

@article{kosloff:JCompPhys:1983,
 author    = {D. Kosloff and R. Kosloff},
 journal   = {J. Comp. Phys.},
 title     = {A Fourier method solution for the time dependent Schr\"odinger equation as a tool in molecular dynamics},
 volume    = {52},
 pages     = {35-53},
 year      = {1983},
}

@article{kosloff:JCompPhys:1986,
 author    = {R. Kosloff and D. Kosloff},
 journal   = {J. Comp. Phys.},
 title     = {Absorbing boundaries for wave propagation problems},
 volume    = {63},
 pages     = {363-376},
 year      = {1986},
}

@article{manolopoulos:JCompPhys:2002,
 author    = {D. E. Manolopoulos},
 journal   = {J. Comp. Phys.},
 title     = {Derivation and reflection properties of a transmission-free absorbing potential},
 volume    = {117},
 pages     = {9552-9559},
 year      = {2002},
}

@article{metiu:JCompPhys:1986,
 author    = {R. Heather and H. Metiu},
 journal   = {J. Comp. Phys.},
 title     = {An efficient procedure for calculating the evolution of the wave function by fast Fourier transform methods for systems with spatially extended wave function and localized potential},
 volume    = {86},
 pages     = {5009-5017},
 year      = {1986},
}

@article{pernot:IJQC:1991,
 author    = {P. Pernot and W. A. Lester Jr.},
 journal   = {Intern. J. Quantum Chem.},
 title     = {Multidimensional wave-packet analysis: Splitting method for time-resolved property determination},
 volume    = {40},
 pages     = {577-588},
 year      = {1991},
}

@article{born:ZPhys:1926,
 author    = {M. Born},
 journal   = {Z. Phys.},
 title     = {Zur Quantenmechanik der Sto{\ss}vorg\"ange,},
 volume    = {37},
 pages     = {863-867},
 year      = {1926},
}

@book{landsman:CQP:2009,
  AUTHOR =       {N. P. Landsman},
  editor =       {D. Greenberger and K. Hentschel and F. Weinert},
  TITLE =        {Born rule and its interpretation},
  PUBLISHER =    {Springer},
  YEAR =         {2009},
  series =       {Compendium of Quantum Physics: Concepts, Experiments, History and Philosophy},
  pages =        {64-70},
  address =      {Berlin},
}

@article{thompson:JCP:1972,
 author    = {D. L. Thompson},
 journal   = {J. Chem. Phys.},
 title     = {On a classical trajectory study of energy transfer in some atom-diatomic molecule systems},
 volume    = {56},
 pages     = {3570-3580},
 year      = {1972},
}

@article{karplus:JCP:1965,
 author    = {M. Karplus and R. N. Porter and R. D. Sharma},
 journal   = {J. Chem. Phys.},
 title     = {Exchange reactions with activation energy. I. Simple barrier potential for (H, H$_2$)},
 volume    = {43},
 pages     = {3259-3287},
 year      = {1965},
}

@article{kerner:CanJPhys:1958,
 author    = {E. H. Kerner},
 journal   = {Can. J. Phys.},
 title     = {Note on the forced and damped oscillator in quantum mechanics},
 volume    = {36},
 pages     = {371-377},
 year      = {1958},
}

@article{schuch:IJQC:1990,
 author    = {D. Schuch},
 journal   = {Int. J. Quantum. Chem.},
 title     = {},
 volume    = {24},
 pages     = {767-},
 year      = {1990},
}

@article{schuch:IJQC:1999,
 author    = {D. Schuch},
 journal   = {Int. J. Quantum. Chem.},
 title     = {Effective description of the dissipative interaction between simple model-systems and their environment},
 volume    = {72},
 pages     = {537-547},
 year      = {1999},
}

@article{majima:AnnPhys:2011,
 author    = {H. Majima and A. Suzuki},
 journal   = {Ann. Phys.},
 title     = {Quantization and instability of the damped harmonic oscillator subject to a time-dependent force},
 volume    = {326},
 pages     = {3000-3012},
 year      = {2011},
}

@article{jannussis:PhysicaA:1980,
 author    = {A. Jannussis and P. Filipakis and Th. Filipakis},
 journal   = {Physica},
 title     = {Quantum friction in phase space},
 volume    = {102A},
 pages     = {561-567},
 year      = {1980},
}

@article{jannussis:PhysLett:1979,
 author    = {A. D. Jannussis and G. N. Brodimas and A. Streclas},
 journal   = {Phys. Lett.},
 title     = {Propagator with friction in quantum mechanics},
 volume    = {74A},
 pages     = {6-10},
 year      = {1979},
}

@article{khandekar:JMathPhys:1979,
 author    = {D. C. Khandekar and S. V. Lawande},
 journal   = {J. Math. Phys.},
 title     = {Exact solution of a time-dependent quantal harmonic oscillator with damping and a perturbative force},
 volume    = {20},
 pages     = {1870-1877},
 year      = {1979},
}

@article{sun:PRA:1995,
 author    = {C.-P. Sun and L.-H. Yu},
 journal   = {Phys. Rev. A},
 title     = {Exact dynamics of a quantum dissipative system in a constant external field},
 volume    = {51},
 pages     = {1845-1853},
 year      = {1995},
}

@article{sun:PRA:1994,
 author    = {L.-H. Yu and C.-P. Sun},
 journal   = {Phys. Rev. A},
 title     = {Evolution of the wave function in a dissipative system},
 volume    = {49},
 pages     = {592-595},
 year      = {1994},
}

@article{schuch:PRA:1997,
 author    = {D. Schuch},
 journal   = {Phys. Rev. A},
 title     = {Nonunitary connection between explicitly time-dependent and nonlinear approaches for the description of dissipative quantum systems},
 volume    = {55},
 pages     = {935-940},
 year      = {1997},
}

@article{schuch:JPA:2001,
 author    = {M. Moshinsky and D. Schuch},
 journal   = {J. Phys. A: Math. Gen.},
 title     = {Diffraction in time with dissipation},
 volume    = {34},
 pages     = {4217-4225},
 year      = {2001},
}

@article{schuch:RevMexFis:2001,
 author    = {M. Moshinsky and D. Schuch and A. Su\'arez-Moreno},
 journal   = {Rev. Mex. F{\'\i}s.},
 title     = {Motion of wave packets with dissipation},
 volume    = {47},
 pages     = {7-10},
 year      = {2001},
}

@article{bowman:JCP:1981,
 author    = {K. M. Christoffel and J. M. Bowman},
 journal   = {J. Chem. Phys.},
 title     = {Quantum and classical dynamics of a coupled doble well oscillator},
 volume    = {74},
 pages     = {5057-5075},
 year      = {1981},
}

@article{guerra:PhysRep:1981,
 author    = {F. Guerra},
 journal   = {Phys. Rep.},
 title     = {Structural aspects of stochastic mechanics and stochastic field theory},
 volume    = {77},
 pages     = {263-312},
 year      = {1981},
}

@article{hsiang:IntJModPhysA:2009,
 author    = {J.-T. Hsiang and L. H. Ford},
 journal   = {Int. J. Mod. Phys. A},
 title     = {Decoherence and recoherence in model quantum systems},
 volume    = {24},
 pages     = {1705-1712},
 year      = {2009},
}

@article{guay:JPA:2003,
 author    = {E. Guay and L. Marchildon},
 journal   = {J. Phys. A: Math. Gen.},
 title     = {Two-particle interference in standard Bohmian quantum mechanics},
 volume    = {36},
 pages     = {5617-5624},
 year      = {2003},
 doi       = {10.1088/0305-4470/36/20/317},
}

@article{walborn:PRA:2002,
 author    = {S. P. Walborn and M. O. Terra Cunha and S. P\'adua and C. H. Monken},
 journal   = {Phys. Rev. A},
 title     = {Double-slit quantum eraser},
 volume    = {65},
 pages     = {033818(1-6)},
 year      = {2002},
 doi       = {10.1103/PhysRevA.65.033818},
}

@article{brida:PRA:2003,
  title = {Biphoton double-slit experiment},
  author = {Brida, G. and Cagliero, E. and Falzetta, G. and Genovese, M. and Gramegna, M. and Predazzi, E.},
  journal = {Phys. Rev. A},
  volume = {68},
  issue = {3},
  pages = {033803},
  numpages = {6},
  year = {2003},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.68.033803},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.68.033803}
}

@article{kwiat:LAS:2002,
 author    = {D. F. V. James and P. G. Kwiat},
 journal   = {Los Alamos Science},
 title     = {Quantum state entanglement: Creation, characterizatin and application},
 volume    = {27},
 pages     = {52-67},
 year      = {2002},
}

@article{ghirardi:JStatPhys:2002,
 author    = {G. Ghirardi and L. Marinatto and T. Weber},
 journal   = {J. Stat. Phys.},
 title     = {Entanglement and properties of composite quantum systems: A conceptual and mathematical analysis},
 volume    = {108},
 pages     = {49-122},
 year      = {2002},
}

@article{ghirardi:PRA:2004,
  title = {General criterion for the entanglement of two indistinguishable particles},
  author = {Ghirardi, GianCarlo and Marinatto, Luca},
  journal = {Phys. Rev. A},
  volume = {70},
  issue = {1},
  pages = {012109},
  numpages = {10},
  year = {2004},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.70.012109},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.70.012109}
}

@article{matzkin:PRA:2011,
  title = {Entanglement in the classical limit: Quantum correlations from classical probabilities},
  author = {Matzkin, A.},
  journal = {Phys. Rev. A},
  volume = {84},
  issue = {2},
  pages = {022111},
  numpages = {5},
  year = {2011},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.84.022111},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.84.022111}
}

@article{pollak:JCP:1980,
 author    = {E. Pollak and M. S. Child},
 journal   = {J. Chem. Phys.},
 title     = {Classical mechanics of a collinear exchange reaction: A direct evaluation of the reaction probability and product distribution},
 volume    = {73},
 pages     = {4373-4380},
 year      = {1980},
}

@article{pollak:JCP:1983,
 author    = {E. Pollak},
 journal   = {J. Chem. Phys.},
 title     = {Classical analysis of collinear light atom transfer reactions},
 volume    = {78},
 pages     = {1228-1236},
 year      = {1983},
}

@article{couder:PRL:2005,
 author    = {Y. Couder and E. Fort and C.-H. Gautier and A. Boudaoud},
 journal   = {Phys. Rev. Lett.},
 title     = {From bouncing to floating: Noncoalescence of drops on a fluid bath},
 volume    = {94},
 pages     = {177801(1-4)},
 year      = {2005},
}

@article{couder:Nature:2005,
 author    = {Y. Couder and S. Proti\`ere and E. Fort and A. Boudaoud},
 journal   = {Nature},
 title     = {Dynamical phenomena: Walking and orbiting droplets},
 volume    = {437},
 pages     = {208},
 year      = {2005},
}

@article{couder:JFluidMech:2006,
 author    = {S. Proti\`ere and A. Boudaoud and Y. Couder},
 journal   = {J. Fluid. Mech.},
 title     = {Particle-wave association on a fluid interface},
 volume    = {554},
 pages     = {85-108},
 year      = {2006},
}

@article{couder:PRL:2006,
 author    = {Y. Couder and E. Fort},
 journal   = {Phys. Rev. Lett.},
 title     = {Single-particle diffraction and interference at a macroscopic scale},
 volume    = {97},
 pages     = {154101(1-4)},
 year      = {2006},
}

@article{couder:PhysFluid:2006,
 author    = {S. Proti\`ere and Y. Couder},
 journal   = {Phys. Fluids},
 title     = {Orbital motion of bouncing drops},
 volume    = {18},
 pages     = {091114},
 year      = {2006},
}

@article{couder:EPL:2008,
 author    = {A. Eddi and D. Terwagne and E. Fort and Y. Couder},
 journal   = {Europhys. Lett.},
 title     = {Wave propelled ratchets and drifting rafts},
 volume    = {87},
 pages     = {44001(1-6)},
 year      = {2008},
}

@article{couder:EPL:2009,
 author    = {A. Eddi and A. Decelle and E. Fort and Y. Couder},
 journal   = {Europhys. Lett.},
 title     = {Archimedean lattices in the bound states of wave interacting particles},
 volume    = {87},
 pages     = {56002(1-6)},
 year      = {2009},
}

@article{couder:PRL:2009,
 author    = {A. Eddi and E. Fort and F. Moisy and Y. Couder},
 journal   = {Phys. Rev. Lett.},
 title     = {Unpredictable tunneling of a classical wave-particle association},
 volume    = {102},
 pages     = {240401(1-4)},
 year      = {2009},
}

@article{couder:PNAS:2010,
 author    = {E. Fort and A. Eddi and A. Boudaoud and J. Moukhtar and Y. Couder},
 journal   = {Proc. Natl. Acad. Sci. USA},
 title     = {Path-memory induced quantization of classical orbits},
 volume    = {108},
 pages     = {17515-17520},
 year      = {2010},
}

@article{couder:EPN:2010,
 author    = {Y. Couder and A. Boudaoud and S. Proti\`ere and E. Fort},
 journal   = {Europhys. News},
 title     = {Walking droplets: A form of wave-particle duality at macroscopic scale?},
 volume    = {41},
 pages     = {14-18},
 year      = {2010},
}

@article{bush:PNAS:2010,
 author    = {J. W. M. Bush},
 journal   = {Proc. Natl. Acad. Sci. USA},
 title     = {Quantum mechanics writ large},
 volume    = {107},
 pages     = {17455-17456},
 year      = {2010},
}

@article{bush:PRE:2013,
 author    = {D. M. Harris and J. Moukhtar and E. Fort and Y. Couder and J. W. M. Bush},
 journal   = {Phys. Rev. E},
 title     = {Wavelike statistics from pilot-wave dynamics in a circular corral},
 volume    = {88},
 pages     = {011001(R)(1-5)},
 year      = {2013},
}

@article{bush:ARFM:2015,
 author    = {J. W. M. Bush},
 journal   = {Annu. Rev. Fluid Mech.},
 title     = {Pilot-wave hydrodynamics},
 volume    = {47},
 pages     = {269-292},
 year      = {2015},
}

@article{swinney:PRL:1993,
 author    = {T. H. Solomon and E. R. Weeks and H. L. Swinney},
 journal   = {Phys. Rev. Lett.},
 title     = {Observation of anomalous diffusion and L\'evy flights in a two-dimensional rotating flow},
 volume    = {71},
 pages     = {3975-2978},
 year      = {1993},
}

@article{klafter:PhysToday:1996,
 author    = {J. Klafter and M. F. Shlesinger and G. Zumofen},
 journal   = {Phys. Today},
 title     = {Beyond Brownian motion},
 volume    = {49},
 pages     = {33-39},
 year      = {1996},
}

@article{sanz:JOSAA:2012,
 author    = {A. S. Sanz and J. Campos-Mart{\'\i}nez and S. Miret-Art\'es},
 journal   = {J. Opt. Am. Soc. A},
 title     = {Transmission properties in waveguides: An optical streamline analysis},
 volume    = {29},
 pages     = {695-701},
 year      = {2012},
}

@article{ketterle:Science:1997,
 author    = {M. R. Andrews and C. G. Townsend and H.-J. Miesner and D. S. Durfee and D. M. Kurn and W. Ketterle},
 journal   = {Science},
 title     = {Observation of interference between two Bose condensates},
 volume    = {275},
 pages     = {637-641},
 year      = {1997},
 doi       = {https://doi.org/10.1126/science.275.5300.637}
}

@article{schumm:NaturePhys:2005,
 author    = {T. Schumm and S. Hofferberth and L. M. Andersson and S. Wildermuth and S. Groth and I. Bar-Joseph and J. Schmiedmayer and P. Kr\"uger},
 journal   = {Nature Phys.},
 title     = {Matter-wave interferometry in a double well on an atom chip},
 volume    = {1},
 pages     = {57-62},
 year      = {2005},
}

@article{burnett:PRA:1992,
 author    = {K. Burnett and V. C. Reed and J. Cooper and P. L. Knight},
 journal   = {Phys. Rev. A},
 title     = {Calculation of the background emitted during high-harmonic generation},
 volume    = {45},
 pages     = {3347-3349},
 year      = {1992},
}

@article{spanner:PRL:2003,
 author    = {M. Spanner},
 journal   = {Phys. Rev. Lett.},
 title     = {Strong field tunnel ionization by real-valued classical trajectories},
 volume    = {90},
 pages     = {233005(1-4)},
 year      = {2003},
}

@article{lai:EPJD:2009,
 author    = {X. Y. Lai and Q. Y. Cai and M. S. Zhan},
 journal   = {Eur. Phys. J. D},
 title     = {Above-threshold ionization photoelectron spectrum from quantum trajectory},
 volume    = {53},
 pages     = {393-396},
 year      = {2009},
}

@article{lai:NJP:2009,
 author    = {X. Y. Lai and Q. Y. Cai and M. S. Zhan},
 journal   = {New J. Phys.},
 title     = {From a quantum to a classical description of intense laser-atom physics with Bohmian trajectories},
 volume    = {11},
 pages     = {113035(1-10)},
 year      = {2009},
}

@article{lai:ChinPhysB:2010,
 author    = {X. Y. Lai and Q. Y. Cai and M. S. Zhan},
 journal   = {Chin. Phys. B},
 title     = {Bohmian mechanics to high-order harmonic generation},
 volume    = {19},
 pages     = {020302(1-5)},
 year      = {2010},
}

@article{botheron:PRA:2009,
 author    = {P. Botheron and B. Pons},
 journal   = {Phys. Rev. A},
 title     = {One-electron atom in a strong and short laser pulse: Comparison of classical and quantum descriptions},
 volume    = {80},
 pages     = {023402(1-10)},
 year      = {2009},
}

@article{botheron:PRA-1:2010,
 author    = {P. Botheron and B. Pons},
 journal   = {Phys. Rev. A},
 title     = {Self-consistent Bohmian description of strong field-driven electron dynamics},
 volume    = {82},
 pages     = {021404R(1-4)},
 year      = {2010},
}

@article{botheron:PRA-2:2010,
 author    = {P. Botheron and B. Pons},
 journal   = {Phys. Rev. A},
 title     = {Classical interpretation of probability oscillations in low-energy atomic collisions},
 volume    = {83},
 pages     = {062704(1-11)},
 year      = {2010},
}

@article{takemoto:JCP:2011,
 author    = {N. Takemoto and A. Becker},
 journal   = {J. Chem. Phys.},
 title     = {Visualization and interpretation of attosecond electron dynamics in laser-driven hydrogen molecular ion using Bohmian trajectories},
 volume    = {134},
 pages     = {074309(1-8)},
 year      = {2011},
}

@article{arndt:FoundPhys:2012,
 author    = {T. Juffmann and S. Nimmrichter and M. Arndt and H. Gleiter and K. Hornberger},
 journal   = {Found. Phys.},
 title     = {New prospects for de Broglie interferometry - Grating diffraction in the far-field and Poisson's spot in the near-field},
 volume    = {42},
 pages     = {98-110},
 year      = {2012},
}

@article{arndt:RMP:2012,
 author    = {K. Hornberger and S. Gerlich and P. Haslinger and S. Nimmrichter and M. Arndt},
 journal   = {Rev. Mod. Phys.},
 title     = {Colloquium: Quantum interference of clusters and molecules},
 volume    = {84},
 pages     = {157-173},
 year      = {2012},
}

@article{arndt:NNanotech:2012,
 author    = {T. Juffmann and A. Milic and M. M\"ullneritsch and P. Asenbaum and A. Tsukernik and J. T\"uxen and M. Mayor and O. Cheshnovsky and M. Arndt},
 journal   = {Nat. Nanotech.},
 title     = {Real-time single-molecule imaging of quantum interference},
 volume    = {7},
 pages     = {297-300},
 year      = {2012},
}

@article{carnal:PRL:1991,
 author    = {O. Carnal and J. Mlynek},
 journal   = {Phys. Rev. Lett.},
 title     = {Young's double-slit experiment with atoms: A simple atom interferometer},
 volume    = {66},
 pages     = {2689-2692},
 year      = {1991},
}

@article{cronin:RMP:2009,
 author    = {A. D. Cronin and J. Schmiedmayer and D. E. Pritchard},
 journal   = {Rev. Mod. Phys.},
 title     = {Optics and interferometry with atoms and molecules},
 volume    = {81},
 pages     = {1051-1129},
 year      = {2009},
}

@article{brabec:RMP:2000,
 author    = {Th. Brabec and F. Krausz},
 journal   = {Rev. Mod. Phys.},
 title     = {Intense few-cycle laser fields: Frontiers of nonlinear optics},
 volume    = {72},
 pages     = {545-591},
 year      = {2000},
}

@article{ganeev:JPhysB:2007,
 author    = {R. A. Ganeev},
 journal   = {J. Phys. B: At. Mol. Opt. Phys.},
 title     = {High-order harmonic generation in a laser plasma: a review of recent achievements},
 volume    = {40},
 pages     = {R213-R253},
 year      = {2007},
}

@article{midorikawa:JJAP:2011,
 author    = {K. Midorikawa},
 journal   = {Jpn. J. Appl. Phys.},
 title     = {High-order harmonic generation and attosecond science},
 volume    = {50},
 pages     = {090001(1-12)},
 year      = {2011},
}

@article{corkum:PRL:1993,
 author    = {P. B. Corkum},
 journal   = {Phys. Rev. Lett.},
 title     = {Plasma perspective on strong field multiphoton ionization},
 volume    = {71},
 pages     = {1994-1997},
 year      = {1993},
}

@article{lewenstein:PRA:1994,
 author    = {M. Lewenstein and Ph. Balcou and M. Yu. Ivanov and A. L'Huillier and P. B. Corkum},
 journal   = {Phys. Rev. A},
 title     = {Theory of high-harmonic generation by low-frequency laser fields},
 volume    = {49},
 pages     = {2117-},
 year      = {1994},
}

@article{altucci:JModOpt:2012,
 author    = {C. Altucci and J. W. G. Tisch and R. Velotta},
 journal   = {J. Mod. Opt.},
 title     = {Single attosecond light pulses from multi-cycle laser sources},
 volume    = {58},
 pages     = {1585-1610},
 year      = {2011},
}

@article{aharonov:PRA:1990,
 author    = {Y. Aharonov and L. Vaidman},
 journal   = {Phys. Rev. A},
 title     = {Properties of a quantum system during the time interval between two measurements},
 volume    = {41},
 pages     = {11-20},
 year      = {1990},
}

@article{hiley:JPhysConfSer:2012,
 author    = {B. J. Hiley},
 journal   = {J. Phys.: Conf. Ser.},
 title     = {Weak values: Approach through the Clifford and Moyal algebras},
 volume    = {361},
 pages     = {012014},
 year      = {2012},
}

@article{work-in-progress:2012,
 author    = {A. S. Sanz and J. Wu and B. B. Augstein and C. Figueira de Morisson Faria},
 journal   = {Phys. Rev. A},
 title     = {Quantum-classical correspondence in the high-order harmonic generation},
 volume    = {},
 pages     = {},
 year      = {work in progress, 2012},
}

@article{ghose:PLA:2001,
 author    = {P. Ghose and A. S. Majumdar and S. Guhab and J. Sau},
 journal   = {Phys. Lett. A},
 title     = {Bohmian trajectories for photons},
 volume    = {290},
 pages     = {205-213},
 year      = {2001},
 doi       = {10.1016/S0375-9601(01)00677-6},
 url       = {https://doi.org/10.1016/S0375-9601(01)00677-6},
}

@article{kogelnik:ProcIEEE:1966,
 author    = {H. Kogelnik and T. Li},
 journal   = {Proc. IEEE},
 title     = {Laser beams and resonators},
 volume    = {54},
 pages     = {1312-1329},
 year      = {1966},
}

@article{mukunda:JOSAA:1985,
 author    = {N. Mukunda and R. Simon and E. C. G. Sudarshan},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Fourier optics for the Maxwell field: Formalism and applications},
 volume    = {2},
 pages     = {416-426},
 year      = {1985},
}

@article{mukunda:JOSAA:1986,
 author    = {R. Simon and E. C. G. Sudarshan and N. Mukunda},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Gaussian-Maxwell beams},
 volume    = {3},
 pages     = {536-540},
 year      = {1986},
}

@article{mukunda:ApplOpt:1987,
 author    = {N. Mukunda and R. Simon and E. C. G. Sudarshan},
 journal   = {Appl. Opt.},
 title     = {Cross polarization in laser beams},
 volume    = {26},
 pages     = {1589-1593},
 year      = {1987},
}

@article{seshadri:JOSAA:1998,
 author    = {S. R. Seshadri},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Electromagnetic Gaussian beam},
 volume    = {15},
 pages     = {2712-2719},
 year      = {1998},
}

@article{mcdonald:notes:2000,
 author    = {K. T. McDonald},
 journal   = {Notes},
 title     = {Gaussian laser beams with radial polarization},
 volume    = {},
 pages     = {1-12},
 year      = {2000},
}

@article{mcdonald:notes:2009-1,
 author    = {K. T. McDonald},
 journal   = {Notes},
 title     = {Second-order paraxial Gaussian beam},
 volume    = {},
 pages     = {1-5},
 year      = {2009},
}

@article{mcdonald:notes:2009-2,
 author    = {K. T. McDonald},
 journal   = {Notes},
 title     = {Reflection of a Gaussian optical beam by a flat mirror},
 volume    = {},
 pages     = {1-12},
 year      = {2009},
}

@article{davis:PRA:1979,
 author    = {L. W. Davis},
 journal   = {Phys. Rev. A},
 title     = {Theory of electromagnetic beams},
 volume    = {19},
 pages     = {1177-1179},
 year      = {1979},
}

@article{barnett:PhilTRSA:2010,
 author    = {S. M. Barnett and R. Loudon},
 journal   = {Phil. Trans. R. Soc. A},
 title     = {The enigma of optical momentum in a medium},
 volume    = {368},
 pages     = {927-939},
 year      = {2010},
}

@article{dahmen:AnnPhys:1998,
 author    = {H. D. Dahmen and E. Gjonaj and T. Stroh},
 journal   = {Ann. Phys. (Leipzig)},
 title     = {Quantile motion of electromagnetic waves in wave guides of varying cross section and dispersive media},
 volume    = {7},
 pages     = {645-653},
 year      = {1998},
}

@article{hesse:JQSRT:2008,
 author    = {E. Hesse},
 journal   = {JQSRT},
 title     = {Modelling diffraction during ray tracing using the concept of energy flow lines},
 volume    = {109},
 pages     = {1374-1383},
 year      = {2008},
}

@article{wyatt:PhysScr:2011,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {Phys. Scr.},
 title     = {Hydrodynamic view of electrodynamics: Energy rays and electromagnetic effective stress},
 volume    = {83},
 pages     = {065403(1-10)},
 year      = {2011},
}

@article{sadreev:PRE:2004,
 author    = {A. F. Sadreev},
 journal   = {Phys. Rev. E},
 title     = {Current statistics for transport through rectangular and circular billiards},
 volume    = {70},
 pages     = {016208(1-7)},
 year      = {2004},
}

@article{sadreev:PRB:2012,
 author    = {E. N. Bulgakov and A. F. Sadreev},
 journal   = {Phys. Rev. B},
 title     = {Giant optical vortex in photonic crystal waveguide with nonlinear optical cavity},
 volume    = {85},
 pages     = {165305(1-6)},
 year      = {2012},
}

@article{zakowicz:PRE:2001,
 author    = {W. \.Zakowicz},
 journal   = {Phys. Rev. E},
 title     = {Light rays and imaging in wave optics},
 volume    = {64},
 pages     = {066610(1-14)},
 year      = {2001},
}

@article{wang:PRB:2004,
 author    = {Z. B. Wang and B. S. Luk'yanchuk and M. H. Hong and Y. Lin and T. C. Chong},
 journal   = {Phys. Rev. B},
 title     = {Energy flow around a small particle investigated by classical Mie theory},
 volume    = {70},
 pages     = {035418(1-12)},
 year      = {2004},
}

@article{lee:AppPhysLett:2007,
 author    = {B. J. Lee and K. Park and Z. M. Zhang},
 journal   = {Appl. Phys. Lett.},
 title     = {Energy pathways in nanoscale thermal radiation},
 volume    = {91},
 pages     = {153101(1-3)},
 year      = {2007},
}

@article{godin:JAcoustSocAm:2009,
 author    = {O. A. Godin},
 journal   = {Appl. Phys. Lett.},
 title     = {Wave refraction at an interface: Snell's law versus Chapman's law},
 volume    = {125},
 pages     = {EL117-EL122},
 year      = {2009},
}

@article{gondran:AJP:2010,
 author    = {M. Gondran and A. Gondran},
 journal   = {Am. J. Phys.},
 title     = {Energy flow lines and the spot of Poisson-Arago},
 volume    = {78},
 pages     = {598-602},
 year      = {2010},
}

@article{holland:ProcRSocA:2005,
 author    = {P. Holland},
 journal   = {Proc. R. Soc. A},
 title     = {Hydrodynamic construction of the electromagnetic field},
 volume    = {461},
 pages     = {3659-3679},
 year      = {2005},
}

@article{erikson:PRE:1994,
 author    = {W. L. Erikson and S. Singh},
 journal   = {Phys. Rev. E},
 title     = {Polarization properties of Maxwell-Gaussian laser beams},
 volume    = {49},
 pages     = {5778-5786},
 year      = {1994},
}

@article{varga:OptCommun:1998,
 author    = {P. Varga and P. T\"{o}r\"{o}k},
 journal   = {Opt. Commun.},
 title     = {The Gaussian wave solution of Maxwell's equations and the validity of scalar wave approximation},
 volume    = {152},
 pages     = {108-118},
 year      = {1998},
}

@article{heller:JCP:1975,
 author    = {E. J. Heller},
 journal   = {J. Chem. Phys.},
 title     = {Time-dependent approach to semiclassical dynamics},
 volume    = {62},
 pages     = {1544-1555},
 year      = {1975},
}

@article{heller:JCP:1981,
 author    = {E. J. Heller},
 journal   = {J. Chem. Phys.},
 title     = {Frozen Gaussians: A very simple semiclassical approximation},
 volume    = {75},
 pages     = {2923-2931},
 year      = {1981},
}

@article{caldirola:NuovoCim:1941,
 author    = {P. Caldirola},
 journal   = {Nuovo cim.},
 title     = {Forze non conservative nella meccanica quantistica},
 volume    = {18},
 pages     = {393-400},
 year      = {1941},
}

@article{kanai:ProgTheorPhys:1948,
 author    = {E. Kanai},
 journal   = {Prog. Theor. Phys.},
 title     = {On the quantization of the dissipative systems},
 volume    = {3},
 pages     = {440-442},
 year      = {1948},
}

@article{caldeira:AnnPhys:1983,
 author    = {A. O. Caldeira and A. J. Leggett},
 journal   = {Ann. Phys. (NY)},
 title     = {Quantum tunneling in a dissipative system},
 volume    = {149},
 pages     = {374-456},
 year      = {1983},
}

@article{caldeira:PhysicaA:1983,
 author    = {A. O. Caldeira and A. J. Leggett},
 journal   = {Physica A},
 title     = {Path integral approach to quantum Brownian motion},
 volume    = {121},
 pages     = {587-616},
 year      = {1983},
}

@BOOK{razavy-bk,
  AUTHOR     = {M. Razavy},
  TITLE      = {Classical and Quantum Dissipative Systems},
  PUBLISHER  = {Imperial College Press},
  YEAR       = {2005},
  address    = {London},
}

@BOOK{morse-bk-1,
  AUTHOR     = {P. M. Morse and H. Feshbach},
  TITLE      = {Methods of Theoretical Physics},
  PUBLISHER  = {McGraw-Hill},
  YEAR       = {1953},
  address    = {New York},
  volume     = {1},
}

@BOOK{morse-bk-2,
  AUTHOR     = {P. M. Morse and H. Feshbach},
  TITLE      = {Methods of Theoretical Physics},
  PUBLISHER  = {McGraw-Hill},
  YEAR       = {1953},
  address    = {New York},
  volume     = {2},
}

@article{gouy:CRASP:1890,
 author    = {L. G. Gouy},
 journal   = {C. R. Acad. Sci. Paris},
 title     = {Sur une propri\'et\'e nouvelle des ondes lumineuses},
 volume    = {110},
 pages     = {1251},
 year      = {1890},
}

@article{gouy:CompRend:1890,
 author    = {L. G. Gouy},
 journal   = {Compt. Rendue. Acad. Sci. Paris},
 title     = {Sur la propagation anomale des ondes},
 volume    = {111},
 pages     = {33},
 year      = {1890},
}

@article{gouy:ACOS:1891,
 author    = {L. G. Gouy},
 journal   = {Ann. Chim. Phys. Ser. 6},
 title     = {Sur la propagation anomale des ondes},
 volume    = {24},
 pages     = {145},
 year      = {1891},
}

@article{boyd:JOSA:1980,
 author    = {R. W. Boyd},
 journal   = {J. Opt. Soc. Am.},
 title     = {Intuitive explanation of the phase anomaly of focused light beams},
 volume    = {70},
 pages     = {877-880},
 year      = {1980},
}

@article{rubinowicz:PhysRev:1938,
 author    = {A. Rubinowicz},
 journal   = {Phys. Rev.},
 title     = {On the anomalous propagation of phase in the focus},
 volume    = {54},
 pages     = {931-936},
 year      = {1938},
}

@article{paschotta:OptExpr:2006,
 author    = {R. Paschotta},
 journal   = {Opt. Express},
 title     = {Beam quality deterioration of lasers caused by intracavity beam distortions},
 volume    = {14},
 pages     = {6069-6074},
 year      = {2006},
}

@article{feng:OptLett:2001,
 author    = {S. Feng and H. G. Winful},
 journal   = {Opt. Express},
 title     = {Physical origin of the Gouy phase shift},
 volume    = {26},
 pages     = {485-487},
 year      = {2001},
}

@article{visser:OptCommun:2010,
 author    = {T. D. Visser and E. Wolf},
 journal   = {Opt. Commun.},
 title     = {The origin of the Gouy phase anomaly and its generalization to astigmatic wavefields},
 volume    = {283},
 pages     = {3371-3375},
 year      = {2010},
}

@article{sanz:EPJD:2007,
 author    = {A. S. Sanz and F. Borondo},
 journal   = {Eur. Phys. J. D},
 title     = {A quantum trajectory description of decoherence},
 volume    = {44},
 pages     = {319-326},
 year      = {2007},
 url       = {https://doi.org/10.1140/epjd/e2007-00191-8},
 doi       = {10.1140/epjd/e2007-00191-8},
}

@article{sanz:CPL:2009-2,
 author    = {A. S. Sanz and F. Borondo},
 journal   = {Chem. Phys. Lett.},
 title     = {Contextuality, decoherence and quantum trajectories},
 volume    = {478},
 pages     = {301-306},
 year      = {2009},
 doi       = {10.1016/j.cplett.2009.07.061},
 url       = {https://www.sciencedirect.com/science/article/pii/S0009261409009038},
}

@article{vink:PRA:1993,
 author    = {J. C. Vink},
 journal   = {Phys. Rev. A},
 title     = {Quantum mechanics in terms of discrete beables},
 volume    = {48},
 pages     = {1808-1818},
 year      = {1993},
}

@article{lorenzen:PRA:2009,
 author    = {F. Lorenzen and M. A. de Ponte and M. H. Y. Moussa},
 journal   = {Phys. Rev. A},
 title     = {Extending Bell's beables to encompass dissipation, decoherence, and the quantum-to-classical transition through quantum trajectories},
 volume    = {80},
 pages     = {032101(1-8)},
 year      = {2009},
}

@article{vandyck:JPA:1994,
 author    = {M. A. Vandyck},
 journal   = {J. Phys. A: Math. Gen.},
 title     = {On the damped harmonic oscillator in the de Broglie-Bohm hidden-variable theory},
 volume    = {27},
 pages     = {1743-1750},
 year      = {1994},
}

@article{shojai:PRAMANA:2004,
 author    = {F. Shojai and A. Shojai},
 journal   = {PRAMANA},
 title     = {On the Bohmian quantum friction},
 volume    = {62},
 pages     = {803-814},
 year      = {2004},
}

@article{tilbi:PhysScr:2007,
 author    = {A. Tilbi and T. Boudjedaa and M. Merad and L. Chetouani},
 journal   = {Phys. Scr.},
 title     = {The Kanai-Caldirola propagator in the de Broglie-Bohm theory},
 volume    = {75},
 pages     = {474-479},
 year      = {2007},
}

@article{garashchuk:JCP:2013,
 author    = {S. Garashchuk and V. Dixit and B. Gu and J. Mazzuca},
 journal   = {J. Chem. Phys.},
 title     = {The Schr\"odinger equation with friction from the quantum trajectory perspective},
 volume    = {138},
 pages     = {054107(1-7)},
 year      = {2013},
}

@article{garashchuk:TheorChemAcc:2012,
 author    = {S. Garashchuk},
 journal   = {Theor. Chem. Acc.},
 title     = {Calculation of the zero-point energy from imaginary-time quantum trajectory dynamics in Cartesian coordinates},
 volume    = {131},
 pages     = {1083(1-10)},
 year      = {2012},
}

@article{bowman:JCP:2011,
 author    = {G. Czak\'o and Y. Wang and J. M. Bowman},
 journal   = {J. Chem. Phys.},
 title     = {Communication: Quasiclassical trajectory calculations of correlated product-state distributions for the dissociation of (H$_2$O)$_2$ and (D$_2$O)$_2$},
 volume    = {135},
 pages     = {151102(1-4},
 year      = {2011},
}

@BOOK{weiss-bk,
  AUTHOR     = {U. Weiss},
  TITLE      = {Quantum Dissipative Systems},
  PUBLISHER  = {World Scientific},
  YEAR       = {1999},
  address    = {Singapore},
}

@article{hakim:prl:1985,
 author    = {F. Guinea and V. Hakim and A. Muramatsu},
 journal   = {Phys. Rev. Lett.},
 title     = {Diffusion and localization of a particle in a periodic potential coupled to a dissipative environment},
 volume    = {54},
 pages     = {263-266},
 year      = {1985},
}

@article{fisher:prb:1985,
 author    = {M. P. A. Fisher and W. Zwerger},
 journal   = {Phys. Rev. B},
 title     = {Quantum Brownian motion in a periodic potential},
 volume    = {32},
 pages     = {6190-6206},
 year      = {1985},
}

@article{zurek:prd:1989,
 author    = {W. G. Unruh and W. H. Zurek},
 journal   = {Phys. Rev. D},
 title     = {Reduction of a wave packet in quantum Brownian motion},
 volume    = {40},
 pages     = {1071-1094},
 year      = {1989},
}

@article{doebner:pla:1992,
 author    = {H.-D. Doebner and G. A. Goldin},
 journal   = {Phys. Lett. A},
 title     = {On a general nonlinear Schr\"odinger equation admitting diffusion currents},
 volume    = {162},
 pages     = {397-401},
 year      = {1992},
}

@article{kostin:jcp:1972,
 author    = {M. D. Kostin},
 journal   = {J. Chem. Phys.},
 title     = {On the Schr\"odinger-Langevin equation},
 volume    = {57},
 pages     = {3589-3591},
 year      = {1972},
}

@article{kochan:pra:2010,
 author    = {D. Kochan},
 journal   = {Phys. Rev. A},
 title     = {Functional integral for non-Lagrangian systems},
 volume    = {81},
 pages     = {022112(1-13)},
 year      = {2010},
}

@article{bateman:PhysRev:1931,
 author    = {H. Bateman},
 journal   = {Phys. Rev.},
 title     = {On dissipative systems and related variational principles},
 volume    = {38},
 pages     = {815-819},
 year      = {1931},
}

@article{brittin:PhysRev:1950,
 author    = {W. E. Brittin},
 journal   = {Phys. Rev.},
 title     = {A note on the quantization of dissipative systems},
 volume    = {77},
 pages     = {396-397},
 year      = {1950},
}

@article{senitzky:PhysRev:1960,
 author    = {I. R. Senitzky},
 journal   = {Phys. Rev.},
 title     = {Dissipation in quantum mechanics. The harmonic oscillator},
 volume    = {119},
 pages     = {670-679},
 year      = {1960},
}

@article{greenberger:JMathPhys:1979,
 author    = {D. M. Greenberger},
 journal   = {J. Math. Phys.},
 title     = {A critique of the major approaches to damping in quantum theory},
 volume    = {20},
 pages     = {762-770},
 year      = {1979},
}

@article{cavalcanti:PRE:1998,
 author    = {R. M. Cavalcanti},
 journal   = {Phys. Rev. E},
 title     = {Wave function of a Brownian particle},
 volume    = {58},
 pages     = {6807-6809},
 year      = {1998},
}

@article{hasse:JMathPhys:1975,
 author    = {R. W. Hasse},
 journal   = {J. Math. Phys.},
 title     = {On the quantum mechanical treatment of dissipative systems},
 volume    = {16},
 pages     = {2005-2011},
 year      = {1975},
}

@article{holst:PRA:2009,
 author    = {T. Resinger and A. A. Patel and H. Reingruber and K. Fladischer and W. E. Ernst and G. Bracco and H. I. Smith and B. Holst},
 journal   = {Phys. Rev. A},
 title     = {Poisson's spot with molecules},
 volume    = {79},
 pages     = {053823(1-4)},
 year      = {2009},
}

@article{holst:PRA:2012,
 author    = {T. Resinger and M. M. Greve and S. D. Eder and G. Bracco and B. Holst},
 journal   = {Phys. Rev. A},
 title     = {Brightness and virtual source size of a supersonic deuterium beam},
 volume    = {86},
 pages     = {043804(1-10)},
 year      = {2012},
}

@article{holst:NJP:2011,
 author    = {T. Resinger and G. Bracco and B. Holst},
 journal   = {New J. Phys},
 title     = {Particle-wave discrimination in Poisson spot experiments},
 volume    = {13},
 pages     = {065016(1-13)},
 year      = {2011},
}

@INBOOK{joos:bk:1996,
  AUTHOR =       {E. Joos},
  editor =       {D. Giulini and E. Joos and C. Kiefer and J. Kupsch and I.-O. Stamatescu and H. D. Zeh},
  TITLE =        {Decoherence and the Appearance of a Classical World in Quantum Theory},
  CHAPTER =      {Decoherence through interaction with the environment},
  pages =        {41-180},
  PUBLISHER =    {Springer},
  YEAR =         {1996},
  address =      {Berlin},
  edition =      {2nd},
}

@BOOK{giulini-bk,
  AUTHOR     = {D. Giulini and E. Joos and C. Kiefer and J. Kupsch and I.-O. Stamatescu and H. D. Zeh},
  TITLE      = {Decoherence and the Appearance of a Classical World in Quantum Theory},
  PUBLISHER  = {Springer},
  YEAR       = {Berlin},
  address    = {1996},
  edition    = {2nd},
}

@BOOK{schlosshauer-bk:2007,
  AUTHOR     = {M. Schlosshauer},
  TITLE      = {Decoherence and the Quantum-to-Classical Transition},
  PUBLISHER  = {Springer},
  YEAR       = {2007},
  address    = {Berlin},
}

@article{miller:JCP-1:2001,
 author    = {H. Wang and M. Thoss and K. L. Sorge and R. Gelabert and X. Gim\'enez and W. H. Miller},
 journal   = {J. Chem. Phys.},
 title     = {Semiclassical description of quantum coherence effects and their quenching: A forward-backward initial value representation study},
 volume    = {114},
 pages     = {2562-2571},
 year      = {2001},
}

@article{miller:JCP-2:2001,
 author    = {R. Gelabert and X. Gim\'enez and M. Thoss and H. Wang and W. H. Miller},
 journal   = {J. Chem. Phys.},
 title     = {Semiclassical description of diffraction and its quenching by the forward-backward version of the initial value representation},
 volume    = {114},
 pages     = {2572-2579},
 year      = {2001},
}

@article{miller:JCP:2012,
 author    = {W. H. Miller},
 journal   = {J. Chem. Phys.},
 title     = {Perspective: Quantum or classical decoherence?},
 volume    = {136},
 pages     = {210901(1-6)},
 year      = {2012},
}

@article{miller:JCP:1970,
 author    = {W. H. Miller},
 journal   = {J. Chem. Phys.},
 title     = {Classical $S$ matrix: Numerical application to inelastic collisions},
 volume    = {53},
 pages     = {3578-3587},
 year      = {1970},
}

@article{miller:FaradayDiscuss:1998,
 author    = {W. H. Miller},
 journal   = {Faraday Discuss.},
 title     = {Quantum and semiclassical theory of chemical reaction rates},
 volume    = {110},
 pages     = {1-21},
 year      = {1998},
}

@article{caldeira:Physica:1983,
 author    = {A. O. Caldeira and A. J. Leggett},
 journal   = {Physica},
 title     = {Path integral approach to quantum Brownian motion},
 volume    = {121A},
 pages     = {587-616},
 year      = {1983},
}

@article{caldeira:AnnPhys:1983,
 author    = {A. O. Caldeira and A. J. Leggett},
 journal   = {Ann. Phys},
 title     = {Quantum tunnelling in a dissipative system},
 volume    = {149},
 pages     = {374-456},
 year      = {1983},
}

@article{caldeira:AnnPhys:1984,
 author    = {A. O. Caldeira and A. J. Leggett},
 journal   = {Ann. Phys.},
 title     = {Erratum to `Quantum tunnelling in a dissipative system'},
 volume    = {153},
 pages     = {445},
 year      = {1984},
}

@BOOK{percival-bk,
  AUTHOR     = {I. C. Percival},
  TITLE      = {Quantum State Diffusion},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {1998},
  address    = {Cambridge},
}

@article{gisin:JPA:1992,
 author    = {N. Gisin and I. C. Percival},
 journal   = {J. Phys. A},
 title     = {The quantum-state diffusion model applied to open systems},
 volume    = {25},
 pages     = {5677-5691},
 year      = {1992},
}

@article{gisin:JPA:1993,
 author    = {N. Gisin and I. C. Percival},
 journal   = {J. Phys. A},
 title     = {The quantum state diffusion picture of physical processes},
 volume    = {26},
 pages     = {2245-2260},
 year      = {1993},
}

@article{gisin:JModOpt:1993,
 author    = {N. Gisin and P. L. Knight and I. C. Percival and R. C. Thompson and D. C. Wilson},
 journal   = {J. Mod. Opt.},
 title     = {Quantum state diffusion theory and a quantum jump experiment},
 volume    = {40},
 pages     = {1663-1671},
 year      = {1993},
}

@BOOK{ito-bk,
  AUTHOR     = {K. It\^o},
  TITLE      = {Foundations of Stochastic Differential Equations in Infinite Dimensional Spaces},
  PUBLISHER  = {SIAM},
  YEAR       = {1984},
  address    = {Philadelphia, PA},
}

@BOOK{ikeda-bk,
  AUTHOR     = {N. Ikeda and S. Watanabe},
  TITLE      = {Stochastic Differential Equations and Diffusion Processes},
  PUBLISHER  = {North-Holland},
  YEAR       = {Amsterdam},
  address    = {1989},
  edition    = {2nd},
}

@article{diosi:JPA:1988,
 author    = {L. Di\'osi},
 journal   = {J. Phys. A},
 title     = {Quantum stochastic processes as models for state vector reduction},
 volume    = {21},
 pages     = {2885-2898},
 year      = {1988},
}

@article{diosi:PLA:1988,
 author    = {L. Di\'osi},
 journal   = {Phys. Lett. A},
 title     = {Continuous quantum measurement and It\^o formalism},
 volume    = {129},
 pages     = {419-423},
 year      = {1988},
}

@article{diosi:ChemPhys:2001,
 author    = {H. M. Wiseman and L. Di\'osi},
 journal   = {Chem. Phys.},
 title     = {Complete parameterization, and invariance, of diffusive quantum trajectories for Markovian open systems},
 volume    = {268},
 pages     = {91-104},
 year      = {2001},
}

@BOOK{accardi-bk,
  AUTHOR     = {L. Accardi and Y. G. Lu and I. Volovich},
  TITLE      = {Quantum Theory and its Stochastic Limit},
  PUBLISHER  = {Springer},
  YEAR       = {2002},
  address    = {Berlin},
}

@BOOK{NumRecipes-bk,
  AUTHOR     = {W. H. Press and S. A. Teukolsky and W. T. Vetterling and B. P. Flannery},
  TITLE      = {Numerical Recipes: The Art of Scientific Computing},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {2007},
  address    = {New York},
  edition    = {3rd},
}

\bibitem{Prezhdo}
 O.V. Prezhdo, Phys. Rev. Lett. {\bf 85}, 4413 (2000).

\bibitem{Han}
 H. Han and P. Brumer, J. Chem. Phys. {\bf 122}, 144316 (2005).


@article{brumer-gong:PRE:1999,
 author    = {J. Gong and P. Brumer},
 journal   = {Phys. Rev. E},
 title     = {Decoherence and correspondence in conservative chaotic dynamics},
 volume    = {60},
 pages     = {1643-1647},
 year      = {1999},
}

@article{prezhdo:PRL:2000,
 author    = {O. V. Prezhdo},
 journal   = {Phys. Rev. Lett.},
 title     = {Quantum anti-Zeno acceleration of a chemical reaction},
 volume    = {85},
 pages     = {4413-4417},
 year      = {2000},
}

@article{brumer-han:JCP:2005,
 author    = {H. Han and P. Brumer},
 journal   = {J. Chem. Phys.},
 title     = {Decoherence effects in reactive scattering},
 volume    = {122},
 pages     = {144316(1-8)},
 year      = {2005},
}

@article{klauder:SIAM:1985,
 author    = {J. R. Klauder and W. P. Petersen},
 journal   = {SIAM J. Numer. Anal.},
 title     = {Numerical integration of multiplicative-noise stochastic differential equations},
 volume    = {22},
 pages     = {1153-1166},
 year      = {1985},
}

@BOOK{carmichael-bk,
  AUTHOR     = {H. Carmichael},
  TITLE      = {An Open Systems Approach to Quantum Optics},
  PUBLISHER  = {Springer},
  YEAR       = {1993},
  address    = {Berlin},
}

@article{sanz:PRE:2012,
 author    = {A. S. Sanz and Y. Elran and P. Brumer},
 journal   = {Phys. Rev. E},
 title     = {Temperature crossover of decoherence rates in chaotic and regular bath dynamics},
 volume    = {85},
 pages     = {036218(1-6)},
 year      = {2012},
}

@article{brumer-elran:JCP:2013,
 author    = {Y. Elran and P. Brumer},
 journal   = {J. Chem. Phys.},
 title     = {Quantum decoherence of I$_2$ in liquid xenon: A classical Wigner approach},
 volume    = {138},
 pages     = {234308(1-11)},
 year      = {2013},
}

@article{brumer-elran:JCP:2004,
 author    = {Y. Elran and P. Brumer},
 journal   = {J. Chem. Phys.},
 title     = {Decoherence in an anharmonic oscillator coupled to a thermal environment: A semiclassical forward-backward approach},
 volume    = {121},
 pages     = {2673-2684},
 year      = {2004},
}

@article{joos-zeh:ZPhysB:1985,
 author    = {E. Joos and H. D. Zeh},
 journal   = {Z. Phys. B},
 title     = {The emergence of classical properties through interaction with the environment},
 volume    = {59},
 pages     = {223-243},
 year      = {1985},
}

@article{muendel:ChemPhys:1986,
 author    = {C. M\"undel and W. Domcke},
 journal   = {Chem. Phys.},
 title     = {Analytic expression for the matrix elements of the Morse Green function with Morse wavefunctions},
 volume    = {105},
 pages     = {137-143},
 year      = {1989},
}

@article{morse:PhysRev:1929,
 author    = {P. M. Morse},
 journal   = {Phys. Rev.},
 title     = {Diatomic molecules according to the wave mechanics. II. Vibrational levels},
 volume    = {34},
 pages     = {57-64},
 year      = {1929},
 doi       = {10.1103/PhysRev.34.57},
}

@article{zurek:PRL:1993,
 author    = {W. H. Zurek and S. Habib and J. P. Paz},
 journal   = {Phys. Rev. Lett.},
 title     = {Coherent states via decoherence},
 volume    = {70},
 pages     = {1187-1190},
 year      = {1993},
}

@article{sanz:JCP:2006,
 author    = {A. S. Sanz and H. Han and P. Brumer},
 journal   = {J. Chem. Phys.},
 title     = {Aspects of quantum coherence in the optical Bloch equations},
 volume    = {124},
 pages     = {214106(1-7)},
 year      = {2006},
}

@article{pollak:JCP:2009,
 author    = {E. Pollak and S. Miret-Art\'es},
 journal   = {J. Chem. Phys.},
 title     = {Classical theory for the in-plane scattering of atoms from corrugated surfaces: Application to the Ar-Ag(111) system},
 volume    = {130},
 pages     = {194710(1-13},
 year      = {2009},
}

@article{pollak:PRL:2010,
 author    = {J. M. Moix and E. Pollak and S. Miret-Art\'es},
 journal   = {Phys. Rev. Lett.},
 title     = {Friction-induced energy-loss rainbows in atom surface scattering},
 volume    = {104},
 pages     = {116103(1-4},
 year      = {2010},
}

@article{hornberger:PRL:2003,
 author    = {K. Hornberger and S. Uttenthaler and B. Brezger and L. Hackerm\"uller and M. Arndt and A. Zeilinger},
 journal   = {Phys. Rev. Lett.},
 title     = {Collisional decoherence observed in matter-wave interferometry},
 volume    = {90},
 pages     = {160401(1-4)},
 year      = {2003},
}

@article{fischbach:PRA:2012,
 author    = {J. Fischbach and M. Freyberger},
 journal   = {Phys. Rev. A},
 title     = {Quantum optical reconstruction scheme using weak values},
 volume    = {86},
 pages     = {052110(1-8)},
 year      = {2012},
}

@article{bliokh:NewJPhys:2013,
 author    = {K. Y. Bliokh and A. Y. Bekshaev and A. G. Kofman and F. Nori},
 journal   = {New J. Phys.},
 title     = {Photon trajectories, anomalous velocities and weak measurements: a classical interpretation},
 volume    = {15},
 pages     = {073022(1-17)},
 year      = {2013},
}

@article{schleich:PRA:2013,
 author    = {W. P. Schleich and M. Freyberger and M. S. Zubairy},
 journal   = {Phys. Rev. A},
 title     = {Reconstruction of Bohm trajectories and wave functions from interferometric measurements},
 volume    = {87},
 pages     = {014102(1-4)},
 year      = {2013},
}

@article{matzkin:PRL:2012,
 author    = {A. Matzkin},
 journal   = {Phys. Rev. Lett.},
 title     = {Observing trajectories with weak measurements in quantum systems in the semiclassical regime},
 volume    = {109},
 pages     = {150407(1-4)},
 year      = {2012},
}

@article{luis:PRA:2013,
 author    = {A. Luis and A. S. Sanz},
 journal   = {Phys. Rev. A},
 title     = {Reconciling quantum trajectories and stationary quantum distributions in single-photon polarization states},
 volume    = {87},
 pages     = {063844(1-8)},
 year      = {2013},
}

@article{lundeen:Nature:2011,
 author    = {J. S. Lundeen and B. Sutherland and Aabid Patel and C. Stewart and Ch. Bamber},
 journal   = {Nature},
 title     = {Direct measurement of the quantum wavefunction},
 volume    = {474},
 pages     = {188-191},
 year      = {2011},
}

@article{aharonov:PRL:1988,
 author    = {Y. Aharonov and D. Z. Albert and L. Vaidman},
 journal   = {Phys. Rev. Lett.},
 title     = {How the result of a measurement of a component of the spin of a spin$-$$\frac{1}{2}$ particle can turn out to be 100},
 volume    = {60},
 pages     = {1351-1354},
 year      = {1988},
}

@article{dressel:RMP:2013,
 author    = {J. Dressel and M. Malik and F. M. Miatto and A. N. Jordan and R. W. Boyd},
 journal   = {Rev. Mod. Phys.},
 title     = {Colloquium: Understanding quantum weak values: Basics and applications},
 volume    = {86},
 pages     = {307-316},
 year      = {2014},
}

@article{wiseman:NewJPhys:2007,
 author    = {H. M. Wiseman},
 journal   = {New J. Phys.},
 title     = {Grounding Bohmian mechanics in weak values and bayesianism},
 volume    = {9},
 pages     = {165(1-12)},
 year      = {2007},
}

@article{mir:NewJPhys:2007,
 author    = {R. Mir and J. S. Lundeen and M. W. Mitchell and A. M. Steinberg and J. L. Garretson and H. M. Wiseman},
 journal   = {New J. Phys.},
 title     = {A double-slit `which-way' experiment on the complementarity-uncertainty debate},
 volume    = {9},
 pages     = {287(1-11)},
 year      = {2007},
}

@article{hirschfelder:JCP:1978,
 author    = {J. O. Hirschfelder},
 journal   = {J. Chem. Phys.},
 title     = {Quantum mechanical equations of change. I},
 volume    = {68},
 pages     = {5151-5162},
 year      = {1978},
}

@article{leavens:FoundPhys:2005,
 author    = {C. R. Leavens},
 journal   = {Found. Phys.},
 title     = {Weak measurements from the point of view of Bohmian mechanics},
 volume    = {35},
 pages     = {469-491},
 year      = {2005},
}

@article{sanz:PhysScr:2013,
 author    = {M. Davidovi\'c and A. S. Sanz and M. Bo\v{z}i\'c and D. Arsenovi\'c and D. Dimi\'c},
 journal   = {Phys. Scr.},
 pages     = {014015(1-5)},
 title     = {Trajectory-based interpretation of Young's experiment, the Arago-Fresnel laws and the Poisson-Arago spot for photons and massive particles},
 volume    = {T153},
 year      = {2013},
 }

@article{ritchie:PRL:1991,
 author    = {N. W. M. Ritchie and J. G. Story and R. G. Hulet},
 journal   = {Phys. Rev. Lett.},
 title     = {Realization of a measurement of a ``weak value''},
 volume    = {66},
 pages     = {1107-1110},
 year      = {1991},
}

@article{bamber:PRL:2012,
 author    = {J. S. Lundeen and Ch. Bamber},
 journal   = {Phys. Rev. Lett.},
 title     = {Procedure for direct measurement of general quantum states using weak measurements},
 volume    = {108},
 pages     = {070402(1-5)},
 year      = {2012},
}

@article{bamber:PRL:2013,
 author    = {Ch. Bamber and J. S. Lundeen},
 journal   = {Phys. Rev. Lett.},
 title     = {Observing Dirac's classical phase space analog to the quantum state},
 volume    = {112},
 pages     = {070405(1-6)},
 year      = {2014},
}

@article{grossmann:JCP:2009,
 author    = {Ch.-M. Goletz and F. Grossmann},
 journal   = {J. Chem. Phys.},
 title     = {Decoherence and dissipation in a molecular system coupled to an environment: An application of semiclassical hybrid dynamics},
 volume    = {130},
 pages     = {244107(1-12)},
 year      = {2009},
}

@article{deMarcus:AJ:1978,
 author    = {W. C. DeMarcus},
 journal   = {Am. J. Phys.},
 title     = {Classical motion of a Morse oscillator},
 volume    = {46},
 pages     = {733-734},
 year      = {1978},
}

@article{braverman:PRL:2013,
  title = {Proposal to Observe the Nonlocality of Bohmian Trajectories with Entangled Photons},
  author = {Braverman, Boris and Simon, Christoph},
  journal = {Phys. Rev. Lett.},
  volume = {110},
  issue = {6},
  pages = {060406},
  numpages = {5},
  year = {2013},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.110.060406},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.110.060406}
}

@article{young:PTRSL:1804,
 author    = {T. Young},
 journal   = {Phil. Trans. R. Soc. Lond.},
 title     = {The Bakerian Lecture. Experimentas and calculations relative to physical optics},
 volume    = {94},
 pages     = {1-16},
 year      = {1804},
}

@BOOK{young:1807,
  AUTHOR     = {T. Young},
  editor     = {W. Savage},
  TITLE      = {A Course of Lectures on Natural Philosophy and the Mechanical Arts},
  PUBLISHER  = {Joseph Johnson},
  YEAR       = {1807},
  address    = {London},
}

@BOOK{feynman:FLP3:1965,
  AUTHOR     = {R. P. Feynman and R. B. Leighton and M. Sands},
  TITLE      = {The Feynman Lectures on Physics},
  PUBLISHER  = {Addison-Wesley},
  YEAR       = {1965},
  volume     = {3},
  address    = {Reading, MA},
}

@BOOK{lipson-bk:2011,
  AUTHOR     = {A. Lipson and S. G. Lipson and H. Lipson},
  TITLE      = {Optical Physics},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {2011},
  address    = {New York},
  edition    = {4th},
}

@BOOK{hecht-bk:2002,
  AUTHOR     = {E. Hecht},
  TITLE      = {Optics},
  PUBLISHER  = {Addison-Wesley Longman},
  YEAR       = {2002},
  address    = {New York},
  edition    = {4th},
}

@article{bohr100-1:2013,
 author    = {News Feature},
 journal   = {Nature},
 title     = {Quantum physics: The quantum atom},
 volume    = {498},
 pages     = {21},
 year      = {6 June 2013},
 source    = {},
}

@article{bohr100-2:2013,
 author    = {Special Issue},
 journal   = {Nature},
 title     = {The quantum atom},
 volume    = {498},
 pages     = {},
 year      = {6 June 2013},
 source    = {www.nature.com/bohr100},
}

@article{forman:HistStud:1971,
 author    = {P. Forman},
 journal   = {Hist. Stud. Phys. Sci.},
 title     = {Weimar Culture, Causality, and Quantum Theory, 1918-1927: Adaptation by German Physicists and Mathematicians to a Hostile Intellectual Environment},
 volume    = {3},
 pages     = {1-115},
 year      = {1971},
}

@BOOK{jammer-bk:1966,
  AUTHOR     = {M. Jammer},
  TITLE      = {The Conceptual Development of Quantum Mechanics},
  PUBLISHER  = {McGraw-Hill},
  YEAR       = {1966},
  address    = {New York},
}

@article{mermin:PhysToday:1989,
 author    = {N. D. Mermin},
 journal   = {Physics Today},
 title     = {What's wrong with this pillow?},
 volume    = {42},
 number    = {4},
 pages     = {9-11},
 year      = {1989},
}

@article{mermin:PhysToday:2004,
 author    = {N. D. Mermin},
 journal   = {Physics Today},
 title     = {Could Feynman have said this?},
 volume    = {57},
 number    = {5},
 pages     = {10-11},
 year      = {2004},
}

@article{broglie:CompRend-2:1926,
 author    = {L. de Broglie},
 journal   = {Comptes Rendus},
 title     = {Sur la possibilit\'e de relier les ph\'enom\`enes d'interf\'erence et de diffraction \'a la th\'eorie des quanta de lumie\`ere},
 volume    = {183},
 pages     = {447-448},
 year      = {1926},
}

@article{broglie:CompRend-1:1926,
 author    = {L. de Broglie},
 journal   = {Comptes Rendus},
 title     = {Rermarques sur la nouvelle M\'ecanique ondulatoire},
 volume    = {183},
 pages     = {272-274},
 year      = {1926},
}

@article{schrodinger:PhysRev:1926,
 author    = {E. Schr\"odinger},
 journal   = {Phys. Rev.},
 title     = {An undulatory theory of the mechanics of atoms and molecules},
 volume    = {28},
 pages     = {1049-1070},
 year      = {1926},
}

@article{waterhouse:JASA:1985,
 author    = {R. V. Waterhouse and T. W. Yates and D. Feit and Y. N. Liu},
 journal   = {J. Acoust. Soc. Am.},
 title     = {Energy streamlines of a sound source},
 volume    = {78},
 pages     = {758-762},
 year      = {1985},
}

@article{waterhouse:JASA:1986-1,
 author    = {R. V. Waterhouse and D. Feit},
 journal   = {J. Acoust. Soc. Am.},
 title     = {Equal-energy streamlines},
 volume    = {80},
 pages     = {681-684},
 year      = {1986},
}

@article{waterhouse:JASA:1986-2,
 author    = {E. A. Skelton and R. V. Waterhouse},
 journal   = {J. Acoust. Soc. Am.},
 title     = {Energy streamlines for a spherical shell scattering plane wave},
 volume    = {80},
 pages     = {1473-1478},
 year      = {1986},
}

@article{waterhouse:JASA:1987-1,
 author    = {R. V. Waterhouse and D. G. Crighton and J. E. Ffowcs-Williams},
 journal   = {J. Acoust. Soc. Am.},
 title     = {A criterion for an energy vortex in a sound field},
 volume    = {81},
 pages     = {1323-1326},
 year      = {1987},
}

@article{waterhouse:JASA:1987-2,
 author    = {R. V. Waterhouse},
 journal   = {J. Acoust. Soc. Am.},
 title     = {Vortex modes in rooms},
 volume    = {82},
 pages     = {1782-1791},
 year      = {1987},
}

@article{lazzeretti:CPL:1981,
 author    = {P. Lazzeretti and R. Zanasi},
 journal   = {Chem. Phys. Lett.},
 title     = {Inconsistency of the ring-current model for the cyclopropenyl cation},
 volume    = {80},
 pages     = {533-536},
 year      = {1981},
}

@article{lazzeretti:IJQC:1984,
 author    = {P. Lazzeretti and E. Rossi and R. Zanasi},
 journal   = {Int. J. Quantum Chem.},
 title     = {Singularities of magnetic-field induced electron current density: A study of the ethylene molecule},
 volume    = {25},
 pages     = {929-940},
 year      = {1984},
}

@article{lazzeretti:PNMRS:2000,
 author    = {P. Lazzeretti},
 journal   = {Prog. Nucl. Magn. Reson. Spect.},
 title     = {Righ currents},
 volume    = {36},
 pages     = {1-88},
 year      = {2000},
}

@article{lazzeretti:IJQC:2011,
 author    = {S. Pelloni and P. Lazzeretti},
 journal   = {Int. J. Quantum Chem.},
 title     = {Stagnation graphs and topological models of magnetic-field induced electron current density for some small molecules in connection with their magnetic symmetry},
 volume    = {111},
 pages     = {356-367},
 year      = {2011},
}

@article{gomes:JCP:1983-1,
 author    = {J. A. N. F. Gomes},
 journal   = {J. Chem. Phys.},
 title     = {Delocalized magnetic currents in benzene},
 volume    = {78},
 pages     = {3133-3139},
 year      = {1983},
}

@article{gomes:JCP:1983-2,
 author    = {J. A. N. F. Gomes},
 journal   = {J. Chem. Phys.},
 title     = {Topological elements of the magnetically induced orbital current densities},
 volume    = {78},
 pages     = {4585-4591},
 year      = {1983},
}

@article{berger:AngewChem:2010,
 author    = {R. J. F. Berger and H. S. Rzepa and D. Scheschkewitz},
 journal   = {Angew. Chem. Int. Ed.},
 title     = {Ring currents in the dismutational aromatic Si$_6$R$_6$},
 volume    = {49},
 pages     = {10006-10009},
 year      = {2010},
}

@article{braunbek:Optik:1952,
 author    = {W. Braunbek and G. Laukien},
 journal   = {Optik},
 title     = {Features of refraction by a semi-plane},
 volume    = {9},
 pages     = {174-179},
 year      = {1952},
}

@article{sommerfeld:MathAnn:1896,
 author    = {A. Sommerfeld},
 journal   = {Math. Ann.},
 title     = {Theorie der diffraction},
 volume    = {47},
 pages     = {317-374},
 year      = {1896},
}

@article{sanz:JPhysConfSer:2012,
 author    = {A. S. Sanz},
 journal   = {J. Phys.: Conf. Ser.},
 title     = {Quantumness beyond quantum mechanics},
 volume    = {361},
 pages     = {012016(1-11)},
 year      = {2012},
}

@article{sanz:EPN:2013,
 author    = {M. Davidovi\'c and A. S. Sanz},
 journal   = {Europhys. News},
 title     = {How does light move? Determining the flow of light without destroying interference},
 volume    = {44},
 number    = {6},
 pages     = {33-36},
 year      = {2013},
 doi       = {10.1051/epn/2013604},
 url       = {https://doi.org/10.1051/epn/2013604},
}

@article{takabayasi:ProgTheorPhys:1952,
 author    = {T. Takabayasi},
 journal   = {Prog. Theor. Phys.},
 title     = {On the formulation of quantum mechanics associated with classical pictures},
 volume    = {8},
 pages     = {143-182},
 year      = {1952},
 doi       = {10.1143/ptp/8.2.143},
 url       = {https://academic.oup.com/ptp/article/8/2/143/1883374}
}

@article{takabayasi:ProgTheorPhys:1953,
 author    = {T. Takabayasi},
 journal   = {Prog. Theor. Phys.},
 title     = {Remarks on the formulation of quantum mechanics with classical pictures and on relations between linear scalar fields and hydrodynamical fields},
 volume    = {9},
 pages     = {187-222},
 year      = {1953},
}

@article{takabayasi:ProgTheorPhys:1983,
 author    = {T. Takabayasi},
 journal   = {Prog. Theor. Phys.},
 title     = {Hydrodynamical formalism of quantum mechanics and Aharonov-Bohm effect},
 volume    = {69},
 pages     = {1323-1344},
 year      = {1983},
}

@article{mccullough:JCP:1969,
 author    = {E. A. McCullough and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Quantum dynamics of the collinear (H,H$_2$) reaction},
 volume    = {51},
 pages     = {1253-1254},
 year      = {1969},
}

@article{mccullough:JCP:1971-1,
 author    = {E. A. McCullough and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Dynamics of the collinear H+H$_2$ reaction. I. Probability density and flux},
 volume    = {54},
 pages     = {3578-3591},
 year      = {1971},
}

@article{mccullough:JCP:1971-2,
 author    = {E. A. McCullough and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Dynamics of the collinear H+H$_2$ reaction. II. Energy analysis},
 volume    = {54},
 pages     = {3592-3600},
 year      = {1971},
}

@article{dewdney:NuovoCimB:1979,
 author    = {C. Philippidis and C. Dewdney and B. J. Hiley},
 journal   = {Nuovo Cimento},
 title     = {Quantum interference and the quantum potential},
 volume    = {52B},
 pages     = {15--28},
 year      = {1979},
 doi       = {https://doi.org/10.1007/BF02743566},
 url       = {https://link.springer.com/article/10.1007/BF02743566}
}

@BOOK{courant-hilbert-bk-1,
  AUTHOR     = {R. Courant and D. Hilbert},
  TITLE      = {Methods of Mathematical Physics},
  PUBLISHER  = {John Wiley \& Sons},
  YEAR       = {1966},
  address    = {New York},
  volume     = {1},
}

@BOOK{courant-hilbert-bk-2,
  AUTHOR     = {R. Courant and D. Hilbert},
  TITLE      = {Methods of Mathematical Physics},
  PUBLISHER  = {John Wiley \& Sons},
  YEAR       = {1966},
  address    = {New York},
  volume     = {2},
}

@article{chevalerias:JOSA:1957,
 author    = {R. Chevalerias and Y. Latron and C. Veret},
 journal   = {J. Opt. Soc. Am.},
 title     = {Methods of interferometry applied to the visualization of flows in wind tunnels},
 volume    = {47},
 pages     = {703-706},
 year      = {1957},
}

@BOOK{hughes-bk,
  editor     = {K. H. Hughes and G. Parlant},
  TITLE      = {Quantum Trajectories},
  PUBLISHER  = {CCP6},
  YEAR       = {2011},
  address    = {Daresbury, UK},
}

@BOOK{sanz:CCP6:2011,
  AUTHOR     = {A. S. Sanz},
  editor     = {K. H. Hughes and G. Parlant},
  TITLE      = {Quantum Trajectories},
  CHAPTER    = {An account on quantum interference from a hydrodynamical perspective},
  pages      = {111-115},
  PUBLISHER  = {CCP6},
  YEAR       = {2011},
  address    = {Daresbury, UK},
}

@article{sanz:CJC:2014,
 author    = {A. S. Sanz},
 journal   = {Can. J. Chem.},
 title     = {Effective Markovian description of decoherence in bound systems},
 volume    = {92},
 pages     = {168-178},
 year      = {2014},
}

@article{schuch:PRA:1983,
 author    = {D. Schuch and K.-M. Chung and H. Hartmann},
 journal   = {Phys. Rev. A},
 title     = {Nonlinear Schr\"odinger-type field equation for the description of dissipative systems. I. Derivation of the nonlinear field equation and one-dimensional example},
 volume    = {24},
 pages     = {1652-1660},
 year      = {1983},
}

@article{schuch:PRA:1984-1,
 author    = {D. Schuch and K.-M. Chung and H. Hartmann},
 journal   = {Phys. Rev. A},
 title     = {Nonlinear Schr\"odinger-type field equation for the description of dissipative systems. II. Frictionally damped motion in a magnetic field},
 volume    = {25},
 pages     = {391-410},
 year      = {1984},
}

@article{schuch:PRA:1984-2,
 author    = {D. Schuch and K.-M. Chung and H. Hartmann},
 journal   = {Phys. Rev. A},
 title     = {Nonlinear Schr\"odinger-type field equation for the description of dissipative systems. III. Frictionally damped free motion as an example for an aperiodic motion},
 volume    = {25},
 pages     = {3086-3092},
 year      = {1984},
}

@BOOK{shamos-bk,
  editor     = {M. H. Shamos},
  TITLE      = {Great Experiments in Physics},
  PUBLISHER  = {Dover},
  YEAR       = {1987},
  address    = {New York},
}

@article{goldberg:AJP:1967,
 author    = {A. Goldberg and H. M. Schey and J. L. Schwartz},
 journal   = {Am. J. Phys.},
 title     = {Computer-generated motion pictures of one-dimensional quantum-mechanical transmission and reflection phenomena},
 volume    = {35},
 pages     = {177-186},
 year      = {1967},
}

@article{mazur:JCP:1959,
 author    = {J. Mazur and R. J. Rubin},
 journal   = {J. Chem. Phys.},
 title     = {Quantum-mechanical calculation of the probability of an exchange reaction for constrained linear encounters},
 volume    = {31},
 pages     = {1395-1412},
 year      = {1959},
}

@article{marcus:JCP:1966,
 author    = {R. A. Marcus},
 journal   = {J. Chem. Phys.},
 title     = {On the analytical mechanics of chemical reactions. Quantum mechanics of linear collisions},
 volume    = {45},
 pages     = {4493-4499},
 year      = {1966},
}

@article{abraham:AJP:1984,
 author    = {I. Galbraith and Y. S. Ching and E. Abraham},
 journal   = {Am. J. Phys.},
 title     = {Two-dimensional time-dependent quantum-mechanical scattering event},
 volume    = {52},
 pages     = {60-68},
 year      = {1984},
}

@article{efthymio:AnnPhys:2012,
 author    = {C. Efthymiopoulos and N. Delis and G. Contopoulos},
 journal   = {Ann. Phys.},
 title     = {Wavepacket approach to particle diffraction by thin targets: Quantum trajectories and arrival times},
 volume    = {327},
 pages     = {438-460},
 year      = {2012},
}

@article{efthymio:IJBC:2012,
 author    = {N. Delis and C. Efthymiopoulos and G. Contopoulos},
 journal   = {Int. J. Bifur. Chaos},
 title     = {Quantum vortices and trajectories in particle diffraction},
 volume    = {22},
 pages     = {1250214(1-17)},
 year      = {2012},
}

@article{muga:PhysRep:2000,
 author    = {J. G. Muga and C. R. Leavens},
 journal   = {Phys. Rep.},
 title     = {Arrival time in quantum mechanics},
 volume    = {338},
 pages     = {353-438},
 year      = {2000},
}

@BOOK{muga-bk-1:LNP:2002,
  editor     = {J. G. Muga and R. Sala Mayato and I. L. Egusquiza},
  TITLE      = {Time in Quantum Mechanics},
  PUBLISHER  = {Springer},
  series     = {Lecture Notes in Physics},
  volume     = {72},
  YEAR       = {2002},
  address    = {Berlin},
}

@BOOK{muga-bk-2:LNP:2009,
  editor     = {J. G. Muga and A. Ruschhaupt and A. del Campo},
  TITLE      = {Time in Quantum Mechanics - Vol.~2},
  PUBLISHER  = {Springer},
  series     = {Lecture Notes in Physics},
  volume     = {789},
  YEAR       = {2009},
  address    = {Berlin},
}

@article{valentini:PRSA:2005,
 author    = {A. Valentini and H. Westman},
 journal   = {Proc. R. Soc. A},
 title     = {Dynamical origin of quantum probabilities},
 volume    = {461},
 pages     = {253-272},
 year      = {2005},
}

@article{valentini:PRSA:2012,
 author    = {M. D. Towler and N. J. Russell and A. Valentini},
 journal   = {Proc. R. Soc. A},
 title     = {Time scales for dynamical relaxation to the Born rule},
 volume    = {468},
 pages     = {990-1013},
 year      = {2012},
}

@article{olkhovsky:NuovoCim:1974,
 author    = {V. S. Olkhovsky and E. Recami and A. J. Gerasimchuk},
 journal   = {Nuovo Cimento},
 title     = {Time operator in quantum mechanics. I. Nonrelativistic case},
 volume    = {22},
 pages     = {263-278},
 year      = {1974},
}

@article{olkhovsky:AMP:2009,
 author    = {V. S. Olkhovsky},
 journal   = {Adv. Math. Phys.},
 title     = {Time as a quantum observable, canonically conjugated to energy, and foundations of self-consistent time analysis of quantum processes},
 volume    = {Article ID 859710},
 pages     = {1-83},
 year      = {2009},
}

@article{wang:AnnPhys:2007,
 author    = {Z.-Y. Wang and C.-D. Xiong},
 journal   = {Ann. Phys.},
 title     = {How to introduce time operator},
 volume    = {322},
 pages     = {2304-2314},
 year      = {2007},
}

@book{pauli-hbk-1,
  address =       {Berlin},
  author =        {W. Pauli},
  chapter =       {Die allgemeinen Prinzipien der Wellenmechanik},
  editor =        {H. Geiger and K. Scheel},
  pages =         {83-272},
  publisher =     {Springer},
  title =         {Handbuch der Physik},
  volume =        {24/1},
  year =          {1933},
  edition =       {2nd},
}

@book{pauli-hbk-1rev,
  address =       {Berlin},
  author =        {W. Pauli},
  chapter =       {Die allgemeinen Prinzipien der Wellenmechanik},
  editor =        {S. Fl\"ugge},
  pages =         {1-168},
  publisher =     {Springer},
  title =         {Handbuch der Physik - Prinzipien der Quantentheorie I},
  volume =        {5/1},
  year =          {1958},
}

@book{pauli-hbk-1rep,
  address =       {Berlin},
  author =        {W. Pauli},
  title  =        {Die allgemeinen Prinzipien der Wellenmechanik},
  editor =        {N. Straumann},
  publisher =     {Springer},
  year =          {1990},
}

@book{pauli-hbk-1eng,
  address =       {Berlin},
  author =        {W. Pauli},
  title  =        {General Principles of Quantum Mechanics},
  editor =        {P. Achuthan and K. Venkatesan},
  publisher =     {Springer},
  year =          {1980},
}

@article{leavens:SSC:1990-1,
 author    = {C. R. Leavens},
 journal   = {Solid State Comm.},
 title     = {Transmission, reflection and dwell times within Bohm's causal interpretation of quantum mechanics},
 volume    = {74},
 pages     = {923-928},
 year      = {1990},
}

@article{leavens:SSC:1990-2,
 author    = {C. R. Leavens},
 journal   = {Solid State Comm.},
 title     = {Traversal times for rectangular barriers within Bohm's causal interpretation of quantum mechanics},
 volume    = {76},
 pages     = {253-261},
 year      = {1990},
}

@article{leavens:PhysLettA:1993,
 author    = {C. R. Leavens},
 journal   = {Phys. Lett. A},
 title     = {Arrival time distributions},
 volume    = {178},
 pages     = {27-32},
 year      = {1993},
}

@article{leavens:FoundPhys:1995,
 author    = {C. R. Leavens},
 journal   = {Solid State Comm.},
 title     = {Bohm Trajectory and Feynman Path Approaches to the ``Tunneling Time Problem''},
 volume    = {25},
 pages     = {229-268},
 year      = {1995},
}

@BOOK{zeh-hbk-1,
  autor      = {H. D. Zeh},
  chapter    = {Time in quantum theory},
  editor     = {D. Greenberger and K. Hentschel and F. Weinert},
  TITLE      = {Compendium of Quantum Physics: Concepts, Experiments, History and Philosophy},
  PUBLISHER  = {Springer},
  pages      = {786-792},
  YEAR       = {2009},
  address    = {Berlin},
}

@BOOK{reichl:1992,
  AUTHOR     = {L. E. Reichl},
  TITLE      = {The Transition to Chaos in Conservative Classical Systems: Quantum Manifestations},
  PUBLISHER  = {Springer},
  YEAR       = {1992},
  address    = {Berlin},
}

@BOOK{mehta:1991,
  AUTHOR     = {M. L. Mehta},
  TITLE      = {Random Matrix Theory},
  PUBLISHER  = {Academic Press},
  YEAR       = {1991},
  address    = {New York},
}

@BOOK{gaspard-bk:1998,
  AUTHOR     = {P. Gaspard},
  TITLE      = {Chaos, Scattering and Statistical Mechanics},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {1998},
  address    = {Cambridge},
}

@article{bohigas:PRL:1984,
 author    = {O. Bohigas and M. J. Giannoni and C. Schmit},
 journal   = {Phys. Rev. Lett.},
 title     = {},
 volume    = {52},
 pages     = {1-},
 year      = {1984},
}

@article{zurek:PRL:1994,
 author    = {W. H. Zurek and J. P. Paz},
 journal   = {Phys. Rev. Lett.},
 title     = {Decoherence, chaos, and the second law},
 volume    = {72},
 pages     = {2508-2511},
 year      = {1994},
}

@article{zaslavskii:SPJETP:1974,
 author    = {G. M. Zaslavskii and N. N. Filonenko},
 journal   = {Sov. Phys. JETP},
 title     = {Statistical properties of the energy spectrum of ``gliding'' electrons with mixed classical trajectories},
 volume    = {38},
 pages     = {317-323},
 year      = {1974},
}

@article{zaslavskii:ZhETF:1973,
 author    = {G. M. Zaslavskii and N. N. Filonenko},
 journal   = {Zh. Eksp. Teor. Fiz.},
 title     = {},
 volume    = {65},
 pages     = {643-656},
 year      = {1973},
}

@article{mcdonald:PRL:1979,
 author    = {S. W. McDonald and A. N. Kaufman},
 journal   = {Phys. Rev. Lett.},
 title     = {},
 volume    = {42},
 pages     = {1189-},
 year      = {1979},
}

@article{heller:PRL:1984,
 author    = {E. J. Heller},
 journal   = {Phys. Rev. Lett.},
 title     = {Bound-state eigenfunctions of classically chaotic Hamiltonian systems: scars of periodic orbits},
 volume    = {53},
 pages     = {1515-1518},
 year      = {1984},
}

@article{bluemel:PhysicsWorld:1990,
 author    = {R. Bl\"umel and U. Smilansky},
 journal   = {Physics World},
 title     = {},
 volume    = {3},
 number    = {2},
 pages     = {30-},
 year      = {1990},
}

@article{baranger:chaos:1993,
 author    = {H. U. Baranger and Others},
 journal   = {Chaos},
 title     = {},
 volume    = {3},
 pages     = {665},
 year      = {1993},
}

@article{marcus:chaos:1993,
 author    = {C. M. Marcus and Others},
 journal   = {Chaos},
 title     = {},
 volume    = {3},
 pages     = {643},
 year      = {1993},
}

@article{fleischmann:PRL:1992,
 author    = {R. Fleischmann and T. Geisel and R. Ketzmerick},
 journal   = {Phys. Rev. Lett.},
 title     = {},
 volume    = {68},
 pages     = {1367-},
 year      = {1992},
}

@article{ketzmerick:PRL:1998,
 author    = {A. S. Sachrajda and Others},
 journal   = {Phys. Rev. Lett.},
 title     = {},
 volume    = {80},
 pages     = {1948-},
 year      = {1998},
}

@article{verges:PRL:1998,
 author    = {P. L. de Andres and J. A. Verg\'es},
 journal   = {Phys. Rev. Lett.},
 title     = {},
 volume    = {80},
 pages     = {980-},
 year      = {1998},
}

@article{fyodorov:PRA:1998,
 author    = {Y. V. Fyodorov and Y. Alhassid},
 journal   = {Phys. Rev. A},
 title     = {},
 volume    = {58},
 pages     = {R3375-},
 year      = {1998},
}

@article{raizen:PRL:1998,
 author    = {Q. Niu and M. G. Raizen},
 journal   = {Phys. Rev. Lett.},
 title     = {},
 volume    = {80},
 pages     = {3491-},
 year      = {1998},
}

@article{gluck:PRL:1999,
 author    = {M. Gl\"uck and A. R. Kolovsky and H. J. Korsch},
 journal   = {Phys. Rev. Lett.},
 title     = {},
 volume    = {83},
 pages     = {891-},
 year      = {1999},
}

@article{seligman:PhysRep:1997,
 author    = {C. Jung and T. H. Seligman},
 journal   = {Phys. Rep.},
 title     = {},
 volume    = {285},
 pages     = {77-},
 year      = {1997},
}

@article{lewenkopf:AnnPhys:1991,
 author    = {C. H. Lewenkopf and H. A. Weidenm\"uller},
 journal   = {Ann. Phys.},
 title     = {},
 volume    = {212},
 pages     = {53-},
 year      = {1991},
}

@BOOK{smilansky-ch:1991,
  author     = {U. Smilansky},
  chapter    = {},
  editor     = {M.-J. Giannoni and A. Voros and J. Zinn-Justin},
  TITLE      = {Chaos and Quantum Physics},
  PUBLISHER  = {North-Holland},
  pages      = {},
  YEAR       = {1991},
  address    = {New York},
}

@BOOK{cushing-bk:1996,
  editor     = {J. T. Cushing and A. Fine and S. Goldstein},
  TITLE      = {Bohmian Mechanics: An Appraisal},
  PUBLISHER  = {Kluwer},
  YEAR       = {1996},
  address    = {Boston},
}

@article{duerr:JStatPhys:1992b,
 author    = {D. D\"urr and S. Goldstein and N. Zangh\`i},
 journal   = {J. Stat. Phys.},
 title     = {Quantum chaos, classical randomness, and Bohmian mechanics},
 volume    = {68},
 pages     = {259-270},
 year      = {1992},
}

@article{frisk:PLA:1997,
 author    = {H. Frisk},
 journal   = {Phys. Lett. A},
 title     = {},
 volume    = {227},
 pages     = {139-},
 year      = {1997},
}

@article{parmenter:PLA:1995,
 author    = {R.H. Parmenter and R. W. Valentine},
 journal   = {Phys. Lett. A},
 title     = {},
 volume    = {201},
 pages     = {1-},
 year      = {1995},
}

@article{parmenter:PLA:1996,
 author    = {R.H. Parmenter and R. W. Valentine},
 journal   = {Phys. Lett. A},
 title     = {},
 volume    = {213},
 pages     = {319-},
 year      = {1996},
}

@article{makowski:PLA:2000,
 author    = {A. J. Makowski and P. Pep{\l}oswski and S. T. Dembi\'nski},
 journal   = {Phys. Lett. A},
 title     = {Chaotic causal trajectories: the role of the phase of stationary states},
 volume    = {266},
 pages     = {241-248},
 year      = {2000},
}

@article{makowski:ActaPhysPolB:2001,
 author    = {A. J. Makowski and M. Fr\c ackowiak},
 journal   = {Acta Physica Polonica B},
 title     = {The simplest non-trivial model of chaotic causal dynamics},
 volume    = {32},
 pages     = {2831-2842},
 year      = {2001},
}

@article{makowski:ActaPhysPolB:2002,
 author    = {A. J. Makowski},
 journal   = {Acta Physica Polonica B},
 title     = {Forced dynamical systems derivable from Bohmian mechanics},
 volume    = {33},
 pages     = {583-592},
 year      = {2002},
}

@article{bonfin:PRE:1998,
 author    = {O. F. de Alcantara Bonfim and J. Florencio and F. C. S\'a Barreto},
 journal   = {Phys. Rev. E},
 title     = {},
 volume    = {58},
 pages     = {R2693-},
 year      = {1998},
}

@article{bonfin:PLA:2000,
 author    = {O. F. de Alcantara Bonfim and J. Florencio and F. C. S\'a Barreto},
 journal   = {Phys. Rev. E},
 title     = {},
 volume    = {277},
 pages     = {129-},
 year      = {2000},
}

@article{faisal:PLA-1:1995,
 author    = {U. Schwengelbeck and F. H. M. Faisal},
 journal   = {Phys. Lett. A},
 title     = {},
 volume    = {199},
 pages     = {281-},
 year      = {1995},
}

@article{faisal:PLA-2:1995,
 author    = {F. H. M. Faisal and U. Schwengelbeck},
 journal   = {Phys. Lett. A},
 title     = {},
 volume    = {207},
 pages     = {31-},
 year      = {1995},
}

@article{iacomelli:PLA:1996,
 author    = {G. Iacomelli and M. Pettini},
 journal   = {Phys. Lett. A},
 title     = {},
 volume    = {212},
 pages     = {29-},
 year      = {1996},
}

@article{chattaraj:PLA:1996,
 author    = {S. Sengupta and P. K. Chattaraj},
 journal   = {Phys. Lett. A},
 title     = {The quantum theory of motion and signatures of chaos in the quantum behaviour of a classically chaotic system},
 volume    = {215},
 pages     = {119-127},
 year      = {1996},
}

@article{chattaraj:CurrentSci:1996,
 author    = {P. K. Chattaraj and S. Sengupta},
 journal   = {Curr. Sci.},
 title     = {Quantum chaos in Rydberg atoms: A quantum potential approach},
 volume    = {71},
 pages     = {134-139},
 year      = {1996},
}

@article{chattaraj:CurrentSci:1998,
 author    = {P. K. Chattaraj and S. Sengupta and A. Poddar},
 journal   = {Curr. Sci.},
 title     = {Chaotic dynamics of some quantum anharmonic oscillators},
 volume    = {74},
 pages     = {758-764},
 year      = {1998},
}

@article{polavieja:PRE:1997,
 author    = {G. Garc\'\i a de Polavieja and M. S. Child},
 journal   = {Phys. Rev. E},
 title     = {Quantum instability of the flux lines in the coherent state representation},
 volume    = {55},
 pages     = {1451-1456},
 year      = {1997},
}

@article{polavieja:PLA:1996,
 author    = {G. Garc\'\i a de Polavieja},
 journal   = {Phys. Lett. A},
 title     = {A causal quantum theory in phase space},
 volume    = {220},
 pages     = {303-314},
 year      = {1996},
}

@article{procaccia:PhysicaD:1983,
 author    = {P. Grassberger and I. Procaccia},
 journal   = {Physica D},
 title     = {},
 volume    = {9},
 pages     = {189-},
 year      = {1983},
}

@article{goldstein:PRE:1999,
 author    = {S. Goldstein},
 journal   = {Phys. Rev. E},
 title     = {},
 volume    = {60},
 pages     = {7578},
 year      = {1999},
}

@article{sprung:PLA:1999,
 author    = {H. Wu and D. W. L. Sprung},
 journal   = {Phys. Lett. A},
 title     = {},
 volume    = {261},
 pages     = {150-},
 year      = {1999},
}

@article{polavieja:PRA:1996,
 author    = {G. Garc{\'\i}a de Polavieja},
 journal   = {Phys. Rev. A},
 title     = {Exponential divergence of neighboring quantal trajectories},
 volume    = {53},
 pages     = {2059-2061},
 year      = {1996},
}

@article{dewdney:PLA:1996,
 author    = {C. Dewdney and Z. Malik},
 journal   = {Phys. Lett. A},
 title     = {},
 volume    = {220},
 pages     = {183-},
 year      = {1996},
}

@article{makowski:PLA:1998,
 author    = {S. Konkel and A. J. Makowski},
 journal   = {Phys. Lett. A},
 title     = {Regular and chaotic causal trajectories for the Bohm potential in a restricted space},
 volume    = {238},
 pages     = {95-100},
 year      = {1998},
}

@article{cushing:PhilosSci:2000,
 author    = {J. T. Cushing},
 journal   = {Philos. Sci.},
 title     = {},
 volume    = {67},
 pages     = {S432-},
 year      = {2000},
}

@article{sales:PRE:2003,
 author    = {J. A. de Sales and J. Florencio},
 journal   = {Phys. Rev. E},
 title     = {Quantum chaotic trajectories in integrable right triangular billiards},
 volume    = {67},
 pages     = {016216(1-6)},
 year      = {2003},
}

@article{sales:PhysicaA:2001,
 author    = {J. A. de Sales and J. Florencio},
 journal   = {Physica A},
 title     = {Bohmian quantum trajectories in a square billiard in the bouncing ball regime},
 volume    = {290},
 pages     = {101-106)},
 year      = {2001},
}

@article{falsaperla:FoundPhys:2002,
 author    = {P. Falsaperla and G. Fonte and G. Salesi},
 journal   = {Found. Phys.},
 title     = {Quantum Lyapunov exponents},
 volume    = {32},
 pages     = {267-294},
 year      = {2002},
}

@article{falsaperla:PLA:2003,
 author    = {P. Falsaperla and G. Fonte},
 journal   = {Phys. Lett. A},
 title     = {On the motion of a single particle near a nodal line in the de Broglie-Bohm interpretation of quantum mechanics},
 volume    = {316},
 pages     = {382-390},
 year      = {2003},
}

@article{wisniacki:EPL:2005,
 author    = {D. A. Wisniacki and E. R. Pujals},
 journal   = {Europhys. Lett.},
 title     = {Motion of vortices implies chaos in Bohmian mechanics},
 volume    = {71},
 pages     = {159-},
 year      = {2005},
}

@article{wisniacki:JPA:2007,
 author    = {D. A. Wisniacki and E. R. Pujals and F. Borondo},
 journal   = {J. Phys. A},
 title     = {},
 volume    = {40},
 pages     = {14353-},
 year      = {2007},
}

@article{schlegel:PLA:2008,
 author    = {K. G. Schlegel and S. F\"orster},
 journal   = {Phys. Lett. A},
 title     = {Deterministic chaos in entangled eigenstates},
 volume    = {372},
 pages     = {3620-3631},
 year      = {2008},
}

@article{bu:PhysicaD:2006,
 author    = {S. Bu},
 journal   = {Physica D},
 title     = {Quantum trajectory of an individual particle in the presence of chaos},
 volume    = {217},
 pages     = {103-106},
 year      = {2006},
}

@article{bennett:JPA:2010,
 author    = {A. Bennett},
 journal   = {J. Phys. A},
 title     = {},
 volume    = {43},
 pages     = {5304-},
 year      = {2010},
}

@article{struyve:NJP:2010,
 author    = {S. Colin and W. Struyve},
 journal   = {New J. Phys.},
 title     = {Quantum non-equilibrium and relaxation to equilibrium for a class of de Broglie-Bohm-type theories},
 volume    = {12},
 pages     = {043008(1-21)},
 year      = {2010},
}

@article{efthymio:JPA:2006,
 author    = {C. Efthymiopoulos and Contopoulos},
 journal   = {J. Phys. A},
 title     = {Chaos in Bohmian quantum mechanics},
 volume    = {39},
 pages     = {1819-1852},
 year      = {2006},
}

@article{efthymio:JPA:2012,
 author    = {G. Contopoulos and N. Delis and C. Efthymiopoulos},
 journal   = {J. Phys. A},
 title     = {Order in de Broglie-Bohm Mechanics},
 volume    = {45},
 pages     = {165301(1-21)},
 year      = {2011},
}

@article{efthymio:JPA:2007,
 author    = {C. Efthymiopoulos and C. Kalapotharakos and G. Contopoulos},
 journal   = {J. Phys. A},
 title     = {Nodal points and the transition from ordered to chaotic Bohmian trajectories},
 volume    = {40},
 pages     = {12945-12972},
 year      = {2007},
}

@article{efthymio:CMDynAstr:2008,
 author    = {G. Contopoulos and C. Efthymiopoulos},
 journal   = {Celest. Mech. Dyn. Astron.},
 title     = {Ordered and chaotic Bohmian trajectories},
 volume    = {102},
 pages     = {219-239},
 year      = {2008},
}

@article{efthymio:PRE:2009,
 author    = {C. Efthymiopoulos and C. Kalapotharakos and G. Contopoulos},
 journal   = {Phys. Rev. E},
 title     = {Origin of chaos near critical points of quantum flow},
 volume    = {79},
 pages     = {036203(1-18)},
 year      = {2009},
}

@article{berry:ProcRSocLondA:1987,
 author    = {M. V. Berry},
 journal   = {Proc. R. Soc. Lond. A},
 title     = {Quantum chaology (The Bakerian Lecture, 1987)},
 volume    = {413},
 pages     = {183-198},
 year      = {1987},
}

@article{berry:PhysScr:1989,
 author    = {M. V. Berry},
 journal   = {Phys. Scr.},
 title     = {Quantum chaology, not quantum chaos},
 volume    = {40},
 pages     = {335-336},
 year      = {1989},
}

@article{leacock:PRL:1983,
 author    = {R. A. Leacock and M. J. Padgett},
 journal   = {Phys. Rev. Lett.},
 title     = {Hamilton-Jacobi theory and the quantum action variable},
 volume    = {50},
 pages     = {3-6},
 year      = {1983},
}

@article{leacock:PRD:1983,
 author    = {R. A. Leacock and M. J. Padgett},
 journal   = {Phys. Rev. D},
 title     = {Hamilton-Jacobi/action-angle quantum mechanics},
 volume    = {28},
 pages     = {2491-2502},
 year      = {1983},
}

@article{jordan:ZPhys:1926,
 author    = {P. Jordan},
 journal   = {Z. Phys.},
 title     = {},
 volume    = {38},
 pages     = {513-},
 year      = {1926},
}

@article{jordan:ZPhys-1:1927,
 author    = {P. Jordan},
 journal   = {Z. Phys.},
 title     = {},
 volume    = {40},
 pages     = {809-},
 year      = {1927},
}

@article{jordan:ZPhys-2:1927,
 author    = {P. Jordan},
 journal   = {Z. Phys.},
 title     = {},
 volume    = {44},
 pages     = {1-},
 year      = {1927},
}

@BOOK{gottfried-bk:1966,
  AUTHOR     = {K. Gottfried},
  TITLE      = {Quantum Mechanics},
  PUBLISHER  = {Benjamin},
  YEAR       = {New York},
  address    = {1966},
  volume     = {1},
}

@article{dirac:PRSLA:1927,
 author    = {P. A. M. Dirac},
 journal   = {Proc. R. Soc. London A},
 title     = {The physical interpretation of the quantum dynamics},
 volume    = {113},
 pages     = {621-641},
 year      = {1927},
}

@article{dirac:PZSov:1933,
 author    = {P. A. M. Dirac},
 journal   = {Phys. Z. Sowjetunion},
 title     = {},
 volume    = {3},
 pages     = {64-},
 year      = {1933},
}

@article{dirac:RMP:1945,
 author    = {P. A. M. Dirac},
 journal   = {Rev. Mod. Phys.},
 title     = {},
 volume    = {17},
 pages     = {195-},
 year      = {1945},
}

@article{jeffreys:PLMS:1925,
 author    = {K. Gottfried},
 journal   = {Proc. London Math. Soc.},
 title     = {},
 volume    = {23},
 pages     = {428-},
 year      = {1925},
}

@article{wentzel:ZPhys:1926,
 author    = {G. Wentzel},
 journal   = {Z. Phys.},
 title     = {},
 volume    = {38},
 pages     = {518-},
 year      = {1926},
}

@article{kramers:ZPhys:1926,
 author    = {H. A. Kramers},
 journal   = {Z. Phys.},
 title     = {},
 volume    = {39},
 pages     = {828-},
 year      = {1926},
}

@article{brillouin:ComptRend:1926,
 author    = {L. Brillouin},
 journal   = {Compt. Rend.},
 title     = {},
 volume    = {183},
 pages     = {24-},
 year      = {1926},
}

@article{floyd:PRD-1:1982,
 author    = {E. R. Floyd},
 journal   = {Phys. Rev. D},
 title     = {},
 volume    = {25},
 pages     = {1547-},
 year      = {1982},
}

@article{floyd:PRD-2:1982,
 author    = {E. R. Floyd},
 journal   = {Phys. Rev. D},
 title     = {},
 volume    = {26},
 pages     = {1339-},
 year      = {1982},
}

@article{floyd:PRD:1984,
 author    = {E. R. Floyd},
 journal   = {Phys. Rev. D},
 title     = {},
 volume    = {29},
 pages     = {1842-},
 year      = {1984},
}

@article{floyd:PRD:1986,
 author    = {E. R. Floyd},
 journal   = {Phys. Rev. D},
 title     = {},
 volume    = {34},
 pages     = {3246-},
 year      = {1986},
}

@article{floyd:FPL:1996,
 author    = {E. R. Floyd},
 journal   = {Found. Phys. Lett.},
 title     = {},
 volume    = {9},
 pages     = {489-},
 year      = {1996},
}

@article{floyd:FPL:2000,
 author    = {E. R. Floyd},
 journal   = {Found. Phys. Lett.},
 title     = {},
 volume    = {13},
 pages     = {235-},
 year      = {2000},
}

@article{floyd:IJMPA:1999,
 author    = {E. R. Floyd},
 journal   = {Int. J. Mod. Phys. A},
 title     = {},
 volume    = {14},
 pages     = {1111-},
 year      = {1999},
}

@article{faraggi:PLA:1998,
 author    = {A. E. Faraggi and M. Matone},
 journal   = {Phys. Lett. A},
 title     = {},
 volume    = {249},
 pages     = {180-},
 year      = {1998},
}

@article{faraggi:PLB:1998,
 author    = {A. E. Faraggi and M. Matone},
 journal   = {Phys. Lett. B},
 title     = {},
 volume    = {437},
 pages     = {369-},
 year      = {1998},
}

@article{faraggi:PLB-1:1999,
 author    = {A. E. Faraggi and M. Matone},
 journal   = {Phys. Lett. B},
 title     = {},
 volume    = {445},
 pages     = {77-},
 year      = {1999},
}

@article{faraggi:PLB-2:1999,
 author    = {A. E. Faraggi and M. Matone},
 journal   = {Phys. Lett. B},
 title     = {},
 volume    = {450},
 pages     = {34-},
 year      = {1999},
}

@article{faraggi:IJMPA:2000,
 author    = {A. E. Faraggi and M. Matone},
 journal   = {Int. J. Mod. Phys. A},
 title     = {},
 volume    = {15},
 pages     = {1869-},
 year      = {2000},
}

@article{john:FPL:2002,
 author    = {M. V. John},
 journal   = {Found. Phys. Lett.},
 title     = {Modified de Broglie-Bohm approach to quantum mechanics},
 volume    = {15},
 pages     = {329-343},
 year      = {2002},
}

@article{john:AnnPhys:2009,
 author    = {M. V. John},
 journal   = {Ann. Phys.},
 title     = {Probability and complex quantum trajectories},
 volume    = {324},
 pages     = {220-231},
 year      = {2009},
}

@article{john:AnnPhys:2010,
 author    = {M. V. John},
 journal   = {Ann. Phys.},
 title     = {Probability and complex quantum trajectories: Finding the missing links},
 volume    = {325},
 pages     = {2132-2139},
 year      = {2010},
}

@article{john:FoundPhys:2013,
 author    = {M. V. John and K. Mathew},
 journal   = {Found. Phys.},
 title     = {Coherent states and modified de Broglie-Bohm complex quantum trajectories},
 volume    = {43},
 pages     = {859-871},
 year      = {2013},
}

@article{fring:PRA:2013,
 author    = {S. Dey and A. Fring},
 journal   = {Phys. Rev. A},
 title     = {Bohmian quantum trajectories from coherent states},
 volume    = {88},
 pages     = {022116(1-12)},
 year      = {2013},
}

@article{tannor:JCP:2006,
 author    = {Y. Goldfarb and I. Degani and D. J. Tannor},
 journal   = {J. Chem. Phys.},
 title     = {Bohmian mechanics with complex action: A new trajectory-based formulation of quantum mechanics},
 volume    = {125},
 pages     = {231103(1-4)},
 year      = {2006},
}

@article{tannor:JCP-2:2007,
 author    = {Y. Goldfarb and D. J. Tannor},
 journal   = {J. Chem. Phys.},
 title     = {Interference in Bohmian mechanics with complex action},
 volume    = {127},
 pages     = {161101(1-4)},
 year      = {2007},
}

@article{tannor:JPCA:2007,
 author    = {Y. Goldfarb and J. Schiff and D. J. Tannor},
 journal   = {J. Chem. Phys.},
 title     = {Unified derivation of Bohmian methods and the incorporation of interference effects},
 volume    = {111},
 pages     = {10416-10421},
 year      = {2007},
}

@article{tannor:JCP-1:2007,
 author    = {Y. Goldfarb and I. Degani and D. J. Tannor},
 journal   = {J. Chem. Phys.},
 title     = {Response to ``Comment on `Bohmian mechanics with complex action: A new trajectory-based formulation of quantum mechanics' '' [J. Chem. Phys. {\bf 127}, 197101 (2007)]},
 volume    = {127},
 pages     = {197102(1-3)},
 year      = {2007},
}

@article{tannor:CP:2007,
 author    = {Y. Goldfarb and I. Degani and D. J. Tannor},
 journal   = {Chem. Phys.},
 title     = {Semiclassical approximation with zero velocity trajectories},
 volume    = {338},
 pages     = {106-112},
 year      = {2007},
}

@article{sanz:JCP:2007,
 author    = {A. S. Sanz and S. Miret-Art\'es},
 journal   = {J. Chem. Phys.},
 title     = {Comment on `Bohmian mechanics with complex action: A new trajectory-based formulation of quantum mechanics' [J. Chem. Phys. {\bf 125}, 231103 (2006)]},
 volume    = {127},
 pages     = {197101(1-3)},
 year      = {2007},
}

@article{chou:JCP:2006,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Computational method for the quantum Hamilton-Jacobi equation: Bound states in one dimension},
 volume    = {125},
 pages     = {174103(1-)},
 year      = {2006},
}

@article{chou:JCP-1:2008,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Quantum trajectories in complex space: One-dimensional stationary scattering problems},
 volume    = {128},
 pages     = {154106(1-)},
 year      = {2008},
}

@article{chou:JCP-2:2008,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Quantum vortices within the complex quantum Hamilton-Jacobi formalism},
 volume    = {128},
 pages     = {234106(1-)},
 year      = {2008},
}

@article{chou:JCP-3:2008,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Quantum streamlines within the complex quantum Hamilton-Jacobi formalism},
 volume    = {129},
 pages     = {124113(1-)},
 year      = {2008},
}

@article{chou:JCP:2010,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Complex-extended Bohmian mechanics},
 volume    = {132},
 pages     = {134102(1-)},
 year      = {2010},
}

@article{chou:JCP:2011,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Wave front-ray synthesis for solving the multidimensional quantum Hamilton-Jacobi equation},
 volume    = {135},
 pages     = {074102(1-)},
 year      = {2011},
}

@article{chou:PRE:2006,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {Phys. Rev. E},
 title     = {Computational method for the quantum Hamilton-Jacobi equation: One-dimensional scattering problems},
 volume    = {74},
 pages     = {066702(1-)},
 year      = {2006},
}

@article{chou:PRA:2007,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {Phys. Rev. A},
 title     = {Quantum trajectories in complex space},
 volume    = {76},
 pages     = {012115(1-)},
 year      = {2007},
}

@article{chou:PRA:2008,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {Phys. Rev. A},
 title     = {Considerations on the probability density in complex space},
 volume    = {78},
 pages     = {044101(1-)},
 year      = {2007},
}

@article{chou:PRL:2011,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {Phys. Rev. Lett.},
 title     = {Scattered wave packet formalism with Markovian outgoing wave boundary conditions for open quantum systems},
 volume    = {107},
 pages     = {030401(1-)},
 year      = {2011},
}

@article{chou:PRA:2011,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {Phys. Rev. A},
 title     = {Scattered-wave-packet formalism with applications to barrier scattering and quantum transistors},
 volume    = {84},
 pages     = {056707(1-)},
 year      = {2011},
}

@article{trahan:JCP:2003,
 author    = {C. J. Trahan and K. Hughes and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {A new method for wave packet dynamics: Derivative propagation along quantum trajectories},
 volume    = {118},
 pages     = {9911-},
 year      = {2003},
}

@article{yang:AnnPhys-1:2005,
 author    = {C.-D. Yang},
 journal   = {Ann. Phys.},
 title     = {Quantum dynamics of hydrogen atom in complex space},
 volume    = {319},
 pages     = {399-443},
 year      = {2005},
}

@article{yang:AnnPhys-2:2005,
 author    = {C.-D. Yang},
 journal   = {Ann. Phys.},
 title     = {Wave-particle duality in complex space},
 volume    = {319},
 pages     = {445-470},
 year      = {2005},
}

@article{yang:IJQC:2006,
 author    = {C.-D. Yang},
 journal   = {Int. J. Quantum Chem.},
 title     = {Solving quantum trajectories in Coulomb potential by quantum Hamilton-Jacobi theory},
 volume    = {106},
 pages     = {1620-1639},
 year      = {2006},
}

@article{yang:CSF-1:2006,
 author    = {C.-D. Yang},
 journal   = {Chaos, Solitons \& Fractals},
 title     = {On modeling and visualizing single-electron spin motion},
 volume    = {30},
 pages     = {41-50},
 year      = {2006},
}

@article{yang:CSF-2:2006,
 author    = {C.-D. Yang},
 journal   = {Chaos, Solitons \& Fractals},
 title     = {Modeling quantum harmonic oscillator in complex domain},
 volume    = {30},
 pages     = {342-362},
 year      = {2006},
}

@article{yang:AnnPhys:2006,
 author    = {C.-D. Yang},
 journal   = {Ann. Phys.},
 title     = {Quantum Hamilton mechanics: Hamilton equations of quantum motion, origin of quantum operators, and proof of quantization axiom},
 volume    = {321},
 pages     = {2876-2926},
 year      = {2006},
}

@article{yang:CSF-1:2007,
 author    = {C.-D. Yang},
 journal   = {Chaos, Solitons \& Fractals},
 title     = {The origin and proof of quantization axiom ${\bf p} \to \hat{\bf p} = -i\hbar\nabla$ in complex spacetime},
 volume    = {32},
 pages     = {274-283},
 year      = {2007},
}

@article{yang:CSF-2:2007,
 author    = {C.-D. Yang},
 journal   = {Chaos, Solitons \& Fractals},
 title     = {Complex tunneling dynamics},
 volume    = {32},
 pages     = {312-345},
 year      = {2007},
}

@article{yang:CSF-3:2007,
 author    = {C.-D. Yang},
 journal   = {Chaos, Solitons \& Fractals},
 title     = {Quantum motion in complex space},
 volume    = {33},
 pages     = {1073-1092},
 year      = {2007},
}

@article{yang:CSF-4:2007,
 author    = {C.-D. Yang and C.-H. Wei},
 journal   = {Chaos, Solitons \& Fractals},
 title     = {Parameterization of all path integral trajectories},
 volume    = {33},
 pages     = {118-134},
 year      = {2007},
}

@article{chou:PLA:2010,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Geometric phase within the complex quantum Hamilton-Jacobi formalism},
 volume    = {374},
 pages     = {2608-2613},
 year      = {2010},
}

@article{chou:PLA:2009,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Arbitrary Lagrangian-Eulerian rate equation for the Born probability density in complex space},
 volume    = {373},
 pages     = {1811-1817},
 year      = {2009},
}

@article{chou:IJQC:2008,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {Int. J. Quantum Chem.},
 title     = {Riccati differential equation for quantum mechanical bound states: Comparison of numerical integrators},
 volume    = {108},
 pages     = {238-248},
 year      = {2008},
}

@article{swinney:PhysicaD:1985,
 author    = {A. Wolf and J. B. Swift and H. L. Swinney and J. A. Vastano},
 journal   = {Physica D},
 title     = {},
 volume    = {16},
 pages     = {285-},
 year      = {1985},
}

@article{greene:PhysicaD:1987,
 author    = {J. M. Greene},
 journal   = {Physica D},
 title     = {},
 volume    = {24},
 pages     = {213-},
 year      = {1987},
}

@BOOK{baker-bk:1996,
  AUTHOR     = {G. L. Baker and J. P. Gollub},
  TITLE      = {Chaotic Dynamics: An Introduction},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {1996},
  address    = {Cambridge},
  edition    = {2nd Ed.},
}

@BOOK{jordan-bk:1999,
  AUTHOR     = {D. W. Jordan and P. Smith},
  TITLE      = {Nonlinear Ordinary Differential Equations},
  PUBLISHER  = {Oxford University Press},
  YEAR       = {1999},
  address    = {Oxford},
  edition    = {3rd Ed.},
}

@article{bowman:PLA:2002,
 author    = {G. E. Bowman},
 journal   = {Phys. Lett. A},
 title     = {Wave packets and Bohmian mechanics in the kicked rotator},
 volume    = {298},
 pages     = {7-17},
 year      = {2002},
}

@article{frieden:PhysicaA:2009,
 author    = {B. Roy Frieden and B. H. Soffer},
 journal   = {Physica A},
 title     = {de Broglie's wave hypothesis from Fisher information},
 volume    = {388},
 pages     = {1315-1330},
 year      = {2002},
}

@article{rosen:AJP-1:1964,
 author    = {N. Rosen},
 journal   = {Am. J. Phys.},
 title     = {Identical motion in quantum and in classical mechanics},
 volume    = {32},
 pages     = {377-379},
 year      = {1964},
}

@article{rosen:AJP-2:1964,
 author    = {N. Rosen},
 journal   = {Am. J. Phys.},
 title     = {The relation between classical and quantum mechanics},
 volume    = {32},
 pages     = {597-600},
 year      = {1964},
}

@article{rosen:AJP:1965,
 author    = {N. Rosen},
 journal   = {Am. J. Phys.},
 title     = {Mixed states in classical mechanics},
 volume    = {33},
 pages     = {146-150},
 year      = {1965},
}

@article{rosen:FoundPhys:1986,
 author    = {N. Rosen},
 journal   = {Found. Phys.},
 title     = {Quantum particles and classical particles},
 volume    = {16},
 pages     = {687-700},
 year      = {1986},
}

@article{allori:JOptB:2002,
 author    = {V. Allori and Detlef D\"urr and N. Zangh{\`\i} and S. Goldstein},
 journal   = {J. Opt. B},
 title     = {Seven steps toward the classical world},
 volume    = {4},
 pages     = {482-488},
 year      = {2002},
}

@inproceedings{berry:LesHouches:1991,
  AUTHOR     = {M. V. Berry},
  CHAPTER    = {Some quantum-to-classical asymptotics},
  editor     = {M.-J. Giannoni and A. Voros and J. Zinn-Justin},
  booktitle  = {Chaos and Quantum Physics},
  pages      = {251-304},
  PUBLISHER  = {North-Holland},
  YEAR       = {1996},
  address    = {Amsterdam},
  series     = {Les Houches Lecture Series LII (1989)},
}

@BOOK{child-bk:1974,
  AUTHOR     = {M. S. Child},
  TITLE      = {Molecular Collision Theory},
  PUBLISHER  = {Academic Press},
  YEAR       = {1974},
  address    = {London},
}

@BOOK{bolivar-bk:2004,
  AUTHOR     = {A. O. Bolivar},
  TITLE      = {Quantum-Classical Correspondence. Dynamical Quantization and the Classical Limit},
  PUBLISHER  = {Springer},
  YEAR       = {2004},
  address    = {Berlin},
}

@article{bolivar:CanJPhys:2003,
 author    = {A. O. Bolivar},
 journal   = {Can. J. Phys.},
 title     = {The Bohm quantum potential and the classical limit of quantum mechanics},
 volume    = {81},
 pages     = {971-976},
 year      = {2003},
}

@article{makowski:PRA-1:2002,
 author    = {A. J. Makowski},
 journal   = {Phys. Rev. A},
 title     = {Exact classical limit of quantum mechanics: Central potentials and specific states},
 volume    = {65},
 pages     = {032103(1-5)},
 year      = {2002},
}

@article{makowski:PRA-2:2002,
 author    = {A. J. Makowski and K. J. G\'orska},
 journal   = {Phys. Rev. A},
 title     = {Bohr's correspondence principle: The cases for which it is exact},
 volume    = {66},
 pages     = {062103(1-6)},
 year      = {2002},
}

@article{bohm:PRL:1985,
 author    = {D. Bohm and B. J. Hiley},
 journal   = {Phys. Rev. Lett.},
 title     = {Unbroken quantum realism, from microscopic to macroscopic levels},
 volume    = {55},
 pages     = {2511-2514},
 year      = {1985},
}

@BOOK{holland-cushing-bk:1996,
  AUTHOR     = {P. R. Holland},
  CHAPTER    = {Is quantum mechanics universal?},
  editor     = {J. T. Cushing and A. Fine and S. Goldstein},
  TITLE      = {Bohmian Mechanics and Quantum Theory: An Appraisal},
  pages      = {99-220},
  PUBLISHER  = {Kluwer},
  YEAR       = {1996},
  address    = {Dordrecht},
}

@BOOK{cushing-butterfield-bk:1999,
  AUTHOR     = {J. T. Cushing},
  CHAPTER    = {Bohmian mechanics and chaos},
  editor     = {J. Butterfield and C. Pagonis},
  TITLE      = {From Physics to Philosophy},
  pages      = {90-107},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {1999},
  address    = {Cambridge},
}

@article{matzkin:PLA:2007,
 author    = {A. Matzkin},
 journal   = {Phys. Lett. A},
 title     = {Can Bohmian trajectories account for quantum recurrences having classical periodicities?},
 volume    = {361},
 pages     = {294-300},
 year      = {2007},
}

@article{matzkin:SHPMP:2008,
 author    = {A. Matzkin and V. Nurock},
 journal   = {Studies in History and Philosophy of Modern Physics B},
 title     = {Classical and Bohmian trajectories in semiclassical systems: Mismatch in dynamics, mismatch in reality?},
 volume    = {39},
 pages     = {17-40},
 year      = {2008},
}

@article{matzkin:JPCS:2009,
 author    = {A. Matzkin},
 journal   = {J. Phys.: Conf. Ser.},
 title     = {Bohmian mechanics and the emergence of classicality},
 volume    = {174},
 pages     = {012039(1-8)},
 year      = {2009},
}

@article{matzkin:FoundPhys:2009,
 author    = {A. Matzkin and V. Nurock},
 journal   = {Found. Phys.},
 title     = {Bohmian Mechanics, the quantum-classical correspondence and the classical limit: The case of the square billiard},
 volume    = {39},
 pages     = {903-920},
 year      = {2009},
}

@article{na:PLA:2002,
 author    = {K. Na and R. E. Wyatt},
 journal   = {Phys. Lett. A},
 title     = {Quantum hydrodynamic analysis of decoherence: quantum trajectories and stress tensor},
 volume    = {306},
 pages     = {97-103},
 year      = {2002},
}

@article{na:PhysScr:2003,
 author    = {K. Na and R. E. Wyatt},
 journal   = {Phys. Scr.},
 title     = {Quantum hydrodynamic analysis of decoherence},
 volume    = {67},
 pages     = {169-180},
 year      = {2003},
}

@article{struyve:JPA:2003,
 author    = {W. Struyve and W. De Baere and J. De Neve and S. De Weirdt},
 journal   = {J. Phys. A},
 title     = {Comment on `Bohmian prediction about a two double-slit experiment and its disagreement with standard quantum mechanics'},
 volume    = {36},
 pages     = {1525-1530},
 year      = {2003},
}

@article{marchildon:JPA:2003,
 author    = {E. Guay and L. Marchildon},
 journal   = {J. Phys. A},
 title     = {Two-particle interference in standard and Bohmian quantum mechanics},
 volume    = {36},
 pages     = {5617-5624},
 year      = {2003},
}

@article{marchildon:JModOpt:2003,
 author    = {L. Marchildon},
 journal   = {J. Mod. Opt.},
 title     = {Two-particle interference devices and compatibility of Bohmian and standard quantum mechanics},
 volume    = {50},
 pages     = {873-879},
 year      = {2003},
}

@article{hiley:FoundPhys:1999,
 author    = {O. Maroney and B. J. Hiley},
 journal   = {Found. Phys.},
 title     = {Quantum state teleportation understood through the Bohm interpretation},
 volume    = {29},
 pages     = {1403-1415},
 year      = {1999},
}

@article{golshani:JPA:2001,
 author    = {M. Golshani and O. Akhavan},
 journal   = {J. Phys. A},
 title     = {Bohmian prediction about a two double-slit experiment and its disagreement with standard quantum mechanics},
 volume    = {34},
 pages     = {5259-5268},
 year      = {2001},
 doi       = {10.1088/0305-4470/34/25/308},
}

@article{ghose:PRAMANA:2002,
 author    = {P. Ghose},
 journal   = {PRAMANA},
 title     = {On the incompatibility of standard quantum mechanics and conventional de Broglie-Bohm theory},
 volume    = {59},
 pages     = {417-424},
 year      = {2002},
 doi       = {10.1007/s12043-002-0136-y},
 url       = {https://doi.org/10.1007/s12043-002-0136-y},
}

@article{dewdney:PLA:1990,
 author    = {M. M. Lam and C. Dewdney},
 journal   = {Phys. Lett. A},
 title     = {Locality and nonlocality in correlated two-particle interferometry},
 volume    = {150},
 pages     = {127-135},
 year      = {1990},
}

@article{dewdney:FoundPhys:1988,
 author    = {C. Dewdney},
 journal   = {Found. Phys.},
 title     = {Nonlocally correlated trajectories in two-particle quantum mechanics},
 volume    = {18},
 pages     = {867-886},
 year      = {1988},
}

@article{maddox:JCP:2001,
 author    = {J. B. Maddox and E. R. Bittner},
 journal   = {J. Chem. Phys.},
 title     = {Quantum relaxation dynamics using Bohmian trajectories},
 volume    = {115},
 pages     = {6309-6316},
 year      = {2001},
}

@article{maddox:PRE:2002,
 author    = {J. B. Maddox and E. R. Bittner},
 journal   = {Phys. Rev. E},
 title     = {Quantum dissipation in unbounded systems},
 volume    = {65},
 pages     = {026143(1-10)},
 year      = {2002},
}

@article{holloway:JCP:2001,
 author    = {Z. S. Wang and G. R. Darling and S. Holloway},
 journal   = {J. Chem. Phys.},
 title     = {Dissociation dynamics from a de Broglie-Bohm perspective},
 volume    = {115},
 pages     = {10373-10381},
 year      = {2001},
}

@article{burghardt:IJQC:2004,
 author    = {I. Burghardt and K. B. M{\o}ller and G. Parlant and L. S. Cederbaum and E. R. Bittner},
 journal   = {Int. J. Quantum Chem.},
 title     = {Quantum hydrodynamics: mixed states, dissipation, and a new hybrid quantum-classical approach},
 volume    = {100},
 pages     = {1153-1162},
 year      = {2004},
}

@article{burghardt:JCP:2004,
 author    = {I. Burghardt and G. Parlant},
 journal   = {J. Chem. Phys.},
 title     = {On the dynamics of coupled Bohmian and phase-space variables: A new hybrid quantum-classical approach},
 volume    = {120},
 pages     = {3055-3058},
 year      = {2004},
}

@article{burghardt:JPCA:2007,
 author    = {K. H. Hughes and S. M. Parry and G. Parlant and I. Burghardt},
 journal   = {J. Phys. Chem. A},
 title     = {A hybrid hydrodynamic-Liouvillian approach to mixed quantum-classical dynamics: Application to tunneling in a double well},
 volume    = {111},
 pages     = {10269-10283},
 year      = {2007},
}

@article{burghardt:JCP-1:2001,
 author    = {I. Burghardt and L. S. Cederbaum},
 journal   = {J. Chem. Phys.},
 title     = {Hydrodynamic equations for mixed quantum states. I. General formulation},
 volume    = {115},
 pages     = {10303-10311},
 year      = {2001},
}

@article{burghardt:JCP-2:2001,
 author    = {I. Burghardt and L. S. Cederbaum},
 journal   = {J. Chem. Phys.},
 title     = {Hydrodynamic equations for mixed quantum states. II. Coupled electronic states},
 volume    = {115},
 pages     = {10312-10322},
 year      = {2001},
}

@article{shnider:SIAM:1999,
 author    = {J. Schiff and S. Schneider},
 journal   = {SIAM J. Numer. Anal.},
 title     = {A natural approach to the numerical integration of Riccati differential equations},
 volume    = {36},
 pages     = {1392-1413},
 year      = {1999},
}

@article{krayzel:JEOS:2010,
 author    = {F. Krayzel and R. Poll\`es and A. Moreau and M. Mihailovic and G. Granet},
 journal   = {J. Eur. Opt. Soc. - Rapid publications},
 title     = {Simulation and analysis of exotic non-specular phenomena},
 volume    = {5},
 pages     = {10025},
 year      = {2010},
}

@article{spin.Bell1971,
 author    = {J. Bell},
 journal   = {Proceedings of the International School of Physics `Enrico Fermi', course IL: Foundations of Quantum Mechanics, New York, Academic},
 pages     = {171-181},
 title     = {Introduction to the hidden variable question},
 volume    = {},
 year      = {1971},
}

@article{spin.Dewdney1986,
 author               = {C. Dewdney and P. R. Holland, and A. Kyprianidis},
 journal              = {Physics Letters},
 pages                = {259-267},
 title                = {What happens in a spin measurement},
 volume               = {119},
 year                 = {1986},
 }

@article{rel.Durr2013,
 author               = {D. D\"urr and S. Goldstein and T. Norsen and W. Struyve and and N. Zangh\`{\i}},
 journal              = {Proc. R. Soc. A},
 pages                = {20130699},
 title                = {Can Bohmian mechanics be made relativistic?},
 volume               = {470},
 year                 = {2013},
 }

@article{rel.Horton2004,
 author               = {G. Horton and C. Dewdney},
 journal              = {J. Phys. A},
 pages                = {11935},
 title                = {A relativistic covariant version of Bohm's quantum field theory for the scalar field},
 volume               = {37},
 year                 = {2004},
 }

@article{rel.Berndl1996,
 author               = {K. Berndl, D. D\"urr, S. Goldstein, and N. Zangh\`{\i}},
 journal              = {Phys. Rev. A},
 pages                = {2062-2073},
 title                = {Nonlocality, Lorentz invariance, and Bohmian quantum theory},
 volume               = {53},
 year                 = {1996},
 }

@article{rel.Horton2001,
 author               = {G. Horton, and C. Dewdney},
 journal              = {J. Phys. A},
 pages                = {9871-9878},
 title                = {A non-local, Lorentz-invariant, hidden-variable interpretation of relativistic quantum mechanics based on particle trajectories},
 volume               = {34},
 year                 = {2001},
 }

@article{rel.Dewdney2002,
 author               = {C. Dewdney, and G. Horton},
 journal              = {J. Phys. A},
 pages                = {10117-10127},
 title                = {Relativistically invariant extension of the de Broglie-Bohm theory of quantum mechanics},
 volume               = {35},
 year                 = {2002},
 }

@article{rel.Tumulka2007,
 author               = {R. Tumulka},
 journal              = {J. Phys. A},
 pages                = {3245-3273},
 title                = {The `unromantic pictures' of quantum theory},
 volume               = {40},
 year                 = {2007},
 }

@article{rel.Tausk2010,
 author               = {D. V. Tausk, and R. Tumulka},
 journal              = {J. Math. Phys.},
 pages                = {122306},
 title                = {Can We Make a Bohmian Electron Reach the Speed of Light, at Least for One Instant?},
 volume               = {51},
 year                 = {2010},
 }


@article{rel.Struyve2010,
 author               = {W. Struyve},
 journal              = {Rep. Prog. Phys.},
 pages                = {106001},
 title                = {Pilot-wave theory and quantum fields},
 volume               = {73},
 year                 = {2010},
 }

@article{qft.Takabayashi1952,
 author               = {T. Takabayashi},
 journal              = {Prog. Theor. Phys.},
 pages                = {143},
 title                = {On the Formulation of Quantum Mechanics associated with Classical Picturess},
 volume               = {8},
 year                 = {1952},
 }

@article{qft.Holland1988,
 author               = {P. R. Holland},
 journal              = {Phys. Lett. A},
 pages                = {9-18},
 title                = {On the Formulation of Quantum Mechanics associated with Classical Picturess},
 volume               = {128},
 year                 = {1988},
 }

@BOOK{qft.Valentini1996,
  AUTHOR     = {A. Valentini},
  CHAPTER    = {},
  editor     = {J.T. Cushing, A. Fine and S. Goldstein},
  TITLE      = {Bohmian Mechanics and quantum Theory: An Appraisal},
  pages      = {},
  PUBLISHER  = {Kluwer, Dordrecht, 45},
  YEAR       = {1996},
  address    = {},
}


@article{qft.Struyve2007,
 author               = {W. Struyve and H. Westman},
 journal              = {Proc. R. Soc. A},
 pages                = {3115-3129},
 title                = {A minimalist pilot-wave model for quantum electrodynamics},
 volume               = {463},
 year                 = {2007},
 }

@article{qc.Callender1994,
 author               = {C. Callender, and R. Weingard},
 journal              = {PSA: Proceedings of the Biennial Meeting of the Philosophy of Science Association 1994},
 pages                = {218-227},
 title                = {The Bohmian Model of Quantum Cosmology},
 volume               = {},
 year                 = {1994},
 }

@article{qc.Pinto2005,
 author               = {N. Pinto-Neto},
 journal              = {Found. Phys.},
 pages                = {577-603},
 title                = {The Bohm interpretation of quantum cosmology},
 volume               = {35},
 year                 = {2005},
 }

@article{qc.Shojai2007,
 author               = {F. Shojai, and S. Molladovoudi},
 journal              = {Gen. Rel. Grav.},
 pages                = {795-813},
 title                = {Quantum cosmology with varying speed of light and Bohmian trajectories},
 volume               = {39},
 year                 = {2007},
 }


@article{qc.deBarros1998,
 author               = {J. A. de Barros, N. Pinto-Neto, M. A. Sagioro-Leal},
 journal              = {Phys. Lett. A},
 pages                = {229-239},
 title                = {The causal interpretation of dust and radiation fluid non-singular quantum cosmologies},
 volume               = {241},
 year                 = {1998},
 }


@article{qc.Shojai1998,
 author               = {F. Shojai and M. Golshani},
 journal              = {Int. J. Mod. Phys. A},
 pages                = {677-693},
 title                = {On the geometrization of Bohmian mechanics; a new approach to quantum gravity},
 volume               = {13},
 year                 = {1998},
 }

@article{qc.Pinto2005b,
 author               = {N. Pinto-Neto, E. Sergio Santini, and F. T. Falciano},
 journal              = {Phys. Lett. A},
 pages                = {131-143},
 title                = {Quantization of Friedmann cosmological models with two fluids: Dust plus radiation},
 volume               = {344},
 year                 = {2005},
 }

@article{qc.Colin2013,
 author               = {S. Colin, and A. Valentini},
 journal              = {Phys. Rev. D},
 pages                = {103515},
 title                = {Mechanism for the suppression of quantum noise at large scales on expanding space},
 volume               = {88},
 year                 = {2013},
 }

@article{gindensperger:JCP:2000,
  author   = {E. Gindensperger and C. Meier and J. A. Beswick},
  journal  = {J. Chem. Phys.},
  title    = {Communications: Mixing quantum and classical dynamics using Bohmian trajectories},
  volume   = {113},
  pages    = {9369-9372},
  year     = {2000},
}

@article{gindensperger:JCP:2002-1,
  author   = {E. Gindensperger and C. Meier and J. A. Beswick},
  journal  = {J. Chem. Phys.},
  title    = {Quantum-classical dynamics including continuum states using quantum trajectories},
  volume   = {116},
  pages    = {8-13},
  year     = {2002},
}

@article{gindensperger:JCP:2002-2,
  author   = {E. Gindensperger and C. Meier and J. A. Beswick},
  journal  = {J. Chem. Phys.},
  title    = {Quantum-classical description of rotational diffractive scattering using Bohmian trajectories: Comparison with full quantum wave packet results},
  volume   = {116},
  pages    = {10051-10059},
  year     = {2002},
}

@article{gindensperger:AdvQuantChem:2004,
  author   = {E. Gindensperger and C. Meier and J. A. Beswick},
  journal  = {Adv. Quant. Chem.},
  title    = {Hybrid quantum/classical dynamics using Bohmian trajectories},
  volume   = {47},
  pages    = {331-346},
  year     = {2004},
}

@article{meier:JCP:2004,
  author   = {C. Meier and J. A. Beswick},
  journal  = {J. Chem. Phys.},
  title    = {Femtosecond pump-probe spectroscopy of I$_2$ in a dense rare gas environment: A mixed quantum-classical study of vibrational decoherence},
  volume   = {121},
  pages    = {4550-4558},
  year     = {2004},
}

@article{meier:PRL:2004,
  author   = {C. Meier},
  journal  = {Phys. Rev. Lett.},
  title    = {Mixed quantum-classical treatment of vibrational decoherence},
  volume   = {93},
  pages    = {173003(1-4)},
  year     = {2004},
}

@inproceedings{drezet:ch:2014,
  AUTHOR    = {A. Drezet},
  editor    = {S. Gao},
  booktitle = {Protective Measurements and Quantum Reality: Toward a New Understanding of Quantum Mechanics},
  CHAPTER   = {Implications of protective measurements on de Broglie-Bohm trajectories},
  pages     = {},
  PUBLISHER = {Cambridge University Press},
  YEAR      = {2014},
  address   = {Cambridge},
  eprint    = {arXiv:1402.7256},
}

@article{durt:PRA:2002,
 author    = {T. Durt and Y. Pierseaux},
 journal   = {Phys. Rev. A},
 title     = {Bohm's interpretation and maximally entangled states},
 volume    = {66},
 pages     = {052109(1-11)},
 year      = {2002},
}

@article{tannor:JCP:2014,
 author    = {N. Zamstein and D. J. Tannor},
 journal   = {J. Chem. Phys.},
 title     = {Communication: Overcoming the root search problem in complex quantum trajectory calculations},
 volume    = {140},
 pages     = {041105},
 year      = {2014},
}

@article{tannor:JCP-1:2012,
 author    = {N. Zamstein and D. J. Tannor},
 journal   = {J. Chem. Phys.},
 title     = {Non-adiabatic molecular dynamics with complex quantum trajectories. I. The diabatic representation},
 volume    = {137},
 pages     = {22A517},
 year      = {2012},
}

@article{tannor:JCP-2:2012,
 author    = {N. Zamstein and D. J. Tannor},
 journal   = {J. Chem. Phys.},
 title     = {Non-adiabatic molecular dynamics with complex quantum trajectories. II. The adiabatic representation},
 volume    = {137},
 pages     = {22A518},
 year      = {2012},
}

@article{rubi:PRE:2001,
 author    = {D. Reguera and M. Rub{\'\i}},
 journal   = {Phys. Rev. E},
 title     = {Kinetic equations for diffusion in the presence of entropic barriers},
 volume    = {64},
 pages     = {061106(1-8)},
 year      = {2001},
}

@article{schuch:PhysScr:2013,
 author    = {D. Schuch},
 journal   = {Phys. Scr.},
 title     = {Is quantum theory intrinsically nonlinear?},
 volume    = {87},
 pages     = {038117(1-10)},
 year      = {2013},
}

@article{schuch:IJQC:1986,
 author    = {D. Schuch},
 journal   = {Int. J. Quantum. Chem.},
 title     = {},
 volume    = {29},
 pages     = {1561-},
 year      = {1986},
}

@article{davisson:PR:1927,
 author    = {C. Davisson and L. H. Germer},
 journal   = {Phys. Rev.},
 title     = {Diffraction of Electrons by a Crystal of Nickel},
 volume    = {30},
 pages     = {705-740},
 year      = {1927},
}

@article{davisson:Nature:1927,
 author    = {C. Davisson and L. H. Germer},
 journal   = {Nature},
 title     = {Reflection of electrons by a crystal of nickel},
 volume    = {119},
 pages     = {558-560},
 year      = {1927},
}

@article{stern:ZPhys:1929,
 author    = {P. Knauer and O. Stern},
 journal   = {Z. Physik},
 title     = {Intensit\"atsmessungen an Molekularstrahlen von Gasen},
 volume    = {53},
 pages     = {766-778},
 year      = {1929},
}

@article{stern:ZPhys:1930,
 author    = {I. Estermann and O. Stern},
 journal   = {Z. Physik},
 title     = {Beugung von Molekularstrahlen},
 volume    = {61},
 pages     = {95-125},
 year      = {1930},
}

@article{stern:ZPhys:1931,
 author    = {I. Estermann and R. Frisch and O. Stern},
 journal   = {Z. Physik},
 title     = {Monochromasierung der de Broglie-Wellen von Molekularstrahlen},
 volume    = {73},
 pages     = {348-365},
 year      = {1931},
}

@article{peres:SHPMP:2002,
 author    = {A. Peres},
 journal   = {Stud. History Philos. Modern Physics},
 title     = {Karl Popper and the Copenhagen interpretation},
 volume    = {33},
 pages     = {23-34},
 year      = {2002},
}

@article{zeilinger:RMP:1988,
 author    = {A. Zeilinger and R. G\"ahler and C. G. Shull and W. Treimer and W. Mampe},
 journal   = {Rev. Mod. Phys.},
 title     = {Single- and double-slit diffraction of neutrons},
 volume    = {60},
 pages     = {1067-1073},
 year      = {1988},
}

@article{zeilinger:AJP:1991,
 author    = {R. G\"ahler and A. Zeilinger},
 journal   = {Am. J. Phys.},
 title     = {Wave-optical experiments with very cold neutrons},
 volume    = {59},
 pages     = {316-324},
 year      = {1991},
}

@article{arndt:Nature:1999,
 author    = {M. Arndt and O. Nairz and J. Vos-Andreae and C. Keller and G. van der Zouw and A. Zeilinger},
 journal   = {Nature},
 title     = {Wave-particle duality of C$_{60}$ molecules},
 volume    = {401},
 pages     = {680-682},
 year      = {1999},
}

@article{arndt:PRL:2003,
 author    = {L. Hackerm\"uller and S. Uttenthaler and K. Hornberger and E. Reiger and B. Brezger and A. Zeilinger and M. Arndt},
 journal   = {Phys. Rev. Lett.},
 title     = {Wave nature of biomolecules and fluorofullerenes},
 volume    = {91},
 pages     = {90408(1-4)},
 year      = {2003},
}

@article{arndt:Angew:2008,
 author    = {S. Gerlich and M. Gring and H. Ulbricht and K. Hornberger and J. T\"uxen and M. Mayor and M. Arndt},
 journal   = {Angew. Chem. Int. Ed.},
 title     = {Matter-wave metrology as a complementary tool for mass spectrometry},
 volume    = {47},
 pages     = {6195-6198},
 year      = {2008},
}

@article{arndt:NatPhys:2007,
 author    = {S. Gerlich and L. Hackerm\"uller and K. Hornberger and A. Stibor and H. Ulbricht and M. Gring and F. Goldfarb and T. Savas and M. M\"uri and M. Mayor and M. Arndt},
 journal   = {A Kapitza-Dirac-Talbot-Lau interferometer for highly polarizable molecules},
 title     = {Nature Phys.},
 volume    = {3},
 pages     = {711-715},
 year      = {2007},
}

@article{sanz:AOP:2014,
 author    = {A. S. Sanz and R. Mart{\'\i}nez-Casado and H. C. Pe\~nate-Rodr{\'\i}guez and G. Rojas-Lorenzo and S. Miret-Art\'es},
 journal   = {Ann. Phys.},
 title     = {Dissipative Bohmian mechanics within the Caldirola-Kanai framework: A trajectory analysis of wave-packet dynamics in viscid media},
 volume    = {347},
 pages     = {1-20},
 year      = {2014},
}

@article{furth:ZPhys:1933,
 author    = {R. F\"urth},
 journal   = {Z. Phys.},
 title     = {\"Uber einige Beziehungen zwischen klassischer Statistik und Quantenmechanik},
 volume    = {81},
 pages     = {143-162},
 year      = {1933},
}

@article{comisar:PhysRev:1965,
 author    = {G. G. Comisar},
 journal   = {Phys. Rev.},
 title     = {Brownian-motion model of nonrelativistic quantum mechanics},
 volume    = {138},
 pages     = {B1332-B1337},
 year      = {1965},
}

@BOOK{fourier-bk,
  AUTHOR     = {J. B. J. Fourier},
  TITLE      = {Th\'eorie analytique de la chaleur},
  PUBLISHER  = {Firmin Didot P\`ere et Fils},
  YEAR       = {1822},
  address    = {Paris},
}

@BOOK{fourier-bk-eng,
  AUTHOR     = {J. B. J. Fourier},
  TRANSLATOR = {A. Freeman},
  TITLE      = {The Analytical Theory of Heat},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {2009},
  address    = {Cambridge},
}

@article{hobson:AJP:2013,
 author    = {A. Hobson},
 journal   = {Am. J. Phys.},
 title     = {There are no particles, there are only fields},
 volume    = {81},
 pages     = {211-223},
 year      = {2013},
}

@article{leon:AOP:2014,
 author    = {M. Rodr{\'\i}guez-V\'azquez and M. del Rey and H. Westman and J. Le\'on},
 journal   = {Ann. Phys.},
 title     = {Local quanta, unitary inequivalence, and vacuum entanglement},
 volume    = {351},
 pages     = {112-137},
 year      = {2014},
}

@article{wilbraham:CDMJ:1848,
 author    = {H. Wilbraham},
 journal   = {Camb. Dublin Math. J.},
 title     = {On a certain periodic function},
 volume    = {3},
 pages     = {198-201},
 year      = {1848},
}

@article{gibbs:Nature:1898,
 author    = {J. W. Gibbs},
 journal   = {Nature},
 title     = {Fourier's series},
 volume    = {59},
 pages     = {200},
 year      = {1898},
}

@article{gibbs:Nature:1899,
 author    = {J. W. Gibbs},
 journal   = {Nature},
 title     = {Fourier's series},
 volume    = {59},
 pages     = {606},
 year      = {1899},
}

@BOOK{Mehra-Feynman-bk,
  AUTHOR     = {J. Mehra},
  TITLE      = {The Beat of a Different Drum: The Life and Science of Richard Feynman},
  PUBLISHER  = {Oxford University Press},
  YEAR       = {1994},
  address    = {Oxford},
}

@BOOK{hawking-bk,
  AUTHOR     = {S. J. Hawking},
  TITLE      = {The Dreams that Stuff is Made of},
  PUBLISHER  = {Running Press},
  YEAR       = {2011},
  address    = {Philadephia, PA},
}

@BOOK{waerden-bk,
  AUTHOR     = {B. L. van der Waerden},
  TITLE      = {Sources of Quantum Mechanics},
  PUBLISHER  = {Dover},
  YEAR       = {1966},
  address    = {New York},
}

@BOOK{broglie-bk:1960,
  AUTHOR     = {L. de Broglie},
  TITLE      = {Non-Linear Wave Mechanics. A Causal Interpretation},
  PUBLISHER  = {Elsevier},
  YEAR       = {1960},
  address    = {Amsterdam},
}

@BOOK{jadczyk-bk:2014,
  AUTHOR     = {A. Jadczyk},
  TITLE      = {Quantum Fractals. From Heisenberg's Uncertainty to Barnsley's Fractality},
  PUBLISHER  = {World Scientific},
  YEAR       = {2014},
  address    = {Singapore},
}

@article{ehrenberg:PPSB:1949,
 author    = {W. Ehrenberg and R. E. Siday},
 journal   = {Proc. Phys. Soc. B},
 title     = {The refractive index in electron optics and the principles of dynamics},
 volume    = {62},
 pages     = {8-21},
 year      = {1949},
}

@article{feynman:RMP:1948,
 author    = {P. R. Feynman},
 journal   = {Rev. Mod. Phys.},
 title     = {Space-time approach to non-relativistic quantum mechanics},
 volume    = {20},
 pages     = {367-387},
 year      = {1948},
}

@article{sanz:foundphys:2015,
 author    = {A. S. Sanz},
 journal   = {Found. Phys.},
 title     = {Investigating puzzling aspects of the quantum theory by means of its hydrodynamic formulation},
 volume    = {45},
 pages     = {1153-1165},
 year      = {2015},
}

@BOOK{kant:1781,
  AUTHOR     = {I. Kant},
  TITLE      = {Critique of Pure Reason},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {1781 [1998]},
  address    = {Cambridge},
  note       = {Trans. by P. Guyer and A. W.Wood},
  series     = {The Cambridge Edition of the Works of Immanuel Kant},
}

@BOOK{nielsen-chuang-bk,
  AUTHOR     = {M. A. Nielsen and I. L. Chuang},
  TITLE      = {Quantum Computation and Quantum Information},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {2000},
  address    = {Cambridge},
}

@BOOK{marage-wallenborn-bk,
  editor     = {P. Marage and G. Wallenborn},
  TITLE      = {The Solvay Councils and the Birth of Modern Physics},
  PUBLISHER  = {Birkh\"auser},
  YEAR       = {1999},
  series     = {Science Networks. Historical Studies},
  volume     = {22},
  address    = {Basel},
}

@BOOK{bacciagaluppi-valentini-bk,
  editor     = {G. Bacciagaluppi and A. Valentini},
  TITLE      = {Quantum Theory at the Crossroads. Reconsidering the 1927 Solvay Conference},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {2009},
  series     = {Science Networks. Historical Studies},
  address    = {Cambridge},
}

@article{benseny:EPJD:2014,
 author    = {A. Benseny and G. Albareda and A. S. Sanz and J. Mompart and X. Oriols},
 journal   = {Eur. Phys. J. D},
 title     = {Applied Bohmian mechanics},
 volume    = {68},
 pages     = {286(1-42)},
 year      = {2014},
}

@article{milena:JRLR:2015,
 author    = {M. Davidovi\'c and M. Bo\v{z}i\'c and A. S. Sanz},
 journal   = {J. Russ. Laser Res.},
 pages     = {329-342},
 title     = {Description of classical and quantum interference in view of the concept of flow line},
 volume    = {36},
 year      = {2015},
}

@article{zeh:FoundPhys:1973,
 author    = {H. D. Zeh},
 journal   = {Found. Phys.},
 title     = {Toward a quantum theory of observation},
 volume    = {3},
 pages     = {109-116},
 year      = {1973},
}

@article{schlosshauer:RMP:2004,
  title = {Decoherence, the measurement problem, and interpretations of quantum mechanics},
  author = {Schlosshauer, Maximilian},
  journal = {Rev. Mod. Phys.},
  volume = {76},
  issue = {4},
  pages = {1267--1305},
  numpages = {0},
  year = {2005},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.76.1267},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.76.1267}
}

@article{schrodinger:ProcCamPS:1935,
 author    = {E. Schr\"odinger},
 journal   = {Math. Proc. Cambridge Philos. Soc.},
 title     = {Discussion of probability relations between separated systems},
 volume    = {31},
 pages     = {555-563},
 year      = {1935},
 doi       = {10.1017/S0305004100013554},
}

@article{schrodinger:ProcCamPS:1936,
 author    = {E. Schr\"odinger},
 journal   = {Math. Proc. Cambridge Philos. Soc.},
 title     = {Probability between separated systems},
 volume    = {32},
 pages     = {446-452},
 year      = {1936},
 doi       = {10.1017/S0305004100019137},
}

@article{luis:AOP:2015,
 author    = {A. Luis and A. S. Sanz},
 journal   = {Ann. Phys.},
 title     = {What dynamics can be expected for mixed states in two-slit experiments?},
 volume    = {357},
 pages     = {95-107},
 year      = {2015},
}

@article{batelaan:NJP:2013,
 author    = {R. Bach and D. Pope and S.-H. Liou and H. Batelaan},
 journal   = {New J. Phys.},
 title     = {Controlled double-slit electron diffraction},
 volume    = {15},
 pages     = {033018(1-7)},
 year      = {2013},
}

@article{walls:PRA:1993,
  title = {Loss of coherence in interferometry},
  author = {Tan, S. M. and Walls, D. F.},
  journal = {Phys. Rev. A},
  volume = {47},
  issue = {6},
  pages = {4663--4676},
  numpages = {0},
  year = {1993},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.47.4663},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.47.4663}
}

@article{walls:Nature:1994,
 author    = {P. Storey and S. Tan and M. Collett and D. Walls},
 journal   = {Nature},
 title     = {Path detection and the uncertainty principle},
 volume    = {357},
 pages     = {626-628},
 year      = {1994},
}

@article{wolf:JOSAA:1957,
 author    = {B. J. Thompson and E. Wolf},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Two-beam interference with partially coherent light},
 volume    = {47},
 pages     = {895-902},
 year      = {1957},
}

@article{zernike:PhysicaV:1938,
 author    = {F. Zernike},
 journal   = {Physica V},
 title     = {The concept of degree of coherence and its application to optical problems},
 volume    = {8},
 pages     = {785-795},
 year      = {1938},
}

@INPROCEEDINGS{sanz:ch-protvino:2015,
  AUTHOR =    {A. S. Sanz},
  TITLE =     {How far can a pragmatist go into quantum theory? -- A critical view of our current understanding of quantum phenomena},
  pages =     {161-171},
  PUBLISHER = {World Scientific},
  YEAR =      {2015},
  crossref =  {petrov-bk:2015},
}

@PROCEEDINGS{petrov-bk:2015,
  editor =    {V. Petrov and R. Ryutin},
  BOOKTITLE = {Particle and Astroparticle Physics, Gravitation and Cosmology: Predictions, Observations and New Projects (Proceedings of the XXXth International Workshop on High Energy Physics)},
  TITLE =     {Particle and Astroparticle Physics, Gravitation and Cosmology: Predictions, Observations and New Projects},
  PUBLISHER = {World Scientific},
  YEAR =      {2015},
  address =   {Singapore},
}

@article{einstein:PhysZeits:1917,
 author    = {A. Einstein},
 journal   = {Physikalische Zeitschrift},
 title     = {Zur Quantentheorie der Strahlung},
 volume    = {18},
 pages     = {121-128},
 year      = {1917},
}

@article{hiley:SHPMP:1997,
 author    = {B. J. Hiley},
 journal   = {Stud. Hist. Phil. Mod. Phys.},
 title     = {Essay Review - Quantum Mechanics: Historical Contingency and the Copenhagen Hegemony by James T. Cushing},
 volume    = {28},
 pages     = {299-305},
 year      = {1997},
}

@article{hiley:JComputElect:2015,
 author    = {B. J. Hiley},
 journal   = {J. Comput. Electron.},
 title     = {On the relationship between the Wigner-Moyal approach and the quantum operator algebra of von Neumann},
 volume    = {14},
 pages     = {869-878},
 year      = {2015},
}

@BOOK{hiley-chap:2016,
 author     = {P. Pylkk\"anen and B. J. Hiley and I. P\"attiniemi},
 editor     = {A. Guay and T. Pradeu},
 title      = {Individuals Across the Sciences},
 CHAPTER    = {Bohm's approach and Individuality},
 pages      = {226-249},
 publisher  = {Oxford University Press},
 year       = {2015},
 address    = {New York},
 preprint   = {arXiv:1405.4772v3 (2014)},
}

@BOOK{bohm-bk:1980,
  AUTHOR     = {D. Bohm},
  TITLE      = {Wholeness and the Implicate Order},
  PUBLISHER  = {Routledge},
  YEAR       = {1980},
  address    = {New York},
}

@BOOK{cushing-bk:1994,
  AUTHOR     = {J. T. Cushing},
  title      = {Quantum Mechanics: Historical Contingency and the Copenhagen Hegemony},
  PUBLISHER  = {University of Chicago Press},
  YEAR       = {1994},
  address    = {Chicago},
}

@article{padgett:AJP:2016,
 author    = {R. S. Aspden and M. J. Padgett and G. C. Spalding},
 journal   = {Am. J. Phys.},
 title     = {Video recording true single-photon double-slit interference},
 volume    = {84},
 pages     = {671-677},
 year      = {2016},
}

@article{sanz:ApplSci:2020,
 author   = {A. S. Sanz and M. Davidovi\'c and M. Bo\v{z}i\'c},
 journal  = {Appl. Sci.},
 title    = {Bohmian-based approach to Gauss-Maxwell beams},
 volume   = {10},
 pages    = {1808(1-25)},
 year     = {2020},
 doi      = {10.3390/app10051808},
 url      = {https://doi.org/10.3390/app10051808},
}

@article{sanz:AOP:2015,
 author    = {A. S. Sanz and M. Davidovi\'c and M. Bo\v{z}i\'c},
 journal   = {Ann. Phys.},
 pages     = {205-221},
 title     = {Full quantum mechanical analysis of atomic three-grating Mach-Zehnder interferometry},
 volume    = {353},
 year      = {2015},
 doi       = {10.1016/j.aop.2014.11.012},
 url       = {https://doi.org/10.1016/j.aop.2014.11.012},
}

@BOOK{sanz:springer:2006,
  AUTHOR     = {A. S. Sanz and S. Miret-Art\'es},
  editor     = {D. A. Micha and I. Burghardt},
  title      = {Quantum Dynamics of Complex Molecular Systems},
  CHAPTER    = {Atom-surface diffraction: A quantum trajectory description},
  pages      = {343-368},
  publisher  = {Springer},
  year       = {2007},
  address    = {Berlin},
}

@article{tumulka:EJP:2005,
 author    = {R. Tumulka},
 journal   = {Eur. J. Phys.},
 title     = {Feynman's path integrals and Bohm's particle paths},
 volume    = {26},
 pages     = {L11-L13},
 year      = {2005},
}

@BOOK{hiley:vaxjo:2003,
  AUTHOR     = {B. J. Hiley},
  editor     = {A. Khrennikov},
  title      = {Quantum Theory: Reconsiderations of Foundations - 2},
  CHAPTER    = {Phase space descriptions of quantum phenomena},
  pages      = {267-286},
  publisher  = {V\"axj\"o University Press},
  year       = {2003},
  address    = {V\"axj\"o},
}

@article{EPR:PhysRev:1935,
  title = {Can Quantum-Mechanical Description of Physical Reality Be Considered Complete?},
  author = {Einstein, A. and Podolsky, B. and Rosen, N.},
  journal = {Phys. Rev.},
  volume = {47},
  issue = {10},
  pages = {777--780},
  numpages = {0},
  year = {1935},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.47.777},
  url = {https://link.aps.org/doi/10.1103/PhysRev.47.777}
}

@article{milburn:PTRSLA:2003,
 author    = {J. P. Dowling and G. J. Milburn},
 journal   = {Phil. Trans. Roy. Soc. Lond. A},
 title     = {Quantum technology: The second quantum revolution},
 volume    = {361},
 pages     = {1655-1674},
 year      = {2003},
 doi       = {10.1098/rsta.2003.1227},
 url       = {https://doi.org/10.1098/rsta.2003.1227},
}

@article{hiley:BMFRS:1997,
 author    = {B. J. Hiley},
 journal   = {Biogr. Mems. Fell. R. Soc.},
 title     = {David Joseph Bohm. 20 December 1917 -- 27 October 1992: Elected F.R.S. 1990},
 volume    = {43},
 pages     = {107-131},
 year      = {1997},
}

@article{ziman:PRSL:1953,
 author    = {J. M. Ziman},
 journal   = {Proc. Roy. Soc. Lond. A},
 title     = {Quantum hydrodynamics and the theory of liquid helium},
 volume    = {219},
 pages     = {257-270},
 year      = {1953},
}

@article{bierter:JLTP:1969,
 author    = {W. Bierter and H. L. Morrison},
 journal   = {J. Low Temp. Phys.},
 title     = {Derivation of the Landau quantum hydrodynamics for interacting Bose systems},
 volume    = {1},
 pages     = {65-71},
 year      = {1969},
}

@article{landau:JPUSSR:1941,
 author    = {L. D. Landau},
 journal   = {J. Phys. (USSR)},
 title     = {The theory of superfluidity of helium II},
 volume    = {5},
 pages     = {71--100},
 year      = {1941},
}

@article{london:RMP:1945,
 author    = {F. London},
 journal   = {Rev. Mod. Phys.},
 title     = {Planck's constant and low temperature transfer},
 volume    = {17},
 pages     = {310-320},
 year      = {1945},
}

@article{fetter:JPCM:2001,
 author    = {A. L. Fetter and A. A. Svidzinsky},
 journal   = {J. Phys.: Condens. Matter},
 title     = {Vortices in a trapped dilute Bose-Einstein condensate},
 volume    = {13},
 pages     = {R135-R194},
 year      = {2001},
}

@article{moshinsky:PhysRev:1952,
 author    = {M. Moshinsky},
 journal   = {Phys. Rev.},
 title     = {Diffraction in time},
 volume    = {88},
 pages     = {625-631},
 year      = {1952},
}

@article{moshinsky:PhysRev:1951,
 author    = {M. Moshinsky},
 journal   = {Phys. Rev.},
 title     = {Boundary conditions and time-dependent states},
 volume    = {84},
 pages     = {525-532},
 year      = {1951},
}

@article{moshinsky:AJP:1976,
 author    = {M. Moshinsky},
 journal   = {Am. J. Phys.},
 title     = {Diffraction in time and the time-energy uncertainty relation},
 volume    = {44},
 pages     = {1037-1042},
 year      = {1976},
}

@article{kleber:PhysRep:1994,
 author    = {M. Kleber},
 journal   = {Phys. Rep.},
 title     = {Exact solutions for time-dependent phenomena in quantum mechanics},
 volume    = {236},
 pages     = {331-393},
 year      = {1994},
}

@article{muga:PhysRep:2009,
 author    = {A. del Campo and G. Garc{\'\i}a-Calder\'on and J. G. Muga},
 journal   = {Phys. Rep.},
 title     = {Quantum transients},
 volume    = {476},
 pages     = {1-50},
 year      = {2009},
}

@article{muga:JPA:2006,
 author    = {A. del Campo and J. G. Muga},
 journal   = {J. Phys. A},
 title     = {Matter-wave diffraction in time with a linear potential},
 volume    = {39},
 pages     = {5897-5906},
 year      = {2006},
}

@article{dalibard:PRL:1996,
 author    = {A. Szriftgiser and D. Gu\'ery-Odelin and M. Arndt and J. Dalibard},
 journal   = {Phys. Rev. Lett.},
 title     = {Atomic wave diffraction and interference using temporal slits},
 volume    = {77},
 pages     = {4-7},
 year      = {1996},
}

@article{brukner:PRA:1997,
 author    = {\v{C}. Brukner and A. Zeilinger},
 journal   = {Phys. Rev. A},
 title     = {Diffraction of matter waves in space and in time},
 volume    = {56},
 pages     = {3804-3824},
 year      = {1997},
}

@article{goussev:PRA:2013,
 author    = {A. Goussev},
 journal   = {Phys. Rev. A},
 title     = {Diffraction in time: An exactly solvable model},
 volume    = {87},
 pages     = {053621(1-4)},
 year      = {2013},
}

@article{dorlas:IJTP:2014,
 author    = {M Beau and T. C. Dorlas},
 journal   = {Int. J. Theor. Phys.},
 title     = {Three-dimensional quantum slit diffraction and diffraction in time},
 volume    = {54},
 pages     = {1882-1907},
 year      = {2015},
}

@article{horwitz:FoundPhys:2007,
 author    = {L. P. Horwitz},
 journal   = {Found. Phys.},
 title     = {Quantum interference in time},
 volume    = {37},
 pages     = {734-746},
 year      = {2007},
}

@article{talbot:PhilMag:1836,
	author = {H. F. Talbot},
	title = {LXXVI. Facts relating to optical science. No. IV},
	journal = {London Edinburgh Philos. Mag. \& J. Sci.e},
	volume = {9},
	number = {56},
	pages = {401--407},
	year = {1836},
	publisher = {Taylor \& Francis},
	doi = {10.1080/14786443608649032},
	URL = {https://doi.org/10.1080/14786443608649032},
	eprint = {https://doi.org/10.1080/14786443608649032},
}

@article{rayleigh:PhilosMag:1881,
	author = {Lord Rayleigh},
	title = {XXV. On copying diffraction-gratings, and on some phenomena connected therewith },
	journal = {London Edinburgh Philos. Mag. \& J. Sci.e},
	volume = {11},
	number = {67},
	pages = {196--205},
	year = {1881},
	publisher = {Taylor \& Francis},
	doi = {10.1080/14786448108626995},
	URL = {https://doi.org/10.1080/14786448108626995},
	eprint = {https://doi.org/10.1080/14786448108626995},
}

@article{arndt:OptExpress:2009,
 author    = {W. B. Case and M. Tomandl and S. Deachapunya and M. Arndt},
 journal   = {Opt. Express},
 title     = {Realization of optical carpets in the {Talbot} and {Talbot-Lau} configurations},
 volume    = {17},
 pages     = {20966-20974},
 year      = {2009},
}

@article{wang:PRL:2017,
 author    = {X. Wang and H. Chen and H. Liu and L. Xu and Ch. Sheng and Sh. Zhu},
 journal   = {Phys. Rev. Lett.},
 title     = {Self-focusing and the {talbot} effect in conformal transformation optics},
 volume    = {119},
 pages     = {033902(1-5)},
 year      = {2017},
}

@article{cronin:NJP:2009,
 author    = {B. J. McMorran and A. D. Cronin},
 journal   = {New J. Phys.},
 title     = {An electron {talbot} interferometer},
 volume    = {11},
 pages     = {033021(1-7)},
 year      = {2009},
}

@article{pritchard:PRA:1995,
 author    = {M. S. Chapman and Ch. R. Ekstrom and T. D. Hammond and J. Schmiedmayer and B. R. Tannian and S. Wehinger and D. E. Pritchard},
 journal   = {Phys. Rev. A},
 title     = {Near-field imaging of atom diffraction gratings: The atomic {talbot} effect},
 volume    = {51},
 pages     = {R14-R17},
 year      = {1995},
}

@article{arndt:PRL:2002,
 author    = {B. Brezger and L. Hackerm\"uller and S. Uttenthaler and J. Petschinka and M. Arndt and A. Zeilinger},
 journal   = {Phys. Rev. Lett.},
 title     = {Matter-Wave interferometer for large molecules},
 volume    = {88},
 pages     = {100404(1-4)},
 year      = {2002},
}

@BOOK{agrawal-bk:2010,
  AUTHOR     = {G. P. Agrawal},
  TITLE      = {Fiber-Optic Communication Systems},
  PUBLISHER  = {Wiley},
  YEAR       = {2010},
  address    = {Hoboken, NJ},
  edition    = {4th},
}

@article{wojcik:PRL:2000,
 author    = {D. W\'ojcik and I. Bia{\l}ynicki-Birula and D. \.{Z}yczkowski},
 journal   = {Phys. Rev. Lett.},
 title     = {Time evolution of quantum fractals},
 volume    = {85},
 pages     = {5022-5025},
 year      = {2000},
 doi       = {10.1103/PhysRevLett.85.5022},
}

@article{berry:PhysWorld:2001,
 author    = {M. Berry and I. Marzoli and W. Schleich},
 journal   = {Phys. World},
 title     = {Quantum carpets, carpets of light},
 volume    = {14},
 number = {6},
 pages     = {39-43},
 year      = {2001},
 doi = {10.1088/2058-7058/14/6/30},
 url = {https://dx.doi.org/10.1088/2058-7058/14/6/30},
}

@article{kaplan:PRA:2000,
 author    = {A. E. Kaplan and I. Marzoli and W. E. Lamb, Jr. and W. P. Schleich},
 journal   = {Phys. Rev. A},
 title     = {Multimode interference: Highly regular pattern formation in quantum wave-packet evolution},
 volume    = {61},
 pages     = {032101-032107},
 year      = {2000},
}

@article{kaplan:PhysScr:1998,
 author    = {A. E. Kaplan and P. Stifter and K. A. H. van Leeuwen and W. E. Lamb, Jr. and W. P. Schleich},
 journal   = {Phys. Scr.},
 title     = {Intermode traces -- Fundamental interference phenomenon in quantum and wave physics},
 volume    = {T76},
 pages     = {93-97},
 year      = {1998},
}

@article{marzoli:ActaPhysSlo:1998,
 author    = {I. Marzoli and F. Saif and I. Bialynicki-Birula and O. M. Friesch and A. E. Kaplan and W. P. Schleich},
 journal   = {Acta Phys. Slovaca},
 title     = {Quantum carpets made simple},
 volume    = {48},
 pages     = {323-333},
 year      = {1998},
}

@article{robinett:PhysRep:2004,
 author    = {R. W. Robinett},
 journal   = {Phys. Rep.},
 title     = {Quantum wave packet revivals},
 volume    = {392},
 pages     = {1-119},
 year      = {2004},
}

@article{robinett:AJP:2000,
 author    = {R. W. Robinett},
 journal   = {Am. J. Phys.},
 title     = {Visualizing the collapse and revival of wave packets in the infinite square well using expectation values},
 volume    = {68},
 pages     = {410},
 year      = {2000},
}

@article{sanz:FrontPhys:2019,
 author    = {A. S. Sanz},
 journal   = {Front. Phys.},
 title     = {Bohm's approach to quantum mechanics: Alternative theory or practical picture?},
 volume    = {14},
 pages     = {11301},
 year      = {2019},
 doi       = {https://doi.org/10.1007/s11467-018-0853-4},
 url       = {https://link.springer.com/article/10.1007/s11467-018-0853-4}
}

@BOOK{ashcroft-bk,
  AUTHOR     = {N. W. Ashcroft and N. D. Mermin},
  TITLE      = {Solid State Physics},
  PUBLISHER  = {Harcourt College Publishers},
  YEAR       = {1976},
  address    = {Fort Worth, USA},
}

@article{sanz:JPhysConfSer:2014,
 author    = {A. S. Sanz},
 journal   = {J. Phys.: Conf. Ser.},
 title     = {Particles, waves and trajectories: 210 years after Young's experiment},
 volume    = {504},
 pages     = {012028(1-14)},
 year      = {2014},
}

@article{sanz:PRA:2017,
 author    = {A. S. Sanz and M. Davidovi\'c and M. Bo\v{z}i\'c},
 journal   = {Phys. Rev. A},
 title     = {Bohmian approach to Gaussian-Maxwell beams},
 volume    = {},
 pages     = {1-15},
 year      = {submitted, 2017},
}

@article{keith:PRL:1991,
 author    = {D. W. Keith and C. R. Ekstrom and Q. A. Turchette and D. E. Pritchard},
 journal   = {Phys. Rev. Lett.},
 title     = {An interferometer for atoms},
 volume    = {66},
 pages     = {2693-2696},
 year      = {1991},
}

@article{sanz:PhysScr:2019,
 author    = {J. Tounli and A. Alvarado and A. S. Sanz},
 journal   = {Phys. Scr.},
 title     = {Boundary bound diffraction: A combined spectral and Bohmian mechanics},
 volume    = {94},
 pages     = {035202(1-15)},
 year      = {2019},
 doi       = {10.1088/1402-4896/aaf484},
}

@article{toennies:PRL:1999-1,
 author    = {R. E. Grisenti and W. Sch\"ollkopf and J. P. Toennies},
 journal   = {Phys. Rev. Lett.},
 title     = {Determination of atom-surface van der Waals potentials from transmission-grating diffraction intensities},
 volume    = {83},
 pages     = {1755-1758},
 year      = {1999},
}

@article{toennies:PRL:2000,
 author    = {R. E. Grisenti and W. Sch\"ollkopf and J. P. Toennies and G. C. Hegerfeldt and T. K\"ohler and M. Stoll},
 journal   = {Phys. Rev. Lett.},
 title     = {Determination of the bond length and binding energy of the Helium dimer by diffraction from a transmission grating},
 volume    = {85},
 pages     = {2284-2287},
 year      = {2000},
}

@article{toennies:PRA:2000,
 author    = {R. E. Grisenti and W. Sch\"ollkopf and J. P. Toennies and J. R. Manson},
 journal   = {Phys. Rev. Lett.},
 title     = {He-atom diffraction from nanostructure transmission gratings: The role of imperfections},
 volume    = {61},
 pages     = {033608(1-15)},
 year      = {2000},
}

@article{toennies:science:1994,
 author    = {W. Sch\"ollkopf and J. P. Toennies},
 journal   = {Science},
 title     = {Nondestructive mass selection of small van der waals clusters},
 volume    = {266},
 pages     = {1345-1348},
 year      = {1994},
}

@article{toennies:PRL:1999-2,
 author    = {R. B. Doak and R. E. Grisenti and S. Rehbein and G. Schmahl and J. P. Toennies and Ch. W\"oll},
 journal   = {Phys. Rev. Lett.},
 title     = {Towards realization of an atomic de Broglie microscope: Helium atom focusing using Fresnel zone plates},
 volume    = {83},
 pages     = {4229-4232},
 year      = {1999},
}

@article{phillips:rmp:1998,
 author    = {W. D. Phillips},
 journal   = {Rev. Mod. Phys.},
 title     = {Laser cooling and trapping of neutral atoms},
 volume    = {70},
 pages     = {721-741},
 year      = {1998},
}

@article{grimm:aamop:2000,
 author    = {R. Grimm and M. Weidem\"uller and Yu. B. Ovchinnikov},
 journal   = {Adv. At. Mol. Opt. Phys.},
 title     = {Optical dipole traps for neutral atoms},
 volume    = {42},
 pages     = {95-170},
 year      = {2000},
}

@article{einstein:AnnPhys:1905-1,
 author    = {A. Einstein},
 journal   = {Ann. Phys.},
 title     = {\"Uber einen die Erzeugung und Verwandlung des Lichtes betreffenden heuristischen Gesichtspunkt},
 volume    = {17},
 pages     = {132-148},
 year      = {1905},
}

@article{arndt:NaturePhys:2014,
 author    = {M. Arndt and K. Hornberger},
 journal   = {Nature Phys.},
 title     = {Testing the limits of quantum mechanical superpositions},
 volume    = {10},
 pages     = {271-277},
 year      = {2014},
}

@article{taylor:ProcCambPhilSoc:1909,
 author    = {G. I. Taylor},
 journal   = {Proc. Camb. Philos. Soc.},
 title     = {Interference fringes with feeble light},
 volume    = {15},
 pages     = {114-115},
 year      = {1909},
}

@article{heisenberg:ZPhys:1925,
 author    = {W. Heisenberg},
 journal   = {Z. Phys.},
 title     = {\"Uber quantentheoretische Umdeutung kinematischer und mechanischer Beziehungen},
 volume    = {33},
 pages     = {879-880},
 year      = {1925},
}

@article{richardson:PRA:2014,
 author    = {Ch. D. Richardson and P. Schlagheck and J. Martin and N. Vandewalle and T. Bastin},
 journal   = {Phys. Rev. A},
 title     = {Nonlinear Schr\"odinger wave equation with linear quantum behavior},
 volume    = {89},
 pages     = {032118},
 year      = {2014},
}

@article{chou:AOP:2016,
 author    = {C.-C. Chou},
 journal   = {Ann. Phys.},
 title     = {Trajectory description of the quantum-classical transition for wave packet interference},
 volume    = {371},
 pages     = {437-459},
 year      = {2016},
}

@BOOK{Shizgal-bk:2015,
  AUTHOR     = {B. Shizgal},
  TITLE      = {Spectral Methods in Chemistry and Physics: Applications to Kinetic Theory and Quantum Mechanics},
  PUBLISHER  = {Springer},
  series     = {Scientific Computation},
  YEAR       = {2015},
  address    = {Heidelberg},
}

@INBOOK{calvo-waveguides-bk,
  AUTHOR =       {R. F. \'Alvarez-Estrada and M. L. Calvo},
  editor =       {M. L. Calvo and V. Lakshminarayanan},
  TITLE =        {Optical Waveguides: From Theory to Applied Technologies},
  CHAPTER =      {Neutron Waveguides and Applications},
  pages =        {331-385},
  PUBLISHER =    {CRC Press},
  YEAR =         {2007},
  address =      {New York},
}

@article{hofmann:chemrev:1996,
 author    = {F. Hofmann and J. P. Toennies},
 journal   = {Chem. Rev.},
 title     = {High-resolution helium atom time-of-flight spectroscopy of low-frequency vibrations of adsorbates},
 volume    = {96},
 pages     = {1307-1326},
 year      = {1996},
 doi       = {10.1021/cr9502209},
}

@article{lahee:JCP:1987,
 author    = {A. M. Lahee and J. R. Manson and J. P. Toennies and Ch. W\"oll},
 journal   = {J. Chem. Phys.},
 title     = {Helium atom differential cross sections for scattering from single adsorbed CO molecules on a Pt(111) surface},
 volume    = {86},
 pages     = {7194-7203},
 year      = {1987},
 doi       = {10.1063/1.452321},
}

@article{lahee:PRL:1986,
 author    = {A. M. Lahee and J. R. Manson and J. P. Toennies and Ch. W\"oll},
 journal   = {Phys. Rev. Lett.},
 title     = {Observation of interference oscillations in helium scattering from single surface defects},
 volume    = {57},
 pages     = {471-474},
 year      = {1986},
 doi       = {10.1103/PhysRevLett.57.471},
}

@article{yinnon:JCP:1988,
 author    = {A. T. Yinnon and R. Kosloff and R. B. Gerber},
 journal   = {J. Chem. Phys.},
 title     = {Atom scattering from isolated adsorbates on surfaces: Rainbows, diffraction interferences, and trapping resonances},
 volume    = {88},
 pages     = {7209-7220},
 year      = {1988},
 doi       = {10.1063/1.454373},
}

@article{lemoine:JCP:1994-1,
 author    = {M.-N. Carr\'e and D. Lemoine},
 journal   = {J. Chem. Phys.},
 title     = {Fully quantum study of the 3D diffractive scattering of He from isolated CO adsorbates on Pt(111)},
 volume    = {101},
 pages     = {5305-5312},
 year      = {1994},
 doi       = {10.1063/1.467384},
}

@article{lemoine:PRL:1998,
 author    = {D. Lemoine},
 journal   = {Phys. Rev. Lett.},
 title     = {Atomic scattering from single adsorbates: What can we learn from the gas phase?},
 volume    = {81},
 pages     = {461-464},
 year      = {1998},
 doi       = {10.1103/PhysRevLett.81.461},
}

@article{kleyn:physrep:1991,
 author    = {A. W. Kleyn and T. C. M. Horn},
 journal   = {Phys. Rep.},
 title     = {Rainbow scattering from solid surfaces},
 volume    = {199},
 pages     = {191-230},
 year      = {1991},
 doi       = {10.1016/0370-1573(91)90032-H},
}

@article{drolshagen:JCP:1987,
 author    = {G. Drolshagen and R. Vollmer},
 journal   = {J. Chem. Phys.},
 title     = {Atom scattering from surfaces with isolated impurities: Calculations for hard wall and soft potentials},
 volume    = {87},
 pages     = {4948-4957},
 year      = {1987},
 doi       = {10.1063/1.452807},
}

@article{graham:JCP:1996,
 author    = {A. P. Graham and F. Hofman and J. P. Toennies and J. R. Manson},
 journal   = {J. Chem. Phys.},
 title     = {Helium atom scattering from isolated CO molecules on copper(001)},
 volume    = {105},
 pages     = {2093-2098},
 year      = {1996},
 doi       = {10.1063/1.472075},
}

@article{choi:JCP:1997-1,
 author    = {B. H. Choi and K. T. Tang and J. P. Toennies},
 journal   = {J. Chem. Phys.},
 title     = {Interpretation of helium atom scattering from isolated CO molecules on copper (001) based on an exact quantum mechanical model},
 volume    = {107},
 pages     = {1631-1633},
 year      = {1997},
 doi       = {10.1063/1.474514},
}

@article{choi:JCP:1997-2,
 author    = {B. H. Choi and K. T. Tang and J. P. Toennies},
 journal   = {J. Chem. Phys.},
 title     = {Quantum-mechanical scattering of an atom from a rigid hemisphere on a flat surface},
 volume    = {107},
 pages     = {9437-9446},
 year      = {1997},
 doi       = {10.1063/1.475240},
}

@article{choi:JCP:2000,
 author    = {B. H. Choi and A. P. Graham and K. T. Tang and J. P. Toennies},
 journal   = {J. Chem. Phys.},
 title     = {Helium atom scattering from isolated CO molecules on a Pt(111) surface: Experiment versus close-coupling calculations for a realistic He-CO potential},
 volume    = {112},
 pages     = {10538-10547},
 year      = {2000},
 doi       = {10.1063/1.481687},
}

@article{drolshagen:surfsci:1984,
 author    = {G. Drolshagen and E. J. Heller},
 journal   = {Surf. Sci.},
 title     = {A wavepacket approach to gas-surface scattering: Application to surfaces with imperfections},
 volume    = {139},
 pages     = {260-280},
 year      = {1984},
 doi       = {10.1016/0039-6028(84)90021-9},
}

@article{lemoine:JCP:1994-2,
 author    = {D. Lemoine},
 journal   = {J. Chem. Phys.},
 title     = {Quantum flux analysis of the scattering of oriented NO molecules from surfaces},
 volume    = {101},
 pages     = {4343-4356},
 year      = {1994},
 doi       = {10.1063/1.467485},
}

@article{gerber:CPL:1984,
 author    = {R. B. Gerber and A. T. Yinnon and R. Kosloff},
 journal   = {Chem. Phys. Lett.},
 title     = {Effects of isolated impurities on atom scattering from crystalline surfaces: Exact quantum-mechanical calculations},
 volume    = {105},
 pages     = {523-526},
 year      = {1984},
 doi       = {10.1016/0009-2614(84)80103-7},
}

@BOOK{joachain-bk,
  AUTHOR     = {C. J. Joachain},
  TITLE      = {Quantum Collision Theory},
  PUBLISHER  = {North-Holland},
  YEAR       = {Amsterdam},
  address    = {1975},
}

@article{glebov:PRL:1997,
 author    = {A. Glebov and J. R. Manson and Skofronick and J. P. Toennies},
 journal   = {Phys. Rev. Lett.},
 title     = {Defect-mediated diffraction resonances in surface scattering},
 volume    = {78},
 pages     = {1508-1511},
 year      = {1997},
 doi       = {10.1103/PhysRevLett.78.1508},
}

@article{farias:repprogphys:1998,
 author    = {D. Far{\'\i}as and K.-H. Rieder},
 journal   = {Rep. Prog. Phys.},
 title     = {Atomic beam diffraction from solid surfaces},
 volume    = {61},
 pages     = {1575-1664},
 year      = {1998},
 doi       = {10.1088/0034-4885/61/12/001},
}

@article{davidovic:JRLR:2017,
 author    = {M. D. Davidovi\'c and M. D. Davidovi\'c and A. S. Sanz and M. Bo\v{z}i\'c and D. Vasiljevi\'c},
 journal   = {J. Russ. Laser Res.},
 title     = {Trajectory-based interpretation of the laser light diffraction by a sharp edge},
 pages     = {438-447},
 volume    = {39},
 year      = {2018},
}

@BOOK{collett-spie,
  AUTHOR     = {E. Collett},
  TITLE      = {Field Guide to Polarization},
  PUBLISHER  = {SPIE},
  YEAR       = {2005},
  address    = {Bellingham, Washington USA},
}

@inproceedings{sbitnev:InTech:2012,
   author = {V. I. Sbitnev},
  chapter = {Bohmian trajectories and the path integral paradigm -- Complexified Lagrangian mechanics},
booktitle = {Theoretical Concepts of Quantum Mechanics},
     year = {2012},
   editor = {M. R. Pahlavani},
    pages = {313-334},
publisher = {InTech},
  address = {Rijeka},
}

@inproceedings{sbitnev:InTech:2013,
   author = {V. I. Sbitnev},
  chapter = {Generalized path integral technique: nanoparticles incident on a slit grating, matter wave interference},
booktitle = {Advances in Quantum Mechanics},
     year = {2013},
   editor = {P. Bracken},
    pages = {183-211},
publisher = {InTech},
  address = {Rijeka},
}

@article{sbitnev:FoundPhys:2016,
 author    = {V. I. Sbitnev},
 journal   = {Found. Phys.},
 title     = {Hydrodynamics of the physical vacuum: I. Scalar quantum sector},
 volume    = {46},
 pages     = {606-619},
 year      = {2016},
 doi       = {10.1007/s10701-015-9980-8},
}

@article{bohm:PhysRep:1989,
 author    = {D. Bohm and B. J. Hiley},
 journal   = {Phys. Rep.},
 title     = {Non-Locality and Locality in the Stochastic Interpretation of Quantum Mechanics},
 volume    = {172},
 pages     = {93-122},
 year      = {1989},
}

@article{struyve:JPA:2018,
 author    = {R. Dubertrand and J.-B. Shim and W. Struyve},
 journal   = {J. Phys. A},
 title     = {Bohmian trajectories for the half-line barrier},
 volume    = {51},
 pages     = {085302(1-22)},
 year      = {2018},
}

@BOOK{gilder-bk,
  AUTHOR     = {L. Gilder},
  TITLE      = {The Age of Entanglement. When Quantum Physics was Reborn},
  PUBLISHER  = {Alfred A. Knopf},
  YEAR       = {2008},
  address    = {New York},
}

@BOOK{aczel-bk,
  AUTHOR     = {A. D. Aczel},
  TITLE      = {Entanglement. The Greatest Mystery in Physics},
  PUBLISHER  = {Four Walls Eight Windows},
  YEAR       = {2001},
  address    = {New York},
}

@article{azanna:optica:2018,
 author    = {L. Romero Cort\'es and M. Seghilani and R. Maram and J. Aza{\~n}a},
 journal   = {Optica},
 title     = {Full-field broadband invisibility through reversible wave frequency-spectrum control},
 volume    = {5},
 pages     = {779-786},
 year      = {2018},
}

@article{choi:OptExp:2014,
 author    = {J. S. Choi and J. C. Howell},
 journal   = {Opt. Express},
 title     = {Paraxial ray optics cloaking},
 volume    = {22},
 pages     = {29465-29478},
 year      = {2014},
}

@article{choi:OptExp:2015,
 author    = {J. S. Choi and J. C. Howell},
 journal   = {Opt. Express},
 title     = {Paraxial full-field cloaking},
 volume    = {23},
 pages     = {15857-15862},
 year      = {2015},
}

@BOOK{milton-bk,
  AUTHOR     = {M. Katz},
  TITLE      = {Introduction to Geometrical Optics},
  PUBLISHER  = {World Scientific},
  YEAR       = {2002},
  address    = {New Jersey},
}

@BOOK{pedrotti-bk,
  AUTHOR     = {F. L. Pedrotti and L. M. Pedrotti and L. S. Pedrotti},
  TITLE      = {Introduction to Optics},
  PUBLISHER  = {Pearson},
  YEAR       = {2014},
  address    = {UK},
}

@article{smith:Science:2006,
 author    = {D. Schurig and J. J. Mock and B. J. Justice and S. A. Cummer and J. B. Pendry and A. F. Starr and D. R. Smith},
 journal   = {Science},
 title     = {Metamaterial electromagnetic cloak at microwave frequencies},
 volume    = {314},
 pages     = {977-980},
 year      = {2006},
}

@article{engheta:PRE:2005,
 author    = {A. Al\`u and N. Engheta},
 journal   = {Phys. Rev. E},
 title     = {Achieving transparency with plasmonic and metamaterial coatings},
 volume    = {72},
 pages     = {016623(1-9)},
 year      = {2005},
}

@article{engheta:PRE:2006,
 author    = {A. Al\`u and N. Engheta},
 journal   = {Phys. Rev. E},
 title     = {Erratum: Achieving transparency with plasmonic and metamaterial coatings [Phys. Rev. E, 72, 016623 (2005)]},
 volume    = {73},
 pages     = {019906(E)},
 year      = {2006},
}

@article{shalaev:NatPhot:2007,
 author    = {W. Cai and U. K. Chettiar and A. V. Kildishev and V. M. Shalaev},
 journal   = {Nat. Photon.},
 title     = {Optical cloaking with metamaterials},
 volume    = {1},
 pages     = {224-227},
 year      = {2007},
}

@BOOK{steinmeyer-bk,
  AUTHOR     = {J. Steinmeyer},
  TITLE      = {Hiding the Elephant -- How Magicians Invented the Impossible and Learned to Disappear},
  PUBLISHER  = {Carroll \& Graf Publishers},
  YEAR       = {2003},
  address    = {New York},
}

@article{zepf:physteach:2004,
 author    = {T. H. Zepf},
 journal   = {Physics Teacher},
 title     = {The Haunted Physics Lab},
 volume    = {42},
 pages     = {404-408},
 year      = {2004},
}

@article{marques:AJP:2011,
 author    = {M. C. Vel\'azquez-Ahumada and M. J. Freire and J. M. Algar{\'\i}n and R. Marques},
 journal   = {Am. J. Phys.},
 title     = {Demonstration of negative refraction of microwaves},
 volume    = {79},
 pages     = {349-352},
 year      = {2011},
}

@article{gennaro:AJP:2016,
 author    = {J. T. Wilkinson and Ch. B. Whitehouse and R. F. Oulton and S. D. Gennaro},
 journal   = {Am. J. Phys.},
 title     = {An undergraduate experiment demonstrating the physics of metamaterials with acoustic waves and soda cans},
 volume    = {84},
 pages     = {14-20},
 year      = {2016},
}

@article{fleming:AJP:2017,
 author    = {S. Fleming},
 journal   = {Am. J. Phys.},
 title     = {Metamaterial hyperlens demonstration of propagation without diffraction},
 volume    = {85},
 pages     = {173-177},
 year      = {2017},
}

@article{thompson:AJP:2008,
 author    = {M. Sipos and B. G. Thompson},
 journal   = {Am. J. Phys.},
 title     = {Electrodynamics on a grid: The finite-difference time-domain method applied to optics and cloaking},
 volume    = {76},
 pages     = {464-469},
 year      = {2008},
}

@article{longhi:AJP:2017,
 author    = {S. A. R. Horsley and S. Longhi},
 journal   = {Am. J. Phys.},
 title     = {One-way invisibility in isotropic dielectric optical media},
 volume    = {85},
 pages     = {439-446},
 year      = {2017},
}

@article{choi:ApplOpt:2014,
 author    = {J. C. Howell and J. B. Howell and J. S. Choi},
 journal   = {Appl. Opt.},
 title     = {Amplitude-only, passive, broadband, optical spatial cloaking of very large objects},
 volume    = {53},
 pages     = {1958-1963},
 year      = {2014},
}

@article{sanchezsoto:EJP:2008,
 author    = {J. J. Monz\'on and A. G. Barriuso and L. L. S\'anchez-Soto},
 journal   = {Eur. J. Phys.},
 title     = {Geometric picture of optical complementary media},
 volume    = {29},
 pages     = {431-437},
 year      = {2008},
}

@article{sanchezsoto:PhysRep:2012,
 author    = {L. L. S\'anchez-Soto and J. J. Monz\'on and A. G. Barriuso and J. F. Cari{\~n}ena},
 journal   = {Phys. Rep.},
 title     = {The transfer matrix: A geometrical perspective},
 volume    = {513},
 pages     = {191-227},
 year      = {2013},
}

@BOOK{rowling:HarryPotter:2007,
  AUTHOR     = {J. K. Rowling},
  TITLE      = {Harry Potter and the Deathly Hallows},
  PUBLISHER  = {Bloomsbury Publishing},
  YEAR       = {2007},
  address    = {New York},
  edition    = {1st},
}

@article{durt:EPL:2016,
 author    = {Th. Durt},
 journal   = {EPL},
 title     = {Generalized guidance equation for peaked quantum solitons and effective gravity},
 volume    = {114},
 pages     = {10004(1-6)},
 year      = {2016},
}

@article{pope:FrontPhys:2017,
 author    = {Th. Pope and W. Hofer},
 journal   = {Front. Phys.},
 title     = {Spin in the extended electron model},
 volume    = {12},
 pages     = {128503(1-5)},
 year      = {2017},
}

@article{long:SciChina:2018,
 author    = {G.-L. Long and W. Qin and Zh. Yang and J.-L. Li},
 journal   = {Sci. China-Phys. Mech. Astron.},
 title     = {Realistic interpretation of quantum mechanics and encounter-delayed-choice experiment},
 volume    = {61},
 pages     = {030311(1-8)},
 year      = {2018},
}

@article{zhou:SciBull:2017,
 author    = {Zh.-Y. Zhou and Zh.-H. Zhu and Sh.-L. Liu and Y.-H. Li and Sh. Shi and D.-Sh. Ding and L.-X. Chen and W. Gao and G.-C. Guo and B.-S. Shi},
 journal   = {Sci. Bull.},
 title     = {Quantum twisted double-slits experiments: confirming wavefunctions' physical reality},
 volume    = {62},
 pages     = {1185-1192},
 year      = {2017},
}

@article{yuan:LSA:2016,
 author    = {G. H. Yuan and S. Vezzoli and Ch. Altuzarra and E. T. F. Rogers and Ch. Couteau and C. Soci and N. I. Zheludev},
 journal   = {Light-Sci. Appl.},
 title     = {Quantum super-oscillation of a single photon},
 volume    = {5},
 pages     = {e16127(1-6)},
 year      = {2016},
}

@article{li:EPL:2017,
 author    = {Zh.-Y. Li},
 journal   = {EPL},
 title     = {Weak-measurement Mach-Zehnder interferometer for testing wave-particle duality},
 volume    = {117},
 pages     = {50005(1-6)},
 year      = {2017},
}

@BOOK{rauch-bk,
  AUTHOR     = {H. Rauch and S. A. Werner},
  TITLE      = {Neutron Interferometry. Lessons in Experimental Quantum Mechanics},
  PUBLISHER  = {Oxford University Press},
  YEAR       = {2000},
  address    = {New York},
}

@BOOK{rauch-bk-2,
  AUTHOR     = {H. Rauch and S. A. Werner},
  TITLE      = {Neutron Interferometry. Lessons in Experimental Quantum Mechanics, Wave-Particle Duality, and Entanglement},
  PUBLISHER  = {Oxford University Press},
  YEAR       = {2015},
  address    = {New York},
}

@BOOK{willis-bk,
  AUTHOR     = {B. T. M. Willis and C. J. Carlile},
  TITLE      = {Experimental Neutron Scattering},
  PUBLISHER  = {Oxford University Press},
  YEAR       = {2009},
  address    = {Oxford University Press},
}

@article{klein:RPP:1983,
 author    = {A. G. Klein and S. A. Werner},
 journal   = {Rev. Prog. Phys.},
 title     = {Neutron optics},
 volume    = {46},
 pages     = {259-335},
 year      = {1983},
}

@article{hasegawa:physicaB:2011,
 author    = {K. Durstberger-Rennhofer and Y. Hasegawa},
 journal   = {Physica B},
 title     = {Energy entanglement in neutron interferometry},
 volume    = {406},
 pages     = {2373-2376},
 year      = {2011},
}

@article{hasegawa:physicaB:2018,
 author    = {T. Denkmayr and J. Dressel and H. Geppert-Kleinrath and Y. Hasegawa and S. Sponar},
 journal   = {Physica B},
 title     = {Weak values from strong interactions in neutron interferometry},
 volume    = {551},
 pages     = {339-346},
 year      = {2018},
}

@article{dewdney:PhysLett:1985,
 author    = {C. Dewdney},
 journal   = {Phys. Lett.},
 title     = {Particle trajectories and interference in a time-dependent model of neutron single crystal interferometry},
 volume    = {109A},
 pages     = {377-384},
 year      = {1985},
}

@BOOK{sanz:neutron:2020,
  AUTHOR     = {A. S. Sanz},
  editor     = {M. L. Calvo and R. F. \'Alvarez-Estrada},
  title      = {Advances in Neutron Optics},
  CHAPTER    = {Neutron matter-wave diffraction: a computational perspective},
  pages      = {79-122},
  publisher  = {CRC Press},
  year       = {2020},
  address    = {Boca Rat\'on, FL},
}

@BOOK{bohm-bk:QTh,
  AUTHOR     = {D. Bohm},
  TITLE      = {Quantum Theory},
  PUBLISHER  = {Dover (first printed by Prentice Hall in 1951)},
  YEAR       = {1989},
  address    = {New York},
}

@article{bennet:PRL:1993,
 author    = {Ch. H. Bennett and G. Brassard and C. Cr\'epeau and R. Jozsa and A. Peres and W. K. Wootters},
 journal   = {Phys. Rev. Lett.},
 title     = {Teleporting an unknown quantum state via dual classical and Einstein-Podolsky-Rosen channels},
 volume    = {70},
 pages     ={1895-1899},
 year      = {1993},
}

@article{bouwmeester:nature:1997,
 author    = {D. Bouwmeester and J.-W. Pan and K. Mattle and M. Eibl and H. Weinfurter and A. Zeilinger},
 journal   = {Nature},
 title     = {Experimental quantum teleportation},
 volume    = {390},
 pages   = {575-579},
 year      = {1997},
}

@article{zeilinger:nature:2003,
 author    = {I. Marcikic and H. de Riedmatten and W. Tittel and H. Zbinden and N. Gisin},
 journal   = {Nature},
 title     = {Long-distance teleportation of qubits at telecommunication wavelengths},
 volume    = {421},
 pages   = {509-513},
 year      = {2003},
}

@article{zeilinger:nature:2012,
 author    = {X.-S. Ma and T. Herbst and T. Scheidl and D. Wang and S. Kropatschek and W. Naylor and B. Wittmann and A. Mech and J. Kofler and E. Anisimova and V. Makarov and Th. Jennewein and R. Ursin and A. Zeilinger},
 journal   = {Nature},
 title     = {Quantum teleportation over 143 kilometres using active feed-forward},
 volume    = {489},
 pages   = {269-273},
 year      = {2012},
}

@article{JWPan:science:2017,
 author    = {J. Yin and Y. Cao and Y.-H. Li and Sh.-K. Liao and L. Zhang and J.-G. Ren and W.-Q. Cai and W.-Y. Liu and B. Li and H. Dai and G.-B. Li and Q.-M. Lu and Y.-H. Gong and Y. Xu and Sh.-L. Li and F.-Zh. Li and Y.-Y. Yin and Z.-Q. Jiang and M. Li and J.-J. Jia and G. Ren and D. He and Y.-L. Zhou and X.-X. Zhang and N. Wang and X. Chang and Zh.-C. Zhu and N.-L. Liu and Y.-A. Chen and Ch.-Y. Lu and R. Shu and Ch.-Zh. Peng and J.-Y. Wang and J.-W. Pan},
 journal   = {Science},
 title     = {Satellite-based entanglement distribution over 1200 kilometers},
 volume    = {356},
 pages  = {1140-1144},
 year      = {2017},
}

@article{JWPan:PRL:2017,
 author    = {J. Yin and Y. Cao and Y.-H. Li and J.-G. Ren and S.-K. Liao and L. Zhang and W.-Q. Cai and W.-Y. Liu and B. Li and H. Dai and M. Li and Y.-M. Huang and L. Deng and L. Li and Q. Zhang and N.-L. Liu and Y.-A. Chen and Ch.-Y. Lu and R. Shu and Ch.-Zh. Peng and J.-Y. Wang and J.-W. Pan},
 journal   = {Phys. Rev. Lett.},
 title     = {Satellite-to-ground entanglement-based quantum key distribution},
 volume    = {119},
 pages   ={200501(1-5)},
 year      = {2017},
}

@article{li:SciBull:2016,
 author    = {T.-C. Li and Z.-Q. Yin},
 journal   = {Sci. Bull.},
 title     = {Quantum superposition, entanglement, and state teleportation of a microorganism on an electromechanical oscillator},
 volume    = {61},
 pages   = {163-171},
 year      = {2016},
}

@article{landsman:nature:2019,
 author    = {K. A. Landsman and C. Figgatt and T. Schuster and N. M. Linke and B. Yoshida and N. Y. Yao and C. Monroe},
 journal   = {Nature},
 title     = {Verified quantum information scrambling},
 volume    = {567},
 pages   = {61-64},
 year      = {2019},
}

@article{zelinger-JWPan:PRL:2019,
 author    = {Y.-H. Luo and H.-S. Zhong and M. Erhard and X.-L. Wang and L.-Ch. Peng and M. Krenn and X. Jiang and L. Li and N.-L. Liu and Ch.-Y. Lu and A. Zeilinger and J.-W. Pan},
 journal   = {Phys. Rev. Lett.},
 title     = {Quantum teleportation in high dimensions},
 volume    = {123},
 pages   = {070505(1-4)},
 year      = {2019},
}

@article{kauffman:NJP:2002,
 author    = {L. H. Kauffman and S. J. Lomonaco},
 journal   = {New J. Phys.},
 title     = {Quantum entanglement and topological entanglement},
 volume    = {4},
 pages    = {73(1-18)},
 year      = {2002},
}

@inproceedings{kauffman:QICII:2004,
  AUTHOR     = {L. H. Kauffman and S. J. Lomonaco},
  CHAPTER    = {Quantum knots},
  editor     = {E. Donkor and A. R. Pirich and H. E. Brandt},
  booktitle  = {Quantum Information and Computation II},
  volume   = {5436},
  pages      = {268-284},
  PUBLISHER  = {SPIE},
  YEAR       = {2004},
  address    = {Bellingham, WA},
  series     = {Proc. SPIE},
}

@article{kauffman:OptSpectr:2005,
 author    = {L. H. Kauffman},
 journal   = {Opt. Spectrosc.},
 title     = {Teleportation topology},
 volume    = {99},
 pages   = {227-232},
 year      = {2005},
}

@inproceedings{kauffman:QICII:2014,
  AUTHOR     = {L. H. Kauffman and S. J. Lomonaco},
  CHAPTER    = {Quantum diagrams and quantum networks},
  editor     = {E. Donkor and A. R. Pirich and H. E. Brandt and M. R. Frey and S. J. Lomonaco and J. M. Myers},
  booktitle  = {Quantum Information and Computation II},
  volume   = {9123},
  pages      = {91230P(1-14)},
  PUBLISHER  = {SPIE},
  YEAR       = {2004},
  address    = {Bellingham, WA},
  series     = {Proc. SPIE},
}

@article{kauffman:QIP:2018,
 author    = {L. H. Kauffman and S. J. Lomonaco},
 journal   = {Quantum Inf. Process.},
 title     = {Braiding, Majorana fermions, Fibonacci particles and topological quantum computing},
 volume    = {17},
 pages   = {201(1-81)},
 year      = {2018},
}

@article{kauffman:NJP:2004,
 author    = {L. H. Kauffman and S. J. Lomonaco},
 journal   = {New J. Phys.},
 title     = {Braiding operators are universal quantum gates},
 volume    = {6},
 pages    = {134(1-40)},
 year      = {2004},
}

@article{karlsson:PRA:1998,
 author    = {A. Karlsson and M. Bourennane},
 journal   = {Phys. Rev. A},
 title     = {Quantum teleportation using three-particle entanglement},
 volume    = {58},
 pages     ={4394-4400},
 year      = {1998},
}

@article{mironov:universe:2019,
 author    = {S. Mironov},
 journal   = {Universe},
 title     = {Topological entanglement and knots},
 volume    = {5},
 pages   = {60(1-10)},
 year      = {2019},
}

@article{mironov:JHEP:2019,
 author    = {D. Melnikov and A. Mironov and S. Mironov and A. Morozov and An. Morozov},
 journal   = {J. High Ener. Phys.},
 title     = {From topological to quantum entanglement},
 volume    = {2019},
 pages   = {116(1-12)},
 year      = {2019},
}

@article{quinta:PRA:2018,
 author    = {G. M. Quinta and R. Andr\'e},
 journal   = {Phys. Rev. A},
 title     = {Classifying quantum entanglement through topological links},
 volume    = {97},
 pages   = {042307(1-12)},
 year      = {2018},
}

@article{peres:PRL:1996,
 author    = {A. Peres},
 journal   = {Phys. Rev. Lett.},
 title     = {Separability criterion for density matrices},
 volume    = {77},
 pages  = {1413-1415},
 year      = {1996},
}

@article{horodecki:PLA:1996,
 author    = {M. Horodecki and P. Horodecki and R. Horodecki},
 journal   = {Phys. Lett. A},
 title     = {Separability of mixed states: necessary and sufficient conditions},
 volume    = {223},
 pages  = {1-8},
 year      = {1996},
}

@article{horodecki:PLA:2001,
 author    = {M. Horodecki and P. Horodecki and R. Horodecki},
 journal   = {Phys. Lett. A},
 title     = {Separability of n-particle mixed states: necessary and sufficient conditions in terms of linear maps},
 volume    = {283},
 pages  = {1-7},
 year      = {2001},
}

@article{horodecki:OSID:2006,
 author    = {M. Horodecki and P. Horodecki and R. Horodecki},
 journal   = {Open Sys. Inf. Dyn.},
 title     = {Separability of mixed quantum states: Linear contractions and permutation criteria},
 volume    = {13},
 pages  = {103-111},
 year      = {2006},
}

@article{horodecki:RMP:2009,
 author    = {R. Horodecki and P. Horodecki and M. Horodecki and K. Horodecki},
 journal   = {Rev. Mod. Phys.},
 title     = {Quantum entanglement},
 volume    = {81},
 pages   = {865-942},
 year      = {2009},
}

@article{cirac:PRL:1999,
 author    = {W. D\"ur and J. I. Cirac and R. Tarrach},
 journal   = {Phys. Rev. Lett.},
 title     = {Separability and distillability of multiparticle quantum systems},
 volume    = {83},
 pages   ={3562-3565},
 year      = {1999},
}

@article{cirac:PRA:2000,
 author    = {W. D\"ur and J. I. Cirac},
 journal   = {Phys. Rev. A},
 title     = {Classification of multiqubit mixed states: Separability and distillability properties},
 volume    = {61},
 pages   = {042314(1-11)},
 year      = {2000},
}

@article{gisin:entropy:2019,
 author    = {N. Gisin},
 journal   = {Entropy},
 title     = {Entanglement 25 years after quantum teleportation: testing joint measurements in quantum networks},
 volume    = {21},
 pages     = {325(1-12)},
 year      = {2019},
}

@article{qureshi:AJP:2016,
 author    = {T. Qureshi},
 journal   = {Am. J. Phys.},
 title     = {Quantitative wave-particle duality},
 volume    = {},
 pages     = {},
 year      = {2016},
}

@article{omnes:RMP:1992,
  title = {Consistent interpretations of quantum mechanics},
  author = {Omn\`es, Roland},
  journal = {Rev. Mod. Phys.},
  volume = {64},
  issue = {2},
  pages = {339--382},
  numpages = {0},
  year = {1992},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.64.339},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.64.339}
}


@article{tonomura:PRL:1986,
  title = {Evidence for Aharonov-Bohm effect with magnetic field completely shielded from electron wave},
  author = {Tonomura, Akira and Osakabe, Nobuyuki and Matsuda, Tsuyoshi and Kawasaki, Takeshi and Endo, Junji and Yano, Shinichiro and Yamada, Hiroji},
  journal = {Phys. Rev. Lett.},
  volume = {56},
  issue = {8},
  pages = {792--795},
  numpages = {0},
  year = {1986},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.56.792},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.56.792}
}

@article{heisengerg:ZPhys:1927,
 author    = {W. Heisenberg},
 journal   = {Z. Phys.},
 title     = {\"Uber den anschaulichen Inhalt der quantentheoretischen Kinematik und Mechanik},
 volume    = {43},
 pages     = {172},
 year      = {1927},
}

@article{breitenberger:FoundPhys:1985,
 author    = {E. Breitenberger},
 journal   = {Found. Phys.},
 title     = {Uncertainty measures and uncertainty relations for angle observables},
 volume    = {15},
 pages     = {353-364},
 year      = {1985},
}

@article{stelzer:OptCommun:2000,
 author    = {E. H. Stelzer and S. Grill},
 journal   = {Opt. Commun.},
 title     = {The uncertainty principle applied to estimate focal spot dimensions},
 volume    = {173},
 pages     = {51-56},
 year      = {2000},
}

@article{alonso:JOSAA:2000,
 author    = {M. Alonso and G. Forbes},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Uncertainty products for nonparaxial wave fields},
 volume    = {17},
 pages     = {2391-2402},
 year      = {2000},
}

@article{santarsiero:JOSAA:2006-1,
 author    = {M. Alonso and R. Borghi and M. Santarsiero},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Nonparaxial fields with maximum joint spatial-directional localization. I. Scalar case},
 volume    = {23},
 pages     = {691-700},
 year      = {2006},
}

@article{santarsiero:JOSAA:2006-2,
 author    = {M. Alonso and R. Borghi and M. Santarsiero},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Nonparaxial fields with maximum joint spatial-directional localization. II. Vectorial case},
 volume    = {23},
 pages     = {701-702},
 year      = {2006},
}

@article{chisolm:AJP:2001,
 author    = {E. D. Chisolm},
 journal   = {Am. J. Phys.},
 title     = {Generalizing the Heisenberg uncertainty relation},
 volume    = {69},
 pages     = {368-371},
 year      = {2001},
}

@article{padgett:NJP:2004,
 author    = {S. Franke-Arnold and S. M. Barnett and E. Yao and J. Leach and J. Courtial and M. Padgett},
 journal   = {New J. Phys.},
 title     = {Uncertainty principle for angular position and angular momentum},
 volume    = {6},
 pages     = {103},
 year      = {2004},
}

@article{padgett:JMO:2008,
 author    = {M. Padgett},
 journal   = {J. Mod. Opt.},
 title     = {On the focussing of light, as limited by the uncertainty principle},
 volume    = {55},
 pages     = {3083-3089},
 year      = {2008},
}

@article{ricaud:AdvComputMath:2014,
 author    = {B. Ricaud and B. Torr\'esani},
 journal   = {Adv. Comput. Math.},
 title     = {A survey of uncertainty principles and some signal processing applications},
 volume    = {40},
 pages     = {629-650},
 year      = {2014},
}

@PROCEEDINGS{siegman:ProcSPIE:1990,
   author = {A. E. Siegman},
    title = {New developments in laser resonators},
booktitle = {Optical Resonators},
     year = {1990},
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = {1224},
   editor = {E. Donkor and A. R. Pirich and H. E. Brandt},
    pages = {2-14},
publisher = {SPIE},
  address = {Bellingham, WA},
}

@article{belanger:OptLett:1991,
 author    = {P. A. Belanger},
 journal   = {Opt. Lett.},
 title     = {Beam propagation and the ABCD ray matrices},
 volume    = {16},
 pages     = {196-198},
 year      = {1991},
}

@article{serna:JOSAA:1991,
	author = {J. Serna and R. Mart\'{i}nez-Herrero and P. M. Mej\'{i}as},
	journal = {J. Opt. Soc. Am. A},
	number = {7},
	pages = {1094--1098},
	publisher = {Optica Publishing Group},
	title = {Parametric characterization of general partially coherent beams propagating through ABCD optical systems},
	volume = {8},
	month = {Jul},
	year = {1991},
	url = {https://opg.optica.org/josaa/abstract.cfm?URI=josaa-8-7-1094},
	doi = {10.1364/JOSAA.8.001094},
}

@article{martinezherrero:OptLett:1993,
 author    = {R. Mart{\'\i}nez-Herrero and P. M. Mej{\'\i}as},
 journal   = {Opt. Lett},
 title     = {Second-order spatial characterization of hard-edge diffracted beams},
 volume    = {18},
 pages     = {1669-1671},
 year      = {1993},
}

@article{martinezherrero:OptLett:1995,
 author    = {R. Mart{\'\i}nez-Herrero and P. M. Mej{\'\i}as and M. Arias},
 journal   = {Opt. Lett.},
 title     = {Parametric characterization of coherent, lowest-order Gaussian beams propagating through hard-edged apertures},
 volume    = {20},
 pages     = {124-126},
 year      = {1995},
}

@article{martinezherrero:JOSAA:2003,
 author    = {R. Mart{\'\i}nez-Herrero and P. M. Mej{\'\i}as and S. Bosch and A. Carnicer},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Spatial width and power-content ratio of hard-edge diffracted beams},
 volume    = {20},
 pages     = {388-391},
 year      = {2003},
}

@article{lindfors:NatPhoton:2007,
 author    = {K. Lindfords and A. Priimagi and T. Set\"al\"a and A. Shevchenko and A. T. Friberg and M. Kaivola},
 journal   = {Nat. Photon.},
 title     = {Local polarization of tightly focused unpolarized light},
 volume    = {1},
 pages     = {228-231},
 year      = {2007},
}

@article{yzuel:OptLett:2007,
 author    = {J. Davis and C. Tuvey and O. L\'opez-Coronado and J. Campos and M. Yzuel and C. Iemmi},
 journal   = {Opt. Lett.},
 title     = {Tailoring the depth of focus for optical imaging systems using a Fourier transform approach},
 volume    = {32},
 pages     = {844-846},
 year      = {2007},
}

@article{zhan:AdvOptPhoton:2009,
 author    = {Q. Zhan},
 journal   = {Adv. Opt. Photon.},
 title     = {Cylindrical vector beams: from mathematical concepts to applications},
 volume    = {1},
 pages     = {1-57},
 year      = {2009},
}

@article{reid:NatPhoton:2008,
 author    = {K. A. Serrels and E. Ramsay and R. J. Warburton and D. T. Reid},
 journal   = {Nat. Photon.},
 title     = {Nanoscale optical microscopy in the vectorial focusing regime},
 volume    = {2},
 pages     = {311-314},
 year      = {2008},
}

@article{sheppard:NatPhoton:2008,
 author    = {H. Wang and L. Shi and B. Lukyanchuk and C. Sheppard and C. T. Chong},
 journal   = {Nat. Photon.},
 title     = {Creation of a needle of longitudinally polarized light in vacuum using binary optics},
 volume    = {2},
 pages     = {501-505},
 year      = {2008},
}

@article{dholakia:OptExp:2009,
 author    = {T. Cizmar and K. Dholakia},
 journal   = {Opt. Express},
 title     = {Tunable Bessel light modes: engineering the axial propagation},
 volume    = {17},
 pages     = {15558-15570},
 year      = {2009},
}

@article{martinezherrero:OptLett:2013,
 author    = {R. Mart{\'\i}nez-Herrero and I. Juvells and A. Carnicer},
 journal   = {Opt. Lett.},
 title     = {On the physical realizability of highly focused electromagnetic field distributions},
 volume    = {38},
 pages     = {2065-2067},
 year      = {2013},
 url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-38-12-2065},
 doi = {10.1364/OL.38.002065}
}

@article{martinezherrero:OptExp:2016,
 author    = {A. Carnicer and I. Juvells and B. Javidi and R. Mart{\'\i}nez-Herrero},
 journal   = {Opt. Express},
 title     = {Optical encryption in the longitudinal domain of focused fields},
 volume    = {24},
 pages     = {6793-6801},
 year      = {2016},
}

@article{martinezherrero:SciRep:2018,
 author    = {R. Mart{\'\i}nez-Herrero and D. Maluenda and I. Juvells and A. Carnicer},
 journal   = {Sci. Rep.},
 title     = {Synthesis of light needles with tunable length and nearly constant irradiance},
 volume    = {8},
 pages     = {2657},
 year      = {2018},
 doi       = {https://doi.org/10.1038/s41598-018-21007-7}
}

@article{martinezherrero:OSACont:2019,
 author    = {D. Maluenda and I. Juvells and R. Mart{\'\i}nez-Herrero and A. Carnicer},
 journal   = {OSA Continuum},
 title     = {Modeling axial irradiance distortion in holographic optical needles produced with high numerical aperture lenses},
 volume    = {2},
 pages     = {1539-1547},
 year      = {2019},
}

@article{sheppard:JOSAA:1988,
 author    = {C. Sheppard and Z. Hegedus},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Axial behavior of pupil-plane filters},
 volume    = {5},
 pages     = {643-647},
 year      = {1988},
}

@article{sheppard:JMO:1994,
 author    = {C. J. R. Sheppard and K. G. Larkin},
 journal   = {J. Mod. Opt.},
 title     = {Optimal concentration of electromagnetic radiation},
 volume    = {41},
 pages     = {1495-1505},
 year      = {1994},
}

@article{martinezcorral:OptLett:2001,
 author    = {M. Mart{\'\i}nez-Corral and L. Mu{\~n}oz-Escriv\'a and M. Kowalczyk and T. Cichocki},
 journal   = {Opt. Lett.},
 title     = {One-dimensional iterative algorithm for three-dimensional point-spread function engineering},
 volume    = {26},
 pages     = {1861-1863},
 year      = {2001},
}

@article{martinezcorral:OptExp:2002,
 author    = {M. Mart{\'\i}nez-Corral and M. Caballero and E. Stelzer and J. Swoger},
 journal   = {Opt. Express},
 title     = {Tailoring the axial shape of the point spread function using the Toraldo concept},
 volume    = {10},
 pages     = {98-103},
 year      = {2002},
}

@article{sheppard:OptLett:2007,
 author    = {C. Sheppard and S. Ledesma and J. Campos and J. Escalera},
 journal   = {Opt. Lett.},
 title     = {Improved expressions for performance parameters for complex filters},
 volume    = {32},
 pages     = {1713-1715},
 year      = {2007},
}

@article{sheppard:OptLett:2008-1,
 author    = {C. Sheppard},
 journal   = {Opt. Lett.},
 title     = {Filter performance parameters for high-aperture focusing},
 volume    = {32},
 pages     = {1653-1655},
 year      = {2008},
}

@article{sheppard:OptLett:2008-2,
 author    = {C. Sheppard and M. Mart{\'\i}nez-Corral},
 journal   = {Opt. Lett.},
 title     = {Filter performance parameters for vectorial high-aperture wave fields},
 volume    = {33},
 pages     = {476-478},
 year      = {2008},
}

@article{sheppard:OptLett:2011,
 author    = {C. Sheppard},
 journal   = {Opt. Lett.},
 title     = {Binary phase filters with a maximally-flat response},
 volume    = {36},
 pages     = {1386-1388},
 year      = {2011},
}

@article{sheppard:OptExp:2013,
 author    = {C. Sheppard},
 journal   = {Opt. Express},
 title     = {Pupil filters for generation of light sheets},
 volume    = {21},
 pages     = {6339-6345},
 year      = {2013},
}

@article{richards:PRSLAM:1959,
 author    = {B. Richards and E. Wolf},
 journal   = {Proc. Roy. Soc. Lond. A Math.},
 title     = {Electromagnetic diffraction in optical systems. II. structure of the image field in an aplanatic system},
 volume    = {253},
 pages     = {358-379},
 year      = {1959},
 doi = {10.1098/rspa.1959.0200},
 url = {https://doi.org/10.1098/rspa.1959.0200},
}

@article{martinezherrero:OptExp:2014,
 author    = {R. Mart{\'\i}nez-Herrero and D. Maluenda and I. Juvells and A. Carnicer},
 journal   = {Opt. Express},
 title     = {Experimental implementation  of  tightly  focused  beams  with  unpolarized  transversal  component  at any plane},
 volume    = {22},
 pages     = {32419-32428},
 year      = {2014},
}

@article{zhang:PRL:2019,
 author    = {H. Hu and Q. Gan and Q. Zhan},
 journal   = {Phys. Rev. Lett.},
 title     = {Generation of a nondiffracting superchiral optical needle for circular dichroism imaging of sparse subdiffraction objects},
 volume    = {122},
 pages     = {223901},
 year      = {2019},
}

@article{wang:OptCommun:2016,
 author    = {B. Yan and L. Yue and Z. Wang},
 journal   = {Opt. Commun.},
 title     = {Engineering near-field focusing of a microsphere lens with pupil masks},
 volume    = {370},
 pages     = {140-144},
 year      = {2016},
}

@article{bandres:JOSAA:2005,
 author    = {J. C. Guti\'errez-Vega and M. A. Bandres},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Helmholtz-Gauss waves},
 volume    = {22},
 pages     = {289-298},
 year      = {2005},
}

@article{bandres:OptLett:2005,
 author    = {M. A. Bandres and J. C. Guti\'errez-Vega},
 journal   = {Opt. Lett.},
 title     = {Vector Helmholtz-Gauss and vector Laplace-Gauss beams},
 volume    = {30},
 pages     = {2155-2157},
 year      = {2005},
}

@article{bandres:OptExp:2006,
 author    = {R. I. Hern\'andez-Aranda and J. C. Guti\'errez-Vega and M. Guizar-Sicairos and M. A. Bandres},
 journal   = {Opt. Express},
 title     = {Propagation of generalized vector Helmholtz-Gauss beams through paraxial optical systems},
 volume    = {14},
 pages     = {8974-8988},
 year      = {2006},
}

@article{busch:PhysRep:2007,
 author    = {P. Busch and T. Heinonen and P. Lahti},
 journal   = {Phys. Rep.},
 title     = {Heisenberg's uncertainty principle},
 volume    = {452},
 pages     = {155-176},
 year      = {2007},
}

@article{maccone:PRL:2014,
 author    = {L. Maccone and A. K. Pati},
 journal   = {Phys. Rev. Lett.},
 title     = {Stronger uncertainty relations for all incompatible observables},
 volume    = {113},
 pages     = {260401(1-},
 year      = {2014},
}

@article{kempf:PRD:1995,
 author    = {A. Kempf and G. Mangano and R. B. Mann},
 journal   = {Phys. Rev. D},
 title     = {Hilbert space representation of the minimal length uncertainty principle},
 volume    = {52},
 pages     = {1108-1118},
 year      = {1995},
}

@article{scardigli:PhysLettB:1999,
 author    = {F. Scardigli},
 journal   = {Phys. Lett. B},
 title     = {Generalized uncertainty principle in quantum gravity from micro-black hole gedanken experiment},
 volume    = {452},
 pages     = {39-44},
 year      = {199},
}

@article{veneziano:EPL:1986,
 author    = {G. Veneziano},
 journal   = {Europhys. Lett.},
 title     = {A string nature needs just two constants},
 volume    = {2},
 pages     = {199-204},
 year      = {1986},
}

@article{buoninfante:EurPhysJC:2019,
 author    = {L. Buoninfante and G. G. Luciano and L. Petruzziello},
 journal   = {Eur. Phys. J. C},
 title     = {Generalized uncertainty principle and corpuscular gravity},
 volume    = {79},
 pages     = {663(1-8)},
 year      = {2019},
}

@article{steinberg:PRL:2012,
 author    = {L. A. Rozema and A. Darabi and D. H. Mahler and A. Hayat and Y. Soudagar and A. M. Steinberg},
 journal   = {Phys. Rev. Lett.},
 title     = {Violation of Heisenberg's measurement-disturbance relationship by weak measurements},
 volume    = {109},
 pages     = {100404(1-5)},
 year      = {2012},
}

@article{busch:PRL:2013,
 author    = {P. Busch and P. Lahti and R. F. Werner},
 journal   = {Phys. Rev. Lett.},
 title     = {Proof of Heisenberg's error-disturbance relation},
 volume    = {111},
 pages     = {160405(1-5)},
 year      = {2013},
}

@article{harris:JOSA:1969,
 author    = {F. S. Harris, Jr. and M. S. Tavenner and R. L. Mitchell},
 journal   = {J. Opt. Soc. Am.},
 title     = {Single-slit Fresnel diffraction patterns: comparison of experimental and theoretical results},
 volume    = {59},
 pages     = {293-296},
 year      = {1969},
}

@article{panuski:PhysTeacher:2016,
 author    = {Ch. L. Panuski and C. E. Mungan},
 journal   = {Phys. Teacher},
 title     = {Single-slit diffraction: transitioning from geometric optics to the Fraunhofer regime},
 volume    = {54},
 pages     = {356-359},
 year      = {2016},
}

@article{becs1,
  title = {Theory of Bose-Einstein condensation in trapped gases},
  author = {F. Dalfovo and S. Giorgini and L. P. Pitaevskii and S. Stringari},
  journal = {Rev. Mod. Phys.},
  volume = {71},
  issue = {3},
  pages = {463--512},
  numpages = {0},
  year = {1999},
}

@book{pitaevskii2016bose,
  title={Bose-Einstein condensation and superfluidity},
  author={L. P. Pitaevskii and S. Stringari},
  volume={164},
  year={2016},
  publisher={Oxford University Press},
}

@book{pethick2008bose,
  title={Bose--Einstein condensation in dilute gases},
  author={Ch. J. Pethick and H. Smith},
  year={2008},
  publisher={Cambridge university press},
}

@article{mewes,
  title = {Output Coupler for Bose-Einstein Condensed Atoms},
  author = {Mewes, M.-O. and Andrews, M. R. and Kurn, D. M. and Durfee, D. S. and Townsend, C. G. and Ketterle, W.},
  journal = {Phys. Rev. Lett.},
  volume = {78},
  issue = {4},
  pages = {582--585},
  numpages = {0},
  year = {1997},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.78.582},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.78.582}
}

@article {Andrews637,
    author = {Andrews, M. R. and Townsend, C. G. and Miesner, H.-J. and Durfee, D. S. and Kurn, D. M. and Ketterle, W.},
    title = {Observation of Interference Between Two Bose Condensates},
    volume = {275},
    number = {5300},
    pages = {637--641},
    year = {1997},
    journal = {Science},
    doi     = {https://doi.org/10.1126/science.275.5300.637}
}

@article{ketterle,
  title = {Nobel lecture: When atoms behave as waves: Bose-Einstein condensation and the atom laser},
  author = {Ketterle, Wolfgang},
  journal = {Rev. Mod. Phys.},
  volume = {74},
  issue = {4},
  pages = {1131--1151},
  numpages = {0},
  year = {2002},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.74.1131},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.74.1131}
}

@article{javanainen1997phase,
  title = {Phase and Phase Diffusion of a Split Bose-Einstein Condensate},
  author = {Javanainen, Juha and Wilkens, Martin},
  journal = {Phys. Rev. Lett.},
  volume = {78},
  issue = {25},
  pages = {4675--4678},
  numpages = {0},
  year = {1997},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.78.4675},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.78.4675}
}


@article{javanainen1996quantum,
  title = {Quantum Phase of a Bose-Einstein Condensate with an Arbitrary Number of Atoms},
  author = {Javanainen, Juha and Yoo, Sung Mi},
  journal = {Phys. Rev. Lett.},
  volume = {76},
  issue = {2},
  pages = {161--164},
  numpages = {0},
  year = {1996},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.76.161},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.76.161}
}

@article{ahufinger1,
  title = {Creation and mobility of discrete solitons in Bose-Einstein condensates},
  author = {Ahufinger, V. and Sanpera, A. and Pedri, P. and Santos, L. and Lewenstein, M.},
  journal = {Phys. Rev. A},
  volume = {69},
  issue = {5},
  pages = {053604},
  numpages = {7},
  year = {2004},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.69.053604},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.69.053604}
}

@article{ahufinger2,
  title = {Adiabatic splitting, transport, and self-trapping of a Bose-Einstein condensate in a double-well potential},
  author = {Ottaviani, C. and Ahufinger, V. and Corbal\'an, R. and Mompart, J.},
  journal = {Phys. Rev. A},
  volume = {81},
  issue = {4},
  pages = {043621},
  numpages = {8},
  year = {2010},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.81.043621},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.81.043621}
}

@article{polo2013soliton,
  title = {Soliton-based matter-wave interferometer},
  author = {Polo, J. and Ahufinger, V.},
  journal = {Phys. Rev. A},
  volume = {88},
  issue = {5},
  pages = {053628},
  numpages = {8},
  year = {2013},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.88.053628},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.88.053628}
}

@article{Ji_2016,
	author = {Shen-Tong Ji and Yuan-Sheng Wang and Yue-E Luo and Xue-Shen Liu},
	title = {Generating periodic interference in Bose-Einstein condensates},
    journal = {Chin. Phys. B},
	doi = {10.1088/1674-1056/25/9/090303},
	url = {https://doi.org/10.1088/1674-1056/25/9/090303},
	year = {2016},
	month = {aug},
	publisher = {{IOP} Publishing},
	volume = {25},
	number = {9},
	pages = {090303}
}


@article{bao2003numerical,
author = {Weizhu Bao and Dieter Jaksch and Peter A. Markowich},
title = {Numerical solution of the Gross-Pitaevskii equation for Bose-Einstein condensation},
journal = {J. Comput. Phys.},
volume = {187},
number = {1},
pages = {318-342},
year = {2003},
issn = {0021-9991},
doi = {https://doi.org/10.1016/S0021-9991(03)00102-5},
url = {https://www.sciencedirect.com/science/article/pii/S0021999103001025}
}

@article{ANTOINE20132621,
author = {Xavier Antoine and Weizhu Bao and Christophe Besse},
title = {Computational methods for the dynamics of the nonlinear Schr\"odinger/Gross-Pitaevskii equations},
journal = {Comp. Phys. Comm.},
volume = {184},
number = {12},
pages = {2621-2633},
year = {2013},
issn = {0010-4655},
doi = {https://doi.org/10.1016/j.cpc.2013.07.012},
url = {https://www.sciencedirect.com/science/article/pii/S0010465513002403}
}

@article{huang2006creation,
  title = {Creation, detection, and decoherence of macroscopic quantum superposition states in double-well Bose-Einstein condensates},
  author = {Y. P. Huang and M. G. Moore},
  journal = {Phys. Rev. A},
  volume = {73},
  issue = {2},
  pages = {023606},
  numpages = {20},
  year = {2006},
}

@article{wang2007effect,
  title = {Effect of decoherence on the dynamics of Bose-Einstein condensates in a double-well potential},
  author = {Wang, W. and Fu, L. B. and Yi, X. X.},
  journal = {Phys. Rev. A},
  volume = {75},
  issue = {4},
  pages = {045601},
  numpages = {4},
  year = {2007},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.75.045601},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.75.045601}
}

@article{ai2004influence,
  title={Influence of Decoherence on Interference Between Two Bose-Einstein Condensates},
  author={Ai-Hua, Zeng and Le-Man, Kuang},
  journal={Commun. Theor. Phys},
  volume={41},
  number={1},
  pages={41},
  year={2004},
}

@article{Lee2012,
author= {Lee, Chaohong and Huang, Jiahao and Deng, Haiming and Dai, Hui and Xu, Jun},
title={Nonlinear quantum interferometry with Bose condensed atoms},
journal={Front. Phys.},
year={2012},
volume={7},
pages={109--130},
doi={https://doi.org/10.1007/s11467-011-0228-6},
url={https://link.springer.com/article/10.1007/s11467-011-0228-6}
}

@article{PhysRevLett.100.080405,
  title = {Atom Interferometry with a Weakly Interacting Bose-Einstein Condensate},
  author = {Fattori, M. and D'Errico, C. and Roati, G. and Zaccanti, M. and Jona-Lasinio, M. and Modugno, M. and Inguscio, M. and Modugno, G.},
  journal = {Phys. Rev. Lett.},
  volume = {100},
  issue = {8},
  pages = {080405},
  numpages = {4},
  year = {2008},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.100.080405},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.100.080405}
}

@article{PhysRevLett.95.070401,
  title = {Bose-Einstein Condensate in a Random Potential},
  author = {Lye, J. E. and Fallani, L. and Modugno, M. and Wiersma, D. S. and Fort, C. and Inguscio, M.},
  journal = {Phys. Rev. Lett.},
  volume = {95},
  issue = {7},
  pages = {070401},
  numpages = {4},
  year = {2005},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.95.070401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.95.070401}
}

@article{PhysRevA.66.021601,
  title = {Free expansion of a Bose-Einstein condensate in a one-dimensional optical lattice},
  author = {Morsch, O. and Cristiani, M. and M\"uller, J. H. and Ciampini, D. and Arimondo, E.},
  journal = {Phys. Rev. A},
  volume = {66},
  issue = {2},
  pages = {021601(R)},
  numpages = {4},
  year = {2002},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.66.021601},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.66.021601}
}

@Inbook{Morsch2002,
author="Morsch, Oliver and Arimondo, Ennio",
editor="Dauxois, Thierry and Ruffo, Stefano and Arimondo, Ennio and Wilkens, Martin",
title="Ultracold Atoms and Bose-Einstein Condensates in Optical Lattices",
bookTitle="Dynamics and Thermodynamics of Systems with Long-Range Interactions",
year="2002",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="312--331",
}

@article{PhysRevE.92.013201,
  title = {Stationary solutions for the nonlinear Schr\"odinger equation modeling three-dimensional spherical Bose-Einstein condensates in general potentials},
  author = {Mallory, Kristina and Van Gorder, Robert A.},
  journal = {Phys. Rev. E},
  volume = {92},
  issue = {1},
  pages = {013201},
  numpages = {21},
  year = {2015},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.92.013201},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.92.013201}
}

@article{PhysRevE.85.056608,
  title = {Matter-wave solutions in Bose-Einstein condensates with harmonic and Gaussian potentials},
  author = {Yan, Zhenya and Jiang, Dongmei},
  journal = {Phys. Rev. E},
  volume = {85},
  issue = {5},
  pages = {056608},
  numpages = {11},
  year = {2012},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.85.056608},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.85.056608}
}

@article{PhysRevE.75.036214,
  title = {Dynamics of Bose-Einstein condensates under the influence of periodic and harmonic potentials},
  author = {Berry, N. Hawk and Kutz, J. Nathan},
  journal = {Phys. Rev. E},
  volume = {75},
  issue = {3},
  pages = {036214},
  numpages = {9},
  year = {2007},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.75.036214},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.75.036214}
}

@article{PhysRevE.89.013204,
  title = {Stationary solutions for the 1$+$1 nonlinear Schr\"odinger equation modeling attractive Bose-Einstein condensates in small potentials},
  author = {Mallory, Kristina and Van Gorder, Robert A.},
  journal = {Phys. Rev. E},
  volume = {89},
  issue = {1},
  pages = {013204},
  numpages = {11},
  year = {2014},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.89.013204},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.89.013204}
}

@article{PhysRevE.62.1382,
  title = {Numerical solution of the Gross-Pitaevskii equation using an explicit finite-difference scheme: An application to trapped Bose-Einstein condensates},
  author = {Cerimele, M. M. and Chiofalo, M. L. and Pistella, F. and Succi, S. and Tosi, M. P.},
  journal = {Phys. Rev. E},
  volume = {62},
  issue = {1},
  pages = {1382--1389},
  numpages = {0},
  year = {2000},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.62.1382},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.62.1382}
}

@article{dalfovo1999theory,
  title = {Theory of Bose-Einstein condensation in trapped gases},
  author = {Dalfovo, Franco and Giorgini, Stefano and Pitaevskii, Lev P. and Stringari, Sandro},
  journal = {Rev. Mod. Phys.},
  volume = {71},
  issue = {3},
  pages = {463--512},
  numpages = {0},
  year = {1999},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.71.463},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.71.463}
}

@article{parker2003soliton,
  title = {Soliton-Sound Interactions in Quasi-One-Dimensional Bose-Einstein Condensates},
  author = {Parker, N. G. and Proukakis, N. P. and Leadbeater, M. and Adams, C. S.},
  journal = {Phys. Rev. Lett.},
  volume = {90},
  issue = {22},
  pages = {220401},
  numpages = {4},
  year = {2003},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.90.220401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.90.220401}
}

@article{parker2010dark,
  title = {Dark soliton decay due to trap anharmonicity in atomic Bose-Einstein condensates},
  author = {Parker, N. G. and Proukakis, N. P. and Adams, C. S.},
  journal = {Phys. Rev. A},
  volume = {81},
  issue = {3},
  pages = {033606},
  numpages = {10},
  year = {2010},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.81.033606},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.81.033606}
}

@article {Anderson198,
author = {M. H. Anderson  and J. R. Ensher  and M. R. Matthews  and C. E. Wieman  and E. A. Cornell },
title = {Observation of Bose-Einstein Condensation in a Dilute Atomic Vapor},
journal = {Science},
volume = {269},
number = {5221},
pages = {198-201},
year = {1995},
doi = {10.1126/science.269.5221.198},
URL = {https://www.science.org/doi/abs/10.1126/science.269.5221.198}
}

@article{PhysRevLett.75.1687,
  title = {Evidence of Bose-Einstein Condensation in an Atomic Gas with Attractive Interactions},
  author = {Bradley, C. C. and Sackett, C. A. and Tollett, J. J. and Hulet, R. G.},
  journal = {Phys. Rev. Lett.},
  volume = {75},
  issue = {9},
  pages = {1687--1690},
  numpages = {0},
  year = {1995},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.75.1687},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.75.1687}
}

@article{PhysRevLett.75.3969,
  title = {Bose-Einstein Condensation in a Gas of Sodium Atoms},
  author = {Davis, K. B. and Mewes, M. -O. and Andrews, M. R. and van Druten, N. J. and Durfee, D. S. and Kurn, D. M. and Ketterle, W.},
  journal = {Phys. Rev. Lett.},
  volume = {75},
  issue = {22},
  pages = {3969--3973},
  numpages = {0},
  year = {1995},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.75.3969},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.75.3969}
}

@article{PhysRevLett.85.1795,
  title = {Stable ${}^{85}\mathrm{Rb}$ Bose-Einstein Condensates with Widely Tunable Interactions},
  author = {Cornish, S. L. and Claussen, N. R. and Roberts, J. L. and Cornell, E. A. and Wieman, C. E.},
  journal = {Phys. Rev. Lett.},
  volume = {85},
  issue = {9},
  pages = {1795--1798},
  numpages = {0},
  year = {2000},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.85.1795},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.85.1795}
}

@incollection{sanz2019bohmian,
  author={A.S. Sanz},
  title={Bohmian pathways into chemistry: A brief overview},
  booktitle={Applied Bohmian mechanics: From nanoscale systems to cosmology},
  editor={Oriols, Xavier and Mompart, Jordi},
  year={2019},
  publisher={Panstanford Pub},
  pages={257-330},
  year={2019},
}

@article{landau:PhysRev:1941,
  title = {Theory of the Superfluidity of Helium II},
  author = {Landau, L.},
  journal = {Phys. Rev.},
  volume = {60},
  issue = {4},
  pages = {356--358},
  numpages = {0},
  year = {1941},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.60.356},
  url = {https://link.aps.org/doi/10.1103/PhysRev.60.356}
}


@phdthesis{Weller2009DynamicsAI,
  title={Dynamics and interaction of dark solitons in Bose-Einstein condensates},
  author={Andreas Weller},
  year={2009},
}

@PHDTHESIS{ronzheimer:PhDThesis:2008,
  AUTHOR =       {J. Ph. Ronzheimer},
  TITLE =        {Interactions of Dark Solitons in Cigar Shaped Bose-Einstein Condensates},
  SCHOOL =       {Kirchhoff-Institut f\"ur Physik, University of Heidelberg},
  YEAR =         {2008},
  address =      {Germany},
}

@PHDTHESIS{weller:PhDThesis:2009,
  AUTHOR =       {A. Weller},
  TITLE =        {Dynamics and Interaction of Dark Solitons in Bose-Einstein Condensates},
  SCHOOL =       {University of Heidelberg},
  YEAR =         {2009},
  address =      {Germany},
}

@article{sanz:PRA:2005,
  title = {Loss of coherence in double-slit diffraction experiments},
  author = {Sanz, A. S. and Borondo, F. and Bastiaans, M. J.},
  journal = {Phys. Rev. A},
  volume = {71},
  issue = {4},
  pages = {042103},
  numpages = {7},
  year = {2005},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.71.042103},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.71.042103}
}


@article{tounli:arxiv:2019-2,
 author    = {J. Tounli and A. S. Sanz},
 journal   = {arXiv:},
 title     = {BEC with quantum state diffusion},
 volume    = {},
 pages     = {},
 year      = {submitted, 2019},
}

@BOOK{benseny:PanStanford:2012,
  AUTHOR     = {A. Benseny and J. Bagud\`a and X. Oriols and G. Birkl and J. Mompart},
  editor     = {X. Oriols and J. Mompart},
  title      = {Applied Bohmian Mechanics: From Nanoscale Systems to Cosmology},
  CHAPTER    = {Atomtronics: Coherent control of atomic flow via adiabatic passage},
  pages      = {189-233},
  publisher  = {Pan Standford Publishing},
  year       = {2012},
  address    = {Singapore},
}

@BOOK{bricmont-bk,
  AUTHOR     = {J. Bricmont},
  TITLE      = {Making Sense of Quantum Mechanics},
  PUBLISHER  = {Springer},
  YEAR       = {2016},
  address    = {Berlin},
}

@article{steinberg:SciAdv:2016,
 author    = {D. H. Mahler and L. Rozema and K. Fisher and L. Vermeyden and K. J. Resch and H. M. Wiseman and A. Steinberg},
 journal   = {Sci. Adv.},
 title     = {Experimental nonlocal and surreal Bohmian trajectories},
 volume    = {2},
 pages     = {e1501466},
 year      = {2016},
 doi       = {10.1126/sciadv.150146},
}

@article{DeRaedt:PhysicaE:2010,
 author    = {H. De Raedt and S. Zhao and S. Yuan and F. Jin and K. Michielsen and S. Miyashita},
 journal   = {Physica E},
 title     = {Event-by-event simulation of quantum phenomena},
 volume    = {42},
 pages     = {298-302},
 year      = {2010},
}

@article{DeRaedt:JPSJ:2010,
 author    = {F. Jin and S. Yuan and H. De Raedt and K. Michielsen and S. Miyashita},
 journal   = {J. Phys. Soc. Jpn.},
 title     = {Corpuscular model of two-beam interference and double-slit experiments with single photons},
 volume    = {79},
 pages     = {074401(1-14)},
 year      = {2010},
}

@article{webb:IJTP:2011,
 author    = {G. F. Webb},
 journal   = {Int. J. Theor. Phys.},
 title     = {Event based interpretation of Schr\"odinger's equation for the two-slit experiment},
 volume    = {50},
 pages     = {3571-3601},
 year      = {2011},
}

@article{muser-hiley:SciAm:2013,
   author =       {G. Muser},
   title =        {The wholeness of quantum reality: An interview with physicist Basil Hiley},
   journal =      {Sci. Am.},
   volume =       {November 4},
   year =         {2013},
   url = {https://blogs.scientificamerican.com/critical-opalescence/the-wholeness-of-quantum-reality-an-interview-with-physicist-basil-hiley/},
   note =         {Online: https://blogs.scientificamerican.com/critical-opalescence/the-wholeness-of-quantum-reality-an-interview-with-physicist-basil-hiley/},
 }

@article{dirac:PRSLA:1931,
 author    = {P. A. M. Dirac},
 journal   = {Proc. R. Soc. Lond. A},
 title     = {Quantised singularities in the electromagnetic field},
 volume    = {133},
 pages     = {60-72},
 year      = {1931},
}

@article{pennings:JLightTech:1995,
 author    = {L. B. Soldano and E. C. M. Pennings},
 journal   = {J. Light. Tech.},
 title     = {Optical multi-model interference devices based on self-imaging: Principles and applications},
 volume    = {13},
 pages     = {615-627},
 year      = {1995},
}

@article{pusey:NaturePhys:2012,
 author    = {M. F. Pusey and J. Barrett and T. Rudolph},
 journal   = {Nature Phys.},
 title     = {On the reality of the quantum state},
 volume    = {8},
 pages     = {475-478},
 year      = {2012},
}

@article{sudarshan:PRD:1989,
 author    = {I. M. Duck and P. M. Stevenson and E. C. G. Sudarshan},
 journal   = {Phys. Rev. D},
 title     = {The sense in which a ``weak measurement'' of a spin-1/2 particle's spin component yields a value 100},
 volume    = {40},
 pages     = {2112-2117},
 year      = {1989},
}

@article{sanz:FrontPhys:submit21,
 author    = {A. S. Sanz},
 journal   = {Front. Phys.},
 title     = {Unveiling the hidden symmetries behind entangled bipartite continuous-variable systems by means of Bohmian mechanics},
 volume    = {},
 pages     = {},
 year      = {submitted, 2021},
}

@article{umul:Optik:2020,
 author    = {Y. Z. Umul},
 journal   = {Optik},
 title     = {On the reality of the Bohmian potential},
 volume    = {224},
 pages     = {165729(1-5)},
 year      = {2020},
}

@article{hojman:arxiv:2021,
 author    = {S. A. Hojman and F. A. Asenjo and H. M. Moya-Cessa and F. Soto-Eguibar},
 journal   = {Preprint},
 title     = {Bohm potential is real and its effects are measurable},
 volume    = {},
 pages     = {1-4},
 year      = {2021},
 archivePrefix = {arXiv},
 eprint        = {2101.06738},
}

@article{tounli:arxiv:2021,
 author    = {J. Tounli and A. S. Sanz},
 journal   = {},
 title     = {},
 volume    = {},
 pages     = {},
 year      = {in preparation},
}

@BOOK{eberly-bk,
  AUTHOR     = {L. Allen and J. H. Eberly},
  TITLE      = {Optical Resonance and Two-Level Atoms},
  PUBLISHER  = {Dover},
  YEAR       = {1975},
  address    = {New York},
}

@article{zurek:PhysToday:1991,
 author    = {W. H. Zurek},
 journal   = {Phys. Today},
 title     = {Decoherence and the transition from quantum to classical},
 volume    = {44(10)},
 pages     = {36-44},
 year      = {1991},
 doi       = {10.1063/1.881293},
 url       = {https://doi.org/10.1063/1.881293},
}

@article{zurek:PhysToday-rev:2003,
 author    = {W. H. Zurek},
 journal   = {Los Alamos Science},
 title     = {Decoherence and the transition from quantum to classical -- Revisited},
 volume    = {27},
 pages     = {2-25},
 year      = {2002},
}

@article{mathew:MPLB:2013,
 author    = {A. Mathew and M. K. Nandy},
 journal   = {Mod. Phys. Lett. B},
 title     = {Decoherence study of electron spin states in quantum dots using a simplistic model},
 volume    = {27},
 pages     = {1350119(1-9)},
 year      = {2013},
}

@article{khaetskii:PRL:2002,
 author    = {A. V. Khaetskii and D. Loss and L. Glazman},
 journal   = {Phys. Rev. Lett.},
 title     = {Electron spin decoherence in quantum dots due to interaction with nuclei},
 volume    = {88},
 pages     = {186802(1-4)},
 year      = {2002},
}

@article{altaisky:EPJWebConf:2016,
 author = {M. V. Altaisky and N. N. Zolnikova and N. E. Kaputkina and V. A. Krylov and Yu. E. Lozovik and N. S. Dattani},
 title  = {Decoherence and entanglement simulation in a model of quantum neural wetwork based on quantum dots},
 journal = {EPJ Web of Conferences},
 year = {2016},
 volume = {108},
 pages = {02006(1-6)},
}

@article{kendon:PRA:2003,
 author    = {V. Kendon and B. Tregenna},
 journal   = {Phys. Rev. A},
 title     = {Decoherence can be useful in quantum walks},
 volume    = {67},
 pages     = {042315(1-6)},
 year      = {2003},
}

@article{yin:PRA:2008,
 author    = {Y. Yin and D. E. Katsanos and S. N. Evangelou},
 journal   = {Phys. Rev. A},
 title     = {Quantum walks on a random environment},
 volume    = {77},
 pages     = {022302(1-7)},
 year      = {2008},
}

@article{kimm:PRA:2002,
 author    = {K. Kimm and H. H. Kwon},
 journal   = {Phys. Rev. A},
 title     = {Decoherence of the quantum gate in Milburn's model of decoherence},
 volume    = {65},
 pages     = {022311(1-5)},
 year      = {2002},
}

@article{leman:CTP:1998,
 author    = {K. Leman},
 journal   = {Commun. Theor. Phys.},
 title     = {Decoherence induced by discontinuous and stochastic unitary evolution of qubits in quantum computers},
 volume    = {29},
 pages     = {169-172},
 year      = {1998},
}

@article{ziman:PRA:2005,
 author    = {M. Ziman and V. Bu\v{z}ek},
 journal   = {Phys. Rev. A},
 title     = {All (qubit) decoherences: Complete characterization and physical implementation},
 volume    = {72},
 pages     = {022110(1-9)},
 year      = {2005},
}

@article{czerwinski:IJTP:2016,
 author    = {A. Czerwinski},
 journal   = {Int. J. Theor. Phys.},
 title     = {Applications of the stroboscopic tomography to selected 2-level decoherence models},
 volume    = {55},
 pages     = {658-668},
 year      = {2016},
}

@article{floss:PRB:2019,
 author    = {I. Floss and C. Lemell and K. Yabana and J. Burgd\"orfer},
 journal   = {Phys. Rev. B},
 title     = {Incorporating decoherence into solid-state time-dependent density functional theory},
 volume    = {99},
 pages     = {224301(1-14)},
 year      = {2019},
}

@article{petruccione:PRAppl:2018,
 author    = {S. G. Dlamini and J. T. Francis and X. Zhang and \c{S}. K. \"Ozdemir and S. Nic Chormaic and F. Petruccione and M. S. Tame},
 journal   = {Phys. Rev. Appl.},
 title     = {Probing decoherence in plasmonic waveguides in the quantum regime},
 volume    = {9},
 pages     = {024003(1-10)},
 year      = {2018},
}

@article{chen:CTP:2013,
 author    = {C. Chen and Y. B. Gao},
 journal   = {Commun. Theor. Phys.},
 title     = {Quantum decoherence of charge qubit coupled to nonlinear nanomechanical resonator},
 volume    = {60},
 pages     = {531-534},
 year      = {2013},
}

@article{schroll:PRA:2003,
 author    = {C. Schroll and W. Belzig and C. Bruder},
 journal   = {Phys. Rev. A},
 title     = {Decoherence of cold atomic gases in magnetic microtraps},
 volume    = {68},
 pages     = {043618(1-14)},
 year      = {2003},
}

@article{duan:ChinPhysLett:1997,
 author    = {L.-M. Duan and G.-C. Guo},
 journal   = {Chinese Phys. Lett.},
 title     = {Scheme for reducing decoherence in quantum computer memory by transformation to the coherence-preserving states},
 volume    = {14},
 pages     = {488-491},
 year      = {1997},
}

@article{novais:PRL2006,
 author    = {E. Novais and H. U. Baranger},
 journal   = {Phys. Rev. Lett.},
 title     = {Decoherence by correlated noise and quantum error correction},
 volume    = {97},
 pages     = {040501(1-4)},
 year      = {2006},
}

@article{lei:PRA:2011,
 author    = {Ch. U. Lei and W.-M. Zhang},
 journal   = {Phys. Rev. A},
 title     = {Decoherence suppression of open quantums systems through a strong coupling to non-Markovian reservoirs},
 volume    = {84},
 pages     = {052116(1-5)},
 year      = {2011},
}

@article{ahsan:QIC:2018,
 author    = {M. Ahsan and S. A. Z. Naqvi},
 journal   = {Quantum Inf. Comput.},
 title     = {Performance of topological quantum error correction in the presence of correlated noise},
 volume    = {18},
 pages     = {743-778},
 year      = {2018},
}

@article{batelaan:NJP:2018,
 author    = {P. J. Beierle and L. Zhang and H. Batelaan},
 journal   = {New J. Phys.},
 title     = {Experimental test of decoherence theory using electron matter waves},
 volume    = {20},
 pages     = {113030(1-12)},
 year      = {2018},
}

@article{zeilinger:NJP:2018,
 author    = {S. K. Joshi and J. Pienaar and T. C. Ralph and L. Cacciapuoti and W. McCutcheon and J. Rarity and D. Giggenbach and J. G. Lim and V. Makarov and I. Fuentes and Th. Scheidl and E. Beckert and M. Bourennane and D. E. Bruschi and A. Cabello and J. Capmany and A. Carrasco-Casado and E. Diamanti and M. Du\v{s}ek and D. Elser and A. Gulinatti and R. H. Hadfield and Th. Jennewein and R. Kaltenbaek and M. A. Krainak and H. K. Lo and C. Marquardt and G. Milburn and M. Peev and A. Poppe and V. Pruneri and R. Renner and C. Salomon and J. Skaar and N. Solomos and M. Stip\v{c}evic and J. P. Torres and M. Toyoshima and P. Villoresi and I. Walrnsley and G. Weihs and H. Weinfurter and A. Zeilinger and M. Zukowski and R. Ursin},
 journal   = {New J. Phys.},
 title     = {Space QUEST mission proposal: Experimentally testing decoherence due to gravity},
 volume    = {20},
 pages     = {063016(1-21)},
 year      = {2018},
}

@article{schleich:NJP:2013,
	doi = {10.1088/1367-2630/15/1/013052},
	url = {https://dx.doi.org/10.1088/1367-2630/15/1/013052},
	year = {2013},
	month = {jan},
	publisher = {IOP Publishing},
	volume = {15},
	number = {1},
	pages = {013052},
	author = {P Kazemi and S Chaturvedi and I Marzoli and R F O'Connell and W P Schleich},
	title = {Quantum carpets: a tool to observe decoherence},
	journal = {New J. Phys.},
}

@article{taylor:PCPS:1909,
 author    = {G. I. Taylor},
 journal   = {Proc. Cambridge Phil. Soc.},
 title     = {Interference fringes with feeble light},
 volume    = {15},
 pages     = {114-115},
 year      = {1909},
}

@article{dempster:PhysRev:1927,
 author    = {A. J. Dempster and H. F. Batho},
 journal   = {Phys. Rev.},
 title     = {Light quanta and interference},
 volume    = {30},
 pages     = {644-648},
 year      = {1927},
}

@article{davis:IEEEJQuantumElectron:1979,
 author    = {C. C. Davis},
 journal   = {IEEE J. Quantum Electron.},
 title     = {Single-photon optical heterodyning},
 volume    = {QE--15},
 pages     = {26-29},
 year      = {1979},
}

@article{aspect:EPL:1986,
 author    = {P. Grangier and G. Roger and A. Aspect},
 journal   = {Europhys. Lett.},
 title     = {Experimental evidence for a photon anticorrelation effect on a beam splitter: A new light on single-photon interferences},
 volume    = {1},
 pages     = {173-179},
 year      = {1986},
}

@article{kimura:OptCommun:1989,
 author    = {T. Okoshi and A. Hirose and K. Kimura},
 journal   = {Opt. Commun.},
 title     = {A simple experiment elucidating the duality of light as wave and photon},
 volume    = {72},
 pages     = {7-12},
 year      = {1989},
}

@article{rose:AdvBiolMedPhys:1957,
 author    = {A. Rose},
 journal   = {Adv. Biol. Med. Phys.},
 title     = {Quantum effects in human vision},
 volume    = {5},
 pages     = {211-242},
 year      = {1957},
}

@article{drezet:AnnFondLdBroglie:2021,
 author    = {A. Drezet and B. Stock},
 journal   = {Ann. Fond. Louis de Broglie},
 title     = {A causal and continous interpretation of the quantum theory: About an original manuscript by David Bohm sent to Louis de Broglie in 1951},
 volume    = {},
 pages     = {1-27},
 year      = {2001},
 preprint  = {arXiv:2103.0057},
}

@BOOK{elmore-heald-bk:1969,
  AUTHOR     = {W. C. Elmore and M. A. Heald},
  TITLE      = {Physics of Waves},
  PUBLISHER  = {McGraw-Hill},
  YEAR       = {1969},
  address    = {New York},
}

@article{davidovic:PhysTeacher:2019,
 author    = {M. D. Davidovi\'c and M. Bo\v{z}i\'c},
 journal   = {Phys. Teacher},
 title     = {Geometrical, Fresnel, and Fraunhofer regimes of single-slit diffraction},
 volume    = {57},
 pages     = {176-178},
 year      = {2019},
}

@article{shirali:MathMag:2011,
 author    = {Sh. A. Shirali},
 journal   = {Math. Mag.},
 title     = {The Bhaskara-Aryabhata approximation to the sine function},
 volume    = {84},
 pages     = {98-107},
 year      = {2011},
 doi       = {10.4169/math.mag.84.2.98},
}

@article{honrubia:PRA:2021,
 author    = {E. Honrubia and A. S. Sanz},
 journal   = {Phys. Rev. A},
 title     = {Decoherence in quantum cavities: Environmental erasure of carpet-type structures},
 volume    = {103},
 pages     = {062210},
 year      = {2021},
 doi       = {10.1103/PhysRevA.103.062210},
}

@BOOK{mandelbrot-bk:1977,
  AUTHOR     = {B. B. Mandelbrot},
  TITLE      = {Fractals. Form, Chance, and Dimension},
  PUBLISHER  = {W. H. Freeman and Co.},
  YEAR       = {1977},
  address    = {New York},
}

@BOOK{mandelbrot-bk:1983,
  AUTHOR     = {B. B. Mandelbrot},
  TITLE      = {The Fractal Geometry of Nature},
  PUBLISHER  = {W. H. Freeman and Co.},
  YEAR       = {1983},
  address    = {New York},
}

@article{hall:JPA:2004,
 author    = {M. J. W. Hall},
 journal   = {J. Phys. A: Math. Gen.},
 title     = {Incompleteness of trajectory-based interpretations of quantum mechanics},
 volume    = {37},
 pages     = {9549-9556},
 year      = {2004},
 doi       = {10.1088/0305-4470/37/40/015},
}

@BOOK{bouwmeester-bk:2000,
	editor     = {D. Bouwmeester and A. Ekert and A. Zeilinger},
	TITLE      = {The Physics of Quantum Information},
	PUBLISHER  = {Springer},
	YEAR       = {2000},
	address    = {Berlin},
}

@article{furuya:PRL:1998,
	title = {Quantum Dynamical Manifestation of Chaotic Behavior in the Process of Entanglement},
	author = {Furuya, K. and Nemes, M. C. and Pellegrino, G. Q.},
	journal = {Phys. Rev. Lett.},
	volume = {80},
	issue = {25},
	pages = {5524--5527},
	numpages = {0},
	year = {1998},
	month = {Jun},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.80.5524},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.80.5524}
}

@article{furuya:PRA:2005,
	title = {Semiclassical limit of the entanglement in closed pure systems},
	author = {Angelo, Renato M. and Furuya, K.},
	journal = {Phys. Rev. A},
	volume = {71},
	issue = {4},
	pages = {042321},
	numpages = {7},
	year = {2005},
	month = {Apr},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.71.042321},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.71.042321}
}

@article{sarkar:PRE:1999,
	title = {Signatures of chaos in the entanglement of two coupled quantum kicked tops},
	author = {Miller, Paul A. and Sarkar, Sarben},
	journal = {Phys. Rev. E},
	volume = {60},
	issue = {2},
	pages = {1542--1550},
	numpages = {0},
	year = {1999},
	month = {Aug},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevE.60.1542},
	url = {https://link.aps.org/doi/10.1103/PhysRevE.60.1542}
}

@article{ghose:PRA:2004,
	title = {Entanglement dynamics in chaotic systems},
	author = {Ghose, Shohini and Sanders, Barry C.},
	journal = {Phys. Rev. A},
	volume = {70},
	issue = {6},
	pages = {062315},
	numpages = {5},
	year = {2004},
	month = {Dec},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.70.062315},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.70.062315}
}

@article{zurek:PhysicaD:1995,
	title = {Quantum chaos: a decoherent definition},
	journal = {Physica D: Nonlinear Phenomena},
	volume = {83},
	number = {1},
	pages = {300-308},
	year = {1995},
	note = {Quantum Complexity in Mesoscopic Systems},
	issn = {0167-2789},
	doi = {https://doi.org/10.1016/0167-2789(94)00271-Q},
	url = {https://www.sciencedirect.com/science/article/pii/016727899400271Q},
	author = {Wojciech Hubert Zurek and Juan Pablo Paz},
	abstract = {We show that the rate of increase of Von Neumann entropy computed from the reduced density matrix of an open quantum system is an excellent indicator of the dynamical behavior of its classical Hamiltonian counterpart. In decohering quantum analogs of systems which exhibit classical Hamiltonian chaos entropy production rate quickly tends to a constant which is given by the sum of the positive Lyapunov exponents, and falls off only as the system approaches equilibrium. By contrast, integrable systems tend to have an entropy production rate which decreases as t−1 well before equilibrium is attained. Thus, behavior of quantum systems in contact with the environment can be used as a test to determine the nature of their Hamiltonian evolution.}
}

@article{brumer-hamilton:PRA:1982,
	title = {Relaxation rates for two-dimensional deterministic mappings},
	author = {Hamilton, Ian and Brumer, Paul},
	journal = {Phys. Rev. A},
	volume = {25},
	issue = {6},
	pages = {3457--3459},
	numpages = {0},
	year = {1982},
	month = {Jun},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.25.3457},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.25.3457}
}

@article{brumer-hamilton:JCP:1983,
	author = {Hamilton,Ian  and Brumer,Paul },
	title = {Intramolecular relaxation in N=2 Hamiltonian systems: The role of the K entropy},
	journal = {J. Chem. Phys.},
	volume = {78},
	number = {5},
	pages = {2682-2690},
	year = {1983},
	doi = {10.1063/1.445027},
    URL = {https://doi.org/10.1063/1.445027},
}

@article{brumer-christoffel:PRA:1986,
	title = {Quantum and classical dynamics in the stadium billiard},
	author = {Christoffel, Kurt M. and Brumer, Paul},
	journal = {Phys. Rev. A},
	volume = {33},
	issue = {2},
	pages = {1309--1321},
	numpages = {0},
	year = {1986},
	month = {Feb},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.33.1309},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.33.1309}
}

@article{brumer-pattnayak:PRL:1996,
	title = {Exponential Divergence and Long Time Relaxation in Chaotic Quantum Dynamics},
	author = {Pattanayak, Arjendu K. and Brumer, Paul},
	journal = {Phys. Rev. Lett.},
	volume = {77},
	issue = {1},
	pages = {59--62},
	numpages = {0},
	year = {1996},
	month = {Jul},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.77.59},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.77.59}
}

@article{brumer-pattnayak:PRL:1997,
	title = {Exponentially Rapid Decoherence of Quantum Chaotic Systems},
	author = {Pattanayak, Arjendu K. and Brumer, Paul},
	journal = {Phys. Rev. Lett.},
	volume = {79},
	issue = {21},
	pages = {4131--4134},
	numpages = {0},
	year = {1997},
	month = {Nov},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.79.4131},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.79.4131}
}

@article{brumer-pattnayak:PRE:1997,
	title = {Chaos and Lyapunov exponents in classical and quantal distribution dynamics},
	author = {Pattanayak, Arjendu K. and Brumer, Paul},
	journal = {Phys. Rev. E},
	volume = {56},
	issue = {5},
	pages = {5174--5177},
	numpages = {0},
	year = {1997},
	month = {Nov},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevE.56.5174},
	url = {https://link.aps.org/doi/10.1103/PhysRevE.56.5174}
}

@article{shepelyansky:PRA:2003,
	title = {Entanglement versus relaxation and decoherence in a quantum algorithm for quantum chaos},
	author = {Bettelli, S. and Shepelyansky, D. L.},
	journal = {Phys. Rev. A},
	volume = {67},
	issue = {5},
	pages = {054303},
	numpages = {4},
	year = {2003},
	month = {May},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.67.054303},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.67.054303}
}

@article{brumer-jaffe:JPC:1984,
	author = {Jaffe, Charles and Brumer, Paul},
	title = {Classical Liouville mechanics and intramolecular relaxation dynamics},
	journal = {J. Phys. Chem.},
	volume = {88},
	number = {21},
	pages = {4829-4839},
	year = {1984},
	doi = {10.1021/j150665a007},
	URL = {https://doi.org/10.1021/j150665a007},
}

@article{brumer-jaffe:JCP:1985,
	author = {Jaffé, Charles and Brumer,Paul },
	title = {Classical‐quantum correspondence in the distribution dynamics of integrable systems},
	journal = {J. Chem. Phys.},
	volume = {82},
	number = {5},
	pages = {2330-2340},
	year = {1985},
	doi = {10.1063/1.448946},
	URL = {https://doi.org/10.1063/1.448946},
}

@article{brumer-jaffe:PRL:1985,
	title = {Classical Analog of Pure-State Quantum Dynamics},
	author = {Jaff\'e, Charles and Kanfer, Sheldon and Brumer, Paul},
	journal = {Phys. Rev. Lett.},
	volume = {54},
	pages = {8--10},
	year = {1985},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.54.8},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.54.8},
}

@article{brumer-wilkie:PRA:1997-1,
	title = {Quantum-classical correspondence via Liouville dynamics. I. Integrable systems and the chaotic spectral decomposition},
	author = {Wilkie, Joshua and Brumer, Paul},
	journal = {Phys. Rev. A},
	volume = {55},
	issue = {1},
	pages = {27--42},
	numpages = {0},
	year = {1997},
	month = {Jan},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.55.27},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.55.27}
}

@article{brumer-wilkie:PRA:1997-2,
	title = {Quantum-classical correspondence via Liouville dynamics. II. Correspondence for chaotic Hamiltonian systems},
	author = {Wilkie, Joshua and Brumer, Paul},
	journal = {Phys. Rev. A},
	volume = {55},
	issue = {1},
	pages = {43--61},
	numpages = {0},
	year = {1997},
	month = {Jan},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.55.43},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.55.43}
}

@article{wigner:PhysRev:1932,
	title = {On the Quantum Correction For Thermodynamic Equilibrium},
	author = {Wigner, E.},
	journal = {Phys. Rev.},
	volume = {40},
	issue = {5},
	pages = {749--759},
	numpages = {0},
	year = {1932},
	month = {Jun},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRev.40.749},
	url = {https://link.aps.org/doi/10.1103/PhysRev.40.749}
}

@article{moyal:MathProcCambrdPhilSoc:1949,
	title={Quantum mechanics as a statistical theory},
	volume={45},
	DOI={10.1017/S0305004100000487},
	number={1},
	journal={Mathematical Proceedings of the Cambridge Philosophical Society},
	publisher={Cambridge University Press},
	author={Moyal, J. E.},
	year={1949},
	pages={99–124},
}

@article{bell:physics:1964,
	title = {On the Einstein Podolsky Rosen paradox},
	author = {Bell, J. S.},
	journal = {Physics Physique Fizika},
	volume = {1},
	issue = {3},
	pages = {195--200},
	numpages = {6},
	year = {1964},
	month = {Nov},
	publisher = {American Physical Society},
	doi = {10.1103/PhysicsPhysiqueFizika.1.195},
	url = {https://link.aps.org/doi/10.1103/PhysicsPhysiqueFizika.1.195}
}

@article{bell:RMP:1966,
	title = {On the Problem of Hidden Variables in Quantum Mechanics},
	author = {J. S. Bell},
	journal = {Rev. Mod. Phys.},
	volume = {38},
	issue = {3},
	pages = {447--452},
	numpages = {0},
	year = {1966},
	month = {Jul},
	publisher = {American Physical Society},
	doi = {10.1103/RevModPhys.38.447},
	url = {https://link.aps.org/doi/10.1103/RevModPhys.38.447}
}

@article{bennett-brassard:PRL:1993,
	title = {Teleporting an unknown quantum state via dual classical and Einstein-Podolsky-Rosen channels},
	author = {Bennett, Charles H. and Brassard, Gilles and Cr\'epeau, Claude and Jozsa, Richard and Peres, Asher and Wootters, William K.},
	journal = {Phys. Rev. Lett.},
	volume = {70},
	issue = {13},
	pages = {1895--1899},
	numpages = {0},
	year = {1993},
	month = {Mar},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.70.1895},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.70.1895}
}

@article{boschi-popescu:PRL:1998,
	title = {Experimental Realization of Teleporting an Unknown Pure Quantum State via Dual Classical and Einstein-Podolsky-Rosen Channels},
	author = {Boschi, D. and Branca, S. and De Martini, F. and Hardy, L. and Popescu, S.},
	journal = {Phys. Rev. Lett.},
	volume = {80},
	issue = {6},
	pages = {1121--1125},
	numpages = {0},
	year = {1998},
	month = {Feb},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.80.1121},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.80.1121}
}

@article{ghirardi:JStatPhys:2002,
 author    = {G. Ghirardi and L. Marinatto and T. Weber},
 journal   = {J. Stat. Phys.},
 title     = {Entanglement and properties of composite quantum systems: A conceptual and mathematical analysis},
 volume    = {108},
 pages     = {49--122},
 year      = {2002},
 doi       = {10.1023/A:1015439502289},
 url       = {https://doi.org/10.1023/A:1015439502289},
}

@article{plenio-vedral:PRL:1997,
	title = {Quantifying entanglement},
	author = {Vedral, V. and Plenio, M. B. and Rippin, M. A. and Knight, P. L.},
	journal = {Phys. Rev. Lett.},
	volume = {78},
	issue = {12},
	pages = {2275--2279},
	numpages = {0},
	year = {1997},
	month = {Mar},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.78.2275},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.78.2275},
}

@article{plenio-vedral:PRA:1998,
	title = {Entanglement measures and purification procedures},
	author = {Vedral, V. and Plenio, M. B.},
	journal = {Phys. Rev. A},
	volume = {57},
	issue = {3},
	pages = {1619--1633},
	numpages = {0},
	year = {1998},
	month = {Mar},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.57.1619},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.57.1619}
}

@article{horodecki:QuantumInfComp:2001,
	author    = {Michal Horodecki},
	title     = {Entanglement measures},
	journal   = {Quantum Inf. Comput.},
	volume    = {1},
	number    = {1},
	pages     = {3--26},
	year      = {2001},
	url       = {https://doi.org/10.26421/QIC1.1-2},
	doi       = {10.26421/QIC1.1-2},
	timestamp = {Thu, 29 Apr 2021 18:05:34 +0200},
	biburl    = {https://dblp.org/rec/journals/qic/Horodecki01.bib},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{bruss:JMathPhys:2002,
	author = {Bru{\ss}, Dagmar},
	title = {Characterizing entanglement},
	journal = {Journal of Mathematical Physics},
	volume = {43},
	number = {9},
	pages = {4237-4251},
	year = {2002},
	doi = {10.1063/1.1494474},	
	URL = {https://doi.org/10.1063/1.1494474},
}

@article{buzek-knigh:PRA:1992,
	title = {Schr\"odinger-cat states in the resonant Jaynes-Cummings model: Collapse and revival of oscillations of the photon-number distribution},
	author = {Bu\ifmmode \check{z}\else \v{z}\fi{}ek, V. and Moya-Cessa, H. and Knight, P. L. and Phoenix, S. J. D.},
	journal = {Phys. Rev. A},
	volume = {45},
	issue = {11},
	pages = {8190--8203},
	numpages = {0},
	year = {1992},
	month = {Jun},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.45.8190},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.45.8190}
}

@article{bennett-smolin:PRL:1996,
	title = {Purification of Noisy Entanglement and Faithful Teleportation via Noisy Channels},
	author = {Bennett, Charles H. and Brassard, Gilles and Popescu, Sandu and Schumacher, Benjamin and Smolin, John A. and Wootters, William K.},
	journal = {Phys. Rev. Lett.},
	volume = {76},
	issue = {5},
	pages = {722--725},
	numpages = {0},
	year = {1996},
	month = {Jan},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.76.722},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.76.722}
}

@article{bennett-smolin:PRL:1997,
	title = {Purification of Noisy Entanglement and Faithful Teleportation via Noisy Channels[Phys. Rev. Lett. 76, 722 (1996)]},
	author = {Bennett, Charles H. and Brassard, Gilles and Popescu, Sandu and Schumacher, Benjamin and Smolin, John A. and Wootters, William K.},
	journal = {Phys. Rev. Lett.},
	volume = {78},
	issue = {10},
	pages = {2031--2031},
	numpages = {0},
	year = {1997},
	month = {Mar},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.78.2031},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.78.2031}
}

@article{bennett-smolin:PRA:1996,
	title = {Mixed-state entanglement and quantum error correction},
	author = {Bennett, Charles H. and DiVincenzo, David P. and Smolin, John A. and Wootters, William K.},
	journal = {Phys. Rev. A},
	volume = {54},
	issue = {5},
	pages = {3824--3851},
	numpages = {0},
	year = {1996},
	month = {Nov},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.54.3824},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.54.3824}
}

@article{verstraete:PRA:2003,
	title = {Maximal entanglement versus entropy for mixed quantum states},
	author = {Wei, Tzu-Chieh and Nemoto, Kae and Goldbart, Paul M. and Kwiat, Paul G. and Munro, William J. and Verstraete, Frank},
	journal = {Phys. Rev. A},
	volume = {67},
	issue = {2},
	pages = {022110},
	numpages = {12},
	year = {2003},
	month = {Feb},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.67.022110},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.67.022110}
}

@article{peres:PRL:1996,
	title = {Separability Criterion for Density Matrices},
	author = {Peres, Asher},
	journal = {Phys. Rev. Lett.},
	volume = {77},
	issue = {8},
	pages = {1413--1415},
	numpages = {0},
	year = {1996},
	month = {Aug},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.77.1413},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.77.1413}
}

@article{duan-cirac-zoller:PRL:2000,
	title = {Inseparability Criterion for Continuous Variable Systems},
	author = {Duan, Lu-Ming and Giedke, G. and Cirac, J. I. and Zoller, P.},
	journal = {Phys. Rev. Lett.},
	volume = {84},
	issue = {12},
	pages = {2722--2725},
	numpages = {0},
	year = {2000},
	month = {Mar},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.84.2722},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.84.2722}
}

@article{simon:PRL:2000,
	title = {Peres-Horodecki Separability Criterion for Continuous Variable Systems},
	author = {Simon, R.},
	journal = {Phys. Rev. Lett.},
	volume = {84},
	issue = {12},
	pages = {2726--2729},
	numpages = {0},
	year = {2000},
	month = {Mar},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.84.2726},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.84.2726}
}

@article{horodecki:PhysLettA:1996,
	title = {Separability of mixed states: necessary and sufficient conditions},
	journal = {Physics Letters A},
	volume = {223},
	number = {1},
	pages = {1-8},
	year = {1996},
	issn = {0375-9601},
	doi = {https://doi.org/10.1016/S0375-9601(96)00706-2},
	url = {https://www.sciencedirect.com/science/article/pii/S0375960196007062},
	author = {Michał Horodecki and Paweł Horodecki and Ryszard Horodecki},
	abstract = {We provide necessary and sufficient conditions for the separability of mixed states. As a result we obtain a simple criterion of the separability for 2 × 2 and 2 × 3 systems. Here, the positivity of the partial transposition of a state is necessary and sufficient for its separability. However, this is not the case in general. Some examples of mixtures which demonstrate the utility of the criterion are considered.}
}

@article{wehrl:RMP:1978,
	title = {General properties of entropy},
	author = {Wehrl, Alfred},
	journal = {Rev. Mod. Phys.},
	volume = {50},
	issue = {2},
	pages = {221--260},
	numpages = {0},
	year = {1978},
	month = {Apr},
	publisher = {American Physical Society},
	doi = {10.1103/RevModPhys.50.221},
	url = {https://link.aps.org/doi/10.1103/RevModPhys.50.221}
}

@article{wehrl:RepMathPhys:1979,
	title = {On the relation between classical and quantum-mechanical entropy},
	journal = {Reports on Mathematical Physics},
	volume = {16},
	number = {3},
	pages = {353-358},
	year = {1979},
	issn = {0034-4877},
	doi = {https://doi.org/10.1016/0034-4877(79)90070-3},
	url = {https://www.sciencedirect.com/science/article/pii/0034487779900703},
	author = {Alfred Wehrl},
	abstract = {We discuss the problem how to define the classical entropy and prove an inequality that establishes its relation to the quantum-mechanical entropy. Furthermore we show that it is monotonic.}
}

@article{wehrl:RepMathPhys:1991,
	title = {The many facets of entropy},
	journal = {Reports on Mathematical Physics},
	volume = {30},
	number = {1},
	pages = {119-129},
	year = {1991},
	issn = {0034-4877},
	doi = {https://doi.org/10.1016/0034-4877(91)90045-O},
	url = {https://www.sciencedirect.com/science/article/pii/003448779190045O},
	author = {A. Wehrl},
	abstract = {Several notions of entropy are discussed: classical entropies (Boltzmann, Gibbs, Shannon, quantum-mechanical entropy, skew entropy, among other notions as well as classical and quantum-mechanical dynamical entropies.}
}

@article{popescu-rohrlich:PRA:1997,
	title = {Thermodynamics and the measure of entanglement},
	author = {Popescu, Sandu and Rohrlich, Daniel},
	journal = {Phys. Rev. A},
	volume = {56},
	issue = {5},
	pages = {R3319--R3321},
	numpages = {0},
	year = {1997},
	month = {Nov},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.56.R3319},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.56.R3319}
}

@article{HDmeyer:JCP:1986,
	author = {Meyer, Hans-Dieter},
	title = {Theory of the Liapunov exponents of Hamiltonian systems and a numerical study on the transition from regular to irregular classical motion},
	journal = {J. Chem. Phys.},
	volume = {84},
	number = {6},
	pages = {3147-3161},
	year = {1986},
	doi = {10.1063/1.450296},
    URL = {https://doi.org/10.1063/1.450296},
}

@article{dahlqvist:PRL:1990,
	title = {Existence of stable orbits in the ${\mathit{x}}^{2}$${\mathit{y}}^{2}$ potential},
	author = {Dahlqvist, Per and Russberg, Gunnar},
	journal = {Phys. Rev. Lett.},
	volume = {65},
	issue = {23},
	pages = {2837--2838},
	numpages = {0},
	year = {1990},
	month = {Dec},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.65.2837},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.65.2837}
}

@article{bohigas:PhysRep:1993,
	title = {Manifestations of classical phase space structures in quantum mechanics},
	journal = {Physics Reports},
	volume = {223},
	number = {2},
	pages = {43-133},
	year = {1993},
	issn = {0370-1573},
	doi = {https://doi.org/10.1016/0370-1573(93)90109-Q},
	url = {https://www.sciencedirect.com/science/article/pii/037015739390109Q},
	author = {O. Bohigas and S. Tomsovic and D. Ullmo},
	abstract = {Using two coupled quartic oscillators for illustration, the quantum mechanics of simple systems whose classical analogs have varying degrees of non-integrability is investigated. By taking advantage of discrete symmetries and dynamical quasidegeneracies it is shown that Percival's semiclassical classification scheme, i.e., eigenstates may be separated into a regular and an irregular group, basically works. This allows us to probe deeply into the workings of semiclassical quantization in mixed phase space systems. Some observations of intermediate status states are made. The standard modeling of quantum fluctuation properties exhibited by the irregular states and levels by random matrix ensembles is then put on a physical footing. Generalized ensembles are constructed incorporating such classical information as fluxes crossing partial barriers and relative fractions of phase space volume occupied by interesting subregions. The ensembles apply equally well to both spectral and eigenstate properties. They typically show non-universal, but nevertheless characteristic level fluctuations. In addition, they predict “semiclassical localization” of eigenfunctions and “quantum suppression of chaos” which are quantitatively borne out in the quantum systems.}
}

@article{eckhardt-pollak:PRA:1989,
	title = {Quantum mechanics of a classically chaotic system: Observations on scars, periodic orbits, and vibrational adiabaticity},
	author = {Eckhardt, Bruno and Hose, Gabriel and Pollak, Eli},
	journal = {Phys. Rev. A},
	volume = {39},
	issue = {8},
	pages = {3776--3793},
	numpages = {0},
	year = {1989},
	month = {Apr},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.39.3776},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.39.3776}
}

@article{polavieja-borondo:PRL:1994,
	title = {Scars in Groups of Eigenstates in a Classically Chaotic System},
	author = {de Polavieja, G. G. and Borondo, F. and Benito, R. M.},
	journal = {Phys. Rev. Lett.},
	volume = {73},
	issue = {12},
	pages = {1613--1616},
	numpages = {0},
	year = {1994},
	month = {Sep},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.73.1613},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.73.1613}
}

@article{brumer-gong:PRA:2003,
	title = {Intrinsic decoherence dynamics in smooth Hamiltonian systems: Quantum-classical correspondence},
	author = {Gong, Jiangbin and Brumer, Paul},
	journal = {Phys. Rev. A},
	volume = {68},
	issue = {2},
	pages = {022101},
	numpages = {8},
	year = {2003},
	month = {Aug},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.68.022101},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.68.022101}
}

@article{vedral-maruyama:PRA:2005,
	title = {Thermodynamical detection of entanglement by Maxwell's demons},
	author = {Maruyama, Koji and Morikoshi, Fumiaki and Vedral, Vlatko},
	journal = {Phys. Rev. A},
	volume = {71},
	issue = {1},
	pages = {012108},
	numpages = {5},
	year = {2005},
	month = {Jan},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.71.012108},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.71.012108}
}

@article{shannon:BellSystTechJ:1948-1,
	author={Shannon, C. E.},
	journal={The Bell System Technical Journal}, 
	title={A mathematical theory of communication}, 
	year={1948},
	volume={27},
	number={3},
	pages={379--423},
	doi={10.1002/j.1538-7305.1948.tb01338.x},
}

@article{shannon:BellSystTechJ:1948-2,
	author={Shannon, C. E.},
	journal={The Bell System Technical Journal}, 
	title={A mathematical theory of communication}, 
	year={1948},
	volume={27},
	number={4},
	pages={623--656},
	doi={10.1002/j.1538-7305.1948.tb00917.x},
}

@ARTICLE{shannon:BellSystTechJ:1949,
	author={Shannon, C. E.},
	journal={The Bell System Technical Journal}, 
	title={Communication theory of secrecy systems}, 
	year={1949},
	volume={28},
	number={4},
	pages={656--715},
	doi={10.1002/j.1538-7305.1949.tb00928.x},
}

@article{weyl:ZPhys:1927,
 author    = {H. Weyl},
 journal   = {Zeitschrift f{\"{u}}r Physik},
 title     = {Quantenmechanik und Gruppentheorie},
 volume    = {46},
 pages     = {1--46},
 year      = {1927},
 doi       = {10.1007/BF02055756},
 url       = {https://doi.org/10.1007/BF02055756},
}

@article{gosson:Quanta:2018,
	author = {Maurice de Gosson},
	title = {Quantum Harmonic Analysis of the Density Matrix},
	journal = {Quanta},
	volume = {7},
	number = {1},
	year = {2018},
	abstract = {We will study rigorously the notion of mixed states and their density matrices. We will also discuss the quantum-mechanical consequences of possible variations of Planck's constant h. This review has been written having in mind two readerships: mathematical physicists and quantum physicists. The mathematical rigor is maximal, but the language and notation we use throughout should be familiar to physicists.Quanta 2018; 7: 74–110.},
	issn = {1314-7374},
	pages = {74--110},
	doi = {10.12743/quanta.v7i1.74},
	url = {http://quanta.ws/ojs/index.php/quanta/article/view/74},
}

@article{brumer-gong:PRL:2003,
	title = {When is Quantum Decoherence Dynamics Classical?},
	author = {Gong, Jiangbin and Brumer, Paul},
	journal = {Phys. Rev. Lett.},
	volume = {90},
	issue = {5},
	pages = {050402},
	numpages = {4},
	year = {2003},
	month = {Feb},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.90.050402},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.90.050402}
}

@article{brumer-gong:JModOpt:2003,
	author = {J. Gong and P. Brumer},
	title = {Quantum versus classical decoherence dynamics},
	journal = {Journal of Modern Optics},
	volume = {50},
	number = {15-17},
	pages = {2411-2422},
	year  = {2003},
	publisher = {Taylor & Francis},
	doi = {10.1080/09500340308233572},
	URL = {https://www.tandfonline.com/doi/abs/10.1080/09500340308233572},
	eprint = {https://www.tandfonline.com/doi/pdf/10.1080/09500340308233572},	
}

@article{milburn:PRA:1986,
	title = {Quantum and classical Liouville dynamics of the anharmonic oscillator},
	author = {Milburn, G. J.},
	journal = {Phys. Rev. A},
	volume = {33},
	issue = {1},
	pages = {674--685},
	numpages = {0},
	year = {1986},
	month = {Jan},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.33.674},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.33.674}
}

@article{joy:ModPhysLettB:1993,
	author    = {M. P. Joy and M. Sabir},
	journal   = {Mod. Phys. Lett. B},
	title     = {Chaos and quantum fluctuations in a quartic Hamiltonian system},
	volume    = {7},
	pages     = {1421--1427},
	year      = {1993},
	doi       = {10.1142/S0217984993001466},
    url       = {https://www.worldscientific.com/doi/10.1142/S0217984993001466},
}

@article{sanz:PRE:2012,
	title = {Temperature crossover of decoherence rates in chaotic and regular bath dynamics},
	author = {Sanz, A. S. and Elran, Y. and Brumer, P.},
	journal = {Phys. Rev. E},
	volume = {85},
	issue = {3},
	pages = {036218},
	numpages = {6},
	year = {2012},
	month = {Mar},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevE.85.036218},
	url = {https://link.aps.org/doi/10.1103/PhysRevE.85.036218},
}

@article{scully:JCP:1982,
	author = {Lee,Hai‐Woong  and Scully,Marlan O. },
	title = {Wigner phase‐space description of a Morse oscillator},
	journal = {J. Chem. Phys.},
	volume = {77},
	number = {9},
	pages = {4604-4610},
	year = {1982},
	doi = {10.1063/1.444412},
	URL = {https://doi.org/10.1063/1.444412},
	eprint = {https://doi.org/10.1063/1.444412},	
}

@article{schlosshauer:PhysRep:2019,
	author = {Maximilian Schlosshauer},
	title = {Quantum decoherence},
	journal = {Phys. Rep.},
	volume = {831},
	pages = {1-57},
	year = {2019},
	note = {Quantum decoherence},
	issn = {0370-1573},
	doi = {https://doi.org/10.1016/j.physrep.2019.10.001},
	url = {https://www.sciencedirect.com/science/article/pii/S0370157319303084},
}

@article{philippidis:NuovoCim:1982,
	author = {C. Philippidis and D. Bohm and R. D. Kaye},
	title = {The Aharonov-Bohm effect and the quantum potential},
	journal = {Nuovo Cim. B},
	volume = {71},
	pages = {57-88},
	year = {1982},
	issn = {1826-9877},
	doi = {10.1007/BF02721695},
	url = {https://doi.org/10.1007/BF02721695},
}

@BOOK{peres-bk,
  AUTHOR     = {A. Peres},
  TITLE      = {Quantum Theory: Concepts and Methods},
  PUBLISHER  = {Kluwer Academic Publishers},
  YEAR       = {2002},
  address    = {New York},
}

@article{aiello:OptLett:2016,
author = {Andrea Aiello},
journal = {Opt. Lett.},
number = {7},
pages = {1668--1671},
publisher = {Optica Publishing Group},
title = {Spontaneous generation of singularities in paraxial optical fields},
volume = {41},
month = {Apr},
year = {2016},
url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-41-7-1668},
doi = {10.1364/OL.41.001668}
}

@article{aiello:OSACont:2020,
author = {Andrea Aiello and Martin Pa\'{u}r and Bohumil Stoklasa and Zden\v{e}k Hradil and Jaroslav \v{R}eh\'{a}\v{c}ek and Luis L. S\'{a}nchez-Soto},
journal = {OSA Continuum},
number = {9},
pages = {2387--2394},
publisher = {Optica Publishing Group},
title = {Observation of concentrating paraxial beams},
volume = {3},
month = {Sep},
year = {2020},
url = {https://opg.optica.org/osac/abstract.cfm?URI=osac-3-9-2387},
doi = {10.1364/OSAC.400410}
}

@article{porras:PRA:2021,
  title = {Exploding paraxial beams, vortex beams, and cylindrical beams of light with finite power in linear media, and their enhanced longitudinal field},
  author = {Porras, Miguel A.},
  journal = {Phys. Rev. A},
  volume = {103},
  issue = {3},
  pages = {033506},
  numpages = {7},
  year = {2021},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.103.033506},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.103.033506}
}

@article{berry:AJP:1979,
 author    = {M. V. Berry and N. L. Balazs},
 journal   = {Am. J. Phys.},
 title     = {Nonspreading wave packets},
 volume    = {47},
 pages     = {264-267},
 year      = {1979},
 doi       = {10.1119/1.11855},
}

@article{unnikrishnan:AJP:1996,
 author    = {K. Unnikrishnan and A. R. P. Rau},
 journal   = {Am. J. Phys.},
 title     = {Uniqueness of the {Airy}  packet in quantum mechanics},
 volume    = {64},
 pages     = {1034-1035},
 year      = {1996},
 doi       = {10.1119/1.18322},
}

@article{greenberger:AJP:1980,
	author = {D. M. Greenberger},
	title = {Comment on ``Nonspreading wave packets’’},
	journal = {Am. J. Phys.},
	volume = {48},
	number = {3},
	pages = {256-256},
	year = {1980},
	doi = {10.1119/1.12308},
	URL = {https://doi.org/10.1119/1.12308},
	eprint = {https://doi.org/10.1119/1.12308},
}

@article{besieris:AJP:1994,
	author = {I. M. Besieris and A. M. Shaarawi and R. W. Ziolkowski},
	title = {Nondispersive accelerating wave packets},
	journal = {Am. J. Phys.},
	volume = {62},
	number = {6},
	pages = {519-521},
	year = {1994},
	doi = {10.1119/1.17510},	
	URL = {https://doi.org/10.1119/1.17510},
	eprint = {https://doi.org/10.1119/1.17510},	
}

@article{nguyen:ApplMathComput:2012,
	title = {Construction of accelerating wavepackets},
	author = {H. Nguyen and J. Lekner},
	journal = {Appl. Math. Comput.},
	volume = {218},
	number = {22},
	pages = {10990-10997},
	year = {2012},
    doi = {https://doi.org/10.1016/j.amc.2012.04.060},
	url = {https://www.sciencedirect.com/science/article/pii/S0096300312004596},
}

@article{lekner:EJP:2009,
	title = {Airy wavepacket solutions of the Schr\"odinger equation},
    journal = {Eur. J. Phys.},
	author = {J. Lekner},
	doi = {10.1088/0143-0807/30/3/l04},
	url = {https://doi.org/10.1088/0143-0807/30/3/l04},
	year = 2009,
	month = {apr},
	publisher = {{IOP} Publishing},
	volume = {30},
	number = {3},
	pages = {L43--L46},
}

@Article{arie:Fluids:2019,
	AUTHOR = {G. G. Rozenman and S. Fu and A. Arie and L. Shemer},
	TITLE = {Quantum Mechanical and Optical Analogies in Surface Gravity Water Waves},
	JOURNAL = {Fluids},
	VOLUME = {4},
	YEAR = {2019},
	NUMBER = {2},
	ARTICLE-NUMBER = {96},
	URL = {https://www.mdpi.com/2311-5521/4/2/96},
	DOI = {10.3390/fluids4020096},
}

@article{arie:PRL:2015-1,
	title = {Propagation Dynamics of {Airy}  Water-Wave Pulses},
	author = {Fu, Shenhe and Tsur, Yuval and Zhou, Jianying and Shemer, Lev and Arie, Ady},
	journal = {Phys. Rev. Lett.},
	volume = {115},
	issue = {3},
	pages = {034501},
	numpages = {5},
	year = {2015},
	month = {Jul},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.115.034501},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.115.034501}
}

@article{arie:PhysScr:2019,
	title = {Nanostructuring of electron beams},
    journal = {Phys. Scr.},
	author = {Roy Shiloh and Peng-Han Lu and Roei Remez and Amir H Tavabi and Giulio Pozzi and Rafal E Dunin-Borkowski and Ady Arie},
	doi = {10.1088/1402-4896/aaf258},
	url = {https://doi.org/10.1088/1402-4896/aaf258},
	year = {2019},
	month = {jan},
	publisher = {{IOP} Publishing},
	volume = {94},
	number = {3},
	pages = {034004},
}

@article{voloch:Nature:2013,
	author    = {N. Voloch-Bloch and Y. Lereah and Y. Lilach and A. Gover and A. Arie},
	journal   = {Nature},
	title     = {Generation of electron {Airy}  beams},
	volume    = {494},
	pages     = {331-335},
	year      = {2013},
	doi = {https://doi.org/10.1038/nature11840},
}

@article{wang:JPlasmaPhys:2016,
 title={Airy-like electron plasma wave},
 journal={J. Plasma Phys.},
 author={H. Li and X. Li and J. Wang},
 volume={82},
 DOI={10.1017/S0022377816000039},
 number={1},
 publisher={Cambridge University Press},
 year={2016},
 pages={905820103},
}

@ARTICLE{kang:IEEEJQE:2017,	
	title={Nonparaxial Accelerating Electron Beams}, 
	author={Y. Kang and Y. Zhang and C. Li and H. Zhong and Y. Zhang and M. R. Beli\'c},
	journal={IEEE J. Quantum Electron.}, 
	year={2017},
	volume={53},
	number={2},
	pages={1-6},
	doi={10.1109/JQE.2017.2677382},
}

@article{christodoulides:PRL:2007,
title = {Observation of Accelerating {Airy}  Beams},
author = {Siviloglou, G. A. and Broky, J. and Dogariu, A. and Christodoulides, D. N.},
journal = {Phys. Rev. Lett.},
volume = {99},
issue = {21},
pages = {213901},
numpages = {4},
year = {2007},
month = {Nov},
publisher = {American Physical Society},
doi = {10.1103/PhysRevLett.99.213901},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.99.213901}
}

@article{arie:PRL:2015-2,
  title = {Unveiling the Orbital Angular Momentum and Acceleration of Electron Beams},
  author = {Shiloh, Roy and Tsur, Yuval and Remez, Roei and Lereah, Yossi and Malomed, Boris A. and Shvedov, Vladlen and Hnatovsky, Cyril and Krolikowski, Wieslaw and Arie, Ady},
  journal = {Phys. Rev. Lett.},
  volume = {114},
  issue = {9},
  pages = {096102},
  numpages = {5},
  year = {2015},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.114.096102},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.114.096102}
}

@article{efremidis:PRA:2021,
  title = {Dynamics of self-accelerating electron beams in a homogeneous magnetic field},
  author = {Goutsoulas, Michael and Efremidis, Nikolaos K.},
  journal = {Phys. Rev. A},
  volume = {103},
  issue = {1},
  pages = {013519},
  numpages = {7},
  year = {2021},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.103.013519},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.103.013519}
}

@article{efremidis:PRA:2013,
  title = {Accelerating and abruptly autofocusing matter waves},
  author = {Efremidis, Nikolaos K. and Paltoglou, Vassilis and von Klitzing, Wolf},
  journal = {Phys. Rev. A},
  volume = {87},
  issue = {4},
  pages = {043637},
  numpages = {9},
  year = {2013},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.87.043637},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.87.043637}
}

@article{yuce:MPLB:2015,
author = {Yuce, C.},
title = {Self-accelerating matter waves},
journal = {Modern Physics Letters B},
volume = {29},
number = {28},
pages = {1550171},
year = {2015},
doi = {10.1142/S0217984915501717},
URL = {https://doi.org/10.1142/S0217984915501717},
eprint = {https://doi.org/10.1142/S0217984915501717},
}

@article{christodoulides:Optica:2019,
	title = {Airy beams and accelerating waves: an overview of recent advances},
	author = {Nikolaos K. Efremidis and Zhigang Chen and Mordechai Segev and Demetrios N. Christodoulides},
	journal = {Optica},
	keywords = {Airy beams; Medical imaging; Near field scanning optical microscopy; Nonlinear wave mixing; Optical force; Spatial light modulators},
	number = {5},
	pages = {686--701},
	publisher = {Optica Publishing Group},
	volume = {6},
	month = {May},
	year = {2019},
	url = {http://opg.optica.org/optica/abstract.cfm?URI=optica-6-5-686},
	doi = {10.1364/OPTICA.6.000686},
}

@article{gori:OptLett:2007,
author = {F. Gori and M. Santarsiero},
journal = {Opt. Lett.},
number = {24},
pages = {3531--3533},
publisher = {Optica Publishing Group},
title = {Devising genuine spatial correlation functions},
volume = {32},
month = {Dec},
year = {2007},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-32-24-3531},
doi = {10.1364/OL.32.003531},
}

@article{martinezherrero:OptLett:2009-1,
author = {R. Mart\'{i}nez-Herrero and P. M. Mej\'{i}as and F. Gori},
journal = {Opt. Lett.},
number = {9},
pages = {1399--1401},
publisher = {Optica Publishing Group},
title = {Genuine cross-spectral densities and pseudo-modal expansions},
volume = {34},
month = {May},
year = {2009},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-34-9-1399},
doi = {10.1364/OL.34.001399},
}

@article{martinezherrero:OptLett:2009-2,
author = {Rosario Mart\'{i}nez-Herrero and Pedro M. Mej\'{i}as},
journal = {Opt. Lett.},
number = {15},
pages = {2303--2305},
publisher = {Optica Publishing Group},
title = {Elementary-field expansions of genuine cross-spectral density matrices},
volume = {34},
month = {Aug},
year = {2009},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-34-15-2303},
doi = {10.1364/OL.34.002303},
}

@article{martinezherrero:JOSAA:2021,
author = {Franco Gori and Rosario Mart\'{i}nez-Herrero},
journal = {J. Opt. Soc. Am. A},
number = {5},
pages = {737--748},
publisher = {Optica Publishing Group},
title = {Reproducing Kernel Hilbert spaces for wave optics: tutorial},
volume = {38},
month = {May},
year = {2021},
url = {http://opg.optica.org/josaa/abstract.cfm?URI=josaa-38-5-737},
doi = {10.1364/JOSAA.422738},
}

@BOOK{mandelwolf-bk,
  AUTHOR =       {L. Mandel and E. Wolf},
  TITLE =        {Optical Coherence and Quantum Optics},
  PUBLISHER =    {Cambridge University Press},
  YEAR =         {1995},
  address =      {Cambridge},
}

@article{qureshi:OptLett:2021,
author = {Tabish Qureshi},
journal = {Opt. Lett.},
number = {3},
pages = {492--495},
publisher = {Optica Publishing Group},
title = {Predictability, distinguishability, and entanglement},
volume = {46},
month = {Feb},
year = {2021},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-46-3-492},
doi = {10.1364/OL.415556},
}

@article{ponomarenko:OptLett:2021,
author = {Morteza Hajati and Vincent Sieben and Sergey A. Ponomarenko},
journal = {Opt. Lett.},
number = {16},
pages = {3961--3964},
publisher = {Optica Publishing Group},
title = {Airy beams on incoherent background},
volume = {46},
month = {Aug},
year = {2021},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-46-16-3961},
doi = {10.1364/OL.434168},
}

@article{lumer:Optica:2015,
author = {Yaakov Lumer and Yi Liang and Ran Schley and Ido Kaminer and Elad Greenfield and Daohong Song and Xinzheng Zhang and Jingjun Xu and Zhigang Chen and Mordechai Segev},
journal = {Optica},
number = {10},
pages = {886--892},
publisher = {Optica Publishing Group},
title = {Incoherent self-accelerating beams},
volume = {2},
month = {Oct},
year = {2015},
url = {http://opg.optica.org/optica/abstract.cfm?URI=optica-2-10-886},
doi = {10.1364/OPTICA.2.000886},
}

@article{christodoulides:OptLett:2007,
author = {Georgios A. Siviloglou and Demetrios N. Christodoulides},
journal = {Opt. Lett.},
number = {8},
pages = {979--981},
publisher = {Optica Publishing Group},
title = {Accelerating finite energy {Airy}  beams},
volume = {32},
month = {Apr},
year = {2007},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-32-8-979},
doi = {10.1364/OL.32.000979},
}

@article{forbes:NatCommun:2013,
author = {S. Ngcobo and I. Litvin and L. Burger, and A. Forbes},
journal = {Nat. Commun.},
number = {1},
pages = {2289},
title = {A digital laser for on-demand laser modes},
volume = {4},
year = {2013},
url = {https://doi.org/10.1038/ncomms3289},
doi = {10.1038/ncomms3289},
}

@article{arie:OptLett:2011,
author = {Gil Porat and Ido Dolev and Omri Barlev and Ady Arie},
journal = {Opt. Lett.},
number = {20},
pages = {4119--4121},
publisher = {Optica Publishing Group},
title = {Airy beam laser},
volume = {36},
month = {Oct},
year = {2011},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-36-20-4119},
doi = {10.1364/OL.36.004119},
}

@article{liu:OptExpress:2020,
author = {Xin Liu and Dening Xia and Yashar E. Monfared and Chunhao Liang and Fei Wang and Yangjian Cai and Pujuan Ma},
journal = {Opt. Express},
number = {7},
pages = {9777-9785},
title = {Generation of novel partially coherent truncated {Airy}  beams via Fourier phase processing},
volume = {28},
year = {2020},
url = {https://doi.org/10.1038/ncomms3289},
doi = {10.1364/OE.390477},
}

@article{christodoulides:OptExpress:2008,
author = {John Broky and Georgios A. Siviloglou and Aristide Dogariu and Demetrios N. Christodoulides},
journal = {Opt. Express},
number = {17},
pages = {12880--12891},
publisher = {Optica Publishing Group},
title = {Self-healing properties of optical {Airy}  beams},
volume = {16},
month = {Aug},
year = {2008},
url = {http://opg.optica.org/oe/abstract.cfm?URI=oe-16-17-12880},
doi = {10.1364/OE.16.012880},
}

@incollection{korotkova:ProgOpt:2020,
	author = {O. Korotkova and G. Gbur},
	title = {Chapter Four - Applications of optical coherence theory},
	editor = {T. D. Visser},
	series = {Prog. Opt.},
	publisher = {Elsevier},
	volume = {65},
	pages = {43-104},
	year = {2020},
	booktitle = {A Tribute to Emil Wolf},
	issn = {0079-6638},
	doi = {https://doi.org/10.1016/bs.po.2019.11.004},
	url = {https://www.sciencedirect.com/science/article/pii/S0079663819300204},
}

@article{berry:PTRSA:2002,
 author    = {M. V. Berry},
 journal   = {Phil. Trans. R. Soc. A.},
 title     = {Exuberant interference: rainbows, tides, edges, (de)coherence \ldots},
 volume    = {360},
 pages     = {1023--1037},
 year      = {2002},
 doi       = {10.1098/rsta.2001.0979},
}

@article{berry:PhysToday:2017,
 author    = {M. V. Berry},
 journal   = {Phys. Today},
 title     = {Approaches to studying our history},
 volume    = {70},
 issue     = {3},
 month     = {March},
 pages     = {11--12},
 year      = {2017},
 doi       = {10.1063/PT.3.3478},
}

@article{braunbek:ZNaturA:1951,
 author    = {W. Braunbek},
 journal   = {Z. Naturforsch. A},
 title     = {Zur Darstellung von Wellenfeldern},
 volume    = {6},
 pages     = {12--15},
 year      = {1951},
 doi       = {10.1515/zna-1951-0102},
}

@ARTICLE{wong:FrontPhys:2021,
author={Ren, Yu-Xuan and He, Hongsen and Tang, Huajun and Wong, Kenneth K. Y.},
TITLE={Non-diffracting light wave: Fundamentals and biomedical applications},      
JOURNAL={Front. Phys.},   
pages={698343(1--30)},   
VOLUME={9},           
YEAR={2021},      
URL={https://www.frontiersin.org/articles/10.3389/fphy.2021.698343},       
DOI={10.3389/fphy.2021.698343},
}

@article{greenberger:RMP:1979,
  title = {Coherence effects in neutron diffraction and gravity experiments},
  author = {Greenberger, Daniel M. and Overhauser, A. W.},
  journal = {Rev. Mod. Phys.},
  volume = {51},
  issue = {1},
  pages = {43--78},
  numpages = {0},
  year = {1979},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.51.43},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.51.43}
}

@article{colella:PRL:1975,
  title = {Observation of Gravitationally Induced Quantum Interference},
  author = {Colella, R. and Overhauser, A. W. and Werner, S. A.},
  journal = {Phys. Rev. Lett.},
  volume = {34},
  issue = {23},
  pages = {1472--1474},
  numpages = {0},
  year = {1975},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.34.1472},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.34.1472}
}

@article{langhoff:AJP:1971,
author = {Langhoff, P. W.},
title = {Schr\"odinger Particle in a Gravitational Well},
journal = {Am. J. Phys.},
volume = {39},
number = {8},
pages = {954-957},
year = {1971},
doi = {10.1119/1.1986333},
URL = {https://doi.org/10.1119/1.1986333},
eprint = {https://doi.org/10.1119/1.1986333},
}

@article{gibbs:AJP:1975,
author = {Gibbs, R. L.},
title = {The quantum bouncer},
journal = {American Journal of Physics},
volume = {43},
number = {1},
pages = {25-28},
year = {1975},
doi = {10.1119/1.10024},
URL = {https://doi.org/10.1119/1.10024},
eprint = {https://doi.org/10.1119/1.10024},
}

@article{desko:AJP:1983,
author = {Desko, R. D. and Bord, D. J.},
title = {The quantum bouncer revisited},
journal = {Am. J. Phys.},
volume = {51},
number = {1},
pages = {82-84},
year = {1983},
doi = {10.1119/1.13400},
URL = {https://doi.org/10.1119/1.13400},
eprint = {https://doi.org/10.1119/1.13400},
}

@article{geabanacloche:AJP:1999,
author = {Gea-Banacloche, J.},
title = {A quantum bouncing ball},
journal = {Am. J. Phys.},
volume = {67},
number = {9},
pages = {776-782},
year = {1999},
doi = {10.1119/1.19124},
URL = {https://doi.org/10.1119/1.19124},
eprint = {https://doi.org/10.1119/1.19124},
}

@article{nesvizhevsky:NuclInstMethPhys:2000,
title = {Search for quantum states of the neutron in a gravitational field: gravitational levels},
journal = {Nucl. Instrum. Methods Phys. Res. A},
volume = {440},
number = {3},
pages = {754-759},
year = {2000},
issn = {0168-9002},
doi = {10.1016/S0168-9002(99)01077-3},
url = {https://www.sciencedirect.com/science/article/pii/S0168900299010773},
author = {V. V. Nesvizhevsky and H. B\"orner and A. M. Gagarski and G. A. Petrov and A. K. Petukhov and H. Abele and S. B\"a{\ss}ler and T St\"oferle and S. M. Soloviev},
}

@article{nesvizhevsky:Nature:2002,
 author    = {V. V. Nesvizhevsky and H. G. B\"orner and A. K. Petukhov and H. Abele and S. B\"a{\ss}ler and F. J. Rue{\ss}, T. St\"oferle and A. Westphal and A. M. Gagarski and G. A. Petrov and A. V. Strelkov},
 journal   = {Nature},
 title     = {Quantum states of neutrons in the Earth's gravitational field},
 volume    = {415},
 pages     = {297-299},
 year      = {2002},
 doi       = {10.1038/415297a},
}

@article{nesvizhevsky:EurPhysJC:2005,
 author    = {V. V. Nesvizhevsky and A. K. Petukhov and H. G. B\"orner and T. A. Baranova and A. M. Gagarski and G. A. Petrov and K. V. Protasov and A. Yu. Voronin and S. B\"a{\ss}ler and H. Abele and A. Westphal and L. Lucovac},
 journal   = {Eur. Phys. J. C},
 title     = {Study of the neutron quantum states in the gravity field},
 volume    = {40},
 pages     = {479--491},
 year      = {2005},
 doi       = {10.1140/epjc/s2005-02135-y},
}

@misc{NIST:DLMF,
         key = "{\relax DLMF}",
       title = "{\it NIST Digital Library of Mathematical Functions}",
howpublished = "http://dlmf.nist.gov/, Release 1.1.6 of 2022-06-30",
         url = "http://dlmf.nist.gov/",
        note = "F.~W.~J. Olver, A.~B. {Olde Daalhuis}, D.~W. Lozier, B.~I. Schneider,
                R.~F. Boisvert, C.~W. Clark, B.~R. Miller, B.~V. Saunders,
                H.~S. Cohl, and M.~A. McClain, eds."}

@article{wang:JQuantSpectrRadTrans:2022,
title = {Dual autofocusing circular {Airy}  beams with different initial launch angles},
journal = {Journal of Quantitative Spectroscopy and Radiative Transfer},
volume = {278},
pages = {108010},
year = {2022},
issn = {0022-4073},
doi = {10.1016/j.jqsrt.2021.108010},
url = {https://www.sciencedirect.com/science/article/pii/S002240732100501X},
author = {Yingfei Wang and Yunfeng Jiang},
}

@article{christodoulides:OptLett:2010,
author = {Nikolaos K. Efremidis and Demetrios N. Christodoulides},
journal = {Opt. Lett.},
number = {23},
pages = {4045--4047},
publisher = {Optica Publishing Group},
title = {Abruptly autofocusing waves},
volume = {35},
month = {Dec},
year = {2010},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-35-23-4045},
doi = {10.1364/OL.35.004045},
}

@article{christodoulides:OptLett:2011-1,
author = {Ioannis Chremmos and Peng Zhang and Jai Prakash and Nikolaos K. Efremidis and Demetrios N. Christodoulides and Zhigang Chen},
journal = {Opt. Lett.},
number = {18},
pages = {3675--3677},
publisher = {Optica Publishing Group},
title = {Fourier-space generation of abruptly autofocusing beams and optical bottle beams},
volume = {36},
month = {Sep},
year = {2011},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-36-18-3675},
doi = {10.1364/OL.36.003675},
}

@article{christodoulides:OptLett:2011-2,
author = {Dimitrios G. Papazoglou and Nikolaos K. Efremidis and Demetrios N. Christodoulides and Stelios Tzortzakis},
journal = {Opt. Lett.},
number = {10},
pages = {1842--1844},
publisher = {Optica Publishing Group},
title = {Observation of abruptly autofocusing waves},
volume = {36},
month = {May},
year = {2011},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-36-10-1842},
doi = {10.1364/OL.36.001842},
}

@article{tzortzakis:NatCommun:2013,
 author    = {P. Panagiotopoulos and D. G. Papazoglou and A. Couairon and S. Tzortzakis},
 journal   = {Nat. Commun.},
 title     = {Sharply autofocused ring-Airy beams transforming into non-linear intense light bullets},
 volume    = {4},
 pages     = {2622(1-6)},
 year      = {2013},
 doi       = {10.1038/ncomms3622},
 url       = {https://doi.org/10.1038/ncomms3622},
}

@article{bliokh:PhysRep:2015,
	title = {Transverse and longitudinal angular momenta of light},
	journal = {Phys. Rep.},
	volume = {592},
	pages = {1-38},
	year = {2015},
	issn = {0370-1573},
	doi = {10.1016/j.physrep.2015.06.003},
	url = {https://www.sciencedirect.com/science/article/pii/S0370157315003336},
	author = {Konstantin Y. Bliokh and Franco Nori},
}

@article{serbo:PhysUsp:2018,
	author    = {B. A. Knyazev and V. G. Serbo},
	journal   = {Phys. Usp.},
	title     = {Beams of photons with nonzero projections of orbital angular momenta: New results},
	volume    = {61},
	pages     = {449--479},
	year      = {2018},
	doi = {10.3367/UFNr.2018.02.038306},
}

@article{andreev:JOSAB:2022,
	author = {A. V. Andreev and O. A. Shoutova and S. M. Trushin and S. Yu. Stremoukhov},
	journal = {J. Opt. Soc. Am. B},
	keywords = {Circular polarization; Femtosecond lasers; First order optics; Gaussian beams; Nonlinear optical crystals; Process control},
	number = {7},
	pages = {1775--1782},
	publisher = {Optica Publishing Group},
	title = {3D Stokes parameters for vector focal fields},
	volume = {39},
	month = {Jul},
	year = {2022},
	url = {https://opg.optica.org/josab/abstract.cfm?URI=josab-39-7-1775},
	doi = {10.1364/JOSAB.455841},
}

@article{qiwenzhan:OptCommun:2020,
	title = {Generation of three-dimensionally homogenized focal spot with uniform intensity distribution using vectorial optical fields},
	journal = {Opt. Commun.},
	volume = {464},
	pages = {125530},
	year = {2020},
	issn = {0030-4018},
	doi = {10.1016/j.optcom.2020.125530},
	url = {https://www.sciencedirect.com/science/article/pii/S0030401820301589},
	author = {Elforjani Jera and Sichao Zhou and Qiwen Zhan},
	keywords = {Optical microscopy, Focal field shaping, Homogenized intensity, Polarization},
}

@article{forbes:NatPhotonics:2021,
	author    = {A. Forbes and M. de Oliveira and M. R. Dennis},
	journal   = {Nat. Photonics},
	title     = {Structured light},
	volume    = {15},
	pages     = {253-262},
	year      = {2021},
    doi       = {10.1038/s41566-021-00780-4},
}

@article{maluenda:OptExpress:2014,
	author = {David Maluenda and Rosario Mart\'{i}nez-Herrero and Ignasi Juvells and Artur Carnicer},
	journal = {Opt. Express},
	keywords = {Computer holography; Polarization; Spatial light modulators; Circular polarization; Computer generated holograms; High numerical aperture optics; Numerical simulation; Spatial light modulators; Vector beams},
	number = {6},
	pages = {6859--6867},
	publisher = {Optica Publishing Group},
	title = {Synthesis of highly focused fields with circular polarization at any transverse plane},
	volume = {22},
	month = {Mar},
	year = {2014},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-22-6-6859},
	doi = {10.1364/OE.22.006859},
}

@article{brakenhoff:JMicrosc:1979,
	author = {Brakenhoff, G. J. and Blom, P. and Barends, P.},
	title = {Confocal scanning light microscopy with high aperture immersion lenses},
	journal = {J. Microsc.},
	volume = {117},
	number = {2},
	pages = {219-232},
	doi = {10.1111/j.1365-2818.1979.tb01178.x},
	url = {https://onlinelibrary.wiley.com/doi/abs/10.1111/j.1365-2818.1979.tb01178.x},
	eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1111/j.1365-2818.1979.tb01178.x},
    year = {1979}
}

@article{biss:OptLett:2003,
	author = {D. P. Biss and T. G. Brown},
	journal = {Opt. Lett.},
	keywords = {Nonlinear optics at surfaces; Nonlinear optics at surfaces; Polarization; Azimuthally polarized beams; Optical vortices; Polarized light; Thin films; Ti:sapphire lasers; Vector beams},
	number = {11},
	pages = {923--925},
	publisher = {Optica Publishing Group},
	title = {Polarization-vortex-driven second-harmonic generation},
	volume = {28},
	month = {Jun},
	year = {2003},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-28-11-923},
	doi = {10.1364/OL.28.000923},
}

@article{opron:OptLett:2003,
	author = {Dan Oron and Eran Tal and Yaron Silberberg},
	journal = {Opt. Lett.},
	keywords = {Three-dimensional image acquisition; Scanning microscopy; Multiharmonic generation; Ultrafast nonlinear optics; Circular polarization; Femtosecond lasers; Fluorescence microscopy; Multiphoton microscopy; Phase matching; Refractive index},
	number = {23},
	pages = {2315--2317},
	publisher = {Optica Publishing Group},
	title = {Depth-resolved multiphoton polarization microscopy by third-harmonic generation},
	volume = {28},
	month = {Dec},
	year = {2003},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-28-23-2315},
	doi = {10.1364/OL.28.002315},
}

@article{sheppard:ApplOpt:2004,
	author = {Colin J. R. Sheppard and Amarjyoti Choudhury},
	journal = {Appl. Opt.},
	keywords = {Diffraction theory; Microscopy; Optical recording; Confocal microscopy; Diffractive optical elements; High numerical aperture optics; Optical lithography; Optical systems; Point spread function},
	number = {22},
	pages = {4322--4327},
	publisher = {Optica Publishing Group},
	title = {Annular pupils, radial polarization, and superresolution},
	volume = {43},
	month = {Aug},
	year = {2004},
	url = {https://opg.optica.org/ao/abstract.cfm?URI=ao-43-22-4322},
	doi = {10.1364/AO.43.004322}
}

@inproceedings{serrels:ConfLasers:2008,
	author = {K. A. Serrels and E. Ramsay and R. J. Warburton and D.T. Reid},
	booktitle = {Conference on Lasers and Electro-Optics/Quantum Electronics and Laser Science Conference and Photonic Applications Systems Technologies},
	journal = {Conference on Lasers and Electro-Optics/Quantum Electronics and Laser Science Conference and Photonic Applications Systems Technologies},
	keywords = {Microscopy; Other areas of optics; Resolution; Nonlinear microscopy; Beam structure; Femtosecond lasers; High numerical aperture optics; Imaging systems; Point spread function; Refractive index},
	pages = {QThD3},
	publisher = {Optica Publishing Group},
	title = {Nanoscale Optical Microscopy in the Vectorial Focusing Regime},
	year = {2008},
	url = {https://opg.optica.org/abstract.cfm?URI=QELS-2008-QThD3}
}

@article{gorodetski:PRL:2008,
	title = {Observation of the Spin-Based Plasmonic Effect in Nanoscale Structures},
	author = {Gorodetski, Y. and Niv, A. and Kleiner, V. and Hasman, E.},
	journal = {Phys. Rev. Lett.},
	volume = {101},
	issue = {4},
	pages = {043903},
	numpages = {4},
	year = {2008},
	month = {Jul},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.101.043903},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.101.043903}
}

@article{masihzadeh:OptLett:2009,
	author = {Omid Masihzadeh and Philip Schlup and Randy A. Bartels},
	journal = {Opt. Lett.},
	keywords = {Phase retrieval; Scanning microscopy; Spatial light modulators; Polarization; Ultrafast nonlinear optics; Nonlinear microscopy; Analog to digital converters; Circular polarization; Nonlinear microscopy; Raman scattering; Spatial frequency; Spatial resolution},
	number = {8},
	pages = {1240--1242},
	publisher = {Optica Publishing Group},
	title = {Enhanced spatial resolution in third-harmonic microscopy through polarization switching},
	volume = {34},
	month = {Apr},
	year = {2009},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-34-8-1240},
	doi = {10.1364/OL.34.001240}
}

@article{vuong:PRL:2010,
	title = {Electromagnetic Spin-Orbit Interactions via Scattering of Subwavelength Apertures},
	author = {Vuong, L. T. and Adam, A. J. L. and Brok, J. M. and Planken, P. C. M. and Urbach, H. P.},
	journal = {Phys. Rev. Lett.},
	volume = {104},
	issue = {8},
	pages = {083903},
	numpages = {4},
	year = {2010},
	month = {Feb},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.104.083903},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.104.083903}
}

@article{qiwenzhan:OptLett:2006,
	author = {Qiwen Zhan},
	journal = {Opt. Lett.},
	keywords = {Diffraction theory; Polarization; Circular polarization; Cylindrical vector beams; Laser beams; Light beams; Optical angular momentum; Vortex beams},
	number = {7},
	pages = {867--869},
	publisher = {Optica Publishing Group},
	title = {Properties of circularly polarized vortex beams},
	volume = {31},
	month = {Apr},
	year = {2006},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-31-7-867},
	doi = {10.1364/OL.31.000867}
}

@article{maurer:NewJPhys:2007,
	doi = {10.1088/1367-2630/9/3/078},
	url = {https://doi.org/10.1088/1367-2630/9/3/078},
	year = 2007,
	month = {mar},
	publisher = {{IOP} Publishing},
	volume = {9},
	number = {3},
	pages = {78--78},
	author = {Christian Maurer and Alexander Jesacher and Severin Fürhapter and Stefan Bernet and Monika Ritsch-Marte},
	title = {Tailoring of arbitrary optical vector beams},
	journal = {New J. Phys.},
}

@article{wang:OptExpr:2010,
	author = {Xi-Lin Wang and Yongnan Li and Jing Chen and Cheng-Shan Guo and Jianping Ding and Hui-Tian Wang},
	journal = {Opt. Express},
	keywords = {Interferometry; Polarization; Spatial light modulators; Light matter interactions; Near field optics; Nonlinear optics; Optical elements; Optical systems; Polarization},
	number = {10},
	pages = {10786--10795},
	publisher = {Optica Publishing Group},
	title = {A new type of vector fields with hybrid states of polarization},
	volume = {18},
	month = {May},
	year = {2010},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-18-10-10786},
	doi = {10.1364/OE.18.010786}
}

@article{wang:OptLett:2007,
	author = {Xi-Lin Wang and Jianping Ding and Wei-Jiang Ni and Cheng-Shan Guo and Hui-Tian Wang},
	journal = {Opt. Lett.},
	keywords = {Diffractive optics; Spatial filtering; Diffraction gratings; Polarization; Laser beams; Light beams; Liquid crystal modulators; Spatial frequency; Spatial light modulators; Vector beams},
	number = {24},
	pages = {3549--3551},
	publisher = {Optica Publishing Group},
	title = {Generation of arbitrary vector beams with a spatial light modulator and a common path interferometric arrangement},
	volume = {32},
	month = {Dec},
	year = {2007},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-32-24-3549},
	doi = {10.1364/OL.32.003549}
}

@article{moreno:OptExpr:2011,
	author = {Ignacio Moreno and Claudio Iemmi and Juan Campos and Maria J. Yzuel},
	journal = {Opt. Express},
	keywords = {Spatial light modulators; Polarization; Frequency filtering ; Azimuthally polarized beams; Computer generated holograms; Diffractive optical elements; Fourier optics; Liquid crystal modulators; Matrix methods},
	number = {5},
	pages = {4583--4594},
	publisher = {Optica Publishing Group},
	title = {Jones matrix treatment for optical Fourier processors with structured polarization},
	volume = {19},
	month = {Feb},
	year = {2011},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-19-5-4583},
	doi = {10.1364/OE.19.004583}
}

@article{maluenda:OptExpr:2013,
	author = {David Maluenda and Ignasi Juvells and Rosario Mart\'{i}nez-Herrero and Artur Carnicer},
	journal = {Opt. Express},
	keywords = {Computer holography; Polarization; Spatial light modulators; Computer generated holograms; Light beams; Light matter interactions; Liquid crystal displays; Optical communications; Optical systems},
	number = {5},
	pages = {5432--5439},
	publisher = {Optica Publishing Group},
	title = {Reconfigurable beams with arbitrary polarization and shape distributions at a given plane},
	volume = {21},
	month = {Mar},
	year = {2013},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-21-5-5432},
	doi = {10.1364/OE.21.005432}
}

@article{waller:OptExpr:2013,
	author = {Erik H. Waller and Georg von Freymann},
	journal = {Opt. Express},
	keywords = {Diffractive optics; Spatial light modulators; Active or adaptive optics; Grating prisms; Light matter interactions; Optical trapping; Polarized light; Spatial frequency; Vector beams},
	number = {23},
	pages = {28167--28174},
	publisher = {Optica Publishing Group},
	title = {Independent spatial intensity, phase and polarization distributions},
	volume = {21},
	month = {Nov},
	year = {2013},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-21-23-28167},
	doi = {10.1364/OE.21.028167}
}

@article{han:OptExpr:2013,
	author = {Wei Han and Yanfang Yang and Wen Cheng and Qiwen Zhan},
	journal = {Opt. Express},
	keywords = {Phase modulation; Computer holography; Polarization; Spatial light modulators; Azimuthally polarized beams; Diffractive optical elements; Liquid crystal devices; Liquid crystal modulators; Optical fields; Polarization control},
	number = {18},
	pages = {20692--20706},
	publisher = {Optica Publishing Group},
	title = {Vectorial optical field generator for the creation of arbitrarily complex fields},
	volume = {21},
	month = {Sep},
	year = {2013},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-21-18-20692},
	doi = {10.1364/OE.21.020692}
}

@article{chengshanguo:OptLett:2014,
	author = {Cheng-Shan Guo and Zhen-Yu Rong and Shu-Zhen Wang},
	journal = {Opt. Lett.},
	keywords = {Computer holography; Phase modulation; Spatial light modulators; Polarization; Beam structure; Gaussian beams; Laser beams; Optical elements; Spatial light modulators; Vector beams},
	number = {2},
	pages = {386--389},
	publisher = {Optica Publishing Group},
	title = {Double-channel vector spatial light modulator for generation of arbitrary complex vector beams},
	volume = {39},
	month = {Jan},
	year = {2014},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-39-2-386},
	doi = {10.1364/OL.39.000386}
}

@article{zhenyurong:OptExpr:2014,
	author = {Zhen-Yu Rong and Yu-Jing Han and Shu-Zhen Wang and Cheng-Shan Guo},
	journal = {Opt. Express},
	keywords = {Computer holography; Interferometry; Liquid-crystal devices; Polarization; Spatial light modulators; Cylindrical vector beams; Diffractive optical elements; Light beams; Liquid crystal modulators; Spatial light modulators; Vector beams},
	number = {2},
	pages = {1636--1644},
	publisher = {Optica Publishing Group},
	title = {Generation of arbitrary vector beams with cascaded liquid crystal spatial light modulators},
	volume = {22},
	month = {Jan},
	year = {2014},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-22-2-1636},
	doi = {10.1364/OE.22.001636}
}

@article{novotny:PRL:2001,
	title = {Longitudinal Field Modes Probed by Single Molecules},
	author = {Novotny, L. and Beversluis, M. R. and Youngworth, K. S. and Brown, T. G.},
	journal = {Phys. Rev. Lett.},
	volume = {86},
	issue = {23},
	pages = {5251--5254},
	numpages = {0},
	year = {2001},
	month = {Jun},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.86.5251},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.86.5251}
}

@article{novotny:ApplPhysLett:2003,
	author = {A. Bouhelier M. R. and Beversluis L. Novotny},
	title = {Near-field scattering of longitudinal fields},
	journal = {Applied Physics Letters},
	volume = {82},
	number = {25},
	pages = {4596-4598},
	year = {2003},
	doi = {10.1063/1.1586482},
	URL = {https://doi.org/10.1063/1.1586482},
	eprint = {https://doi.org/10.1063/1.1586482}
}

@article{kitamura:OptExpr:2010,
	author    = {K. Kitamura and K. Sakai K. and S. Noda},
	journal   = {Opt. Express},
	title     = {Sub-wavelength focal spot with long depth of focus generated by radially polarized, narrow- width annular beam},
	volume    = {18},
	pages     = {4518–4525},
	year      = {2010},
	doi       = {https://doi.org/10.1364/oe.18.004518}
}

@article{jia:ApplPhysLett:2005,
	author = {B. Jia and X. Gan and M. Gu},
	title = {Direct observation of a pure focused evanescent field of a high numerical aperture objective lens by scanning near-field optical microscopy},
	journal = {Appl. Phys. Lett.},
	volume = {86},
	number = {13},
	pages = {131110},
	year = {2005},
	doi = {10.1063/1.1886250},
	URL = {https://doi.org/10.1063/1.1886250},
	eprint = {https://doi.org/10.1063/1.1886250}
}

@article{wang:FrontOptoelectron:2012,
	author = {J. Wang and Q. Wang and M. Zhang},
	title = {Development and prospect of near-field optical measurements and characterizations},
	publisher = {Front. Optoelectron.},
	year = {2012},
	journal = {Front. Optoelectron.},
	volume = {5},
	number = {2},
	pages = {171-181},
	url = {https://journal.hep.com.cn/foe/EN/abstract/article_3890.shtml},
	doi = {10.1007/s12200-012-0257-y}
}    

@article{khonina:JOpt:2013,
	doi = {10.1088/2040-8978/15/8/085704},
	url = {https://doi.org/10.1088/2040-8978/15/8/085704},
	year = {2013},
	month = {jul},
	publisher = {{IOP} Publishing},
	volume = {15},
	number = {8},
	pages = {085704},
	author = {Svetlana N Khonina and Sergey V Karpeev and Sergey V Alferov and Dmitry A Savelyev and Janne Laukkanen and Jari Turunen},
	title = {Experimental demonstration of the generation of the longitudinal E-field component on the optical axis with high-numerical-aperture binary axicons illuminated by linearly and circularly polarized beams},
	journal = {J. Opt.},
}

@article{khonina:JOSAA:2014,
	author = {S. V. Alferov and S. N. Khonina and S. V. Karpeev},
	journal = {J. Opt. Soc. Am. A},
	keywords = {Near-field microscopy; Optical vortices ; Electric fields; Electromagnetic radiation; Near field microscopy; Phase plates; Phase shift; Zone plates},
	number = {4},
	pages = {802--807},
	publisher = {Optica Publishing Group},
	title = {Study of polarization properties of fiber-optics probes with use of a binary phase plate},
	volume = {31},
	month = {Apr},
	year = {2014},
	url = {https://opg.optica.org/josaa/abstract.cfm?URI=josaa-31-4-802},
	doi = {10.1364/JOSAA.31.000802}
}

@article{khonina:ApplOpt:2013,
	author = {Victor V. Kotlyar and Sergey S. Stafeev and Yikun Liu and Liam O'Faolain and Alexey A. Kovalev},
	journal = {Appl. Opt.},
	keywords = {Binary optics; Near-field microscopy; Gaussian beams; Laser beams; Light fields; Near field scanning optical microscopy; Optical elements; Zone plates},
	number = {3},
	pages = {330--339},
	publisher = {Optica Publishing Group},
	title = {Analysis of the shape of a subwavelength focal spot for the linearly polarized light},
	volume = {52},
	month = {Jan},
	year = {2013},
	url = {https://opg.optica.org/ao/abstract.cfm?URI=ao-52-3-330},
	doi = {10.1364/AO.52.000330}
}

@article{qiwenzhan:OptLett:2009,
	author = {Weibin Chen and Qiwen Zhan},
	journal = {Opt. Lett.},
	keywords = {Diffraction theory; Scanning microscopy; Surface plasmons; Polarization; Diffraction limit; Interference; Near field scanning optical microscopy; Resonance; Surface plasmons; Surface waves},
	number = {6},
	pages = {722--724},
	publisher = {Optica Publishing Group},
	title = {Realization of an evanescent Bessel beam via surface plasmon interference excited by a radially polarized beam},
	volume = {34},
	month = {Mar},
	year = {2009},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-34-6-722},
	doi = {10.1364/OL.34.000722}
}

@article{khonina:OptLett:2013,
	author = {S. N. Khonina and S. V. Alferov and S. V. Karpeev},
	journal = {Opt. Lett.},
	keywords = {Diffraction; Polarization; Near-field microscopy; Circular polarization; Electric fields; Laser beams; Near field microscopy; Numerical simulation; Vortex beams},
	number = {17},
	pages = {3223--3226},
	publisher = {Optica Publishing Group},
	title = {Strengthening the longitudinal component of the sharply focused electric field by means of higher-order laser beams},
	volume = {38},
	month = {Sep},
	year = {2013},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-38-17-3223},
	doi = {10.1364/OL.38.003223}
}

@article{carnicer:EJP:2012,
	doi = {10.1088/0143-0807/33/5/1235},
	url = {https://doi.org/10.1088/0143-0807/33/5/1235},
	year = 2012,
	month = {jul},
	publisher = {{IOP} Publishing},
	volume = {33},
	number = {5},
	pages = {1235--1247},
	author = {Artur Carnicer and Ignasi Juvells and David Maluenda and Rosario Mart{\'{\i}}nez-Herrero and Pedro M Mej{\'{\i}}as},
	title = {On the longitudinal component of paraxial fields},
	journal = {Eur. J. Phys.}
}

@article{maucher:PRL:2018,
  title = {Creating complex optical longitudinal polarization structures},
  author = {Maucher, F. and Skupin, S. and Gardiner, S. A. and Hughes, I. G.},
  journal = {Phys. Rev. Lett.},
  volume = {120},
  issue = {16},
  pages = {163903},
  numpages = {5},
  year = {2018},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.120.163903},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.120.163903}
}

@article{khonina:OptLett:2020,
author = {Svetlana N. Khonina and Andrey V. Ustinov and Alexey P. Porfirev},
journal = {Opt. Lett.},
keywords = {Azimuthally polarized beams; Cylindrical vector beams; Laser beams; Numerical analysis; Optical tweezers; Vector beams},
number = {15},
pages = {4112--4115},
publisher = {Optica Publishing Group},
title = {Vector Lissajous laser beams},
volume = {45},
month = {Aug},
year = {2020},
url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-45-15-4112},
doi = {10.1364/OL.398209}
}

@article{manjavacas:ACSOmega:2022,
 author    = {L. Zundel and J. R. Deop-Ruano and R. Mart{\'\i}nez-Herrero and A. Manjavacas},
 journal   = {ACS Omega},
 title     = {Lattice resonances excited by finite-width light beams},
 volume    = {7},
 issue     = {35},
 pages     = {31431-31441},
 year      = {2022},
 doi       = {https://doi.org/10.1021/acsomega.2c03847}
}

@BOOK{gellmann-bk:1964,
   title =     {The eightfold way},
   author =    {Gell-Mann M. and Ne'eman Y.},
   publisher = {W. A. Benjamin},
   address   = {New York},
   year =      {1964},
   series =    {Frontiers in Physics Series: Lecture Note & Reprint Series},
   url =       {libgen.li/file.php?md5=819f1fb387c7f4564304d7114fe1f888},
}

@article{GellMann:PhysRev:1962,
  title = {Symmetries of Baryons and Mesons},
  author = {Gell-Mann, Murray},
  journal = {Phys. Rev.},
  volume = {125},
  issue = {3},
  pages = {1067--1084},
  numpages = {0},
  year = {1962},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.125.1067},
  url = {https://link.aps.org/doi/10.1103/PhysRev.125.1067},
}

@article{friberg:PRE:2002,
  title = {Degree of polarization for optical near fields},
  author = {Set\"al\"a, T. and Shevchenko, A. and Kaivola, M. and Friberg, A. T.},
  journal = {Phys. Rev. E},
  volume = {66},
  issue = {1},
  pages = {016615},
  numpages = {7},
  year = {2002},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.66.016615},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.66.016615}
}

@article{sheppard:PRA:2014,
  title = {Jones and Stokes parameters for polarization in three dimensions},
  author = {Sheppard, Colin J. R.},
  journal = {Phys. Rev. A},
  volume = {90},
  issue = {2},
  pages = {023809},
  numpages = {5},
  year = {2014},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.90.023809},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.90.023809}
}

@article{maluenda:SciRep:2021,
 author    = {D. Maluenda and M. Avi{\~n}o\'a and K. Ahmadi and R. Mart{\'\i}nez-Herrero and A. Carnicer},
 journal   = {Sci. Rep.},
 title     = {Experimental estimation of the longitudinal component of a highly focused electromagnetic field},
 volume    = {11},
 pages     = {17992},
 year      = {2021},
 doi       = {https://doi.org/10.1038/s41598-021-97164-z}
}

@article{MartinezHerrero:OptExpr:2020,
author = {R. Mart\'{i}nez-Herrero and A. Carnicer and I. Juvells and A. S. Sanz},
journal = {Opt. Express},
keywords = {Adaptive optics; Diffractive optics; High numerical aperture optics; Holographic memory; Optical fields; Optical systems},
number = {20},
pages = {29676--29690},
publisher = {Optica Publishing Group},
title = {Uncertainty principle for axial power content of highly focused fields},
volume = {28},
month = {Sep},
year = {2020},
url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-28-20-29676},
doi = {10.1364/OE.401073}
}

@misc{localStokesPipeline,
  howpublished = {\url{https://colab.research.google.com/github/WavefrontEngUB/stokes3D/blob/master/Report.ipynb}}
}

@article{arrizon:OptLetters:2003,
  title={Complex modulation with a twisted-nematic liquid-crystal spatial light modulator: double-pixel approach},
  author={Arriz{\'o}n, Victor},
  journal={Opt. Lett.},
  volume={28},
  number={15},
  pages={1359--1361},
  year={2003},
  publisher={Optica Publishing Group},
  doi = {10.1364/OL.28.001359},
  url = {https://doi.org/10.1364/OL.28.001359},
}

@article{nieto-vesperinas:LSA:2022,
 author    = {Nieto-Vesperinas, Manuel and Xu, Xiaohao},
 journal   = {Light Sci. Appl.},
 title     = {The complex Maxwell stress tensor theorem: The imaginary stress tensor and the reactive strength of orbital momentum. A novel scenery underlying electromagnetic optical forces},
 volume    = {11},
 pages     = {297},
 year      = {2022},
 doi       = {10.1038/s41377-022-00979-2},
 url       = {https://doi.org/10.1038/s41377-022-00979-2},
}

@article{leuchs:PRL:2003,
	title = {Sharper Focus for a Radially Polarized Light Beam},
	author = {Dorn, R. and Quabis, S. and Leuchs, G.},
	journal = {Phys. Rev. Lett.},
	volume = {91},
	issue = {23},
	pages = {233901},
	numpages = {4},
	year = {2003},
	month = {Dec},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.91.233901},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.91.233901}
}

@article{bouhelier2003near,
  title={Near-field scattering of longitudinal fields},
  author={Bouhelier, Alexandre and Beversluis, Michael R and Novotny, Lukas},
  journal={Appl. Phys. Lett.},
  volume={82},
  number={25},
  pages={4596--4598},
  year={2003},
  publisher={American Institute of Physics},
  doi = {10.1063/1.1586482},
  url = {https://doi.org/10.1063/1.1586482},  
}

@article{hao2007experimental,
  title={Experimental measurement of longitudinal component in the vicinity of focused radially polarized beam},
  author={Hao, Bing and Leger, James},
  journal={Opt. Express},
  volume={15},
  number={6},
  pages={3550--3556},
  year={2007},
  publisher={Optical Society of America},
  doi = {10.1364/OE.15.003550},
  url = {https://doi.org/10.1364/OE.15.003550},
}

@article{fienup:OptLet:1978,
  title={Reconstruction of an object from the modulus of its Fourier transform},
  author={Fienup, James R},
  journal={Opt. Lett.},
  volume={3},
  number={1},
  pages={27--29},
  year={1978},
  publisher={Optica Publishing Group},
  doi = {10.1364/OL.3.000027},
  url = {https://doi.org/10.1364/OL.3.000027},
}

@article{sanz:AnnFondLdB:2021,
 author    = {A. S. Sanz},
 journal   = {Ann. Fond. Louis de Broglie},
 title     = {Bohm's quantum ``non-mechanics'': An alternative quantum theoryw with its own ontology?},
 volume    = {46},
 pages     = {19-63},
 year      = {2021},
 url       = {https://fondationlouisdebroglie.org/AFLB-461/aflb461m955.htm}
}

@article{sanz:JOSAA:2022,
author = {A. S. Sanz},
journal = {J. Opt. Soc. Am. A},
keywords = {Airy beams; Light beams; Light diffraction; Phase shift; Photons; Structured light},
number = {12},
pages = {C79--C85},
publisher = {Optica Publishing Group},
title = {Flux trajectory analysis of {Airy} -type beams},
volume = {39},
month = {Dec},
year = {2022},
url = {https://opg.optica.org/josaa/abstract.cfm?URI=josaa-39-12-C79},
doi = {10.1364/JOSAA.472653}
}

@article{pati:Pramana:2001,
 author    = {A. K. Pati and M. Zukowski},
 journal   = {Pramana - J. Phys.},
 title     = {Interference due to coherence swapping},
 volume    = {56},
 pages     = {393--401},
 year      = {2001},
 doi       = {10.1007/s12043-001-0133-6},
 url       = {https://doi.org/10.1007/s12043-001-0133-6}
}

@article{sanz:ENTROPY:2022,
AUTHOR = {Sanz, A. S.},
TITLE = {Quantum-classical entropy analysis for nonlinearly-coupled continuous-variable bipartite systems},
JOURNAL = {Entropy},
VOLUME = {24},
YEAR = {2022},
NUMBER = {2},
ARTICLE-NUMBER = {190},
URL = {https://www.mdpi.com/1099-4300/24/2/190},
ISSN = {1099-4300},
DOI = {10.3390/e24020190}
}

@article{sanz:PRResearch:2023,
 author    = {A. S. Sanz and A. Aiello and L. L. S\'anchez-Soto},
 journal   = {Phys. Rev. Research},
 title     = {A quantum trajectory analysis of singular wave functions},
 volume    = {},
 pages     = {},
 year      = {to be published, 2023},
 doi       = {},
 url       = {},
}

@misc{sanz2023quantum,
      title={A quantum trajectory analysis of singular wave functions}, 
      author={A. S. Sanz and L. L. Sanchez-Soto and A. Aiello},
      year={2023},
      eprint={arXiv:2301.13207 (pre-print)},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@article{sanz:PRA:2022,
  title = {Partially coherent {Airy}  beams: A cross-spectral-density approach},
  author = {Mart\'{\i}nez-Herrero, R. and Sanz, A. S.},
  journal = {Phys. Rev. A},
  volume = {106},
  issue = {5},
  pages = {053512},
  numpages = {12},
  year = {2022},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.106.053512},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.106.053512}
}

@ARTICLE{wang:FrontPhys:2021,
AUTHOR={Wang, Jian and Liang, Yize},   
TITLE={Generation and Detection of Structured Light: A Review},      
JOURNAL={Front. Phys.},      
VOLUME={9},
pages={688284},          
YEAR={2021},      
URL={https://www.frontiersin.org/articles/10.3389/fphy.2021.688284},       
DOI={10.3389/fphy.2021.688284},
}

@article{tzemos:PRE:2021,
	title = {Ergodicity and Born's rule in an entangled three-qubit Bohmian system},
	author = {Tzemos, Athanasios C. and Contopoulos, George},
	journal = {Phys. Rev. E},
	volume = {104},
	issue = {5},
	pages = {054211},
	numpages = {14},
	year = {2021},
	month = {Nov},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevE.104.054211},
	url = {https://link.aps.org/doi/10.1103/PhysRevE.104.054211}
}

@article{tzemos:PRE:2020,
	title = {Ergodicity and Born's rule in an entangled two-qubit Bohmian system},
	author = {Tzemos, Athanasios C. and Contopoulos, George},
	journal = {Phys. Rev. E},
	volume = {102},
	issue = {4},
	pages = {042205},
	numpages = {13},
	year = {2020},
	month = {Oct},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevE.102.042205},
	url = {https://link.aps.org/doi/10.1103/PhysRevE.102.042205}
}

@article{tzemos:PhysScr:2021,
	doi = {10.1088/1402-4896/abf18a},
	url = {https://dx.doi.org/10.1088/1402-4896/abf18a},
	year = {2021},
	month = {apr},
	publisher = {IOP Publishing},
	volume = {96},
	number = {6},
	pages = {065209},
	author = {A C Tzemos and G Contopoulos},
	title = {The role of chaotic and ordered trajectories in establishing Born’s rule},
	journal = {Physica Scripta},
}

@Article{plastino:Entropy:2018,
	AUTHOR = {Zander, Claudia and Plastino, Angel Ricardo},
	TITLE = {Revisiting Entanglement within the Bohmian Approach to Quantum Mechanics},
	JOURNAL = {Entropy},
	VOLUME = {20},
	YEAR = {2018},
	NUMBER = {6},
	ARTICLE-NUMBER = {473},
	URL = {https://www.mdpi.com/1099-4300/20/6/473},
	PubMedID = {33265563},
	ISSN = {1099-4300},
	DOI = {10.3390/e20060473}
}

@article{sanz:PhysScr:2022,
	doi = {10.1088/1402-4896/ac6460},
	url = {https://dx.doi.org/10.1088/1402-4896/ac6460},
	year = {2022},
	month = {apr},
	publisher = {IOP Publishing},
	volume = {97},
	number = {5},
	pages = {055507},
	author = {A. Garc{\'\i}a-S\'anchez and A. S Sanz},
	title = {Analysis of the gradual transition from the near to the far field in single-slit diffraction},
	journal = {Phys. Scr.},
}

@article{Efremidis:Optica:2019,
	author = {Nikolaos K. Efremidis and Zhigang Chen and Mordechai Segev and Demetrios N. Christodoulides},
	journal = {Optica},
	keywords = {Airy beams; Medical imaging; Near field scanning optical microscopy; Nonlinear wave mixing; Optical force; Spatial light modulators},
	number = {5},
	pages = {686--701},
	publisher = {Optica Publishing Group},
	title = {Airy beams and accelerating waves: an overview of recent advances},
	volume = {6},
	month = {May},
	year = {2019},
	url = {https://opg.optica.org/optica/abstract.cfm?URI=optica-6-5-686},
	doi = {10.1364/OPTICA.6.000686}
}

@article{Xu:OE:2022,
	author = {Danlin Xu and Yujun Liu and Zhenwu Mo and Junjie Jiang and Jingyi Shi and Zehong Liang and You Wu and Jiajia Zhao and Haobin Yang and Haiqi Huang and Hongzhan Liu and Lingling Shui and Dongmei Deng},
	journal = {Opt. Express},
	number = {1},
	pages = {232--242},
	publisher = {Optica Publishing Group},
	title = {Shaping autofocusing {Airy}  beams through the modification of Fourier spectrum},
	volume = {30},
	month = {Jan},
	year = {2022},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-30-1-232},
	doi = {10.1364/OE.444396}
}

@Article{Zhang:ApplSci:2017,
	AUTHOR = {Zhang, Yiqi and Zhong, Hua and Beli\'c, Milivoj R. and Zhang, Yanpeng},
	TITLE = {Guided Self-Accelerating {Airy}  Beam--A Mini-Review},
	JOURNAL = {Appl. Sci.},
	VOLUME = {7},
	YEAR = {2017},
	NUMBER = {4},
	ARTICLE-NUMBER = {341},
	URL = {https://www.mdpi.com/2076-3417/7/4/341},
	ISSN = {2076-3417},
	DOI = {10.3390/app7040341}
}

@BOOK{margenau-moseley-bk,
  AUTHOR     = {H. Margenau and G. Moseley Murphy},
  TITLE      = {The Mathematics of Physics and Chemistry},
  PUBLISHER  = {D. Van Nostrand},
  YEAR       = {1943},
  address    = {Princeton, NJ},
}

@Article{Schleich:PNAS:2013,
	AUTHOR = {Wolfgang P. Schleich and Daniel M. Greenberger and Donald H. Kobe and Marlan O. Scully},
	TITLE = {Schr\"odinger equation revisited},
	JOURNAL = {Proc. Nat. Acad. Sci.},
	VOLUME = {110},
	YEAR = {2013},
	NUMBER = {14},
	ARTICLE-NUMBER = {5374-5379},
	URL = {https://doi.org/10.1073/pnas.130247511},
	DOI = {10.1073/pnas.1302475110}
}

@article{fink:AJP:2022,
    author = {Catheline, Stefan and Delattre, Victor and Laloy-Borgna, Gabrielle and Faure, Fréderic and Fink, Mathias},
    title = "{Gravitational lens effect revisited through membrane waves}",
    journal = {Am. J. Phys.},
    volume = {90},
    number = {1},
    pages = {47-50},
    year = {2022},
    month = {01},
    issn = {0002-9505},
    doi = {10.1119/10.0006612},
    url = {https://doi.org/10.1119/10.0006612},
    eprint = {https://pubs.aip.org/aapt/ajp/article-pdf/90/1/47/16184728/47\_1\_online.pdf},
}

@article{ohanian:AJP:1987,
    author = {Ohanian, Hans C.},
    title = "{The black hole as a gravitational ``lens''}",
    journal = {Am. J. Phys.},
    volume = {55},
    number = {5},
    pages = {428-432},
    year = {1987},
    month = {05},
    issn = {0002-9505},
    doi = {10.1119/1.15126},
    url = {https://doi.org/10.1119/1.15126},
    eprint = {https://pubs.aip.org/aapt/ajp/article-pdf/55/5/428/11852596/428\_1\_online.pdf},
}

@article{selmke:AJP:2021,
    author = {Selmke, Markus},
    title = "{An optical N-body gravitational lens analogy}",
    journal = {Am. J. Phys.},
    volume = {89},
    number = {1},
    pages = {11-20},
    year = {2021},
    month = {01},
    issn = {0002-9505},
    doi = {10.1119/10.0002117},
    url = {https://doi.org/10.1119/10.0002117},
    eprint = {https://pubs.aip.org/aapt/ajp/article-pdf/89/1/11/12936275/11\_1\_online.pdf},
}

@article{liebes:AJP:1969,
    author = {Liebes, Sidney, Jr.},
    title = "{Gravitational Lens Simulator}",
    journal = {Am. J. Phys.},
    volume = {37},
    number = {1},
    pages = {103-104},
    year = {1969},
    month = {01},
    issn = {0002-9505},
    doi = {10.1119/1.1975345},
    url = {https://doi.org/10.1119/1.1975345},
    eprint = {https://pubs.aip.org/aapt/ajp/article-pdf/37/1/103/10113862/103\_1\_online.pdf},
}

@article{nandor:AJP:1996,
    author = {Nandor, M. J. and Helliwell, T. M.},
    title = "{Fermat's principle and multiple imaging by gravitational lenses}",
    journal = {Am. J. Phys.},
    volume = {64},
    number = {1},
    pages = {45-49},
    year = {1996},
    month = {01},
    issn = {0002-9505},
    doi = {10.1119/1.18291},
    url = {https://doi.org/10.1119/1.18291},
    eprint = {https://pubs.aip.org/aapt/ajp/article-pdf/64/1/45/11828268/45\_1\_online.pdf},
}

@article{turrell:AJP:2023,
    author = {George, Brett C. and Kontou, Eleni-Alexandra and Przewoznik, Patrycja and Turrell, Eleanor},
    title = "{An exploration of circumbinary systems using gravitational microlensing}",
    journal = {Am. J. Phys.},
    volume = {91},
    number = {3},
    pages = {182-192},
    year = {2023},
    month = {03},
    issn = {0002-9505},
    doi = {10.1119/5.0088604},
    url = {https://doi.org/10.1119/5.0088604},
    eprint = {https://pubs.aip.org/aapt/ajp/article-pdf/91/3/182/16736587/182\_1\_online.pdf},
}

@article{alfaro:AJP:2001,
    author = {Alfaro, Francisco Frutos},
    title = "{A computer program to visualize gravitational lenses}",
    journal = {Am. J. Phys.},
    volume = {69},
    number = {2},
    pages = {218-222},
    year = {2001},
    month = {02},
    issn = {0002-9505},
    doi = {10.1119/1.1290251},
    url = {https://doi.org/10.1119/1.1290251},
    eprint = {https://pubs.aip.org/aapt/ajp/article-pdf/69/2/218/7529764/218\_1\_online.pdf},
}

@article{icke:AJP:1980,
    author = {Icke, Vincent},
    title = "{Construction of a gravitational lens}",
    journal = {Am. J. Phys.},
    volume = {48},
    number = {10},
    pages = {883-886},
    year = {1980},
    month = {10},
    issn = {0002-9505},
    doi = {10.1119/1.12284},
    url = {https://doi.org/10.1119/1.12284},
    eprint = {https://pubs.aip.org/aapt/ajp/article-pdf/48/10/883/11397371/883\_1\_online.pdf},
}

@article{higbie:AJP:1981,
    author = {Higbie, J.},
    title = "{Gravitational lens}",
    journal = {Am. J. Phys.},
    volume = {49},
    number = {7},
    pages = {652-655},
    year = {1981},
    month = {07},
    issn = {0002-9505},
    doi = {10.1119/1.12440},
    url = {https://doi.org/10.1119/1.12440},
    eprint = {https://pubs.aip.org/aapt/ajp/article-pdf/49/7/652/12126808/652\_1\_online.pdf},
}

@article{drosdoff:AJP:2005,
    author = {Drosdoff, D. and Widom, A.},
    title = "{Snell's law from an elementary particle viewpoint}",
    journal = {Am. J. Phys.},
    volume = {73},
    number = {10},
    pages = {973-975},
    year = {2005},
    month = {10},
    issn = {0002-9505},
    doi = {10.1119/1.2000974},
    url = {https://doi.org/10.1119/1.2000974},
    eprint = {https://pubs.aip.org/aapt/ajp/article-pdf/73/10/973/12842782/973\_1\_online.pdf},
}

@article{ros:PhysEd:2008,
doi = {10.1088/0031-9120/43/5/007},
url = {https://dx.doi.org/10.1088/0031-9120/43/5/007},
year = {2008},
month = {sep},
publisher = {},
volume = {43},
number = {5},
pages = {506},
author = {Rosa M Ros},
title = {Gravitational lenses in the classroom},
journal = {Physics Education},
}

@Article{sanz:ENTROPY:2023,
AUTHOR = {A. S. Sanz},
TITLE = {Young's experiment with entangled bipartite systems: The role of underlying quantum velocity fields},
JOURNAL = {Entropy},
VOLUME = {25},
YEAR = {2023},
NUMBER = {7},
ARTICLE-NUMBER = {1077},
URL = {https://www.mdpi.com/1099-4300/25/7/1077},
PubMedID = {37510022},
ISSN = {1099-4300},
DOI = {10.3390/e25071077},
}

@article{plenio:RMP:2017,
	title = {Colloquium: Quantum coherence as a resource},
	author = {Streltsov, Alexander and Adesso, Gerardo and Plenio, Martin B.},
	journal = {Rev. Mod. Phys.},
	volume = {89},
	issue = {4},
	pages = {041003},
	numpages = {34},
	year = {2017},
	month = {Oct},
	publisher = {American Physical Society},
	doi = {10.1103/RevModPhys.89.041003},
	url = {https://link.aps.org/doi/10.1103/RevModPhys.89.041003}
}

@incollection{patorski:ProgOpt:1989,
	title = {I The self-imaging phenomenon and its applications},
	editor = {E. Wolf},
	series = {Progress in Optics},
	publisher = {Elsevier},
	volume = {27},
	pages = {1-108},
	year = {1989},
	issn = {0079-6638},
	doi = {https://doi.org/10.1016/S0079-6638(08)70084-2},
	url = {https://www.sciencedirect.com/science/article/pii/S0079663808700842},
	author = {Krzysztof Patorski},
}

@article{berry:JModOpt:1996,
	author = {M. V. Berry and S. Klein},
	title = {Integer, fractional and fractal {talbot} effects},
	journal = {J. Mod. Opt.},
	volume = {43},
	number = {10},
	pages = {2139--2164},
	year = {1996},
	publisher = {Taylor \& Francis},
	doi = {10.1080/09500349608232876},
	URL = {https://doi.org/10.1080/09500349608232876},
	eprint = {https://doi.org/10.1080/09500349608232876},
}

@article{winthrop:JOSA:1965,
	author = {John T. Winthrop and C. R. Worthington},
	journal = {J. Opt. Soc. Am.},
	number = {4},
	pages = {373--381},
	publisher = {Optica Publishing Group},
	title = {Theory of Fresnel Images. I. Plane Periodic Objects in Monochromatic Light$\ast$},
	volume = {55},
	month = {Apr},
	year = {1965},
	url = {https://opg.optica.org/abstract.cfm?URI=josa-55-4-373},
	doi = {10.1364/JOSA.55.000373},
}

@article{xiao:AdvOptPhoton:2013,
	author = {Jianming Wen and Yong Zhang and Min Xiao},
	journal = {Adv. Opt. Photon.},
	number = {1},
	pages = {83--130},
	publisher = {Optica Publishing Group},
	title = {The {talbot} effect: recent advances in classical optics, nonlinear optics, and quantum optics},
	volume = {5},
	month = {Mar},
	year = {2013},
	url = {https://opg.optica.org/aop/abstract.cfm?URI=aop-5-1-83},
	doi = {10.1364/AOP.5.000083},
}

@article{manjavacas:OL:2017,
	author = {L. Zundel and R. Mart\'{\i}nez-Herrero and A. Manjavacas},
	journal = {Opt. Lett.},
	number = {20},
	pages = {4143--4146},
	publisher = {Optica Publishing Group},
	title = {Flat top surface plasmon polariton beams},
	volume = {42},
	month = {Oct},
	year = {2017},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-42-20-4143},
	doi = {10.1364/OL.42.004143},
}

@article{manjavacas:PRA:2016,
	title = {Basis for paraxial surface-plasmon-polariton packets},
	author = {Mart{\'\i}nez-Herrero, Rosario and Manjavacas, Alejandro},
	journal = {Phys. Rev. A},
	volume = {94},
	issue = {6},
	pages = {063829},
	numpages = {5},
	year = {2016},
	month = {Dec},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.94.063829},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.94.063829}
}

@article{christodoulides:OL:2010,
	author = {Alessandro Salandrino and Demetrios N. Christodoulides},
	journal = {Opt. Lett.},
	number = {12},
	pages = {2082--2084},
	publisher = {Optica Publishing Group},
	title = {Airy plasmon: a nondiffracting surface wave},
	volume = {35},
	month = {Jun},
	year = {2010},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-35-12-2082},
	doi = {10.1364/OL.35.002082},
}

@article{chen:OL:2023,
	author = {Yanru Chen and Zhifeng Tu and Hongcheng Hu and Junxi Zhang and Zien Feng and Ziyu Wang and Weiyi Hong and Dongmei Deng},
	journal = {Opt. Lett.},
	number = {8},
	pages = {2030--2033},
	publisher = {Optica Publishing Group},
	title = {Olver plasmon: an accelerating surface wave with various orders},
	volume = {48},
	month = {Apr},
	year = {2023},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-48-8-2030},
	doi = {10.1364/OL.487750},
}

@article{hu:ResPhys:2021,
	title = {{Pearcey} plasmon: An autofocusing surface wave},
	journal = {Res. Phys.},
	volume = {26},
	pages = {104416},
	year = {2021},
	issn = {2211-3797},
	doi = {https://doi.org/10.1016/j.rinp.2021.104416},
	url = {https://www.sciencedirect.com/science/article/pii/S2211379721005350},
	author = {Hongcheng Hu and Chuangjie Xu and Manshuo Lin and Dongmei Deng},
}

@article{minovich:PRL:2011,
	title = {Generation and Near-Field Imaging of {Airy}  Surface Plasmons},
	author = {Minovich, Alexander and Klein, Angela E. and Janunts, Norik and Pertsch, Thomas and Neshev, Dragomir N. and Kivshar, Yuri S.},
	journal = {Phys. Rev. Lett.},
	volume = {107},
	issue = {11},
	pages = {116802},
	numpages = {4},
	year = {2011},
	month = {Sep},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.107.116802},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.107.116802}
}

@BOOK{raether-bk,
  AUTHOR     = {H. Raether},
  TITLE      = {Surface Plasmons on Smooth and Rough Surfaces and on Gratings},
  PUBLISHER  = {Springer-Verlag},
  YEAR       = {1988},
  address    = {Berlin},
}

@article{razueva:SIGMA:2018,
	title = {Higher derivatives of {Airy}  functions and of their products},
	author = {E. G. Abramochikin and E. V. Razueva},
	journal = {SIGMA},
	volume = {14},
	pages = {042},
	numpages = {26},
	year = {2018},
	publisher = {American Physical Society},
	doi = {10.3842/SIGMA.2018.042},
	url = {https://www.emis.de/journals/SIGMA/2018/042/}
}

@article{brychkov:ITSF:2012,
	author = {Yu. A. Brychkov},
	title = {On higher derivatives of the Bessel and related functions},
	journal = {Integral Transforms Spec. Funct.},
	volume = {24},
	number = {8},
	pages = {607--612},
	year = {2013},
	publisher = {Taylor \& Francis},
	doi = {10.1080/10652469.2012.726826},
	URL = {https://doi.org/10.1080/10652469.2012.726826},
}

@misc{laurenzi:arxiv:2017,
	title={Integrals containing the logarithm of the {Airy}  function $Ai'(x)$}, 
	author={Bernard J. Laurenzi},
	year={2017},
	eprint={1712.10332v1},
	archivePrefix={arXiv},
	primaryClass={math.CA},
	url={https://arxiv.org/abs/1712.10332},
    doi={10.48550/arXiv.1712.10332},
}

@article{Wu:AdvMat:2014,
author = {Wu, Yanwen and Zhang, Chengdong and Estakhri, N. Mohammadi and Zhao, Yang and Kim, Jisun and Zhang, Matt and Liu, Xing-Xiang and Pribil, Greg K. and Alù, Andrea and Shih, Chih-Kang and Li, Xiaoqin},
title = {Intrinsic Optical Properties and Enhanced Plasmonic Response of Epitaxial Silver},
journal = {Adv. Mater.},
volume = {26},
number = {35},
pages = {6106-6110},
doi = {10.1002/adma.201401474},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/adma.201401474},
year = {2014},
}

@article{Wu:AdvMat:2014corr,
author = {Wu, Yanwen and Zhang, Chengdong and Estakhri, N. Mohammadi and Zhao, Yang and Kim, Jisun and Zhang, Matt and Liu, Xing-Xiang and Pribil, Greg K. and Alù, Andrea and Shih, Chih-Kang and Li, Xiaoqin},
title = {Intrinsic Optical Properties and Enhanced Plasmonic Response of Epitaxial Silver},
journal = {Adv. Mater.},
volume = {26},
number = {35},
pages = {6106-6110},
doi = {10.1002/adma.201401474},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/adma.201401474},
year = {2014}
}

@article{Archambault:PRB:2009,
	title = {Surface plasmon Fourier optics},
	author = {Archambault, A. and Teperik, T. V. and Marquier, F. and Greffet, J. J.},
	journal = {Phys. Rev. B},
	volume = {79},
	issue = {19},
	pages = {195414},
	numpages = {8},
	year = {2009},
	month = {May},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevB.79.195414},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.79.195414}
}

@article{teperik:OE:2009,
	author = {T. V. Teperik and A. Archambault and F. Marquier and J. J. Greffet},
	journal = {Opt. Express},
	number = {20},
	pages = {17483--17490},
	publisher = {Optica Publishing Group},
	title = {Huygens-Fresnel principle for surface plasmons},
	volume = {17},
	month = {Sep},
	year = {2009},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-17-20-17483},
	doi = {10.1364/OE.17.017483},
}

@article{manjavacas:OE:2015,
	author = {Rosario Mart{\'\i}nez-Herrero and Aitor Garc{\'\i}a-Ruiz and Alejandro Manjavacas},
	journal = {Opt. Express},
	number = {22},
	pages = {28574--28583},
	publisher = {Optica Publishing Group},
	title = {Parametric characterization of surface plasmon polaritons at a lossy interface},
	volume = {23},
	month = {Nov},
	year = {2015},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-23-22-28574},
	doi = {10.1364/OE.23.028574},
}

@article{MartinezHerrero:OE:2008,
	author = {R. Mart\'{i}nez-Herrero and P. M. Mej\'{i}as and A. Carnicer},
	journal = {Opt. Express},
	number = {5},
	pages = {2845--2858},
	publisher = {Optica Publishing Group},
	title = {Evanescent field of vectorial highly non-paraxial beams},
	volume = {16},
	month = {Mar},
	year = {2008},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-16-5-2845},
	doi = {10.1364/OE.16.002845},
}

@article{friberg:OL:2013,
	author = {Andreas Norrman and Tero Set\"{a}l\"{a} and Ari T. Friberg},
	journal = {Opt. Lett.},
	number = {7},
	pages = {1119--1121},
	publisher = {Optica Publishing Group},
	title = {Exact surface-plasmon polariton solutions at a lossy interface},
	volume = {38},
	month = {Apr},
	year = {2013},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-38-7-1119},
	doi = {10.1364/OL.38.001119},
}

@article{serna:ApplOpt:1993,
author = {J. Serna and P. M. Mej\'{i}as and R. Mart\'{i}nez-Herrero},
journal = {Appl. Opt.},
number = {7},
pages = {1084--1086},
publisher = {Optica Publishing Group},
title = {Beam quality changes in Hermite--Gauss mode fields propagating through Gaussian apertures},
volume = {32},
month = {Mar},
year = {1993},
url = {https://opg.optica.org/ao/abstract.cfm?URI=ao-32-7-1084},
doi = {10.1364/AO.32.001084},
}

@inproceedings{siegman:SPIE:1993,
author = {Anthony E. Siegman},
title = {{Defining, measuring, and optimizing laser beam quality}},
volume = {1868},
booktitle = {Laser Resonators and Coherent Optics: Modeling, Technology, and Applications},
editor = {Anup Bhowmik},
organization = {International Society for Optics and Photonics},
publisher = {SPIE},
pages = {2--12},
year = {1993},
doi = {10.1117/12.150601},
URL = {https://doi.org/10.1117/12.150601}
}

@article{ruan:OL:2024,
author = {Zhang Ruan and Junxi Zhang and Yanru Chen and Zien Feng and Yanghong Li and Hailong Wu and Shibin Wen and Guanghui Wang and Dongmei Deng},
journal = {Opt. Lett.},
number = {16},
pages = {4673--4676},
publisher = {Optica Publishing Group},
title = {{Pearcey Talbot}-like plasmon: a plasmonic bottle array generation scheme},
volume = {49},
month = {Aug},
year = {2024},
url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-49-16-4673},
doi = {10.1364/OL.531141},
}

@article{minovich:LasPhotRev:2014,
author = {Minovich, Alexander E. and Klein, Angela E. and Neshev, Dragomir N. and Pertsch, Thomas and Kivshar, Yuri S. and Christodoulides, Demetrios N.},
title = {{Airy}  plasmons: non-diffracting optical surface waves},
journal = {Laser Photonics Rev.},
volume = {8},
number = {2},
pages = {221-232},
doi = {https://doi.org/10.1002/lpor.201300055},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/lpor.201300055},
year = {2014}
}

@article{li:PRL:2011,
  title = {Plasmonic {Airy}  Beam Generated by In-Plane Diffraction},
  author = {Li, L. and Li, T. and Wang, S. M. and Zhang, C. and Zhu, S. N.},
  journal = {Phys. Rev. Lett.},
  volume = {107},
  issue = {12},
  pages = {126804},
  numpages = {4},
  year = {2011},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.107.126804},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.107.126804}
}

@article{arie:LasPhotRev:2016,
author = {Epstein, Itai and Tsur, Yuval and Arie, Ady},
title = {Surface-plasmon wavefront and spectral shaping by near-field holography},
journal = {Laser Photonics Rev.},
volume = {10},
number = {3},
pages = {360-381},
doi = {https://doi.org/10.1002/lpor.201500242},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/lpor.201500242},
year = {2016}
}

@article{zhang:OL:2011,
author = {Peng Zhang and Sheng Wang and Yongmin Liu and Xiaobo Yin and Changgui Lu and Zhigang Chen and Xiang Zhang},
journal = {Opt. Lett.},
number = {16},
pages = {3191--3193},
publisher = {Optica Publishing Group},
title = {Plasmonic {Airy}  beams with dynamically controlled trajectories},
volume = {36},
month = {Aug},
year = {2011},
url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-36-16-3191},
doi = {10.1364/OL.36.003191},
}

@article{arie:ACSPhoton:2017,
author = {Tsur, Yuval and Epstein, Itai and Remez, Roei and Arie, Ady},
title = {Wavefront Shaping of Plasmonic Beams by Selective Coupling},
journal = {ACS Photonics},
volume = {4},
number = {6},
pages = {1339--1343},
doi = {10.1021/acsphotonics.7b00346},
url = { https://doi.org/10.1021/acsphotonics.7b00346},
year = {2017}
}

@article{Zhang:JPhysD:2012,
doi = {10.1088/0022-3727/45/11/113001},
url = {https://dx.doi.org/10.1088/0022-3727/45/11/113001},
year = {2012},
month = {feb},
publisher = {IOP Publishing},
volume = {45},
number = {11},
pages = {113001},
author = {Junxi Zhang and Lide Zhang and Wei Xu},
title = {Surface plasmon polaritons: physics and applications},
journal = {J. Phys. D: Appl. Phys.},
}

@article{sanz:OE:2024,
	author = {A. S. Sanz and R. Mart\'{i}nez-Herrero},
	journal = {Opt. Express},
	keywords = {{Airy}  beams; Beam propagation methods; Fourier transforms; Light beams; Refractive index; Structured light},
	number = {4},
	pages = {5592--5606},
	publisher = {Optica Publishing Group},
	title = {Exploring the dynamics of finite-energy {Airy}  beams: a trajectory analysis perspective},
	volume = {32},
	month = {Feb},
	year = {2024},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-32-4-5592},
	doi = {10.1364/OE.507577},
}

@article{johnson:PRB:1972,
	title = {Optical Constants of the Noble Metals},
	author = {Johnson, P. B. and Christy, R. W.},
	journal = {Phys. Rev. B},
	volume = {6},
	issue = {12},
	pages = {4370--4379},
	numpages = {0},
	year = {1972},
	month = {Dec},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevB.6.4370},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.6.4370}
}

@article{ferrera:PhysRevMater:2019,
	title = {Temperature-dependent permittivity of silver and implications for thermoplasmonics},
	author = {Ferrera, Marzia and Magnozzi, Michele and Bisio, Francesco and Canepa, Maurizio},
	journal = {Phys. Rev. Mater.},
	volume = {3},
	issue = {10},
	pages = {105201},
	numpages = {6},
	year = {2019},
	month = {Oct},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevMaterials.3.105201},
	url = {https://link.aps.org/doi/10.1103/PhysRevMaterials.3.105201}
}

@article{jiang:SciRep:2016,
	title = {Realistic silver optical constants for plasmonics},
	author = {Jiang, Yajie and Pillai, Supriya and Green, Martin A.},
	journal = {Sci. Rep.},
	volume = {6},
	issue = {1},
	pages = {30605},
	numpages = {6},
	year = {2016},
	publisher = {American Physical Society},
	doi = {10.1038/srep30605},
	url = {https://doi.org/10.1038/srep30605}
}

@article{yang:PRB:2015,
	title = {Optical dielectric function of silver},
	author = {Yang, Honghua U. and D'Archangel, Jeffrey and Sundheimer, Michael L. and Tucker, Eric and Boreman, Glenn D. and Raschke, Markus B.},
	journal = {Phys. Rev. B},
	volume = {91},
	issue = {23},
	pages = {235137},
	numpages = {11},
	year = {2015},
	month = {Jun},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevB.91.235137},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.91.235137}
}

@article{mcpeak:ACSPhoton:2015,
	title = {Plasmonic films can easily be better: rules and recipes},
	author = {McPeak, Kevin M. and Jayanti, Sriharsha V. and Kress, Stephan J. P. and Meyer, Stefan and Iotti, Stelio and Rossinelli, Aurelio and Norris, David J.},
	journal = {ACS Photonics},
	volume = {2},
	issue = {3},
	pages = {326--333},
	year = {2015},
	doi = {10.1021/ph5004237},
	url = {https://doi.org/10.1021/ph5004237}
}

@article{zhou:ProgQuantumElectron:2019,
	title = {Quantum plasmonics get applied},
	journal = {Prog. Quantum Electron.},
	volume = {65},
	pages = {1-20},
	year = {2019},
	issn = {0079-6727},
	doi = {https://doi.org/10.1016/j.pquantelec.2019.04.002},
	url = {https://www.sciencedirect.com/science/article/pii/S0079672719300084},
	author = {Zhang-Kai Zhou and Jingfeng Liu and Yanjun Bao and Lin Wu and Ching Eng Png and Xue-Hua Wang and Cheng-Wei Qiu},
}

@article{maradudin:PhysRep:2005,
	title = {Nano-optics of surface plasmon polaritons},
	journal = {Phys. Rep.},
	volume = {408},
	number = {3},
	pages = {131-314},
	year = {2005},
	issn = {0370-1573},
	doi = {https://doi.org/10.1016/j.physrep.2004.11.001},
	url = {https://www.sciencedirect.com/science/article/pii/S0370157304004600},
	author = {Anatoly V. Zayats and Igor I. Smolyaninov and Alexei A. Maradudin},
}

@ARTICLE{xiangang:IEEEPhotJ:2012,
	author={Luo, Xiangang and Yan, Lianshan},
	journal={IEEE Photonics J.}, 
	title={Surface Plasmon Polaritons and Its Applications}, 
	year={2012},
	volume={4},
	number={2},
	pages={590-595},
	doi={10.1109/JPHOT.2012.2189436},
}

@article{anwar:DigCommunNet:2018,
	title = {Recent advancements in surface plasmon polaritons-plasmonics in subwavelength structures in microwave and terahertz regimes},
	journal = {Digit. Commun. Netw.},
	volume = {4},
	number = {4},
	pages = {244-257},
	year = {2018},
	issn = {2352-8648},
	doi = {https://doi.org/10.1016/j.dcan.2017.08.004},
	url = {https://www.sciencedirect.com/science/article/pii/S2352864817301992},
	author = {Rana Sadaf Anwar and Huansheng Ning and Lingfeng Mao},
}

@article{echenique:RepProgPhys:2006,
	doi = {10.1088/0034-4885/70/1/R01},
	url = {https://dx.doi.org/10.1088/0034-4885/70/1/R01},
	year = {2006},
	month = {dec},
	publisher = {},
	volume = {70},
	number = {1},
	pages = {1},
	author = {J M Pitarke and V M Silkin and E V Chulkov and P M Echenique},
	title = {Theory of surface plasmons and surface-plasmon polaritons},
	journal = {Rep. Prog. Phys.},
}

@article{Liu:OE:2019,
	author = {Wanguo Liu and Hai Hu and Fenghua Liu and Hua Zhao},
	journal = {Opt. Express},
	number = {4},
	pages = {4714--4726},
	publisher = {Optica Publishing Group},
	title = {Manipulating light trace in a gradient-refractive-index medium: a Lagrangian optics method},
	volume = {27},
	month = {Feb},
	year = {2019},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-27-4-4714},
	doi = {10.1364/OE.27.004714},
}

@BOOK{raju-bk,
	AUTHOR     = {Thokala Soloman Raju},
	TITLE      = {Controllable Nonlinear Waves in Graded-Index Waveguides (GRIN)},
	PUBLISHER  = {Springer},
	YEAR       = {2024},
	address    = {Singapore},
	doi = {https://doi.org/10.1007/978-981-97-0441-5},
    isbn = {978-981-97-0440-8},
}

@article{kneipp:JPCM:2002,
	doi = {10.1088/0953-8984/14/18/202},
	url = {https://dx.doi.org/10.1088/0953-8984/14/18/202},
	year = {2002},
	month = {apr},
	volume = {14},
	number = {18},
	pages = {R597},
	author = {Katrin Kneipp and  Harald Kneipp and  Irving Itzkan and  Ramachandra R Dasari and  Michael S Feld},
	title = {Surface-enhanced Raman scattering and biophysics},
	journal = {J. Phys.: Condens. Matter},
}

@article{saouli:MatToday:2020,
	title = {Simulation of spectral response of SPR multilayers nanostructures detector intended for biomedical application},
	journal = {Mater. Today: Proc.},
	volume = {31},
	pages = {S24-S27},
	year = {2020},
	issn = {2214-7853},
	doi = {10.1016/j.matpr.2020.05.278},
	url = {https://www.sciencedirect.com/science/article/pii/S2214785320338396},
	author = {Abdelali Saouli and Chouaib Saouli},
}

@article{altewischer:Naure:2002,
	title = {Plasmon-assisted transmission of entangled photons},
	journal = {Nature},
	volume = {418},
	number = {6895},
	pages = {3094-306},
	year = {2002},
	issn = {2214-7853},
	doi = {10.1038/nature00869},
	url = {https://doi.org/10.1038/nature00869},
	author = {E. Altewischer and M. P. van Exter and J. P. Woerdman},
}

@article{gric:JOpt:2017,
	doi = {10.1088/2040-8986/aa75fd},
	url = {https://dx.doi.org/10.1088/2040-8986/aa75fd},
	year = {2017},
	month = {jul},
	publisher = {IOP Publishing},
	volume = {19},
	number = {8},
	pages = {085101},
	author = {Tatjana Gric and Ortwin Hess},
	title = {Surface plasmon polaritons at the interface of two nanowire metamaterials},
	journal = {J. Opt.},
}

@article{gric:JIMTW:2018,
	doi = {10.1007/s10762-018-0516-0},
	url = {https://doi.org/10.1007/s10762-018-0516-0},
	year = {2018},
	volume = {39},
	number = {10},
	pages = {1028--1038},
	author = {Tatjana Gric and and Andrei Gorodetsky and Aleksej Trofimov and Edik Rafailov},
	title = {Tunable Plasmonic Properties and Absorption Enhancement in Terahertz Photoconductive Antenna Based on Optimized Plasmonic Nanostructures},
	journal = {J. Infrared Millim. Terahertz Waves},
}

@article{dholakia:NatPhoton:2008,
	doi = {10.1038/nphoton.2008.201},
	url = {https://doi.org/10.1038/nphoton.2008.201},
	year = {2008},
	volume = {2},
	number = {11},
	pages = {675--678},
	author = {Baumgartl, J\"org and Mazilu, Michael and Dholakia, Kishan},
	title = {Optically mediated particle clearing using {Airy}  wavepackets},
	journal = {Nat. Photonics},
}

@article{dholakia:NatMethods:2014,
	doi = {10.1038/nmeth.2922},
	url = {https://doi.org/10.1038/nmeth.2922},
	year = {2014},
	volume = {11},
	number = {5},
	pages = {541--544},
	author = {Vettenburg, Tom and Dalgarno, Heather I. C. and Nylk, Jonathan and Coll-Llad\'o, Clara and Ferrier, David E K and \v{C}i\v{z}m\'ar, Tom\'a\v{s} and Gunn-Moore, Frank J. and Dholakia, Kishan},
	title = {Light-sheet microscopy using an {Airy}  beam},
	journal = {Nat. Methods},
}

@article{,
 author    = {},
 journal   = {},
 title     = {},
 volume    = {},
 pages     = {},
 year      = {},
 doi       = {},
 url       = {},
}

@BOOK{,
  AUTHOR     = {},
  TITLE      = {},
  PUBLISHER  = {},
  YEAR       = {},
  address    = {},
}


@article{doi:10.1021/nl802044t,
author = {Manjavacas, A. and García de Abajo, F. J.},
title = {Robust Plasmon Waveguides in Strongly Interacting Nanowire Arrays},
journal = {Nano Lett.},
volume = {9},
number = {4},
pages = {1285-1289},
year = {2009},
doi = {10.1021/nl802044t}

}
%note ={PMID: 18672946},
%URL = {https://doi.org/10.1021/nl802044t},
%eprint = {https://doi.org/10.1021/nl802044t}




@article{Manjavacas:09,
author = {A. Manjavacas and F. J. Garc\'{i}a de Abajo},
journal = {Opt. Express},
keywords = {Waveguides; Surface plasmons; Plasmonics; Attenuation; Elastic scattering; Multiple scattering; Nanowires; Surface plasmon polaritons; Surface plasmons},
number = {22},
pages = {19401--19413},
publisher = {Optica Publishing Group},
title = {Coupling of gap plasmons in multi-wire waveguides},
volume = {17},
month = {Oct},
year = {2009},
url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-17-22-19401},
doi = {10.1364/OE.17.019401},
abstract = {We investigate the coupling of gap plasmons in various configurations of neighboring metallic nanowires. Starting with the basic element defining a gap plasmon, consisting of two neighboring silver wires, we study the energy splitting and symmetry properties of hybridized plasmons resulting from the interaction of two wire pairs. The system is shown to display non-avoided crossings of hybridized modes, and it evolves at short distances towards a degenerate system consisting of four wires arranged in a square, where two new gap plasmons emerge from redshifted higher-energy modes. The gap modes of three neighboring wires are also described in a continuous transition from a coplanar configuration to an equilateral triangle arrangement. The interaction between wire pairs is shown to be weak enough to prevent efficient transfer of plasmon signal from a pair to the other one, which is beneficial to avoid crosstalking, but not to produce waveguide couplers. The coupling is significantly increased by placing a wire of rectangular cross section in between the wire pairs, thus allowing us to achieve large plasmon-signal transfers within propagation distances below the attenuation length. Our results can find application in the design of signal-processing devices based upon gap plasmons.},
}



@article{kocsis:Science:2011,
 author  = {S. Kocsis and B. Braverman and S. Ravets and M. J. Stevens and R. P. Mirin and L. K. Shalm and A. M. Steinberg},
 journal = {Science},
 title   = {Observing the average trajectories of single photons in a two-slit interferometer},
 volume  = {332},
 pages   = {1170-1173},
 year    = {2011},
 doi     = {10.1126/science.1202218},
}

@article{coalson:JLightTech:1994,
 author               = {R. D. Coalson and D. K. Pant and A. Ali and D. W. Langer},
 journal              = {J. Light. Tech.},
 pages                = {1015-1022},
 title                = {Computing the eigenmodes of lossy field-induced optical waveguides},
 volume               = {12},
 year                 = {1994},
}

@article{herrmann:AJP:2002,
 author               = {T. W\"unscher and H. Hauptmann and F. Herrmann},
 journal              = {Am. J. Phys.},
 pages                = {599-606},
 title                = {Which way does the light go?},
 volume               = {70},
 year                 = {2002},
}

@article{jcm:wg-lanz:03,
 author               = {J. Campos-Mart{\'\i}nez and Rob D. Coalson},
 journal              = {Appl. Opt.},
 journal-iso          = {Appl. Optics},
 keywords-plus        = {OPTICAL WAVE-GUIDES; SCHRODINGER-EQUATION; PROPAGATION; DESIGN},
 language             = {English},
 month                = {MAR 20},
 number               = {9},
 number-of-cited-refe = {20},
 pages                = {1732-1742},
 publisher            = {OPTICAL SOC AMER},
 subject-category     = {Optics},
 times-cited          = {0},
 title                = {The wide-angle equation and its solution through the short-time iterative Lanczos method},
 type                 = {Article},
 unique-id            = {ISI:000181708400020},
 volume               = {42},
 year                 = {2003},
}

@article{mataloni:PRL:2010,
 author               = {L. Sansoni and F. Sciarrino and G. Vallone and P. Mataloni and A. Crespi and R. Ramponi and R. Osellame},
 journal              = {Phys. Rev. Lett.},
 pages                = {200503(1-4)},
 title                = {Polarization entangled state measurement on a chip},
 volume               = {105},
 year                 = {2010},
}

@article{pepe:AppOpt:1999,
 author               = {D. K. Pant and R. D. Coalson and M. I. Hern{\'a}ndez and J. Campos-Mart{\'\i}nez},
 journal              = {Appl. Opt.},
 pages                = {3917-3923},
 title                = {Optimal control theory for optical waveguide design: Application to $Y$-branch structures},
 volume               = {38},
 year                 = {1999},
}

@article{pepe:AppOpt:2003,
 author               = {J. Campos-Mart{\'\i}nez and R. D. Coalson},
 journal              = {Appl. Opt.},
 pages                = {1732-1742},
 title                = {The wide-angle equation and its solution through the short-time iterative Lanczos method},
 volume               = {42},
 year                 = {2003},
}

@article{pepe:JLightTech:1998,
 author               = {D. K. Pant and R. D. Coalson and M. I. Hern{\'a}ndez and J. Campos-Mart{\'\i}nez},
 journal              = {J. Light. Tech.},
 pages                = {292-300},
 title                = {Optimal control theory for the design of optical waveguides},
 volume               = {16},
 year                 = {1998},
}

@article{politi:science:2008,
 author               = {A. Politi and M. J. Cryan and J. G. Rarity and S. Yu and J. L. O'Brien},
 journal              = {Science},
 pages                = {646-649},
 title                = {Silica-on-silicon waveguide quantum circuits},
 volume               = {320},
 year                 = {2008},
}

@article{sanz:AnnPhysPhoton:2010,
 author               = {A. S. Sanz and M. Davidovi\'c and M. Bo\v{z}i\'c and S. Miret-Art\'es},
 journal              = {Ann. Phys.},
 pages                = {763-784},
 title                = {Understanding interference experiments with polarized light through photon trajectories},
 volume               = {325},
 year                 = {2010},
 doi                  = {10.1016/j.aop.2009.12.005},
 url                  = {https://doi.org/10.1016/j.aop.2009.12.005},
}

@article{sanz:JCP-Talbot:2007,
 author               = {A. S. Sanz and S. Miret-Art\'es},
 journal              = {J. Chem. Phys.},
 pages                = {234106(1-11)},
 title                = {A causal look into the quantum {talbot} effect},
 volume               = {126},
 year                 = {2007},
 doi                  = {10.1063/1.2741555},
}

@article{sanz:JPA:2008,
	doi = {10.1088/1751-8113/41/43/435303},
	url = {https://doi.org/10.1088/1751-8113/41/43/435303},
	year = {2008},
	month = {sep},
	publisher = {{IOP} Publishing},
	volume = {41},
	number = {43},
	pages = {435303},
	author = {A S Sanz and S Miret-Art{\'{e}}s},
	title = {A trajectory-based understanding of quantum interference},
	journal = {J. Phys. A: Math. Theor.}
}

@article{sanz:JRLR:2010,
 author               = {M. Bo\v{z}i\'c and M. Davidovi\'c and T. L. Dimitrova and S. Miret-Art\'es and A. S. Sanz and A. Weis},
 journal              = {J. Russ. Laser Res.},
 pages                = {117-128},
 title                = {Generalized Arago-Fresnel laws: The EME-flow-line description},
 volume               = {31},
 year                 = {2010},
}

@article{sanz:PhysScrPhoton:2009,
 author               = {M. Davidovi\'c and A. S. Sanz and D. Arsenovi\'c and M. Bo\v{z}i\'c and S. Miret-Art\'es},
 journal              = {Phys. Scr.},
 pages                = {014009(1-5)},
 title                = {Electromagnetic energy flow lines as possible paths of photons},
 volume               = {T135},
 year                 = {2009},
}

@article{parker:AJP:1971,
 author               = {S. Parker},
 journal              = {Am. J. Phys.},
 pages                = {420-424},
 title                = {A single-photon double-slit interference experiment},
 volume               = {39},
 year                 = {1971},
}

@article{parker:AJP:1972,
 author               = {S. Parker},
 journal              = {Am. J. Phys.},
 pages                = {1003-1007},
 title                = {Single-photon double-slit interference -- A demonstration},
 volume               = {49},
 year                 = {1972},
}

@article{rueckner:AJP:1996,
 author               = {W. Rueckner and P. Titcomb},
 journal              = {Am. J. Phys.},
 pages                = {184-188},
 title                = {A lecture demonstration of single photon interference},
 volume               = {64},
 year                 = {1996},
}

@article{weis:AJP:2008,
 author               = {T. L. Dimitrova and A. Weis},
 journal              = {Am. J. Phys.},
 pages                = {137-142},
 title                = {The wave-particle duality of light: A demonstration experiment},
 volume               = {76},
 year                 = {2008},
}

@article{weis:EJP:2010,
 author               = {T. L. Dimitrova and A. Weis},
 journal              = {Eur. J. Phys.},
 pages                = {625-637},
 title                = {Single photon quantum erasing: A demonstration experiment},
 volume               = {31},
 year                 = {2010},
}

@article{weis:PhysScr:2009,
 author               = {T. L. Dimitrova and A. Weis},
 journal              = {Phys. Scr.},
 pages                = {014003(1-4)},
 title                = {Lecture demonstrations of interference and quantum erasing with single photons},
 volume               = {T135},
 year                 = {2009},
}

@article{xiang:naturecomm:2011,
 author               = {J. S. Volker and Y. Ziliang and F. Rupert and W. Yuan and B. Guy and Y. Xiaobo and Z. Xiang},
 journal              = {Nat. Commun.},
 pages                = {331(1-5)},
 title                = {Experimental demonstration of low-loss optical waveguiding at deep sub-wavelength scales},
 volume               = {2},
 year                 = {2011},
}

@article{banerjee-josaa:89,
 author   = {S. Banerjee and A. Sharma},
 journal  = {J. Opt. Soc. Am. A},
 pages    = {1884-1894},
 title    = {Propagation characteristic of optical waveguiding structures by direct solution of the Helmholtz equation for total fields},
 volume   = {6},
 year     = {1989},
}

@article{scarmozzino-rev:00,
 author    = {R. Scarmozzino and A. Gopinath and R. Pregla and S. Herlfert },
 journal   = {J. Opt. Soc. Am. A},
 pages     = {150-162},
 title     = {Numerical techniques for modeling guided-wave photonic devices},
 volume    = {6},
 year      = {2000},
}

@article{min-fiber:97,
 author    = {D.-S. Min and D. W. Langer and D. K. Pant and R. D. Coalson},
 journal   = {Fiber Integr. Opt.},
 pages     = {331-342},
 title     = {Numerical techniques for modeling guided-wave photonic devices},
 volume    = {16},
 year      = {1997},
}

@article{feit-fleck:JCompPhys:1982,
 author    = {M. D. Feit and J. A. Fleck, Jr. and A. Steiger},
 journal   = {J. Comput. Phys.},
 title     = {Solution of the Schr\"odinger equation by a spectral method},
 volume = {47},
 number = {3},
 pages = {412-433},
 year = {1982},
 issn = {0021-9991},
 doi = {https://doi.org/10.1016/0021-9991(82)90091-2},
 url = {https://www.sciencedirect.com/science/article/pii/0021999182900912}
}

@article{feit-fleck:JCP:1983,
 author    = {M. D. Feit and J. A. Fleck, Jr.},
 journal   = {J. Chem. Phys.},
 volume    = {78},
 title     = {Solution of the Schr\"odinger equation by a spectral method II: Vibrational energy levels of triatomic molecules},
 pages     = {301-308},
 year      = {1983},
}

@article{feit-fleck:JCP:1984,
 author    = {M. D. Feit and J. A. Fleck, Jr.},
 journal   = {J. Chem. Phys.},
 volume    = {80},
 title     = {Wave packet dynamics and chaos in the H\'enon-Heiles system},
 pages     = {2578-2584},
 year      = {1984},
}

@article{feit-fleck:ApplOpt:1978,
 author    = {M. D. Feit and J. A. Fleck, Jr.},
 journal   = {Appl. Opt.},
 number = {24},
 pages = {3990--3998},
 publisher = {Optica Publishing Group},
 title = {Light propagation in graded-index optical fibers},
 volume = {17},
 month = {Dec},
 year = {1978},
 url = {https://opg.optica.org/ao/abstract.cfm?URI=ao-17-24-3990},
 doi = {10.1364/AO.17.003990}
}

@article{feit-fleck:ApplOpt:1980-1,
 author    = {M. D. Feit and J. A. Fleck, Jr.},
 journal   = {Appl. Opt.},
 number = {7},
 pages = {1154--1164},
 publisher = {Optica Publishing Group},
 title = {Computation of mode properties in optical fiber waveguides by a propagating beam method},
 volume = {19},
 month = {Apr},
 year = {1980},
 url = {https://opg.optica.org/ao/abstract.cfm?URI=ao-19-7-1154},
 doi = {10.1364/AO.19.001154}
}

@article{feit-fleck:ApplOpt:1980-2,
 author    = {M. D. Feit and J. A. Fleck, Jr.},
 journal   = {Appl. Opt.},
 volume    = {19},
 title     = {Computation of mode eigenfunctions in graded-index optical fibers by the propagating beam method},
 pages     = {2240-2246},
 year      = {1980},
}

@article{feit-fleck:ApplOpt:1980-3,
 author    = {M. D. Feit and J. A. Fleck, Jr.},
 journal   = {Appl. Opt.},
 volume    = {19},
 title     = {Model properties and dispersion for two optical fiber-index profiles by the propagating beam method},
 pages     = {3140-3150},
 year      = {1980},
}

@BOOK{bornwolf-bk,
  AUTHOR =       {M. Born and E. Wolf},
  TITLE =        {Principles of Optics. Electromagnetic Theory of Propagation, Interference and Diffraction of Light},
  PUBLISHER =    {Cambridge University Press},
  YEAR =         {1999},
  address =      {Cambridge},
  edition =      {7th},
}

@BOOK{buchdahl-bk,
  AUTHOR =       {H. A. Buchdahl},
  TITLE =        {An Introduction to Hamiltonian Optics},
  PUBLISHER =    {Cambridge University Press},
  YEAR =         {1970},
  address =      {Cambridge},
}

@BOOK{buchdahl-bk-old,
  AUTHOR =       {H. A. Buchdahl},
  TITLE =        {An Introduction to Hamiltonian Optics},
  PUBLISHER =    {Dover},
  YEAR =         {1993},
  address =      {New York},
}

@article{glogel:JOSA:1969,
 author    = {D. Gloge and D. Marcuse},
 journal   = {J. Opt. Soc. Am.},
 title     = {Formal quantum theory of light rays},
 volume    = {59},
 pages     = {1629-1631},
 year      = {1969},
}

@article{kahn:JOSA:1983,
 author    = {W. K. Kahn and S. Yang},
 journal   = {J. Opt. Soc. Am.},
 title     = {Hamiltonian analysis of beams in an optical slab guide},
 volume    = {73},
 pages     = {684-690},
 year      = {1983},
}

@article{longhi:PRE:2003,
 author    = {S. Longhi and D. Janner and M. Marano and P. Laporta},
 journal   = {Phys. Rev. E},
 title     = {Quantum-mechanical analogy of beam propagation in waveguides with a bent axis: Dynamic-model stabilization and radiation-loss suppresion},
 volume    = {67},
 pages     = {036601(1-9)},
 year      = {2003},
}

@article{bohm:PR:1952-1,
  title = {A Suggested Interpretation of the Quantum Theory in Terms of ``Hidden'' Variables. I},
  author = {Bohm, David},
  journal = {Phys. Rev.},
  volume = {85},
  issue = {2},
  pages = {166--179},
  numpages = {0},
  year = {1952},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.85.166},
  url = {https://link.aps.org/doi/10.1103/PhysRev.85.166}
}

@article{bohm:PR:1952-2,
  title = {A Suggested Interpretation of the Quantum Theory in Terms of ``Hidden'' Variables. II},
  author = {Bohm, David},
  journal = {Phys. Rev.},
  volume = {85},
  issue = {2},
  pages = {180--193},
  numpages = {0},
  year = {1952},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.85.180},
  url = {https://link.aps.org/doi/10.1103/PhysRev.85.180}
}

@BOOK{holland-bk,
  AUTHOR =       {P. R. Holland},
  TITLE =        {The Quantum Theory of Motion},
  PUBLISHER =    {Cambridge University Press},
  YEAR =         {1993},
  address =      {Cambridge},
}

@article{madelung:ZPhys:1926,
 author    = {E. Madelung},
 journal   = {Z. Phys.},
 title     = {Quantentheorie in hydrodynamischer Form},
 volume    = {40},
 issue     = {3},
 pages     = {322--326},
 year      = {1926},
 doi = {https://doi.org/10.1007/BF01400372},
 url = {https://link.springer.com/article/10.1007/BF01400372},
}

@article{birula:PRD:1971,
 author    = {I. Bialynicki-Birula and Z. Bialynicka-Birula},
 journal   = {Phys. Rev. D},
 title     = {Magnetic monopoles in the hydrodynamic formulation of quantum mechanics},
 volume    = {3},
 pages     = {2410-2412},
 year      = {1971},
}

@BOOK{birula-bk,
  AUTHOR     = {I. Bialynicki-Birula and M. Cieplak and J. Kaminski},
  TITLE      = {Theory of Quanta},
  PUBLISHER  = {Oxford University Press},
  YEAR       = {1992},
  address    = {Oxford},
}

@article{hirsch:JCP:1974-1,
 author    = {J. O. Hirschfelder and A. C. Christoph and W. E. Palke},
 journal   = {J. Chem. Phys.},
 title     = {Quantum mechanical streamlines. I. Square potential barrier},
 volume    = {61},
 pages     = {5435-5455},
 year      = {1974},
}

@article{hirsch:JCP:1974-2,
 author    = {J. O. Hirschfelder and C. J. Goebel and L. W. Bruch},
 journal   = {J. Chem. Phys.},
 title     = {Quantized vortices around wavefunction nodes. II},
 volume    = {61},
 pages     = {5456-5459},
 year      = {1974},
}

@article{hirsch:JCP:1976-1,
 author    = {J. O. Hirschfelder and K. T. Tang},
 journal   = {J. Chem. Phys.},
 title     = {Quantum mechanical streamlines. III. Idealized reactive atom-diatomic molecule collision},
 volume    = {64},
 pages     = {760-785},
 year      = {1976},
}

@article{hirsch:JCP:1976-2,
 author    = {J. O. Hirschfelder and K. T. Tang},
 journal   = {J. Chem. Phys.},
 title     = {Quantum mechanical streamlines. IV. Collision of two sphere with square potential wells or barriers},
 volume    = {65},
 pages     = {470-486},
 year      = {1976},
}

@article{hirsch:JCP:1977,
 author    = {J. O. Hirschfelder},
 journal   = {J. Chem. Phys.},
 title     = {The angular momentum, creation, and significance of quantized vortices},
 volume    = {67},
 pages     = {5477-5483},
 year      = {1977},
}

@BOOK{wyatt-bk,
  AUTHOR     = {R. E. Wyatt},
  TITLE      = {Quantum Dynamics with Trajectories},
  PUBLISHER  = {Springer},
  YEAR       = {2005},
  address    = {New York},
}

@BOOK{duerr-bk:2009,
  AUTHOR     = {D. D\"urr and S. Teufel},
  TITLE      = {Bohmian Mechanics. The Physics and Mathematics of Quantum Theory},
  PUBLISHER  = {Springer},
  YEAR       = {2009},
  address    = {Berlin},
}

@BOOK{duerr-bk:2013,
  AUTHOR     = {D. D\"urr and S. Goldstein and N. Zangh\`{\i}},
  TITLE      = {Quantum Physics without Quantum Philosophy},
  PUBLISHER  = {Springer},
  YEAR       = {2013},
  address    = {Berlin},
}

@BOOK{press-bk-1,
  AUTHOR     = {W. H. Press and S. A. Teukolsky and W. T. Vetterling and B. P. Flannery},
  TITLE      = {Numerical Recipes in Fortran 77: The Art of Scientific Computing},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {1992},
  address    = {Cambridge},
  volume     = {1st},
  edition    = {2nd},
}

@BOOK{press-bk-2,
  AUTHOR     = {W. H. Press and s. A. Teukolsky and W. T. Vetterling and B. P. Flannery},
  TITLE      = {Numerical Recipes in Fortran 90: The Art of Parallel Scientific Computing},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {1996},
  address    = {Cambridge},
  volume     = {2nd},
  edition    = {2nd},
}

@article{sanz:JPCM:2002,
 author    = {A. S. Sanz and F. Borondo and S. Miret-Art\'es},
 journal   = {J. Phys.: Condens. Matter},
 title     = {Particle diffraction studied using quantum trajectories},
 volume    = {14},
 pages     = {6109-6145},
 year      = {2002},
 doi       = {10.1088/0953-8984/14/24/312},
}

@article{sanz:CP:2011,
 author    = {A. S. Sanz and D. L\'opez-Dur\'an and T. Gonz\'alez-Lezana},
 journal   = {Chem. Phys.},
 title     = {Investigating transition state resonances in the time domain by means of Bohmian mechanics: The F+HD reaction},
 volume    = {399},
 pages     = {151-161},
 year      = {2012},
}

@article{tien:RMP:1977,
 author    = {P. K. Tien},
 journal   = {Rev. Mod. Phys.},
 title     = {Integrated optics and new wave phenomena in optical waveguides},
 volume    = {49},
 pages     = {361-420},
 year      = {1981},
}

@article{tien:radiosci:1981,
 author    = {P. K. Tien},
 journal   = {Radio Sci.},
 title     = {Rules of refractive index and a potential well model of the optical waveguides},
 volume    = {16},
 pages     = {437-444},
 year      = {1981},
}

@article{leforestier:jcompphys:1991,
 author    = {C. Leforestier and R. H. Bisseling and C. Cerjan and M. D. Feit and R. Friesner
 and A. Guldberg and A. Hammerich and G. Jolicard and W. Karrlein and H.-D. Meyer and N. Lipkin
 and O. Roncero and R. Kosloff},
 journal   = {J. Comp. Phys.},
 title     = {A comparison of different propagation schemes for the time dependent schr\"odinger equation},
 volume    = {94},
 pages     = {59-80},
 year      = {1991},
}

@book{zurek-bk,
  author     = {W. H. Zurek and J. A. Wheeler},
  title      = {Quantum Theory of Measurement},
  publisher  = {Princeton University Press},
  year       = {1983},
  address    = {Princeton, NJ},
}

@book{belinfante-bk,
  author     = {F. J. Belinfante},
  title      = {A Survey of Hidden-Variables Theories},
  publisher  = {Pergamon},
  year       = {1973},
  address    = {New York},
}

@book{tarozzi-bk,
  author     = {},
  editor     = {G. Tarozzi and A. van der Merwe},
  title      = {Open Questions in Quantum Physics},
  publisher  = {Reidel},
  year       = {1985},
  address    = {Dordrecht},
}

@book{ballentine-bk,
  author     = {L. E. Ballentine},
  title      = {Quantum Mechanics. A Modern Development},
  publisher  = {World Scientific},
  year       = {1998},
  address    = {Singapore},
}

@article{bell:physics:1964,
 author    = {J. S. Bell},
 journal   = {Physics},
 title     = {On the Einstein-Podolsky-Rosen Paradox},
 volume    = {1},
 pages     = {195-200},
 year      = {1964},
}

@article{bell:RMP:1966,
 author    = {J. S. Bell},
 journal   = {Rev. Mod. Phys.},
 title     = {On the problem of hidden variables in quantum mechanics},
 volume    = {38},
 pages     = {447-452},
 year      = {1966},
}

@article{aspect:PRL:1981,
 author    = {A. Aspect and P. Grangier and G. Roger},
 journal   = {Phys. Rev. Lett.},
 title     = {Experimental tests of realistic local theories via Bell's theorem},
 volume    = {47},
 pages     = {460-463},
 year      = {1981},
}

@article{aspect:PRL:1982-1,
 author    = {A. Aspect and P. Grangier and G. Roger},
 journal   = {Phys. Rev. Lett.},
 title     = {Experimental realization of Einstein-Podolsky-Rosen-Bohm gedankenexperiment: A new violation of Bell's inequalities},
 volume    = {49},
 pages     = {91-94},
 year      = {1982},
}

@article{aspect:PRL:1982-2,
 author    = {A. Aspect and J. Dalibard and G. Roger},
 journal   = {Phys. Rev. Lett.},
 title     = {Experimental test of Bell's inequalities using time-varying analyzers},
 volume    = {49},
 pages     = {1804-1807},
 year      = {1982},
}

@article{goldstein:phystoday:1,
 author    = {S. Goldstein},
 journal   = {Phys. Today},
 title     = {Quantum theory without observers. Part I},
 volume    = {51},
 issue     = {3},
 pages     = {42-46},
 year      = {1998},
}

@article{goldstein:phystoday:2,
 author    = {S. Goldstein},
 journal   = {Phys. Today},
 title     = {Quantum theory without observers. Part II},
 volume    = {51},
 issue     = {4},
 pages     = {38-42},
 year      = {1998},
}

@book{chattaraj-bk,
  editor     = {P. K. Chattaraj},
  title      = {Quantum Trajectories},
  publisher  = {CRC Taylor and Francis},
  year       = {2010},
  address    = {New York},
}

@BOOK{sanz:CRC:2010,
  AUTHOR     = {A. S. Sanz and X. Gim\'enez and J. M. Bofill and S. Miret-Art\'es},
  editor     = {P. K. Chattaraj},
  title      = {Quantum Trajectories},
  CHAPTER    = {Time-dependent density functional theory from a Bohmian perspective},
  pages      = {105-119},
  publisher  = {CRC Taylor and Francis},
  year       = {2010},
  address    = {New York},
}

@book{oriols-bk,
  editor     = {X. Oriols and J. Mompart},
  title      = {Applied Bohmian Mechanics: From Nanoscale Systems to Cosmology},
  publisher  = {Pan Standford Publishing},
  year       = {2012},
  address    = {Singapore},
}

@BOOK{sanz:PanStanford:2012,
  AUTHOR     = {A. S. Sanz and S. Miret-Art\'es},
  editor     = {X. Oriols and J. Mompart},
  title      = {Applied Bohmian Mechanics: From Nanoscale Systems to Cosmology},
  CHAPTER    = {The role of trajectories in quantum chemistry and chemical physics},
  pages      = {235-301},
  publisher  = {Pan Standford Publishing},
  year       = {2012},
  address    = {Singapore},
}

@article{wyatt:prl:1999,
 author    = {C. L. Lopreore and R. E. Wyatt},
 journal   = {Phys. Rev. Lett.},
 title     = {Quantum wave packet dynamics with trajectories},
 volume    = {82},
 pages     = {5190-5193},
 year      = {1999},
}

@article{wyatt:cpl:1999,
 author    = {C. L. Lopreore and R. E. Wyatt},
 journal   = {Chem. Phys. Lett.},
 title     = {Quantum wave packet dynamics with trajectories: reflections on a downhill ramp potential},
 volume    = {325},
 pages     = {73-78},
 year      = {2000},
}

@article{sanz:EPL:2001,
 author    = {A. S. Sanz and F. Borondo and S. Miret-Art\'es},
 journal   = {Europhys. Lett.},
 title     = {On the classical limit in atom-surface diffraction},
 volume    = {55},
 pages     = {303-309},
 year      = {2001},
}

@article{sanz:prb:2000,
 author    = {A. S. Sanz and F. Borondo and S. Miret-Art\'es},
 journal   = {Phys. Rev. B},
 title     = {Causal trajectories description of atom diffraction by surfaces},
 volume    = {61},
 pages     = {7743-7751},
 year      = {2000},
}

@book{bell-bk,
  author     = {J. S. Bell},
  title      = {Speakable and Unspeakable in Quantum Mechanics},
  publisher  = {Cambridge University Press},
  year       = {1987},
  address    = {Cambridge},
}

@article{englert:zna:1993-1,
 author    = {B.-G. Englert and M. O. Scully and G. S\"ussmann and H. Walther},
 journal   = {Z. Naturforsch. A},
 title     = {Surrealistic Bohm trajectories},
 volume    = {47},
 pages     = {1175-1186},
 year      = {1993},
}

@article{duerr:zna:1993,
 author    = {D. D\"urr and W. Fusseder and S. Goldstein and N. Zangh\`i},
 journal   = {Z. Naturforsch. A},
 title     = {Comment on `Surrealistic Bohm trajectories'},
 volume    = {48},
 pages     = {1261-1262},
 year      = {1993},
}

@article{duerr:JStatPhys:1992a,
 author    = {D. D\"urr and S. Goldstein and N. Zangh\`{\i}},
 journal   = {J. Stat. Phys.},
 title     = {Quantum equilibrium and the origin of absolute uncertainty},
 volume    = {67},
 pages     = {843-907},
 year      = {1992},
}

@article{englert:zna:1993-2,
 author    = {B.-G. Englert and M. O. Scully and G. S\"ussmann and and H. Walther},
 journal   = {Z. Naturforsch. A},
 title     = {Reply to comment on `Surrealistic Bohm trajectories'},
 volume    = {48},
 pages     = {1263-1264},
 year      = {1993},
}

@article{scully:PhysScr:1998,
 author    = {M. O. Scully},
 journal   = {Phys. Scr.},
 title     = {Do Bohm trajectories always provide a trustworthy physical picture of particle motion?},
 volume    = {T76},
 pages     = {41-46},
 year      = {1998},
}

@article{jonsson:ZPhys:1961,
 author    = {C. J\"onsson},
 journal   = {Z. Phys.},
 title     = {Elektroneninterferenzen an mehreren k\"unstlich hergestellten Feinspalten},
 volume    = {161},
 pages     = {454-474},
 year      = {1961},
}

@article{jonsson:AJP:1974,
 author    = {C. J\"onsson and D. Brandt and S. Hirschi},
 journal   = {Am. J. Phys.},
 title     = {Electron diffraction at multiple slits},
 volume    = {42},
 pages     = {4-11},
 year      = {1974},
}

@article{hirschi:AJP:1974,
 author    = {S. Hirschi},
 journal   = {Am. J. Phys.},
 title     = {Erratum: ``Electron diffraction at multiple slits'' [Am. J. Phys. 42, 4 (1974)]},
 volume    = {42},
 pages     = {423},
 year      = {1974},
}

@article{pozzi:AJP:1973,
 author    = {O. Donati and G. F. Missiroli and G. Pozzi},
 journal   = {Am. J. Phys.},
 title     = {An experiment on electron interference},
 volume    = {41},
 pages     = {639-644},
 year      = {1973},
}

@article{pozzi:AJP:1976,
 author    = {P. G. Merli and G. F. Missiroli and G. Pozzi},
 journal   = {Am. J. Phys.},
 title     = {On the statistical aspect of electron interference phenomena},
 volume    = {44},
 pages     = {306-307},
 year      = {1976},
}

@article{pozzi:AJP:1978,
 author    = {G. Matteucci and G. Pozzi},
 journal   = {Am. J. Phys.},
 title     = {Two further experiments on electron interference},
 volume    = {46},
 pages     = {619-623},
 year      = {1978},
}

@article{pozzi:AJP:2007,
 author    = {S. Frabboni and G.-C. Gazzadi and G. Pozzi},
 journal   = {Am. J. Phys.},
 title     = {Young's double-slit interference experiment with electrons},
 volume    = {75},
 pages     = {1053-1055},
 year      = {2007},
}

@article{pozzi:EJP:2013,
 author    = {G. Matteucci and M. Pezzi and G. Pozzi and G. L. Alberghi and F. Giorgi and  A. Gabrielli and N. S. Cesari and M. Villa and A. Zoccoli and S. Frabboni and G. C. Gazzadi},
 journal   = {Eur. J. Phys.},
 title     = {Build-up of interference patterns with single electrons},
 volume    = {34},
 pages     = {511-517},
 year      = {2013},
}

@article{tonomura:ajp:1989,
 author    = {A. Tonomura and J. Endo and T. Matsuda and T. Kawasaki and H. Ezawa},
 journal   = {Am. J. Phys.},
 title     = {Demonstration of single-electron buildup of an interference pattern},
 volume    = {57},
 pages     = {117-120},
 year      = {1989},
}

@article{shimizu:pra:1992,
 author    = {F. Shimizu and K. Shimizu and H. Takuma},
 journal   = {Phys. Rev. A},
 title     = {Double-slit interference with ultracold metastable neon atoms},
 volume    = {46},
 pages     = {R17-R20},
 year      = {1992},
}

@article{cerofolini:lnc:1980,
 author    = {C. F. Cerofolini},
 journal   = {Lett. Nuovo Cim.},
 title     = {On the nature of the subquantum medium},
 volume    = {29},
 pages     = {305-309},
 year      = {1980},
}

@article{nelson:pr:1966,
 author    = {E. Nelson},
 journal   = {Phys. Rev.},
 title     = {Derivation of the Schr\"odinger equation from Newtonian mechanics},
 volume    = {150},
 pages     = {1079-1085},
 year      = {1966},
}

@article{penna:jmp:1969,
 author    = {L. de la Pe{\~n}a-Auerbach},
 journal   = {J. Math. Phys.},
 title     = {New formulation of stochastic theory and quantum mechanics},
 volume    = {10},
 pages     = {1620-1630},
 year      = {1969},
}

@article{penna:jmp:1971,
 author    = {L. de la Pe{\~n}a-Auerbach},
 journal   = {J. Math. Phys.},
 title     = {Stochastic theory of quantum mechanics for particles with spin},
 volume    = {12},
 pages     = {453-461},
 year      = {1971},
}

@article{bohm:pr:1954,
 author    = {D. Bohm and J. P. Vigier},
 journal   = {Phys. Rev.},
 title     = {Model of the causal interpretation of quantum theory in terms of a fluid with irregular fluctuations},
 volume    = {96},
 pages     = {208-216},
 year      = {1954},
}

@article{sanz:cpl:2007,
title = {Aspects of nonlocality from a quantum trajectory perspective: A WKB approach to Bohmian mechanics},
journal = {Chem. Phys. Lett.},
volume = {445},
number = {4},
pages = {350-354},
year = {2007},
issn = {0009-2614},
doi = {https://doi.org/10.1016/j.cplett.2007.08.002},
url = {https://www.sciencedirect.com/science/article/pii/S0009261407010561},
author = {A. S. Sanz and S. Miret-Art\'es},
}

@article{berry:JPA:1996,
 author    = {M. V. Berry},
 journal   = {J. Phys. A: Math. Theor.},
 title     = {Quantum fractals in boxes},
 volume    = {29},
 pages     = {6617-6629},
 year      = {1996},
 doi       = {10.1088/0305-4470/29/20/016},
}

@article{sanz:JPA:2005,
 author    = {A. S. Sanz},
 journal   = {J. Phys. A: Math. Theor.},
 title     = {A Bohmian approach to quantum fractals},
 volume    = {38},
 pages     = {6037-6049},
 year      = {2005},
 doi       = {10.1088/0305-4470/38/26/013},
}

@article{sanz:cpl:2008,
 author    = {A. S. Sanz and S. Miret-Art\'es},
 journal   = {Chem. Phys. Lett.},
 title     = {Interplay of causticity and vorticality within the complex quantum Hamilton-Jacobi formalism},
 volume    = {458},
 pages     = {239-243},
 year      = {2008},
}

@article{chou:prl:2009,
 author    = {C.-C. Chou and A. S. Sanz and S. Miret-Art\'es and R. E. Wyatt},
 journal   = {Phys. Rev. Lett.},
 title     = {Hydrodynamic view of wave-packet interference: Quantum caves},
 volume    = {102},
 pages     = {250401(1-4)},
 year      = {2009},
}

@article{chou:annphys:2010,
 author    = {C.-C. Chou and A. S. Sanz and S. Miret-Art\'es and R. E. Wyatt},
 journal   = {Ann. Phys.},
 title     = {Quantum interference within the complex quantum Hamilton-Jacobi formalism},
 volume    = {325},
 pages     = {2193-2211},
 year      = {2010},
}

@article{sanz:jcp:2004,
 author    = {A. S. Sanz and F. Borondo and S. Miret-Art\'es},
 journal   = {J. Chem. Phys.},
 title     = {Quantum trajectories in atom-surface scattering with single adsorbates: The role of quantum vortices},
 volume    = {120},
 pages     = {8794-8806},
 year      = {2004},
 doi       = {10.1063/1.1683136},
}

@article{sanz:prb:2004,
 author    = {A. S. Sanz and F. Borondo and S. Miret-Art\'es},
 journal   = {Phys. Rev. B},
 title     = {Role of quantum vortices in atomic scattering from single adsorbates},
 volume    = {69},
 pages     = {115413(1-5)},
 year      = {2004},
 doi       = {10.1103/PhysRevB.69.115413},
}

@article{sanz:cpl:2009,
 author    = {A. S. Sanz and X. Gim\'enez and J. M. Bofill and S. Miret-Art\'es},
 journal   = {Chem. Phys. Lett.},
 title     = {Understanding chemical reactions within a generalized Hamilton-Jacobi framework},
 volume    = {478},
 pages     = {89-96},
 year      = {2009},
}

@article{sanz:cpl:2010E,
 author    = {A. S. Sanz and X. Gim\'enez and J. M. Bofill and S. Miret-Art\'es},
 journal   = {Chem. Phys. Lett.},
 title     = {Erratum to `Understanding chemical reactions within a generalized Hamilton-Jacobi framework' [Chem. Phys. Lett. {\bf 478} (2009) 89]},
 volume    = {488},
 pages     = {235-236},
 year      = {2010},
}

@article{prosser:ijtp:1976-1,
 author    = {R. D. Prosser},
 journal   = {Int. J. Theor. Phys.},
 title     = {The interpretation of diffraction and interference in terms of energy flow},
 volume    = {15},
 pages     = {169-180},
 year      = {1976},
}

@article{prosser:ijtp:1976-2,
 author    = {R. D. Prosser},
 journal   = {Int. J. Theor. Phys.},
 title     = {Quantum theory and the nature of interference},
 volume    = {15},
 pages     = {181-193},
 year      = {1976},
}

@book{scully-zubairy-bk,
  author     = {M. O. Scully and S. Zubairy},
  title      = {Quantum Optics},
  publisher  = {Cambridge University Press},
  year       = {1997},
  address    = {Cambridge},
}

@article{ehrenberg:procphyssocb:1949,
 author    = {W. Ehrenberg and R. E. Siday},
 journal   = {Proc. Phys. Soc. B},
 title     = {The refractive index in electron optics and the principles of dynamics},
 volume    = {62},
 pages     = {8-21},
 year      = {1949},
}

@article{aharonov:pr:1959,
 author    = {Y. Aharonov and D. Bohm},
 journal   = {Phys. Rev.},
 title     = {Significance of electromagnetic potentials in the quantum theory},
 volume    = {115},
 pages     = {485-491},
 year      = {1959},
}

@article{aharonov:pr:1961,
 author    = {Y. Aharonov and D. Bohm},
 journal   = {Phys. Rev.},
 title     = {Further considerations on electromagnetic potentials in the quantum theory},
 volume    = {123},
 pages     = {1511-1524},
 year      = {1961},
}

@article{josephson:rmp:1974,
 author    = {B. D. Josephson},
 journal   = {Rev. Mod. Phys.},
 title     = {The discovery of tunnelling supercurrents},
 volume    = {46},
 pages     = {251-254},
 year      = {1974},
}

@article{bohm:nuovocim:1976,
 author    = {D. Bohm and B. J. Hiley},
 journal   = {Nuovo Cim.},
 title     = {Non-locality and polarisation correlations of annihilation quanta},
 volume    = {35B},
 pages     = {137-144},
 year      = {1967},
}

@article{butt:jpg:1976,
 author    = {A. R. Wilson and J. Lowe and D. K. Butt},
 journal   = {J. Phys. G},
 title     = {Measurement of the relative planes of polarization of annihilation quanta as a function of separation distance},
 volume    = {2},
 pages     = {613-624},
 year      = {1976},
}

@book{bohm-hiley-bk,
  author     = {D. Bohm and B. J. Hiley},
  title      = {The Undivided Universe},
  publisher  = {Routledge},
  year       = {1993},
  address    = {New York},
}

@book{wheeler:1978,
  AUTHOR =       {J. A. Wheeler},
  editor =       {A. R. Marlow},
  TITLE =        {The past and the delayed-choice double-slit experiment},
  PUBLISHER =    {Academic Press},
  YEAR =         {1978},
  series =       {Mathematical Foundations of Quantum Theory},
  pages =        {9-47},
  address =      {New York},
}

@book{wheeler:1983,
  AUTHOR =       {W. A. Miller and J. A. Wheeler},
  editor =       {S. Kamefuchi and},
  TITLE =        {Delayed-choice experiments and Bohr's elementary quantum phenomenon},
  PUBLISHER =    {Physical Society of Japan},
  YEAR =         {1983},
  series =       {Proc. Int. Symp. Foundation of Quantum Mechanics (Tokyo)},
  pages =        {140-151},
  address =      {Tokyo},
}

@article{hiley:physscr:2006,
 author    = {B. J. Hiley and R. E. Callaghan},
 journal   = {Phys. Scr.},
 title     = {Delayed-choice experiments and the Bohm approach},
 volume    = {74},
 pages     = {336-348},
 year      = {2006},
}

@article{hiley:arxiv:2011,
 author    = {M. de Gosson and B. J. Hiley},
 journal   = {arXiv:1010.2622v2},
 title     = {Zeno paradox for Bohmian trajectories: The unfolding of the metatron},
 volume    = {},
 pages     = {},
 year      = {2011},
}

@article{hiley:foundphys:1982,
 author    = {C. Dewdney and B. J. Hiley},
 journal   = {Found. Phys.},
 title     = {A quantum potential description of one-dimensional time-dependent scattering from square barriers},
 volume    = {12},
 pages     = {27-48},
 year      = {1982},
}

@article{wyatt:JCP:1999,
 author    = {R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Quantum wave packet dynamics with trajectories: Application to reactive scattering},
 volume    = {111},
 pages     = {4406-4413},
 year      = {1999},
}

@BOOK{schiff-bk,
  AUTHOR     = {L. I. Schiff},
  TITLE      = {Quantum Mechanics},
  PUBLISHER  = {McGraw-Hill},
  YEAR       = {1968},
  address    = {Singapore},
  edition    = {3rd},
}

@BOOK{liboff-bk,
  AUTHOR     = {R. L. Liboff},
  TITLE      = {Introductory Quantum Mechanics},
  PUBLISHER  = {Addison-Wesley},
  YEAR       = {1980},
  address    = {Reading, MA},
}

@article{brumer:pra:2006,
 author    = {P. Brumer and J. Gong},
 journal   = {Phys. Rev. A},
 title     = {Born rule in quantum and classical mechanics},
 volume    = {73},
 pages     = {052109(1-4)},
 year      = {2006},
}

@article{sanz:jcp:2005,
 author    = {A. S. Sanz and S. Miret-Art\'es},
 journal   = {J. Chem. Phys.},
 title     = {Quantum trajectories in elastic atom-surface scattering: Threshold and selective adsorption resonances},
 volume    = {122},
 pages     = {014702(1-12},
 year      = {2005},
}

@article{elster:1899,
 author    = {J. Elster and H. Geitel},
 journal   = {Verhandlungen der Deutschen Physikalischen Gesellschaft},
 title     = {\"Uber den Einflu{\ss} eines magnetischen Feldes auf die durch die Becquerelstrahlen bewirkte Leitf\"ahigkeit der Luft},
 volume    = {1},
 pages     = {136-138},
 year      = {1899},
}

@BOOK{goldstein-bk,
  AUTHOR     = {H. Goldstein and C. Poole and J. Safko},
  TITLE      = {Classical Mechanics},
  PUBLISHER  = {Addison Wesley},
  YEAR       = {2001},
  address    = {New York},
  edition    = {3rd},
}

@BOOK{tannor-bk,
  AUTHOR     = {D. J. Tannor},
  TITLE      = {Introduction to Quantum Mechanics: A Time-Dependent Perspective},
  PUBLISHER  = {University Science Books},
  YEAR       = {2006},
  address    = {Sausalito, CA},
}

@BOOK{feynman-bk1,
  AUTHOR     = {R. P. Feynman and A. R. Hibbs},
  TITLE      = {Quantum Mechanics and Path Integrals},
  PUBLISHER  = {McGraw-Hill},
  YEAR       = {1965},
  address    = {New York},
}

@BOOK{feynman-bk2,
  AUTHOR     = {R. P. Feynman},
  TITLE      = {Path Integral Approach to Quantum Mechanics},
  PUBLISHER  = {University Science Books},
  YEAR       = {2006},
  address    = {Sausalito, CA},
}

@article{egger:MonWeaRev:1996,
 author    = {J. Egger},
 journal   = {Am. Meteor. Soc.},
 title     = {Volume conservation in phase space: A fresh look at numerical integration schemes},
 volume    = {124},
 pages     = {1955-1964},
 year      = {1996},
}

@article{sommer:MonWeaRev:2010,
 author    = {M. Sommer and S. Reich},
 journal   = {Am. Meteor. Soc.},
 title     = {Phase space volume conservation under space and time discretization schemes for the shallow-water equations},
 volume    = {138},
 pages     = {4229-4236},
 year      = {2010},
}

@BOOK{mazur-bk:2007,
  AUTHOR     = {J. Mazur},
  TITLE      = {Zeno's Paradox: Unraveling the Ancient Mystery behind the Science of Space and Time},
  PUBLISHER  = {Plume},
  YEAR       = {2007},
  address    = {New York},
}

@article{sanz:JPA:2011,
 author    = {A. S. Sanz and S. Miret-Art\'es},
 journal   = {J. Phys. A: Math. Theor.},
 title     = {Setting-up tunneling conditions by means of Bohmian mechanics},
 volume    = {44},
 pages     = {485301(1-17)},
 year      = {2011},
}

@article{gonzalo:PRA:2011,
 author    = {M. A. Porras and A. Luis and I. Gonzalo and A. S. Sanz},
 journal   = {Phys. Rev. A},
 title     = {Zeno dynamics in wave packet diffraction spreading},
 volume    = {84},
 pages     = {052109(1-6)},
 year      = {2011},
}

@article{misra:JMathPhys:1977,
 author    = {B. Misra and E. C. G. Sudarshan},
 journal   = {J. Math. Phys.},
 title     = {The Zeno's paradox in quantum theory},
 volume    = {18},
 pages     = {756-763},
 year      = {1977},
}

@article{misra:PRD:1977,
 author    = {C. B. Chiu and E. C. G. Sudarshan and B. Misra},
 journal   = {Phys. Rev. D},
 title     = {Time evolution of unstable quantum systems and a resolution of Zeno's paradox},
 volume    = {16},
 pages     = {520-529},
 year      = {1977},
}

@article{peres:AmJPhys:1980,
 author    = {A. Peres},
 journal   = {Am. J. Phys.},
 title     = {Zeno paradox in quantum theory},
 volume    = {48},
 pages     = {931-932},
 year      = {1980},
}

@article{pascazio:JPA:2008,
 author    = {P. Facchi and S. Pascazio},
 journal   = {J. Phys. A: Math. Theor.},
 title     = {Quantum Zeno dynamics: mathematical and physical aspects},
 volume    = {41},
 pages     = {493001(1-45)},
 year      = {2008},
}

@article{pascazio:PRL:2001,
 author    = {P. Facchi and H. Nakazato and S. Pascazio},
 journal   = {Phys. Rev. Lett.},
 title     = {From the quantum zeno to the inverse quantum Zeno effect},
 volume    = {86},
 pages     = {2699-2702},
 year      = {2001},
}

@article{itano:PRA:1990,
 author    = {W. M. Itano and D. J. Heinzen and J. J. Bollinger and D. J. Wineland},
 journal   = {Phys. Rev. A},
 title     = {Quantum Zeno effect},
 volume    = {41},
 pages     = {2295-2300},
 year      = {1990},
}

@article{cook:PhysScr:1988,
 author    = {R. J. Cook},
 journal   = {Phys. Scr.},
 title     = {What are quantum jumps?},
 volume    = {T21},
 pages     = {49-51},
 year      = {1988},
}

@BOOK{dirac-bk:1930,
  AUTHOR     = {P. A. M. Dirac},
  TITLE      = {Principles of Quantum Mechanics},
  PUBLISHER  = {Oxford University Press},
  YEAR       = {1930},
  address    = {Oxford},
}

@BOOK{vonNeumann-bk:1932,
  AUTHOR     = {J. von Neumann},
  TITLE      = {Die Mathematische Grundlagen der Quantenmechanik},
  PUBLISHER  = {Springer Verlag},
  YEAR       = {1932},
  address    = {Berlin},
}

@BOOK{vonNeumann-bk:1932En,
  AUTHOR     = {J. von Neumann and R. T. Beyer (transl.)},
  TITLE      = {Mathematical Foundations of Quantum Mechanics},
  PUBLISHER  = {Princeton University Press},
  YEAR       = {1955},
  address    = {Princeton},
}

@BOOK{parker-bk:1994,
  AUTHOR     = {C. B. Parker},
  TITLE      = {McGraw Hill Encyclopaedia of Physics},
  PUBLISHER  = {McGraw Hill},
  YEAR       = {1994},
  address    = {Princeton},
  edition    = {2nd},
}

@article{raizen:PRL:2001,
 author    = {M. C. Fischer and B. Guti\'errez-Medina and M. G. Raizen},
 journal   = {Phys. Rev. Lett.},
 title     = {Observation of the quantum Zeno and anti-Zeno effects in an unstable system},
 volume    = {87},
 pages     = {040402(1-4)},
 year      = {2001},
}

@article{raizen:Nature:1997,
 author    = {S. R. Wilkinson and C. F. Bharucha and M. C. Fischer and K. W. Madison and P. R. Morrow and Q. Niu and B. Sundaram and M. G. Raizen},
 journal   = {Nature},
 title     = {Experimental evidence for non-exponential decay in quantumtunnelling},
 volume    = {387},
 pages     = {575-577},
 year      = {1997},
}

@article{luis:PRA:1998,
 author    = {A. Luis and L. S\'anchez-Soto},
 journal   = {Phys. Rev. A},
 title     = {Anti-Zeno effect in parametric down-conversion},
 volume    = {57},
 pages     = {781-787},
 year      = {1998},
}

@article{kaulakys:PRA:1997,
 author    = {B. Kaulakys and V. Gontis},
 journal   = {Phys. Rev. A},
 title     = {Quantum anti-Zeno effect},
 volume    = {56},
 pages     = {1131-1137},
 year      = {1997},
}

@article{kofman:Nature:2000,
 author    = {A. G. Kofman and G. Kurizki},
 journal   = {Nature},
 title     = {Acceleration of quantum decay processes by frequent observations},
 volume    = {405},
 pages     = {546-550},
 year      = {2000},
}

@BOOK{kloeden-bk:1992,
  AUTHOR     = {P. E. Kloeden and E. Platen},
  TITLE      = {Numerical Solution of Stochastic Differential Equations},
  PUBLISHER  = {Springer},
  YEAR       = {1992},
  address    = {Berlin},
}

@BOOK{breuer-bk:2002,
  AUTHOR     = {H.-P. Breuer and F. Petruccione},
  TITLE      = {The Theory of Open Quantum Systems},
  PUBLISHER  = {Oxford University Press},
  YEAR       = {2002},
  address    = {Oxford},
}

@article{tomas:2011,
 author    = {C. Sanz-Sanz and A. S. Sanz and T. Gonz\'alez-Lezana and O. Roncero and S. Miret-Art\'es},
 journal   = {},
 title     = {Revisiting Zeno's paradox: Flying arrows for atom-diatom reactions},
 volume    = {},
 pages     = {(1-4)},
 year      = {submitted, 2011},
 archivePrefix        = {arXiv},
 eprint               = {1111.1520},
}

@article{coffey:JPA:2008,
 author    = {T. M. Coffey and R. E. Wyatt and W. C. Schieve},
 journal   = {J. Phys. A: Math. Theor.},
 title     = {Monte Carlo generation of Bohmian trajectories},
 volume    = {41},
 pages     = {335304},
 year      = {2008},
}

@article{coffey:JPA:2010,
 author    = {T. M. Coffey and R. E. Wyatt and W. C. Schieve},
 journal   = {J. Phys. A: Math. Theor.},
 title     = {Quantum trajectories from kinematic considerations},
 volume    = {43},
 pages     = {335301},
 year      = {2010},
}

@article{brandt:PLA:1998,
 author    = {S. Brandt and H. Dahmen and E. Gjonaj and T. Stroh},
 journal   = {Phys. Lett. A},
 title     = {Quantile motion and tunneling},
 volume    = {249},
 pages     = {265},
 year      = {1998},
}

@article{englert:PRL:1996,
 author    = {B.-G. Englert},
 journal   = {Phys. Rev. Lett.},
 title     = {Fringe visibility and which-way information: An inequality},
 volume    = {77},
 pages     = {2154-2157},
 year      = {1996},
}

@article{chapman:PRL:1995,
 author    = {M. S. Chapman and T. D. Hammond and A. Lenef and J. Schmiedmayer and R. A. Rubenstein and E. Smith and D. E. Pritchard},
 journal   = {Phys. Rev. Lett.},
 title     = {Photon scattering from atoms in an atom interferometer: Coherence lost and regained},
 volume    = {75},
 pages     = {3783-3787},
 year      = {1995},
}

@article{fonseca-guerra:JComputChem:2004,
 author    = {C. Fonseca-Guerra and J.-W. Handgraaf and E. J. Baerends and F. M. Bickelhaupt},
 journal   = {J. Comput. Chem.},
 title     = {Voronoi deformation density (VDD) charges: Assessment of the Mulliken, Bader, Hirshfeld, Weinhold, and VDD methods for charge analysis},
 volume    = {25},
 pages     = {189-210},
 year      = {2004},
}

@article{sanz:AJP:2012,
 author    = {A. S. Sanz and S. Miret-Art\'es},
 journal   = {Am. J. Phys.},
 title     = {Quantum phase analysis with quantum trajectories: A step towards the creation of a Bohmian thinking},
 volume    = {80},
 pages     = {525-533},
 year      = {2012},
doi = {10.1119/1.3698324},
URL = {https://doi.org/10.1119/1.3698324},
}

@PROCEEDINGS{dorlas:SPIE:2004,
   author = {T. C. Dorlas and R. F. O'Connell},
    title = {Quantum Zeno and anti-Zeno effects: An exact model},
booktitle = {Quantum Information and Computation II},
     year = {2004},
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = {5436},
   eprint = {arXiv:quant-ph/0501098},
   editor = {E. Donkor and A. R. Pirich and H. E. Brandt},
    pages = {194-201},
publisher = {SPIE},
  address = {Bellingham, WA},
}

@article{sanz:AnnPhys:2012,
 author    = {A. S. Sanz and C. Sanz-Sanz and T. Gonz\'alez-Lezana and O. Roncero and S. Miret-Art\'es},
 journal   = {Ann. Phys.},
 title     = {Quantum Zeno effect: Quantum shuffling and Markovianity},
 volume    = {327},
 pages     = {1277-1289},
 year      = {2012},
}

@article{octavio:JCP:2012,
 author    = {C. Sanz-Sanz and A. S. Sanz and T. Gonz\'alez-Lezana and O. Roncero and S. Miret-Art\'es},
 journal   = {J. Chem. Phys.},
 title     = {Communication: Quantum Zeno-based control mechanism for molecular fragmentation},
 volume    = {136},
 pages     = {121101(1-4)},
 year      = {2012},
}

@article{helen:JPCM:2011,
 author    = {H. C. Pe\~nate-Rodr{\'\i}guez and R. Mart{\'\i}nez-Casado and G. Rojas-Lorenzo and A. S. Sanz and S. Miret-Art\'es},
 journal   = {J. Phys.: Condens. Matter},
 title     = {Quantum Zeno and anti-Zeno effects in surface diffusion of interacting adsorbates},
 volume    = {24},
 pages     = {104013(1-10)},
 year      = {2012},
}

@BOOK{gutzwiller:1990,
  AUTHOR     = {M. C. Gutzwiller},
  TITLE      = {Chaos in Classical and Quantum Mechanics},
  PUBLISHER  = {Springer-Verlag},
  YEAR       = {1990},
  address    = {New York},
}

@article{sanz:PhysRep:2007,
 author    = {A. S. Sanz and S. Miret-Art\'es},
 journal   = {Phys. Rep.},
 title     = {Selective adsorption resonances: Quantum and stochastic approaches},
 volume    = {451},
 pages     = {37-154},
 year      = {2007},
}

@article{fortagh:RMP:2007,
 author    = {J. Fort\'agh and C. Zimmermann},
 journal   = {Rev. Mod. Phys.},
 title     = {Magnetic microtraps for ultracold atoms},
 volume    = {79},
 pages     = {235-289},
 year      = {2007},
}

@BOOK{brumer-bk:2003,
  AUTHOR     = {M. Shapiro and P. Brumer},
  TITLE      = {Principles of the Quantum Control of Molecular Processes},
  PUBLISHER  = {Wiley},
  YEAR       = {2003},
  address    = {New York},
}

@article{sanz:AnnPhys:2013,
 author    = {A. S. Sanz and S. Miret-Art\'es},
 journal   = {Ann. Phys.},
 title     = {On the unique mapping relationship between initial and final quantum states},
 volume    = {339},
 pages     = {11-21},
 year      = {2013},
}

@article{sinha:Science:2010,
 author    = {U. Sinha and C. Couteau and T. Jennewein and R. Laflamme and G. Weihs},
 journal   = {Science},
 title     = {Ruling out multi-order interference in quantum mechanics},
 volume    = {329},
 pages     = {418-421},
 year      = {2010},
}

@article{uiberacker:Nature:2007,
 author    = {M. Uiberacker and Th. Uphues and M. Schultze and A. J. Verhoef and V. Yakovlev and M. F. Kling
              and J. Rauschenberger and N. M. Kabachnik and H. Schr\"oder and M. Lezius and K. L. Kompa and
              H.-G. Muller and M. J. J. Vrakking and S. Hendel and U. Kleineberg and U. Heinzmann and M. Drescher
              and F. Krausz},
 journal   = {Nature},
 title     = {Attosecond real-time observation of electron tunneling in atoms},
 volume    = {446},
 pages     = {627-632},
 year      = {2007},
}

@article{arndt:NatCommun:2011,
 author    = {S. Gerlich and S. Eibenberger and M. Tomandl and S. Nimmrichter and K. Hornberger and P. J. Fagan and J. T\"uxen and M. Mayor and M. Arndt},
 journal   = {Nat. Commun.},
 title     = {Quantum interference of large organic molecules},
 volume    = {2:263},
 pages     = {1-5},
 year      = {2011},
}

@article{bowman:JCP:1975,
 author    = {C. J. Ray and J. M. Bowman},
 journal   = {J. Chem. Phys.},
 title     = {Quasiclassical trajectory calculation of He-LiF(001) diffraction scattering},
 volume    = {63},
 pages     = {5231-5234},
 year      = {1975},
}

@article{bowman:JCP:1977,
 author    = {C. J. Ray and J. M. Bowman},
 journal   = {J. Chem. Phys.},
 title     = {Quasiclassical studies of rigid rotor-solid surface diffraction scattering},
 volume    = {66},
 pages     = {1122-1126},
 year      = {1977},
}

@article{diaz:PRL:2004,
 author    = {D. Far{\'\i}as and C. D{\'\i}az and P. Rivi\`ere and H. F. Busnego and P. Nieto and M. F. Somers and G. J. Kroes and A. Salin and F. Mart{\'\i}n},
 journal   = {Phys. Rev. Lett.},
 title     = {In-plane and out-of-plane diffraction of H$_2$ from metal surfaces},
 volume    = {93},
 pages     = {246104(1-4)},
 year      = {2004},
}

@article{diaz:PRB:2005,
 author    = {C. D{\'\i}az and M. F. Somers and G. J. Kroes and H. F. Busnego and A. Salin and F. Mart{\'\i}n},
 journal   = {Phys. Rev. B},
 title     = {Quantum and classical dynamics of H$_2$ scattering from Pd(111) at off-normal incidence},
 volume    = {72},
 pages     = {035401(1-10)},
 year      = {2005},
}

@article{diaz:JCP:2005,
 author    = {C. D{\'\i}az and H. F. Busnego and P. Rivi\`ere and D. Far{\'\i}as and P. Nieto and M. F. Somers and G. J. Kroes and A. Salin and F. Mart{\'\i}n},
 journal   = {J. Chem. Phys.},
 title     = {A classical dynamics method for H$_2$ diffraction from metal surfaces},
 volume    = {122},
 pages     = {154706(1-8)},
 year      = {2005},
}

@article{miller:JPCA:2011,
 author    = {W. H. Miller},
 journal   = {J. Phys. Chem. A},
 title     = {The semiclassical initial value representation: A potentially practical way for adding quantum effects to classical molecular dynamics simulations},
 volume    = {105},
 pages     = {2942-2955},
 year      = {2001},
}

@article{pollak:PRL:2003,
 author    = {S. Zhang and E. Pollak},
 journal   = {Phys. Rev. Lett.},
 title     = {Monte Carlo method for evaluating the quantum real time propagator},
 volume    = {91},
 pages     = {190201(1-4)},
 year      = {2003},
}

@BOOK{zhang-bk,
  AUTHOR     = {J. Z. H. Zhang},
  TITLE      = {Theory and Application of Quantum Molecular Dynamics},
  PUBLISHER  = {World Scientific},
  YEAR       = {1999},
  address    = {Singapore},
}

@article{bittner:JCP:2003,
 author    = {E. R. Bittner},
 journal   = {J. Chem. Phys.},
 title     = {Quantum initial value representation using approximate Bohmian trajectories},
 volume    = {119},
 pages     = {1358-1364},
 year      = {2003},
}

@article{makri:JCP:2003,
 author    = {Y. Zhao and N. Makri},
 journal   = {J. Chem. Phys.},
 title     = {Bohmian versus semiclassical description of interference phenomena},
 volume    = {119},
 pages     = {60-67},
 year      = {2003},
}

@article{makri:JPCA-1:2004,
 author    = {J. Liu and N. Makri},
 journal   = {J. Phys. Chem. A},
 title     = {Forward-backward quantum dynamics for time correlation functions},
 volume    = {108},
 pages     = {806-812},
 year      = {2004},
}

@article{makri:JPCA-2:2004,
 author    = {J. Liu and N. Makri},
 journal   = {J. Phys. Chem. A},
 title     = {Monte Carlo Bohmian dynamics from trajectory stability properties},
 volume    = {108},
 pages     = {5408-5416},
 year      = {2004},
}

@article{makri:MolPhys:2005,
 author    = {J. Liu and N. Makri},
 journal   = {Mol. Phys.},
 title     = {Bohm's formulation in imaginary time: estimation of energy eigenvalues},
 volume    = {103},
 pages     = {1083-1090},
 year      = {2005},
}

@article{franco:JCP:2017,
 author  = {B. Gu. and I. Franco},
 journal  = {J. Chem. Phys.},
 title  = {Partial hydrodynamic representation of quantum molecular dynamics},
 volume  = {146},
 pages  = {194104(1-8)},
 year   = {2017},
}

@BOOK{sanz-bk-1,
  AUTHOR     = {A. S. Sanz and S. Miret-Art\'es},
  TITLE      = {A Trajectory Description of Quantum Processes. I. Fundamentals},
  PUBLISHER  = {Springer},
  volume     = {850},
  series     = {Lecture Notes in Physics},
  YEAR       = {2012},
  address    = {Berlin},
}

@BOOK{sanz-bk-2,
  AUTHOR     = {A. S. Sanz and S. Miret-Art\'es},
  TITLE      = {A Trajectory Description of Quantum Processes. II. Applications},
  PUBLISHER  = {Springer},
  volume     = {831},
  series     = {Lecture Notes in Physics},
  YEAR       = {2014},
  address    = {Berlin},
}

@article{ballentine:RMP:1979,
 author    = {L. E. Ballentine},
 journal   = {Rev. Mod. Phys.},
 title     = {The statistical interpretation of quantum mechanics},
 volume    = {42},
 pages     = {358-381},
 year      = {1979},
}

@article{sanz:SSR:2004,
 author    = {R. Guantes and A. S. Sanz and J. Margalef-Roig and S. Miret-Art\'es},
 journal   = {Surf. Sci. Rep.},
 title     = {Atom-surface diffraction: a trajectory description},
 volume    = {53},
 pages     = {199-330},
 year      = {2004},
}

@article{kosloff:JCP:1983,
 author    = {R. Kosloff and D. Kosloff},
 journal   = {J. Chem. Phys.},
 title     = {A Fourier method solution for the time dependent Schr\"odinger equation: A study of the reaction H$^+$+H$_2$, D$^+$+HD, and D$^+$+H$_2$},
 volume    = {79},
 pages     = {1823-1833},
 year      = {1983},
}

@article{kosloff:JCompPhys:1983,
 author    = {D. Kosloff and R. Kosloff},
 journal   = {J. Comp. Phys.},
 title     = {A Fourier method solution for the time dependent Schr\"odinger equation as a tool in molecular dynamics},
 volume    = {52},
 pages     = {35-53},
 year      = {1983},
}

@article{kosloff:JCompPhys:1986,
 author    = {R. Kosloff and D. Kosloff},
 journal   = {J. Comp. Phys.},
 title     = {Absorbing boundaries for wave propagation problems},
 volume    = {63},
 pages     = {363-376},
 year      = {1986},
}

@article{manolopoulos:JCompPhys:2002,
 author    = {D. E. Manolopoulos},
 journal   = {J. Comp. Phys.},
 title     = {Derivation and reflection properties of a transmission-free absorbing potential},
 volume    = {117},
 pages     = {9552-9559},
 year      = {2002},
}

@article{metiu:JCompPhys:1986,
 author    = {R. Heather and H. Metiu},
 journal   = {J. Comp. Phys.},
 title     = {An efficient procedure for calculating the evolution of the wave function by fast Fourier transform methods for systems with spatially extended wave function and localized potential},
 volume    = {86},
 pages     = {5009-5017},
 year      = {1986},
}

@article{pernot:IJQC:1991,
 author    = {P. Pernot and W. A. Lester Jr.},
 journal   = {Intern. J. Quantum Chem.},
 title     = {Multidimensional wave-packet analysis: Splitting method for time-resolved property determination},
 volume    = {40},
 pages     = {577-588},
 year      = {1991},
}

@article{born:ZPhys:1926,
 author    = {M. Born},
 journal   = {Z. Phys.},
 title     = {Zur Quantenmechanik der Sto{\ss}vorg\"ange,},
 volume    = {37},
 pages     = {863-867},
 year      = {1926},
}

@book{landsman:CQP:2009,
  AUTHOR =       {N. P. Landsman},
  editor =       {D. Greenberger and K. Hentschel and F. Weinert},
  TITLE =        {Born rule and its interpretation},
  PUBLISHER =    {Springer},
  YEAR =         {2009},
  series =       {Compendium of Quantum Physics: Concepts, Experiments, History and Philosophy},
  pages =        {64-70},
  address =      {Berlin},
}

@article{thompson:JCP:1972,
 author    = {D. L. Thompson},
 journal   = {J. Chem. Phys.},
 title     = {On a classical trajectory study of energy transfer in some atom-diatomic molecule systems},
 volume    = {56},
 pages     = {3570-3580},
 year      = {1972},
}

@article{karplus:JCP:1965,
 author    = {M. Karplus and R. N. Porter and R. D. Sharma},
 journal   = {J. Chem. Phys.},
 title     = {Exchange reactions with activation energy. I. Simple barrier potential for (H, H$_2$)},
 volume    = {43},
 pages     = {3259-3287},
 year      = {1965},
}

@article{kerner:CanJPhys:1958,
 author    = {E. H. Kerner},
 journal   = {Can. J. Phys.},
 title     = {Note on the forced and damped oscillator in quantum mechanics},
 volume    = {36},
 pages     = {371-377},
 year      = {1958},
}

@article{schuch:IJQC:1990,
 author    = {D. Schuch},
 journal   = {Int. J. Quantum. Chem.},
 title     = {},
 volume    = {24},
 pages     = {767-},
 year      = {1990},
}

@article{schuch:IJQC:1999,
 author    = {D. Schuch},
 journal   = {Int. J. Quantum. Chem.},
 title     = {Effective description of the dissipative interaction between simple model-systems and their environment},
 volume    = {72},
 pages     = {537-547},
 year      = {1999},
}

@article{majima:AnnPhys:2011,
 author    = {H. Majima and A. Suzuki},
 journal   = {Ann. Phys.},
 title     = {Quantization and instability of the damped harmonic oscillator subject to a time-dependent force},
 volume    = {326},
 pages     = {3000-3012},
 year      = {2011},
}

@article{jannussis:PhysicaA:1980,
 author    = {A. Jannussis and P. Filipakis and Th. Filipakis},
 journal   = {Physica},
 title     = {Quantum friction in phase space},
 volume    = {102A},
 pages     = {561-567},
 year      = {1980},
}

@article{jannussis:PhysLett:1979,
 author    = {A. D. Jannussis and G. N. Brodimas and A. Streclas},
 journal   = {Phys. Lett.},
 title     = {Propagator with friction in quantum mechanics},
 volume    = {74A},
 pages     = {6-10},
 year      = {1979},
}

@article{khandekar:JMathPhys:1979,
 author    = {D. C. Khandekar and S. V. Lawande},
 journal   = {J. Math. Phys.},
 title     = {Exact solution of a time-dependent quantal harmonic oscillator with damping and a perturbative force},
 volume    = {20},
 pages     = {1870-1877},
 year      = {1979},
}

@article{sun:PRA:1995,
 author    = {C.-P. Sun and L.-H. Yu},
 journal   = {Phys. Rev. A},
 title     = {Exact dynamics of a quantum dissipative system in a constant external field},
 volume    = {51},
 pages     = {1845-1853},
 year      = {1995},
}

@article{sun:PRA:1994,
 author    = {L.-H. Yu and C.-P. Sun},
 journal   = {Phys. Rev. A},
 title     = {Evolution of the wave function in a dissipative system},
 volume    = {49},
 pages     = {592-595},
 year      = {1994},
}

@article{schuch:PRA:1997,
 author    = {D. Schuch},
 journal   = {Phys. Rev. A},
 title     = {Nonunitary connection between explicitly time-dependent and nonlinear approaches for the description of dissipative quantum systems},
 volume    = {55},
 pages     = {935-940},
 year      = {1997},
}

@article{schuch:JPA:2001,
 author    = {M. Moshinsky and D. Schuch},
 journal   = {J. Phys. A: Math. Gen.},
 title     = {Diffraction in time with dissipation},
 volume    = {34},
 pages     = {4217-4225},
 year      = {2001},
}

@article{schuch:RevMexFis:2001,
 author    = {M. Moshinsky and D. Schuch and A. Su\'arez-Moreno},
 journal   = {Rev. Mex. F{\'\i}s.},
 title     = {Motion of wave packets with dissipation},
 volume    = {47},
 pages     = {7-10},
 year      = {2001},
}

@article{bowman:JCP:1981,
 author    = {K. M. Christoffel and J. M. Bowman},
 journal   = {J. Chem. Phys.},
 title     = {Quantum and classical dynamics of a coupled doble well oscillator},
 volume    = {74},
 pages     = {5057-5075},
 year      = {1981},
}

@article{guerra:PhysRep:1981,
 author    = {F. Guerra},
 journal   = {Phys. Rep.},
 title     = {Structural aspects of stochastic mechanics and stochastic field theory},
 volume    = {77},
 pages     = {263-312},
 year      = {1981},
}

@article{hsiang:IntJModPhysA:2009,
 author    = {J.-T. Hsiang and L. H. Ford},
 journal   = {Int. J. Mod. Phys. A},
 title     = {Decoherence and recoherence in model quantum systems},
 volume    = {24},
 pages     = {1705-1712},
 year      = {2009},
}

@article{guay:JPA:2003,
 author    = {E. Guay and L. Marchildon},
 journal   = {J. Phys. A: Math. Gen.},
 title     = {Two-particle interference in standard Bohmian quantum mechanics},
 volume    = {36},
 pages     = {5617-5624},
 year      = {2003},
 doi       = {10.1088/0305-4470/36/20/317},
}

@article{walborn:PRA:2002,
 author    = {S. P. Walborn and M. O. Terra Cunha and S. P\'adua and C. H. Monken},
 journal   = {Phys. Rev. A},
 title     = {Double-slit quantum eraser},
 volume    = {65},
 pages     = {033818(1-6)},
 year      = {2002},
 doi       = {10.1103/PhysRevA.65.033818},
}

@article{brida:PRA:2003,
  title = {Biphoton double-slit experiment},
  author = {Brida, G. and Cagliero, E. and Falzetta, G. and Genovese, M. and Gramegna, M. and Predazzi, E.},
  journal = {Phys. Rev. A},
  volume = {68},
  issue = {3},
  pages = {033803},
  numpages = {6},
  year = {2003},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.68.033803},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.68.033803}
}

@article{kwiat:LAS:2002,
 author    = {D. F. V. James and P. G. Kwiat},
 journal   = {Los Alamos Science},
 title     = {Quantum state entanglement: Creation, characterizatin and application},
 volume    = {27},
 pages     = {52-67},
 year      = {2002},
}

@article{ghirardi:JStatPhys:2002,
 author    = {G. Ghirardi and L. Marinatto and T. Weber},
 journal   = {J. Stat. Phys.},
 title     = {Entanglement and properties of composite quantum systems: A conceptual and mathematical analysis},
 volume    = {108},
 pages     = {49-122},
 year      = {2002},
}

@article{ghirardi:PRA:2004,
  title = {General criterion for the entanglement of two indistinguishable particles},
  author = {Ghirardi, GianCarlo and Marinatto, Luca},
  journal = {Phys. Rev. A},
  volume = {70},
  issue = {1},
  pages = {012109},
  numpages = {10},
  year = {2004},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.70.012109},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.70.012109}
}

@article{matzkin:PRA:2011,
  title = {Entanglement in the classical limit: Quantum correlations from classical probabilities},
  author = {Matzkin, A.},
  journal = {Phys. Rev. A},
  volume = {84},
  issue = {2},
  pages = {022111},
  numpages = {5},
  year = {2011},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.84.022111},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.84.022111}
}

@article{pollak:JCP:1980,
 author    = {E. Pollak and M. S. Child},
 journal   = {J. Chem. Phys.},
 title     = {Classical mechanics of a collinear exchange reaction: A direct evaluation of the reaction probability and product distribution},
 volume    = {73},
 pages     = {4373-4380},
 year      = {1980},
}

@article{pollak:JCP:1983,
 author    = {E. Pollak},
 journal   = {J. Chem. Phys.},
 title     = {Classical analysis of collinear light atom transfer reactions},
 volume    = {78},
 pages     = {1228-1236},
 year      = {1983},
}

@article{couder:PRL:2005,
 author    = {Y. Couder and E. Fort and C.-H. Gautier and A. Boudaoud},
 journal   = {Phys. Rev. Lett.},
 title     = {From bouncing to floating: Noncoalescence of drops on a fluid bath},
 volume    = {94},
 pages     = {177801(1-4)},
 year      = {2005},
}

@article{couder:Nature:2005,
 author    = {Y. Couder and S. Proti\`ere and E. Fort and A. Boudaoud},
 journal   = {Nature},
 title     = {Dynamical phenomena: Walking and orbiting droplets},
 volume    = {437},
 pages     = {208},
 year      = {2005},
}

@article{couder:JFluidMech:2006,
 author    = {S. Proti\`ere and A. Boudaoud and Y. Couder},
 journal   = {J. Fluid. Mech.},
 title     = {Particle-wave association on a fluid interface},
 volume    = {554},
 pages     = {85-108},
 year      = {2006},
}

@article{couder:PRL:2006,
 author    = {Y. Couder and E. Fort},
 journal   = {Phys. Rev. Lett.},
 title     = {Single-particle diffraction and interference at a macroscopic scale},
 volume    = {97},
 pages     = {154101(1-4)},
 year      = {2006},
}

@article{couder:PhysFluid:2006,
 author    = {S. Proti\`ere and Y. Couder},
 journal   = {Phys. Fluids},
 title     = {Orbital motion of bouncing drops},
 volume    = {18},
 pages     = {091114},
 year      = {2006},
}

@article{couder:EPL:2008,
 author    = {A. Eddi and D. Terwagne and E. Fort and Y. Couder},
 journal   = {Europhys. Lett.},
 title     = {Wave propelled ratchets and drifting rafts},
 volume    = {87},
 pages     = {44001(1-6)},
 year      = {2008},
}

@article{couder:EPL:2009,
 author    = {A. Eddi and A. Decelle and E. Fort and Y. Couder},
 journal   = {Europhys. Lett.},
 title     = {Archimedean lattices in the bound states of wave interacting particles},
 volume    = {87},
 pages     = {56002(1-6)},
 year      = {2009},
}

@article{couder:PRL:2009,
 author    = {A. Eddi and E. Fort and F. Moisy and Y. Couder},
 journal   = {Phys. Rev. Lett.},
 title     = {Unpredictable tunneling of a classical wave-particle association},
 volume    = {102},
 pages     = {240401(1-4)},
 year      = {2009},
}

@article{couder:PNAS:2010,
 author    = {E. Fort and A. Eddi and A. Boudaoud and J. Moukhtar and Y. Couder},
 journal   = {Proc. Natl. Acad. Sci. USA},
 title     = {Path-memory induced quantization of classical orbits},
 volume    = {108},
 pages     = {17515-17520},
 year      = {2010},
}

@article{couder:EPN:2010,
 author    = {Y. Couder and A. Boudaoud and S. Proti\`ere and E. Fort},
 journal   = {Europhys. News},
 title     = {Walking droplets: A form of wave-particle duality at macroscopic scale?},
 volume    = {41},
 pages     = {14-18},
 year      = {2010},
}

@article{bush:PNAS:2010,
 author    = {J. W. M. Bush},
 journal   = {Proc. Natl. Acad. Sci. USA},
 title     = {Quantum mechanics writ large},
 volume    = {107},
 pages     = {17455-17456},
 year      = {2010},
}

@article{bush:PRE:2013,
 author    = {D. M. Harris and J. Moukhtar and E. Fort and Y. Couder and J. W. M. Bush},
 journal   = {Phys. Rev. E},
 title     = {Wavelike statistics from pilot-wave dynamics in a circular corral},
 volume    = {88},
 pages     = {011001(R)(1-5)},
 year      = {2013},
}

@article{bush:ARFM:2015,
 author    = {J. W. M. Bush},
 journal   = {Annu. Rev. Fluid Mech.},
 title     = {Pilot-wave hydrodynamics},
 volume    = {47},
 pages     = {269-292},
 year      = {2015},
}

@article{swinney:PRL:1993,
 author    = {T. H. Solomon and E. R. Weeks and H. L. Swinney},
 journal   = {Phys. Rev. Lett.},
 title     = {Observation of anomalous diffusion and L\'evy flights in a two-dimensional rotating flow},
 volume    = {71},
 pages     = {3975-2978},
 year      = {1993},
}

@article{klafter:PhysToday:1996,
 author    = {J. Klafter and M. F. Shlesinger and G. Zumofen},
 journal   = {Phys. Today},
 title     = {Beyond Brownian motion},
 volume    = {49},
 pages     = {33-39},
 year      = {1996},
}

@article{sanz:JOSAA:2012,
 author    = {A. S. Sanz and J. Campos-Mart{\'\i}nez and S. Miret-Art\'es},
 journal   = {J. Opt. Am. Soc. A},
 title     = {Transmission properties in waveguides: An optical streamline analysis},
 volume    = {29},
 pages     = {695-701},
 year      = {2012},
}

@article{ketterle:Science:1997,
 author    = {M. R. Andrews and C. G. Townsend and H.-J. Miesner and D. S. Durfee and D. M. Kurn and W. Ketterle},
 journal   = {Science},
 title     = {Observation of interference between two Bose condensates},
 volume    = {275},
 pages     = {637-641},
 year      = {1997},
 doi       = {https://doi.org/10.1126/science.275.5300.637}
}

@article{schumm:NaturePhys:2005,
 author    = {T. Schumm and S. Hofferberth and L. M. Andersson and S. Wildermuth and S. Groth and I. Bar-Joseph and J. Schmiedmayer and P. Kr\"uger},
 journal   = {Nature Phys.},
 title     = {Matter-wave interferometry in a double well on an atom chip},
 volume    = {1},
 pages     = {57-62},
 year      = {2005},
}

@article{burnett:PRA:1992,
 author    = {K. Burnett and V. C. Reed and J. Cooper and P. L. Knight},
 journal   = {Phys. Rev. A},
 title     = {Calculation of the background emitted during high-harmonic generation},
 volume    = {45},
 pages     = {3347-3349},
 year      = {1992},
}

@article{spanner:PRL:2003,
 author    = {M. Spanner},
 journal   = {Phys. Rev. Lett.},
 title     = {Strong field tunnel ionization by real-valued classical trajectories},
 volume    = {90},
 pages     = {233005(1-4)},
 year      = {2003},
}

@article{lai:EPJD:2009,
 author    = {X. Y. Lai and Q. Y. Cai and M. S. Zhan},
 journal   = {Eur. Phys. J. D},
 title     = {Above-threshold ionization photoelectron spectrum from quantum trajectory},
 volume    = {53},
 pages     = {393-396},
 year      = {2009},
}

@article{lai:NJP:2009,
 author    = {X. Y. Lai and Q. Y. Cai and M. S. Zhan},
 journal   = {New J. Phys.},
 title     = {From a quantum to a classical description of intense laser-atom physics with Bohmian trajectories},
 volume    = {11},
 pages     = {113035(1-10)},
 year      = {2009},
}

@article{lai:ChinPhysB:2010,
 author    = {X. Y. Lai and Q. Y. Cai and M. S. Zhan},
 journal   = {Chin. Phys. B},
 title     = {Bohmian mechanics to high-order harmonic generation},
 volume    = {19},
 pages     = {020302(1-5)},
 year      = {2010},
}

@article{botheron:PRA:2009,
 author    = {P. Botheron and B. Pons},
 journal   = {Phys. Rev. A},
 title     = {One-electron atom in a strong and short laser pulse: Comparison of classical and quantum descriptions},
 volume    = {80},
 pages     = {023402(1-10)},
 year      = {2009},
}

@article{botheron:PRA-1:2010,
 author    = {P. Botheron and B. Pons},
 journal   = {Phys. Rev. A},
 title     = {Self-consistent Bohmian description of strong field-driven electron dynamics},
 volume    = {82},
 pages     = {021404R(1-4)},
 year      = {2010},
}

@article{botheron:PRA-2:2010,
 author    = {P. Botheron and B. Pons},
 journal   = {Phys. Rev. A},
 title     = {Classical interpretation of probability oscillations in low-energy atomic collisions},
 volume    = {83},
 pages     = {062704(1-11)},
 year      = {2010},
}

@article{takemoto:JCP:2011,
 author    = {N. Takemoto and A. Becker},
 journal   = {J. Chem. Phys.},
 title     = {Visualization and interpretation of attosecond electron dynamics in laser-driven hydrogen molecular ion using Bohmian trajectories},
 volume    = {134},
 pages     = {074309(1-8)},
 year      = {2011},
}

@article{arndt:FoundPhys:2012,
 author    = {T. Juffmann and S. Nimmrichter and M. Arndt and H. Gleiter and K. Hornberger},
 journal   = {Found. Phys.},
 title     = {New prospects for de Broglie interferometry - Grating diffraction in the far-field and Poisson's spot in the near-field},
 volume    = {42},
 pages     = {98-110},
 year      = {2012},
}

@article{arndt:RMP:2012,
 author    = {K. Hornberger and S. Gerlich and P. Haslinger and S. Nimmrichter and M. Arndt},
 journal   = {Rev. Mod. Phys.},
 title     = {Colloquium: Quantum interference of clusters and molecules},
 volume    = {84},
 pages     = {157-173},
 year      = {2012},
}

@article{arndt:NNanotech:2012,
 author    = {T. Juffmann and A. Milic and M. M\"ullneritsch and P. Asenbaum and A. Tsukernik and J. T\"uxen and M. Mayor and O. Cheshnovsky and M. Arndt},
 journal   = {Nat. Nanotech.},
 title     = {Real-time single-molecule imaging of quantum interference},
 volume    = {7},
 pages     = {297-300},
 year      = {2012},
}

@article{carnal:PRL:1991,
 author    = {O. Carnal and J. Mlynek},
 journal   = {Phys. Rev. Lett.},
 title     = {Young's double-slit experiment with atoms: A simple atom interferometer},
 volume    = {66},
 pages     = {2689-2692},
 year      = {1991},
}

@article{cronin:RMP:2009,
 author    = {A. D. Cronin and J. Schmiedmayer and D. E. Pritchard},
 journal   = {Rev. Mod. Phys.},
 title     = {Optics and interferometry with atoms and molecules},
 volume    = {81},
 pages     = {1051-1129},
 year      = {2009},
}

@article{brabec:RMP:2000,
 author    = {Th. Brabec and F. Krausz},
 journal   = {Rev. Mod. Phys.},
 title     = {Intense few-cycle laser fields: Frontiers of nonlinear optics},
 volume    = {72},
 pages     = {545-591},
 year      = {2000},
}

@article{ganeev:JPhysB:2007,
 author    = {R. A. Ganeev},
 journal   = {J. Phys. B: At. Mol. Opt. Phys.},
 title     = {High-order harmonic generation in a laser plasma: a review of recent achievements},
 volume    = {40},
 pages     = {R213-R253},
 year      = {2007},
}

@article{midorikawa:JJAP:2011,
 author    = {K. Midorikawa},
 journal   = {Jpn. J. Appl. Phys.},
 title     = {High-order harmonic generation and attosecond science},
 volume    = {50},
 pages     = {090001(1-12)},
 year      = {2011},
}

@article{corkum:PRL:1993,
 author    = {P. B. Corkum},
 journal   = {Phys. Rev. Lett.},
 title     = {Plasma perspective on strong field multiphoton ionization},
 volume    = {71},
 pages     = {1994-1997},
 year      = {1993},
}

@article{lewenstein:PRA:1994,
 author    = {M. Lewenstein and Ph. Balcou and M. Yu. Ivanov and A. L'Huillier and P. B. Corkum},
 journal   = {Phys. Rev. A},
 title     = {Theory of high-harmonic generation by low-frequency laser fields},
 volume    = {49},
 pages     = {2117-},
 year      = {1994},
}

@article{altucci:JModOpt:2012,
 author    = {C. Altucci and J. W. G. Tisch and R. Velotta},
 journal   = {J. Mod. Opt.},
 title     = {Single attosecond light pulses from multi-cycle laser sources},
 volume    = {58},
 pages     = {1585-1610},
 year      = {2011},
}

@article{aharonov:PRA:1990,
 author    = {Y. Aharonov and L. Vaidman},
 journal   = {Phys. Rev. A},
 title     = {Properties of a quantum system during the time interval between two measurements},
 volume    = {41},
 pages     = {11-20},
 year      = {1990},
}

@article{hiley:JPhysConfSer:2012,
 author    = {B. J. Hiley},
 journal   = {J. Phys.: Conf. Ser.},
 title     = {Weak values: Approach through the Clifford and Moyal algebras},
 volume    = {361},
 pages     = {012014},
 year      = {2012},
}

@article{work-in-progress:2012,
 author    = {A. S. Sanz and J. Wu and B. B. Augstein and C. Figueira de Morisson Faria},
 journal   = {Phys. Rev. A},
 title     = {Quantum-classical correspondence in the high-order harmonic generation},
 volume    = {},
 pages     = {},
 year      = {work in progress, 2012},
}

@article{ghose:PLA:2001,
 author    = {P. Ghose and A. S. Majumdar and S. Guhab and J. Sau},
 journal   = {Phys. Lett. A},
 title     = {Bohmian trajectories for photons},
 volume    = {290},
 pages     = {205-213},
 year      = {2001},
 doi       = {10.1016/S0375-9601(01)00677-6},
 url       = {https://doi.org/10.1016/S0375-9601(01)00677-6},
}

@article{kogelnik:ProcIEEE:1966,
 author    = {H. Kogelnik and T. Li},
 journal   = {Proc. IEEE},
 title     = {Laser beams and resonators},
 volume    = {54},
 pages     = {1312-1329},
 year      = {1966},
}

@article{mukunda:JOSAA:1985,
 author    = {N. Mukunda and R. Simon and E. C. G. Sudarshan},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Fourier optics for the Maxwell field: Formalism and applications},
 volume    = {2},
 pages     = {416-426},
 year      = {1985},
}

@article{mukunda:JOSAA:1986,
 author    = {R. Simon and E. C. G. Sudarshan and N. Mukunda},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Gaussian-Maxwell beams},
 volume    = {3},
 pages     = {536-540},
 year      = {1986},
}

@article{mukunda:ApplOpt:1987,
 author    = {N. Mukunda and R. Simon and E. C. G. Sudarshan},
 journal   = {Appl. Opt.},
 title     = {Cross polarization in laser beams},
 volume    = {26},
 pages     = {1589-1593},
 year      = {1987},
}

@article{seshadri:JOSAA:1998,
 author    = {S. R. Seshadri},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Electromagnetic Gaussian beam},
 volume    = {15},
 pages     = {2712-2719},
 year      = {1998},
}

@article{mcdonald:notes:2000,
 author    = {K. T. McDonald},
 journal   = {Notes},
 title     = {Gaussian laser beams with radial polarization},
 volume    = {},
 pages     = {1-12},
 year      = {2000},
}

@article{mcdonald:notes:2009-1,
 author    = {K. T. McDonald},
 journal   = {Notes},
 title     = {Second-order paraxial Gaussian beam},
 volume    = {},
 pages     = {1-5},
 year      = {2009},
}

@article{mcdonald:notes:2009-2,
 author    = {K. T. McDonald},
 journal   = {Notes},
 title     = {Reflection of a Gaussian optical beam by a flat mirror},
 volume    = {},
 pages     = {1-12},
 year      = {2009},
}

@article{davis:PRA:1979,
 author    = {L. W. Davis},
 journal   = {Phys. Rev. A},
 title     = {Theory of electromagnetic beams},
 volume    = {19},
 pages     = {1177-1179},
 year      = {1979},
}

@article{barnett:PhilTRSA:2010,
 author    = {S. M. Barnett and R. Loudon},
 journal   = {Phil. Trans. R. Soc. A},
 title     = {The enigma of optical momentum in a medium},
 volume    = {368},
 pages     = {927-939},
 year      = {2010},
}

@article{dahmen:AnnPhys:1998,
 author    = {H. D. Dahmen and E. Gjonaj and T. Stroh},
 journal   = {Ann. Phys. (Leipzig)},
 title     = {Quantile motion of electromagnetic waves in wave guides of varying cross section and dispersive media},
 volume    = {7},
 pages     = {645-653},
 year      = {1998},
}

@article{hesse:JQSRT:2008,
 author    = {E. Hesse},
 journal   = {JQSRT},
 title     = {Modelling diffraction during ray tracing using the concept of energy flow lines},
 volume    = {109},
 pages     = {1374-1383},
 year      = {2008},
}

@article{wyatt:PhysScr:2011,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {Phys. Scr.},
 title     = {Hydrodynamic view of electrodynamics: Energy rays and electromagnetic effective stress},
 volume    = {83},
 pages     = {065403(1-10)},
 year      = {2011},
}

@article{sadreev:PRE:2004,
 author    = {A. F. Sadreev},
 journal   = {Phys. Rev. E},
 title     = {Current statistics for transport through rectangular and circular billiards},
 volume    = {70},
 pages     = {016208(1-7)},
 year      = {2004},
}

@article{sadreev:PRB:2012,
 author    = {E. N. Bulgakov and A. F. Sadreev},
 journal   = {Phys. Rev. B},
 title     = {Giant optical vortex in photonic crystal waveguide with nonlinear optical cavity},
 volume    = {85},
 pages     = {165305(1-6)},
 year      = {2012},
}

@article{zakowicz:PRE:2001,
 author    = {W. \.Zakowicz},
 journal   = {Phys. Rev. E},
 title     = {Light rays and imaging in wave optics},
 volume    = {64},
 pages     = {066610(1-14)},
 year      = {2001},
}

@article{wang:PRB:2004,
 author    = {Z. B. Wang and B. S. Luk'yanchuk and M. H. Hong and Y. Lin and T. C. Chong},
 journal   = {Phys. Rev. B},
 title     = {Energy flow around a small particle investigated by classical Mie theory},
 volume    = {70},
 pages     = {035418(1-12)},
 year      = {2004},
}

@article{lee:AppPhysLett:2007,
 author    = {B. J. Lee and K. Park and Z. M. Zhang},
 journal   = {Appl. Phys. Lett.},
 title     = {Energy pathways in nanoscale thermal radiation},
 volume    = {91},
 pages     = {153101(1-3)},
 year      = {2007},
}

@article{godin:JAcoustSocAm:2009,
 author    = {O. A. Godin},
 journal   = {Appl. Phys. Lett.},
 title     = {Wave refraction at an interface: Snell's law versus Chapman's law},
 volume    = {125},
 pages     = {EL117-EL122},
 year      = {2009},
}

@article{gondran:AJP:2010,
 author    = {M. Gondran and A. Gondran},
 journal   = {Am. J. Phys.},
 title     = {Energy flow lines and the spot of Poisson-Arago},
 volume    = {78},
 pages     = {598-602},
 year      = {2010},
}

@article{holland:ProcRSocA:2005,
 author    = {P. Holland},
 journal   = {Proc. R. Soc. A},
 title     = {Hydrodynamic construction of the electromagnetic field},
 volume    = {461},
 pages     = {3659-3679},
 year      = {2005},
}

@article{erikson:PRE:1994,
 author    = {W. L. Erikson and S. Singh},
 journal   = {Phys. Rev. E},
 title     = {Polarization properties of Maxwell-Gaussian laser beams},
 volume    = {49},
 pages     = {5778-5786},
 year      = {1994},
}

@article{varga:OptCommun:1998,
 author    = {P. Varga and P. T\"{o}r\"{o}k},
 journal   = {Opt. Commun.},
 title     = {The Gaussian wave solution of Maxwell's equations and the validity of scalar wave approximation},
 volume    = {152},
 pages     = {108-118},
 year      = {1998},
}

@article{heller:JCP:1975,
 author    = {E. J. Heller},
 journal   = {J. Chem. Phys.},
 title     = {Time-dependent approach to semiclassical dynamics},
 volume    = {62},
 pages     = {1544-1555},
 year      = {1975},
}

@article{heller:JCP:1981,
 author    = {E. J. Heller},
 journal   = {J. Chem. Phys.},
 title     = {Frozen Gaussians: A very simple semiclassical approximation},
 volume    = {75},
 pages     = {2923-2931},
 year      = {1981},
}

@article{caldirola:NuovoCim:1941,
 author    = {P. Caldirola},
 journal   = {Nuovo cim.},
 title     = {Forze non conservative nella meccanica quantistica},
 volume    = {18},
 pages     = {393-400},
 year      = {1941},
}

@article{kanai:ProgTheorPhys:1948,
 author    = {E. Kanai},
 journal   = {Prog. Theor. Phys.},
 title     = {On the quantization of the dissipative systems},
 volume    = {3},
 pages     = {440-442},
 year      = {1948},
}

@article{caldeira:AnnPhys:1983,
 author    = {A. O. Caldeira and A. J. Leggett},
 journal   = {Ann. Phys. (NY)},
 title     = {Quantum tunneling in a dissipative system},
 volume    = {149},
 pages     = {374-456},
 year      = {1983},
}

@article{caldeira:PhysicaA:1983,
 author    = {A. O. Caldeira and A. J. Leggett},
 journal   = {Physica A},
 title     = {Path integral approach to quantum Brownian motion},
 volume    = {121},
 pages     = {587-616},
 year      = {1983},
}

@BOOK{razavy-bk,
  AUTHOR     = {M. Razavy},
  TITLE      = {Classical and Quantum Dissipative Systems},
  PUBLISHER  = {Imperial College Press},
  YEAR       = {2005},
  address    = {London},
}

@BOOK{morse-bk-1,
  AUTHOR     = {P. M. Morse and H. Feshbach},
  TITLE      = {Methods of Theoretical Physics},
  PUBLISHER  = {McGraw-Hill},
  YEAR       = {1953},
  address    = {New York},
  volume     = {1},
}

@BOOK{morse-bk-2,
  AUTHOR     = {P. M. Morse and H. Feshbach},
  TITLE      = {Methods of Theoretical Physics},
  PUBLISHER  = {McGraw-Hill},
  YEAR       = {1953},
  address    = {New York},
  volume     = {2},
}

@article{gouy:CRASP:1890,
 author    = {L. G. Gouy},
 journal   = {C. R. Acad. Sci. Paris},
 title     = {Sur une propri\'et\'e nouvelle des ondes lumineuses},
 volume    = {110},
 pages     = {1251},
 year      = {1890},
}

@article{gouy:CompRend:1890,
 author    = {L. G. Gouy},
 journal   = {Compt. Rendue. Acad. Sci. Paris},
 title     = {Sur la propagation anomale des ondes},
 volume    = {111},
 pages     = {33},
 year      = {1890},
}

@article{gouy:ACOS:1891,
 author    = {L. G. Gouy},
 journal   = {Ann. Chim. Phys. Ser. 6},
 title     = {Sur la propagation anomale des ondes},
 volume    = {24},
 pages     = {145},
 year      = {1891},
}

@article{boyd:JOSA:1980,
 author    = {R. W. Boyd},
 journal   = {J. Opt. Soc. Am.},
 title     = {Intuitive explanation of the phase anomaly of focused light beams},
 volume    = {70},
 pages     = {877-880},
 year      = {1980},
}

@article{rubinowicz:PhysRev:1938,
 author    = {A. Rubinowicz},
 journal   = {Phys. Rev.},
 title     = {On the anomalous propagation of phase in the focus},
 volume    = {54},
 pages     = {931-936},
 year      = {1938},
}

@article{paschotta:OptExpr:2006,
 author    = {R. Paschotta},
 journal   = {Opt. Express},
 title     = {Beam quality deterioration of lasers caused by intracavity beam distortions},
 volume    = {14},
 pages     = {6069-6074},
 year      = {2006},
}

@article{feng:OptLett:2001,
 author    = {S. Feng and H. G. Winful},
 journal   = {Opt. Express},
 title     = {Physical origin of the Gouy phase shift},
 volume    = {26},
 pages     = {485-487},
 year      = {2001},
}

@article{visser:OptCommun:2010,
 author    = {T. D. Visser and E. Wolf},
 journal   = {Opt. Commun.},
 title     = {The origin of the Gouy phase anomaly and its generalization to astigmatic wavefields},
 volume    = {283},
 pages     = {3371-3375},
 year      = {2010},
}

@article{sanz:EPJD:2007,
 author    = {A. S. Sanz and F. Borondo},
 journal   = {Eur. Phys. J. D},
 title     = {A quantum trajectory description of decoherence},
 volume    = {44},
 pages     = {319-326},
 year      = {2007},
 url       = {https://doi.org/10.1140/epjd/e2007-00191-8},
 doi       = {10.1140/epjd/e2007-00191-8},
}

@article{sanz:CPL:2009-2,
 author    = {A. S. Sanz and F. Borondo},
 journal   = {Chem. Phys. Lett.},
 title     = {Contextuality, decoherence and quantum trajectories},
 volume    = {478},
 pages     = {301-306},
 year      = {2009},
 doi       = {10.1016/j.cplett.2009.07.061},
 url       = {https://www.sciencedirect.com/science/article/pii/S0009261409009038},
}

@article{vink:PRA:1993,
 author    = {J. C. Vink},
 journal   = {Phys. Rev. A},
 title     = {Quantum mechanics in terms of discrete beables},
 volume    = {48},
 pages     = {1808-1818},
 year      = {1993},
}

@article{lorenzen:PRA:2009,
 author    = {F. Lorenzen and M. A. de Ponte and M. H. Y. Moussa},
 journal   = {Phys. Rev. A},
 title     = {Extending Bell's beables to encompass dissipation, decoherence, and the quantum-to-classical transition through quantum trajectories},
 volume    = {80},
 pages     = {032101(1-8)},
 year      = {2009},
}

@article{vandyck:JPA:1994,
 author    = {M. A. Vandyck},
 journal   = {J. Phys. A: Math. Gen.},
 title     = {On the damped harmonic oscillator in the de Broglie-Bohm hidden-variable theory},
 volume    = {27},
 pages     = {1743-1750},
 year      = {1994},
}

@article{shojai:PRAMANA:2004,
 author    = {F. Shojai and A. Shojai},
 journal   = {PRAMANA},
 title     = {On the Bohmian quantum friction},
 volume    = {62},
 pages     = {803-814},
 year      = {2004},
}

@article{tilbi:PhysScr:2007,
 author    = {A. Tilbi and T. Boudjedaa and M. Merad and L. Chetouani},
 journal   = {Phys. Scr.},
 title     = {The Kanai-Caldirola propagator in the de Broglie-Bohm theory},
 volume    = {75},
 pages     = {474-479},
 year      = {2007},
}

@article{garashchuk:JCP:2013,
 author    = {S. Garashchuk and V. Dixit and B. Gu and J. Mazzuca},
 journal   = {J. Chem. Phys.},
 title     = {The Schr\"odinger equation with friction from the quantum trajectory perspective},
 volume    = {138},
 pages     = {054107(1-7)},
 year      = {2013},
}

@article{garashchuk:TheorChemAcc:2012,
 author    = {S. Garashchuk},
 journal   = {Theor. Chem. Acc.},
 title     = {Calculation of the zero-point energy from imaginary-time quantum trajectory dynamics in Cartesian coordinates},
 volume    = {131},
 pages     = {1083(1-10)},
 year      = {2012},
}

@article{bowman:JCP:2011,
 author    = {G. Czak\'o and Y. Wang and J. M. Bowman},
 journal   = {J. Chem. Phys.},
 title     = {Communication: Quasiclassical trajectory calculations of correlated product-state distributions for the dissociation of (H$_2$O)$_2$ and (D$_2$O)$_2$},
 volume    = {135},
 pages     = {151102(1-4},
 year      = {2011},
}

@BOOK{weiss-bk,
  AUTHOR     = {U. Weiss},
  TITLE      = {Quantum Dissipative Systems},
  PUBLISHER  = {World Scientific},
  YEAR       = {1999},
  address    = {Singapore},
}

@article{hakim:prl:1985,
 author    = {F. Guinea and V. Hakim and A. Muramatsu},
 journal   = {Phys. Rev. Lett.},
 title     = {Diffusion and localization of a particle in a periodic potential coupled to a dissipative environment},
 volume    = {54},
 pages     = {263-266},
 year      = {1985},
}

@article{fisher:prb:1985,
 author    = {M. P. A. Fisher and W. Zwerger},
 journal   = {Phys. Rev. B},
 title     = {Quantum Brownian motion in a periodic potential},
 volume    = {32},
 pages     = {6190-6206},
 year      = {1985},
}

@article{zurek:prd:1989,
 author    = {W. G. Unruh and W. H. Zurek},
 journal   = {Phys. Rev. D},
 title     = {Reduction of a wave packet in quantum Brownian motion},
 volume    = {40},
 pages     = {1071-1094},
 year      = {1989},
}

@article{doebner:pla:1992,
 author    = {H.-D. Doebner and G. A. Goldin},
 journal   = {Phys. Lett. A},
 title     = {On a general nonlinear Schr\"odinger equation admitting diffusion currents},
 volume    = {162},
 pages     = {397-401},
 year      = {1992},
}

@article{kostin:jcp:1972,
 author    = {M. D. Kostin},
 journal   = {J. Chem. Phys.},
 title     = {On the Schr\"odinger-Langevin equation},
 volume    = {57},
 pages     = {3589-3591},
 year      = {1972},
}

@article{kochan:pra:2010,
 author    = {D. Kochan},
 journal   = {Phys. Rev. A},
 title     = {Functional integral for non-Lagrangian systems},
 volume    = {81},
 pages     = {022112(1-13)},
 year      = {2010},
}

@article{bateman:PhysRev:1931,
 author    = {H. Bateman},
 journal   = {Phys. Rev.},
 title     = {On dissipative systems and related variational principles},
 volume    = {38},
 pages     = {815-819},
 year      = {1931},
}

@article{brittin:PhysRev:1950,
 author    = {W. E. Brittin},
 journal   = {Phys. Rev.},
 title     = {A note on the quantization of dissipative systems},
 volume    = {77},
 pages     = {396-397},
 year      = {1950},
}

@article{senitzky:PhysRev:1960,
 author    = {I. R. Senitzky},
 journal   = {Phys. Rev.},
 title     = {Dissipation in quantum mechanics. The harmonic oscillator},
 volume    = {119},
 pages     = {670-679},
 year      = {1960},
}

@article{greenberger:JMathPhys:1979,
 author    = {D. M. Greenberger},
 journal   = {J. Math. Phys.},
 title     = {A critique of the major approaches to damping in quantum theory},
 volume    = {20},
 pages     = {762-770},
 year      = {1979},
}

@article{cavalcanti:PRE:1998,
 author    = {R. M. Cavalcanti},
 journal   = {Phys. Rev. E},
 title     = {Wave function of a Brownian particle},
 volume    = {58},
 pages     = {6807-6809},
 year      = {1998},
}

@article{hasse:JMathPhys:1975,
 author    = {R. W. Hasse},
 journal   = {J. Math. Phys.},
 title     = {On the quantum mechanical treatment of dissipative systems},
 volume    = {16},
 pages     = {2005-2011},
 year      = {1975},
}

@article{holst:PRA:2009,
 author    = {T. Resinger and A. A. Patel and H. Reingruber and K. Fladischer and W. E. Ernst and G. Bracco and H. I. Smith and B. Holst},
 journal   = {Phys. Rev. A},
 title     = {Poisson's spot with molecules},
 volume    = {79},
 pages     = {053823(1-4)},
 year      = {2009},
}

@article{holst:PRA:2012,
 author    = {T. Resinger and M. M. Greve and S. D. Eder and G. Bracco and B. Holst},
 journal   = {Phys. Rev. A},
 title     = {Brightness and virtual source size of a supersonic deuterium beam},
 volume    = {86},
 pages     = {043804(1-10)},
 year      = {2012},
}

@article{holst:NJP:2011,
 author    = {T. Resinger and G. Bracco and B. Holst},
 journal   = {New J. Phys},
 title     = {Particle-wave discrimination in Poisson spot experiments},
 volume    = {13},
 pages     = {065016(1-13)},
 year      = {2011},
}

@INBOOK{joos:bk:1996,
  AUTHOR =       {E. Joos},
  editor =       {D. Giulini and E. Joos and C. Kiefer and J. Kupsch and I.-O. Stamatescu and H. D. Zeh},
  TITLE =        {Decoherence and the Appearance of a Classical World in Quantum Theory},
  CHAPTER =      {Decoherence through interaction with the environment},
  pages =        {41-180},
  PUBLISHER =    {Springer},
  YEAR =         {1996},
  address =      {Berlin},
  edition =      {2nd},
}

@BOOK{giulini-bk,
  AUTHOR     = {D. Giulini and E. Joos and C. Kiefer and J. Kupsch and I.-O. Stamatescu and H. D. Zeh},
  TITLE      = {Decoherence and the Appearance of a Classical World in Quantum Theory},
  PUBLISHER  = {Springer},
  YEAR       = {Berlin},
  address    = {1996},
  edition    = {2nd},
}

@BOOK{schlosshauer-bk:2007,
  AUTHOR     = {M. Schlosshauer},
  TITLE      = {Decoherence and the Quantum-to-Classical Transition},
  PUBLISHER  = {Springer},
  YEAR       = {2007},
  address    = {Berlin},
}

@article{miller:JCP-1:2001,
 author    = {H. Wang and M. Thoss and K. L. Sorge and R. Gelabert and X. Gim\'enez and W. H. Miller},
 journal   = {J. Chem. Phys.},
 title     = {Semiclassical description of quantum coherence effects and their quenching: A forward-backward initial value representation study},
 volume    = {114},
 pages     = {2562-2571},
 year      = {2001},
}

@article{miller:JCP-2:2001,
 author    = {R. Gelabert and X. Gim\'enez and M. Thoss and H. Wang and W. H. Miller},
 journal   = {J. Chem. Phys.},
 title     = {Semiclassical description of diffraction and its quenching by the forward-backward version of the initial value representation},
 volume    = {114},
 pages     = {2572-2579},
 year      = {2001},
}

@article{miller:JCP:2012,
 author    = {W. H. Miller},
 journal   = {J. Chem. Phys.},
 title     = {Perspective: Quantum or classical decoherence?},
 volume    = {136},
 pages     = {210901(1-6)},
 year      = {2012},
}

@article{miller:JCP:1970,
 author    = {W. H. Miller},
 journal   = {J. Chem. Phys.},
 title     = {Classical $S$ matrix: Numerical application to inelastic collisions},
 volume    = {53},
 pages     = {3578-3587},
 year      = {1970},
}

@article{miller:FaradayDiscuss:1998,
 author    = {W. H. Miller},
 journal   = {Faraday Discuss.},
 title     = {Quantum and semiclassical theory of chemical reaction rates},
 volume    = {110},
 pages     = {1-21},
 year      = {1998},
}

@article{caldeira:Physica:1983,
 author    = {A. O. Caldeira and A. J. Leggett},
 journal   = {Physica},
 title     = {Path integral approach to quantum Brownian motion},
 volume    = {121A},
 pages     = {587-616},
 year      = {1983},
}

@article{caldeira:AnnPhys:1983,
 author    = {A. O. Caldeira and A. J. Leggett},
 journal   = {Ann. Phys},
 title     = {Quantum tunnelling in a dissipative system},
 volume    = {149},
 pages     = {374-456},
 year      = {1983},
}

@article{caldeira:AnnPhys:1984,
 author    = {A. O. Caldeira and A. J. Leggett},
 journal   = {Ann. Phys.},
 title     = {Erratum to `Quantum tunnelling in a dissipative system'},
 volume    = {153},
 pages     = {445},
 year      = {1984},
}

@BOOK{percival-bk,
  AUTHOR     = {I. C. Percival},
  TITLE      = {Quantum State Diffusion},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {1998},
  address    = {Cambridge},
}

@article{gisin:JPA:1992,
 author    = {N. Gisin and I. C. Percival},
 journal   = {J. Phys. A},
 title     = {The quantum-state diffusion model applied to open systems},
 volume    = {25},
 pages     = {5677-5691},
 year      = {1992},
}

@article{gisin:JPA:1993,
 author    = {N. Gisin and I. C. Percival},
 journal   = {J. Phys. A},
 title     = {The quantum state diffusion picture of physical processes},
 volume    = {26},
 pages     = {2245-2260},
 year      = {1993},
}

@article{gisin:JModOpt:1993,
 author    = {N. Gisin and P. L. Knight and I. C. Percival and R. C. Thompson and D. C. Wilson},
 journal   = {J. Mod. Opt.},
 title     = {Quantum state diffusion theory and a quantum jump experiment},
 volume    = {40},
 pages     = {1663-1671},
 year      = {1993},
}

@BOOK{ito-bk,
  AUTHOR     = {K. It\^o},
  TITLE      = {Foundations of Stochastic Differential Equations in Infinite Dimensional Spaces},
  PUBLISHER  = {SIAM},
  YEAR       = {1984},
  address    = {Philadelphia, PA},
}

@BOOK{ikeda-bk,
  AUTHOR     = {N. Ikeda and S. Watanabe},
  TITLE      = {Stochastic Differential Equations and Diffusion Processes},
  PUBLISHER  = {North-Holland},
  YEAR       = {Amsterdam},
  address    = {1989},
  edition    = {2nd},
}

@article{diosi:JPA:1988,
 author    = {L. Di\'osi},
 journal   = {J. Phys. A},
 title     = {Quantum stochastic processes as models for state vector reduction},
 volume    = {21},
 pages     = {2885-2898},
 year      = {1988},
}

@article{diosi:PLA:1988,
 author    = {L. Di\'osi},
 journal   = {Phys. Lett. A},
 title     = {Continuous quantum measurement and It\^o formalism},
 volume    = {129},
 pages     = {419-423},
 year      = {1988},
}

@article{diosi:ChemPhys:2001,
 author    = {H. M. Wiseman and L. Di\'osi},
 journal   = {Chem. Phys.},
 title     = {Complete parameterization, and invariance, of diffusive quantum trajectories for Markovian open systems},
 volume    = {268},
 pages     = {91-104},
 year      = {2001},
}

@BOOK{accardi-bk,
  AUTHOR     = {L. Accardi and Y. G. Lu and I. Volovich},
  TITLE      = {Quantum Theory and its Stochastic Limit},
  PUBLISHER  = {Springer},
  YEAR       = {2002},
  address    = {Berlin},
}

@BOOK{NumRecipes-bk,
  AUTHOR     = {W. H. Press and S. A. Teukolsky and W. T. Vetterling and B. P. Flannery},
  TITLE      = {Numerical Recipes: The Art of Scientific Computing},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {2007},
  address    = {New York},
  edition    = {3rd},
}

\bibitem{Prezhdo}
 O.V. Prezhdo, Phys. Rev. Lett. {\bf 85}, 4413 (2000).

\bibitem{Han}
 H. Han and P. Brumer, J. Chem. Phys. {\bf 122}, 144316 (2005).


@article{brumer-gong:PRE:1999,
 author    = {J. Gong and P. Brumer},
 journal   = {Phys. Rev. E},
 title     = {Decoherence and correspondence in conservative chaotic dynamics},
 volume    = {60},
 pages     = {1643-1647},
 year      = {1999},
}

@article{prezhdo:PRL:2000,
 author    = {O. V. Prezhdo},
 journal   = {Phys. Rev. Lett.},
 title     = {Quantum anti-Zeno acceleration of a chemical reaction},
 volume    = {85},
 pages     = {4413-4417},
 year      = {2000},
}

@article{brumer-han:JCP:2005,
 author    = {H. Han and P. Brumer},
 journal   = {J. Chem. Phys.},
 title     = {Decoherence effects in reactive scattering},
 volume    = {122},
 pages     = {144316(1-8)},
 year      = {2005},
}

@article{klauder:SIAM:1985,
 author    = {J. R. Klauder and W. P. Petersen},
 journal   = {SIAM J. Numer. Anal.},
 title     = {Numerical integration of multiplicative-noise stochastic differential equations},
 volume    = {22},
 pages     = {1153-1166},
 year      = {1985},
}

@BOOK{carmichael-bk,
  AUTHOR     = {H. Carmichael},
  TITLE      = {An Open Systems Approach to Quantum Optics},
  PUBLISHER  = {Springer},
  YEAR       = {1993},
  address    = {Berlin},
}

@article{sanz:PRE:2012,
 author    = {A. S. Sanz and Y. Elran and P. Brumer},
 journal   = {Phys. Rev. E},
 title     = {Temperature crossover of decoherence rates in chaotic and regular bath dynamics},
 volume    = {85},
 pages     = {036218(1-6)},
 year      = {2012},
}

@article{brumer-elran:JCP:2013,
 author    = {Y. Elran and P. Brumer},
 journal   = {J. Chem. Phys.},
 title     = {Quantum decoherence of I$_2$ in liquid xenon: A classical Wigner approach},
 volume    = {138},
 pages     = {234308(1-11)},
 year      = {2013},
}

@article{brumer-elran:JCP:2004,
 author    = {Y. Elran and P. Brumer},
 journal   = {J. Chem. Phys.},
 title     = {Decoherence in an anharmonic oscillator coupled to a thermal environment: A semiclassical forward-backward approach},
 volume    = {121},
 pages     = {2673-2684},
 year      = {2004},
}

@article{joos-zeh:ZPhysB:1985,
 author    = {E. Joos and H. D. Zeh},
 journal   = {Z. Phys. B},
 title     = {The emergence of classical properties through interaction with the environment},
 volume    = {59},
 pages     = {223-243},
 year      = {1985},
}

@article{muendel:ChemPhys:1986,
 author    = {C. M\"undel and W. Domcke},
 journal   = {Chem. Phys.},
 title     = {Analytic expression for the matrix elements of the Morse Green function with Morse wavefunctions},
 volume    = {105},
 pages     = {137-143},
 year      = {1989},
}

@article{morse:PhysRev:1929,
 author    = {P. M. Morse},
 journal   = {Phys. Rev.},
 title     = {Diatomic molecules according to the wave mechanics. II. Vibrational levels},
 volume    = {34},
 pages     = {57-64},
 year      = {1929},
 doi       = {10.1103/PhysRev.34.57},
}

@article{zurek:PRL:1993,
 author    = {W. H. Zurek and S. Habib and J. P. Paz},
 journal   = {Phys. Rev. Lett.},
 title     = {Coherent states via decoherence},
 volume    = {70},
 pages     = {1187-1190},
 year      = {1993},
}

@article{sanz:JCP:2006,
 author    = {A. S. Sanz and H. Han and P. Brumer},
 journal   = {J. Chem. Phys.},
 title     = {Aspects of quantum coherence in the optical Bloch equations},
 volume    = {124},
 pages     = {214106(1-7)},
 year      = {2006},
}

@article{pollak:JCP:2009,
 author    = {E. Pollak and S. Miret-Art\'es},
 journal   = {J. Chem. Phys.},
 title     = {Classical theory for the in-plane scattering of atoms from corrugated surfaces: Application to the Ar-Ag(111) system},
 volume    = {130},
 pages     = {194710(1-13},
 year      = {2009},
}

@article{pollak:PRL:2010,
 author    = {J. M. Moix and E. Pollak and S. Miret-Art\'es},
 journal   = {Phys. Rev. Lett.},
 title     = {Friction-induced energy-loss rainbows in atom surface scattering},
 volume    = {104},
 pages     = {116103(1-4},
 year      = {2010},
}

@article{hornberger:PRL:2003,
 author    = {K. Hornberger and S. Uttenthaler and B. Brezger and L. Hackerm\"uller and M. Arndt and A. Zeilinger},
 journal   = {Phys. Rev. Lett.},
 title     = {Collisional decoherence observed in matter-wave interferometry},
 volume    = {90},
 pages     = {160401(1-4)},
 year      = {2003},
}

@article{fischbach:PRA:2012,
 author    = {J. Fischbach and M. Freyberger},
 journal   = {Phys. Rev. A},
 title     = {Quantum optical reconstruction scheme using weak values},
 volume    = {86},
 pages     = {052110(1-8)},
 year      = {2012},
}

@article{bliokh:NewJPhys:2013,
 author    = {K. Y. Bliokh and A. Y. Bekshaev and A. G. Kofman and F. Nori},
 journal   = {New J. Phys.},
 title     = {Photon trajectories, anomalous velocities and weak measurements: a classical interpretation},
 volume    = {15},
 pages     = {073022(1-17)},
 year      = {2013},
}

@article{schleich:PRA:2013,
 author    = {W. P. Schleich and M. Freyberger and M. S. Zubairy},
 journal   = {Phys. Rev. A},
 title     = {Reconstruction of Bohm trajectories and wave functions from interferometric measurements},
 volume    = {87},
 pages     = {014102(1-4)},
 year      = {2013},
}

@article{matzkin:PRL:2012,
 author    = {A. Matzkin},
 journal   = {Phys. Rev. Lett.},
 title     = {Observing trajectories with weak measurements in quantum systems in the semiclassical regime},
 volume    = {109},
 pages     = {150407(1-4)},
 year      = {2012},
}

@article{luis:PRA:2013,
 author    = {A. Luis and A. S. Sanz},
 journal   = {Phys. Rev. A},
 title     = {Reconciling quantum trajectories and stationary quantum distributions in single-photon polarization states},
 volume    = {87},
 pages     = {063844(1-8)},
 year      = {2013},
}

@article{lundeen:Nature:2011,
 author    = {J. S. Lundeen and B. Sutherland and Aabid Patel and C. Stewart and Ch. Bamber},
 journal   = {Nature},
 title     = {Direct measurement of the quantum wavefunction},
 volume    = {474},
 pages     = {188-191},
 year      = {2011},
}

@article{aharonov:PRL:1988,
 author    = {Y. Aharonov and D. Z. Albert and L. Vaidman},
 journal   = {Phys. Rev. Lett.},
 title     = {How the result of a measurement of a component of the spin of a spin$-$$\frac{1}{2}$ particle can turn out to be 100},
 volume    = {60},
 pages     = {1351-1354},
 year      = {1988},
}

@article{dressel:RMP:2013,
 author    = {J. Dressel and M. Malik and F. M. Miatto and A. N. Jordan and R. W. Boyd},
 journal   = {Rev. Mod. Phys.},
 title     = {Colloquium: Understanding quantum weak values: Basics and applications},
 volume    = {86},
 pages     = {307-316},
 year      = {2014},
}

@article{wiseman:NewJPhys:2007,
 author    = {H. M. Wiseman},
 journal   = {New J. Phys.},
 title     = {Grounding Bohmian mechanics in weak values and bayesianism},
 volume    = {9},
 pages     = {165(1-12)},
 year      = {2007},
}

@article{mir:NewJPhys:2007,
 author    = {R. Mir and J. S. Lundeen and M. W. Mitchell and A. M. Steinberg and J. L. Garretson and H. M. Wiseman},
 journal   = {New J. Phys.},
 title     = {A double-slit `which-way' experiment on the complementarity-uncertainty debate},
 volume    = {9},
 pages     = {287(1-11)},
 year      = {2007},
}

@article{hirschfelder:JCP:1978,
 author    = {J. O. Hirschfelder},
 journal   = {J. Chem. Phys.},
 title     = {Quantum mechanical equations of change. I},
 volume    = {68},
 pages     = {5151-5162},
 year      = {1978},
}

@article{leavens:FoundPhys:2005,
 author    = {C. R. Leavens},
 journal   = {Found. Phys.},
 title     = {Weak measurements from the point of view of Bohmian mechanics},
 volume    = {35},
 pages     = {469-491},
 year      = {2005},
}

@article{sanz:PhysScr:2013,
 author    = {M. Davidovi\'c and A. S. Sanz and M. Bo\v{z}i\'c and D. Arsenovi\'c and D. Dimi\'c},
 journal   = {Phys. Scr.},
 pages     = {014015(1-5)},
 title     = {Trajectory-based interpretation of Young's experiment, the Arago-Fresnel laws and the Poisson-Arago spot for photons and massive particles},
 volume    = {T153},
 year      = {2013},
 }

@article{ritchie:PRL:1991,
 author    = {N. W. M. Ritchie and J. G. Story and R. G. Hulet},
 journal   = {Phys. Rev. Lett.},
 title     = {Realization of a measurement of a ``weak value''},
 volume    = {66},
 pages     = {1107-1110},
 year      = {1991},
}

@article{bamber:PRL:2012,
 author    = {J. S. Lundeen and Ch. Bamber},
 journal   = {Phys. Rev. Lett.},
 title     = {Procedure for direct measurement of general quantum states using weak measurements},
 volume    = {108},
 pages     = {070402(1-5)},
 year      = {2012},
}

@article{bamber:PRL:2013,
 author    = {Ch. Bamber and J. S. Lundeen},
 journal   = {Phys. Rev. Lett.},
 title     = {Observing Dirac's classical phase space analog to the quantum state},
 volume    = {112},
 pages     = {070405(1-6)},
 year      = {2014},
}

@article{grossmann:JCP:2009,
 author    = {Ch.-M. Goletz and F. Grossmann},
 journal   = {J. Chem. Phys.},
 title     = {Decoherence and dissipation in a molecular system coupled to an environment: An application of semiclassical hybrid dynamics},
 volume    = {130},
 pages     = {244107(1-12)},
 year      = {2009},
}

@article{deMarcus:AJ:1978,
 author    = {W. C. DeMarcus},
 journal   = {Am. J. Phys.},
 title     = {Classical motion of a Morse oscillator},
 volume    = {46},
 pages     = {733-734},
 year      = {1978},
}

@article{braverman:PRL:2013,
  title = {Proposal to Observe the Nonlocality of Bohmian Trajectories with Entangled Photons},
  author = {Braverman, Boris and Simon, Christoph},
  journal = {Phys. Rev. Lett.},
  volume = {110},
  issue = {6},
  pages = {060406},
  numpages = {5},
  year = {2013},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.110.060406},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.110.060406}
}

@article{young:PTRSL:1804,
 author    = {T. Young},
 journal   = {Phil. Trans. R. Soc. Lond.},
 title     = {The Bakerian Lecture. Experimentas and calculations relative to physical optics},
 volume    = {94},
 pages     = {1-16},
 year      = {1804},
}

@BOOK{young:1807,
  AUTHOR     = {T. Young},
  editor     = {W. Savage},
  TITLE      = {A Course of Lectures on Natural Philosophy and the Mechanical Arts},
  PUBLISHER  = {Joseph Johnson},
  YEAR       = {1807},
  address    = {London},
}

@BOOK{feynman:FLP3:1965,
  AUTHOR     = {R. P. Feynman and R. B. Leighton and M. Sands},
  TITLE      = {The Feynman Lectures on Physics},
  PUBLISHER  = {Addison-Wesley},
  YEAR       = {1965},
  volume     = {3},
  address    = {Reading, MA},
}

@BOOK{lipson-bk:2011,
  AUTHOR     = {A. Lipson and S. G. Lipson and H. Lipson},
  TITLE      = {Optical Physics},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {2011},
  address    = {New York},
  edition    = {4th},
}

@BOOK{hecht-bk:2002,
  AUTHOR     = {E. Hecht},
  TITLE      = {Optics},
  PUBLISHER  = {Addison-Wesley Longman},
  YEAR       = {2002},
  address    = {New York},
  edition    = {4th},
}

@article{bohr100-1:2013,
 author    = {News Feature},
 journal   = {Nature},
 title     = {Quantum physics: The quantum atom},
 volume    = {498},
 pages     = {21},
 year      = {6 June 2013},
 source    = {},
}

@article{bohr100-2:2013,
 author    = {Special Issue},
 journal   = {Nature},
 title     = {The quantum atom},
 volume    = {498},
 pages     = {},
 year      = {6 June 2013},
 source    = {www.nature.com/bohr100},
}

@article{forman:HistStud:1971,
 author    = {P. Forman},
 journal   = {Hist. Stud. Phys. Sci.},
 title     = {Weimar Culture, Causality, and Quantum Theory, 1918-1927: Adaptation by German Physicists and Mathematicians to a Hostile Intellectual Environment},
 volume    = {3},
 pages     = {1-115},
 year      = {1971},
}

@BOOK{jammer-bk:1966,
  AUTHOR     = {M. Jammer},
  TITLE      = {The Conceptual Development of Quantum Mechanics},
  PUBLISHER  = {McGraw-Hill},
  YEAR       = {1966},
  address    = {New York},
}

@article{mermin:PhysToday:1989,
 author    = {N. D. Mermin},
 journal   = {Physics Today},
 title     = {What's wrong with this pillow?},
 volume    = {42},
 number    = {4},
 pages     = {9-11},
 year      = {1989},
}

@article{mermin:PhysToday:2004,
 author    = {N. D. Mermin},
 journal   = {Physics Today},
 title     = {Could Feynman have said this?},
 volume    = {57},
 number    = {5},
 pages     = {10-11},
 year      = {2004},
}

@article{broglie:CompRend-2:1926,
 author    = {L. de Broglie},
 journal   = {Comptes Rendus},
 title     = {Sur la possibilit\'e de relier les ph\'enom\`enes d'interf\'erence et de diffraction \'a la th\'eorie des quanta de lumie\`ere},
 volume    = {183},
 pages     = {447-448},
 year      = {1926},
}

@article{broglie:CompRend-1:1926,
 author    = {L. de Broglie},
 journal   = {Comptes Rendus},
 title     = {Rermarques sur la nouvelle M\'ecanique ondulatoire},
 volume    = {183},
 pages     = {272-274},
 year      = {1926},
}

@article{schrodinger:PhysRev:1926,
 author    = {E. Schr\"odinger},
 journal   = {Phys. Rev.},
 title     = {An undulatory theory of the mechanics of atoms and molecules},
 volume    = {28},
 pages     = {1049-1070},
 year      = {1926},
}

@article{waterhouse:JASA:1985,
 author    = {R. V. Waterhouse and T. W. Yates and D. Feit and Y. N. Liu},
 journal   = {J. Acoust. Soc. Am.},
 title     = {Energy streamlines of a sound source},
 volume    = {78},
 pages     = {758-762},
 year      = {1985},
}

@article{waterhouse:JASA:1986-1,
 author    = {R. V. Waterhouse and D. Feit},
 journal   = {J. Acoust. Soc. Am.},
 title     = {Equal-energy streamlines},
 volume    = {80},
 pages     = {681-684},
 year      = {1986},
}

@article{waterhouse:JASA:1986-2,
 author    = {E. A. Skelton and R. V. Waterhouse},
 journal   = {J. Acoust. Soc. Am.},
 title     = {Energy streamlines for a spherical shell scattering plane wave},
 volume    = {80},
 pages     = {1473-1478},
 year      = {1986},
}

@article{waterhouse:JASA:1987-1,
 author    = {R. V. Waterhouse and D. G. Crighton and J. E. Ffowcs-Williams},
 journal   = {J. Acoust. Soc. Am.},
 title     = {A criterion for an energy vortex in a sound field},
 volume    = {81},
 pages     = {1323-1326},
 year      = {1987},
}

@article{waterhouse:JASA:1987-2,
 author    = {R. V. Waterhouse},
 journal   = {J. Acoust. Soc. Am.},
 title     = {Vortex modes in rooms},
 volume    = {82},
 pages     = {1782-1791},
 year      = {1987},
}

@article{lazzeretti:CPL:1981,
 author    = {P. Lazzeretti and R. Zanasi},
 journal   = {Chem. Phys. Lett.},
 title     = {Inconsistency of the ring-current model for the cyclopropenyl cation},
 volume    = {80},
 pages     = {533-536},
 year      = {1981},
}

@article{lazzeretti:IJQC:1984,
 author    = {P. Lazzeretti and E. Rossi and R. Zanasi},
 journal   = {Int. J. Quantum Chem.},
 title     = {Singularities of magnetic-field induced electron current density: A study of the ethylene molecule},
 volume    = {25},
 pages     = {929-940},
 year      = {1984},
}

@article{lazzeretti:PNMRS:2000,
 author    = {P. Lazzeretti},
 journal   = {Prog. Nucl. Magn. Reson. Spect.},
 title     = {Righ currents},
 volume    = {36},
 pages     = {1-88},
 year      = {2000},
}

@article{lazzeretti:IJQC:2011,
 author    = {S. Pelloni and P. Lazzeretti},
 journal   = {Int. J. Quantum Chem.},
 title     = {Stagnation graphs and topological models of magnetic-field induced electron current density for some small molecules in connection with their magnetic symmetry},
 volume    = {111},
 pages     = {356-367},
 year      = {2011},
}

@article{gomes:JCP:1983-1,
 author    = {J. A. N. F. Gomes},
 journal   = {J. Chem. Phys.},
 title     = {Delocalized magnetic currents in benzene},
 volume    = {78},
 pages     = {3133-3139},
 year      = {1983},
}

@article{gomes:JCP:1983-2,
 author    = {J. A. N. F. Gomes},
 journal   = {J. Chem. Phys.},
 title     = {Topological elements of the magnetically induced orbital current densities},
 volume    = {78},
 pages     = {4585-4591},
 year      = {1983},
}

@article{berger:AngewChem:2010,
 author    = {R. J. F. Berger and H. S. Rzepa and D. Scheschkewitz},
 journal   = {Angew. Chem. Int. Ed.},
 title     = {Ring currents in the dismutational aromatic Si$_6$R$_6$},
 volume    = {49},
 pages     = {10006-10009},
 year      = {2010},
}

@article{braunbek:Optik:1952,
 author    = {W. Braunbek and G. Laukien},
 journal   = {Optik},
 title     = {Features of refraction by a semi-plane},
 volume    = {9},
 pages     = {174-179},
 year      = {1952},
}

@article{sommerfeld:MathAnn:1896,
 author    = {A. Sommerfeld},
 journal   = {Math. Ann.},
 title     = {Theorie der diffraction},
 volume    = {47},
 pages     = {317-374},
 year      = {1896},
}

@article{sanz:JPhysConfSer:2012,
 author    = {A. S. Sanz},
 journal   = {J. Phys.: Conf. Ser.},
 title     = {Quantumness beyond quantum mechanics},
 volume    = {361},
 pages     = {012016(1-11)},
 year      = {2012},
}

@article{sanz:EPN:2013,
 author    = {M. Davidovi\'c and A. S. Sanz},
 journal   = {Europhys. News},
 title     = {How does light move? Determining the flow of light without destroying interference},
 volume    = {44},
 number    = {6},
 pages     = {33-36},
 year      = {2013},
 doi       = {10.1051/epn/2013604},
 url       = {https://doi.org/10.1051/epn/2013604},
}

@article{takabayasi:ProgTheorPhys:1952,
 author    = {T. Takabayasi},
 journal   = {Prog. Theor. Phys.},
 title     = {On the formulation of quantum mechanics associated with classical pictures},
 volume    = {8},
 pages     = {143-182},
 year      = {1952},
 doi       = {10.1143/ptp/8.2.143},
 url       = {https://academic.oup.com/ptp/article/8/2/143/1883374}
}

@article{takabayasi:ProgTheorPhys:1953,
 author    = {T. Takabayasi},
 journal   = {Prog. Theor. Phys.},
 title     = {Remarks on the formulation of quantum mechanics with classical pictures and on relations between linear scalar fields and hydrodynamical fields},
 volume    = {9},
 pages     = {187-222},
 year      = {1953},
}

@article{takabayasi:ProgTheorPhys:1983,
 author    = {T. Takabayasi},
 journal   = {Prog. Theor. Phys.},
 title     = {Hydrodynamical formalism of quantum mechanics and Aharonov-Bohm effect},
 volume    = {69},
 pages     = {1323-1344},
 year      = {1983},
}

@article{mccullough:JCP:1969,
 author    = {E. A. McCullough and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Quantum dynamics of the collinear (H,H$_2$) reaction},
 volume    = {51},
 pages     = {1253-1254},
 year      = {1969},
}

@article{mccullough:JCP:1971-1,
 author    = {E. A. McCullough and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Dynamics of the collinear H+H$_2$ reaction. I. Probability density and flux},
 volume    = {54},
 pages     = {3578-3591},
 year      = {1971},
}

@article{mccullough:JCP:1971-2,
 author    = {E. A. McCullough and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Dynamics of the collinear H+H$_2$ reaction. II. Energy analysis},
 volume    = {54},
 pages     = {3592-3600},
 year      = {1971},
}

@article{dewdney:NuovoCimB:1979,
 author    = {C. Philippidis and C. Dewdney and B. J. Hiley},
 journal   = {Nuovo Cimento},
 title     = {Quantum interference and the quantum potential},
 volume    = {52B},
 pages     = {15--28},
 year      = {1979},
 doi       = {https://doi.org/10.1007/BF02743566},
 url       = {https://link.springer.com/article/10.1007/BF02743566}
}

@BOOK{courant-hilbert-bk-1,
  AUTHOR     = {R. Courant and D. Hilbert},
  TITLE      = {Methods of Mathematical Physics},
  PUBLISHER  = {John Wiley \& Sons},
  YEAR       = {1966},
  address    = {New York},
  volume     = {1},
}

@BOOK{courant-hilbert-bk-2,
  AUTHOR     = {R. Courant and D. Hilbert},
  TITLE      = {Methods of Mathematical Physics},
  PUBLISHER  = {John Wiley \& Sons},
  YEAR       = {1966},
  address    = {New York},
  volume     = {2},
}

@article{chevalerias:JOSA:1957,
 author    = {R. Chevalerias and Y. Latron and C. Veret},
 journal   = {J. Opt. Soc. Am.},
 title     = {Methods of interferometry applied to the visualization of flows in wind tunnels},
 volume    = {47},
 pages     = {703-706},
 year      = {1957},
}

@BOOK{hughes-bk,
  editor     = {K. H. Hughes and G. Parlant},
  TITLE      = {Quantum Trajectories},
  PUBLISHER  = {CCP6},
  YEAR       = {2011},
  address    = {Daresbury, UK},
}

@BOOK{sanz:CCP6:2011,
  AUTHOR     = {A. S. Sanz},
  editor     = {K. H. Hughes and G. Parlant},
  TITLE      = {Quantum Trajectories},
  CHAPTER    = {An account on quantum interference from a hydrodynamical perspective},
  pages      = {111-115},
  PUBLISHER  = {CCP6},
  YEAR       = {2011},
  address    = {Daresbury, UK},
}

@article{sanz:CJC:2014,
 author    = {A. S. Sanz},
 journal   = {Can. J. Chem.},
 title     = {Effective Markovian description of decoherence in bound systems},
 volume    = {92},
 pages     = {168-178},
 year      = {2014},
}

@article{schuch:PRA:1983,
 author    = {D. Schuch and K.-M. Chung and H. Hartmann},
 journal   = {Phys. Rev. A},
 title     = {Nonlinear Schr\"odinger-type field equation for the description of dissipative systems. I. Derivation of the nonlinear field equation and one-dimensional example},
 volume    = {24},
 pages     = {1652-1660},
 year      = {1983},
}

@article{schuch:PRA:1984-1,
 author    = {D. Schuch and K.-M. Chung and H. Hartmann},
 journal   = {Phys. Rev. A},
 title     = {Nonlinear Schr\"odinger-type field equation for the description of dissipative systems. II. Frictionally damped motion in a magnetic field},
 volume    = {25},
 pages     = {391-410},
 year      = {1984},
}

@article{schuch:PRA:1984-2,
 author    = {D. Schuch and K.-M. Chung and H. Hartmann},
 journal   = {Phys. Rev. A},
 title     = {Nonlinear Schr\"odinger-type field equation for the description of dissipative systems. III. Frictionally damped free motion as an example for an aperiodic motion},
 volume    = {25},
 pages     = {3086-3092},
 year      = {1984},
}

@BOOK{shamos-bk,
  editor     = {M. H. Shamos},
  TITLE      = {Great Experiments in Physics},
  PUBLISHER  = {Dover},
  YEAR       = {1987},
  address    = {New York},
}

@article{goldberg:AJP:1967,
 author    = {A. Goldberg and H. M. Schey and J. L. Schwartz},
 journal   = {Am. J. Phys.},
 title     = {Computer-generated motion pictures of one-dimensional quantum-mechanical transmission and reflection phenomena},
 volume    = {35},
 pages     = {177-186},
 year      = {1967},
}

@article{mazur:JCP:1959,
 author    = {J. Mazur and R. J. Rubin},
 journal   = {J. Chem. Phys.},
 title     = {Quantum-mechanical calculation of the probability of an exchange reaction for constrained linear encounters},
 volume    = {31},
 pages     = {1395-1412},
 year      = {1959},
}

@article{marcus:JCP:1966,
 author    = {R. A. Marcus},
 journal   = {J. Chem. Phys.},
 title     = {On the analytical mechanics of chemical reactions. Quantum mechanics of linear collisions},
 volume    = {45},
 pages     = {4493-4499},
 year      = {1966},
}

@article{abraham:AJP:1984,
 author    = {I. Galbraith and Y. S. Ching and E. Abraham},
 journal   = {Am. J. Phys.},
 title     = {Two-dimensional time-dependent quantum-mechanical scattering event},
 volume    = {52},
 pages     = {60-68},
 year      = {1984},
}

@article{efthymio:AnnPhys:2012,
 author    = {C. Efthymiopoulos and N. Delis and G. Contopoulos},
 journal   = {Ann. Phys.},
 title     = {Wavepacket approach to particle diffraction by thin targets: Quantum trajectories and arrival times},
 volume    = {327},
 pages     = {438-460},
 year      = {2012},
}

@article{efthymio:IJBC:2012,
 author    = {N. Delis and C. Efthymiopoulos and G. Contopoulos},
 journal   = {Int. J. Bifur. Chaos},
 title     = {Quantum vortices and trajectories in particle diffraction},
 volume    = {22},
 pages     = {1250214(1-17)},
 year      = {2012},
}

@article{muga:PhysRep:2000,
 author    = {J. G. Muga and C. R. Leavens},
 journal   = {Phys. Rep.},
 title     = {Arrival time in quantum mechanics},
 volume    = {338},
 pages     = {353-438},
 year      = {2000},
}

@BOOK{muga-bk-1:LNP:2002,
  editor     = {J. G. Muga and R. Sala Mayato and I. L. Egusquiza},
  TITLE      = {Time in Quantum Mechanics},
  PUBLISHER  = {Springer},
  series     = {Lecture Notes in Physics},
  volume     = {72},
  YEAR       = {2002},
  address    = {Berlin},
}

@BOOK{muga-bk-2:LNP:2009,
  editor     = {J. G. Muga and A. Ruschhaupt and A. del Campo},
  TITLE      = {Time in Quantum Mechanics - Vol.~2},
  PUBLISHER  = {Springer},
  series     = {Lecture Notes in Physics},
  volume     = {789},
  YEAR       = {2009},
  address    = {Berlin},
}

@article{valentini:PRSA:2005,
 author    = {A. Valentini and H. Westman},
 journal   = {Proc. R. Soc. A},
 title     = {Dynamical origin of quantum probabilities},
 volume    = {461},
 pages     = {253-272},
 year      = {2005},
}

@article{valentini:PRSA:2012,
 author    = {M. D. Towler and N. J. Russell and A. Valentini},
 journal   = {Proc. R. Soc. A},
 title     = {Time scales for dynamical relaxation to the Born rule},
 volume    = {468},
 pages     = {990-1013},
 year      = {2012},
}

@article{olkhovsky:NuovoCim:1974,
 author    = {V. S. Olkhovsky and E. Recami and A. J. Gerasimchuk},
 journal   = {Nuovo Cimento},
 title     = {Time operator in quantum mechanics. I. Nonrelativistic case},
 volume    = {22},
 pages     = {263-278},
 year      = {1974},
}

@article{olkhovsky:AMP:2009,
 author    = {V. S. Olkhovsky},
 journal   = {Adv. Math. Phys.},
 title     = {Time as a quantum observable, canonically conjugated to energy, and foundations of self-consistent time analysis of quantum processes},
 volume    = {Article ID 859710},
 pages     = {1-83},
 year      = {2009},
}

@article{wang:AnnPhys:2007,
 author    = {Z.-Y. Wang and C.-D. Xiong},
 journal   = {Ann. Phys.},
 title     = {How to introduce time operator},
 volume    = {322},
 pages     = {2304-2314},
 year      = {2007},
}

@book{pauli-hbk-1,
  address =       {Berlin},
  author =        {W. Pauli},
  chapter =       {Die allgemeinen Prinzipien der Wellenmechanik},
  editor =        {H. Geiger and K. Scheel},
  pages =         {83-272},
  publisher =     {Springer},
  title =         {Handbuch der Physik},
  volume =        {24/1},
  year =          {1933},
  edition =       {2nd},
}

@book{pauli-hbk-1rev,
  address =       {Berlin},
  author =        {W. Pauli},
  chapter =       {Die allgemeinen Prinzipien der Wellenmechanik},
  editor =        {S. Fl\"ugge},
  pages =         {1-168},
  publisher =     {Springer},
  title =         {Handbuch der Physik - Prinzipien der Quantentheorie I},
  volume =        {5/1},
  year =          {1958},
}

@book{pauli-hbk-1rep,
  address =       {Berlin},
  author =        {W. Pauli},
  title  =        {Die allgemeinen Prinzipien der Wellenmechanik},
  editor =        {N. Straumann},
  publisher =     {Springer},
  year =          {1990},
}

@book{pauli-hbk-1eng,
  address =       {Berlin},
  author =        {W. Pauli},
  title  =        {General Principles of Quantum Mechanics},
  editor =        {P. Achuthan and K. Venkatesan},
  publisher =     {Springer},
  year =          {1980},
}

@article{leavens:SSC:1990-1,
 author    = {C. R. Leavens},
 journal   = {Solid State Comm.},
 title     = {Transmission, reflection and dwell times within Bohm's causal interpretation of quantum mechanics},
 volume    = {74},
 pages     = {923-928},
 year      = {1990},
}

@article{leavens:SSC:1990-2,
 author    = {C. R. Leavens},
 journal   = {Solid State Comm.},
 title     = {Traversal times for rectangular barriers within Bohm's causal interpretation of quantum mechanics},
 volume    = {76},
 pages     = {253-261},
 year      = {1990},
}

@article{leavens:PhysLettA:1993,
 author    = {C. R. Leavens},
 journal   = {Phys. Lett. A},
 title     = {Arrival time distributions},
 volume    = {178},
 pages     = {27-32},
 year      = {1993},
}

@article{leavens:FoundPhys:1995,
 author    = {C. R. Leavens},
 journal   = {Solid State Comm.},
 title     = {Bohm Trajectory and Feynman Path Approaches to the ``Tunneling Time Problem''},
 volume    = {25},
 pages     = {229-268},
 year      = {1995},
}

@BOOK{zeh-hbk-1,
  autor      = {H. D. Zeh},
  chapter    = {Time in quantum theory},
  editor     = {D. Greenberger and K. Hentschel and F. Weinert},
  TITLE      = {Compendium of Quantum Physics: Concepts, Experiments, History and Philosophy},
  PUBLISHER  = {Springer},
  pages      = {786-792},
  YEAR       = {2009},
  address    = {Berlin},
}

@BOOK{reichl:1992,
  AUTHOR     = {L. E. Reichl},
  TITLE      = {The Transition to Chaos in Conservative Classical Systems: Quantum Manifestations},
  PUBLISHER  = {Springer},
  YEAR       = {1992},
  address    = {Berlin},
}

@BOOK{mehta:1991,
  AUTHOR     = {M. L. Mehta},
  TITLE      = {Random Matrix Theory},
  PUBLISHER  = {Academic Press},
  YEAR       = {1991},
  address    = {New York},
}

@BOOK{gaspard-bk:1998,
  AUTHOR     = {P. Gaspard},
  TITLE      = {Chaos, Scattering and Statistical Mechanics},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {1998},
  address    = {Cambridge},
}

@article{bohigas:PRL:1984,
 author    = {O. Bohigas and M. J. Giannoni and C. Schmit},
 journal   = {Phys. Rev. Lett.},
 title     = {},
 volume    = {52},
 pages     = {1-},
 year      = {1984},
}

@article{zurek:PRL:1994,
 author    = {W. H. Zurek and J. P. Paz},
 journal   = {Phys. Rev. Lett.},
 title     = {Decoherence, chaos, and the second law},
 volume    = {72},
 pages     = {2508-2511},
 year      = {1994},
}

@article{zaslavskii:SPJETP:1974,
 author    = {G. M. Zaslavskii and N. N. Filonenko},
 journal   = {Sov. Phys. JETP},
 title     = {Statistical properties of the energy spectrum of ``gliding'' electrons with mixed classical trajectories},
 volume    = {38},
 pages     = {317-323},
 year      = {1974},
}

@article{zaslavskii:ZhETF:1973,
 author    = {G. M. Zaslavskii and N. N. Filonenko},
 journal   = {Zh. Eksp. Teor. Fiz.},
 title     = {},
 volume    = {65},
 pages     = {643-656},
 year      = {1973},
}

@article{mcdonald:PRL:1979,
 author    = {S. W. McDonald and A. N. Kaufman},
 journal   = {Phys. Rev. Lett.},
 title     = {},
 volume    = {42},
 pages     = {1189-},
 year      = {1979},
}

@article{heller:PRL:1984,
 author    = {E. J. Heller},
 journal   = {Phys. Rev. Lett.},
 title     = {Bound-state eigenfunctions of classically chaotic Hamiltonian systems: scars of periodic orbits},
 volume    = {53},
 pages     = {1515-1518},
 year      = {1984},
}

@article{bluemel:PhysicsWorld:1990,
 author    = {R. Bl\"umel and U. Smilansky},
 journal   = {Physics World},
 title     = {},
 volume    = {3},
 number    = {2},
 pages     = {30-},
 year      = {1990},
}

@article{baranger:chaos:1993,
 author    = {H. U. Baranger and Others},
 journal   = {Chaos},
 title     = {},
 volume    = {3},
 pages     = {665},
 year      = {1993},
}

@article{marcus:chaos:1993,
 author    = {C. M. Marcus and Others},
 journal   = {Chaos},
 title     = {},
 volume    = {3},
 pages     = {643},
 year      = {1993},
}

@article{fleischmann:PRL:1992,
 author    = {R. Fleischmann and T. Geisel and R. Ketzmerick},
 journal   = {Phys. Rev. Lett.},
 title     = {},
 volume    = {68},
 pages     = {1367-},
 year      = {1992},
}

@article{ketzmerick:PRL:1998,
 author    = {A. S. Sachrajda and Others},
 journal   = {Phys. Rev. Lett.},
 title     = {},
 volume    = {80},
 pages     = {1948-},
 year      = {1998},
}

@article{verges:PRL:1998,
 author    = {P. L. de Andres and J. A. Verg\'es},
 journal   = {Phys. Rev. Lett.},
 title     = {},
 volume    = {80},
 pages     = {980-},
 year      = {1998},
}

@article{fyodorov:PRA:1998,
 author    = {Y. V. Fyodorov and Y. Alhassid},
 journal   = {Phys. Rev. A},
 title     = {},
 volume    = {58},
 pages     = {R3375-},
 year      = {1998},
}

@article{raizen:PRL:1998,
 author    = {Q. Niu and M. G. Raizen},
 journal   = {Phys. Rev. Lett.},
 title     = {},
 volume    = {80},
 pages     = {3491-},
 year      = {1998},
}

@article{gluck:PRL:1999,
 author    = {M. Gl\"uck and A. R. Kolovsky and H. J. Korsch},
 journal   = {Phys. Rev. Lett.},
 title     = {},
 volume    = {83},
 pages     = {891-},
 year      = {1999},
}

@article{seligman:PhysRep:1997,
 author    = {C. Jung and T. H. Seligman},
 journal   = {Phys. Rep.},
 title     = {},
 volume    = {285},
 pages     = {77-},
 year      = {1997},
}

@article{lewenkopf:AnnPhys:1991,
 author    = {C. H. Lewenkopf and H. A. Weidenm\"uller},
 journal   = {Ann. Phys.},
 title     = {},
 volume    = {212},
 pages     = {53-},
 year      = {1991},
}

@BOOK{smilansky-ch:1991,
  author     = {U. Smilansky},
  chapter    = {},
  editor     = {M.-J. Giannoni and A. Voros and J. Zinn-Justin},
  TITLE      = {Chaos and Quantum Physics},
  PUBLISHER  = {North-Holland},
  pages      = {},
  YEAR       = {1991},
  address    = {New York},
}

@BOOK{cushing-bk:1996,
  editor     = {J. T. Cushing and A. Fine and S. Goldstein},
  TITLE      = {Bohmian Mechanics: An Appraisal},
  PUBLISHER  = {Kluwer},
  YEAR       = {1996},
  address    = {Boston},
}

@article{duerr:JStatPhys:1992b,
 author    = {D. D\"urr and S. Goldstein and N. Zangh\`i},
 journal   = {J. Stat. Phys.},
 title     = {Quantum chaos, classical randomness, and Bohmian mechanics},
 volume    = {68},
 pages     = {259-270},
 year      = {1992},
}

@article{frisk:PLA:1997,
 author    = {H. Frisk},
 journal   = {Phys. Lett. A},
 title     = {},
 volume    = {227},
 pages     = {139-},
 year      = {1997},
}

@article{parmenter:PLA:1995,
 author    = {R.H. Parmenter and R. W. Valentine},
 journal   = {Phys. Lett. A},
 title     = {},
 volume    = {201},
 pages     = {1-},
 year      = {1995},
}

@article{parmenter:PLA:1996,
 author    = {R.H. Parmenter and R. W. Valentine},
 journal   = {Phys. Lett. A},
 title     = {},
 volume    = {213},
 pages     = {319-},
 year      = {1996},
}

@article{makowski:PLA:2000,
 author    = {A. J. Makowski and P. Pep{\l}oswski and S. T. Dembi\'nski},
 journal   = {Phys. Lett. A},
 title     = {Chaotic causal trajectories: the role of the phase of stationary states},
 volume    = {266},
 pages     = {241-248},
 year      = {2000},
}

@article{makowski:ActaPhysPolB:2001,
 author    = {A. J. Makowski and M. Fr\c ackowiak},
 journal   = {Acta Physica Polonica B},
 title     = {The simplest non-trivial model of chaotic causal dynamics},
 volume    = {32},
 pages     = {2831-2842},
 year      = {2001},
}

@article{makowski:ActaPhysPolB:2002,
 author    = {A. J. Makowski},
 journal   = {Acta Physica Polonica B},
 title     = {Forced dynamical systems derivable from Bohmian mechanics},
 volume    = {33},
 pages     = {583-592},
 year      = {2002},
}

@article{bonfin:PRE:1998,
 author    = {O. F. de Alcantara Bonfim and J. Florencio and F. C. S\'a Barreto},
 journal   = {Phys. Rev. E},
 title     = {},
 volume    = {58},
 pages     = {R2693-},
 year      = {1998},
}

@article{bonfin:PLA:2000,
 author    = {O. F. de Alcantara Bonfim and J. Florencio and F. C. S\'a Barreto},
 journal   = {Phys. Rev. E},
 title     = {},
 volume    = {277},
 pages     = {129-},
 year      = {2000},
}

@article{faisal:PLA-1:1995,
 author    = {U. Schwengelbeck and F. H. M. Faisal},
 journal   = {Phys. Lett. A},
 title     = {},
 volume    = {199},
 pages     = {281-},
 year      = {1995},
}

@article{faisal:PLA-2:1995,
 author    = {F. H. M. Faisal and U. Schwengelbeck},
 journal   = {Phys. Lett. A},
 title     = {},
 volume    = {207},
 pages     = {31-},
 year      = {1995},
}

@article{iacomelli:PLA:1996,
 author    = {G. Iacomelli and M. Pettini},
 journal   = {Phys. Lett. A},
 title     = {},
 volume    = {212},
 pages     = {29-},
 year      = {1996},
}

@article{chattaraj:PLA:1996,
 author    = {S. Sengupta and P. K. Chattaraj},
 journal   = {Phys. Lett. A},
 title     = {The quantum theory of motion and signatures of chaos in the quantum behaviour of a classically chaotic system},
 volume    = {215},
 pages     = {119-127},
 year      = {1996},
}

@article{chattaraj:CurrentSci:1996,
 author    = {P. K. Chattaraj and S. Sengupta},
 journal   = {Curr. Sci.},
 title     = {Quantum chaos in Rydberg atoms: A quantum potential approach},
 volume    = {71},
 pages     = {134-139},
 year      = {1996},
}

@article{chattaraj:CurrentSci:1998,
 author    = {P. K. Chattaraj and S. Sengupta and A. Poddar},
 journal   = {Curr. Sci.},
 title     = {Chaotic dynamics of some quantum anharmonic oscillators},
 volume    = {74},
 pages     = {758-764},
 year      = {1998},
}

@article{polavieja:PRE:1997,
 author    = {G. Garc\'\i a de Polavieja and M. S. Child},
 journal   = {Phys. Rev. E},
 title     = {Quantum instability of the flux lines in the coherent state representation},
 volume    = {55},
 pages     = {1451-1456},
 year      = {1997},
}

@article{polavieja:PLA:1996,
 author    = {G. Garc\'\i a de Polavieja},
 journal   = {Phys. Lett. A},
 title     = {A causal quantum theory in phase space},
 volume    = {220},
 pages     = {303-314},
 year      = {1996},
}

@article{procaccia:PhysicaD:1983,
 author    = {P. Grassberger and I. Procaccia},
 journal   = {Physica D},
 title     = {},
 volume    = {9},
 pages     = {189-},
 year      = {1983},
}

@article{goldstein:PRE:1999,
 author    = {S. Goldstein},
 journal   = {Phys. Rev. E},
 title     = {},
 volume    = {60},
 pages     = {7578},
 year      = {1999},
}

@article{sprung:PLA:1999,
 author    = {H. Wu and D. W. L. Sprung},
 journal   = {Phys. Lett. A},
 title     = {},
 volume    = {261},
 pages     = {150-},
 year      = {1999},
}

@article{polavieja:PRA:1996,
 author    = {G. Garc{\'\i}a de Polavieja},
 journal   = {Phys. Rev. A},
 title     = {Exponential divergence of neighboring quantal trajectories},
 volume    = {53},
 pages     = {2059-2061},
 year      = {1996},
}

@article{dewdney:PLA:1996,
 author    = {C. Dewdney and Z. Malik},
 journal   = {Phys. Lett. A},
 title     = {},
 volume    = {220},
 pages     = {183-},
 year      = {1996},
}

@article{makowski:PLA:1998,
 author    = {S. Konkel and A. J. Makowski},
 journal   = {Phys. Lett. A},
 title     = {Regular and chaotic causal trajectories for the Bohm potential in a restricted space},
 volume    = {238},
 pages     = {95-100},
 year      = {1998},
}

@article{cushing:PhilosSci:2000,
 author    = {J. T. Cushing},
 journal   = {Philos. Sci.},
 title     = {},
 volume    = {67},
 pages     = {S432-},
 year      = {2000},
}

@article{sales:PRE:2003,
 author    = {J. A. de Sales and J. Florencio},
 journal   = {Phys. Rev. E},
 title     = {Quantum chaotic trajectories in integrable right triangular billiards},
 volume    = {67},
 pages     = {016216(1-6)},
 year      = {2003},
}

@article{sales:PhysicaA:2001,
 author    = {J. A. de Sales and J. Florencio},
 journal   = {Physica A},
 title     = {Bohmian quantum trajectories in a square billiard in the bouncing ball regime},
 volume    = {290},
 pages     = {101-106)},
 year      = {2001},
}

@article{falsaperla:FoundPhys:2002,
 author    = {P. Falsaperla and G. Fonte and G. Salesi},
 journal   = {Found. Phys.},
 title     = {Quantum Lyapunov exponents},
 volume    = {32},
 pages     = {267-294},
 year      = {2002},
}

@article{falsaperla:PLA:2003,
 author    = {P. Falsaperla and G. Fonte},
 journal   = {Phys. Lett. A},
 title     = {On the motion of a single particle near a nodal line in the de Broglie-Bohm interpretation of quantum mechanics},
 volume    = {316},
 pages     = {382-390},
 year      = {2003},
}

@article{wisniacki:EPL:2005,
 author    = {D. A. Wisniacki and E. R. Pujals},
 journal   = {Europhys. Lett.},
 title     = {Motion of vortices implies chaos in Bohmian mechanics},
 volume    = {71},
 pages     = {159-},
 year      = {2005},
}

@article{wisniacki:JPA:2007,
 author    = {D. A. Wisniacki and E. R. Pujals and F. Borondo},
 journal   = {J. Phys. A},
 title     = {},
 volume    = {40},
 pages     = {14353-},
 year      = {2007},
}

@article{schlegel:PLA:2008,
 author    = {K. G. Schlegel and S. F\"orster},
 journal   = {Phys. Lett. A},
 title     = {Deterministic chaos in entangled eigenstates},
 volume    = {372},
 pages     = {3620-3631},
 year      = {2008},
}

@article{bu:PhysicaD:2006,
 author    = {S. Bu},
 journal   = {Physica D},
 title     = {Quantum trajectory of an individual particle in the presence of chaos},
 volume    = {217},
 pages     = {103-106},
 year      = {2006},
}

@article{bennett:JPA:2010,
 author    = {A. Bennett},
 journal   = {J. Phys. A},
 title     = {},
 volume    = {43},
 pages     = {5304-},
 year      = {2010},
}

@article{struyve:NJP:2010,
 author    = {S. Colin and W. Struyve},
 journal   = {New J. Phys.},
 title     = {Quantum non-equilibrium and relaxation to equilibrium for a class of de Broglie-Bohm-type theories},
 volume    = {12},
 pages     = {043008(1-21)},
 year      = {2010},
}

@article{efthymio:JPA:2006,
 author    = {C. Efthymiopoulos and Contopoulos},
 journal   = {J. Phys. A},
 title     = {Chaos in Bohmian quantum mechanics},
 volume    = {39},
 pages     = {1819-1852},
 year      = {2006},
}

@article{efthymio:JPA:2012,
 author    = {G. Contopoulos and N. Delis and C. Efthymiopoulos},
 journal   = {J. Phys. A},
 title     = {Order in de Broglie-Bohm Mechanics},
 volume    = {45},
 pages     = {165301(1-21)},
 year      = {2011},
}

@article{efthymio:JPA:2007,
 author    = {C. Efthymiopoulos and C. Kalapotharakos and G. Contopoulos},
 journal   = {J. Phys. A},
 title     = {Nodal points and the transition from ordered to chaotic Bohmian trajectories},
 volume    = {40},
 pages     = {12945-12972},
 year      = {2007},
}

@article{efthymio:CMDynAstr:2008,
 author    = {G. Contopoulos and C. Efthymiopoulos},
 journal   = {Celest. Mech. Dyn. Astron.},
 title     = {Ordered and chaotic Bohmian trajectories},
 volume    = {102},
 pages     = {219-239},
 year      = {2008},
}

@article{efthymio:PRE:2009,
 author    = {C. Efthymiopoulos and C. Kalapotharakos and G. Contopoulos},
 journal   = {Phys. Rev. E},
 title     = {Origin of chaos near critical points of quantum flow},
 volume    = {79},
 pages     = {036203(1-18)},
 year      = {2009},
}

@article{berry:ProcRSocLondA:1987,
 author    = {M. V. Berry},
 journal   = {Proc. R. Soc. Lond. A},
 title     = {Quantum chaology (The Bakerian Lecture, 1987)},
 volume    = {413},
 pages     = {183-198},
 year      = {1987},
}

@article{berry:PhysScr:1989,
 author    = {M. V. Berry},
 journal   = {Phys. Scr.},
 title     = {Quantum chaology, not quantum chaos},
 volume    = {40},
 pages     = {335-336},
 year      = {1989},
}

@article{leacock:PRL:1983,
 author    = {R. A. Leacock and M. J. Padgett},
 journal   = {Phys. Rev. Lett.},
 title     = {Hamilton-Jacobi theory and the quantum action variable},
 volume    = {50},
 pages     = {3-6},
 year      = {1983},
}

@article{leacock:PRD:1983,
 author    = {R. A. Leacock and M. J. Padgett},
 journal   = {Phys. Rev. D},
 title     = {Hamilton-Jacobi/action-angle quantum mechanics},
 volume    = {28},
 pages     = {2491-2502},
 year      = {1983},
}

@article{jordan:ZPhys:1926,
 author    = {P. Jordan},
 journal   = {Z. Phys.},
 title     = {},
 volume    = {38},
 pages     = {513-},
 year      = {1926},
}

@article{jordan:ZPhys-1:1927,
 author    = {P. Jordan},
 journal   = {Z. Phys.},
 title     = {},
 volume    = {40},
 pages     = {809-},
 year      = {1927},
}

@article{jordan:ZPhys-2:1927,
 author    = {P. Jordan},
 journal   = {Z. Phys.},
 title     = {},
 volume    = {44},
 pages     = {1-},
 year      = {1927},
}

@BOOK{gottfried-bk:1966,
  AUTHOR     = {K. Gottfried},
  TITLE      = {Quantum Mechanics},
  PUBLISHER  = {Benjamin},
  YEAR       = {New York},
  address    = {1966},
  volume     = {1},
}

@article{dirac:PRSLA:1927,
 author    = {P. A. M. Dirac},
 journal   = {Proc. R. Soc. London A},
 title     = {The physical interpretation of the quantum dynamics},
 volume    = {113},
 pages     = {621-641},
 year      = {1927},
}

@article{dirac:PZSov:1933,
 author    = {P. A. M. Dirac},
 journal   = {Phys. Z. Sowjetunion},
 title     = {},
 volume    = {3},
 pages     = {64-},
 year      = {1933},
}

@article{dirac:RMP:1945,
 author    = {P. A. M. Dirac},
 journal   = {Rev. Mod. Phys.},
 title     = {},
 volume    = {17},
 pages     = {195-},
 year      = {1945},
}

@article{jeffreys:PLMS:1925,
 author    = {K. Gottfried},
 journal   = {Proc. London Math. Soc.},
 title     = {},
 volume    = {23},
 pages     = {428-},
 year      = {1925},
}

@article{wentzel:ZPhys:1926,
 author    = {G. Wentzel},
 journal   = {Z. Phys.},
 title     = {},
 volume    = {38},
 pages     = {518-},
 year      = {1926},
}

@article{kramers:ZPhys:1926,
 author    = {H. A. Kramers},
 journal   = {Z. Phys.},
 title     = {},
 volume    = {39},
 pages     = {828-},
 year      = {1926},
}

@article{brillouin:ComptRend:1926,
 author    = {L. Brillouin},
 journal   = {Compt. Rend.},
 title     = {},
 volume    = {183},
 pages     = {24-},
 year      = {1926},
}

@article{floyd:PRD-1:1982,
 author    = {E. R. Floyd},
 journal   = {Phys. Rev. D},
 title     = {},
 volume    = {25},
 pages     = {1547-},
 year      = {1982},
}

@article{floyd:PRD-2:1982,
 author    = {E. R. Floyd},
 journal   = {Phys. Rev. D},
 title     = {},
 volume    = {26},
 pages     = {1339-},
 year      = {1982},
}

@article{floyd:PRD:1984,
 author    = {E. R. Floyd},
 journal   = {Phys. Rev. D},
 title     = {},
 volume    = {29},
 pages     = {1842-},
 year      = {1984},
}

@article{floyd:PRD:1986,
 author    = {E. R. Floyd},
 journal   = {Phys. Rev. D},
 title     = {},
 volume    = {34},
 pages     = {3246-},
 year      = {1986},
}

@article{floyd:FPL:1996,
 author    = {E. R. Floyd},
 journal   = {Found. Phys. Lett.},
 title     = {},
 volume    = {9},
 pages     = {489-},
 year      = {1996},
}

@article{floyd:FPL:2000,
 author    = {E. R. Floyd},
 journal   = {Found. Phys. Lett.},
 title     = {},
 volume    = {13},
 pages     = {235-},
 year      = {2000},
}

@article{floyd:IJMPA:1999,
 author    = {E. R. Floyd},
 journal   = {Int. J. Mod. Phys. A},
 title     = {},
 volume    = {14},
 pages     = {1111-},
 year      = {1999},
}

@article{faraggi:PLA:1998,
 author    = {A. E. Faraggi and M. Matone},
 journal   = {Phys. Lett. A},
 title     = {},
 volume    = {249},
 pages     = {180-},
 year      = {1998},
}

@article{faraggi:PLB:1998,
 author    = {A. E. Faraggi and M. Matone},
 journal   = {Phys. Lett. B},
 title     = {},
 volume    = {437},
 pages     = {369-},
 year      = {1998},
}

@article{faraggi:PLB-1:1999,
 author    = {A. E. Faraggi and M. Matone},
 journal   = {Phys. Lett. B},
 title     = {},
 volume    = {445},
 pages     = {77-},
 year      = {1999},
}

@article{faraggi:PLB-2:1999,
 author    = {A. E. Faraggi and M. Matone},
 journal   = {Phys. Lett. B},
 title     = {},
 volume    = {450},
 pages     = {34-},
 year      = {1999},
}

@article{faraggi:IJMPA:2000,
 author    = {A. E. Faraggi and M. Matone},
 journal   = {Int. J. Mod. Phys. A},
 title     = {},
 volume    = {15},
 pages     = {1869-},
 year      = {2000},
}

@article{john:FPL:2002,
 author    = {M. V. John},
 journal   = {Found. Phys. Lett.},
 title     = {Modified de Broglie-Bohm approach to quantum mechanics},
 volume    = {15},
 pages     = {329-343},
 year      = {2002},
}

@article{john:AnnPhys:2009,
 author    = {M. V. John},
 journal   = {Ann. Phys.},
 title     = {Probability and complex quantum trajectories},
 volume    = {324},
 pages     = {220-231},
 year      = {2009},
}

@article{john:AnnPhys:2010,
 author    = {M. V. John},
 journal   = {Ann. Phys.},
 title     = {Probability and complex quantum trajectories: Finding the missing links},
 volume    = {325},
 pages     = {2132-2139},
 year      = {2010},
}

@article{john:FoundPhys:2013,
 author    = {M. V. John and K. Mathew},
 journal   = {Found. Phys.},
 title     = {Coherent states and modified de Broglie-Bohm complex quantum trajectories},
 volume    = {43},
 pages     = {859-871},
 year      = {2013},
}

@article{fring:PRA:2013,
 author    = {S. Dey and A. Fring},
 journal   = {Phys. Rev. A},
 title     = {Bohmian quantum trajectories from coherent states},
 volume    = {88},
 pages     = {022116(1-12)},
 year      = {2013},
}

@article{tannor:JCP:2006,
 author    = {Y. Goldfarb and I. Degani and D. J. Tannor},
 journal   = {J. Chem. Phys.},
 title     = {Bohmian mechanics with complex action: A new trajectory-based formulation of quantum mechanics},
 volume    = {125},
 pages     = {231103(1-4)},
 year      = {2006},
}

@article{tannor:JCP-2:2007,
 author    = {Y. Goldfarb and D. J. Tannor},
 journal   = {J. Chem. Phys.},
 title     = {Interference in Bohmian mechanics with complex action},
 volume    = {127},
 pages     = {161101(1-4)},
 year      = {2007},
}

@article{tannor:JPCA:2007,
 author    = {Y. Goldfarb and J. Schiff and D. J. Tannor},
 journal   = {J. Chem. Phys.},
 title     = {Unified derivation of Bohmian methods and the incorporation of interference effects},
 volume    = {111},
 pages     = {10416-10421},
 year      = {2007},
}

@article{tannor:JCP-1:2007,
 author    = {Y. Goldfarb and I. Degani and D. J. Tannor},
 journal   = {J. Chem. Phys.},
 title     = {Response to ``Comment on `Bohmian mechanics with complex action: A new trajectory-based formulation of quantum mechanics' '' [J. Chem. Phys. {\bf 127}, 197101 (2007)]},
 volume    = {127},
 pages     = {197102(1-3)},
 year      = {2007},
}

@article{tannor:CP:2007,
 author    = {Y. Goldfarb and I. Degani and D. J. Tannor},
 journal   = {Chem. Phys.},
 title     = {Semiclassical approximation with zero velocity trajectories},
 volume    = {338},
 pages     = {106-112},
 year      = {2007},
}

@article{sanz:JCP:2007,
 author    = {A. S. Sanz and S. Miret-Art\'es},
 journal   = {J. Chem. Phys.},
 title     = {Comment on `Bohmian mechanics with complex action: A new trajectory-based formulation of quantum mechanics' [J. Chem. Phys. {\bf 125}, 231103 (2006)]},
 volume    = {127},
 pages     = {197101(1-3)},
 year      = {2007},
}

@article{chou:JCP:2006,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Computational method for the quantum Hamilton-Jacobi equation: Bound states in one dimension},
 volume    = {125},
 pages     = {174103(1-)},
 year      = {2006},
}

@article{chou:JCP-1:2008,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Quantum trajectories in complex space: One-dimensional stationary scattering problems},
 volume    = {128},
 pages     = {154106(1-)},
 year      = {2008},
}

@article{chou:JCP-2:2008,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Quantum vortices within the complex quantum Hamilton-Jacobi formalism},
 volume    = {128},
 pages     = {234106(1-)},
 year      = {2008},
}

@article{chou:JCP-3:2008,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Quantum streamlines within the complex quantum Hamilton-Jacobi formalism},
 volume    = {129},
 pages     = {124113(1-)},
 year      = {2008},
}

@article{chou:JCP:2010,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Complex-extended Bohmian mechanics},
 volume    = {132},
 pages     = {134102(1-)},
 year      = {2010},
}

@article{chou:JCP:2011,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Wave front-ray synthesis for solving the multidimensional quantum Hamilton-Jacobi equation},
 volume    = {135},
 pages     = {074102(1-)},
 year      = {2011},
}

@article{chou:PRE:2006,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {Phys. Rev. E},
 title     = {Computational method for the quantum Hamilton-Jacobi equation: One-dimensional scattering problems},
 volume    = {74},
 pages     = {066702(1-)},
 year      = {2006},
}

@article{chou:PRA:2007,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {Phys. Rev. A},
 title     = {Quantum trajectories in complex space},
 volume    = {76},
 pages     = {012115(1-)},
 year      = {2007},
}

@article{chou:PRA:2008,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {Phys. Rev. A},
 title     = {Considerations on the probability density in complex space},
 volume    = {78},
 pages     = {044101(1-)},
 year      = {2007},
}

@article{chou:PRL:2011,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {Phys. Rev. Lett.},
 title     = {Scattered wave packet formalism with Markovian outgoing wave boundary conditions for open quantum systems},
 volume    = {107},
 pages     = {030401(1-)},
 year      = {2011},
}

@article{chou:PRA:2011,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {Phys. Rev. A},
 title     = {Scattered-wave-packet formalism with applications to barrier scattering and quantum transistors},
 volume    = {84},
 pages     = {056707(1-)},
 year      = {2011},
}

@article{trahan:JCP:2003,
 author    = {C. J. Trahan and K. Hughes and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {A new method for wave packet dynamics: Derivative propagation along quantum trajectories},
 volume    = {118},
 pages     = {9911-},
 year      = {2003},
}

@article{yang:AnnPhys-1:2005,
 author    = {C.-D. Yang},
 journal   = {Ann. Phys.},
 title     = {Quantum dynamics of hydrogen atom in complex space},
 volume    = {319},
 pages     = {399-443},
 year      = {2005},
}

@article{yang:AnnPhys-2:2005,
 author    = {C.-D. Yang},
 journal   = {Ann. Phys.},
 title     = {Wave-particle duality in complex space},
 volume    = {319},
 pages     = {445-470},
 year      = {2005},
}

@article{yang:IJQC:2006,
 author    = {C.-D. Yang},
 journal   = {Int. J. Quantum Chem.},
 title     = {Solving quantum trajectories in Coulomb potential by quantum Hamilton-Jacobi theory},
 volume    = {106},
 pages     = {1620-1639},
 year      = {2006},
}

@article{yang:CSF-1:2006,
 author    = {C.-D. Yang},
 journal   = {Chaos, Solitons \& Fractals},
 title     = {On modeling and visualizing single-electron spin motion},
 volume    = {30},
 pages     = {41-50},
 year      = {2006},
}

@article{yang:CSF-2:2006,
 author    = {C.-D. Yang},
 journal   = {Chaos, Solitons \& Fractals},
 title     = {Modeling quantum harmonic oscillator in complex domain},
 volume    = {30},
 pages     = {342-362},
 year      = {2006},
}

@article{yang:AnnPhys:2006,
 author    = {C.-D. Yang},
 journal   = {Ann. Phys.},
 title     = {Quantum Hamilton mechanics: Hamilton equations of quantum motion, origin of quantum operators, and proof of quantization axiom},
 volume    = {321},
 pages     = {2876-2926},
 year      = {2006},
}

@article{yang:CSF-1:2007,
 author    = {C.-D. Yang},
 journal   = {Chaos, Solitons \& Fractals},
 title     = {The origin and proof of quantization axiom ${\bf p} \to \hat{\bf p} = -i\hbar\nabla$ in complex spacetime},
 volume    = {32},
 pages     = {274-283},
 year      = {2007},
}

@article{yang:CSF-2:2007,
 author    = {C.-D. Yang},
 journal   = {Chaos, Solitons \& Fractals},
 title     = {Complex tunneling dynamics},
 volume    = {32},
 pages     = {312-345},
 year      = {2007},
}

@article{yang:CSF-3:2007,
 author    = {C.-D. Yang},
 journal   = {Chaos, Solitons \& Fractals},
 title     = {Quantum motion in complex space},
 volume    = {33},
 pages     = {1073-1092},
 year      = {2007},
}

@article{yang:CSF-4:2007,
 author    = {C.-D. Yang and C.-H. Wei},
 journal   = {Chaos, Solitons \& Fractals},
 title     = {Parameterization of all path integral trajectories},
 volume    = {33},
 pages     = {118-134},
 year      = {2007},
}

@article{chou:PLA:2010,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Geometric phase within the complex quantum Hamilton-Jacobi formalism},
 volume    = {374},
 pages     = {2608-2613},
 year      = {2010},
}

@article{chou:PLA:2009,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {J. Chem. Phys.},
 title     = {Arbitrary Lagrangian-Eulerian rate equation for the Born probability density in complex space},
 volume    = {373},
 pages     = {1811-1817},
 year      = {2009},
}

@article{chou:IJQC:2008,
 author    = {C.-C. Chou and R. E. Wyatt},
 journal   = {Int. J. Quantum Chem.},
 title     = {Riccati differential equation for quantum mechanical bound states: Comparison of numerical integrators},
 volume    = {108},
 pages     = {238-248},
 year      = {2008},
}

@article{swinney:PhysicaD:1985,
 author    = {A. Wolf and J. B. Swift and H. L. Swinney and J. A. Vastano},
 journal   = {Physica D},
 title     = {},
 volume    = {16},
 pages     = {285-},
 year      = {1985},
}

@article{greene:PhysicaD:1987,
 author    = {J. M. Greene},
 journal   = {Physica D},
 title     = {},
 volume    = {24},
 pages     = {213-},
 year      = {1987},
}

@BOOK{baker-bk:1996,
  AUTHOR     = {G. L. Baker and J. P. Gollub},
  TITLE      = {Chaotic Dynamics: An Introduction},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {1996},
  address    = {Cambridge},
  edition    = {2nd Ed.},
}

@BOOK{jordan-bk:1999,
  AUTHOR     = {D. W. Jordan and P. Smith},
  TITLE      = {Nonlinear Ordinary Differential Equations},
  PUBLISHER  = {Oxford University Press},
  YEAR       = {1999},
  address    = {Oxford},
  edition    = {3rd Ed.},
}

@article{bowman:PLA:2002,
 author    = {G. E. Bowman},
 journal   = {Phys. Lett. A},
 title     = {Wave packets and Bohmian mechanics in the kicked rotator},
 volume    = {298},
 pages     = {7-17},
 year      = {2002},
}

@article{frieden:PhysicaA:2009,
 author    = {B. Roy Frieden and B. H. Soffer},
 journal   = {Physica A},
 title     = {de Broglie's wave hypothesis from Fisher information},
 volume    = {388},
 pages     = {1315-1330},
 year      = {2002},
}

@article{rosen:AJP-1:1964,
 author    = {N. Rosen},
 journal   = {Am. J. Phys.},
 title     = {Identical motion in quantum and in classical mechanics},
 volume    = {32},
 pages     = {377-379},
 year      = {1964},
}

@article{rosen:AJP-2:1964,
 author    = {N. Rosen},
 journal   = {Am. J. Phys.},
 title     = {The relation between classical and quantum mechanics},
 volume    = {32},
 pages     = {597-600},
 year      = {1964},
}

@article{rosen:AJP:1965,
 author    = {N. Rosen},
 journal   = {Am. J. Phys.},
 title     = {Mixed states in classical mechanics},
 volume    = {33},
 pages     = {146-150},
 year      = {1965},
}

@article{rosen:FoundPhys:1986,
 author    = {N. Rosen},
 journal   = {Found. Phys.},
 title     = {Quantum particles and classical particles},
 volume    = {16},
 pages     = {687-700},
 year      = {1986},
}

@article{allori:JOptB:2002,
 author    = {V. Allori and Detlef D\"urr and N. Zangh{\`\i} and S. Goldstein},
 journal   = {J. Opt. B},
 title     = {Seven steps toward the classical world},
 volume    = {4},
 pages     = {482-488},
 year      = {2002},
}

@inproceedings{berry:LesHouches:1991,
  AUTHOR     = {M. V. Berry},
  CHAPTER    = {Some quantum-to-classical asymptotics},
  editor     = {M.-J. Giannoni and A. Voros and J. Zinn-Justin},
  booktitle  = {Chaos and Quantum Physics},
  pages      = {251-304},
  PUBLISHER  = {North-Holland},
  YEAR       = {1996},
  address    = {Amsterdam},
  series     = {Les Houches Lecture Series LII (1989)},
}

@BOOK{child-bk:1974,
  AUTHOR     = {M. S. Child},
  TITLE      = {Molecular Collision Theory},
  PUBLISHER  = {Academic Press},
  YEAR       = {1974},
  address    = {London},
}

@BOOK{bolivar-bk:2004,
  AUTHOR     = {A. O. Bolivar},
  TITLE      = {Quantum-Classical Correspondence. Dynamical Quantization and the Classical Limit},
  PUBLISHER  = {Springer},
  YEAR       = {2004},
  address    = {Berlin},
}

@article{bolivar:CanJPhys:2003,
 author    = {A. O. Bolivar},
 journal   = {Can. J. Phys.},
 title     = {The Bohm quantum potential and the classical limit of quantum mechanics},
 volume    = {81},
 pages     = {971-976},
 year      = {2003},
}

@article{makowski:PRA-1:2002,
 author    = {A. J. Makowski},
 journal   = {Phys. Rev. A},
 title     = {Exact classical limit of quantum mechanics: Central potentials and specific states},
 volume    = {65},
 pages     = {032103(1-5)},
 year      = {2002},
}

@article{makowski:PRA-2:2002,
 author    = {A. J. Makowski and K. J. G\'orska},
 journal   = {Phys. Rev. A},
 title     = {Bohr's correspondence principle: The cases for which it is exact},
 volume    = {66},
 pages     = {062103(1-6)},
 year      = {2002},
}

@article{bohm:PRL:1985,
 author    = {D. Bohm and B. J. Hiley},
 journal   = {Phys. Rev. Lett.},
 title     = {Unbroken quantum realism, from microscopic to macroscopic levels},
 volume    = {55},
 pages     = {2511-2514},
 year      = {1985},
}

@BOOK{holland-cushing-bk:1996,
  AUTHOR     = {P. R. Holland},
  CHAPTER    = {Is quantum mechanics universal?},
  editor     = {J. T. Cushing and A. Fine and S. Goldstein},
  TITLE      = {Bohmian Mechanics and Quantum Theory: An Appraisal},
  pages      = {99-220},
  PUBLISHER  = {Kluwer},
  YEAR       = {1996},
  address    = {Dordrecht},
}

@BOOK{cushing-butterfield-bk:1999,
  AUTHOR     = {J. T. Cushing},
  CHAPTER    = {Bohmian mechanics and chaos},
  editor     = {J. Butterfield and C. Pagonis},
  TITLE      = {From Physics to Philosophy},
  pages      = {90-107},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {1999},
  address    = {Cambridge},
}

@article{matzkin:PLA:2007,
 author    = {A. Matzkin},
 journal   = {Phys. Lett. A},
 title     = {Can Bohmian trajectories account for quantum recurrences having classical periodicities?},
 volume    = {361},
 pages     = {294-300},
 year      = {2007},
}

@article{matzkin:SHPMP:2008,
 author    = {A. Matzkin and V. Nurock},
 journal   = {Studies in History and Philosophy of Modern Physics B},
 title     = {Classical and Bohmian trajectories in semiclassical systems: Mismatch in dynamics, mismatch in reality?},
 volume    = {39},
 pages     = {17-40},
 year      = {2008},
}

@article{matzkin:JPCS:2009,
 author    = {A. Matzkin},
 journal   = {J. Phys.: Conf. Ser.},
 title     = {Bohmian mechanics and the emergence of classicality},
 volume    = {174},
 pages     = {012039(1-8)},
 year      = {2009},
}

@article{matzkin:FoundPhys:2009,
 author    = {A. Matzkin and V. Nurock},
 journal   = {Found. Phys.},
 title     = {Bohmian Mechanics, the quantum-classical correspondence and the classical limit: The case of the square billiard},
 volume    = {39},
 pages     = {903-920},
 year      = {2009},
}

@article{na:PLA:2002,
 author    = {K. Na and R. E. Wyatt},
 journal   = {Phys. Lett. A},
 title     = {Quantum hydrodynamic analysis of decoherence: quantum trajectories and stress tensor},
 volume    = {306},
 pages     = {97-103},
 year      = {2002},
}

@article{na:PhysScr:2003,
 author    = {K. Na and R. E. Wyatt},
 journal   = {Phys. Scr.},
 title     = {Quantum hydrodynamic analysis of decoherence},
 volume    = {67},
 pages     = {169-180},
 year      = {2003},
}

@article{struyve:JPA:2003,
 author    = {W. Struyve and W. De Baere and J. De Neve and S. De Weirdt},
 journal   = {J. Phys. A},
 title     = {Comment on `Bohmian prediction about a two double-slit experiment and its disagreement with standard quantum mechanics'},
 volume    = {36},
 pages     = {1525-1530},
 year      = {2003},
}

@article{marchildon:JPA:2003,
 author    = {E. Guay and L. Marchildon},
 journal   = {J. Phys. A},
 title     = {Two-particle interference in standard and Bohmian quantum mechanics},
 volume    = {36},
 pages     = {5617-5624},
 year      = {2003},
}

@article{marchildon:JModOpt:2003,
 author    = {L. Marchildon},
 journal   = {J. Mod. Opt.},
 title     = {Two-particle interference devices and compatibility of Bohmian and standard quantum mechanics},
 volume    = {50},
 pages     = {873-879},
 year      = {2003},
}

@article{hiley:FoundPhys:1999,
 author    = {O. Maroney and B. J. Hiley},
 journal   = {Found. Phys.},
 title     = {Quantum state teleportation understood through the Bohm interpretation},
 volume    = {29},
 pages     = {1403-1415},
 year      = {1999},
}

@article{golshani:JPA:2001,
 author    = {M. Golshani and O. Akhavan},
 journal   = {J. Phys. A},
 title     = {Bohmian prediction about a two double-slit experiment and its disagreement with standard quantum mechanics},
 volume    = {34},
 pages     = {5259-5268},
 year      = {2001},
 doi       = {10.1088/0305-4470/34/25/308},
}

@article{ghose:PRAMANA:2002,
 author    = {P. Ghose},
 journal   = {PRAMANA},
 title     = {On the incompatibility of standard quantum mechanics and conventional de Broglie-Bohm theory},
 volume    = {59},
 pages     = {417-424},
 year      = {2002},
 doi       = {10.1007/s12043-002-0136-y},
 url       = {https://doi.org/10.1007/s12043-002-0136-y},
}

@article{dewdney:PLA:1990,
 author    = {M. M. Lam and C. Dewdney},
 journal   = {Phys. Lett. A},
 title     = {Locality and nonlocality in correlated two-particle interferometry},
 volume    = {150},
 pages     = {127-135},
 year      = {1990},
}

@article{dewdney:FoundPhys:1988,
 author    = {C. Dewdney},
 journal   = {Found. Phys.},
 title     = {Nonlocally correlated trajectories in two-particle quantum mechanics},
 volume    = {18},
 pages     = {867-886},
 year      = {1988},
}

@article{maddox:JCP:2001,
 author    = {J. B. Maddox and E. R. Bittner},
 journal   = {J. Chem. Phys.},
 title     = {Quantum relaxation dynamics using Bohmian trajectories},
 volume    = {115},
 pages     = {6309-6316},
 year      = {2001},
}

@article{maddox:PRE:2002,
 author    = {J. B. Maddox and E. R. Bittner},
 journal   = {Phys. Rev. E},
 title     = {Quantum dissipation in unbounded systems},
 volume    = {65},
 pages     = {026143(1-10)},
 year      = {2002},
}

@article{holloway:JCP:2001,
 author    = {Z. S. Wang and G. R. Darling and S. Holloway},
 journal   = {J. Chem. Phys.},
 title     = {Dissociation dynamics from a de Broglie-Bohm perspective},
 volume    = {115},
 pages     = {10373-10381},
 year      = {2001},
}

@article{burghardt:IJQC:2004,
 author    = {I. Burghardt and K. B. M{\o}ller and G. Parlant and L. S. Cederbaum and E. R. Bittner},
 journal   = {Int. J. Quantum Chem.},
 title     = {Quantum hydrodynamics: mixed states, dissipation, and a new hybrid quantum-classical approach},
 volume    = {100},
 pages     = {1153-1162},
 year      = {2004},
}

@article{burghardt:JCP:2004,
 author    = {I. Burghardt and G. Parlant},
 journal   = {J. Chem. Phys.},
 title     = {On the dynamics of coupled Bohmian and phase-space variables: A new hybrid quantum-classical approach},
 volume    = {120},
 pages     = {3055-3058},
 year      = {2004},
}

@article{burghardt:JPCA:2007,
 author    = {K. H. Hughes and S. M. Parry and G. Parlant and I. Burghardt},
 journal   = {J. Phys. Chem. A},
 title     = {A hybrid hydrodynamic-Liouvillian approach to mixed quantum-classical dynamics: Application to tunneling in a double well},
 volume    = {111},
 pages     = {10269-10283},
 year      = {2007},
}

@article{burghardt:JCP-1:2001,
 author    = {I. Burghardt and L. S. Cederbaum},
 journal   = {J. Chem. Phys.},
 title     = {Hydrodynamic equations for mixed quantum states. I. General formulation},
 volume    = {115},
 pages     = {10303-10311},
 year      = {2001},
}

@article{burghardt:JCP-2:2001,
 author    = {I. Burghardt and L. S. Cederbaum},
 journal   = {J. Chem. Phys.},
 title     = {Hydrodynamic equations for mixed quantum states. II. Coupled electronic states},
 volume    = {115},
 pages     = {10312-10322},
 year      = {2001},
}

@article{shnider:SIAM:1999,
 author    = {J. Schiff and S. Schneider},
 journal   = {SIAM J. Numer. Anal.},
 title     = {A natural approach to the numerical integration of Riccati differential equations},
 volume    = {36},
 pages     = {1392-1413},
 year      = {1999},
}

@article{krayzel:JEOS:2010,
 author    = {F. Krayzel and R. Poll\`es and A. Moreau and M. Mihailovic and G. Granet},
 journal   = {J. Eur. Opt. Soc. - Rapid publications},
 title     = {Simulation and analysis of exotic non-specular phenomena},
 volume    = {5},
 pages     = {10025},
 year      = {2010},
}

@article{spin.Bell1971,
 author    = {J. Bell},
 journal   = {Proceedings of the International School of Physics `Enrico Fermi', course IL: Foundations of Quantum Mechanics, New York, Academic},
 pages     = {171-181},
 title     = {Introduction to the hidden variable question},
 volume    = {},
 year      = {1971},
}

@article{spin.Dewdney1986,
 author               = {C. Dewdney and P. R. Holland, and A. Kyprianidis},
 journal              = {Physics Letters},
 pages                = {259-267},
 title                = {What happens in a spin measurement},
 volume               = {119},
 year                 = {1986},
 }

@article{rel.Durr2013,
 author               = {D. D\"urr and S. Goldstein and T. Norsen and W. Struyve and and N. Zangh\`{\i}},
 journal              = {Proc. R. Soc. A},
 pages                = {20130699},
 title                = {Can Bohmian mechanics be made relativistic?},
 volume               = {470},
 year                 = {2013},
 }

@article{rel.Horton2004,
 author               = {G. Horton and C. Dewdney},
 journal              = {J. Phys. A},
 pages                = {11935},
 title                = {A relativistic covariant version of Bohm's quantum field theory for the scalar field},
 volume               = {37},
 year                 = {2004},
 }

@article{rel.Berndl1996,
 author               = {K. Berndl, D. D\"urr, S. Goldstein, and N. Zangh\`{\i}},
 journal              = {Phys. Rev. A},
 pages                = {2062-2073},
 title                = {Nonlocality, Lorentz invariance, and Bohmian quantum theory},
 volume               = {53},
 year                 = {1996},
 }

@article{rel.Horton2001,
 author               = {G. Horton, and C. Dewdney},
 journal              = {J. Phys. A},
 pages                = {9871-9878},
 title                = {A non-local, Lorentz-invariant, hidden-variable interpretation of relativistic quantum mechanics based on particle trajectories},
 volume               = {34},
 year                 = {2001},
 }

@article{rel.Dewdney2002,
 author               = {C. Dewdney, and G. Horton},
 journal              = {J. Phys. A},
 pages                = {10117-10127},
 title                = {Relativistically invariant extension of the de Broglie-Bohm theory of quantum mechanics},
 volume               = {35},
 year                 = {2002},
 }

@article{rel.Tumulka2007,
 author               = {R. Tumulka},
 journal              = {J. Phys. A},
 pages                = {3245-3273},
 title                = {The `unromantic pictures' of quantum theory},
 volume               = {40},
 year                 = {2007},
 }

@article{rel.Tausk2010,
 author               = {D. V. Tausk, and R. Tumulka},
 journal              = {J. Math. Phys.},
 pages                = {122306},
 title                = {Can We Make a Bohmian Electron Reach the Speed of Light, at Least for One Instant?},
 volume               = {51},
 year                 = {2010},
 }


@article{rel.Struyve2010,
 author               = {W. Struyve},
 journal              = {Rep. Prog. Phys.},
 pages                = {106001},
 title                = {Pilot-wave theory and quantum fields},
 volume               = {73},
 year                 = {2010},
 }

@article{qft.Takabayashi1952,
 author               = {T. Takabayashi},
 journal              = {Prog. Theor. Phys.},
 pages                = {143},
 title                = {On the Formulation of Quantum Mechanics associated with Classical Picturess},
 volume               = {8},
 year                 = {1952},
 }

@article{qft.Holland1988,
 author               = {P. R. Holland},
 journal              = {Phys. Lett. A},
 pages                = {9-18},
 title                = {On the Formulation of Quantum Mechanics associated with Classical Picturess},
 volume               = {128},
 year                 = {1988},
 }

@BOOK{qft.Valentini1996,
  AUTHOR     = {A. Valentini},
  CHAPTER    = {},
  editor     = {J.T. Cushing, A. Fine and S. Goldstein},
  TITLE      = {Bohmian Mechanics and quantum Theory: An Appraisal},
  pages      = {},
  PUBLISHER  = {Kluwer, Dordrecht, 45},
  YEAR       = {1996},
  address    = {},
}


@article{qft.Struyve2007,
 author               = {W. Struyve and H. Westman},
 journal              = {Proc. R. Soc. A},
 pages                = {3115-3129},
 title                = {A minimalist pilot-wave model for quantum electrodynamics},
 volume               = {463},
 year                 = {2007},
 }

@article{qc.Callender1994,
 author               = {C. Callender, and R. Weingard},
 journal              = {PSA: Proceedings of the Biennial Meeting of the Philosophy of Science Association 1994},
 pages                = {218-227},
 title                = {The Bohmian Model of Quantum Cosmology},
 volume               = {},
 year                 = {1994},
 }

@article{qc.Pinto2005,
 author               = {N. Pinto-Neto},
 journal              = {Found. Phys.},
 pages                = {577-603},
 title                = {The Bohm interpretation of quantum cosmology},
 volume               = {35},
 year                 = {2005},
 }

@article{qc.Shojai2007,
 author               = {F. Shojai, and S. Molladovoudi},
 journal              = {Gen. Rel. Grav.},
 pages                = {795-813},
 title                = {Quantum cosmology with varying speed of light and Bohmian trajectories},
 volume               = {39},
 year                 = {2007},
 }


@article{qc.deBarros1998,
 author               = {J. A. de Barros, N. Pinto-Neto, M. A. Sagioro-Leal},
 journal              = {Phys. Lett. A},
 pages                = {229-239},
 title                = {The causal interpretation of dust and radiation fluid non-singular quantum cosmologies},
 volume               = {241},
 year                 = {1998},
 }


@article{qc.Shojai1998,
 author               = {F. Shojai and M. Golshani},
 journal              = {Int. J. Mod. Phys. A},
 pages                = {677-693},
 title                = {On the geometrization of Bohmian mechanics; a new approach to quantum gravity},
 volume               = {13},
 year                 = {1998},
 }

@article{qc.Pinto2005b,
 author               = {N. Pinto-Neto, E. Sergio Santini, and F. T. Falciano},
 journal              = {Phys. Lett. A},
 pages                = {131-143},
 title                = {Quantization of Friedmann cosmological models with two fluids: Dust plus radiation},
 volume               = {344},
 year                 = {2005},
 }

@article{qc.Colin2013,
 author               = {S. Colin, and A. Valentini},
 journal              = {Phys. Rev. D},
 pages                = {103515},
 title                = {Mechanism for the suppression of quantum noise at large scales on expanding space},
 volume               = {88},
 year                 = {2013},
 }

@article{gindensperger:JCP:2000,
  author   = {E. Gindensperger and C. Meier and J. A. Beswick},
  journal  = {J. Chem. Phys.},
  title    = {Communications: Mixing quantum and classical dynamics using Bohmian trajectories},
  volume   = {113},
  pages    = {9369-9372},
  year     = {2000},
}

@article{gindensperger:JCP:2002-1,
  author   = {E. Gindensperger and C. Meier and J. A. Beswick},
  journal  = {J. Chem. Phys.},
  title    = {Quantum-classical dynamics including continuum states using quantum trajectories},
  volume   = {116},
  pages    = {8-13},
  year     = {2002},
}

@article{gindensperger:JCP:2002-2,
  author   = {E. Gindensperger and C. Meier and J. A. Beswick},
  journal  = {J. Chem. Phys.},
  title    = {Quantum-classical description of rotational diffractive scattering using Bohmian trajectories: Comparison with full quantum wave packet results},
  volume   = {116},
  pages    = {10051-10059},
  year     = {2002},
}

@article{gindensperger:AdvQuantChem:2004,
  author   = {E. Gindensperger and C. Meier and J. A. Beswick},
  journal  = {Adv. Quant. Chem.},
  title    = {Hybrid quantum/classical dynamics using Bohmian trajectories},
  volume   = {47},
  pages    = {331-346},
  year     = {2004},
}

@article{meier:JCP:2004,
  author   = {C. Meier and J. A. Beswick},
  journal  = {J. Chem. Phys.},
  title    = {Femtosecond pump-probe spectroscopy of I$_2$ in a dense rare gas environment: A mixed quantum-classical study of vibrational decoherence},
  volume   = {121},
  pages    = {4550-4558},
  year     = {2004},
}

@article{meier:PRL:2004,
  author   = {C. Meier},
  journal  = {Phys. Rev. Lett.},
  title    = {Mixed quantum-classical treatment of vibrational decoherence},
  volume   = {93},
  pages    = {173003(1-4)},
  year     = {2004},
}

@inproceedings{drezet:ch:2014,
  AUTHOR    = {A. Drezet},
  editor    = {S. Gao},
  booktitle = {Protective Measurements and Quantum Reality: Toward a New Understanding of Quantum Mechanics},
  CHAPTER   = {Implications of protective measurements on de Broglie-Bohm trajectories},
  pages     = {},
  PUBLISHER = {Cambridge University Press},
  YEAR      = {2014},
  address   = {Cambridge},
  eprint    = {arXiv:1402.7256},
}

@article{durt:PRA:2002,
 author    = {T. Durt and Y. Pierseaux},
 journal   = {Phys. Rev. A},
 title     = {Bohm's interpretation and maximally entangled states},
 volume    = {66},
 pages     = {052109(1-11)},
 year      = {2002},
}

@article{tannor:JCP:2014,
 author    = {N. Zamstein and D. J. Tannor},
 journal   = {J. Chem. Phys.},
 title     = {Communication: Overcoming the root search problem in complex quantum trajectory calculations},
 volume    = {140},
 pages     = {041105},
 year      = {2014},
}

@article{tannor:JCP-1:2012,
 author    = {N. Zamstein and D. J. Tannor},
 journal   = {J. Chem. Phys.},
 title     = {Non-adiabatic molecular dynamics with complex quantum trajectories. I. The diabatic representation},
 volume    = {137},
 pages     = {22A517},
 year      = {2012},
}

@article{tannor:JCP-2:2012,
 author    = {N. Zamstein and D. J. Tannor},
 journal   = {J. Chem. Phys.},
 title     = {Non-adiabatic molecular dynamics with complex quantum trajectories. II. The adiabatic representation},
 volume    = {137},
 pages     = {22A518},
 year      = {2012},
}

@article{rubi:PRE:2001,
 author    = {D. Reguera and M. Rub{\'\i}},
 journal   = {Phys. Rev. E},
 title     = {Kinetic equations for diffusion in the presence of entropic barriers},
 volume    = {64},
 pages     = {061106(1-8)},
 year      = {2001},
}

@article{schuch:PhysScr:2013,
 author    = {D. Schuch},
 journal   = {Phys. Scr.},
 title     = {Is quantum theory intrinsically nonlinear?},
 volume    = {87},
 pages     = {038117(1-10)},
 year      = {2013},
}

@article{schuch:IJQC:1986,
 author    = {D. Schuch},
 journal   = {Int. J. Quantum. Chem.},
 title     = {},
 volume    = {29},
 pages     = {1561-},
 year      = {1986},
}

@article{davisson:PR:1927,
 author    = {C. Davisson and L. H. Germer},
 journal   = {Phys. Rev.},
 title     = {Diffraction of Electrons by a Crystal of Nickel},
 volume    = {30},
 pages     = {705-740},
 year      = {1927},
}

@article{davisson:Nature:1927,
 author    = {C. Davisson and L. H. Germer},
 journal   = {Nature},
 title     = {Reflection of electrons by a crystal of nickel},
 volume    = {119},
 pages     = {558-560},
 year      = {1927},
}

@article{stern:ZPhys:1929,
 author    = {P. Knauer and O. Stern},
 journal   = {Z. Physik},
 title     = {Intensit\"atsmessungen an Molekularstrahlen von Gasen},
 volume    = {53},
 pages     = {766-778},
 year      = {1929},
}

@article{stern:ZPhys:1930,
 author    = {I. Estermann and O. Stern},
 journal   = {Z. Physik},
 title     = {Beugung von Molekularstrahlen},
 volume    = {61},
 pages     = {95-125},
 year      = {1930},
}

@article{stern:ZPhys:1931,
 author    = {I. Estermann and R. Frisch and O. Stern},
 journal   = {Z. Physik},
 title     = {Monochromasierung der de Broglie-Wellen von Molekularstrahlen},
 volume    = {73},
 pages     = {348-365},
 year      = {1931},
}

@article{peres:SHPMP:2002,
 author    = {A. Peres},
 journal   = {Stud. History Philos. Modern Physics},
 title     = {Karl Popper and the Copenhagen interpretation},
 volume    = {33},
 pages     = {23-34},
 year      = {2002},
}

@article{zeilinger:RMP:1988,
 author    = {A. Zeilinger and R. G\"ahler and C. G. Shull and W. Treimer and W. Mampe},
 journal   = {Rev. Mod. Phys.},
 title     = {Single- and double-slit diffraction of neutrons},
 volume    = {60},
 pages     = {1067-1073},
 year      = {1988},
}

@article{zeilinger:AJP:1991,
 author    = {R. G\"ahler and A. Zeilinger},
 journal   = {Am. J. Phys.},
 title     = {Wave-optical experiments with very cold neutrons},
 volume    = {59},
 pages     = {316-324},
 year      = {1991},
}

@article{arndt:Nature:1999,
 author    = {M. Arndt and O. Nairz and J. Vos-Andreae and C. Keller and G. van der Zouw and A. Zeilinger},
 journal   = {Nature},
 title     = {Wave-particle duality of C$_{60}$ molecules},
 volume    = {401},
 pages     = {680-682},
 year      = {1999},
}

@article{arndt:PRL:2003,
 author    = {L. Hackerm\"uller and S. Uttenthaler and K. Hornberger and E. Reiger and B. Brezger and A. Zeilinger and M. Arndt},
 journal   = {Phys. Rev. Lett.},
 title     = {Wave nature of biomolecules and fluorofullerenes},
 volume    = {91},
 pages     = {90408(1-4)},
 year      = {2003},
}

@article{arndt:Angew:2008,
 author    = {S. Gerlich and M. Gring and H. Ulbricht and K. Hornberger and J. T\"uxen and M. Mayor and M. Arndt},
 journal   = {Angew. Chem. Int. Ed.},
 title     = {Matter-wave metrology as a complementary tool for mass spectrometry},
 volume    = {47},
 pages     = {6195-6198},
 year      = {2008},
}

@article{arndt:NatPhys:2007,
 author    = {S. Gerlich and L. Hackerm\"uller and K. Hornberger and A. Stibor and H. Ulbricht and M. Gring and F. Goldfarb and T. Savas and M. M\"uri and M. Mayor and M. Arndt},
 journal   = {A Kapitza-Dirac-Talbot-Lau interferometer for highly polarizable molecules},
 title     = {Nature Phys.},
 volume    = {3},
 pages     = {711-715},
 year      = {2007},
}

@article{sanz:AOP:2014,
 author    = {A. S. Sanz and R. Mart{\'\i}nez-Casado and H. C. Pe\~nate-Rodr{\'\i}guez and G. Rojas-Lorenzo and S. Miret-Art\'es},
 journal   = {Ann. Phys.},
 title     = {Dissipative Bohmian mechanics within the Caldirola-Kanai framework: A trajectory analysis of wave-packet dynamics in viscid media},
 volume    = {347},
 pages     = {1-20},
 year      = {2014},
}

@article{furth:ZPhys:1933,
 author    = {R. F\"urth},
 journal   = {Z. Phys.},
 title     = {\"Uber einige Beziehungen zwischen klassischer Statistik und Quantenmechanik},
 volume    = {81},
 pages     = {143-162},
 year      = {1933},
}

@article{comisar:PhysRev:1965,
 author    = {G. G. Comisar},
 journal   = {Phys. Rev.},
 title     = {Brownian-motion model of nonrelativistic quantum mechanics},
 volume    = {138},
 pages     = {B1332-B1337},
 year      = {1965},
}

@BOOK{fourier-bk,
  AUTHOR     = {J. B. J. Fourier},
  TITLE      = {Th\'eorie analytique de la chaleur},
  PUBLISHER  = {Firmin Didot P\`ere et Fils},
  YEAR       = {1822},
  address    = {Paris},
}

@BOOK{fourier-bk-eng,
  AUTHOR     = {J. B. J. Fourier},
  TRANSLATOR = {A. Freeman},
  TITLE      = {The Analytical Theory of Heat},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {2009},
  address    = {Cambridge},
}

@article{hobson:AJP:2013,
 author    = {A. Hobson},
 journal   = {Am. J. Phys.},
 title     = {There are no particles, there are only fields},
 volume    = {81},
 pages     = {211-223},
 year      = {2013},
}

@article{leon:AOP:2014,
 author    = {M. Rodr{\'\i}guez-V\'azquez and M. del Rey and H. Westman and J. Le\'on},
 journal   = {Ann. Phys.},
 title     = {Local quanta, unitary inequivalence, and vacuum entanglement},
 volume    = {351},
 pages     = {112-137},
 year      = {2014},
}

@article{wilbraham:CDMJ:1848,
 author    = {H. Wilbraham},
 journal   = {Camb. Dublin Math. J.},
 title     = {On a certain periodic function},
 volume    = {3},
 pages     = {198-201},
 year      = {1848},
}

@article{gibbs:Nature:1898,
 author    = {J. W. Gibbs},
 journal   = {Nature},
 title     = {Fourier's series},
 volume    = {59},
 pages     = {200},
 year      = {1898},
}

@article{gibbs:Nature:1899,
 author    = {J. W. Gibbs},
 journal   = {Nature},
 title     = {Fourier's series},
 volume    = {59},
 pages     = {606},
 year      = {1899},
}

@BOOK{Mehra-Feynman-bk,
  AUTHOR     = {J. Mehra},
  TITLE      = {The Beat of a Different Drum: The Life and Science of Richard Feynman},
  PUBLISHER  = {Oxford University Press},
  YEAR       = {1994},
  address    = {Oxford},
}

@BOOK{hawking-bk,
  AUTHOR     = {S. J. Hawking},
  TITLE      = {The Dreams that Stuff is Made of},
  PUBLISHER  = {Running Press},
  YEAR       = {2011},
  address    = {Philadephia, PA},
}

@BOOK{waerden-bk,
  AUTHOR     = {B. L. van der Waerden},
  TITLE      = {Sources of Quantum Mechanics},
  PUBLISHER  = {Dover},
  YEAR       = {1966},
  address    = {New York},
}

@BOOK{broglie-bk:1960,
  AUTHOR     = {L. de Broglie},
  TITLE      = {Non-Linear Wave Mechanics. A Causal Interpretation},
  PUBLISHER  = {Elsevier},
  YEAR       = {1960},
  address    = {Amsterdam},
}

@BOOK{jadczyk-bk:2014,
  AUTHOR     = {A. Jadczyk},
  TITLE      = {Quantum Fractals. From Heisenberg's Uncertainty to Barnsley's Fractality},
  PUBLISHER  = {World Scientific},
  YEAR       = {2014},
  address    = {Singapore},
}

@article{ehrenberg:PPSB:1949,
 author    = {W. Ehrenberg and R. E. Siday},
 journal   = {Proc. Phys. Soc. B},
 title     = {The refractive index in electron optics and the principles of dynamics},
 volume    = {62},
 pages     = {8-21},
 year      = {1949},
}

@article{feynman:RMP:1948,
 author    = {P. R. Feynman},
 journal   = {Rev. Mod. Phys.},
 title     = {Space-time approach to non-relativistic quantum mechanics},
 volume    = {20},
 pages     = {367-387},
 year      = {1948},
}

@article{sanz:foundphys:2015,
 author    = {A. S. Sanz},
 journal   = {Found. Phys.},
 title     = {Investigating puzzling aspects of the quantum theory by means of its hydrodynamic formulation},
 volume    = {45},
 pages     = {1153-1165},
 year      = {2015},
}

@BOOK{kant:1781,
  AUTHOR     = {I. Kant},
  TITLE      = {Critique of Pure Reason},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {1781 [1998]},
  address    = {Cambridge},
  note       = {Trans. by P. Guyer and A. W.Wood},
  series     = {The Cambridge Edition of the Works of Immanuel Kant},
}

@BOOK{nielsen-chuang-bk,
  AUTHOR     = {M. A. Nielsen and I. L. Chuang},
  TITLE      = {Quantum Computation and Quantum Information},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {2000},
  address    = {Cambridge},
}

@BOOK{marage-wallenborn-bk,
  editor     = {P. Marage and G. Wallenborn},
  TITLE      = {The Solvay Councils and the Birth of Modern Physics},
  PUBLISHER  = {Birkh\"auser},
  YEAR       = {1999},
  series     = {Science Networks. Historical Studies},
  volume     = {22},
  address    = {Basel},
}

@BOOK{bacciagaluppi-valentini-bk,
  editor     = {G. Bacciagaluppi and A. Valentini},
  TITLE      = {Quantum Theory at the Crossroads. Reconsidering the 1927 Solvay Conference},
  PUBLISHER  = {Cambridge University Press},
  YEAR       = {2009},
  series     = {Science Networks. Historical Studies},
  address    = {Cambridge},
}

@article{benseny:EPJD:2014,
 author    = {A. Benseny and G. Albareda and A. S. Sanz and J. Mompart and X. Oriols},
 journal   = {Eur. Phys. J. D},
 title     = {Applied Bohmian mechanics},
 volume    = {68},
 pages     = {286(1-42)},
 year      = {2014},
}

@article{milena:JRLR:2015,
 author    = {M. Davidovi\'c and M. Bo\v{z}i\'c and A. S. Sanz},
 journal   = {J. Russ. Laser Res.},
 pages     = {329-342},
 title     = {Description of classical and quantum interference in view of the concept of flow line},
 volume    = {36},
 year      = {2015},
}

@article{zeh:FoundPhys:1973,
 author    = {H. D. Zeh},
 journal   = {Found. Phys.},
 title     = {Toward a quantum theory of observation},
 volume    = {3},
 pages     = {109-116},
 year      = {1973},
}

@article{schlosshauer:RMP:2004,
  title = {Decoherence, the measurement problem, and interpretations of quantum mechanics},
  author = {Schlosshauer, Maximilian},
  journal = {Rev. Mod. Phys.},
  volume = {76},
  issue = {4},
  pages = {1267--1305},
  numpages = {0},
  year = {2005},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.76.1267},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.76.1267}
}

@article{schrodinger:ProcCamPS:1935,
 author    = {E. Schr\"odinger},
 journal   = {Math. Proc. Cambridge Philos. Soc.},
 title     = {Discussion of probability relations between separated systems},
 volume    = {31},
 pages     = {555-563},
 year      = {1935},
 doi       = {10.1017/S0305004100013554},
}

@article{schrodinger:ProcCamPS:1936,
 author    = {E. Schr\"odinger},
 journal   = {Math. Proc. Cambridge Philos. Soc.},
 title     = {Probability between separated systems},
 volume    = {32},
 pages     = {446-452},
 year      = {1936},
 doi       = {10.1017/S0305004100019137},
}

@article{luis:AOP:2015,
 author    = {A. Luis and A. S. Sanz},
 journal   = {Ann. Phys.},
 title     = {What dynamics can be expected for mixed states in two-slit experiments?},
 volume    = {357},
 pages     = {95-107},
 year      = {2015},
}

@article{batelaan:NJP:2013,
 author    = {R. Bach and D. Pope and S.-H. Liou and H. Batelaan},
 journal   = {New J. Phys.},
 title     = {Controlled double-slit electron diffraction},
 volume    = {15},
 pages     = {033018(1-7)},
 year      = {2013},
}

@article{walls:PRA:1993,
  title = {Loss of coherence in interferometry},
  author = {Tan, S. M. and Walls, D. F.},
  journal = {Phys. Rev. A},
  volume = {47},
  issue = {6},
  pages = {4663--4676},
  numpages = {0},
  year = {1993},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.47.4663},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.47.4663}
}

@article{walls:Nature:1994,
 author    = {P. Storey and S. Tan and M. Collett and D. Walls},
 journal   = {Nature},
 title     = {Path detection and the uncertainty principle},
 volume    = {357},
 pages     = {626-628},
 year      = {1994},
}

@article{wolf:JOSAA:1957,
 author    = {B. J. Thompson and E. Wolf},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Two-beam interference with partially coherent light},
 volume    = {47},
 pages     = {895-902},
 year      = {1957},
}

@article{zernike:PhysicaV:1938,
 author    = {F. Zernike},
 journal   = {Physica V},
 title     = {The concept of degree of coherence and its application to optical problems},
 volume    = {8},
 pages     = {785-795},
 year      = {1938},
}

@INPROCEEDINGS{sanz:ch-protvino:2015,
  AUTHOR =    {A. S. Sanz},
  TITLE =     {How far can a pragmatist go into quantum theory? -- A critical view of our current understanding of quantum phenomena},
  pages =     {161-171},
  PUBLISHER = {World Scientific},
  YEAR =      {2015},
  crossref =  {petrov-bk:2015},
}

@PROCEEDINGS{petrov-bk:2015,
  editor =    {V. Petrov and R. Ryutin},
  BOOKTITLE = {Particle and Astroparticle Physics, Gravitation and Cosmology: Predictions, Observations and New Projects (Proceedings of the XXXth International Workshop on High Energy Physics)},
  TITLE =     {Particle and Astroparticle Physics, Gravitation and Cosmology: Predictions, Observations and New Projects},
  PUBLISHER = {World Scientific},
  YEAR =      {2015},
  address =   {Singapore},
}

@article{einstein:PhysZeits:1917,
 author    = {A. Einstein},
 journal   = {Physikalische Zeitschrift},
 title     = {Zur Quantentheorie der Strahlung},
 volume    = {18},
 pages     = {121-128},
 year      = {1917},
}

@article{hiley:SHPMP:1997,
 author    = {B. J. Hiley},
 journal   = {Stud. Hist. Phil. Mod. Phys.},
 title     = {Essay Review - Quantum Mechanics: Historical Contingency and the Copenhagen Hegemony by James T. Cushing},
 volume    = {28},
 pages     = {299-305},
 year      = {1997},
}

@article{hiley:JComputElect:2015,
 author    = {B. J. Hiley},
 journal   = {J. Comput. Electron.},
 title     = {On the relationship between the Wigner-Moyal approach and the quantum operator algebra of von Neumann},
 volume    = {14},
 pages     = {869-878},
 year      = {2015},
}

@BOOK{hiley-chap:2016,
 author     = {P. Pylkk\"anen and B. J. Hiley and I. P\"attiniemi},
 editor     = {A. Guay and T. Pradeu},
 title      = {Individuals Across the Sciences},
 CHAPTER    = {Bohm's approach and Individuality},
 pages      = {226-249},
 publisher  = {Oxford University Press},
 year       = {2015},
 address    = {New York},
 preprint   = {arXiv:1405.4772v3 (2014)},
}

@BOOK{bohm-bk:1980,
  AUTHOR     = {D. Bohm},
  TITLE      = {Wholeness and the Implicate Order},
  PUBLISHER  = {Routledge},
  YEAR       = {1980},
  address    = {New York},
}

@BOOK{cushing-bk:1994,
  AUTHOR     = {J. T. Cushing},
  title      = {Quantum Mechanics: Historical Contingency and the Copenhagen Hegemony},
  PUBLISHER  = {University of Chicago Press},
  YEAR       = {1994},
  address    = {Chicago},
}

@article{padgett:AJP:2016,
 author    = {R. S. Aspden and M. J. Padgett and G. C. Spalding},
 journal   = {Am. J. Phys.},
 title     = {Video recording true single-photon double-slit interference},
 volume    = {84},
 pages     = {671-677},
 year      = {2016},
}

@article{sanz:ApplSci:2020,
 author   = {A. S. Sanz and M. Davidovi\'c and M. Bo\v{z}i\'c},
 journal  = {Appl. Sci.},
 title    = {Bohmian-based approach to Gauss-Maxwell beams},
 volume   = {10},
 pages    = {1808(1-25)},
 year     = {2020},
 doi      = {10.3390/app10051808},
 url      = {https://doi.org/10.3390/app10051808},
}

@article{sanz:AOP:2015,
 author    = {A. S. Sanz and M. Davidovi\'c and M. Bo\v{z}i\'c},
 journal   = {Ann. Phys.},
 pages     = {205-221},
 title     = {Full quantum mechanical analysis of atomic three-grating Mach-Zehnder interferometry},
 volume    = {353},
 year      = {2015},
 doi       = {10.1016/j.aop.2014.11.012},
 url       = {https://doi.org/10.1016/j.aop.2014.11.012},
}

@BOOK{sanz:springer:2006,
  AUTHOR     = {A. S. Sanz and S. Miret-Art\'es},
  editor     = {D. A. Micha and I. Burghardt},
  title      = {Quantum Dynamics of Complex Molecular Systems},
  CHAPTER    = {Atom-surface diffraction: A quantum trajectory description},
  pages      = {343-368},
  publisher  = {Springer},
  year       = {2007},
  address    = {Berlin},
}

@article{tumulka:EJP:2005,
 author    = {R. Tumulka},
 journal   = {Eur. J. Phys.},
 title     = {Feynman's path integrals and Bohm's particle paths},
 volume    = {26},
 pages     = {L11-L13},
 year      = {2005},
}

@BOOK{hiley:vaxjo:2003,
  AUTHOR     = {B. J. Hiley},
  editor     = {A. Khrennikov},
  title      = {Quantum Theory: Reconsiderations of Foundations - 2},
  CHAPTER    = {Phase space descriptions of quantum phenomena},
  pages      = {267-286},
  publisher  = {V\"axj\"o University Press},
  year       = {2003},
  address    = {V\"axj\"o},
}

@article{EPR:PhysRev:1935,
  title = {Can Quantum-Mechanical Description of Physical Reality Be Considered Complete?},
  author = {Einstein, A. and Podolsky, B. and Rosen, N.},
  journal = {Phys. Rev.},
  volume = {47},
  issue = {10},
  pages = {777--780},
  numpages = {0},
  year = {1935},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.47.777},
  url = {https://link.aps.org/doi/10.1103/PhysRev.47.777}
}

@article{milburn:PTRSLA:2003,
 author    = {J. P. Dowling and G. J. Milburn},
 journal   = {Phil. Trans. Roy. Soc. Lond. A},
 title     = {Quantum technology: The second quantum revolution},
 volume    = {361},
 pages     = {1655-1674},
 year      = {2003},
 doi       = {10.1098/rsta.2003.1227},
 url       = {https://doi.org/10.1098/rsta.2003.1227},
}

@article{hiley:BMFRS:1997,
 author    = {B. J. Hiley},
 journal   = {Biogr. Mems. Fell. R. Soc.},
 title     = {David Joseph Bohm. 20 December 1917 -- 27 October 1992: Elected F.R.S. 1990},
 volume    = {43},
 pages     = {107-131},
 year      = {1997},
}

@article{ziman:PRSL:1953,
 author    = {J. M. Ziman},
 journal   = {Proc. Roy. Soc. Lond. A},
 title     = {Quantum hydrodynamics and the theory of liquid helium},
 volume    = {219},
 pages     = {257-270},
 year      = {1953},
}

@article{bierter:JLTP:1969,
 author    = {W. Bierter and H. L. Morrison},
 journal   = {J. Low Temp. Phys.},
 title     = {Derivation of the Landau quantum hydrodynamics for interacting Bose systems},
 volume    = {1},
 pages     = {65-71},
 year      = {1969},
}

@article{landau:JPUSSR:1941,
 author    = {L. D. Landau},
 journal   = {J. Phys. (USSR)},
 title     = {The theory of superfluidity of helium II},
 volume    = {5},
 pages     = {71--100},
 year      = {1941},
}

@article{london:RMP:1945,
 author    = {F. London},
 journal   = {Rev. Mod. Phys.},
 title     = {Planck's constant and low temperature transfer},
 volume    = {17},
 pages     = {310-320},
 year      = {1945},
}

@article{fetter:JPCM:2001,
 author    = {A. L. Fetter and A. A. Svidzinsky},
 journal   = {J. Phys.: Condens. Matter},
 title     = {Vortices in a trapped dilute Bose-Einstein condensate},
 volume    = {13},
 pages     = {R135-R194},
 year      = {2001},
}

@article{moshinsky:PhysRev:1952,
 author    = {M. Moshinsky},
 journal   = {Phys. Rev.},
 title     = {Diffraction in time},
 volume    = {88},
 pages     = {625-631},
 year      = {1952},
}

@article{moshinsky:PhysRev:1951,
 author    = {M. Moshinsky},
 journal   = {Phys. Rev.},
 title     = {Boundary conditions and time-dependent states},
 volume    = {84},
 pages     = {525-532},
 year      = {1951},
}

@article{moshinsky:AJP:1976,
 author    = {M. Moshinsky},
 journal   = {Am. J. Phys.},
 title     = {Diffraction in time and the time-energy uncertainty relation},
 volume    = {44},
 pages     = {1037-1042},
 year      = {1976},
}

@article{kleber:PhysRep:1994,
 author    = {M. Kleber},
 journal   = {Phys. Rep.},
 title     = {Exact solutions for time-dependent phenomena in quantum mechanics},
 volume    = {236},
 pages     = {331-393},
 year      = {1994},
}

@article{muga:PhysRep:2009,
 author    = {A. del Campo and G. Garc{\'\i}a-Calder\'on and J. G. Muga},
 journal   = {Phys. Rep.},
 title     = {Quantum transients},
 volume    = {476},
 pages     = {1-50},
 year      = {2009},
}

@article{muga:JPA:2006,
 author    = {A. del Campo and J. G. Muga},
 journal   = {J. Phys. A},
 title     = {Matter-wave diffraction in time with a linear potential},
 volume    = {39},
 pages     = {5897-5906},
 year      = {2006},
}

@article{dalibard:PRL:1996,
 author    = {A. Szriftgiser and D. Gu\'ery-Odelin and M. Arndt and J. Dalibard},
 journal   = {Phys. Rev. Lett.},
 title     = {Atomic wave diffraction and interference using temporal slits},
 volume    = {77},
 pages     = {4-7},
 year      = {1996},
}

@article{brukner:PRA:1997,
 author    = {\v{C}. Brukner and A. Zeilinger},
 journal   = {Phys. Rev. A},
 title     = {Diffraction of matter waves in space and in time},
 volume    = {56},
 pages     = {3804-3824},
 year      = {1997},
}

@article{goussev:PRA:2013,
 author    = {A. Goussev},
 journal   = {Phys. Rev. A},
 title     = {Diffraction in time: An exactly solvable model},
 volume    = {87},
 pages     = {053621(1-4)},
 year      = {2013},
}

@article{dorlas:IJTP:2014,
 author    = {M Beau and T. C. Dorlas},
 journal   = {Int. J. Theor. Phys.},
 title     = {Three-dimensional quantum slit diffraction and diffraction in time},
 volume    = {54},
 pages     = {1882-1907},
 year      = {2015},
}

@article{horwitz:FoundPhys:2007,
 author    = {L. P. Horwitz},
 journal   = {Found. Phys.},
 title     = {Quantum interference in time},
 volume    = {37},
 pages     = {734-746},
 year      = {2007},
}

@article{talbot:PhilMag:1836,
	author = {H. F. Talbot},
	title = {LXXVI. Facts relating to optical science. No. IV},
	journal = {London Edinburgh Philos. Mag. \& J. Sci.e},
	volume = {9},
	number = {56},
	pages = {401--407},
	year = {1836},
	publisher = {Taylor \& Francis},
	doi = {10.1080/14786443608649032},
	URL = {https://doi.org/10.1080/14786443608649032},
	eprint = {https://doi.org/10.1080/14786443608649032},
}

@article{rayleigh:PhilosMag:1881,
	author = {Lord Rayleigh},
	title = {XXV. On copying diffraction-gratings, and on some phenomena connected therewith },
	journal = {London Edinburgh Philos. Mag. \& J. Sci.e},
	volume = {11},
	number = {67},
	pages = {196--205},
	year = {1881},
	publisher = {Taylor \& Francis},
	doi = {10.1080/14786448108626995},
	URL = {https://doi.org/10.1080/14786448108626995},
	eprint = {https://doi.org/10.1080/14786448108626995},
}

@article{arndt:OptExpress:2009,
 author    = {W. B. Case and M. Tomandl and S. Deachapunya and M. Arndt},
 journal   = {Opt. Express},
 title     = {Realization of optical carpets in the {talbot} and {Talbot-Lau} configurations},
 volume    = {17},
 pages     = {20966-20974},
 year      = {2009},
}

@article{wang:PRL:2017,
 author    = {X. Wang and H. Chen and H. Liu and L. Xu and Ch. Sheng and Sh. Zhu},
 journal   = {Phys. Rev. Lett.},
 title     = {Self-focusing and the {Talbot} effect in conformal transformation optics},
 volume    = {119},
 pages     = {033902(1-5)},
 year      = {2017},
}

@article{cronin:NJP:2009,
 author    = {B. J. McMorran and A. D. Cronin},
 journal   = {New J. Phys.},
 title     = {An electron {talbot} interferometer},
 volume    = {11},
 pages     = {033021(1-7)},
 year      = {2009},
}

@article{pritchard:PRA:1995,
 author    = {M. S. Chapman and Ch. R. Ekstrom and T. D. Hammond and J. Schmiedmayer and B. R. Tannian and S. Wehinger and D. E. Pritchard},
 journal   = {Phys. Rev. A},
 title     = {Near-field imaging of atom diffraction gratings: The atomic {talbot} effect},
 volume    = {51},
 pages     = {R14-R17},
 year      = {1995},
}

@article{arndt:PRL:2002,
 author    = {B. Brezger and L. Hackerm\"uller and S. Uttenthaler and J. Petschinka and M. Arndt and A. Zeilinger},
 journal   = {Phys. Rev. Lett.},
 title     = {Matter-Wave interferometer for large molecules},
 volume    = {88},
 pages     = {100404(1-4)},
 year      = {2002},
}

@BOOK{agrawal-bk:2010,
  AUTHOR     = {G. P. Agrawal},
  TITLE      = {Fiber-Optic Communication Systems},
  PUBLISHER  = {Wiley},
  YEAR       = {2010},
  address    = {Hoboken, NJ},
  edition    = {4th},
}

@article{wojcik:PRL:2000,
 author    = {D. W\'ojcik and I. Bia{\l}ynicki-Birula and D. \.{Z}yczkowski},
 journal   = {Phys. Rev. Lett.},
 title     = {Time evolution of quantum fractals},
 volume    = {85},
 pages     = {5022-5025},
 year      = {2000},
 doi       = {10.1103/PhysRevLett.85.5022},
}

@article{berry:PhysWorld:2001,
 author    = {M. Berry and I. Marzoli and W. Schleich},
 journal   = {Phys. World},
 title     = {Quantum carpets, carpets of light},
 volume    = {14},
 number = {6},
 pages     = {39-43},
 year      = {2001},
 doi = {10.1088/2058-7058/14/6/30},
 url = {https://dx.doi.org/10.1088/2058-7058/14/6/30},
}

@article{kaplan:PRA:2000,
 author    = {A. E. Kaplan and I. Marzoli and W. E. Lamb, Jr. and W. P. Schleich},
 journal   = {Phys. Rev. A},
 title     = {Multimode interference: Highly regular pattern formation in quantum wave-packet evolution},
 volume    = {61},
 pages     = {032101-032107},
 year      = {2000},
}

@article{kaplan:PhysScr:1998,
 author    = {A. E. Kaplan and P. Stifter and K. A. H. van Leeuwen and W. E. Lamb, Jr. and W. P. Schleich},
 journal   = {Phys. Scr.},
 title     = {Intermode traces -- Fundamental interference phenomenon in quantum and wave physics},
 volume    = {T76},
 pages     = {93-97},
 year      = {1998},
}

@article{marzoli:ActaPhysSlo:1998,
 author    = {I. Marzoli and F. Saif and I. Bialynicki-Birula and O. M. Friesch and A. E. Kaplan and W. P. Schleich},
 journal   = {Acta Phys. Slovaca},
 title     = {Quantum carpets made simple},
 volume    = {48},
 pages     = {323-333},
 year      = {1998},
}

@article{robinett:PhysRep:2004,
 author    = {R. W. Robinett},
 journal   = {Phys. Rep.},
 title     = {Quantum wave packet revivals},
 volume    = {392},
 pages     = {1-119},
 year      = {2004},
}

@article{robinett:AJP:2000,
 author    = {R. W. Robinett},
 journal   = {Am. J. Phys.},
 title     = {Visualizing the collapse and revival of wave packets in the infinite square well using expectation values},
 volume    = {68},
 pages     = {410},
 year      = {2000},
}

@article{sanz:FrontPhys:2019,
 author    = {A. S. Sanz},
 journal   = {Front. Phys.},
 title     = {Bohm's approach to quantum mechanics: Alternative theory or practical picture?},
 volume    = {14},
 pages     = {11301},
 year      = {2019},
 doi       = {https://doi.org/10.1007/s11467-018-0853-4},
 url       = {https://link.springer.com/article/10.1007/s11467-018-0853-4}
}

@BOOK{ashcroft-bk,
  AUTHOR     = {N. W. Ashcroft and N. D. Mermin},
  TITLE      = {Solid State Physics},
  PUBLISHER  = {Harcourt College Publishers},
  YEAR       = {1976},
  address    = {Fort Worth, USA},
}

@article{sanz:JPhysConfSer:2014,
 author    = {A. S. Sanz},
 journal   = {J. Phys.: Conf. Ser.},
 title     = {Particles, waves and trajectories: 210 years after Young's experiment},
 volume    = {504},
 pages     = {012028(1-14)},
 year      = {2014},
}

@article{sanz:PRA:2017,
 author    = {A. S. Sanz and M. Davidovi\'c and M. Bo\v{z}i\'c},
 journal   = {Phys. Rev. A},
 title     = {Bohmian approach to Gaussian-Maxwell beams},
 volume    = {},
 pages     = {1-15},
 year      = {submitted, 2017},
}

@article{keith:PRL:1991,
 author    = {D. W. Keith and C. R. Ekstrom and Q. A. Turchette and D. E. Pritchard},
 journal   = {Phys. Rev. Lett.},
 title     = {An interferometer for atoms},
 volume    = {66},
 pages     = {2693-2696},
 year      = {1991},
}

@article{sanz:PhysScr:2019,
 author    = {J. Tounli and A. Alvarado and A. S. Sanz},
 journal   = {Phys. Scr.},
 title     = {Boundary bound diffraction: A combined spectral and Bohmian mechanics},
 volume    = {94},
 pages     = {035202(1-15)},
 year      = {2019},
 doi       = {10.1088/1402-4896/aaf484},
}

@article{toennies:PRL:1999-1,
 author    = {R. E. Grisenti and W. Sch\"ollkopf and J. P. Toennies},
 journal   = {Phys. Rev. Lett.},
 title     = {Determination of atom-surface van der Waals potentials from transmission-grating diffraction intensities},
 volume    = {83},
 pages     = {1755-1758},
 year      = {1999},
}

@article{toennies:PRL:2000,
 author    = {R. E. Grisenti and W. Sch\"ollkopf and J. P. Toennies and G. C. Hegerfeldt and T. K\"ohler and M. Stoll},
 journal   = {Phys. Rev. Lett.},
 title     = {Determination of the bond length and binding energy of the Helium dimer by diffraction from a transmission grating},
 volume    = {85},
 pages     = {2284-2287},
 year      = {2000},
}

@article{toennies:PRA:2000,
 author    = {R. E. Grisenti and W. Sch\"ollkopf and J. P. Toennies and J. R. Manson},
 journal   = {Phys. Rev. Lett.},
 title     = {He-atom diffraction from nanostructure transmission gratings: The role of imperfections},
 volume    = {61},
 pages     = {033608(1-15)},
 year      = {2000},
}

@article{toennies:science:1994,
 author    = {W. Sch\"ollkopf and J. P. Toennies},
 journal   = {Science},
 title     = {Nondestructive mass selection of small van der waals clusters},
 volume    = {266},
 pages     = {1345-1348},
 year      = {1994},
}

@article{toennies:PRL:1999-2,
 author    = {R. B. Doak and R. E. Grisenti and S. Rehbein and G. Schmahl and J. P. Toennies and Ch. W\"oll},
 journal   = {Phys. Rev. Lett.},
 title     = {Towards realization of an atomic de Broglie microscope: Helium atom focusing using Fresnel zone plates},
 volume    = {83},
 pages     = {4229-4232},
 year      = {1999},
}

@article{phillips:rmp:1998,
 author    = {W. D. Phillips},
 journal   = {Rev. Mod. Phys.},
 title     = {Laser cooling and trapping of neutral atoms},
 volume    = {70},
 pages     = {721-741},
 year      = {1998},
}

@article{grimm:aamop:2000,
 author    = {R. Grimm and M. Weidem\"uller and Yu. B. Ovchinnikov},
 journal   = {Adv. At. Mol. Opt. Phys.},
 title     = {Optical dipole traps for neutral atoms},
 volume    = {42},
 pages     = {95-170},
 year      = {2000},
}

@article{einstein:AnnPhys:1905-1,
 author    = {A. Einstein},
 journal   = {Ann. Phys.},
 title     = {\"Uber einen die Erzeugung und Verwandlung des Lichtes betreffenden heuristischen Gesichtspunkt},
 volume    = {17},
 pages     = {132-148},
 year      = {1905},
}

@article{arndt:NaturePhys:2014,
 author    = {M. Arndt and K. Hornberger},
 journal   = {Nature Phys.},
 title     = {Testing the limits of quantum mechanical superpositions},
 volume    = {10},
 pages     = {271-277},
 year      = {2014},
}

@article{taylor:ProcCambPhilSoc:1909,
 author    = {G. I. Taylor},
 journal   = {Proc. Camb. Philos. Soc.},
 title     = {Interference fringes with feeble light},
 volume    = {15},
 pages     = {114-115},
 year      = {1909},
}

@article{heisenberg:ZPhys:1925,
 author    = {W. Heisenberg},
 journal   = {Z. Phys.},
 title     = {\"Uber quantentheoretische Umdeutung kinematischer und mechanischer Beziehungen},
 volume    = {33},
 pages     = {879-880},
 year      = {1925},
}

@article{richardson:PRA:2014,
 author    = {Ch. D. Richardson and P. Schlagheck and J. Martin and N. Vandewalle and T. Bastin},
 journal   = {Phys. Rev. A},
 title     = {Nonlinear Schr\"odinger wave equation with linear quantum behavior},
 volume    = {89},
 pages     = {032118},
 year      = {2014},
}

@article{chou:AOP:2016,
 author    = {C.-C. Chou},
 journal   = {Ann. Phys.},
 title     = {Trajectory description of the quantum-classical transition for wave packet interference},
 volume    = {371},
 pages     = {437-459},
 year      = {2016},
}

@BOOK{Shizgal-bk:2015,
  AUTHOR     = {B. Shizgal},
  TITLE      = {Spectral Methods in Chemistry and Physics: Applications to Kinetic Theory and Quantum Mechanics},
  PUBLISHER  = {Springer},
  series     = {Scientific Computation},
  YEAR       = {2015},
  address    = {Heidelberg},
}

@INBOOK{calvo-waveguides-bk,
  AUTHOR =       {R. F. \'Alvarez-Estrada and M. L. Calvo},
  editor =       {M. L. Calvo and V. Lakshminarayanan},
  TITLE =        {Optical Waveguides: From Theory to Applied Technologies},
  CHAPTER =      {Neutron Waveguides and Applications},
  pages =        {331-385},
  PUBLISHER =    {CRC Press},
  YEAR =         {2007},
  address =      {New York},
}

@article{hofmann:chemrev:1996,
 author    = {F. Hofmann and J. P. Toennies},
 journal   = {Chem. Rev.},
 title     = {High-resolution helium atom time-of-flight spectroscopy of low-frequency vibrations of adsorbates},
 volume    = {96},
 pages     = {1307-1326},
 year      = {1996},
 doi       = {10.1021/cr9502209},
}

@article{lahee:JCP:1987,
 author    = {A. M. Lahee and J. R. Manson and J. P. Toennies and Ch. W\"oll},
 journal   = {J. Chem. Phys.},
 title     = {Helium atom differential cross sections for scattering from single adsorbed CO molecules on a Pt(111) surface},
 volume    = {86},
 pages     = {7194-7203},
 year      = {1987},
 doi       = {10.1063/1.452321},
}

@article{lahee:PRL:1986,
 author    = {A. M. Lahee and J. R. Manson and J. P. Toennies and Ch. W\"oll},
 journal   = {Phys. Rev. Lett.},
 title     = {Observation of interference oscillations in helium scattering from single surface defects},
 volume    = {57},
 pages     = {471-474},
 year      = {1986},
 doi       = {10.1103/PhysRevLett.57.471},
}

@article{yinnon:JCP:1988,
 author    = {A. T. Yinnon and R. Kosloff and R. B. Gerber},
 journal   = {J. Chem. Phys.},
 title     = {Atom scattering from isolated adsorbates on surfaces: Rainbows, diffraction interferences, and trapping resonances},
 volume    = {88},
 pages     = {7209-7220},
 year      = {1988},
 doi       = {10.1063/1.454373},
}

@article{lemoine:JCP:1994-1,
 author    = {M.-N. Carr\'e and D. Lemoine},
 journal   = {J. Chem. Phys.},
 title     = {Fully quantum study of the 3D diffractive scattering of He from isolated CO adsorbates on Pt(111)},
 volume    = {101},
 pages     = {5305-5312},
 year      = {1994},
 doi       = {10.1063/1.467384},
}

@article{lemoine:PRL:1998,
 author    = {D. Lemoine},
 journal   = {Phys. Rev. Lett.},
 title     = {Atomic scattering from single adsorbates: What can we learn from the gas phase?},
 volume    = {81},
 pages     = {461-464},
 year      = {1998},
 doi       = {10.1103/PhysRevLett.81.461},
}

@article{kleyn:physrep:1991,
 author    = {A. W. Kleyn and T. C. M. Horn},
 journal   = {Phys. Rep.},
 title     = {Rainbow scattering from solid surfaces},
 volume    = {199},
 pages     = {191-230},
 year      = {1991},
 doi       = {10.1016/0370-1573(91)90032-H},
}

@article{drolshagen:JCP:1987,
 author    = {G. Drolshagen and R. Vollmer},
 journal   = {J. Chem. Phys.},
 title     = {Atom scattering from surfaces with isolated impurities: Calculations for hard wall and soft potentials},
 volume    = {87},
 pages     = {4948-4957},
 year      = {1987},
 doi       = {10.1063/1.452807},
}

@article{graham:JCP:1996,
 author    = {A. P. Graham and F. Hofman and J. P. Toennies and J. R. Manson},
 journal   = {J. Chem. Phys.},
 title     = {Helium atom scattering from isolated CO molecules on copper(001)},
 volume    = {105},
 pages     = {2093-2098},
 year      = {1996},
 doi       = {10.1063/1.472075},
}

@article{choi:JCP:1997-1,
 author    = {B. H. Choi and K. T. Tang and J. P. Toennies},
 journal   = {J. Chem. Phys.},
 title     = {Interpretation of helium atom scattering from isolated CO molecules on copper (001) based on an exact quantum mechanical model},
 volume    = {107},
 pages     = {1631-1633},
 year      = {1997},
 doi       = {10.1063/1.474514},
}

@article{choi:JCP:1997-2,
 author    = {B. H. Choi and K. T. Tang and J. P. Toennies},
 journal   = {J. Chem. Phys.},
 title     = {Quantum-mechanical scattering of an atom from a rigid hemisphere on a flat surface},
 volume    = {107},
 pages     = {9437-9446},
 year      = {1997},
 doi       = {10.1063/1.475240},
}

@article{choi:JCP:2000,
 author    = {B. H. Choi and A. P. Graham and K. T. Tang and J. P. Toennies},
 journal   = {J. Chem. Phys.},
 title     = {Helium atom scattering from isolated CO molecules on a Pt(111) surface: Experiment versus close-coupling calculations for a realistic He-CO potential},
 volume    = {112},
 pages     = {10538-10547},
 year      = {2000},
 doi       = {10.1063/1.481687},
}

@article{drolshagen:surfsci:1984,
 author    = {G. Drolshagen and E. J. Heller},
 journal   = {Surf. Sci.},
 title     = {A wavepacket approach to gas-surface scattering: Application to surfaces with imperfections},
 volume    = {139},
 pages     = {260-280},
 year      = {1984},
 doi       = {10.1016/0039-6028(84)90021-9},
}

@article{lemoine:JCP:1994-2,
 author    = {D. Lemoine},
 journal   = {J. Chem. Phys.},
 title     = {Quantum flux analysis of the scattering of oriented NO molecules from surfaces},
 volume    = {101},
 pages     = {4343-4356},
 year      = {1994},
 doi       = {10.1063/1.467485},
}

@article{gerber:CPL:1984,
 author    = {R. B. Gerber and A. T. Yinnon and R. Kosloff},
 journal   = {Chem. Phys. Lett.},
 title     = {Effects of isolated impurities on atom scattering from crystalline surfaces: Exact quantum-mechanical calculations},
 volume    = {105},
 pages     = {523-526},
 year      = {1984},
 doi       = {10.1016/0009-2614(84)80103-7},
}

@BOOK{joachain-bk,
  AUTHOR     = {C. J. Joachain},
  TITLE      = {Quantum Collision Theory},
  PUBLISHER  = {North-Holland},
  YEAR       = {Amsterdam},
  address    = {1975},
}

@article{glebov:PRL:1997,
 author    = {A. Glebov and J. R. Manson and Skofronick and J. P. Toennies},
 journal   = {Phys. Rev. Lett.},
 title     = {Defect-mediated diffraction resonances in surface scattering},
 volume    = {78},
 pages     = {1508-1511},
 year      = {1997},
 doi       = {10.1103/PhysRevLett.78.1508},
}

@article{farias:repprogphys:1998,
 author    = {D. Far{\'\i}as and K.-H. Rieder},
 journal   = {Rep. Prog. Phys.},
 title     = {Atomic beam diffraction from solid surfaces},
 volume    = {61},
 pages     = {1575-1664},
 year      = {1998},
 doi       = {10.1088/0034-4885/61/12/001},
}

@article{davidovic:JRLR:2017,
 author    = {M. D. Davidovi\'c and M. D. Davidovi\'c and A. S. Sanz and M. Bo\v{z}i\'c and D. Vasiljevi\'c},
 journal   = {J. Russ. Laser Res.},
 title     = {Trajectory-based interpretation of the laser light diffraction by a sharp edge},
 pages     = {438-447},
 volume    = {39},
 year      = {2018},
}

@BOOK{collett-spie,
  AUTHOR     = {E. Collett},
  TITLE      = {Field Guide to Polarization},
  PUBLISHER  = {SPIE},
  YEAR       = {2005},
  address    = {Bellingham, Washington USA},
}

@inproceedings{sbitnev:InTech:2012,
   author = {V. I. Sbitnev},
  chapter = {Bohmian trajectories and the path integral paradigm -- Complexified Lagrangian mechanics},
booktitle = {Theoretical Concepts of Quantum Mechanics},
     year = {2012},
   editor = {M. R. Pahlavani},
    pages = {313-334},
publisher = {InTech},
  address = {Rijeka},
}

@inproceedings{sbitnev:InTech:2013,
   author = {V. I. Sbitnev},
  chapter = {Generalized path integral technique: nanoparticles incident on a slit grating, matter wave interference},
booktitle = {Advances in Quantum Mechanics},
     year = {2013},
   editor = {P. Bracken},
    pages = {183-211},
publisher = {InTech},
  address = {Rijeka},
}

@article{sbitnev:FoundPhys:2016,
 author    = {V. I. Sbitnev},
 journal   = {Found. Phys.},
 title     = {Hydrodynamics of the physical vacuum: I. Scalar quantum sector},
 volume    = {46},
 pages     = {606-619},
 year      = {2016},
 doi       = {10.1007/s10701-015-9980-8},
}

@article{bohm:PhysRep:1989,
 author    = {D. Bohm and B. J. Hiley},
 journal   = {Phys. Rep.},
 title     = {Non-Locality and Locality in the Stochastic Interpretation of Quantum Mechanics},
 volume    = {172},
 pages     = {93-122},
 year      = {1989},
}

@article{struyve:JPA:2018,
 author    = {R. Dubertrand and J.-B. Shim and W. Struyve},
 journal   = {J. Phys. A},
 title     = {Bohmian trajectories for the half-line barrier},
 volume    = {51},
 pages     = {085302(1-22)},
 year      = {2018},
}

@BOOK{gilder-bk,
  AUTHOR     = {L. Gilder},
  TITLE      = {The Age of Entanglement. When Quantum Physics was Reborn},
  PUBLISHER  = {Alfred A. Knopf},
  YEAR       = {2008},
  address    = {New York},
}

@BOOK{aczel-bk,
  AUTHOR     = {A. D. Aczel},
  TITLE      = {Entanglement. The Greatest Mystery in Physics},
  PUBLISHER  = {Four Walls Eight Windows},
  YEAR       = {2001},
  address    = {New York},
}

@article{azanna:optica:2018,
 author    = {L. Romero Cort\'es and M. Seghilani and R. Maram and J. Aza{\~n}a},
 journal   = {Optica},
 title     = {Full-field broadband invisibility through reversible wave frequency-spectrum control},
 volume    = {5},
 pages     = {779-786},
 year      = {2018},
}

@article{choi:OptExp:2014,
 author    = {J. S. Choi and J. C. Howell},
 journal   = {Opt. Express},
 title     = {Paraxial ray optics cloaking},
 volume    = {22},
 pages     = {29465-29478},
 year      = {2014},
}

@article{choi:OptExp:2015,
 author    = {J. S. Choi and J. C. Howell},
 journal   = {Opt. Express},
 title     = {Paraxial full-field cloaking},
 volume    = {23},
 pages     = {15857-15862},
 year      = {2015},
}

@BOOK{milton-bk,
  AUTHOR     = {M. Katz},
  TITLE      = {Introduction to Geometrical Optics},
  PUBLISHER  = {World Scientific},
  YEAR       = {2002},
  address    = {New Jersey},
}

@BOOK{pedrotti-bk,
  AUTHOR     = {F. L. Pedrotti and L. M. Pedrotti and L. S. Pedrotti},
  TITLE      = {Introduction to Optics},
  PUBLISHER  = {Pearson},
  YEAR       = {2014},
  address    = {UK},
}

@article{smith:Science:2006,
 author    = {D. Schurig and J. J. Mock and B. J. Justice and S. A. Cummer and J. B. Pendry and A. F. Starr and D. R. Smith},
 journal   = {Science},
 title     = {Metamaterial electromagnetic cloak at microwave frequencies},
 volume    = {314},
 pages     = {977-980},
 year      = {2006},
}

@article{engheta:PRE:2005,
 author    = {A. Al\`u and N. Engheta},
 journal   = {Phys. Rev. E},
 title     = {Achieving transparency with plasmonic and metamaterial coatings},
 volume    = {72},
 pages     = {016623(1-9)},
 year      = {2005},
}

@article{engheta:PRE:2006,
 author    = {A. Al\`u and N. Engheta},
 journal   = {Phys. Rev. E},
 title     = {Erratum: Achieving transparency with plasmonic and metamaterial coatings [Phys. Rev. E, 72, 016623 (2005)]},
 volume    = {73},
 pages     = {019906(E)},
 year      = {2006},
}

@article{shalaev:NatPhot:2007,
 author    = {W. Cai and U. K. Chettiar and A. V. Kildishev and V. M. Shalaev},
 journal   = {Nat. Photon.},
 title     = {Optical cloaking with metamaterials},
 volume    = {1},
 pages     = {224-227},
 year      = {2007},
}

@BOOK{steinmeyer-bk,
  AUTHOR     = {J. Steinmeyer},
  TITLE      = {Hiding the Elephant -- How Magicians Invented the Impossible and Learned to Disappear},
  PUBLISHER  = {Carroll \& Graf Publishers},
  YEAR       = {2003},
  address    = {New York},
}

@article{zepf:physteach:2004,
 author    = {T. H. Zepf},
 journal   = {Physics Teacher},
 title     = {The Haunted Physics Lab},
 volume    = {42},
 pages     = {404-408},
 year      = {2004},
}

@article{marques:AJP:2011,
 author    = {M. C. Vel\'azquez-Ahumada and M. J. Freire and J. M. Algar{\'\i}n and R. Marques},
 journal   = {Am. J. Phys.},
 title     = {Demonstration of negative refraction of microwaves},
 volume    = {79},
 pages     = {349-352},
 year      = {2011},
}

@article{gennaro:AJP:2016,
 author    = {J. T. Wilkinson and Ch. B. Whitehouse and R. F. Oulton and S. D. Gennaro},
 journal   = {Am. J. Phys.},
 title     = {An undergraduate experiment demonstrating the physics of metamaterials with acoustic waves and soda cans},
 volume    = {84},
 pages     = {14-20},
 year      = {2016},
}

@article{fleming:AJP:2017,
 author    = {S. Fleming},
 journal   = {Am. J. Phys.},
 title     = {Metamaterial hyperlens demonstration of propagation without diffraction},
 volume    = {85},
 pages     = {173-177},
 year      = {2017},
}

@article{thompson:AJP:2008,
 author    = {M. Sipos and B. G. Thompson},
 journal   = {Am. J. Phys.},
 title     = {Electrodynamics on a grid: The finite-difference time-domain method applied to optics and cloaking},
 volume    = {76},
 pages     = {464-469},
 year      = {2008},
}

@article{longhi:AJP:2017,
 author    = {S. A. R. Horsley and S. Longhi},
 journal   = {Am. J. Phys.},
 title     = {One-way invisibility in isotropic dielectric optical media},
 volume    = {85},
 pages     = {439-446},
 year      = {2017},
}

@article{choi:ApplOpt:2014,
 author    = {J. C. Howell and J. B. Howell and J. S. Choi},
 journal   = {Appl. Opt.},
 title     = {Amplitude-only, passive, broadband, optical spatial cloaking of very large objects},
 volume    = {53},
 pages     = {1958-1963},
 year      = {2014},
}

@article{sanchezsoto:EJP:2008,
 author    = {J. J. Monz\'on and A. G. Barriuso and L. L. S\'anchez-Soto},
 journal   = {Eur. J. Phys.},
 title     = {Geometric picture of optical complementary media},
 volume    = {29},
 pages     = {431-437},
 year      = {2008},
}

@article{sanchezsoto:PhysRep:2012,
 author    = {L. L. S\'anchez-Soto and J. J. Monz\'on and A. G. Barriuso and J. F. Cari{\~n}ena},
 journal   = {Phys. Rep.},
 title     = {The transfer matrix: A geometrical perspective},
 volume    = {513},
 pages     = {191-227},
 year      = {2013},
}

@BOOK{rowling:HarryPotter:2007,
  AUTHOR     = {J. K. Rowling},
  TITLE      = {Harry Potter and the Deathly Hallows},
  PUBLISHER  = {Bloomsbury Publishing},
  YEAR       = {2007},
  address    = {New York},
  edition    = {1st},
}

@article{durt:EPL:2016,
 author    = {Th. Durt},
 journal   = {EPL},
 title     = {Generalized guidance equation for peaked quantum solitons and effective gravity},
 volume    = {114},
 pages     = {10004(1-6)},
 year      = {2016},
}

@article{pope:FrontPhys:2017,
 author    = {Th. Pope and W. Hofer},
 journal   = {Front. Phys.},
 title     = {Spin in the extended electron model},
 volume    = {12},
 pages     = {128503(1-5)},
 year      = {2017},
}

@article{long:SciChina:2018,
 author    = {G.-L. Long and W. Qin and Zh. Yang and J.-L. Li},
 journal   = {Sci. China-Phys. Mech. Astron.},
 title     = {Realistic interpretation of quantum mechanics and encounter-delayed-choice experiment},
 volume    = {61},
 pages     = {030311(1-8)},
 year      = {2018},
}

@article{zhou:SciBull:2017,
 author    = {Zh.-Y. Zhou and Zh.-H. Zhu and Sh.-L. Liu and Y.-H. Li and Sh. Shi and D.-Sh. Ding and L.-X. Chen and W. Gao and G.-C. Guo and B.-S. Shi},
 journal   = {Sci. Bull.},
 title     = {Quantum twisted double-slits experiments: confirming wavefunctions' physical reality},
 volume    = {62},
 pages     = {1185-1192},
 year      = {2017},
}

@article{yuan:LSA:2016,
 author    = {G. H. Yuan and S. Vezzoli and Ch. Altuzarra and E. T. F. Rogers and Ch. Couteau and C. Soci and N. I. Zheludev},
 journal   = {Light-Sci. Appl.},
 title     = {Quantum super-oscillation of a single photon},
 volume    = {5},
 pages     = {e16127(1-6)},
 year      = {2016},
}

@article{li:EPL:2017,
 author    = {Zh.-Y. Li},
 journal   = {EPL},
 title     = {Weak-measurement Mach-Zehnder interferometer for testing wave-particle duality},
 volume    = {117},
 pages     = {50005(1-6)},
 year      = {2017},
}

@BOOK{rauch-bk,
  AUTHOR     = {H. Rauch and S. A. Werner},
  TITLE      = {Neutron Interferometry. Lessons in Experimental Quantum Mechanics},
  PUBLISHER  = {Oxford University Press},
  YEAR       = {2000},
  address    = {New York},
}

@BOOK{rauch-bk-2,
  AUTHOR     = {H. Rauch and S. A. Werner},
  TITLE      = {Neutron Interferometry. Lessons in Experimental Quantum Mechanics, Wave-Particle Duality, and Entanglement},
  PUBLISHER  = {Oxford University Press},
  YEAR       = {2015},
  address    = {New York},
}

@BOOK{willis-bk,
  AUTHOR     = {B. T. M. Willis and C. J. Carlile},
  TITLE      = {Experimental Neutron Scattering},
  PUBLISHER  = {Oxford University Press},
  YEAR       = {2009},
  address    = {Oxford University Press},
}

@article{klein:RPP:1983,
 author    = {A. G. Klein and S. A. Werner},
 journal   = {Rev. Prog. Phys.},
 title     = {Neutron optics},
 volume    = {46},
 pages     = {259-335},
 year      = {1983},
}

@article{hasegawa:physicaB:2011,
 author    = {K. Durstberger-Rennhofer and Y. Hasegawa},
 journal   = {Physica B},
 title     = {Energy entanglement in neutron interferometry},
 volume    = {406},
 pages     = {2373-2376},
 year      = {2011},
}

@article{hasegawa:physicaB:2018,
 author    = {T. Denkmayr and J. Dressel and H. Geppert-Kleinrath and Y. Hasegawa and S. Sponar},
 journal   = {Physica B},
 title     = {Weak values from strong interactions in neutron interferometry},
 volume    = {551},
 pages     = {339-346},
 year      = {2018},
}

@article{dewdney:PhysLett:1985,
 author    = {C. Dewdney},
 journal   = {Phys. Lett.},
 title     = {Particle trajectories and interference in a time-dependent model of neutron single crystal interferometry},
 volume    = {109A},
 pages     = {377-384},
 year      = {1985},
}

@BOOK{sanz:neutron:2020,
  AUTHOR     = {A. S. Sanz},
  editor     = {M. L. Calvo and R. F. \'Alvarez-Estrada},
  title      = {Advances in Neutron Optics},
  CHAPTER    = {Neutron matter-wave diffraction: a computational perspective},
  pages      = {79-122},
  publisher  = {CRC Press},
  year       = {2020},
  address    = {Boca Rat\'on, FL},
}

@BOOK{bohm-bk:QTh,
  AUTHOR     = {D. Bohm},
  TITLE      = {Quantum Theory},
  PUBLISHER  = {Dover (first printed by Prentice Hall in 1951)},
  YEAR       = {1989},
  address    = {New York},
}

@article{bennet:PRL:1993,
 author    = {Ch. H. Bennett and G. Brassard and C. Cr\'epeau and R. Jozsa and A. Peres and W. K. Wootters},
 journal   = {Phys. Rev. Lett.},
 title     = {Teleporting an unknown quantum state via dual classical and Einstein-Podolsky-Rosen channels},
 volume    = {70},
 pages     ={1895-1899},
 year      = {1993},
}

@article{bouwmeester:nature:1997,
 author    = {D. Bouwmeester and J.-W. Pan and K. Mattle and M. Eibl and H. Weinfurter and A. Zeilinger},
 journal   = {Nature},
 title     = {Experimental quantum teleportation},
 volume    = {390},
 pages   = {575-579},
 year      = {1997},
}

@article{zeilinger:nature:2003,
 author    = {I. Marcikic and H. de Riedmatten and W. Tittel and H. Zbinden and N. Gisin},
 journal   = {Nature},
 title     = {Long-distance teleportation of qubits at telecommunication wavelengths},
 volume    = {421},
 pages   = {509-513},
 year      = {2003},
}

@article{zeilinger:nature:2012,
 author    = {X.-S. Ma and T. Herbst and T. Scheidl and D. Wang and S. Kropatschek and W. Naylor and B. Wittmann and A. Mech and J. Kofler and E. Anisimova and V. Makarov and Th. Jennewein and R. Ursin and A. Zeilinger},
 journal   = {Nature},
 title     = {Quantum teleportation over 143 kilometres using active feed-forward},
 volume    = {489},
 pages   = {269-273},
 year      = {2012},
}

@article{JWPan:science:2017,
 author    = {J. Yin and Y. Cao and Y.-H. Li and Sh.-K. Liao and L. Zhang and J.-G. Ren and W.-Q. Cai and W.-Y. Liu and B. Li and H. Dai and G.-B. Li and Q.-M. Lu and Y.-H. Gong and Y. Xu and Sh.-L. Li and F.-Zh. Li and Y.-Y. Yin and Z.-Q. Jiang and M. Li and J.-J. Jia and G. Ren and D. He and Y.-L. Zhou and X.-X. Zhang and N. Wang and X. Chang and Zh.-C. Zhu and N.-L. Liu and Y.-A. Chen and Ch.-Y. Lu and R. Shu and Ch.-Zh. Peng and J.-Y. Wang and J.-W. Pan},
 journal   = {Science},
 title     = {Satellite-based entanglement distribution over 1200 kilometers},
 volume    = {356},
 pages  = {1140-1144},
 year      = {2017},
}

@article{JWPan:PRL:2017,
 author    = {J. Yin and Y. Cao and Y.-H. Li and J.-G. Ren and S.-K. Liao and L. Zhang and W.-Q. Cai and W.-Y. Liu and B. Li and H. Dai and M. Li and Y.-M. Huang and L. Deng and L. Li and Q. Zhang and N.-L. Liu and Y.-A. Chen and Ch.-Y. Lu and R. Shu and Ch.-Zh. Peng and J.-Y. Wang and J.-W. Pan},
 journal   = {Phys. Rev. Lett.},
 title     = {Satellite-to-ground entanglement-based quantum key distribution},
 volume    = {119},
 pages   ={200501(1-5)},
 year      = {2017},
}

@article{li:SciBull:2016,
 author    = {T.-C. Li and Z.-Q. Yin},
 journal   = {Sci. Bull.},
 title     = {Quantum superposition, entanglement, and state teleportation of a microorganism on an electromechanical oscillator},
 volume    = {61},
 pages   = {163-171},
 year      = {2016},
}

@article{landsman:nature:2019,
 author    = {K. A. Landsman and C. Figgatt and T. Schuster and N. M. Linke and B. Yoshida and N. Y. Yao and C. Monroe},
 journal   = {Nature},
 title     = {Verified quantum information scrambling},
 volume    = {567},
 pages   = {61-64},
 year      = {2019},
}

@article{zelinger-JWPan:PRL:2019,
 author    = {Y.-H. Luo and H.-S. Zhong and M. Erhard and X.-L. Wang and L.-Ch. Peng and M. Krenn and X. Jiang and L. Li and N.-L. Liu and Ch.-Y. Lu and A. Zeilinger and J.-W. Pan},
 journal   = {Phys. Rev. Lett.},
 title     = {Quantum teleportation in high dimensions},
 volume    = {123},
 pages   = {070505(1-4)},
 year      = {2019},
}

@article{kauffman:NJP:2002,
 author    = {L. H. Kauffman and S. J. Lomonaco},
 journal   = {New J. Phys.},
 title     = {Quantum entanglement and topological entanglement},
 volume    = {4},
 pages    = {73(1-18)},
 year      = {2002},
}

@inproceedings{kauffman:QICII:2004,
  AUTHOR     = {L. H. Kauffman and S. J. Lomonaco},
  CHAPTER    = {Quantum knots},
  editor     = {E. Donkor and A. R. Pirich and H. E. Brandt},
  booktitle  = {Quantum Information and Computation II},
  volume   = {5436},
  pages      = {268-284},
  PUBLISHER  = {SPIE},
  YEAR       = {2004},
  address    = {Bellingham, WA},
  series     = {Proc. SPIE},
}

@article{kauffman:OptSpectr:2005,
 author    = {L. H. Kauffman},
 journal   = {Opt. Spectrosc.},
 title     = {Teleportation topology},
 volume    = {99},
 pages   = {227-232},
 year      = {2005},
}

@inproceedings{kauffman:QICII:2014,
  AUTHOR     = {L. H. Kauffman and S. J. Lomonaco},
  CHAPTER    = {Quantum diagrams and quantum networks},
  editor     = {E. Donkor and A. R. Pirich and H. E. Brandt and M. R. Frey and S. J. Lomonaco and J. M. Myers},
  booktitle  = {Quantum Information and Computation II},
  volume   = {9123},
  pages      = {91230P(1-14)},
  PUBLISHER  = {SPIE},
  YEAR       = {2004},
  address    = {Bellingham, WA},
  series     = {Proc. SPIE},
}

@article{kauffman:QIP:2018,
 author    = {L. H. Kauffman and S. J. Lomonaco},
 journal   = {Quantum Inf. Process.},
 title     = {Braiding, Majorana fermions, Fibonacci particles and topological quantum computing},
 volume    = {17},
 pages   = {201(1-81)},
 year      = {2018},
}

@article{kauffman:NJP:2004,
 author    = {L. H. Kauffman and S. J. Lomonaco},
 journal   = {New J. Phys.},
 title     = {Braiding operators are universal quantum gates},
 volume    = {6},
 pages    = {134(1-40)},
 year      = {2004},
}

@article{karlsson:PRA:1998,
 author    = {A. Karlsson and M. Bourennane},
 journal   = {Phys. Rev. A},
 title     = {Quantum teleportation using three-particle entanglement},
 volume    = {58},
 pages     ={4394-4400},
 year      = {1998},
}

@article{mironov:universe:2019,
 author    = {S. Mironov},
 journal   = {Universe},
 title     = {Topological entanglement and knots},
 volume    = {5},
 pages   = {60(1-10)},
 year      = {2019},
}

@article{mironov:JHEP:2019,
 author    = {D. Melnikov and A. Mironov and S. Mironov and A. Morozov and An. Morozov},
 journal   = {J. High Ener. Phys.},
 title     = {From topological to quantum entanglement},
 volume    = {2019},
 pages   = {116(1-12)},
 year      = {2019},
}

@article{quinta:PRA:2018,
 author    = {G. M. Quinta and R. Andr\'e},
 journal   = {Phys. Rev. A},
 title     = {Classifying quantum entanglement through topological links},
 volume    = {97},
 pages   = {042307(1-12)},
 year      = {2018},
}

@article{peres:PRL:1996,
 author    = {A. Peres},
 journal   = {Phys. Rev. Lett.},
 title     = {Separability criterion for density matrices},
 volume    = {77},
 pages  = {1413-1415},
 year      = {1996},
}

@article{horodecki:PLA:1996,
 author    = {M. Horodecki and P. Horodecki and R. Horodecki},
 journal   = {Phys. Lett. A},
 title     = {Separability of mixed states: necessary and sufficient conditions},
 volume    = {223},
 pages  = {1-8},
 year      = {1996},
}

@article{horodecki:PLA:2001,
 author    = {M. Horodecki and P. Horodecki and R. Horodecki},
 journal   = {Phys. Lett. A},
 title     = {Separability of n-particle mixed states: necessary and sufficient conditions in terms of linear maps},
 volume    = {283},
 pages  = {1-7},
 year      = {2001},
}

@article{horodecki:OSID:2006,
 author    = {M. Horodecki and P. Horodecki and R. Horodecki},
 journal   = {Open Sys. Inf. Dyn.},
 title     = {Separability of mixed quantum states: Linear contractions and permutation criteria},
 volume    = {13},
 pages  = {103-111},
 year      = {2006},
}

@article{horodecki:RMP:2009,
 author    = {R. Horodecki and P. Horodecki and M. Horodecki and K. Horodecki},
 journal   = {Rev. Mod. Phys.},
 title     = {Quantum entanglement},
 volume    = {81},
 pages   = {865-942},
 year      = {2009},
}

@article{cirac:PRL:1999,
 author    = {W. D\"ur and J. I. Cirac and R. Tarrach},
 journal   = {Phys. Rev. Lett.},
 title     = {Separability and distillability of multiparticle quantum systems},
 volume    = {83},
 pages   ={3562-3565},
 year      = {1999},
}

@article{cirac:PRA:2000,
 author    = {W. D\"ur and J. I. Cirac},
 journal   = {Phys. Rev. A},
 title     = {Classification of multiqubit mixed states: Separability and distillability properties},
 volume    = {61},
 pages   = {042314(1-11)},
 year      = {2000},
}

@article{gisin:entropy:2019,
 author    = {N. Gisin},
 journal   = {Entropy},
 title     = {Entanglement 25 years after quantum teleportation: testing joint measurements in quantum networks},
 volume    = {21},
 pages     = {325(1-12)},
 year      = {2019},
}

@article{qureshi:AJP:2016,
 author    = {T. Qureshi},
 journal   = {Am. J. Phys.},
 title     = {Quantitative wave-particle duality},
 volume    = {},
 pages     = {},
 year      = {2016},
}

@article{omnes:RMP:1992,
  title = {Consistent interpretations of quantum mechanics},
  author = {Omn\`es, Roland},
  journal = {Rev. Mod. Phys.},
  volume = {64},
  issue = {2},
  pages = {339--382},
  numpages = {0},
  year = {1992},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.64.339},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.64.339}
}


@article{tonomura:PRL:1986,
  title = {Evidence for Aharonov-Bohm effect with magnetic field completely shielded from electron wave},
  author = {Tonomura, Akira and Osakabe, Nobuyuki and Matsuda, Tsuyoshi and Kawasaki, Takeshi and Endo, Junji and Yano, Shinichiro and Yamada, Hiroji},
  journal = {Phys. Rev. Lett.},
  volume = {56},
  issue = {8},
  pages = {792--795},
  numpages = {0},
  year = {1986},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.56.792},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.56.792}
}

@article{heisengerg:ZPhys:1927,
 author    = {W. Heisenberg},
 journal   = {Z. Phys.},
 title     = {\"Uber den anschaulichen Inhalt der quantentheoretischen Kinematik und Mechanik},
 volume    = {43},
 pages     = {172},
 year      = {1927},
}

@article{breitenberger:FoundPhys:1985,
 author    = {E. Breitenberger},
 journal   = {Found. Phys.},
 title     = {Uncertainty measures and uncertainty relations for angle observables},
 volume    = {15},
 pages     = {353-364},
 year      = {1985},
}

@article{stelzer:OptCommun:2000,
 author    = {E. H. Stelzer and S. Grill},
 journal   = {Opt. Commun.},
 title     = {The uncertainty principle applied to estimate focal spot dimensions},
 volume    = {173},
 pages     = {51-56},
 year      = {2000},
}

@article{alonso:JOSAA:2000,
 author    = {M. Alonso and G. Forbes},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Uncertainty products for nonparaxial wave fields},
 volume    = {17},
 pages     = {2391-2402},
 year      = {2000},
}

@article{santarsiero:JOSAA:2006-1,
 author    = {M. Alonso and R. Borghi and M. Santarsiero},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Nonparaxial fields with maximum joint spatial-directional localization. I. Scalar case},
 volume    = {23},
 pages     = {691-700},
 year      = {2006},
}

@article{santarsiero:JOSAA:2006-2,
 author    = {M. Alonso and R. Borghi and M. Santarsiero},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Nonparaxial fields with maximum joint spatial-directional localization. II. Vectorial case},
 volume    = {23},
 pages     = {701-702},
 year      = {2006},
}

@article{chisolm:AJP:2001,
 author    = {E. D. Chisolm},
 journal   = {Am. J. Phys.},
 title     = {Generalizing the Heisenberg uncertainty relation},
 volume    = {69},
 pages     = {368-371},
 year      = {2001},
}

@article{padgett:NJP:2004,
 author    = {S. Franke-Arnold and S. M. Barnett and E. Yao and J. Leach and J. Courtial and M. Padgett},
 journal   = {New J. Phys.},
 title     = {Uncertainty principle for angular position and angular momentum},
 volume    = {6},
 pages     = {103},
 year      = {2004},
}

@article{padgett:JMO:2008,
 author    = {M. Padgett},
 journal   = {J. Mod. Opt.},
 title     = {On the focussing of light, as limited by the uncertainty principle},
 volume    = {55},
 pages     = {3083-3089},
 year      = {2008},
}

@article{ricaud:AdvComputMath:2014,
 author    = {B. Ricaud and B. Torr\'esani},
 journal   = {Adv. Comput. Math.},
 title     = {A survey of uncertainty principles and some signal processing applications},
 volume    = {40},
 pages     = {629-650},
 year      = {2014},
}

@PROCEEDINGS{siegman:ProcSPIE:1990,
   author = {A. E. Siegman},
    title = {New developments in laser resonators},
booktitle = {Optical Resonators},
     year = {1990},
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = {1224},
   editor = {E. Donkor and A. R. Pirich and H. E. Brandt},
    pages = {2-14},
publisher = {SPIE},
  address = {Bellingham, WA},
}

@article{belanger:OptLett:1991,
 author    = {P. A. Belanger},
 journal   = {Opt. Lett.},
 title     = {Beam propagation and the ABCD ray matrices},
 volume    = {16},
 pages     = {196-198},
 year      = {1991},
}

@article{martinezherrero:JOSAA:1991,
 author    = {J. Serna and R. Mart{\'\i}nez-Herrero and P. M. Mej{\'\i}as},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Parametric characterization of general partially coherent beams propagating through ABCD optical systems},
 volume    = {8},
 pages     = {1094-1098},
 year      = {1991},
}

@article{martinezherrero:OptLett:1993,
 author    = {R. Mart{\'\i}nez-Herrero and P. M. Mej{\'\i}as},
 journal   = {Opt. Lett},
 title     = {Second-order spatial characterization of hard-edge diffracted beams},
 volume    = {18},
 pages     = {1669-1671},
 year      = {1993},
}

@article{martinezherrero:OptLett:1995,
 author    = {R. Mart{\'\i}nez-Herrero and P. M. Mej{\'\i}as and M. Arias},
 journal   = {Opt. Lett.},
 title     = {Parametric characterization of coherent, lowest-order Gaussian beams propagating through hard-edged apertures},
 volume    = {20},
 pages     = {124-126},
 year      = {1995},
}

@article{martinezherrero:JOSAA:2003,
 author    = {R. Mart{\'\i}nez-Herrero and P. M. Mej{\'\i}as and S. Bosch and A. Carnicer},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Spatial width and power-content ratio of hard-edge diffracted beams},
 volume    = {20},
 pages     = {388-391},
 year      = {2003},
}

@article{lindfors:NatPhoton:2007,
 author    = {K. Lindfords and A. Priimagi and T. Set\"al\"a and A. Shevchenko and A. T. Friberg and M. Kaivola},
 journal   = {Nat. Photon.},
 title     = {Local polarization of tightly focused unpolarized light},
 volume    = {1},
 pages     = {228-231},
 year      = {2007},
}

@article{yzuel:OptLett:2007,
 author    = {J. Davis and C. Tuvey and O. L\'opez-Coronado and J. Campos and M. Yzuel and C. Iemmi},
 journal   = {Opt. Lett.},
 title     = {Tailoring the depth of focus for optical imaging systems using a Fourier transform approach},
 volume    = {32},
 pages     = {844-846},
 year      = {2007},
}

@article{zhan:AdvOptPhoton:2009,
 author    = {Q. Zhan},
 journal   = {Adv. Opt. Photon.},
 title     = {Cylindrical vector beams: from mathematical concepts to applications},
 volume    = {1},
 pages     = {1-57},
 year      = {2009},
}

@article{reid:NatPhoton:2008,
 author    = {K. A. Serrels and E. Ramsay and R. J. Warburton and D. T. Reid},
 journal   = {Nat. Photon.},
 title     = {Nanoscale optical microscopy in the vectorial focusing regime},
 volume    = {2},
 pages     = {311-314},
 year      = {2008},
}

@article{sheppard:NatPhoton:2008,
 author    = {H. Wang and L. Shi and B. Lukyanchuk and C. Sheppard and C. T. Chong},
 journal   = {Nat. Photon.},
 title     = {Creation of a needle of longitudinally polarized light in vacuum using binary optics},
 volume    = {2},
 pages     = {501-505},
 year      = {2008},
}

@article{dholakia:OptExp:2009,
 author    = {T. Cizmar and K. Dholakia},
 journal   = {Opt. Express},
 title     = {Tunable Bessel light modes: engineering the axial propagation},
 volume    = {17},
 pages     = {15558-15570},
 year      = {2009},
}

@article{martinezherrero:OptLett:2013,
 author    = {R. Mart{\'\i}nez-Herrero and I. Juvells and A. Carnicer},
 journal   = {Opt. Lett.},
 title     = {On the physical realizability of highly focused electromagnetic field distributions},
 volume    = {38},
 pages     = {2065-2067},
 year      = {2013},
 url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-38-12-2065},
 doi = {10.1364/OL.38.002065}
}

@article{martinezherrero:OptExp:2016,
 author    = {A. Carnicer and I. Juvells and B. Javidi and R. Mart{\'\i}nez-Herrero},
 journal   = {Opt. Express},
 title     = {Optical encryption in the longitudinal domain of focused fields},
 volume    = {24},
 pages     = {6793-6801},
 year      = {2016},
}

@article{martinezherrero:SciRep:2018,
 author    = {R. Mart{\'\i}nez-Herrero and D. Maluenda and I. Juvells and A. Carnicer},
 journal   = {Sci. Rep.},
 title     = {Synthesis of light needles with tunable length and nearly constant irradiance},
 volume    = {8},
 pages     = {2657},
 year      = {2018},
 doi       = {https://doi.org/10.1038/s41598-018-21007-7}
}

@article{martinezherrero:OSACont:2019,
 author    = {D. Maluenda and I. Juvells and R. Mart{\'\i}nez-Herrero and A. Carnicer},
 journal   = {OSA Continuum},
 title     = {Modeling axial irradiance distortion in holographic optical needles produced with high numerical aperture lenses},
 volume    = {2},
 pages     = {1539-1547},
 year      = {2019},
}

@article{sheppard:JOSAA:1988,
 author    = {C. Sheppard and Z. Hegedus},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Axial behavior of pupil-plane filters},
 volume    = {5},
 pages     = {643-647},
 year      = {1988},
}

@article{sheppard:JMO:1994,
 author    = {C. J. R. Sheppard and K. G. Larkin},
 journal   = {J. Mod. Opt.},
 title     = {Optimal concentration of electromagnetic radiation},
 volume    = {41},
 pages     = {1495-1505},
 year      = {1994},
}

@article{martinezcorral:OptLett:2001,
 author    = {M. Mart{\'\i}nez-Corral and L. Mu{\~n}oz-Escriv\'a and M. Kowalczyk and T. Cichocki},
 journal   = {Opt. Lett.},
 title     = {One-dimensional iterative algorithm for three-dimensional point-spread function engineering},
 volume    = {26},
 pages     = {1861-1863},
 year      = {2001},
}

@article{martinezcorral:OptExp:2002,
 author    = {M. Mart{\'\i}nez-Corral and M. Caballero and E. Stelzer and J. Swoger},
 journal   = {Opt. Express},
 title     = {Tailoring the axial shape of the point spread function using the Toraldo concept},
 volume    = {10},
 pages     = {98-103},
 year      = {2002},
}

@article{sheppard:OptLett:2007,
 author    = {C. Sheppard and S. Ledesma and J. Campos and J. Escalera},
 journal   = {Opt. Lett.},
 title     = {Improved expressions for performance parameters for complex filters},
 volume    = {32},
 pages     = {1713-1715},
 year      = {2007},
}

@article{sheppard:OptLett:2008-1,
 author    = {C. Sheppard},
 journal   = {Opt. Lett.},
 title     = {Filter performance parameters for high-aperture focusing},
 volume    = {32},
 pages     = {1653-1655},
 year      = {2008},
}

@article{sheppard:OptLett:2008-2,
 author    = {C. Sheppard and M. Mart{\'\i}nez-Corral},
 journal   = {Opt. Lett.},
 title     = {Filter performance parameters for vectorial high-aperture wave fields},
 volume    = {33},
 pages     = {476-478},
 year      = {2008},
}

@article{sheppard:OptLett:2011,
 author    = {C. Sheppard},
 journal   = {Opt. Lett.},
 title     = {Binary phase filters with a maximally-flat response},
 volume    = {36},
 pages     = {1386-1388},
 year      = {2011},
}

@article{sheppard:OptExp:2013,
 author    = {C. Sheppard},
 journal   = {Opt. Express},
 title     = {Pupil filters for generation of light sheets},
 volume    = {21},
 pages     = {6339-6345},
 year      = {2013},
}

@article{richards:PRSLAM:1959,
 author    = {B. Richards and E. Wolf},
 journal   = {Proc. Roy. Soc. Lond. A Math.},
 title     = {Electromagnetic diffraction in optical systems. II. structure of the image field in an aplanatic system},
 volume    = {253},
 pages     = {358-379},
 year      = {1959},
 doi = {10.1098/rspa.1959.0200},
 url = {https://doi.org/10.1098/rspa.1959.0200},
}

@article{martinezherrero:OptExp:2014,
 author    = {R. Mart{\'\i}nez-Herrero and D. Maluenda and I. Juvells and A. Carnicer},
 journal   = {Opt. Express},
 title     = {Experimental implementation  of  tightly  focused  beams  with  unpolarized  transversal  component  at any plane},
 volume    = {22},
 pages     = {32419-32428},
 year      = {2014},
}

@article{zhang:PRL:2019,
 author    = {H. Hu and Q. Gan and Q. Zhan},
 journal   = {Phys. Rev. Lett.},
 title     = {Generation of a nondiffracting superchiral optical needle for circular dichroism imaging of sparse subdiffraction objects},
 volume    = {122},
 pages     = {223901},
 year      = {2019},
}

@article{wang:OptCommun:2016,
 author    = {B. Yan and L. Yue and Z. Wang},
 journal   = {Opt. Commun.},
 title     = {Engineering near-field focusing of a microsphere lens with pupil masks},
 volume    = {370},
 pages     = {140-144},
 year      = {2016},
}

@article{bandres:JOSAA:2005,
 author    = {J. C. Guti\'errez-Vega and M. A. Bandres},
 journal   = {J. Opt. Soc. Am. A},
 title     = {Helmholtz-Gauss waves},
 volume    = {22},
 pages     = {289-298},
 year      = {2005},
}

@article{bandres:OptLett:2005,
 author    = {M. A. Bandres and J. C. Guti\'errez-Vega},
 journal   = {Opt. Lett.},
 title     = {Vector Helmholtz-Gauss and vector Laplace-Gauss beams},
 volume    = {30},
 pages     = {2155-2157},
 year      = {2005},
}

@article{bandres:OptExp:2006,
 author    = {R. I. Hern\'andez-Aranda and J. C. Guti\'errez-Vega and M. Guizar-Sicairos and M. A. Bandres},
 journal   = {Opt. Express},
 title     = {Propagation of generalized vector Helmholtz-Gauss beams through paraxial optical systems},
 volume    = {14},
 pages     = {8974-8988},
 year      = {2006},
}

@article{busch:PhysRep:2007,
 author    = {P. Busch and T. Heinonen and P. Lahti},
 journal   = {Phys. Rep.},
 title     = {Heisenberg's uncertainty principle},
 volume    = {452},
 pages     = {155-176},
 year      = {2007},
}

@article{maccone:PRL:2014,
 author    = {L. Maccone and A. K. Pati},
 journal   = {Phys. Rev. Lett.},
 title     = {Stronger uncertainty relations for all incompatible observables},
 volume    = {113},
 pages     = {260401(1-},
 year      = {2014},
}

@article{kempf:PRD:1995,
 author    = {A. Kempf and G. Mangano and R. B. Mann},
 journal   = {Phys. Rev. D},
 title     = {Hilbert space representation of the minimal length uncertainty principle},
 volume    = {52},
 pages     = {1108-1118},
 year      = {1995},
}

@article{scardigli:PhysLettB:1999,
 author    = {F. Scardigli},
 journal   = {Phys. Lett. B},
 title     = {Generalized uncertainty principle in quantum gravity from micro-black hole gedanken experiment},
 volume    = {452},
 pages     = {39-44},
 year      = {199},
}

@article{veneziano:EPL:1986,
 author    = {G. Veneziano},
 journal   = {Europhys. Lett.},
 title     = {A string nature needs just two constants},
 volume    = {2},
 pages     = {199-204},
 year      = {1986},
}

@article{buoninfante:EurPhysJC:2019,
 author    = {L. Buoninfante and G. G. Luciano and L. Petruzziello},
 journal   = {Eur. Phys. J. C},
 title     = {Generalized uncertainty principle and corpuscular gravity},
 volume    = {79},
 pages     = {663(1-8)},
 year      = {2019},
}

@article{steinberg:PRL:2012,
 author    = {L. A. Rozema and A. Darabi and D. H. Mahler and A. Hayat and Y. Soudagar and A. M. Steinberg},
 journal   = {Phys. Rev. Lett.},
 title     = {Violation of Heisenberg's measurement-disturbance relationship by weak measurements},
 volume    = {109},
 pages     = {100404(1-5)},
 year      = {2012},
}

@article{busch:PRL:2013,
 author    = {P. Busch and P. Lahti and R. F. Werner},
 journal   = {Phys. Rev. Lett.},
 title     = {Proof of Heisenberg's error-disturbance relation},
 volume    = {111},
 pages     = {160405(1-5)},
 year      = {2013},
}

@article{harris:JOSA:1969,
 author    = {F. S. Harris, Jr. and M. S. Tavenner and R. L. Mitchell},
 journal   = {J. Opt. Soc. Am.},
 title     = {Single-slit Fresnel diffraction patterns: comparison of experimental and theoretical results},
 volume    = {59},
 pages     = {293-296},
 year      = {1969},
}

@article{panuski:PhysTeacher:2016,
 author    = {Ch. L. Panuski and C. E. Mungan},
 journal   = {Phys. Teacher},
 title     = {Single-slit diffraction: transitioning from geometric optics to the Fraunhofer regime},
 volume    = {54},
 pages     = {356-359},
 year      = {2016},
}

@article{becs1,
  title = {Theory of Bose-Einstein condensation in trapped gases},
  author = {F. Dalfovo and S. Giorgini and L. P. Pitaevskii and S. Stringari},
  journal = {Rev. Mod. Phys.},
  volume = {71},
  issue = {3},
  pages = {463--512},
  numpages = {0},
  year = {1999},
}

@book{pitaevskii2016bose,
  title={Bose-Einstein condensation and superfluidity},
  author={L. P. Pitaevskii and S. Stringari},
  volume={164},
  year={2016},
  publisher={Oxford University Press},
}

@book{pethick2008bose,
  title={Bose--Einstein condensation in dilute gases},
  author={Ch. J. Pethick and H. Smith},
  year={2008},
  publisher={Cambridge university press},
}

@article{mewes,
  title = {Output Coupler for Bose-Einstein Condensed Atoms},
  author = {Mewes, M.-O. and Andrews, M. R. and Kurn, D. M. and Durfee, D. S. and Townsend, C. G. and Ketterle, W.},
  journal = {Phys. Rev. Lett.},
  volume = {78},
  issue = {4},
  pages = {582--585},
  numpages = {0},
  year = {1997},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.78.582},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.78.582}
}

@article {Andrews637,
    author = {Andrews, M. R. and Townsend, C. G. and Miesner, H.-J. and Durfee, D. S. and Kurn, D. M. and Ketterle, W.},
    title = {Observation of Interference Between Two Bose Condensates},
    volume = {275},
    number = {5300},
    pages = {637--641},
    year = {1997},
    journal = {Science},
    doi     = {https://doi.org/10.1126/science.275.5300.637}
}

@article{ketterle,
  title = {Nobel lecture: When atoms behave as waves: Bose-Einstein condensation and the atom laser},
  author = {Ketterle, Wolfgang},
  journal = {Rev. Mod. Phys.},
  volume = {74},
  issue = {4},
  pages = {1131--1151},
  numpages = {0},
  year = {2002},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.74.1131},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.74.1131}
}

@article{javanainen1997phase,
  title = {Phase and Phase Diffusion of a Split Bose-Einstein Condensate},
  author = {Javanainen, Juha and Wilkens, Martin},
  journal = {Phys. Rev. Lett.},
  volume = {78},
  issue = {25},
  pages = {4675--4678},
  numpages = {0},
  year = {1997},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.78.4675},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.78.4675}
}


@article{javanainen1996quantum,
  title = {Quantum Phase of a Bose-Einstein Condensate with an Arbitrary Number of Atoms},
  author = {Javanainen, Juha and Yoo, Sung Mi},
  journal = {Phys. Rev. Lett.},
  volume = {76},
  issue = {2},
  pages = {161--164},
  numpages = {0},
  year = {1996},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.76.161},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.76.161}
}

@article{ahufinger1,
  title = {Creation and mobility of discrete solitons in Bose-Einstein condensates},
  author = {Ahufinger, V. and Sanpera, A. and Pedri, P. and Santos, L. and Lewenstein, M.},
  journal = {Phys. Rev. A},
  volume = {69},
  issue = {5},
  pages = {053604},
  numpages = {7},
  year = {2004},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.69.053604},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.69.053604}
}

@article{ahufinger2,
  title = {Adiabatic splitting, transport, and self-trapping of a Bose-Einstein condensate in a double-well potential},
  author = {Ottaviani, C. and Ahufinger, V. and Corbal\'an, R. and Mompart, J.},
  journal = {Phys. Rev. A},
  volume = {81},
  issue = {4},
  pages = {043621},
  numpages = {8},
  year = {2010},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.81.043621},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.81.043621}
}

@article{polo2013soliton,
  title = {Soliton-based matter-wave interferometer},
  author = {Polo, J. and Ahufinger, V.},
  journal = {Phys. Rev. A},
  volume = {88},
  issue = {5},
  pages = {053628},
  numpages = {8},
  year = {2013},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.88.053628},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.88.053628}
}

@article{Ji_2016,
	author = {Shen-Tong Ji and Yuan-Sheng Wang and Yue-E Luo and Xue-Shen Liu},
	title = {Generating periodic interference in Bose-Einstein condensates},
    journal = {Chin. Phys. B},
	doi = {10.1088/1674-1056/25/9/090303},
	url = {https://doi.org/10.1088/1674-1056/25/9/090303},
	year = {2016},
	month = {aug},
	publisher = {{IOP} Publishing},
	volume = {25},
	number = {9},
	pages = {090303}
}


@article{bao2003numerical,
author = {Weizhu Bao and Dieter Jaksch and Peter A. Markowich},
title = {Numerical solution of the Gross-Pitaevskii equation for Bose-Einstein condensation},
journal = {J. Comput. Phys.},
volume = {187},
number = {1},
pages = {318-342},
year = {2003},
issn = {0021-9991},
doi = {https://doi.org/10.1016/S0021-9991(03)00102-5},
url = {https://www.sciencedirect.com/science/article/pii/S0021999103001025}
}

@article{ANTOINE20132621,
author = {Xavier Antoine and Weizhu Bao and Christophe Besse},
title = {Computational methods for the dynamics of the nonlinear Schr\"odinger/Gross-Pitaevskii equations},
journal = {Comp. Phys. Comm.},
volume = {184},
number = {12},
pages = {2621-2633},
year = {2013},
issn = {0010-4655},
doi = {https://doi.org/10.1016/j.cpc.2013.07.012},
url = {https://www.sciencedirect.com/science/article/pii/S0010465513002403}
}

@article{huang2006creation,
  title = {Creation, detection, and decoherence of macroscopic quantum superposition states in double-well Bose-Einstein condensates},
  author = {Y. P. Huang and M. G. Moore},
  journal = {Phys. Rev. A},
  volume = {73},
  issue = {2},
  pages = {023606},
  numpages = {20},
  year = {2006},
}

@article{wang2007effect,
  title = {Effect of decoherence on the dynamics of Bose-Einstein condensates in a double-well potential},
  author = {Wang, W. and Fu, L. B. and Yi, X. X.},
  journal = {Phys. Rev. A},
  volume = {75},
  issue = {4},
  pages = {045601},
  numpages = {4},
  year = {2007},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.75.045601},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.75.045601}
}

@article{ai2004influence,
  title={Influence of Decoherence on Interference Between Two Bose-Einstein Condensates},
  author={Ai-Hua, Zeng and Le-Man, Kuang},
  journal={Commun. Theor. Phys},
  volume={41},
  number={1},
  pages={41},
  year={2004},
}

@article{Lee2012,
author= {Lee, Chaohong and Huang, Jiahao and Deng, Haiming and Dai, Hui and Xu, Jun},
title={Nonlinear quantum interferometry with Bose condensed atoms},
journal={Front. Phys.},
year={2012},
volume={7},
pages={109--130},
doi={https://doi.org/10.1007/s11467-011-0228-6},
url={https://link.springer.com/article/10.1007/s11467-011-0228-6}
}

@article{PhysRevLett.100.080405,
  title = {Atom Interferometry with a Weakly Interacting Bose-Einstein Condensate},
  author = {Fattori, M. and D'Errico, C. and Roati, G. and Zaccanti, M. and Jona-Lasinio, M. and Modugno, M. and Inguscio, M. and Modugno, G.},
  journal = {Phys. Rev. Lett.},
  volume = {100},
  issue = {8},
  pages = {080405},
  numpages = {4},
  year = {2008},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.100.080405},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.100.080405}
}

@article{PhysRevLett.95.070401,
  title = {Bose-Einstein Condensate in a Random Potential},
  author = {Lye, J. E. and Fallani, L. and Modugno, M. and Wiersma, D. S. and Fort, C. and Inguscio, M.},
  journal = {Phys. Rev. Lett.},
  volume = {95},
  issue = {7},
  pages = {070401},
  numpages = {4},
  year = {2005},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.95.070401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.95.070401}
}

@article{PhysRevA.66.021601,
  title = {Free expansion of a Bose-Einstein condensate in a one-dimensional optical lattice},
  author = {Morsch, O. and Cristiani, M. and M\"uller, J. H. and Ciampini, D. and Arimondo, E.},
  journal = {Phys. Rev. A},
  volume = {66},
  issue = {2},
  pages = {021601(R)},
  numpages = {4},
  year = {2002},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.66.021601},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.66.021601}
}

@Inbook{Morsch2002,
author="Morsch, Oliver and Arimondo, Ennio",
editor="Dauxois, Thierry and Ruffo, Stefano and Arimondo, Ennio and Wilkens, Martin",
title="Ultracold Atoms and Bose-Einstein Condensates in Optical Lattices",
bookTitle="Dynamics and Thermodynamics of Systems with Long-Range Interactions",
year="2002",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="312--331",
}

@article{PhysRevE.92.013201,
  title = {Stationary solutions for the nonlinear Schr\"odinger equation modeling three-dimensional spherical Bose-Einstein condensates in general potentials},
  author = {Mallory, Kristina and Van Gorder, Robert A.},
  journal = {Phys. Rev. E},
  volume = {92},
  issue = {1},
  pages = {013201},
  numpages = {21},
  year = {2015},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.92.013201},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.92.013201}
}

@article{PhysRevE.85.056608,
  title = {Matter-wave solutions in Bose-Einstein condensates with harmonic and Gaussian potentials},
  author = {Yan, Zhenya and Jiang, Dongmei},
  journal = {Phys. Rev. E},
  volume = {85},
  issue = {5},
  pages = {056608},
  numpages = {11},
  year = {2012},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.85.056608},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.85.056608}
}

@article{PhysRevE.75.036214,
  title = {Dynamics of Bose-Einstein condensates under the influence of periodic and harmonic potentials},
  author = {Berry, N. Hawk and Kutz, J. Nathan},
  journal = {Phys. Rev. E},
  volume = {75},
  issue = {3},
  pages = {036214},
  numpages = {9},
  year = {2007},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.75.036214},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.75.036214}
}

@article{PhysRevE.89.013204,
  title = {Stationary solutions for the 1$+$1 nonlinear Schr\"odinger equation modeling attractive Bose-Einstein condensates in small potentials},
  author = {Mallory, Kristina and Van Gorder, Robert A.},
  journal = {Phys. Rev. E},
  volume = {89},
  issue = {1},
  pages = {013204},
  numpages = {11},
  year = {2014},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.89.013204},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.89.013204}
}

@article{PhysRevE.62.1382,
  title = {Numerical solution of the Gross-Pitaevskii equation using an explicit finite-difference scheme: An application to trapped Bose-Einstein condensates},
  author = {Cerimele, M. M. and Chiofalo, M. L. and Pistella, F. and Succi, S. and Tosi, M. P.},
  journal = {Phys. Rev. E},
  volume = {62},
  issue = {1},
  pages = {1382--1389},
  numpages = {0},
  year = {2000},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.62.1382},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.62.1382}
}

@article{dalfovo1999theory,
  title = {Theory of Bose-Einstein condensation in trapped gases},
  author = {Dalfovo, Franco and Giorgini, Stefano and Pitaevskii, Lev P. and Stringari, Sandro},
  journal = {Rev. Mod. Phys.},
  volume = {71},
  issue = {3},
  pages = {463--512},
  numpages = {0},
  year = {1999},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.71.463},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.71.463}
}

@article{parker2003soliton,
  title = {Soliton-Sound Interactions in Quasi-One-Dimensional Bose-Einstein Condensates},
  author = {Parker, N. G. and Proukakis, N. P. and Leadbeater, M. and Adams, C. S.},
  journal = {Phys. Rev. Lett.},
  volume = {90},
  issue = {22},
  pages = {220401},
  numpages = {4},
  year = {2003},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.90.220401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.90.220401}
}

@article{parker2010dark,
  title = {Dark soliton decay due to trap anharmonicity in atomic Bose-Einstein condensates},
  author = {Parker, N. G. and Proukakis, N. P. and Adams, C. S.},
  journal = {Phys. Rev. A},
  volume = {81},
  issue = {3},
  pages = {033606},
  numpages = {10},
  year = {2010},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.81.033606},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.81.033606}
}

@article {Anderson198,
author = {M. H. Anderson  and J. R. Ensher  and M. R. Matthews  and C. E. Wieman  and E. A. Cornell },
title = {Observation of Bose-Einstein Condensation in a Dilute Atomic Vapor},
journal = {Science},
volume = {269},
number = {5221},
pages = {198-201},
year = {1995},
doi = {10.1126/science.269.5221.198},
URL = {https://www.science.org/doi/abs/10.1126/science.269.5221.198}
}

@article{PhysRevLett.75.1687,
  title = {Evidence of Bose-Einstein Condensation in an Atomic Gas with Attractive Interactions},
  author = {Bradley, C. C. and Sackett, C. A. and Tollett, J. J. and Hulet, R. G.},
  journal = {Phys. Rev. Lett.},
  volume = {75},
  issue = {9},
  pages = {1687--1690},
  numpages = {0},
  year = {1995},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.75.1687},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.75.1687}
}

@article{PhysRevLett.75.3969,
  title = {Bose-Einstein Condensation in a Gas of Sodium Atoms},
  author = {Davis, K. B. and Mewes, M. -O. and Andrews, M. R. and van Druten, N. J. and Durfee, D. S. and Kurn, D. M. and Ketterle, W.},
  journal = {Phys. Rev. Lett.},
  volume = {75},
  issue = {22},
  pages = {3969--3973},
  numpages = {0},
  year = {1995},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.75.3969},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.75.3969}
}

@article{PhysRevLett.85.1795,
  title = {Stable ${}^{85}\mathrm{Rb}$ Bose-Einstein Condensates with Widely Tunable Interactions},
  author = {Cornish, S. L. and Claussen, N. R. and Roberts, J. L. and Cornell, E. A. and Wieman, C. E.},
  journal = {Phys. Rev. Lett.},
  volume = {85},
  issue = {9},
  pages = {1795--1798},
  numpages = {0},
  year = {2000},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.85.1795},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.85.1795}
}

@incollection{sanz2019bohmian,
  author={A.S. Sanz},
  title={Bohmian pathways into chemistry: A brief overview},
  booktitle={Applied Bohmian mechanics: From nanoscale systems to cosmology},
  editor={Oriols, Xavier and Mompart, Jordi},
  year={2019},
  publisher={Panstanford Pub},
  pages={257-330},
  year={2019},
}

@article{landau:PhysRev:1941,
  title = {Theory of the Superfluidity of Helium II},
  author = {Landau, L.},
  journal = {Phys. Rev.},
  volume = {60},
  issue = {4},
  pages = {356--358},
  numpages = {0},
  year = {1941},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.60.356},
  url = {https://link.aps.org/doi/10.1103/PhysRev.60.356}
}


@phdthesis{Weller2009DynamicsAI,
  title={Dynamics and interaction of dark solitons in Bose-Einstein condensates},
  author={Andreas Weller},
  year={2009},
}

@PHDTHESIS{ronzheimer:PhDThesis:2008,
  AUTHOR =       {J. Ph. Ronzheimer},
  TITLE =        {Interactions of Dark Solitons in Cigar Shaped Bose-Einstein Condensates},
  SCHOOL =       {Kirchhoff-Institut f\"ur Physik, University of Heidelberg},
  YEAR =         {2008},
  address =      {Germany},
}

@PHDTHESIS{weller:PhDThesis:2009,
  AUTHOR =       {A. Weller},
  TITLE =        {Dynamics and Interaction of Dark Solitons in Bose-Einstein Condensates},
  SCHOOL =       {University of Heidelberg},
  YEAR =         {2009},
  address =      {Germany},
}

@article{sanz:PRA:2005,
  title = {Loss of coherence in double-slit diffraction experiments},
  author = {Sanz, A. S. and Borondo, F. and Bastiaans, M. J.},
  journal = {Phys. Rev. A},
  volume = {71},
  issue = {4},
  pages = {042103},
  numpages = {7},
  year = {2005},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.71.042103},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.71.042103}
}


@article{tounli:arxiv:2019-2,
 author    = {J. Tounli and A. S. Sanz},
 journal   = {arXiv:},
 title     = {BEC with quantum state diffusion},
 volume    = {},
 pages     = {},
 year      = {submitted, 2019},
}

@BOOK{benseny:PanStanford:2012,
  AUTHOR     = {A. Benseny and J. Bagud\`a and X. Oriols and G. Birkl and J. Mompart},
  editor     = {X. Oriols and J. Mompart},
  title      = {Applied Bohmian Mechanics: From Nanoscale Systems to Cosmology},
  CHAPTER    = {Atomtronics: Coherent control of atomic flow via adiabatic passage},
  pages      = {189-233},
  publisher  = {Pan Standford Publishing},
  year       = {2012},
  address    = {Singapore},
}

@BOOK{bricmont-bk,
  AUTHOR     = {J. Bricmont},
  TITLE      = {Making Sense of Quantum Mechanics},
  PUBLISHER  = {Springer},
  YEAR       = {2016},
  address    = {Berlin},
}

@article{steinberg:SciAdv:2016,
 author    = {D. H. Mahler and L. Rozema and K. Fisher and L. Vermeyden and K. J. Resch and H. M. Wiseman and A. Steinberg},
 journal   = {Sci. Adv.},
 title     = {Experimental nonlocal and surreal Bohmian trajectories},
 volume    = {2},
 pages     = {e1501466},
 year      = {2016},
 doi       = {10.1126/sciadv.150146},
}

@article{DeRaedt:PhysicaE:2010,
 author    = {H. De Raedt and S. Zhao and S. Yuan and F. Jin and K. Michielsen and S. Miyashita},
 journal   = {Physica E},
 title     = {Event-by-event simulation of quantum phenomena},
 volume    = {42},
 pages     = {298-302},
 year      = {2010},
}

@article{DeRaedt:JPSJ:2010,
 author    = {F. Jin and S. Yuan and H. De Raedt and K. Michielsen and S. Miyashita},
 journal   = {J. Phys. Soc. Jpn.},
 title     = {Corpuscular model of two-beam interference and double-slit experiments with single photons},
 volume    = {79},
 pages     = {074401(1-14)},
 year      = {2010},
}

@article{webb:IJTP:2011,
 author    = {G. F. Webb},
 journal   = {Int. J. Theor. Phys.},
 title     = {Event based interpretation of Schr\"odinger's equation for the two-slit experiment},
 volume    = {50},
 pages     = {3571-3601},
 year      = {2011},
}

@article{muser-hiley:SciAm:2013,
   author =       {G. Muser},
   title =        {The wholeness of quantum reality: An interview with physicist Basil Hiley},
   journal =      {Sci. Am.},
   volume =       {November 4},
   year =         {2013},
   url = {https://blogs.scientificamerican.com/critical-opalescence/the-wholeness-of-quantum-reality-an-interview-with-physicist-basil-hiley/},
   note =         {Online: https://blogs.scientificamerican.com/critical-opalescence/the-wholeness-of-quantum-reality-an-interview-with-physicist-basil-hiley/},
 }

@article{dirac:PRSLA:1931,
 author    = {P. A. M. Dirac},
 journal   = {Proc. R. Soc. Lond. A},
 title     = {Quantised singularities in the electromagnetic field},
 volume    = {133},
 pages     = {60-72},
 year      = {1931},
}

@article{pennings:JLightTech:1995,
 author    = {L. B. Soldano and E. C. M. Pennings},
 journal   = {J. Light. Tech.},
 title     = {Optical multi-model interference devices based on self-imaging: Principles and applications},
 volume    = {13},
 pages     = {615-627},
 year      = {1995},
}

@article{pusey:NaturePhys:2012,
 author    = {M. F. Pusey and J. Barrett and T. Rudolph},
 journal   = {Nature Phys.},
 title     = {On the reality of the quantum state},
 volume    = {8},
 pages     = {475-478},
 year      = {2012},
}

@article{sudarshan:PRD:1989,
 author    = {I. M. Duck and P. M. Stevenson and E. C. G. Sudarshan},
 journal   = {Phys. Rev. D},
 title     = {The sense in which a ``weak measurement'' of a spin-1/2 particle's spin component yields a value 100},
 volume    = {40},
 pages     = {2112-2117},
 year      = {1989},
}

@article{sanz:FrontPhys:submit21,
 author    = {A. S. Sanz},
 journal   = {Front. Phys.},
 title     = {Unveiling the hidden symmetries behind entangled bipartite continuous-variable systems by means of Bohmian mechanics},
 volume    = {},
 pages     = {},
 year      = {submitted, 2021},
}

@article{umul:Optik:2020,
 author    = {Y. Z. Umul},
 journal   = {Optik},
 title     = {On the reality of the Bohmian potential},
 volume    = {224},
 pages     = {165729(1-5)},
 year      = {2020},
}

@article{hojman:arxiv:2021,
 author    = {S. A. Hojman and F. A. Asenjo and H. M. Moya-Cessa and F. Soto-Eguibar},
 journal   = {Preprint},
 title     = {Bohm potential is real and its effects are measurable},
 volume    = {},
 pages     = {1-4},
 year      = {2021},
 archivePrefix = {arXiv},
 eprint        = {2101.06738},
}

@article{tounli:arxiv:2021,
 author    = {J. Tounli and A. S. Sanz},
 journal   = {},
 title     = {},
 volume    = {},
 pages     = {},
 year      = {in preparation},
}

@BOOK{eberly-bk,
  AUTHOR     = {L. Allen and J. H. Eberly},
  TITLE      = {Optical Resonance and Two-Level Atoms},
  PUBLISHER  = {Dover},
  YEAR       = {1975},
  address    = {New York},
}

@article{zurek:PhysToday:1991,
 author    = {W. H. Zurek},
 journal   = {Phys. Today},
 title     = {Decoherence and the transition from quantum to classical},
 volume    = {44(10)},
 pages     = {36-44},
 year      = {1991},
 doi       = {10.1063/1.881293},
 url       = {https://doi.org/10.1063/1.881293},
}

@article{zurek:PhysToday-rev:2003,
 author    = {W. H. Zurek},
 journal   = {Los Alamos Science},
 title     = {Decoherence and the transition from quantum to classical -- Revisited},
 volume    = {27},
 pages     = {2-25},
 year      = {2002},
}

@article{mathew:MPLB:2013,
 author    = {A. Mathew and M. K. Nandy},
 journal   = {Mod. Phys. Lett. B},
 title     = {Decoherence study of electron spin states in quantum dots using a simplistic model},
 volume    = {27},
 pages     = {1350119(1-9)},
 year      = {2013},
}

@article{khaetskii:PRL:2002,
 author    = {A. V. Khaetskii and D. Loss and L. Glazman},
 journal   = {Phys. Rev. Lett.},
 title     = {Electron spin decoherence in quantum dots due to interaction with nuclei},
 volume    = {88},
 pages     = {186802(1-4)},
 year      = {2002},
}

@article{altaisky:EPJWebConf:2016,
 author = {M. V. Altaisky and N. N. Zolnikova and N. E. Kaputkina and V. A. Krylov and Yu. E. Lozovik and N. S. Dattani},
 title  = {Decoherence and entanglement simulation in a model of quantum neural wetwork based on quantum dots},
 journal = {EPJ Web of Conferences},
 year = {2016},
 volume = {108},
 pages = {02006(1-6)},
}

@article{kendon:PRA:2003,
 author    = {V. Kendon and B. Tregenna},
 journal   = {Phys. Rev. A},
 title     = {Decoherence can be useful in quantum walks},
 volume    = {67},
 pages     = {042315(1-6)},
 year      = {2003},
}

@article{yin:PRA:2008,
 author    = {Y. Yin and D. E. Katsanos and S. N. Evangelou},
 journal   = {Phys. Rev. A},
 title     = {Quantum walks on a random environment},
 volume    = {77},
 pages     = {022302(1-7)},
 year      = {2008},
}

@article{kimm:PRA:2002,
 author    = {K. Kimm and H. H. Kwon},
 journal   = {Phys. Rev. A},
 title     = {Decoherence of the quantum gate in Milburn's model of decoherence},
 volume    = {65},
 pages     = {022311(1-5)},
 year      = {2002},
}

@article{leman:CTP:1998,
 author    = {K. Leman},
 journal   = {Commun. Theor. Phys.},
 title     = {Decoherence induced by discontinuous and stochastic unitary evolution of qubits in quantum computers},
 volume    = {29},
 pages     = {169-172},
 year      = {1998},
}

@article{ziman:PRA:2005,
 author    = {M. Ziman and V. Bu\v{z}ek},
 journal   = {Phys. Rev. A},
 title     = {All (qubit) decoherences: Complete characterization and physical implementation},
 volume    = {72},
 pages     = {022110(1-9)},
 year      = {2005},
}

@article{czerwinski:IJTP:2016,
 author    = {A. Czerwinski},
 journal   = {Int. J. Theor. Phys.},
 title     = {Applications of the stroboscopic tomography to selected 2-level decoherence models},
 volume    = {55},
 pages     = {658-668},
 year      = {2016},
}

@article{floss:PRB:2019,
 author    = {I. Floss and C. Lemell and K. Yabana and J. Burgd\"orfer},
 journal   = {Phys. Rev. B},
 title     = {Incorporating decoherence into solid-state time-dependent density functional theory},
 volume    = {99},
 pages     = {224301(1-14)},
 year      = {2019},
}

@article{petruccione:PRAppl:2018,
 author    = {S. G. Dlamini and J. T. Francis and X. Zhang and \c{S}. K. \"Ozdemir and S. Nic Chormaic and F. Petruccione and M. S. Tame},
 journal   = {Phys. Rev. Appl.},
 title     = {Probing decoherence in plasmonic waveguides in the quantum regime},
 volume    = {9},
 pages     = {024003(1-10)},
 year      = {2018},
}

@article{chen:CTP:2013,
 author    = {C. Chen and Y. B. Gao},
 journal   = {Commun. Theor. Phys.},
 title     = {Quantum decoherence of charge qubit coupled to nonlinear nanomechanical resonator},
 volume    = {60},
 pages     = {531-534},
 year      = {2013},
}

@article{schroll:PRA:2003,
 author    = {C. Schroll and W. Belzig and C. Bruder},
 journal   = {Phys. Rev. A},
 title     = {Decoherence of cold atomic gases in magnetic microtraps},
 volume    = {68},
 pages     = {043618(1-14)},
 year      = {2003},
}

@article{duan:ChinPhysLett:1997,
 author    = {L.-M. Duan and G.-C. Guo},
 journal   = {Chinese Phys. Lett.},
 title     = {Scheme for reducing decoherence in quantum computer memory by transformation to the coherence-preserving states},
 volume    = {14},
 pages     = {488-491},
 year      = {1997},
}

@article{novais:PRL2006,
 author    = {E. Novais and H. U. Baranger},
 journal   = {Phys. Rev. Lett.},
 title     = {Decoherence by correlated noise and quantum error correction},
 volume    = {97},
 pages     = {040501(1-4)},
 year      = {2006},
}

@article{lei:PRA:2011,
 author    = {Ch. U. Lei and W.-M. Zhang},
 journal   = {Phys. Rev. A},
 title     = {Decoherence suppression of open quantums systems through a strong coupling to non-Markovian reservoirs},
 volume    = {84},
 pages     = {052116(1-5)},
 year      = {2011},
}

@article{ahsan:QIC:2018,
 author    = {M. Ahsan and S. A. Z. Naqvi},
 journal   = {Quantum Inf. Comput.},
 title     = {Performance of topological quantum error correction in the presence of correlated noise},
 volume    = {18},
 pages     = {743-778},
 year      = {2018},
}

@article{batelaan:NJP:2018,
 author    = {P. J. Beierle and L. Zhang and H. Batelaan},
 journal   = {New J. Phys.},
 title     = {Experimental test of decoherence theory using electron matter waves},
 volume    = {20},
 pages     = {113030(1-12)},
 year      = {2018},
}

@article{zeilinger:NJP:2018,
 author    = {S. K. Joshi and J. Pienaar and T. C. Ralph and L. Cacciapuoti and W. McCutcheon and J. Rarity and D. Giggenbach and J. G. Lim and V. Makarov and I. Fuentes and Th. Scheidl and E. Beckert and M. Bourennane and D. E. Bruschi and A. Cabello and J. Capmany and A. Carrasco-Casado and E. Diamanti and M. Du\v{s}ek and D. Elser and A. Gulinatti and R. H. Hadfield and Th. Jennewein and R. Kaltenbaek and M. A. Krainak and H. K. Lo and C. Marquardt and G. Milburn and M. Peev and A. Poppe and V. Pruneri and R. Renner and C. Salomon and J. Skaar and N. Solomos and M. Stip\v{c}evic and J. P. Torres and M. Toyoshima and P. Villoresi and I. Walrnsley and G. Weihs and H. Weinfurter and A. Zeilinger and M. Zukowski and R. Ursin},
 journal   = {New J. Phys.},
 title     = {Space QUEST mission proposal: Experimentally testing decoherence due to gravity},
 volume    = {20},
 pages     = {063016(1-21)},
 year      = {2018},
}

@article{schleich:NJP:2013,
	doi = {10.1088/1367-2630/15/1/013052},
	url = {https://dx.doi.org/10.1088/1367-2630/15/1/013052},
	year = {2013},
	month = {jan},
	publisher = {IOP Publishing},
	volume = {15},
	number = {1},
	pages = {013052},
	author = {P Kazemi and S Chaturvedi and I Marzoli and R F O'Connell and W P Schleich},
	title = {Quantum carpets: a tool to observe decoherence},
	journal = {New J. Phys.},
}

@article{taylor:PCPS:1909,
 author    = {G. I. Taylor},
 journal   = {Proc. Cambridge Phil. Soc.},
 title     = {Interference fringes with feeble light},
 volume    = {15},
 pages     = {114-115},
 year      = {1909},
}

@article{dempster:PhysRev:1927,
 author    = {A. J. Dempster and H. F. Batho},
 journal   = {Phys. Rev.},
 title     = {Light quanta and interference},
 volume    = {30},
 pages     = {644-648},
 year      = {1927},
}

@article{davis:IEEEJQuantumElectron:1979,
 author    = {C. C. Davis},
 journal   = {IEEE J. Quantum Electron.},
 title     = {Single-photon optical heterodyning},
 volume    = {QE--15},
 pages     = {26-29},
 year      = {1979},
}

@article{aspect:EPL:1986,
 author    = {P. Grangier and G. Roger and A. Aspect},
 journal   = {Europhys. Lett.},
 title     = {Experimental evidence for a photon anticorrelation effect on a beam splitter: A new light on single-photon interferences},
 volume    = {1},
 pages     = {173-179},
 year      = {1986},
}

@article{kimura:OptCommun:1989,
 author    = {T. Okoshi and A. Hirose and K. Kimura},
 journal   = {Opt. Commun.},
 title     = {A simple experiment elucidating the duality of light as wave and photon},
 volume    = {72},
 pages     = {7-12},
 year      = {1989},
}

@article{rose:AdvBiolMedPhys:1957,
 author    = {A. Rose},
 journal   = {Adv. Biol. Med. Phys.},
 title     = {Quantum effects in human vision},
 volume    = {5},
 pages     = {211-242},
 year      = {1957},
}

@article{drezet:AnnFondLdBroglie:2021,
 author    = {A. Drezet and B. Stock},
 journal   = {Ann. Fond. Louis de Broglie},
 title     = {A causal and continous interpretation of the quantum theory: About an original manuscript by David Bohm sent to Louis de Broglie in 1951},
 volume    = {},
 pages     = {1-27},
 year      = {2001},
 preprint  = {arXiv:2103.0057},
}

@BOOK{elmore-heald-bk:1969,
  AUTHOR     = {W. C. Elmore and M. A. Heald},
  TITLE      = {Physics of Waves},
  PUBLISHER  = {McGraw-Hill},
  YEAR       = {1969},
  address    = {New York},
}

@article{davidovic:PhysTeacher:2019,
 author    = {M. D. Davidovi\'c and M. Bo\v{z}i\'c},
 journal   = {Phys. Teacher},
 title     = {Geometrical, Fresnel, and Fraunhofer regimes of single-slit diffraction},
 volume    = {57},
 pages     = {176-178},
 year      = {2019},
}

@article{shirali:MathMag:2011,
 author    = {Sh. A. Shirali},
 journal   = {Math. Mag.},
 title     = {The Bhaskara-Aryabhata approximation to the sine function},
 volume    = {84},
 pages     = {98-107},
 year      = {2011},
 doi       = {10.4169/math.mag.84.2.98},
}

@article{honrubia:PRA:2021,
 author    = {E. Honrubia and A. S. Sanz},
 journal   = {Phys. Rev. A},
 title     = {Decoherence in quantum cavities: Environmental erasure of carpet-type structures},
 volume    = {103},
 pages     = {062210},
 year      = {2021},
 doi       = {10.1103/PhysRevA.103.062210},
}

@BOOK{mandelbrot-bk:1977,
  AUTHOR     = {B. B. Mandelbrot},
  TITLE      = {Fractals. Form, Chance, and Dimension},
  PUBLISHER  = {W. H. Freeman and Co.},
  YEAR       = {1977},
  address    = {New York},
}

@BOOK{mandelbrot-bk:1983,
  AUTHOR     = {B. B. Mandelbrot},
  TITLE      = {The Fractal Geometry of Nature},
  PUBLISHER  = {W. H. Freeman and Co.},
  YEAR       = {1983},
  address    = {New York},
}

@article{hall:JPA:2004,
 author    = {M. J. W. Hall},
 journal   = {J. Phys. A: Math. Gen.},
 title     = {Incompleteness of trajectory-based interpretations of quantum mechanics},
 volume    = {37},
 pages     = {9549-9556},
 year      = {2004},
 doi       = {10.1088/0305-4470/37/40/015},
}

@BOOK{bouwmeester-bk:2000,
	editor     = {D. Bouwmeester and A. Ekert and A. Zeilinger},
	TITLE      = {The Physics of Quantum Information},
	PUBLISHER  = {Springer},
	YEAR       = {2000},
	address    = {Berlin},
}

@article{furuya:PRL:1998,
	title = {Quantum Dynamical Manifestation of Chaotic Behavior in the Process of Entanglement},
	author = {Furuya, K. and Nemes, M. C. and Pellegrino, G. Q.},
	journal = {Phys. Rev. Lett.},
	volume = {80},
	issue = {25},
	pages = {5524--5527},
	numpages = {0},
	year = {1998},
	month = {Jun},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.80.5524},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.80.5524}
}

@article{furuya:PRA:2005,
	title = {Semiclassical limit of the entanglement in closed pure systems},
	author = {Angelo, Renato M. and Furuya, K.},
	journal = {Phys. Rev. A},
	volume = {71},
	issue = {4},
	pages = {042321},
	numpages = {7},
	year = {2005},
	month = {Apr},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.71.042321},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.71.042321}
}

@article{sarkar:PRE:1999,
	title = {Signatures of chaos in the entanglement of two coupled quantum kicked tops},
	author = {Miller, Paul A. and Sarkar, Sarben},
	journal = {Phys. Rev. E},
	volume = {60},
	issue = {2},
	pages = {1542--1550},
	numpages = {0},
	year = {1999},
	month = {Aug},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevE.60.1542},
	url = {https://link.aps.org/doi/10.1103/PhysRevE.60.1542}
}

@article{ghose:PRA:2004,
	title = {Entanglement dynamics in chaotic systems},
	author = {Ghose, Shohini and Sanders, Barry C.},
	journal = {Phys. Rev. A},
	volume = {70},
	issue = {6},
	pages = {062315},
	numpages = {5},
	year = {2004},
	month = {Dec},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.70.062315},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.70.062315}
}

@article{zurek:PhysicaD:1995,
	title = {Quantum chaos: a decoherent definition},
	journal = {Physica D: Nonlinear Phenomena},
	volume = {83},
	number = {1},
	pages = {300-308},
	year = {1995},
	note = {Quantum Complexity in Mesoscopic Systems},
	issn = {0167-2789},
	doi = {https://doi.org/10.1016/0167-2789(94)00271-Q},
	url = {https://www.sciencedirect.com/science/article/pii/016727899400271Q},
	author = {Wojciech Hubert Zurek and Juan Pablo Paz},
	abstract = {We show that the rate of increase of Von Neumann entropy computed from the reduced density matrix of an open quantum system is an excellent indicator of the dynamical behavior of its classical Hamiltonian counterpart. In decohering quantum analogs of systems which exhibit classical Hamiltonian chaos entropy production rate quickly tends to a constant which is given by the sum of the positive Lyapunov exponents, and falls off only as the system approaches equilibrium. By contrast, integrable systems tend to have an entropy production rate which decreases as t−1 well before equilibrium is attained. Thus, behavior of quantum systems in contact with the environment can be used as a test to determine the nature of their Hamiltonian evolution.}
}

@article{brumer-hamilton:PRA:1982,
	title = {Relaxation rates for two-dimensional deterministic mappings},
	author = {Hamilton, Ian and Brumer, Paul},
	journal = {Phys. Rev. A},
	volume = {25},
	issue = {6},
	pages = {3457--3459},
	numpages = {0},
	year = {1982},
	month = {Jun},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.25.3457},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.25.3457}
}

@article{brumer-hamilton:JCP:1983,
	author = {Hamilton,Ian  and Brumer,Paul },
	title = {Intramolecular relaxation in N=2 Hamiltonian systems: The role of the K entropy},
	journal = {J. Chem. Phys.},
	volume = {78},
	number = {5},
	pages = {2682-2690},
	year = {1983},
	doi = {10.1063/1.445027},
    URL = {https://doi.org/10.1063/1.445027},
}

@article{brumer-christoffel:PRA:1986,
	title = {Quantum and classical dynamics in the stadium billiard},
	author = {Christoffel, Kurt M. and Brumer, Paul},
	journal = {Phys. Rev. A},
	volume = {33},
	issue = {2},
	pages = {1309--1321},
	numpages = {0},
	year = {1986},
	month = {Feb},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.33.1309},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.33.1309}
}

@article{brumer-pattnayak:PRL:1996,
	title = {Exponential Divergence and Long Time Relaxation in Chaotic Quantum Dynamics},
	author = {Pattanayak, Arjendu K. and Brumer, Paul},
	journal = {Phys. Rev. Lett.},
	volume = {77},
	issue = {1},
	pages = {59--62},
	numpages = {0},
	year = {1996},
	month = {Jul},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.77.59},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.77.59}
}

@article{brumer-pattnayak:PRL:1997,
	title = {Exponentially Rapid Decoherence of Quantum Chaotic Systems},
	author = {Pattanayak, Arjendu K. and Brumer, Paul},
	journal = {Phys. Rev. Lett.},
	volume = {79},
	issue = {21},
	pages = {4131--4134},
	numpages = {0},
	year = {1997},
	month = {Nov},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.79.4131},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.79.4131}
}

@article{brumer-pattnayak:PRE:1997,
	title = {Chaos and Lyapunov exponents in classical and quantal distribution dynamics},
	author = {Pattanayak, Arjendu K. and Brumer, Paul},
	journal = {Phys. Rev. E},
	volume = {56},
	issue = {5},
	pages = {5174--5177},
	numpages = {0},
	year = {1997},
	month = {Nov},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevE.56.5174},
	url = {https://link.aps.org/doi/10.1103/PhysRevE.56.5174}
}

@article{shepelyansky:PRA:2003,
	title = {Entanglement versus relaxation and decoherence in a quantum algorithm for quantum chaos},
	author = {Bettelli, S. and Shepelyansky, D. L.},
	journal = {Phys. Rev. A},
	volume = {67},
	issue = {5},
	pages = {054303},
	numpages = {4},
	year = {2003},
	month = {May},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.67.054303},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.67.054303}
}

@article{brumer-jaffe:JPC:1984,
	author = {Jaffe, Charles and Brumer, Paul},
	title = {Classical Liouville mechanics and intramolecular relaxation dynamics},
	journal = {J. Phys. Chem.},
	volume = {88},
	number = {21},
	pages = {4829-4839},
	year = {1984},
	doi = {10.1021/j150665a007},
	URL = {https://doi.org/10.1021/j150665a007},
}

@article{brumer-jaffe:JCP:1985,
	author = {Jaffé, Charles and Brumer,Paul },
	title = {Classical‐quantum correspondence in the distribution dynamics of integrable systems},
	journal = {J. Chem. Phys.},
	volume = {82},
	number = {5},
	pages = {2330-2340},
	year = {1985},
	doi = {10.1063/1.448946},
	URL = {https://doi.org/10.1063/1.448946},
}

@article{brumer-jaffe:PRL:1985,
	title = {Classical Analog of Pure-State Quantum Dynamics},
	author = {Jaff\'e, Charles and Kanfer, Sheldon and Brumer, Paul},
	journal = {Phys. Rev. Lett.},
	volume = {54},
	pages = {8--10},
	year = {1985},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.54.8},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.54.8},
}

@article{brumer-wilkie:PRA:1997-1,
	title = {Quantum-classical correspondence via Liouville dynamics. I. Integrable systems and the chaotic spectral decomposition},
	author = {Wilkie, Joshua and Brumer, Paul},
	journal = {Phys. Rev. A},
	volume = {55},
	issue = {1},
	pages = {27--42},
	numpages = {0},
	year = {1997},
	month = {Jan},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.55.27},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.55.27}
}

@article{brumer-wilkie:PRA:1997-2,
	title = {Quantum-classical correspondence via Liouville dynamics. II. Correspondence for chaotic Hamiltonian systems},
	author = {Wilkie, Joshua and Brumer, Paul},
	journal = {Phys. Rev. A},
	volume = {55},
	issue = {1},
	pages = {43--61},
	numpages = {0},
	year = {1997},
	month = {Jan},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.55.43},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.55.43}
}

@article{wigner:PhysRev:1932,
	title = {On the Quantum Correction For Thermodynamic Equilibrium},
	author = {Wigner, E.},
	journal = {Phys. Rev.},
	volume = {40},
	issue = {5},
	pages = {749--759},
	numpages = {0},
	year = {1932},
	month = {Jun},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRev.40.749},
	url = {https://link.aps.org/doi/10.1103/PhysRev.40.749}
}

@article{moyal:MathProcCambrdPhilSoc:1949,
	title={Quantum mechanics as a statistical theory},
	volume={45},
	DOI={10.1017/S0305004100000487},
	number={1},
	journal={Mathematical Proceedings of the Cambridge Philosophical Society},
	publisher={Cambridge University Press},
	author={Moyal, J. E.},
	year={1949},
	pages={99–124},
}

@article{bell:physics:1964,
	title = {On the Einstein Podolsky Rosen paradox},
	author = {Bell, J. S.},
	journal = {Physics Physique Fizika},
	volume = {1},
	issue = {3},
	pages = {195--200},
	numpages = {6},
	year = {1964},
	month = {Nov},
	publisher = {American Physical Society},
	doi = {10.1103/PhysicsPhysiqueFizika.1.195},
	url = {https://link.aps.org/doi/10.1103/PhysicsPhysiqueFizika.1.195}
}

@article{bell:RMP:1966,
	title = {On the Problem of Hidden Variables in Quantum Mechanics},
	author = {J. S. Bell},
	journal = {Rev. Mod. Phys.},
	volume = {38},
	issue = {3},
	pages = {447--452},
	numpages = {0},
	year = {1966},
	month = {Jul},
	publisher = {American Physical Society},
	doi = {10.1103/RevModPhys.38.447},
	url = {https://link.aps.org/doi/10.1103/RevModPhys.38.447}
}

@article{bennett-brassard:PRL:1993,
	title = {Teleporting an unknown quantum state via dual classical and Einstein-Podolsky-Rosen channels},
	author = {Bennett, Charles H. and Brassard, Gilles and Cr\'epeau, Claude and Jozsa, Richard and Peres, Asher and Wootters, William K.},
	journal = {Phys. Rev. Lett.},
	volume = {70},
	issue = {13},
	pages = {1895--1899},
	numpages = {0},
	year = {1993},
	month = {Mar},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.70.1895},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.70.1895}
}

@article{boschi-popescu:PRL:1998,
	title = {Experimental Realization of Teleporting an Unknown Pure Quantum State via Dual Classical and Einstein-Podolsky-Rosen Channels},
	author = {Boschi, D. and Branca, S. and De Martini, F. and Hardy, L. and Popescu, S.},
	journal = {Phys. Rev. Lett.},
	volume = {80},
	issue = {6},
	pages = {1121--1125},
	numpages = {0},
	year = {1998},
	month = {Feb},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.80.1121},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.80.1121}
}

@article{ghirardi:JStatPhys:2002,
 author    = {G. Ghirardi and L. Marinatto and T. Weber},
 journal   = {J. Stat. Phys.},
 title     = {Entanglement and properties of composite quantum systems: A conceptual and mathematical analysis},
 volume    = {108},
 pages     = {49--122},
 year      = {2002},
 doi       = {10.1023/A:1015439502289},
 url       = {https://doi.org/10.1023/A:1015439502289},
}

@article{plenio-vedral:PRL:1997,
	title = {Quantifying entanglement},
	author = {Vedral, V. and Plenio, M. B. and Rippin, M. A. and Knight, P. L.},
	journal = {Phys. Rev. Lett.},
	volume = {78},
	issue = {12},
	pages = {2275--2279},
	numpages = {0},
	year = {1997},
	month = {Mar},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.78.2275},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.78.2275},
}

@article{plenio-vedral:PRA:1998,
	title = {Entanglement measures and purification procedures},
	author = {Vedral, V. and Plenio, M. B.},
	journal = {Phys. Rev. A},
	volume = {57},
	issue = {3},
	pages = {1619--1633},
	numpages = {0},
	year = {1998},
	month = {Mar},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.57.1619},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.57.1619}
}

@article{horodecki:QuantumInfComp:2001,
	author    = {Michal Horodecki},
	title     = {Entanglement measures},
	journal   = {Quantum Inf. Comput.},
	volume    = {1},
	number    = {1},
	pages     = {3--26},
	year      = {2001},
	url       = {https://doi.org/10.26421/QIC1.1-2},
	doi       = {10.26421/QIC1.1-2},
	timestamp = {Thu, 29 Apr 2021 18:05:34 +0200},
	biburl    = {https://dblp.org/rec/journals/qic/Horodecki01.bib},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{bruss:JMathPhys:2002,
	author = {Bru{\ss}, Dagmar},
	title = {Characterizing entanglement},
	journal = {Journal of Mathematical Physics},
	volume = {43},
	number = {9},
	pages = {4237-4251},
	year = {2002},
	doi = {10.1063/1.1494474},	
	URL = {https://doi.org/10.1063/1.1494474},
}

@article{buzek-knigh:PRA:1992,
	title = {Schr\"odinger-cat states in the resonant Jaynes-Cummings model: Collapse and revival of oscillations of the photon-number distribution},
	author = {Bu\ifmmode \check{z}\else \v{z}\fi{}ek, V. and Moya-Cessa, H. and Knight, P. L. and Phoenix, S. J. D.},
	journal = {Phys. Rev. A},
	volume = {45},
	issue = {11},
	pages = {8190--8203},
	numpages = {0},
	year = {1992},
	month = {Jun},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.45.8190},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.45.8190}
}

@article{bennett-smolin:PRL:1996,
	title = {Purification of Noisy Entanglement and Faithful Teleportation via Noisy Channels},
	author = {Bennett, Charles H. and Brassard, Gilles and Popescu, Sandu and Schumacher, Benjamin and Smolin, John A. and Wootters, William K.},
	journal = {Phys. Rev. Lett.},
	volume = {76},
	issue = {5},
	pages = {722--725},
	numpages = {0},
	year = {1996},
	month = {Jan},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.76.722},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.76.722}
}

@article{bennett-smolin:PRL:1997,
	title = {Purification of Noisy Entanglement and Faithful Teleportation via Noisy Channels[Phys. Rev. Lett. 76, 722 (1996)]},
	author = {Bennett, Charles H. and Brassard, Gilles and Popescu, Sandu and Schumacher, Benjamin and Smolin, John A. and Wootters, William K.},
	journal = {Phys. Rev. Lett.},
	volume = {78},
	issue = {10},
	pages = {2031--2031},
	numpages = {0},
	year = {1997},
	month = {Mar},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.78.2031},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.78.2031}
}

@article{bennett-smolin:PRA:1996,
	title = {Mixed-state entanglement and quantum error correction},
	author = {Bennett, Charles H. and DiVincenzo, David P. and Smolin, John A. and Wootters, William K.},
	journal = {Phys. Rev. A},
	volume = {54},
	issue = {5},
	pages = {3824--3851},
	numpages = {0},
	year = {1996},
	month = {Nov},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.54.3824},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.54.3824}
}

@article{verstraete:PRA:2003,
	title = {Maximal entanglement versus entropy for mixed quantum states},
	author = {Wei, Tzu-Chieh and Nemoto, Kae and Goldbart, Paul M. and Kwiat, Paul G. and Munro, William J. and Verstraete, Frank},
	journal = {Phys. Rev. A},
	volume = {67},
	issue = {2},
	pages = {022110},
	numpages = {12},
	year = {2003},
	month = {Feb},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.67.022110},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.67.022110}
}

@article{peres:PRL:1996,
	title = {Separability Criterion for Density Matrices},
	author = {Peres, Asher},
	journal = {Phys. Rev. Lett.},
	volume = {77},
	issue = {8},
	pages = {1413--1415},
	numpages = {0},
	year = {1996},
	month = {Aug},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.77.1413},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.77.1413}
}

@article{duan-cirac-zoller:PRL:2000,
	title = {Inseparability Criterion for Continuous Variable Systems},
	author = {Duan, Lu-Ming and Giedke, G. and Cirac, J. I. and Zoller, P.},
	journal = {Phys. Rev. Lett.},
	volume = {84},
	issue = {12},
	pages = {2722--2725},
	numpages = {0},
	year = {2000},
	month = {Mar},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.84.2722},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.84.2722}
}

@article{simon:PRL:2000,
	title = {Peres-Horodecki Separability Criterion for Continuous Variable Systems},
	author = {Simon, R.},
	journal = {Phys. Rev. Lett.},
	volume = {84},
	issue = {12},
	pages = {2726--2729},
	numpages = {0},
	year = {2000},
	month = {Mar},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.84.2726},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.84.2726}
}

@article{horodecki:PhysLettA:1996,
	title = {Separability of mixed states: necessary and sufficient conditions},
	journal = {Physics Letters A},
	volume = {223},
	number = {1},
	pages = {1-8},
	year = {1996},
	issn = {0375-9601},
	doi = {https://doi.org/10.1016/S0375-9601(96)00706-2},
	url = {https://www.sciencedirect.com/science/article/pii/S0375960196007062},
	author = {Michał Horodecki and Paweł Horodecki and Ryszard Horodecki},
	abstract = {We provide necessary and sufficient conditions for the separability of mixed states. As a result we obtain a simple criterion of the separability for 2 × 2 and 2 × 3 systems. Here, the positivity of the partial transposition of a state is necessary and sufficient for its separability. However, this is not the case in general. Some examples of mixtures which demonstrate the utility of the criterion are considered.}
}

@article{wehrl:RMP:1978,
	title = {General properties of entropy},
	author = {Wehrl, Alfred},
	journal = {Rev. Mod. Phys.},
	volume = {50},
	issue = {2},
	pages = {221--260},
	numpages = {0},
	year = {1978},
	month = {Apr},
	publisher = {American Physical Society},
	doi = {10.1103/RevModPhys.50.221},
	url = {https://link.aps.org/doi/10.1103/RevModPhys.50.221}
}

@article{wehrl:RepMathPhys:1979,
	title = {On the relation between classical and quantum-mechanical entropy},
	journal = {Reports on Mathematical Physics},
	volume = {16},
	number = {3},
	pages = {353-358},
	year = {1979},
	issn = {0034-4877},
	doi = {https://doi.org/10.1016/0034-4877(79)90070-3},
	url = {https://www.sciencedirect.com/science/article/pii/0034487779900703},
	author = {Alfred Wehrl},
	abstract = {We discuss the problem how to define the classical entropy and prove an inequality that establishes its relation to the quantum-mechanical entropy. Furthermore we show that it is monotonic.}
}

@article{wehrl:RepMathPhys:1991,
	title = {The many facets of entropy},
	journal = {Reports on Mathematical Physics},
	volume = {30},
	number = {1},
	pages = {119-129},
	year = {1991},
	issn = {0034-4877},
	doi = {https://doi.org/10.1016/0034-4877(91)90045-O},
	url = {https://www.sciencedirect.com/science/article/pii/003448779190045O},
	author = {A. Wehrl},
	abstract = {Several notions of entropy are discussed: classical entropies (Boltzmann, Gibbs, Shannon, quantum-mechanical entropy, skew entropy, among other notions as well as classical and quantum-mechanical dynamical entropies.}
}

@article{popescu-rohrlich:PRA:1997,
	title = {Thermodynamics and the measure of entanglement},
	author = {Popescu, Sandu and Rohrlich, Daniel},
	journal = {Phys. Rev. A},
	volume = {56},
	issue = {5},
	pages = {R3319--R3321},
	numpages = {0},
	year = {1997},
	month = {Nov},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.56.R3319},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.56.R3319}
}

@article{HDmeyer:JCP:1986,
	author = {Meyer, Hans-Dieter},
	title = {Theory of the Liapunov exponents of Hamiltonian systems and a numerical study on the transition from regular to irregular classical motion},
	journal = {J. Chem. Phys.},
	volume = {84},
	number = {6},
	pages = {3147-3161},
	year = {1986},
	doi = {10.1063/1.450296},
    URL = {https://doi.org/10.1063/1.450296},
}

@article{dahlqvist:PRL:1990,
	title = {Existence of stable orbits in the ${\mathit{x}}^{2}$${\mathit{y}}^{2}$ potential},
	author = {Dahlqvist, Per and Russberg, Gunnar},
	journal = {Phys. Rev. Lett.},
	volume = {65},
	issue = {23},
	pages = {2837--2838},
	numpages = {0},
	year = {1990},
	month = {Dec},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.65.2837},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.65.2837}
}

@article{bohigas:PhysRep:1993,
	title = {Manifestations of classical phase space structures in quantum mechanics},
	journal = {Physics Reports},
	volume = {223},
	number = {2},
	pages = {43-133},
	year = {1993},
	issn = {0370-1573},
	doi = {https://doi.org/10.1016/0370-1573(93)90109-Q},
	url = {https://www.sciencedirect.com/science/article/pii/037015739390109Q},
	author = {O. Bohigas and S. Tomsovic and D. Ullmo},
	abstract = {Using two coupled quartic oscillators for illustration, the quantum mechanics of simple systems whose classical analogs have varying degrees of non-integrability is investigated. By taking advantage of discrete symmetries and dynamical quasidegeneracies it is shown that Percival's semiclassical classification scheme, i.e., eigenstates may be separated into a regular and an irregular group, basically works. This allows us to probe deeply into the workings of semiclassical quantization in mixed phase space systems. Some observations of intermediate status states are made. The standard modeling of quantum fluctuation properties exhibited by the irregular states and levels by random matrix ensembles is then put on a physical footing. Generalized ensembles are constructed incorporating such classical information as fluxes crossing partial barriers and relative fractions of phase space volume occupied by interesting subregions. The ensembles apply equally well to both spectral and eigenstate properties. They typically show non-universal, but nevertheless characteristic level fluctuations. In addition, they predict “semiclassical localization” of eigenfunctions and “quantum suppression of chaos” which are quantitatively borne out in the quantum systems.}
}

@article{eckhardt-pollak:PRA:1989,
	title = {Quantum mechanics of a classically chaotic system: Observations on scars, periodic orbits, and vibrational adiabaticity},
	author = {Eckhardt, Bruno and Hose, Gabriel and Pollak, Eli},
	journal = {Phys. Rev. A},
	volume = {39},
	issue = {8},
	pages = {3776--3793},
	numpages = {0},
	year = {1989},
	month = {Apr},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.39.3776},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.39.3776}
}

@article{polavieja-borondo:PRL:1994,
	title = {Scars in Groups of Eigenstates in a Classically Chaotic System},
	author = {de Polavieja, G. G. and Borondo, F. and Benito, R. M.},
	journal = {Phys. Rev. Lett.},
	volume = {73},
	issue = {12},
	pages = {1613--1616},
	numpages = {0},
	year = {1994},
	month = {Sep},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.73.1613},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.73.1613}
}

@article{brumer-gong:PRA:2003,
	title = {Intrinsic decoherence dynamics in smooth Hamiltonian systems: Quantum-classical correspondence},
	author = {Gong, Jiangbin and Brumer, Paul},
	journal = {Phys. Rev. A},
	volume = {68},
	issue = {2},
	pages = {022101},
	numpages = {8},
	year = {2003},
	month = {Aug},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.68.022101},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.68.022101}
}

@article{vedral-maruyama:PRA:2005,
	title = {Thermodynamical detection of entanglement by Maxwell's demons},
	author = {Maruyama, Koji and Morikoshi, Fumiaki and Vedral, Vlatko},
	journal = {Phys. Rev. A},
	volume = {71},
	issue = {1},
	pages = {012108},
	numpages = {5},
	year = {2005},
	month = {Jan},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.71.012108},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.71.012108}
}

@article{shannon:BellSystTechJ:1948-1,
	author={Shannon, C. E.},
	journal={The Bell System Technical Journal}, 
	title={A mathematical theory of communication}, 
	year={1948},
	volume={27},
	number={3},
	pages={379--423},
	doi={10.1002/j.1538-7305.1948.tb01338.x},
}

@article{shannon:BellSystTechJ:1948-2,
	author={Shannon, C. E.},
	journal={The Bell System Technical Journal}, 
	title={A mathematical theory of communication}, 
	year={1948},
	volume={27},
	number={4},
	pages={623--656},
	doi={10.1002/j.1538-7305.1948.tb00917.x},
}

@ARTICLE{shannon:BellSystTechJ:1949,
	author={Shannon, C. E.},
	journal={The Bell System Technical Journal}, 
	title={Communication theory of secrecy systems}, 
	year={1949},
	volume={28},
	number={4},
	pages={656--715},
	doi={10.1002/j.1538-7305.1949.tb00928.x},
}

@article{weyl:ZPhys:1927,
 author    = {H. Weyl},
 journal   = {Zeitschrift f{\"{u}}r Physik},
 title     = {Quantenmechanik und Gruppentheorie},
 volume    = {46},
 pages     = {1--46},
 year      = {1927},
 doi       = {10.1007/BF02055756},
 url       = {https://doi.org/10.1007/BF02055756},
}

@article{gosson:Quanta:2018,
	author = {Maurice de Gosson},
	title = {Quantum Harmonic Analysis of the Density Matrix},
	journal = {Quanta},
	volume = {7},
	number = {1},
	year = {2018},
	abstract = {We will study rigorously the notion of mixed states and their density matrices. We will also discuss the quantum-mechanical consequences of possible variations of Planck's constant h. This review has been written having in mind two readerships: mathematical physicists and quantum physicists. The mathematical rigor is maximal, but the language and notation we use throughout should be familiar to physicists.Quanta 2018; 7: 74–110.},
	issn = {1314-7374},
	pages = {74--110},
	doi = {10.12743/quanta.v7i1.74},
	url = {http://quanta.ws/ojs/index.php/quanta/article/view/74},
}

@article{brumer-gong:PRL:2003,
	title = {When is Quantum Decoherence Dynamics Classical?},
	author = {Gong, Jiangbin and Brumer, Paul},
	journal = {Phys. Rev. Lett.},
	volume = {90},
	issue = {5},
	pages = {050402},
	numpages = {4},
	year = {2003},
	month = {Feb},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.90.050402},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.90.050402}
}

@article{brumer-gong:JModOpt:2003,
	author = {J. Gong and P. Brumer},
	title = {Quantum versus classical decoherence dynamics},
	journal = {Journal of Modern Optics},
	volume = {50},
	number = {15-17},
	pages = {2411-2422},
	year  = {2003},
	publisher = {Taylor & Francis},
	doi = {10.1080/09500340308233572},
	URL = {https://www.tandfonline.com/doi/abs/10.1080/09500340308233572},
	eprint = {https://www.tandfonline.com/doi/pdf/10.1080/09500340308233572},	
}

@article{milburn:PRA:1986,
	title = {Quantum and classical Liouville dynamics of the anharmonic oscillator},
	author = {Milburn, G. J.},
	journal = {Phys. Rev. A},
	volume = {33},
	issue = {1},
	pages = {674--685},
	numpages = {0},
	year = {1986},
	month = {Jan},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.33.674},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.33.674}
}

@article{joy:ModPhysLettB:1993,
	author    = {M. P. Joy and M. Sabir},
	journal   = {Mod. Phys. Lett. B},
	title     = {Chaos and quantum fluctuations in a quartic Hamiltonian system},
	volume    = {7},
	pages     = {1421--1427},
	year      = {1993},
	doi       = {10.1142/S0217984993001466},
    url       = {https://www.worldscientific.com/doi/10.1142/S0217984993001466},
}

@article{sanz:PRE:2012,
	title = {Temperature crossover of decoherence rates in chaotic and regular bath dynamics},
	author = {Sanz, A. S. and Elran, Y. and Brumer, P.},
	journal = {Phys. Rev. E},
	volume = {85},
	issue = {3},
	pages = {036218},
	numpages = {6},
	year = {2012},
	month = {Mar},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevE.85.036218},
	url = {https://link.aps.org/doi/10.1103/PhysRevE.85.036218},
}

@article{scully:JCP:1982,
	author = {Lee,Hai‐Woong  and Scully,Marlan O. },
	title = {Wigner phase‐space description of a Morse oscillator},
	journal = {J. Chem. Phys.},
	volume = {77},
	number = {9},
	pages = {4604-4610},
	year = {1982},
	doi = {10.1063/1.444412},
	URL = {https://doi.org/10.1063/1.444412},
	eprint = {https://doi.org/10.1063/1.444412},	
}

@article{schlosshauer:PhysRep:2019,
	author = {Maximilian Schlosshauer},
	title = {Quantum decoherence},
	journal = {Phys. Rep.},
	volume = {831},
	pages = {1-57},
	year = {2019},
	note = {Quantum decoherence},
	issn = {0370-1573},
	doi = {https://doi.org/10.1016/j.physrep.2019.10.001},
	url = {https://www.sciencedirect.com/science/article/pii/S0370157319303084},
}

@article{philippidis:NuovoCim:1982,
	author = {C. Philippidis and D. Bohm and R. D. Kaye},
	title = {The Aharonov-Bohm effect and the quantum potential},
	journal = {Nuovo Cim. B},
	volume = {71},
	pages = {57-88},
	year = {1982},
	issn = {1826-9877},
	doi = {10.1007/BF02721695},
	url = {https://doi.org/10.1007/BF02721695},
}

@BOOK{peres-bk,
  AUTHOR     = {A. Peres},
  TITLE      = {Quantum Theory: Concepts and Methods},
  PUBLISHER  = {Kluwer Academic Publishers},
  YEAR       = {2002},
  address    = {New York},
}

@article{aiello:OptLett:2016,
author = {Andrea Aiello},
journal = {Opt. Lett.},
number = {7},
pages = {1668--1671},
publisher = {Optica Publishing Group},
title = {Spontaneous generation of singularities in paraxial optical fields},
volume = {41},
month = {Apr},
year = {2016},
url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-41-7-1668},
doi = {10.1364/OL.41.001668}
}

@article{aiello:OSACont:2020,
author = {Andrea Aiello and Martin Pa\'{u}r and Bohumil Stoklasa and Zden\v{e}k Hradil and Jaroslav \v{R}eh\'{a}\v{c}ek and Luis L. S\'{a}nchez-Soto},
journal = {OSA Continuum},
number = {9},
pages = {2387--2394},
publisher = {Optica Publishing Group},
title = {Observation of concentrating paraxial beams},
volume = {3},
month = {Sep},
year = {2020},
url = {https://opg.optica.org/osac/abstract.cfm?URI=osac-3-9-2387},
doi = {10.1364/OSAC.400410}
}

@article{porras:PRA:2021,
  title = {Exploding paraxial beams, vortex beams, and cylindrical beams of light with finite power in linear media, and their enhanced longitudinal field},
  author = {Porras, Miguel A.},
  journal = {Phys. Rev. A},
  volume = {103},
  issue = {3},
  pages = {033506},
  numpages = {7},
  year = {2021},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.103.033506},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.103.033506}
}

@article{berry:AJP:1979,
 author    = {M. V. Berry and N. L. Balazs},
 journal   = {Am. J. Phys.},
 title     = {Nonspreading wave packets},
 volume    = {47},
 pages     = {264-267},
 year      = {1979},
 doi       = {10.1119/1.11855},
}

@article{unnikrishnan:AJP:1996,
 author    = {K. Unnikrishnan and A. R. P. Rau},
 journal   = {Am. J. Phys.},
 title     = {Uniqueness of the {Airy}  packet in quantum mechanics},
 volume    = {64},
 pages     = {1034-1035},
 year      = {1996},
 doi       = {10.1119/1.18322},
}

@article{greenberger:AJP:1980,
	author = {D. M. Greenberger},
	title = {Comment on ``Nonspreading wave packets’’},
	journal = {Am. J. Phys.},
	volume = {48},
	number = {3},
	pages = {256-256},
	year = {1980},
	doi = {10.1119/1.12308},
	URL = {https://doi.org/10.1119/1.12308},
	eprint = {https://doi.org/10.1119/1.12308},
}

@article{besieris:AJP:1994,
	author = {I. M. Besieris and A. M. Shaarawi and R. W. Ziolkowski},
	title = {Nondispersive accelerating wave packets},
	journal = {Am. J. Phys.},
	volume = {62},
	number = {6},
	pages = {519-521},
	year = {1994},
	doi = {10.1119/1.17510},	
	URL = {https://doi.org/10.1119/1.17510},
	eprint = {https://doi.org/10.1119/1.17510},	
}

@article{nguyen:ApplMathComput:2012,
	title = {Construction of accelerating wavepackets},
	author = {H. Nguyen and J. Lekner},
	journal = {Appl. Math. Comput.},
	volume = {218},
	number = {22},
	pages = {10990-10997},
	year = {2012},
    doi = {https://doi.org/10.1016/j.amc.2012.04.060},
	url = {https://www.sciencedirect.com/science/article/pii/S0096300312004596},
}

@article{lekner:EJP:2009,
	title = {Airy wavepacket solutions of the Schr\"odinger equation},
    journal = {Eur. J. Phys.},
	author = {J. Lekner},
	doi = {10.1088/0143-0807/30/3/l04},
	url = {https://doi.org/10.1088/0143-0807/30/3/l04},
	year = 2009,
	month = {apr},
	publisher = {{IOP} Publishing},
	volume = {30},
	number = {3},
	pages = {L43--L46},
}

@Article{arie:Fluids:2019,
	AUTHOR = {G. G. Rozenman and S. Fu and A. Arie and L. Shemer},
	TITLE = {Quantum Mechanical and Optical Analogies in Surface Gravity Water Waves},
	JOURNAL = {Fluids},
	VOLUME = {4},
	YEAR = {2019},
	NUMBER = {2},
	ARTICLE-NUMBER = {96},
	URL = {https://www.mdpi.com/2311-5521/4/2/96},
	DOI = {10.3390/fluids4020096},
}

@article{arie:PRL:2015-1,
	title = {Propagation Dynamics of {Airy}  Water-Wave Pulses},
	author = {Fu, Shenhe and Tsur, Yuval and Zhou, Jianying and Shemer, Lev and Arie, Ady},
	journal = {Phys. Rev. Lett.},
	volume = {115},
	issue = {3},
	pages = {034501},
	numpages = {5},
	year = {2015},
	month = {Jul},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.115.034501},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.115.034501}
}

@article{arie:PhysScr:2019,
	title = {Nanostructuring of electron beams},
    journal = {Phys. Scr.},
	author = {Roy Shiloh and Peng-Han Lu and Roei Remez and Amir H Tavabi and Giulio Pozzi and Rafal E Dunin-Borkowski and Ady Arie},
	doi = {10.1088/1402-4896/aaf258},
	url = {https://doi.org/10.1088/1402-4896/aaf258},
	year = {2019},
	month = {jan},
	publisher = {{IOP} Publishing},
	volume = {94},
	number = {3},
	pages = {034004},
}

@article{voloch:Nature:2013,
	author    = {N. Voloch-Bloch and Y. Lereah and Y. Lilach and A. Gover and A. Arie},
	journal   = {Nature},
	title     = {Generation of electron {Airy}  beams},
	volume    = {494},
	pages     = {331-335},
	year      = {2013},
	doi = {https://doi.org/10.1038/nature11840},
}

@article{wang:JPlasmaPhys:2016,
 title={Airy-like electron plasma wave},
 journal={J. Plasma Phys.},
 author={H. Li and X. Li and J. Wang},
 volume={82},
 DOI={10.1017/S0022377816000039},
 number={1},
 publisher={Cambridge University Press},
 year={2016},
 pages={905820103},
}

@ARTICLE{kang:IEEEJQE:2017,	
	title={Nonparaxial Accelerating Electron Beams}, 
	author={Y. Kang and Y. Zhang and C. Li and H. Zhong and Y. Zhang and M. R. Beli\'c},
	journal={IEEE J. Quantum Electron.}, 
	year={2017},
	volume={53},
	number={2},
	pages={1-6},
	doi={10.1109/JQE.2017.2677382},
}

@article{christodoulides:PRL:2007,
title = {Observation of Accelerating {Airy}  Beams},
author = {Siviloglou, G. A. and Broky, J. and Dogariu, A. and Christodoulides, D. N.},
journal = {Phys. Rev. Lett.},
volume = {99},
issue = {21},
pages = {213901},
numpages = {4},
year = {2007},
month = {Nov},
publisher = {American Physical Society},
doi = {10.1103/PhysRevLett.99.213901},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.99.213901}
}

@article{arie:PRL:2015-2,
  title = {Unveiling the Orbital Angular Momentum and Acceleration of Electron Beams},
  author = {Shiloh, Roy and Tsur, Yuval and Remez, Roei and Lereah, Yossi and Malomed, Boris A. and Shvedov, Vladlen and Hnatovsky, Cyril and Krolikowski, Wieslaw and Arie, Ady},
  journal = {Phys. Rev. Lett.},
  volume = {114},
  issue = {9},
  pages = {096102},
  numpages = {5},
  year = {2015},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.114.096102},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.114.096102}
}

@article{efremidis:PRA:2021,
  title = {Dynamics of self-accelerating electron beams in a homogeneous magnetic field},
  author = {Goutsoulas, Michael and Efremidis, Nikolaos K.},
  journal = {Phys. Rev. A},
  volume = {103},
  issue = {1},
  pages = {013519},
  numpages = {7},
  year = {2021},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.103.013519},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.103.013519}
}

@article{efremidis:PRA:2013,
  title = {Accelerating and abruptly autofocusing matter waves},
  author = {Efremidis, Nikolaos K. and Paltoglou, Vassilis and von Klitzing, Wolf},
  journal = {Phys. Rev. A},
  volume = {87},
  issue = {4},
  pages = {043637},
  numpages = {9},
  year = {2013},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.87.043637},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.87.043637}
}

@article{yuce:MPLB:2015,
author = {Yuce, C.},
title = {Self-accelerating matter waves},
journal = {Modern Physics Letters B},
volume = {29},
number = {28},
pages = {1550171},
year = {2015},
doi = {10.1142/S0217984915501717},
URL = {https://doi.org/10.1142/S0217984915501717},
eprint = {https://doi.org/10.1142/S0217984915501717},
}

@article{christodoulides:Optica:2019,
	title = {Airy beams and accelerating waves: an overview of recent advances},
	author = {Nikolaos K. Efremidis and Zhigang Chen and Mordechai Segev and Demetrios N. Christodoulides},
	journal = {Optica},
	keywords = {Airy beams; Medical imaging; Near field scanning optical microscopy; Nonlinear wave mixing; Optical force; Spatial light modulators},
	number = {5},
	pages = {686--701},
	publisher = {Optica Publishing Group},
	volume = {6},
	month = {May},
	year = {2019},
	url = {http://opg.optica.org/optica/abstract.cfm?URI=optica-6-5-686},
	doi = {10.1364/OPTICA.6.000686},
}

@article{gori:OptLett:2007,
author = {F. Gori and M. Santarsiero},
journal = {Opt. Lett.},
number = {24},
pages = {3531--3533},
publisher = {Optica Publishing Group},
title = {Devising genuine spatial correlation functions},
volume = {32},
month = {Dec},
year = {2007},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-32-24-3531},
doi = {10.1364/OL.32.003531},
}

@article{martinezherrero:OptLett:2009-1,
author = {R. Mart\'{i}nez-Herrero and P. M. Mej\'{i}as and F. Gori},
journal = {Opt. Lett.},
number = {9},
pages = {1399--1401},
publisher = {Optica Publishing Group},
title = {Genuine cross-spectral densities and pseudo-modal expansions},
volume = {34},
month = {May},
year = {2009},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-34-9-1399},
doi = {10.1364/OL.34.001399},
}

@article{martinezherrero:OptLett:2009-2,
author = {Rosario Mart\'{i}nez-Herrero and Pedro M. Mej\'{i}as},
journal = {Opt. Lett.},
number = {15},
pages = {2303--2305},
publisher = {Optica Publishing Group},
title = {Elementary-field expansions of genuine cross-spectral density matrices},
volume = {34},
month = {Aug},
year = {2009},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-34-15-2303},
doi = {10.1364/OL.34.002303},
}

@article{martinezherrero:JOSAA:2021,
author = {Franco Gori and Rosario Mart\'{i}nez-Herrero},
journal = {J. Opt. Soc. Am. A},
number = {5},
pages = {737--748},
publisher = {Optica Publishing Group},
title = {Reproducing Kernel Hilbert spaces for wave optics: tutorial},
volume = {38},
month = {May},
year = {2021},
url = {http://opg.optica.org/josaa/abstract.cfm?URI=josaa-38-5-737},
doi = {10.1364/JOSAA.422738},
}

@BOOK{mandelwolf-bk,
  AUTHOR =       {L. Mandel and E. Wolf},
  TITLE =        {Optical Coherence and Quantum Optics},
  PUBLISHER =    {Cambridge University Press},
  YEAR =         {1995},
  address =      {Cambridge},
}

@article{qureshi:OptLett:2021,
author = {Tabish Qureshi},
journal = {Opt. Lett.},
number = {3},
pages = {492--495},
publisher = {Optica Publishing Group},
title = {Predictability, distinguishability, and entanglement},
volume = {46},
month = {Feb},
year = {2021},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-46-3-492},
doi = {10.1364/OL.415556},
}

@article{ponomarenko:OptLett:2021,
author = {Morteza Hajati and Vincent Sieben and Sergey A. Ponomarenko},
journal = {Opt. Lett.},
number = {16},
pages = {3961--3964},
publisher = {Optica Publishing Group},
title = {Airy beams on incoherent background},
volume = {46},
month = {Aug},
year = {2021},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-46-16-3961},
doi = {10.1364/OL.434168},
}

@article{lumer:Optica:2015,
author = {Yaakov Lumer and Yi Liang and Ran Schley and Ido Kaminer and Elad Greenfield and Daohong Song and Xinzheng Zhang and Jingjun Xu and Zhigang Chen and Mordechai Segev},
journal = {Optica},
number = {10},
pages = {886--892},
publisher = {Optica Publishing Group},
title = {Incoherent self-accelerating beams},
volume = {2},
month = {Oct},
year = {2015},
url = {http://opg.optica.org/optica/abstract.cfm?URI=optica-2-10-886},
doi = {10.1364/OPTICA.2.000886},
}

@article{christodoulides:OptLett:2007,
author = {Georgios A. Siviloglou and Demetrios N. Christodoulides},
journal = {Opt. Lett.},
number = {8},
pages = {979--981},
publisher = {Optica Publishing Group},
title = {Accelerating finite energy {Airy}  beams},
volume = {32},
month = {Apr},
year = {2007},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-32-8-979},
doi = {10.1364/OL.32.000979},
}

@article{forbes:NatCommun:2013,
author = {S. Ngcobo and I. Litvin and L. Burger, and A. Forbes},
journal = {Nat. Commun.},
number = {1},
pages = {2289},
title = {A digital laser for on-demand laser modes},
volume = {4},
year = {2013},
url = {https://doi.org/10.1038/ncomms3289},
doi = {10.1038/ncomms3289},
}

@article{arie:OptLett:2011,
author = {Gil Porat and Ido Dolev and Omri Barlev and Ady Arie},
journal = {Opt. Lett.},
number = {20},
pages = {4119--4121},
publisher = {Optica Publishing Group},
title = {Airy beam laser},
volume = {36},
month = {Oct},
year = {2011},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-36-20-4119},
doi = {10.1364/OL.36.004119},
}

@article{liu:OptExpress:2020,
author = {Xin Liu and Dening Xia and Yashar E. Monfared and Chunhao Liang and Fei Wang and Yangjian Cai and Pujuan Ma},
journal = {Opt. Express},
number = {7},
pages = {9777-9785},
title = {Generation of novel partially coherent truncated {Airy}  beams via Fourier phase processing},
volume = {28},
year = {2020},
url = {https://doi.org/10.1038/ncomms3289},
doi = {10.1364/OE.390477},
}

@article{christodoulides:OptExpress:2008,
author = {John Broky and Georgios A. Siviloglou and Aristide Dogariu and Demetrios N. Christodoulides},
journal = {Opt. Express},
number = {17},
pages = {12880--12891},
publisher = {Optica Publishing Group},
title = {Self-healing properties of optical {Airy}  beams},
volume = {16},
month = {Aug},
year = {2008},
url = {http://opg.optica.org/oe/abstract.cfm?URI=oe-16-17-12880},
doi = {10.1364/OE.16.012880},
}

@incollection{korotkova:ProgOpt:2020,
	author = {O. Korotkova and G. Gbur},
	title = {Chapter Four - Applications of optical coherence theory},
	editor = {T. D. Visser},
	series = {Prog. Opt.},
	publisher = {Elsevier},
	volume = {65},
	pages = {43-104},
	year = {2020},
	booktitle = {A Tribute to Emil Wolf},
	issn = {0079-6638},
	doi = {https://doi.org/10.1016/bs.po.2019.11.004},
	url = {https://www.sciencedirect.com/science/article/pii/S0079663819300204},
}

@article{berry:PTRSA:2002,
 author    = {M. V. Berry},
 journal   = {Phil. Trans. R. Soc. A.},
 title     = {Exuberant interference: rainbows, tides, edges, (de)coherence \ldots},
 volume    = {360},
 pages     = {1023--1037},
 year      = {2002},
 doi       = {10.1098/rsta.2001.0979},
}

@article{berry:PhysToday:2017,
 author    = {M. V. Berry},
 journal   = {Phys. Today},
 title     = {Approaches to studying our history},
 volume    = {70},
 issue     = {3},
 month     = {March},
 pages     = {11--12},
 year      = {2017},
 doi       = {10.1063/PT.3.3478},
}

@article{braunbek:ZNaturA:1951,
 author    = {W. Braunbek},
 journal   = {Z. Naturforsch. A},
 title     = {Zur Darstellung von Wellenfeldern},
 volume    = {6},
 pages     = {12--15},
 year      = {1951},
 doi       = {10.1515/zna-1951-0102},
}

@ARTICLE{wong:FrontPhys:2021,
author={Ren, Yu-Xuan and He, Hongsen and Tang, Huajun and Wong, Kenneth K. Y.},
TITLE={Non-diffracting light wave: Fundamentals and biomedical applications},      
JOURNAL={Front. Phys.},   
pages={698343(1--30)},   
VOLUME={9},           
YEAR={2021},      
URL={https://www.frontiersin.org/articles/10.3389/fphy.2021.698343},       
DOI={10.3389/fphy.2021.698343},
}

@article{greenberger:RMP:1979,
  title = {Coherence effects in neutron diffraction and gravity experiments},
  author = {Greenberger, Daniel M. and Overhauser, A. W.},
  journal = {Rev. Mod. Phys.},
  volume = {51},
  issue = {1},
  pages = {43--78},
  numpages = {0},
  year = {1979},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.51.43},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.51.43}
}

@article{colella:PRL:1975,
  title = {Observation of Gravitationally Induced Quantum Interference},
  author = {Colella, R. and Overhauser, A. W. and Werner, S. A.},
  journal = {Phys. Rev. Lett.},
  volume = {34},
  issue = {23},
  pages = {1472--1474},
  numpages = {0},
  year = {1975},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.34.1472},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.34.1472}
}

@article{langhoff:AJP:1971,
author = {Langhoff, P. W.},
title = {Schr\"odinger Particle in a Gravitational Well},
journal = {Am. J. Phys.},
volume = {39},
number = {8},
pages = {954-957},
year = {1971},
doi = {10.1119/1.1986333},
URL = {https://doi.org/10.1119/1.1986333},
eprint = {https://doi.org/10.1119/1.1986333},
}

@article{gibbs:AJP:1975,
author = {Gibbs, R. L.},
title = {The quantum bouncer},
journal = {American Journal of Physics},
volume = {43},
number = {1},
pages = {25-28},
year = {1975},
doi = {10.1119/1.10024},
URL = {https://doi.org/10.1119/1.10024},
eprint = {https://doi.org/10.1119/1.10024},
}

@article{desko:AJP:1983,
author = {Desko, R. D. and Bord, D. J.},
title = {The quantum bouncer revisited},
journal = {Am. J. Phys.},
volume = {51},
number = {1},
pages = {82-84},
year = {1983},
doi = {10.1119/1.13400},
URL = {https://doi.org/10.1119/1.13400},
eprint = {https://doi.org/10.1119/1.13400},
}

@article{geabanacloche:AJP:1999,
author = {Gea-Banacloche, J.},
title = {A quantum bouncing ball},
journal = {Am. J. Phys.},
volume = {67},
number = {9},
pages = {776-782},
year = {1999},
doi = {10.1119/1.19124},
URL = {https://doi.org/10.1119/1.19124},
eprint = {https://doi.org/10.1119/1.19124},
}

@article{nesvizhevsky:NuclInstMethPhys:2000,
title = {Search for quantum states of the neutron in a gravitational field: gravitational levels},
journal = {Nucl. Instrum. Methods Phys. Res. A},
volume = {440},
number = {3},
pages = {754-759},
year = {2000},
issn = {0168-9002},
doi = {10.1016/S0168-9002(99)01077-3},
url = {https://www.sciencedirect.com/science/article/pii/S0168900299010773},
author = {V. V. Nesvizhevsky and H. B\"orner and A. M. Gagarski and G. A. Petrov and A. K. Petukhov and H. Abele and S. B\"a{\ss}ler and T St\"oferle and S. M. Soloviev},
}

@article{nesvizhevsky:Nature:2002,
 author    = {V. V. Nesvizhevsky and H. G. B\"orner and A. K. Petukhov and H. Abele and S. B\"a{\ss}ler and F. J. Rue{\ss}, T. St\"oferle and A. Westphal and A. M. Gagarski and G. A. Petrov and A. V. Strelkov},
 journal   = {Nature},
 title     = {Quantum states of neutrons in the Earth's gravitational field},
 volume    = {415},
 pages     = {297-299},
 year      = {2002},
 doi       = {10.1038/415297a},
}

@article{nesvizhevsky:EurPhysJC:2005,
 author    = {V. V. Nesvizhevsky and A. K. Petukhov and H. G. B\"orner and T. A. Baranova and A. M. Gagarski and G. A. Petrov and K. V. Protasov and A. Yu. Voronin and S. B\"a{\ss}ler and H. Abele and A. Westphal and L. Lucovac},
 journal   = {Eur. Phys. J. C},
 title     = {Study of the neutron quantum states in the gravity field},
 volume    = {40},
 pages     = {479--491},
 year      = {2005},
 doi       = {10.1140/epjc/s2005-02135-y},
}

@misc{NIST:DLMF,
         key = "{\relax DLMF}",
       title = "{\it NIST Digital Library of Mathematical Functions}",
howpublished = "http://dlmf.nist.gov/, Release 1.1.6 of 2022-06-30",
         url = "http://dlmf.nist.gov/",
        note = "F.~W.~J. Olver, A.~B. {Olde Daalhuis}, D.~W. Lozier, B.~I. Schneider,
                R.~F. Boisvert, C.~W. Clark, B.~R. Miller, B.~V. Saunders,
                H.~S. Cohl, and M.~A. McClain, eds."}

@article{wang:JQuantSpectrRadTrans:2022,
title = {Dual autofocusing circular {Airy}  beams with different initial launch angles},
journal = {Journal of Quantitative Spectroscopy and Radiative Transfer},
volume = {278},
pages = {108010},
year = {2022},
issn = {0022-4073},
doi = {10.1016/j.jqsrt.2021.108010},
url = {https://www.sciencedirect.com/science/article/pii/S002240732100501X},
author = {Yingfei Wang and Yunfeng Jiang},
}

@article{christodoulides:OptLett:2010,
author = {Nikolaos K. Efremidis and Demetrios N. Christodoulides},
journal = {Opt. Lett.},
number = {23},
pages = {4045--4047},
publisher = {Optica Publishing Group},
title = {Abruptly autofocusing waves},
volume = {35},
month = {Dec},
year = {2010},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-35-23-4045},
doi = {10.1364/OL.35.004045},
}

@article{christodoulides:OptLett:2011-1,
author = {Ioannis Chremmos and Peng Zhang and Jai Prakash and Nikolaos K. Efremidis and Demetrios N. Christodoulides and Zhigang Chen},
journal = {Opt. Lett.},
number = {18},
pages = {3675--3677},
publisher = {Optica Publishing Group},
title = {Fourier-space generation of abruptly autofocusing beams and optical bottle beams},
volume = {36},
month = {Sep},
year = {2011},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-36-18-3675},
doi = {10.1364/OL.36.003675},
}

@article{christodoulides:OptLett:2011-2,
author = {Dimitrios G. Papazoglou and Nikolaos K. Efremidis and Demetrios N. Christodoulides and Stelios Tzortzakis},
journal = {Opt. Lett.},
number = {10},
pages = {1842--1844},
publisher = {Optica Publishing Group},
title = {Observation of abruptly autofocusing waves},
volume = {36},
month = {May},
year = {2011},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-36-10-1842},
doi = {10.1364/OL.36.001842},
}

@article{tzortzakis:NatCommun:2013,
 author    = {P. Panagiotopoulos and D. G. Papazoglou and A. Couairon and S. Tzortzakis},
 journal   = {Nat. Commun.},
 title     = {Sharply autofocused ring-Airy beams transforming into non-linear intense light bullets},
 volume    = {4},
 pages     = {2622(1-6)},
 year      = {2013},
 doi       = {10.1038/ncomms3622},
 url       = {https://doi.org/10.1038/ncomms3622},
}

@article{bliokh:PhysRep:2015,
	title = {Transverse and longitudinal angular momenta of light},
	journal = {Phys. Rep.},
	volume = {592},
	pages = {1-38},
	year = {2015},
	issn = {0370-1573},
	doi = {10.1016/j.physrep.2015.06.003},
	url = {https://www.sciencedirect.com/science/article/pii/S0370157315003336},
	author = {Konstantin Y. Bliokh and Franco Nori},
}

@article{serbo:PhysUsp:2018,
	author    = {B. A. Knyazev and V. G. Serbo},
	journal   = {Phys. Usp.},
	title     = {Beams of photons with nonzero projections of orbital angular momenta: New results},
	volume    = {61},
	pages     = {449--479},
	year      = {2018},
	doi = {10.3367/UFNr.2018.02.038306},
}

@article{andreev:JOSAB:2022,
	author = {A. V. Andreev and O. A. Shoutova and S. M. Trushin and S. Yu. Stremoukhov},
	journal = {J. Opt. Soc. Am. B},
	keywords = {Circular polarization; Femtosecond lasers; First order optics; Gaussian beams; Nonlinear optical crystals; Process control},
	number = {7},
	pages = {1775--1782},
	publisher = {Optica Publishing Group},
	title = {3D Stokes parameters for vector focal fields},
	volume = {39},
	month = {Jul},
	year = {2022},
	url = {https://opg.optica.org/josab/abstract.cfm?URI=josab-39-7-1775},
	doi = {10.1364/JOSAB.455841},
}

@article{qiwenzhan:OptCommun:2020,
	title = {Generation of three-dimensionally homogenized focal spot with uniform intensity distribution using vectorial optical fields},
	journal = {Opt. Commun.},
	volume = {464},
	pages = {125530},
	year = {2020},
	issn = {0030-4018},
	doi = {10.1016/j.optcom.2020.125530},
	url = {https://www.sciencedirect.com/science/article/pii/S0030401820301589},
	author = {Elforjani Jera and Sichao Zhou and Qiwen Zhan},
	keywords = {Optical microscopy, Focal field shaping, Homogenized intensity, Polarization},
}

@article{forbes:NatPhotonics:2021,
	author    = {A. Forbes and M. de Oliveira and M. R. Dennis},
	journal   = {Nat. Photonics},
	title     = {Structured light},
	volume    = {15},
	pages     = {253-262},
	year      = {2021},
    doi       = {10.1038/s41566-021-00780-4},
}

@article{maluenda:OptExpress:2014,
	author = {David Maluenda and Rosario Mart\'{i}nez-Herrero and Ignasi Juvells and Artur Carnicer},
	journal = {Opt. Express},
	keywords = {Computer holography; Polarization; Spatial light modulators; Circular polarization; Computer generated holograms; High numerical aperture optics; Numerical simulation; Spatial light modulators; Vector beams},
	number = {6},
	pages = {6859--6867},
	publisher = {Optica Publishing Group},
	title = {Synthesis of highly focused fields with circular polarization at any transverse plane},
	volume = {22},
	month = {Mar},
	year = {2014},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-22-6-6859},
	doi = {10.1364/OE.22.006859},
}

@article{brakenhoff:JMicrosc:1979,
	author = {Brakenhoff, G. J. and Blom, P. and Barends, P.},
	title = {Confocal scanning light microscopy with high aperture immersion lenses},
	journal = {J. Microsc.},
	volume = {117},
	number = {2},
	pages = {219-232},
	doi = {10.1111/j.1365-2818.1979.tb01178.x},
	url = {https://onlinelibrary.wiley.com/doi/abs/10.1111/j.1365-2818.1979.tb01178.x},
	eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1111/j.1365-2818.1979.tb01178.x},
    year = {1979}
}

@article{biss:OptLett:2003,
	author = {D. P. Biss and T. G. Brown},
	journal = {Opt. Lett.},
	keywords = {Nonlinear optics at surfaces; Nonlinear optics at surfaces; Polarization; Azimuthally polarized beams; Optical vortices; Polarized light; Thin films; Ti:sapphire lasers; Vector beams},
	number = {11},
	pages = {923--925},
	publisher = {Optica Publishing Group},
	title = {Polarization-vortex-driven second-harmonic generation},
	volume = {28},
	month = {Jun},
	year = {2003},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-28-11-923},
	doi = {10.1364/OL.28.000923},
}

@article{opron:OptLett:2003,
	author = {Dan Oron and Eran Tal and Yaron Silberberg},
	journal = {Opt. Lett.},
	keywords = {Three-dimensional image acquisition; Scanning microscopy; Multiharmonic generation; Ultrafast nonlinear optics; Circular polarization; Femtosecond lasers; Fluorescence microscopy; Multiphoton microscopy; Phase matching; Refractive index},
	number = {23},
	pages = {2315--2317},
	publisher = {Optica Publishing Group},
	title = {Depth-resolved multiphoton polarization microscopy by third-harmonic generation},
	volume = {28},
	month = {Dec},
	year = {2003},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-28-23-2315},
	doi = {10.1364/OL.28.002315},
}

@article{sheppard:ApplOpt:2004,
	author = {Colin J. R. Sheppard and Amarjyoti Choudhury},
	journal = {Appl. Opt.},
	keywords = {Diffraction theory; Microscopy; Optical recording; Confocal microscopy; Diffractive optical elements; High numerical aperture optics; Optical lithography; Optical systems; Point spread function},
	number = {22},
	pages = {4322--4327},
	publisher = {Optica Publishing Group},
	title = {Annular pupils, radial polarization, and superresolution},
	volume = {43},
	month = {Aug},
	year = {2004},
	url = {https://opg.optica.org/ao/abstract.cfm?URI=ao-43-22-4322},
	doi = {10.1364/AO.43.004322}
}

@inproceedings{serrels:ConfLasers:2008,
	author = {K. A. Serrels and E. Ramsay and R. J. Warburton and D.T. Reid},
	booktitle = {Conference on Lasers and Electro-Optics/Quantum Electronics and Laser Science Conference and Photonic Applications Systems Technologies},
	journal = {Conference on Lasers and Electro-Optics/Quantum Electronics and Laser Science Conference and Photonic Applications Systems Technologies},
	keywords = {Microscopy; Other areas of optics; Resolution; Nonlinear microscopy; Beam structure; Femtosecond lasers; High numerical aperture optics; Imaging systems; Point spread function; Refractive index},
	pages = {QThD3},
	publisher = {Optica Publishing Group},
	title = {Nanoscale Optical Microscopy in the Vectorial Focusing Regime},
	year = {2008},
	url = {https://opg.optica.org/abstract.cfm?URI=QELS-2008-QThD3}
}

@article{gorodetski:PRL:2008,
	title = {Observation of the Spin-Based Plasmonic Effect in Nanoscale Structures},
	author = {Gorodetski, Y. and Niv, A. and Kleiner, V. and Hasman, E.},
	journal = {Phys. Rev. Lett.},
	volume = {101},
	issue = {4},
	pages = {043903},
	numpages = {4},
	year = {2008},
	month = {Jul},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.101.043903},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.101.043903}
}

@article{masihzadeh:OptLett:2009,
	author = {Omid Masihzadeh and Philip Schlup and Randy A. Bartels},
	journal = {Opt. Lett.},
	keywords = {Phase retrieval; Scanning microscopy; Spatial light modulators; Polarization; Ultrafast nonlinear optics; Nonlinear microscopy; Analog to digital converters; Circular polarization; Nonlinear microscopy; Raman scattering; Spatial frequency; Spatial resolution},
	number = {8},
	pages = {1240--1242},
	publisher = {Optica Publishing Group},
	title = {Enhanced spatial resolution in third-harmonic microscopy through polarization switching},
	volume = {34},
	month = {Apr},
	year = {2009},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-34-8-1240},
	doi = {10.1364/OL.34.001240}
}

@article{vuong:PRL:2010,
	title = {Electromagnetic Spin-Orbit Interactions via Scattering of Subwavelength Apertures},
	author = {Vuong, L. T. and Adam, A. J. L. and Brok, J. M. and Planken, P. C. M. and Urbach, H. P.},
	journal = {Phys. Rev. Lett.},
	volume = {104},
	issue = {8},
	pages = {083903},
	numpages = {4},
	year = {2010},
	month = {Feb},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.104.083903},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.104.083903}
}

@article{qiwenzhan:OptLett:2006,
	author = {Qiwen Zhan},
	journal = {Opt. Lett.},
	keywords = {Diffraction theory; Polarization; Circular polarization; Cylindrical vector beams; Laser beams; Light beams; Optical angular momentum; Vortex beams},
	number = {7},
	pages = {867--869},
	publisher = {Optica Publishing Group},
	title = {Properties of circularly polarized vortex beams},
	volume = {31},
	month = {Apr},
	year = {2006},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-31-7-867},
	doi = {10.1364/OL.31.000867}
}

@article{maurer:NewJPhys:2007,
	doi = {10.1088/1367-2630/9/3/078},
	url = {https://doi.org/10.1088/1367-2630/9/3/078},
	year = 2007,
	month = {mar},
	publisher = {{IOP} Publishing},
	volume = {9},
	number = {3},
	pages = {78--78},
	author = {Christian Maurer and Alexander Jesacher and Severin Fürhapter and Stefan Bernet and Monika Ritsch-Marte},
	title = {Tailoring of arbitrary optical vector beams},
	journal = {New J. Phys.},
}

@article{wang:OptExpr:2010,
	author = {Xi-Lin Wang and Yongnan Li and Jing Chen and Cheng-Shan Guo and Jianping Ding and Hui-Tian Wang},
	journal = {Opt. Express},
	keywords = {Interferometry; Polarization; Spatial light modulators; Light matter interactions; Near field optics; Nonlinear optics; Optical elements; Optical systems; Polarization},
	number = {10},
	pages = {10786--10795},
	publisher = {Optica Publishing Group},
	title = {A new type of vector fields with hybrid states of polarization},
	volume = {18},
	month = {May},
	year = {2010},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-18-10-10786},
	doi = {10.1364/OE.18.010786}
}

@article{wang:OptLett:2007,
	author = {Xi-Lin Wang and Jianping Ding and Wei-Jiang Ni and Cheng-Shan Guo and Hui-Tian Wang},
	journal = {Opt. Lett.},
	keywords = {Diffractive optics; Spatial filtering; Diffraction gratings; Polarization; Laser beams; Light beams; Liquid crystal modulators; Spatial frequency; Spatial light modulators; Vector beams},
	number = {24},
	pages = {3549--3551},
	publisher = {Optica Publishing Group},
	title = {Generation of arbitrary vector beams with a spatial light modulator and a common path interferometric arrangement},
	volume = {32},
	month = {Dec},
	year = {2007},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-32-24-3549},
	doi = {10.1364/OL.32.003549}
}

@article{moreno:OptExpr:2011,
	author = {Ignacio Moreno and Claudio Iemmi and Juan Campos and Maria J. Yzuel},
	journal = {Opt. Express},
	keywords = {Spatial light modulators; Polarization; Frequency filtering ; Azimuthally polarized beams; Computer generated holograms; Diffractive optical elements; Fourier optics; Liquid crystal modulators; Matrix methods},
	number = {5},
	pages = {4583--4594},
	publisher = {Optica Publishing Group},
	title = {Jones matrix treatment for optical Fourier processors with structured polarization},
	volume = {19},
	month = {Feb},
	year = {2011},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-19-5-4583},
	doi = {10.1364/OE.19.004583}
}

@article{maluenda:OptExpr:2013,
	author = {David Maluenda and Ignasi Juvells and Rosario Mart\'{i}nez-Herrero and Artur Carnicer},
	journal = {Opt. Express},
	keywords = {Computer holography; Polarization; Spatial light modulators; Computer generated holograms; Light beams; Light matter interactions; Liquid crystal displays; Optical communications; Optical systems},
	number = {5},
	pages = {5432--5439},
	publisher = {Optica Publishing Group},
	title = {Reconfigurable beams with arbitrary polarization and shape distributions at a given plane},
	volume = {21},
	month = {Mar},
	year = {2013},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-21-5-5432},
	doi = {10.1364/OE.21.005432}
}

@article{waller:OptExpr:2013,
	author = {Erik H. Waller and Georg von Freymann},
	journal = {Opt. Express},
	keywords = {Diffractive optics; Spatial light modulators; Active or adaptive optics; Grating prisms; Light matter interactions; Optical trapping; Polarized light; Spatial frequency; Vector beams},
	number = {23},
	pages = {28167--28174},
	publisher = {Optica Publishing Group},
	title = {Independent spatial intensity, phase and polarization distributions},
	volume = {21},
	month = {Nov},
	year = {2013},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-21-23-28167},
	doi = {10.1364/OE.21.028167}
}

@article{han:OptExpr:2013,
	author = {Wei Han and Yanfang Yang and Wen Cheng and Qiwen Zhan},
	journal = {Opt. Express},
	keywords = {Phase modulation; Computer holography; Polarization; Spatial light modulators; Azimuthally polarized beams; Diffractive optical elements; Liquid crystal devices; Liquid crystal modulators; Optical fields; Polarization control},
	number = {18},
	pages = {20692--20706},
	publisher = {Optica Publishing Group},
	title = {Vectorial optical field generator for the creation of arbitrarily complex fields},
	volume = {21},
	month = {Sep},
	year = {2013},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-21-18-20692},
	doi = {10.1364/OE.21.020692}
}

@article{chengshanguo:OptLett:2014,
	author = {Cheng-Shan Guo and Zhen-Yu Rong and Shu-Zhen Wang},
	journal = {Opt. Lett.},
	keywords = {Computer holography; Phase modulation; Spatial light modulators; Polarization; Beam structure; Gaussian beams; Laser beams; Optical elements; Spatial light modulators; Vector beams},
	number = {2},
	pages = {386--389},
	publisher = {Optica Publishing Group},
	title = {Double-channel vector spatial light modulator for generation of arbitrary complex vector beams},
	volume = {39},
	month = {Jan},
	year = {2014},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-39-2-386},
	doi = {10.1364/OL.39.000386}
}

@article{zhenyurong:OptExpr:2014,
	author = {Zhen-Yu Rong and Yu-Jing Han and Shu-Zhen Wang and Cheng-Shan Guo},
	journal = {Opt. Express},
	keywords = {Computer holography; Interferometry; Liquid-crystal devices; Polarization; Spatial light modulators; Cylindrical vector beams; Diffractive optical elements; Light beams; Liquid crystal modulators; Spatial light modulators; Vector beams},
	number = {2},
	pages = {1636--1644},
	publisher = {Optica Publishing Group},
	title = {Generation of arbitrary vector beams with cascaded liquid crystal spatial light modulators},
	volume = {22},
	month = {Jan},
	year = {2014},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-22-2-1636},
	doi = {10.1364/OE.22.001636}
}

@article{novotny:PRL:2001,
	title = {Longitudinal Field Modes Probed by Single Molecules},
	author = {Novotny, L. and Beversluis, M. R. and Youngworth, K. S. and Brown, T. G.},
	journal = {Phys. Rev. Lett.},
	volume = {86},
	issue = {23},
	pages = {5251--5254},
	numpages = {0},
	year = {2001},
	month = {Jun},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.86.5251},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.86.5251}
}

@article{novotny:ApplPhysLett:2003,
	author = {A. Bouhelier M. R. and Beversluis L. Novotny},
	title = {Near-field scattering of longitudinal fields},
	journal = {Applied Physics Letters},
	volume = {82},
	number = {25},
	pages = {4596-4598},
	year = {2003},
	doi = {10.1063/1.1586482},
	URL = {https://doi.org/10.1063/1.1586482},
	eprint = {https://doi.org/10.1063/1.1586482}
}

@article{kitamura:OptExpr:2010,
	author    = {K. Kitamura and K. Sakai K. and S. Noda},
	journal   = {Opt. Express},
	title     = {Sub-wavelength focal spot with long depth of focus generated by radially polarized, narrow- width annular beam},
	volume    = {18},
	pages     = {4518–4525},
	year      = {2010},
	doi       = {https://doi.org/10.1364/oe.18.004518}
}

@article{jia:ApplPhysLett:2005,
	author = {B. Jia and X. Gan and M. Gu},
	title = {Direct observation of a pure focused evanescent field of a high numerical aperture objective lens by scanning near-field optical microscopy},
	journal = {Appl. Phys. Lett.},
	volume = {86},
	number = {13},
	pages = {131110},
	year = {2005},
	doi = {10.1063/1.1886250},
	URL = {https://doi.org/10.1063/1.1886250},
	eprint = {https://doi.org/10.1063/1.1886250}
}

@article{wang:FrontOptoelectron:2012,
	author = {J. Wang and Q. Wang and M. Zhang},
	title = {Development and prospect of near-field optical measurements and characterizations},
	publisher = {Front. Optoelectron.},
	year = {2012},
	journal = {Front. Optoelectron.},
	volume = {5},
	number = {2},
	pages = {171-181},
	url = {https://journal.hep.com.cn/foe/EN/abstract/article_3890.shtml},
	doi = {10.1007/s12200-012-0257-y}
}    

@article{khonina:JOpt:2013,
	doi = {10.1088/2040-8978/15/8/085704},
	url = {https://doi.org/10.1088/2040-8978/15/8/085704},
	year = {2013},
	month = {jul},
	publisher = {{IOP} Publishing},
	volume = {15},
	number = {8},
	pages = {085704},
	author = {Svetlana N Khonina and Sergey V Karpeev and Sergey V Alferov and Dmitry A Savelyev and Janne Laukkanen and Jari Turunen},
	title = {Experimental demonstration of the generation of the longitudinal E-field component on the optical axis with high-numerical-aperture binary axicons illuminated by linearly and circularly polarized beams},
	journal = {J. Opt.},
}

@article{khonina:JOSAA:2014,
	author = {S. V. Alferov and S. N. Khonina and S. V. Karpeev},
	journal = {J. Opt. Soc. Am. A},
	keywords = {Near-field microscopy; Optical vortices ; Electric fields; Electromagnetic radiation; Near field microscopy; Phase plates; Phase shift; Zone plates},
	number = {4},
	pages = {802--807},
	publisher = {Optica Publishing Group},
	title = {Study of polarization properties of fiber-optics probes with use of a binary phase plate},
	volume = {31},
	month = {Apr},
	year = {2014},
	url = {https://opg.optica.org/josaa/abstract.cfm?URI=josaa-31-4-802},
	doi = {10.1364/JOSAA.31.000802}
}

@article{khonina:ApplOpt:2013,
	author = {Victor V. Kotlyar and Sergey S. Stafeev and Yikun Liu and Liam O'Faolain and Alexey A. Kovalev},
	journal = {Appl. Opt.},
	keywords = {Binary optics; Near-field microscopy; Gaussian beams; Laser beams; Light fields; Near field scanning optical microscopy; Optical elements; Zone plates},
	number = {3},
	pages = {330--339},
	publisher = {Optica Publishing Group},
	title = {Analysis of the shape of a subwavelength focal spot for the linearly polarized light},
	volume = {52},
	month = {Jan},
	year = {2013},
	url = {https://opg.optica.org/ao/abstract.cfm?URI=ao-52-3-330},
	doi = {10.1364/AO.52.000330}
}

@article{qiwenzhan:OptLett:2009,
	author = {Weibin Chen and Qiwen Zhan},
	journal = {Opt. Lett.},
	keywords = {Diffraction theory; Scanning microscopy; Surface plasmons; Polarization; Diffraction limit; Interference; Near field scanning optical microscopy; Resonance; Surface plasmons; Surface waves},
	number = {6},
	pages = {722--724},
	publisher = {Optica Publishing Group},
	title = {Realization of an evanescent Bessel beam via surface plasmon interference excited by a radially polarized beam},
	volume = {34},
	month = {Mar},
	year = {2009},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-34-6-722},
	doi = {10.1364/OL.34.000722}
}

@article{khonina:OptLett:2013,
	author = {S. N. Khonina and S. V. Alferov and S. V. Karpeev},
	journal = {Opt. Lett.},
	keywords = {Diffraction; Polarization; Near-field microscopy; Circular polarization; Electric fields; Laser beams; Near field microscopy; Numerical simulation; Vortex beams},
	number = {17},
	pages = {3223--3226},
	publisher = {Optica Publishing Group},
	title = {Strengthening the longitudinal component of the sharply focused electric field by means of higher-order laser beams},
	volume = {38},
	month = {Sep},
	year = {2013},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-38-17-3223},
	doi = {10.1364/OL.38.003223}
}

@article{carnicer:EJP:2012,
	doi = {10.1088/0143-0807/33/5/1235},
	url = {https://doi.org/10.1088/0143-0807/33/5/1235},
	year = 2012,
	month = {jul},
	publisher = {{IOP} Publishing},
	volume = {33},
	number = {5},
	pages = {1235--1247},
	author = {Artur Carnicer and Ignasi Juvells and David Maluenda and Rosario Mart{\'{\i}}nez-Herrero and Pedro M Mej{\'{\i}}as},
	title = {On the longitudinal component of paraxial fields},
	journal = {Eur. J. Phys.}
}

@article{maucher:PRL:2018,
  title = {Creating complex optical longitudinal polarization structures},
  author = {Maucher, F. and Skupin, S. and Gardiner, S. A. and Hughes, I. G.},
  journal = {Phys. Rev. Lett.},
  volume = {120},
  issue = {16},
  pages = {163903},
  numpages = {5},
  year = {2018},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.120.163903},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.120.163903}
}

@article{khonina:OptLett:2020,
author = {Svetlana N. Khonina and Andrey V. Ustinov and Alexey P. Porfirev},
journal = {Opt. Lett.},
keywords = {Azimuthally polarized beams; Cylindrical vector beams; Laser beams; Numerical analysis; Optical tweezers; Vector beams},
number = {15},
pages = {4112--4115},
publisher = {Optica Publishing Group},
title = {Vector Lissajous laser beams},
volume = {45},
month = {Aug},
year = {2020},
url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-45-15-4112},
doi = {10.1364/OL.398209}
}

@article{manjavacas:ACSOmega:2022,
 author    = {L. Zundel and J. R. Deop-Ruano and R. Mart{\'\i}nez-Herrero and A. Manjavacas},
 journal   = {ACS Omega},
 title     = {Lattice resonances excited by finite-width light beams},
 volume    = {7},
 issue     = {35},
 pages     = {31431-31441},
 year      = {2022},
 doi       = {https://doi.org/10.1021/acsomega.2c03847}
}

@BOOK{gellmann-bk:1964,
   title =     {The eightfold way},
   author =    {Gell-Mann M. and Ne'eman Y.},
   publisher = {W. A. Benjamin},
   address   = {New York},
   year =      {1964},
   series =    {Frontiers in Physics Series: Lecture Note & Reprint Series},
   url =       {libgen.li/file.php?md5=819f1fb387c7f4564304d7114fe1f888},
}

@article{GellMann:PhysRev:1962,
  title = {Symmetries of Baryons and Mesons},
  author = {Gell-Mann, Murray},
  journal = {Phys. Rev.},
  volume = {125},
  issue = {3},
  pages = {1067--1084},
  numpages = {0},
  year = {1962},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.125.1067},
  url = {https://link.aps.org/doi/10.1103/PhysRev.125.1067},
}

@article{friberg:PRE:2002,
  title = {Degree of polarization for optical near fields},
  author = {Set\"al\"a, T. and Shevchenko, A. and Kaivola, M. and Friberg, A. T.},
  journal = {Phys. Rev. E},
  volume = {66},
  issue = {1},
  pages = {016615},
  numpages = {7},
  year = {2002},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.66.016615},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.66.016615}
}

@article{sheppard:PRA:2014,
  title = {Jones and Stokes parameters for polarization in three dimensions},
  author = {Sheppard, Colin J. R.},
  journal = {Phys. Rev. A},
  volume = {90},
  issue = {2},
  pages = {023809},
  numpages = {5},
  year = {2014},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.90.023809},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.90.023809}
}

@article{maluenda:SciRep:2021,
 author    = {D. Maluenda and M. Avi{\~n}o\'a and K. Ahmadi and R. Mart{\'\i}nez-Herrero and A. Carnicer},
 journal   = {Sci. Rep.},
 title     = {Experimental estimation of the longitudinal component of a highly focused electromagnetic field},
 volume    = {11},
 pages     = {17992},
 year      = {2021},
 doi       = {https://doi.org/10.1038/s41598-021-97164-z}
}

@article{MartinezHerrero:OptExpr:2020,
author = {R. Mart\'{i}nez-Herrero and A. Carnicer and I. Juvells and A. S. Sanz},
journal = {Opt. Express},
keywords = {Adaptive optics; Diffractive optics; High numerical aperture optics; Holographic memory; Optical fields; Optical systems},
number = {20},
pages = {29676--29690},
publisher = {Optica Publishing Group},
title = {Uncertainty principle for axial power content of highly focused fields},
volume = {28},
month = {Sep},
year = {2020},
url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-28-20-29676},
doi = {10.1364/OE.401073}
}

@misc{localStokesPipeline,
  howpublished = {\url{https://colab.research.google.com/github/WavefrontEngUB/stokes3D/blob/master/Report.ipynb}}
}

@article{arrizon:OptLetters:2003,
  title={Complex modulation with a twisted-nematic liquid-crystal spatial light modulator: double-pixel approach},
  author={Arriz{\'o}n, Victor},
  journal={Opt. Lett.},
  volume={28},
  number={15},
  pages={1359--1361},
  year={2003},
  publisher={Optica Publishing Group},
  doi = {10.1364/OL.28.001359},
  url = {https://doi.org/10.1364/OL.28.001359},
}

@article{nieto-vesperinas:LSA:2022,
 author    = {Nieto-Vesperinas, Manuel and Xu, Xiaohao},
 journal   = {Light Sci. Appl.},
 title     = {The complex Maxwell stress tensor theorem: The imaginary stress tensor and the reactive strength of orbital momentum. A novel scenery underlying electromagnetic optical forces},
 volume    = {11},
 pages     = {297},
 year      = {2022},
 doi       = {10.1038/s41377-022-00979-2},
 url       = {https://doi.org/10.1038/s41377-022-00979-2},
}

@article{leuchs:PRL:2003,
	title = {Sharper Focus for a Radially Polarized Light Beam},
	author = {Dorn, R. and Quabis, S. and Leuchs, G.},
	journal = {Phys. Rev. Lett.},
	volume = {91},
	issue = {23},
	pages = {233901},
	numpages = {4},
	year = {2003},
	month = {Dec},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.91.233901},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.91.233901}
}

@article{bouhelier2003near,
  title={Near-field scattering of longitudinal fields},
  author={Bouhelier, Alexandre and Beversluis, Michael R and Novotny, Lukas},
  journal={Appl. Phys. Lett.},
  volume={82},
  number={25},
  pages={4596--4598},
  year={2003},
  publisher={American Institute of Physics},
  doi = {10.1063/1.1586482},
  url = {https://doi.org/10.1063/1.1586482},  
}

@article{hao2007experimental,
  title={Experimental measurement of longitudinal component in the vicinity of focused radially polarized beam},
  author={Hao, Bing and Leger, James},
  journal={Opt. Express},
  volume={15},
  number={6},
  pages={3550--3556},
  year={2007},
  publisher={Optical Society of America},
  doi = {10.1364/OE.15.003550},
  url = {https://doi.org/10.1364/OE.15.003550},
}

@article{fienup:OptLet:1978,
  title={Reconstruction of an object from the modulus of its Fourier transform},
  author={Fienup, James R},
  journal={Opt. Lett.},
  volume={3},
  number={1},
  pages={27--29},
  year={1978},
  publisher={Optica Publishing Group},
  doi = {10.1364/OL.3.000027},
  url = {https://doi.org/10.1364/OL.3.000027},
}

@article{sanz:AnnFondLdB:2021,
 author    = {A. S. Sanz},
 journal   = {Ann. Fond. Louis de Broglie},
 title     = {Bohm's quantum ``non-mechanics'': An alternative quantum theoryw with its own ontology?},
 volume    = {46},
 pages     = {19-63},
 year      = {2021},
 url       = {https://fondationlouisdebroglie.org/AFLB-461/aflb461m955.htm}
}

@article{sanz:JOSAA:2022,
author = {A. S. Sanz},
journal = {J. Opt. Soc. Am. A},
keywords = {Airy beams; Light beams; Light diffraction; Phase shift; Photons; Structured light},
number = {12},
pages = {C79--C85},
publisher = {Optica Publishing Group},
title = {Flux trajectory analysis of {Airy} -type beams},
volume = {39},
month = {Dec},
year = {2022},
url = {https://opg.optica.org/josaa/abstract.cfm?URI=josaa-39-12-C79},
doi = {10.1364/JOSAA.472653}
}

@article{pati:Pramana:2001,
 author    = {A. K. Pati and M. Zukowski},
 journal   = {Pramana - J. Phys.},
 title     = {Interference due to coherence swapping},
 volume    = {56},
 pages     = {393--401},
 year      = {2001},
 doi       = {10.1007/s12043-001-0133-6},
 url       = {https://doi.org/10.1007/s12043-001-0133-6}
}

@article{sanz:ENTROPY:2022,
AUTHOR = {Sanz, A. S.},
TITLE = {Quantum-classical entropy analysis for nonlinearly-coupled continuous-variable bipartite systems},
JOURNAL = {Entropy},
VOLUME = {24},
YEAR = {2022},
NUMBER = {2},
ARTICLE-NUMBER = {190},
URL = {https://www.mdpi.com/1099-4300/24/2/190},
ISSN = {1099-4300},
DOI = {10.3390/e24020190}
}

@article{sanz:PRResearch:2023,
 author    = {A. S. Sanz and A. Aiello and L. L. S\'anchez-Soto},
 journal   = {Phys. Rev. Research},
 title     = {A quantum trajectory analysis of singular wave functions},
 volume    = {},
 pages     = {},
 year      = {to be published, 2023},
 doi       = {},
 url       = {},
}

@misc{sanz2023quantum,
      title={A quantum trajectory analysis of singular wave functions}, 
      author={A. S. Sanz and L. L. Sanchez-Soto and A. Aiello},
      year={2023},
      eprint={arXiv:2301.13207 (pre-print)},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@article{sanz:PRA:2022,
  title = {Partially coherent {Airy}  beams: A cross-spectral-density approach},
  author = {Mart\'{\i}nez-Herrero, R. and Sanz, A. S.},
  journal = {Phys. Rev. A},
  volume = {106},
  issue = {5},
  pages = {053512},
  numpages = {12},
  year = {2022},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.106.053512},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.106.053512}
}

@ARTICLE{wang:FrontPhys:2021,
AUTHOR={Wang, Jian and Liang, Yize},   
TITLE={Generation and Detection of Structured Light: A Review},      
JOURNAL={Front. Phys.},      
VOLUME={9},
pages={688284},          
YEAR={2021},      
URL={https://www.frontiersin.org/articles/10.3389/fphy.2021.688284},       
DOI={10.3389/fphy.2021.688284},
}

@article{tzemos:PRE:2021,
	title = {Ergodicity and Born's rule in an entangled three-qubit Bohmian system},
	author = {Tzemos, Athanasios C. and Contopoulos, George},
	journal = {Phys. Rev. E},
	volume = {104},
	issue = {5},
	pages = {054211},
	numpages = {14},
	year = {2021},
	month = {Nov},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevE.104.054211},
	url = {https://link.aps.org/doi/10.1103/PhysRevE.104.054211}
}

@article{tzemos:PRE:2020,
	title = {Ergodicity and Born's rule in an entangled two-qubit Bohmian system},
	author = {Tzemos, Athanasios C. and Contopoulos, George},
	journal = {Phys. Rev. E},
	volume = {102},
	issue = {4},
	pages = {042205},
	numpages = {13},
	year = {2020},
	month = {Oct},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevE.102.042205},
	url = {https://link.aps.org/doi/10.1103/PhysRevE.102.042205}
}

@article{tzemos:PhysScr:2021,
	doi = {10.1088/1402-4896/abf18a},
	url = {https://dx.doi.org/10.1088/1402-4896/abf18a},
	year = {2021},
	month = {apr},
	publisher = {IOP Publishing},
	volume = {96},
	number = {6},
	pages = {065209},
	author = {A C Tzemos and G Contopoulos},
	title = {The role of chaotic and ordered trajectories in establishing Born’s rule},
	journal = {Physica Scripta},
}

@Article{plastino:Entropy:2018,
	AUTHOR = {Zander, Claudia and Plastino, Angel Ricardo},
	TITLE = {Revisiting Entanglement within the Bohmian Approach to Quantum Mechanics},
	JOURNAL = {Entropy},
	VOLUME = {20},
	YEAR = {2018},
	NUMBER = {6},
	ARTICLE-NUMBER = {473},
	URL = {https://www.mdpi.com/1099-4300/20/6/473},
	PubMedID = {33265563},
	ISSN = {1099-4300},
	DOI = {10.3390/e20060473}
}

@article{sanz:PhysScr:2022,
	doi = {10.1088/1402-4896/ac6460},
	url = {https://dx.doi.org/10.1088/1402-4896/ac6460},
	year = {2022},
	month = {apr},
	publisher = {IOP Publishing},
	volume = {97},
	number = {5},
	pages = {055507},
	author = {A. Garc{\'\i}a-S\'anchez and A. S Sanz},
	title = {Analysis of the gradual transition from the near to the far field in single-slit diffraction},
	journal = {Phys. Scr.},
}

@article{Efremidis:Optica:2019,
	author = {Nikolaos K. Efremidis and Zhigang Chen and Mordechai Segev and Demetrios N. Christodoulides},
	journal = {Optica},
	keywords = {Airy beams; Medical imaging; Near field scanning optical microscopy; Nonlinear wave mixing; Optical force; Spatial light modulators},
	number = {5},
	pages = {686--701},
	publisher = {Optica Publishing Group},
	title = {Airy beams and accelerating waves: an overview of recent advances},
	volume = {6},
	month = {May},
	year = {2019},
	url = {https://opg.optica.org/optica/abstract.cfm?URI=optica-6-5-686},
	doi = {10.1364/OPTICA.6.000686}
}

@article{Xu:OE:2022,
	author = {Danlin Xu and Yujun Liu and Zhenwu Mo and Junjie Jiang and Jingyi Shi and Zehong Liang and You Wu and Jiajia Zhao and Haobin Yang and Haiqi Huang and Hongzhan Liu and Lingling Shui and Dongmei Deng},
	journal = {Opt. Express},
	keywords = {Airy beams; Laser spectroscopy; Optical fields; Optical tweezers; Surface plasmon polaritons; Surface waves},
	number = {1},
	pages = {232--242},
	publisher = {Optica Publishing Group},
	title = {Shaping autofocusing {Airy}  beams through the modification of Fourier spectrum},
	volume = {30},
	month = {Jan},
	year = {2022},
	url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-30-1-232},
	doi = {10.1364/OE.444396}
}

@Article{Zhang:ApplSci:2017,
	AUTHOR = {Zhang, Yiqi and Zhong, Hua and Beli\'c, Milivoj R. and Zhang, Yanpeng},
	TITLE = {Guided Self-Accelerating {Airy}  Beam--A Mini-Review},
	JOURNAL = {Appl. Sci.},
	VOLUME = {7},
	YEAR = {2017},
	NUMBER = {4},
	ARTICLE-NUMBER = {341},
	URL = {https://www.mdpi.com/2076-3417/7/4/341},
	ISSN = {2076-3417},
	DOI = {10.3390/app7040341}
}

@BOOK{margenau-moseley-bk,
  AUTHOR     = {H. Margenau and G. Moseley Murphy},
  TITLE      = {The Mathematics of Physics and Chemistry},
  PUBLISHER  = {D. Van Nostrand},
  YEAR       = {1943},
  address    = {Princeton, NJ},
}

@Article{Schleich:PNAS:2013,
	AUTHOR = {Wolfgang P. Schleich and Daniel M. Greenberger and Donald H. Kobe and Marlan O. Scully},
	TITLE = {Schr\"odinger equation revisited},
	JOURNAL = {Proc. Nat. Acad. Sci.},
	VOLUME = {110},
	YEAR = {2013},
	NUMBER = {14},
	ARTICLE-NUMBER = {5374-5379},
	URL = {https://doi.org/10.1073/pnas.130247511},
	DOI = {10.1073/pnas.1302475110}
}

@article{fink:AJP:2022,
    author = {Catheline, Stefan and Delattre, Victor and Laloy-Borgna, Gabrielle and Faure, Fréderic and Fink, Mathias},
    title = "{Gravitational lens effect revisited through membrane waves}",
    journal = {Am. J. Phys.},
    volume = {90},
    number = {1},
    pages = {47-50},
    year = {2022},
    month = {01},
    issn = {0002-9505},
    doi = {10.1119/10.0006612},
    url = {https://doi.org/10.1119/10.0006612},
    eprint = {https://pubs.aip.org/aapt/ajp/article-pdf/90/1/47/16184728/47\_1\_online.pdf},
}

@article{ohanian:AJP:1987,
    author = {Ohanian, Hans C.},
    title = "{The black hole as a gravitational ``lens''}",
    journal = {Am. J. Phys.},
    volume = {55},
    number = {5},
    pages = {428-432},
    year = {1987},
    month = {05},
    issn = {0002-9505},
    doi = {10.1119/1.15126},
    url = {https://doi.org/10.1119/1.15126},
    eprint = {https://pubs.aip.org/aapt/ajp/article-pdf/55/5/428/11852596/428\_1\_online.pdf},
}

@article{selmke:AJP:2021,
    author = {Selmke, Markus},
    title = "{An optical N-body gravitational lens analogy}",
    journal = {Am. J. Phys.},
    volume = {89},
    number = {1},
    pages = {11-20},
    year = {2021},
    month = {01},
    issn = {0002-9505},
    doi = {10.1119/10.0002117},
    url = {https://doi.org/10.1119/10.0002117},
    eprint = {https://pubs.aip.org/aapt/ajp/article-pdf/89/1/11/12936275/11\_1\_online.pdf},
}

@article{liebes:AJP:1969,
    author = {Liebes, Sidney, Jr.},
    title = "{Gravitational Lens Simulator}",
    journal = {Am. J. Phys.},
    volume = {37},
    number = {1},
    pages = {103-104},
    year = {1969},
    month = {01},
    issn = {0002-9505},
    doi = {10.1119/1.1975345},
    url = {https://doi.org/10.1119/1.1975345},
    eprint = {https://pubs.aip.org/aapt/ajp/article-pdf/37/1/103/10113862/103\_1\_online.pdf},
}

@article{nandor:AJP:1996,
    author = {Nandor, M. J. and Helliwell, T. M.},
    title = "{Fermat's principle and multiple imaging by gravitational lenses}",
    journal = {Am. J. Phys.},
    volume = {64},
    number = {1},
    pages = {45-49},
    year = {1996},
    month = {01},
    issn = {0002-9505},
    doi = {10.1119/1.18291},
    url = {https://doi.org/10.1119/1.18291},
    eprint = {https://pubs.aip.org/aapt/ajp/article-pdf/64/1/45/11828268/45\_1\_online.pdf},
}

@article{turrell:AJP:2023,
    author = {George, Brett C. and Kontou, Eleni-Alexandra and Przewoznik, Patrycja and Turrell, Eleanor},
    title = "{An exploration of circumbinary systems using gravitational microlensing}",
    journal = {Am. J. Phys.},
    volume = {91},
    number = {3},
    pages = {182-192},
    year = {2023},
    month = {03},
    issn = {0002-9505},
    doi = {10.1119/5.0088604},
    url = {https://doi.org/10.1119/5.0088604},
    eprint = {https://pubs.aip.org/aapt/ajp/article-pdf/91/3/182/16736587/182\_1\_online.pdf},
}

@article{alfaro:AJP:2001,
    author = {Alfaro, Francisco Frutos},
    title = "{A computer program to visualize gravitational lenses}",
    journal = {Am. J. Phys.},
    volume = {69},
    number = {2},
    pages = {218-222},
    year = {2001},
    month = {02},
    issn = {0002-9505},
    doi = {10.1119/1.1290251},
    url = {https://doi.org/10.1119/1.1290251},
    eprint = {https://pubs.aip.org/aapt/ajp/article-pdf/69/2/218/7529764/218\_1\_online.pdf},
}

@article{icke:AJP:1980,
    author = {Icke, Vincent},
    title = "{Construction of a gravitational lens}",
    journal = {Am. J. Phys.},
    volume = {48},
    number = {10},
    pages = {883-886},
    year = {1980},
    month = {10},
    issn = {0002-9505},
    doi = {10.1119/1.12284},
    url = {https://doi.org/10.1119/1.12284},
    eprint = {https://pubs.aip.org/aapt/ajp/article-pdf/48/10/883/11397371/883\_1\_online.pdf},
}

@article{higbie:AJP:1981,
    author = {Higbie, J.},
    title = "{Gravitational lens}",
    journal = {Am. J. Phys.},
    volume = {49},
    number = {7},
    pages = {652-655},
    year = {1981},
    month = {07},
    issn = {0002-9505},
    doi = {10.1119/1.12440},
    url = {https://doi.org/10.1119/1.12440},
    eprint = {https://pubs.aip.org/aapt/ajp/article-pdf/49/7/652/12126808/652\_1\_online.pdf},
}

@article{drosdoff:AJP:2005,
    author = {Drosdoff, D. and Widom, A.},
    title = "{Snell's law from an elementary particle viewpoint}",
    journal = {Am. J. Phys.},
    volume = {73},
    number = {10},
    pages = {973-975},
    year = {2005},
    month = {10},
    issn = {0002-9505},
    doi = {10.1119/1.2000974},
    url = {https://doi.org/10.1119/1.2000974},
    eprint = {https://pubs.aip.org/aapt/ajp/article-pdf/73/10/973/12842782/973\_1\_online.pdf},
}

@article{ros:PhysEd:2008,
doi = {10.1088/0031-9120/43/5/007},
url = {https://dx.doi.org/10.1088/0031-9120/43/5/007},
year = {2008},
month = {sep},
publisher = {},
volume = {43},
number = {5},
pages = {506},
author = {Rosa M Ros},
title = {Gravitational lenses in the classroom},
journal = {Physics Education},
}

@Article{sanz:ENTROPY:2023,
AUTHOR = {A. S. Sanz},
TITLE = {Young's experiment with entangled bipartite systems: The role of underlying quantum velocity fields},
JOURNAL = {Entropy},
VOLUME = {25},
YEAR = {2023},
NUMBER = {7},
ARTICLE-NUMBER = {1077},
URL = {https://www.mdpi.com/1099-4300/25/7/1077},
PubMedID = {37510022},
ISSN = {1099-4300},
DOI = {10.3390/e25071077},
}

@article{plenio:RMP:2017,
	title = {Colloquium: Quantum coherence as a resource},
	author = {Streltsov, Alexander and Adesso, Gerardo and Plenio, Martin B.},
	journal = {Rev. Mod. Phys.},
	volume = {89},
	issue = {4},
	pages = {041003},
	numpages = {34},
	year = {2017},
	month = {Oct},
	publisher = {American Physical Society},
	doi = {10.1103/RevModPhys.89.041003},
	url = {https://link.aps.org/doi/10.1103/RevModPhys.89.041003}
}

@incollection{patorski:ProgOpt:1989,
	title = {I The self-imaging phenomenon and its applications},
	editor = {E. Wolf},
	series = {Progress in Optics},
	publisher = {Elsevier},
	volume = {27},
	pages = {1-108},
	year = {1989},
	issn = {0079-6638},
	doi = {https://doi.org/10.1016/S0079-6638(08)70084-2},
	url = {https://www.sciencedirect.com/science/article/pii/S0079663808700842},
	author = {Krzysztof Patorski},
}

@article{berry:JModOpt:1996,
	author = {M. V. Berry and S. Klein},
	title = {Integer, fractional and fractal {talbot} effects},
	journal = {J. Mod. Opt.},
	volume = {43},
	number = {10},
	pages = {2139--2164},
	year = {1996},
	publisher = {Taylor \& Francis},
	doi = {10.1080/09500349608232876},
	URL = {https://doi.org/10.1080/09500349608232876},
	eprint = {https://doi.org/10.1080/09500349608232876},
}

@article{winthrop:JOSA:1965,
	author = {John T. Winthrop and C. R. Worthington},
	journal = {J. Opt. Soc. Am.},
	number = {4},
	pages = {373--381},
	publisher = {Optica Publishing Group},
	title = {Theory of Fresnel Images. I. Plane Periodic Objects in Monochromatic Light$\ast$},
	volume = {55},
	month = {Apr},
	year = {1965},
	url = {https://opg.optica.org/abstract.cfm?URI=josa-55-4-373},
	doi = {10.1364/JOSA.55.000373},
}

@article{xiao:AdvOptPhoton:2013,
	author = {Jianming Wen and Yong Zhang and Min Xiao},
	journal = {Adv. Opt. Photon.},
	number = {1},
	pages = {83--130},
	publisher = {Optica Publishing Group},
	title = {The {talbot} effect: recent advances in classical optics, nonlinear optics, and quantum optics},
	volume = {5},
	month = {Mar},
	year = {2013},
	url = {https://opg.optica.org/aop/abstract.cfm?URI=aop-5-1-83},
	doi = {10.1364/AOP.5.000083},
}

@article{manjavacas:OL:2017,
	author = {L. Zundel and R. Mart\'{\i}nez-Herrero and A. Manjavacas},
	journal = {Opt. Lett.},
	number = {20},
	pages = {4143--4146},
	publisher = {Optica Publishing Group},
	title = {Flat top surface plasmon polariton beams},
	volume = {42},
	month = {Oct},
	year = {2017},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-42-20-4143},
	doi = {10.1364/OL.42.004143},
}

@article{manjavacas:PRA:2016,
	title = {Basis for paraxial surface-plasmon-polariton packets},
	author = {Martinez-Herrero, Rosario and Manjavacas, Alejandro},
	journal = {Phys. Rev. A},
	volume = {94},
	issue = {6},
	pages = {063829},
	numpages = {5},
	year = {2016},
	month = {Dec},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevA.94.063829},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.94.063829}
}

@article{christodoulides:OL:2010,
	author = {Alessandro Salandrino and Demetrios N. Christodoulides},
	journal = {Opt. Lett.},
	number = {12},
	pages = {2082--2084},
	publisher = {Optica Publishing Group},
	title = {Airy plasmon: a nondiffracting surface wave},
	volume = {35},
	month = {Jun},
	year = {2010},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-35-12-2082},
	doi = {10.1364/OL.35.002082},
}

@article{chen:OL:2023,
	author = {Yanru Chen and Zhifeng Tu and Hongcheng Hu and Junxi Zhang and Zien Feng and Ziyu Wang and Weiyi Hong and Dongmei Deng},
	journal = {Opt. Lett.},
	number = {8},
	pages = {2030--2033},
	publisher = {Optica Publishing Group},
	title = {Olver plasmon: an accelerating surface wave with various orders},
	volume = {48},
	month = {Apr},
	year = {2023},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-48-8-2030},
	doi = {10.1364/OL.487750},
}

@article{hu:ResPhys:2021,
	title = {Pearcey plasmon: An autofocusing surface wave},
	journal = {Res. Phys.},
	volume = {26},
	pages = {104416},
	year = {2021},
	issn = {2211-3797},
	doi = {https://doi.org/10.1016/j.rinp.2021.104416},
	url = {https://www.sciencedirect.com/science/article/pii/S2211379721005350},
	author = {Hongcheng Hu and Chuangjie Xu and Manshuo Lin and Dongmei Deng},
	keywords = {Pearcey plasmon, Autofocusing, Surface plasmon},
}

@article{minovich:PRL:2011,
	title = {Generation and Near-Field Imaging of {Airy}  Surface Plasmons},
	author = {Minovich, Alexander and Klein, Angela E. and Janunts, Norik and Pertsch, Thomas and Neshev, Dragomir N. and Kivshar, Yuri S.},
	journal = {Phys. Rev. Lett.},
	volume = {107},
	issue = {11},
	pages = {116802},
	numpages = {4},
	year = {2011},
	month = {Sep},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.107.116802},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.107.116802}
}


@article{,
 author    = {},
 journal   = {},
 title     = {},
 volume    = {},
 pages     = {},
 year      = {},
 doi       = {},
 url       = {},
}

@BOOK{,
  AUTHOR     = {},
  TITLE      = {},
  PUBLISHER  = {},
  YEAR       = {},
  address    = {},
}


@article{zhang2021plasmonic,
  title={Plasmonic tweezers: for nanoscale optical trapping and beyond},
  author={Zhang, Yuquan and Min, Changjun and Dou, Xiujie and Wang, Xianyou and Urbach, Hendrik Paul and Somekh, Michael G and Yuan, Xiaocong},
  journal={Light Sci. Appl.},
  volume={10},
  number={1},
  pages={59},
  year={2021},
  publisher={Nature Publishing Group UK London}
}

@article{dreher2023focused,
  title={Focused surface plasmon polaritons coherently couple to electronic states in above-threshold electron emission},
  author={Dreher, Pascal and Janoschka, David and Frank, Bettina and Giessen, Harald and Meyer zu Heringdorf, Frank-J},
  journal={Communications Physics},
  volume={6},
  number={1},
  pages={15},
  year={2023},
  publisher={Nature Publishing Group UK London}
}

@article{liu2005focusing,
  title={Focusing surface plasmons with a plasmonic lens},
  author={Liu, Zhaowei and Steele, Jennifer M and Srituravanich, Werayut and Pikus, Yuri and Sun, Cheng and Zhang, Xiang},
  journal={Nano Lett.},
  volume={5},
  number={9},
  pages={1726--1729},
  year={2005},
  publisher={ACS Publications}
}

@article{min2013focused,
  title={Focused plasmonic trapping of metallic particles},
  author={Min, Changjun and Shen, Zhe and Shen, Junfeng and Zhang, Yuquan and Fang, Hui and Yuan, Guanghui and Du, Luping and Zhu, Siwei and Lei, Ting and Yuan, Xiaocong},
  journal={Nat. Communications},
  volume={4},
  number={1},
  pages={2891},
  year={2013},
  publisher={Nature Publishing Group UK London}
}


@article{Klein:OptLett:2012,
	author = {Angela E. Klein and Alexander Minovich and Michael Steinert and Norik Janunts and Andreas T\"{u}nnermann and Dragomir N. Neshev and Yuri S. Kivshar and Thomas Pertsch},
	journal = {Opt. Lett.},
	keywords = {Diffraction; Surface plasmons; Propagation; {Airy}  beams; Destructive interference; Optical data storage; Optical sensing; Optical tweezers; Surface plasmons},
	number = {16},
	pages = {3402--3404},
	publisher = {Optica Publishing Group},
	title = {Controlling plasmonic hot spots by interfering {Airy}  beams},
	volume = {37},
	month = {Aug},
	year = {2012},
	url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-37-16-3402},
	doi = {10.1364/OL.37.003402},
}

@article{lin:PRL:2012,
	title = {Cosine-Gauss Plasmon Beam: A Localized Long-Range Nondiffracting Surface Wave},
	author = {Lin, Jiao and Dellinger, Jean and Genevet, Patrice and Cluzel, Benoit and de Fornel, Frederique and Capasso, Federico},
	journal = {Phys. Rev. Lett.},
	volume = {109},
	issue = {9},
	pages = {093904},
	numpages = {5},
	year = {2012},
	month = {Aug},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.109.093904},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.109.093904}
}

@article{fang:LSA:2015,
	title = {Nanoplasmonic waveguides: towards applications in integrated nanophotonic circuits},
	author = {Fang, Yurui and Sun, Mengtao},
	journal = {Light Sci. Appl.},
	volume = {4},
	issue = {6},
	pages = {e294},
	numpages = {5},
	year = {2015},
	doi = {10.1038/lsa.2015.67},
	url = {https://doi.org/10.1038/lsa.2015.67}
}

